Verification of Bitcoin Script in Agda using Weakest Preconditions for Access Control

This paper contributes to the verification of programs written in Bitcoin's smart contract language SCRIPT in the interactive theorem prover Agda. It focuses on the security property of access control for SCRIPT programs that govern the distribution of Bitcoins. It advocates that weakest preconditions in the context of Hoare triples are the appropriate notion for verifying access control. It aims at obtaining human-readable descriptions of weakest preconditions in order to close the validation gap between user requirements and formal specification of smart contracts. As examples for the proposed approach, the paper focuses on two standard SCRIPT programs that govern the distribution of Bitcoins, Pay to Public Key Hash (P2PKH) and Pay to Multisig (P2MS). The paper introduces an operational semantics of the SCRIPT commands used in P2PKH and P2MS, which is formalised in the Agda proof assistant and reasoned about using Hoare triples. Two methodologies for obtaining human-readable descriptions of weakest preconditions are discussed: (1) a step-by-step approach, which works backwards instruction by instruction through a script, sometimes grouping several instructions together; (2) symbolic execution of the code and translation into a nested case distinction, which allows to read off weakest preconditions as the disjunction of conjunctions of conditions along accepting paths. A syntax for equational reasoning with Hoare Triples is defined in order to formalise those approaches in Agda. Keywords and phrases: Blockchain; Cryptocurrency; Bitcoin; Agda; Verification; Hoare logic; Bitcoin script; P2PKH; P2MS; Access control; Weakest precondition; Predicate transformer semantics; Provable correctness; Symbolic execution; Smart contracts

==> ProofofCorrectnessusingStepbyStepApproach.tex <==
OMITTED 


==> introBitcoinScriptbackup.tex <==
The script run on each Bitcoin node, is an embedded programming language, and is responsible for processing transactions~\cite{brakmic}. The scripting language for Bitcoin is stack-based. A stack is a group of things that is sorted linearly from the top down. This limitation is sometimes called LIFO (last in, first out), as all permitted operations must begin with the top element. The Bitcoin script makes use of this structure to organise and execute transaction-related instructions. Turing-completeness is not achieved for Bitcoin \Script; for example, it cannot execute loops, jumps, or complicated control structures to simplify and secure the transaction verification process~\cite{bistarelli,brakmic}. Every transaction in bitcoin contains a script, and it must return a Boolean True to be accepted as valid. To reach this value, one must solve all the puzzles and provide all the required data by opening scripts. In addition, a script has its own set of commands called Operation Code (Op$\_$Codes). Each operation performed by a script is assigned a specific number, which allows them to be rapidly and simply interpreted by Bitcoin nodes when reading serialised scripts from the blockchain. The OP$\_$Codes are classified into the following categories: ``cryptographic functions, stack functions, flow control, bitwise operation, pseudo-words, and arithmetic instructions''~\cite{brakmic}. Regardless of these categories, each OP$\_$Code begins with OP, such as OP$\_$HASH160, OP$\_$ ADD, OP$\_$ EQUAL and OP$\_$VERIFY. Many standard scripts are used in Bitcoin, but the most common are the pay-to-public-key-hash (P2PKH) script and the pay-to-script-hash (P2SH) script~\cite{wang1hash}. P2PKH~\cite{wang1hash} has an input script referred to as scriptSig and an output called scriptPublicKey. 
\begin{itemize}
\item For clarity, it is useful here to set out the OP$\_$Codes for both the scriptPublicKey and the scriptSig. The codes for the latter are as follows:
\begin{center} $<$sig$>$ $<$pubKey$>$ \end{center}
where sig is abbreviation for signature and pubKey stands for public key.\newline
\item The OP$\_$Codes for the scriptPublicKey are as follows:
\begin{center} OP$\_$DUP OP$\_$HASH160 $<$PublicKeyHash$>$ OP$\_$EQUALVERIFY OP$\_$CHECKSIG \end{center}
\end{itemize}
P2SH ~\cite{wang1hash} enables the sender to dispatch the transaction and deliver it to a single script hash. As a result, the sender does not need to input several public keys in transactions requiring multiple signatures. The instruction for P2SH script is as follows:
\begin{itemize}
\item signatureScript: $<$signature$>$ [signature] [signature . . .] $<$redScript$>$ 
\item publickeyScript: OP$\_$HASH160 $<$redScriptHash$>$ OP $\_$EQUAL
\end{itemize}
where redScript is a script for redeeming. Through redScript, the receiver acquires the right to utilise the asset redScriptHash, which is the hashing of the redeem script.\newline
When more than one signature is utilised, the redScript is as follows:
\begin{itemize}
\item signatureScript: $<$signature$>$ $<$PublicKey$>$ 
\item PubKeyscript: OP$\_$DUP OP$\_$HASH160 $<$PublicKeyHash$>$ OP$\_$EQUALVERIFY OP$\_$CHECKSIG
\end{itemize}













here we should describe
\begin{itemize} 
\item Architecture of the stack of the stack machine of bitcoin (having a stack, instructions, executed in 
sequence)
\item if then elses (discussed in a follow up paper)
\item a note that there is second stack as well, which is not treated in our paper, but could be added by
expanding the state 
\item A few examples of Bitcoin instructions such as   OP\_PUSH, OP\_DUP, and maybe some more complex ones.
\item Locking and unlocking of transaction:
\begin{itemize} 
\item A transaction can have multiple inputs and outputs.
\item Each input has a locking script (called sriptPubKey).
\item Each output has a unlocking script (called script sig).
\item We execute unlocking script. And then the resultint stack is passed on and the locking script is executed.
\begin{itemize} 
\item its not just the concatenation, otherwise the unlocking script could have an open OP\_IF which 
crates some unexepected behaviour in the locking script. 
\end{itemize} 
\end{itemize} 
\end{itemize} 


==> latex-before-sed/paperTypes2021PostProceed/demoEqualityReasoning.tex <==
%% This file has been generated automatically by mkLagda.awk
%% DO NOT EDIT! ALL YOUR CHANGES WILL BE LOST!

\AgdaHide{
\begin{code}%
\>[0]\<%
\\
\>[0]\AgdaKeyword{open}\AgdaSpace{}%
\AgdaKeyword{import}\AgdaSpace{}%
\AgdaModule{basicBitcoinDataType}\<%
\\
\>[0]\AgdaKeyword{module}\AgdaSpace{}%
\AgdaModule{paperTypes2021PostProceed.demoEqualityReasoning}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaBound{param}\AgdaSpace{}%
\AgdaSymbol{:}\AgdaSpace{}%
\AgdaRecord{GlobalParameters}\AgdaSymbol{)}\AgdaSpace{}%
\AgdaKeyword{where}\<%
\\
%
\\[\AgdaEmptyExtraSkip]%
\>[0]\AgdaKeyword{open}\AgdaSpace{}%
\AgdaKeyword{import}\AgdaSpace{}%
\AgdaModule{Data.List.Base}\AgdaSpace{}%
\AgdaKeyword{hiding}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaOperator{\AgdaFunction{\AgdaUnderscore{}++\AgdaUnderscore{}}}\AgdaSpace{}%
\AgdaSymbol{)}\<%
\\
\>[0]\AgdaKeyword{open}\AgdaSpace{}%
\AgdaKeyword{import}\AgdaSpace{}%
\AgdaModule{Data.Nat}%
\>[22]\AgdaKeyword{renaming}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaOperator{\AgdaDatatype{\AgdaUnderscore{}≤\AgdaUnderscore{}}}\AgdaSpace{}%
\AgdaSymbol{to}\AgdaSpace{}%
\AgdaOperator{\AgdaDatatype{\AgdaUnderscore{}≤'\AgdaUnderscore{}}}\AgdaSpace{}%
\AgdaSymbol{;}\AgdaSpace{}%
\AgdaOperator{\AgdaFunction{\AgdaUnderscore{}<\AgdaUnderscore{}}}\AgdaSpace{}%
\AgdaSymbol{to}\AgdaSpace{}%
\AgdaOperator{\AgdaFunction{\AgdaUnderscore{}<'\AgdaUnderscore{}}}\AgdaSymbol{)}\<%
\\
\>[0]\AgdaKeyword{open}\AgdaSpace{}%
\AgdaKeyword{import}\AgdaSpace{}%
\AgdaModule{Data.List}\AgdaSpace{}%
\AgdaKeyword{hiding}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaOperator{\AgdaFunction{\AgdaUnderscore{}++\AgdaUnderscore{}}}%
\>[36]\AgdaSymbol{)}\<%
\\
\>[0]\AgdaKeyword{open}\AgdaSpace{}%
\AgdaKeyword{import}\AgdaSpace{}%
\AgdaModule{Data.Sum}\<%
\\
\>[0]\AgdaKeyword{open}\AgdaSpace{}%
\AgdaKeyword{import}\AgdaSpace{}%
\AgdaModule{Data.Unit}%
\>[23]\AgdaKeyword{hiding}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaOperator{\AgdaRecord{\AgdaUnderscore{}≤\AgdaUnderscore{}}}\AgdaSymbol{)}\<%
\\
\>[0]\AgdaKeyword{open}\AgdaSpace{}%
\AgdaKeyword{import}\AgdaSpace{}%
\AgdaModule{Data.Empty}\<%
\\
\>[0]\AgdaKeyword{open}\AgdaSpace{}%
\AgdaKeyword{import}\AgdaSpace{}%
\AgdaModule{Data.Maybe}\<%
\\
\>[0]\AgdaKeyword{open}\AgdaSpace{}%
\AgdaKeyword{import}\AgdaSpace{}%
\AgdaModule{Data.Bool}%
\>[23]\AgdaKeyword{hiding}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaOperator{\AgdaDatatype{\AgdaUnderscore{}≤\AgdaUnderscore{}}}\AgdaSpace{}%
\AgdaSymbol{;}\AgdaSpace{}%
\AgdaOperator{\AgdaDatatype{\AgdaUnderscore{}<\AgdaUnderscore{}}}\AgdaSpace{}%
\AgdaSymbol{;}\AgdaSpace{}%
\AgdaOperator{\AgdaFunction{if\AgdaUnderscore{}then\AgdaUnderscore{}else\AgdaUnderscore{}}}%
\>[58]\AgdaSymbol{)}%
\>[61]\AgdaKeyword{renaming}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaOperator{\AgdaFunction{\AgdaUnderscore{}∧\AgdaUnderscore{}}}\AgdaSpace{}%
\AgdaSymbol{to}\AgdaSpace{}%
\AgdaOperator{\AgdaFunction{\AgdaUnderscore{}∧b\AgdaUnderscore{}}}\AgdaSpace{}%
\AgdaSymbol{;}\AgdaSpace{}%
\AgdaOperator{\AgdaFunction{\AgdaUnderscore{}∨\AgdaUnderscore{}}}\AgdaSpace{}%
\AgdaSymbol{to}\AgdaSpace{}%
\AgdaOperator{\AgdaFunction{\AgdaUnderscore{}∨b\AgdaUnderscore{}}}\AgdaSpace{}%
\AgdaSymbol{;}\AgdaSpace{}%
\AgdaFunction{T}\AgdaSpace{}%
\AgdaSymbol{to}\AgdaSpace{}%
\AgdaFunction{True}\AgdaSymbol{)}\<%
\\
\>[0]\AgdaKeyword{open}\AgdaSpace{}%
\AgdaKeyword{import}\AgdaSpace{}%
\AgdaModule{Data.Product}\AgdaSpace{}%
\AgdaKeyword{renaming}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaOperator{\AgdaInductiveConstructor{\AgdaUnderscore{},\AgdaUnderscore{}}}\AgdaSpace{}%
\AgdaSymbol{to}\AgdaSpace{}%
\AgdaOperator{\AgdaInductiveConstructor{\AgdaUnderscore{},,\AgdaUnderscore{}}}\AgdaSpace{}%
\AgdaSymbol{)}\<%
\\
\>[0]\AgdaKeyword{open}\AgdaSpace{}%
\AgdaKeyword{import}\AgdaSpace{}%
\AgdaModule{Data.Nat.Base}\AgdaSpace{}%
\AgdaKeyword{hiding}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaOperator{\AgdaDatatype{\AgdaUnderscore{}≤\AgdaUnderscore{}}}\AgdaSpace{}%
\AgdaSymbol{;}\AgdaSpace{}%
\AgdaOperator{\AgdaFunction{\AgdaUnderscore{}<\AgdaUnderscore{}}}\AgdaSymbol{)}\<%
\\
\>[0]\AgdaKeyword{open}\AgdaSpace{}%
\AgdaKeyword{import}\AgdaSpace{}%
\AgdaModule{Data.List.NonEmpty}\AgdaSpace{}%
\AgdaKeyword{hiding}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaField{head}\AgdaSymbol{;}\AgdaSpace{}%
\AgdaOperator{\AgdaFunction{[\AgdaUnderscore{}]}}\AgdaSymbol{)}\<%
\\
\>[0]\AgdaKeyword{open}\AgdaSpace{}%
\AgdaKeyword{import}\AgdaSpace{}%
\AgdaModule{Data.Nat}\AgdaSpace{}%
\AgdaKeyword{using}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaDatatype{ℕ}\AgdaSymbol{;}\AgdaSpace{}%
\AgdaOperator{\AgdaPrimitive{\AgdaUnderscore{}+\AgdaUnderscore{}}}\AgdaSymbol{;}\AgdaSpace{}%
\AgdaOperator{\AgdaFunction{\AgdaUnderscore{}≥\AgdaUnderscore{}}}\AgdaSymbol{;}\AgdaSpace{}%
\AgdaOperator{\AgdaFunction{\AgdaUnderscore{}>\AgdaUnderscore{}}}\AgdaSymbol{;}\AgdaSpace{}%
\AgdaInductiveConstructor{zero}\AgdaSymbol{;}\AgdaSpace{}%
\AgdaInductiveConstructor{suc}\AgdaSymbol{;}\AgdaSpace{}%
\AgdaInductiveConstructor{s≤s}\AgdaSymbol{;}\AgdaSpace{}%
\AgdaInductiveConstructor{z≤n}\AgdaSymbol{)}\<%
\\
\>[0]\AgdaKeyword{import}\AgdaSpace{}%
\AgdaModule{Relation.Binary.PropositionalEquality}\AgdaSpace{}%
\AgdaSymbol{as}\AgdaSpace{}%
\AgdaModule{Eq}\<%
\\
\>[0]\AgdaKeyword{open}\AgdaSpace{}%
\AgdaModule{Eq}\AgdaSpace{}%
\AgdaKeyword{using}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaOperator{\AgdaDatatype{\AgdaUnderscore{}≡\AgdaUnderscore{}}}\AgdaSymbol{;}\AgdaSpace{}%
\AgdaInductiveConstructor{refl}\AgdaSymbol{;}\AgdaSpace{}%
\AgdaFunction{cong}\AgdaSymbol{;}\AgdaSpace{}%
\AgdaKeyword{module}\AgdaSpace{}%
\AgdaModule{≡-Reasoning}\AgdaSymbol{;}\AgdaSpace{}%
\AgdaFunction{sym}\AgdaSymbol{)}\<%
\\
\>[0]\AgdaKeyword{open}\AgdaSpace{}%
\AgdaModule{≡-Reasoning}\<%
\\
\>[0]\AgdaKeyword{open}\AgdaSpace{}%
\AgdaKeyword{import}\AgdaSpace{}%
\AgdaModule{Agda.Builtin.Equality}\<%
\\
%
\\[\AgdaEmptyExtraSkip]%
%
\\[\AgdaEmptyExtraSkip]%
\>[0]\AgdaComment{--our\ libraries}\<%
\\
\>[0]\AgdaKeyword{open}\AgdaSpace{}%
\AgdaKeyword{import}\AgdaSpace{}%
\AgdaModule{libraries.listLib}\<%
\\
\>[0]\AgdaKeyword{open}\AgdaSpace{}%
\AgdaKeyword{import}\AgdaSpace{}%
\AgdaModule{libraries.emptyLib}\<%
\\
\>[0]\AgdaKeyword{open}\AgdaSpace{}%
\AgdaKeyword{import}\AgdaSpace{}%
\AgdaModule{libraries.natLib}\<%
\\
\>[0]\AgdaKeyword{open}\AgdaSpace{}%
\AgdaKeyword{import}\AgdaSpace{}%
\AgdaModule{libraries.boolLib}\<%
\\
\>[0]\AgdaKeyword{open}\AgdaSpace{}%
\AgdaKeyword{import}\AgdaSpace{}%
\AgdaModule{libraries.equalityLib}\<%
\\
\>[0]\AgdaKeyword{open}\AgdaSpace{}%
\AgdaKeyword{import}\AgdaSpace{}%
\AgdaModule{libraries.andLib}\<%
\\
\>[0]\AgdaKeyword{open}\AgdaSpace{}%
\AgdaKeyword{import}\AgdaSpace{}%
\AgdaModule{libraries.miscLib}\<%
\\
\>[0]\AgdaKeyword{open}\AgdaSpace{}%
\AgdaKeyword{import}\AgdaSpace{}%
\AgdaModule{libraries.maybeLib}\<%
\\
\>[0]\AgdaKeyword{open}\AgdaSpace{}%
\AgdaKeyword{import}\AgdaSpace{}%
\AgdaModule{stack}\<%
\\
\>[0]\AgdaKeyword{open}\AgdaSpace{}%
\AgdaKeyword{import}\AgdaSpace{}%
\AgdaModule{stackPredicate}\<%
\\
\>[0]\AgdaKeyword{open}\AgdaSpace{}%
\AgdaKeyword{import}\AgdaSpace{}%
\AgdaModule{semanticBasicOperations}\AgdaSpace{}%
\AgdaBound{param}\<%
\\
\>[0]\AgdaKeyword{open}\AgdaSpace{}%
\AgdaKeyword{import}\AgdaSpace{}%
\AgdaModule{instructionBasic}\<%
\\
\>[0]\AgdaKeyword{open}\AgdaSpace{}%
\AgdaKeyword{import}\AgdaSpace{}%
\AgdaModule{verificationMultiSig}\AgdaSpace{}%
\AgdaBound{param}\<%
\\
\>[0]\AgdaKeyword{open}\AgdaSpace{}%
\AgdaKeyword{import}\AgdaSpace{}%
\AgdaModule{verificationStackScripts.semanticsStackInstructions}\AgdaSpace{}%
\AgdaBound{param}\<%
\\
\>[0]\AgdaKeyword{open}\AgdaSpace{}%
\AgdaKeyword{import}\AgdaSpace{}%
\AgdaModule{verificationStackScripts.stackVerificationLemmas}\AgdaSpace{}%
\AgdaBound{param}\<%
\\
\>[0]\AgdaKeyword{open}\AgdaSpace{}%
\AgdaKeyword{import}\AgdaSpace{}%
\AgdaModule{verificationStackScripts.stackHoareTriple}\AgdaSpace{}%
\AgdaBound{param}\<%
\\
\>[0]\AgdaKeyword{open}\AgdaSpace{}%
\AgdaKeyword{import}\AgdaSpace{}%
\AgdaModule{verificationStackScripts.sPredicate}\<%
\\
\>[0]\AgdaKeyword{open}\AgdaSpace{}%
\AgdaKeyword{import}\AgdaSpace{}%
\AgdaModule{verificationStackScripts.hoareTripleStackBasic}\AgdaSpace{}%
\AgdaBound{param}\<%
\\
\>[0]\AgdaKeyword{open}\AgdaSpace{}%
\AgdaKeyword{import}\AgdaSpace{}%
\AgdaModule{verificationStackScripts.stackState}\<%
\\
\>[0]\AgdaKeyword{open}\AgdaSpace{}%
\AgdaKeyword{import}\AgdaSpace{}%
\AgdaModule{verificationStackScripts.stackSemanticsInstructionsBasic}\AgdaSpace{}%
\AgdaBound{param}\<%
\\
\>[0]\AgdaKeyword{open}\AgdaSpace{}%
\AgdaKeyword{import}\AgdaSpace{}%
\AgdaModule{verificationStackScripts.verificationMultiSigBasic}\AgdaSpace{}%
\AgdaBound{param}\<%
\\
%
\\[\AgdaEmptyExtraSkip]%
%
\\[\AgdaEmptyExtraSkip]%
\>[0]\AgdaComment{--\ postulate\ time₁\ :\ Time}\<%
\\
\>[0]\AgdaComment{--\ postulate\ pbk1\ pbk2\ pbk3\ pbk4\ :\ ℕ}\<%
\\
%
\\[\AgdaEmptyExtraSkip]%
\>[0]\AgdaKeyword{postulate}\<%
\end{code}
} % END AgdaHide

\newcommand{\demoEqualityReasoningprecondition}{
\begin{code}%
\>[0][@{}l@{\AgdaIndent{1}}]%
\>[2]\AgdaPostulate{precondition}\AgdaSpace{}%
\AgdaSymbol{:}\AgdaSpace{}%
\AgdaFunction{StackStatePred}\<%
\end{code}
} % END newcommand

\AgdaHide{
\begin{code}%
\>[0]\<%
\end{code}
} % END AgdaHide

\newcommand{\demoEqualityReasoningpostcondition}{
\begin{code}%
\>[0][@{}l@{\AgdaIndent{1}}]%
\>[2]\AgdaPostulate{postcondition}\AgdaSpace{}%
\AgdaSymbol{:}\AgdaSpace{}%
\AgdaFunction{StackStatePred}\<%
\end{code}
} % END newcommand

\AgdaHide{
\begin{code}%
\>[0]\<%
\end{code}
} % END AgdaHide

\newcommand{\demoEqualityReasoningfsintermediateCond}{
\begin{code}%
\>[0][@{}l@{\AgdaIndent{1}}]%
\>[2]\AgdaPostulate{intermediateCond1}\AgdaSpace{}%
\AgdaSymbol{:}\AgdaSpace{}%
\AgdaFunction{StackStatePred}\<%
\end{code}
} % END newcommand

\AgdaHide{
\begin{code}%
\>[0]\<%
\end{code}
} % END AgdaHide

\newcommand{\demoEqualityReasoningseintermediateCond}{
\begin{code}%
\>[0][@{}l@{\AgdaIndent{1}}]%
\>[2]\AgdaPostulate{intermediateCond2}\AgdaSpace{}%
\AgdaSymbol{:}\AgdaSpace{}%
\AgdaFunction{StackStatePred}\<%
\end{code}
} % END newcommand

\AgdaHide{
\begin{code}%
\>[0]\<%
\end{code}
} % END AgdaHide

\newcommand{\demoEqualityReasoningtrintermediateCond}{
\begin{code}%
\>[0][@{}l@{\AgdaIndent{1}}]%
\>[2]\AgdaPostulate{intermediateCond3}\AgdaSpace{}%
\AgdaSymbol{:}\AgdaSpace{}%
\AgdaFunction{StackStatePred}\<%
\end{code}
} % END newcommand

\AgdaHide{
\begin{code}%
\>[0]\<%
\end{code}
} % END AgdaHide

\newcommand{\demoEqualityReasoningprogone}{
\begin{code}%
\>[0][@{}l@{\AgdaIndent{1}}]%
\>[2]\AgdaPostulate{prog1}\AgdaSpace{}%
\AgdaSymbol{:}\AgdaSpace{}%
\AgdaFunction{BitcoinScriptBasic}\<%
\end{code}
} % END AgdaHide

\newcommand{\demoEqualityReasoningprogtwo}{
\begin{code}%
%
\>[2]\AgdaPostulate{prog2}\AgdaSpace{}%
\AgdaPostulate{prog3}\AgdaSpace{}%
\AgdaSymbol{:}\AgdaSpace{}%
\AgdaFunction{BitcoinScriptBasic}\<%
\end{code}
} % END newcommand

\AgdaHide{
\begin{code}%
\>[0]\<%
\\
\>[0]\<%
\end{code}
} % END AgdaHide

\newcommand{\demoEqualityReasoningproofs}{
\begin{code}%
\>[0][@{}l@{\AgdaIndent{1}}]%
\>[2]\AgdaPostulate{proof1}\AgdaSpace{}%
\AgdaSymbol{:}\AgdaSpace{}%
\AgdaOperator{\AgdaRecord{<}}\AgdaSpace{}%
\AgdaPostulate{precondition}\AgdaSpace{}%
\AgdaOperator{\AgdaRecord{>ⁱᶠᶠ}}\AgdaSpace{}%
\AgdaPostulate{prog1}%
\>[38]\AgdaOperator{\AgdaRecord{<}}\AgdaSpace{}%
\AgdaPostulate{intermediateCond1}\AgdaSpace{}%
\AgdaOperator{\AgdaRecord{>}}\<%
\\
%
\>[2]\AgdaPostulate{proof2}\AgdaSpace{}%
\AgdaSymbol{:}\AgdaSpace{}%
\AgdaOperator{\AgdaRecord{<}}\AgdaSpace{}%
\AgdaPostulate{intermediateCond1}\AgdaSpace{}%
\AgdaOperator{\AgdaRecord{>ⁱᶠᶠ}}\AgdaSpace{}%
\AgdaPostulate{prog2}\AgdaSpace{}%
\AgdaOperator{\AgdaRecord{<}}\AgdaSpace{}%
\AgdaPostulate{intermediateCond2}\AgdaSpace{}%
\AgdaOperator{\AgdaRecord{>}}\<%
\\
%
\>[2]\AgdaPostulate{proof3}\AgdaSpace{}%
\AgdaSymbol{:}\AgdaSpace{}%
\AgdaPostulate{intermediateCond2}\AgdaSpace{}%
\AgdaOperator{\AgdaRecord{<=>ᵖ}}\AgdaSpace{}%
\AgdaPostulate{intermediateCond3}\<%
\\
%
\>[2]\AgdaPostulate{proof4}\AgdaSpace{}%
\AgdaSymbol{:}\AgdaSpace{}%
\AgdaOperator{\AgdaRecord{<}}\AgdaSpace{}%
\AgdaPostulate{intermediateCond3}\AgdaSpace{}%
\AgdaOperator{\AgdaRecord{>ⁱᶠᶠ}}\AgdaSpace{}%
\AgdaPostulate{prog3}\AgdaSpace{}%
\AgdaOperator{\AgdaRecord{<}}\AgdaSpace{}%
\AgdaPostulate{postcondition}\AgdaSpace{}%
\AgdaOperator{\AgdaRecord{>}}\<%
\end{code}
} % END newcommand

\AgdaHide{
\begin{code}%
\>[0]\<%
\end{code}
} % END AgdaHide

\newcommand{\demoEqualityReasoninglemma}{
\begin{code}%
\>[0]\AgdaFunction{theorem}\AgdaSpace{}%
\AgdaSymbol{:}\AgdaSpace{}%
\AgdaOperator{\AgdaRecord{<}}\AgdaSpace{}%
\AgdaPostulate{precondition}\AgdaSpace{}%
\AgdaOperator{\AgdaRecord{>ⁱᶠᶠ}}\AgdaSpace{}%
\AgdaPostulate{prog1}\AgdaSpace{}%
\AgdaOperator{\AgdaFunction{++}}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaPostulate{prog2}\AgdaSpace{}%
\AgdaOperator{\AgdaFunction{++}}\AgdaSpace{}%
\AgdaPostulate{prog3}\AgdaSymbol{)}%
\>[57]\AgdaOperator{\AgdaRecord{<}}%
\>[60]\AgdaPostulate{postcondition}\AgdaSpace{}%
\AgdaOperator{\AgdaRecord{>}}\<%
\\
\>[0]\AgdaFunction{theorem}\AgdaSpace{}%
\AgdaSymbol{=}%
\>[11]\AgdaPostulate{precondition}%
\>[30]\AgdaFunction{<><>⟨}%
\>[37]\AgdaPostulate{prog1}%
\>[45]\AgdaFunction{⟩⟨}%
\>[49]\AgdaPostulate{proof1}%
\>[57]\AgdaFunction{⟩}\<%
\\
%
\>[11]\AgdaPostulate{intermediateCond1}%
\>[30]\AgdaFunction{<><>⟨}%
\>[37]\AgdaPostulate{prog2}%
\>[45]\AgdaFunction{⟩⟨}%
\>[49]\AgdaPostulate{proof2}%
\>[57]\AgdaFunction{⟩}\<%
\\
%
\>[11]\AgdaPostulate{intermediateCond2}%
\>[30]\AgdaFunction{<=>⟨}%
\>[37]\AgdaPostulate{proof3}%
\>[45]\AgdaFunction{⟩}\<%
\\
%
\>[11]\AgdaPostulate{intermediateCond3}%
\>[30]\AgdaFunction{<><>⟨}%
\>[37]\AgdaPostulate{prog3}%
\>[45]\AgdaFunction{⟩⟨}%
\>[49]\AgdaPostulate{proof4}%
\>[57]\AgdaFunction{⟩ᵉ}%
\>[62]\AgdaPostulate{postcondition}%
\>[77]\AgdaOperator{\AgdaFunction{∎p}}\<%
\end{code}
} % END newcommand

\AgdaHide{
\begin{code}%
\>[0]\<%
\end{code}
} % END AgdaHide


==> latex-before-sed/paperTypes2021PostProceed/maybeDef.tex <==
%% This file has been generated automatically by mkLagda.awk
%% DO NOT EDIT! ALL YOUR CHANGES WILL BE LOST!

\AgdaHide{
\begin{code}%
\>[0]\AgdaKeyword{module}\AgdaSpace{}%
\AgdaModule{paperTypes2021PostProceed.maybeDef}\AgdaSpace{}%
\AgdaKeyword{where}\<%
\\
%
\\[\AgdaEmptyExtraSkip]%
\>[0]\<%
\end{code}
} % END AgdaHide

\newcommand{\maybeDefMaybe}{
\begin{code}%
\>[0]\AgdaKeyword{data}\AgdaSpace{}%
\AgdaDatatype{Maybe}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaBound{X}\AgdaSpace{}%
\AgdaSymbol{:}\AgdaSpace{}%
\AgdaPrimitive{Set}\AgdaSymbol{)}\AgdaSpace{}%
\AgdaSymbol{:}\AgdaSpace{}%
\AgdaPrimitive{Set}\AgdaSpace{}%
\AgdaKeyword{where}%
\>[34]\AgdaInductiveConstructor{nothing}\AgdaSpace{}%
\AgdaSymbol{:}%
\>[45]\AgdaDatatype{Maybe}\AgdaSpace{}%
\AgdaBound{X}\AgdaSymbol{;}\AgdaSpace{}%
\AgdaInductiveConstructor{just}%
\>[62]\AgdaSymbol{:}%
\>[65]\AgdaBound{X}\AgdaSpace{}%
\AgdaSymbol{→}\AgdaSpace{}%
\AgdaDatatype{Maybe}\AgdaSpace{}%
\AgdaBound{X}\<%
\end{code}
} % END newcommand

\AgdaHide{
\begin{code}%
\>[0]\<%
\\
%
\\[\AgdaEmptyExtraSkip]%
\>[0]\AgdaFunction{return}\AgdaSpace{}%
\AgdaSymbol{:}\AgdaSpace{}%
\AgdaSymbol{\{}\AgdaBound{A}\AgdaSpace{}%
\AgdaSymbol{:}\AgdaSpace{}%
\AgdaPrimitive{Set}\AgdaSymbol{\}}\AgdaSpace{}%
\AgdaSymbol{→}\AgdaSpace{}%
\AgdaBound{A}\AgdaSpace{}%
\AgdaSymbol{→}\AgdaSpace{}%
\AgdaDatatype{Maybe}\AgdaSpace{}%
\AgdaBound{A}\<%
\\
\>[0]\AgdaFunction{return}\AgdaSpace{}%
\AgdaSymbol{=}\AgdaSpace{}%
\AgdaInductiveConstructor{just}\<%
\\
%
\\[\AgdaEmptyExtraSkip]%
%
\\[\AgdaEmptyExtraSkip]%
\>[0]\AgdaOperator{\AgdaFunction{\AgdaUnderscore{}>>=\AgdaUnderscore{}}}\AgdaSpace{}%
\AgdaSymbol{:}\AgdaSpace{}%
\AgdaSymbol{\{}\AgdaBound{A}\AgdaSpace{}%
\AgdaBound{B}\AgdaSpace{}%
\AgdaSymbol{:}\AgdaSpace{}%
\AgdaPrimitive{Set}\AgdaSymbol{\}}\AgdaSpace{}%
\AgdaSymbol{→}\AgdaSpace{}%
\AgdaDatatype{Maybe}\AgdaSpace{}%
\AgdaBound{A}\AgdaSpace{}%
\AgdaSymbol{→}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaBound{A}\AgdaSpace{}%
\AgdaSymbol{→}\AgdaSpace{}%
\AgdaDatatype{Maybe}\AgdaSpace{}%
\AgdaBound{B}\AgdaSymbol{)}\AgdaSpace{}%
\AgdaSymbol{→}\AgdaSpace{}%
\AgdaDatatype{Maybe}\AgdaSpace{}%
\AgdaBound{B}\<%
\\
\>[0]\AgdaInductiveConstructor{nothing}\AgdaSpace{}%
\AgdaOperator{\AgdaFunction{>>=}}\AgdaSpace{}%
\AgdaBound{q}\AgdaSpace{}%
\AgdaSymbol{=}\AgdaSpace{}%
\AgdaInductiveConstructor{nothing}\<%
\\
\>[0]\AgdaInductiveConstructor{just}\AgdaSpace{}%
\AgdaBound{x}\AgdaSpace{}%
\AgdaOperator{\AgdaFunction{>>=}}\AgdaSpace{}%
\AgdaBound{q}\AgdaSpace{}%
\AgdaSymbol{=}\AgdaSpace{}%
\AgdaBound{q}\AgdaSpace{}%
\AgdaBound{x}\<%
\end{code}
} % END AgdaHide


==> latex-before-sed/paperTypes2021PostProceed/semanticBasicOperationsForTypeSetting.tex <==
%% This file has been generated automatically by mkLagda.awk
%% DO NOT EDIT! ALL YOUR CHANGES WILL BE LOST!

\AgdaHide{
\begin{code}%
\>[0]\AgdaComment{--\textbackslash{}semanticBasicOperationsForTypeSetting}\<%
\\
\>[0]\AgdaKeyword{open}\AgdaSpace{}%
\AgdaKeyword{import}\AgdaSpace{}%
\AgdaModule{basicBitcoinDataType}\<%
\\
%
\\[\AgdaEmptyExtraSkip]%
\>[0]\AgdaKeyword{module}\AgdaSpace{}%
\AgdaModule{paperTypes2021PostProceed.semanticBasicOperationsForTypeSetting}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaBound{param}\AgdaSpace{}%
\AgdaSymbol{:}\AgdaSpace{}%
\AgdaRecord{GlobalParameters}\AgdaSymbol{)}\AgdaSpace{}%
\AgdaKeyword{where}\<%
\\
%
\\[\AgdaEmptyExtraSkip]%
\>[0]\AgdaKeyword{open}\AgdaSpace{}%
\AgdaKeyword{import}\AgdaSpace{}%
\AgdaModule{Data.Nat}%
\>[22]\AgdaKeyword{hiding}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaOperator{\AgdaDatatype{\AgdaUnderscore{}≤\AgdaUnderscore{}}}\AgdaSymbol{)}\<%
\\
\>[0]\AgdaKeyword{open}\AgdaSpace{}%
\AgdaKeyword{import}\AgdaSpace{}%
\AgdaModule{Data.List}\AgdaSpace{}%
\AgdaKeyword{hiding}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaOperator{\AgdaFunction{\AgdaUnderscore{}++\AgdaUnderscore{}}}\AgdaSymbol{)}\<%
\\
\>[0]\AgdaKeyword{open}\AgdaSpace{}%
\AgdaKeyword{import}\AgdaSpace{}%
\AgdaModule{Data.Unit}%
\>[23]\AgdaKeyword{hiding}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaOperator{\AgdaRecord{\AgdaUnderscore{}≤\AgdaUnderscore{}}}\AgdaSymbol{)}\<%
\\
\>[0]\AgdaKeyword{open}\AgdaSpace{}%
\AgdaKeyword{import}\AgdaSpace{}%
\AgdaModule{Data.Empty}\<%
\\
\>[0]\AgdaKeyword{open}\AgdaSpace{}%
\AgdaKeyword{import}\AgdaSpace{}%
\AgdaModule{Data.Bool}%
\>[23]\AgdaKeyword{hiding}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaOperator{\AgdaDatatype{\AgdaUnderscore{}≤\AgdaUnderscore{}}}\AgdaSpace{}%
\AgdaSymbol{;}\AgdaSpace{}%
\AgdaOperator{\AgdaFunction{if\AgdaUnderscore{}then\AgdaUnderscore{}else\AgdaUnderscore{}}}\AgdaSpace{}%
\AgdaSymbol{)}\AgdaSpace{}%
\AgdaKeyword{renaming}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaOperator{\AgdaFunction{\AgdaUnderscore{}∧\AgdaUnderscore{}}}\AgdaSpace{}%
\AgdaSymbol{to}\AgdaSpace{}%
\AgdaOperator{\AgdaFunction{\AgdaUnderscore{}∧b\AgdaUnderscore{}}}\AgdaSpace{}%
\AgdaSymbol{;}\AgdaSpace{}%
\AgdaOperator{\AgdaFunction{\AgdaUnderscore{}∨\AgdaUnderscore{}}}\AgdaSpace{}%
\AgdaSymbol{to}\AgdaSpace{}%
\AgdaOperator{\AgdaFunction{\AgdaUnderscore{}∨b\AgdaUnderscore{}}}\AgdaSpace{}%
\AgdaSymbol{;}\AgdaSpace{}%
\AgdaFunction{T}\AgdaSpace{}%
\AgdaSymbol{to}\AgdaSpace{}%
\AgdaFunction{True}\AgdaSymbol{)}\<%
\\
\>[0]\AgdaKeyword{open}\AgdaSpace{}%
\AgdaKeyword{import}\AgdaSpace{}%
\AgdaModule{Data.Product}\AgdaSpace{}%
\AgdaKeyword{renaming}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaOperator{\AgdaInductiveConstructor{\AgdaUnderscore{},\AgdaUnderscore{}}}\AgdaSpace{}%
\AgdaSymbol{to}\AgdaSpace{}%
\AgdaOperator{\AgdaInductiveConstructor{\AgdaUnderscore{},,\AgdaUnderscore{}}}\AgdaSpace{}%
\AgdaSymbol{)}\<%
\\
\>[0]\AgdaKeyword{open}\AgdaSpace{}%
\AgdaKeyword{import}\AgdaSpace{}%
\AgdaModule{Data.Nat.Base}\AgdaSpace{}%
\AgdaKeyword{hiding}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaOperator{\AgdaDatatype{\AgdaUnderscore{}≤\AgdaUnderscore{}}}\AgdaSymbol{)}\<%
\\
\>[0]\AgdaComment{--\ open\ import\ Data.List.NonEmpty\ hiding\ (head)}\<%
\\
\>[0]\AgdaKeyword{open}\AgdaSpace{}%
\AgdaKeyword{import}\AgdaSpace{}%
\AgdaModule{Data.Maybe}\<%
\\
%
\\[\AgdaEmptyExtraSkip]%
\>[0]\AgdaKeyword{import}\AgdaSpace{}%
\AgdaModule{Relation.Binary.PropositionalEquality}\AgdaSpace{}%
\AgdaSymbol{as}\AgdaSpace{}%
\AgdaModule{Eq}\<%
\\
\>[0]\AgdaKeyword{open}\AgdaSpace{}%
\AgdaModule{Eq}\AgdaSpace{}%
\AgdaKeyword{using}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaOperator{\AgdaDatatype{\AgdaUnderscore{}≡\AgdaUnderscore{}}}\AgdaSymbol{;}\AgdaSpace{}%
\AgdaInductiveConstructor{refl}\AgdaSymbol{;}\AgdaSpace{}%
\AgdaFunction{cong}\AgdaSymbol{;}\AgdaSpace{}%
\AgdaKeyword{module}\AgdaSpace{}%
\AgdaModule{≡-Reasoning}\AgdaSymbol{;}\AgdaSpace{}%
\AgdaFunction{sym}\AgdaSymbol{)}\<%
\\
\>[0]\AgdaKeyword{open}\AgdaSpace{}%
\AgdaModule{≡-Reasoning}\<%
\\
\>[0]\AgdaKeyword{open}\AgdaSpace{}%
\AgdaKeyword{import}\AgdaSpace{}%
\AgdaModule{Agda.Builtin.Equality}\<%
\\
\>[0]\AgdaComment{--open\ import\ Agda.Builtin.Equality.Rewrite}\<%
\\
%
\\[\AgdaEmptyExtraSkip]%
%
\\[\AgdaEmptyExtraSkip]%
\>[0]\AgdaKeyword{open}\AgdaSpace{}%
\AgdaKeyword{import}\AgdaSpace{}%
\AgdaModule{libraries.listLib}\<%
\\
\>[0]\AgdaKeyword{open}\AgdaSpace{}%
\AgdaKeyword{import}\AgdaSpace{}%
\AgdaModule{libraries.natLib}\<%
\\
\>[0]\AgdaKeyword{open}\AgdaSpace{}%
\AgdaKeyword{import}\AgdaSpace{}%
\AgdaModule{libraries.boolLib}\<%
\\
\>[0]\AgdaKeyword{open}\AgdaSpace{}%
\AgdaKeyword{import}\AgdaSpace{}%
\AgdaModule{libraries.andLib}\<%
\\
\>[0]\AgdaKeyword{open}\AgdaSpace{}%
\AgdaKeyword{import}\AgdaSpace{}%
\AgdaModule{libraries.miscLib}\<%
\\
\>[0]\AgdaKeyword{open}\AgdaSpace{}%
\AgdaKeyword{import}\AgdaSpace{}%
\AgdaModule{libraries.maybeLib}\<%
\\
%
\\[\AgdaEmptyExtraSkip]%
\>[0]\AgdaKeyword{open}\AgdaSpace{}%
\AgdaKeyword{import}\AgdaSpace{}%
\AgdaModule{stack}\<%
\\
%
\\[\AgdaEmptyExtraSkip]%
\>[0]\AgdaKeyword{open}\AgdaSpace{}%
\AgdaKeyword{import}\AgdaSpace{}%
\AgdaModule{semanticBasicOperations}\AgdaSpace{}%
\AgdaBound{param}\AgdaSpace{}%
\AgdaKeyword{hiding}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaFunction{executeStackCheckSig3Aux}\AgdaSymbol{;}\AgdaFunction{compareSigsMultiSigAux}\AgdaSymbol{;}\AgdaFunction{compareSigsMultiSig}\AgdaSymbol{;}\AgdaFunction{executeMultiSig3}\AgdaSymbol{;}\AgdaFunction{executeMultiSig2}\AgdaSymbol{;}\AgdaFunction{executeMultiSig}\AgdaSymbol{)}\<%
\\
%
\\[\AgdaEmptyExtraSkip]%
\>[0]\AgdaFunction{executeStackCheckSig3Aux}\AgdaSpace{}%
\AgdaSymbol{:}\AgdaSpace{}%
\AgdaDatatype{Msg}\AgdaSpace{}%
\AgdaSymbol{→}%
\>[34]\AgdaFunction{Stack}\AgdaSpace{}%
\AgdaSymbol{→}\AgdaSpace{}%
\AgdaDatatype{Maybe}\AgdaSpace{}%
\AgdaFunction{Stack}\<%
\\
\>[0]\AgdaFunction{executeStackCheckSig3Aux}\AgdaSpace{}%
\AgdaBound{msg}\AgdaSpace{}%
\AgdaInductiveConstructor{[]}\AgdaSpace{}%
\AgdaSymbol{=}\AgdaSpace{}%
\AgdaInductiveConstructor{nothing}\<%
\\
\>[0]\AgdaFunction{executeStackCheckSig3Aux}\AgdaSpace{}%
\AgdaBound{mst}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaBound{x}\AgdaSpace{}%
\AgdaOperator{\AgdaInductiveConstructor{∷}}\AgdaSpace{}%
\AgdaInductiveConstructor{[]}\AgdaSymbol{)}\AgdaSpace{}%
\AgdaSymbol{=}\AgdaSpace{}%
\AgdaInductiveConstructor{nothing}\<%
\\
\>[0]\AgdaFunction{executeStackCheckSig3Aux}\AgdaSpace{}%
\AgdaBound{msg}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaBound{m}\AgdaSpace{}%
\AgdaOperator{\AgdaInductiveConstructor{∷}}\AgdaSpace{}%
\AgdaBound{k}\AgdaSpace{}%
\AgdaOperator{\AgdaInductiveConstructor{∷}}\AgdaSpace{}%
\AgdaInductiveConstructor{[]}\AgdaSymbol{)}\AgdaSpace{}%
\AgdaSymbol{=}%
\>[45]\AgdaInductiveConstructor{nothing}\<%
\\
\>[0]\AgdaFunction{executeStackCheckSig3Aux}\AgdaSpace{}%
\AgdaBound{msg}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaBound{m}\AgdaSpace{}%
\AgdaOperator{\AgdaInductiveConstructor{∷}}\AgdaSpace{}%
\AgdaBound{k}\AgdaSpace{}%
\AgdaOperator{\AgdaInductiveConstructor{∷}}\AgdaSpace{}%
\AgdaBound{x}\AgdaSpace{}%
\AgdaOperator{\AgdaInductiveConstructor{∷}}\AgdaSpace{}%
\AgdaInductiveConstructor{[]}\AgdaSymbol{)}\AgdaSpace{}%
\AgdaSymbol{=}%
\>[49]\AgdaInductiveConstructor{nothing}\<%
\\
\>[0]\AgdaFunction{executeStackCheckSig3Aux}\AgdaSpace{}%
\AgdaBound{msg}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaBound{m}\AgdaSpace{}%
\AgdaOperator{\AgdaInductiveConstructor{∷}}\AgdaSpace{}%
\AgdaBound{k}\AgdaSpace{}%
\AgdaOperator{\AgdaInductiveConstructor{∷}}\AgdaSpace{}%
\AgdaBound{x}\AgdaSpace{}%
\AgdaOperator{\AgdaInductiveConstructor{∷}}\AgdaSpace{}%
\AgdaBound{f}\AgdaSpace{}%
\AgdaOperator{\AgdaInductiveConstructor{∷}}\AgdaSpace{}%
\AgdaInductiveConstructor{[]}\AgdaSymbol{)}\AgdaSpace{}%
\AgdaSymbol{=}%
\>[53]\AgdaInductiveConstructor{nothing}\<%
\\
\>[0]\AgdaFunction{executeStackCheckSig3Aux}\AgdaSpace{}%
\AgdaBound{msg}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaBound{m}\AgdaSpace{}%
\AgdaOperator{\AgdaInductiveConstructor{∷}}\AgdaSpace{}%
\AgdaBound{k}\AgdaSpace{}%
\AgdaOperator{\AgdaInductiveConstructor{∷}}\AgdaSpace{}%
\AgdaBound{x}\AgdaSpace{}%
\AgdaOperator{\AgdaInductiveConstructor{∷}}\AgdaSpace{}%
\AgdaBound{f}\AgdaSpace{}%
\AgdaOperator{\AgdaInductiveConstructor{∷}}\AgdaSpace{}%
\AgdaBound{l}\AgdaSpace{}%
\AgdaOperator{\AgdaInductiveConstructor{∷}}\AgdaSpace{}%
\AgdaInductiveConstructor{[]}\AgdaSymbol{)}\AgdaSpace{}%
\AgdaSymbol{=}%
\>[57]\AgdaInductiveConstructor{nothing}\<%
\\
\>[0]\AgdaFunction{executeStackCheckSig3Aux}\AgdaSpace{}%
\AgdaBound{msg}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaBound{p1}\AgdaSpace{}%
\AgdaOperator{\AgdaInductiveConstructor{∷}}\AgdaSpace{}%
\AgdaBound{p2}\AgdaSpace{}%
\AgdaOperator{\AgdaInductiveConstructor{∷}}\AgdaSpace{}%
\AgdaBound{p3}\AgdaSpace{}%
\AgdaOperator{\AgdaInductiveConstructor{∷}}\AgdaSpace{}%
\AgdaBound{s1}\AgdaSpace{}%
\AgdaOperator{\AgdaInductiveConstructor{∷}}\AgdaSpace{}%
\AgdaBound{s2}\AgdaSpace{}%
\AgdaOperator{\AgdaInductiveConstructor{∷}}\AgdaSpace{}%
\AgdaBound{s3}\AgdaSpace{}%
\AgdaOperator{\AgdaInductiveConstructor{∷}}\AgdaSpace{}%
\AgdaBound{s}\AgdaSymbol{)}\AgdaSpace{}%
\AgdaSymbol{=}%
\>[66]\AgdaFunction{stackAuxFunction}\AgdaSpace{}%
\AgdaBound{s}\<%
\\
\>[0][@{}l@{\AgdaIndent{0}}]%
\>[7]\AgdaSymbol{((}\AgdaFunction{isSigned}\AgdaSpace{}%
\AgdaBound{msg}\AgdaSpace{}%
\AgdaBound{s1}\AgdaSpace{}%
\AgdaBound{p1}\AgdaSpace{}%
\AgdaSymbol{)}\AgdaSpace{}%
\AgdaOperator{\AgdaFunction{∧b}}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaFunction{isSigned}\AgdaSpace{}%
\AgdaBound{msg}\AgdaSpace{}%
\AgdaBound{s2}\AgdaSpace{}%
\AgdaBound{p2}\AgdaSymbol{)}\AgdaSpace{}%
\AgdaOperator{\AgdaFunction{∧b}}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaFunction{isSigned}\AgdaSpace{}%
\AgdaBound{msg}\AgdaSpace{}%
\AgdaBound{s3}\AgdaSpace{}%
\AgdaBound{p3}\AgdaSymbol{))}\<%
\\
%
\\[\AgdaEmptyExtraSkip]%
%
\\[\AgdaEmptyExtraSkip]%
%
\\[\AgdaEmptyExtraSkip]%
\>[0]\AgdaKeyword{mutual}\<%
\\
\>[0]\AgdaComment{--\textbackslash{}semanticBasicOperationsForTypeSettingcompareSigsMultiSig}\<%
\end{code}
} % END AgdaHide

\newcommand{\semanticBasicOperationsForTypeSettingcompareSigsMultiSig}{
\begin{code}%
\>[0][@{}l@{\AgdaIndent{1}}]%
\>[1]\AgdaFunction{cmpMultiSigs}\AgdaSpace{}%
\AgdaSymbol{:}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaBound{msg}\AgdaSpace{}%
\AgdaSymbol{:}\AgdaSpace{}%
\AgdaDatatype{Msg}\AgdaSymbol{)(}\AgdaBound{sigs}\AgdaSpace{}%
\AgdaBound{pbks}\AgdaSpace{}%
\AgdaSymbol{:}\AgdaSpace{}%
\AgdaDatatype{List}\AgdaSpace{}%
\AgdaDatatype{ℕ}\AgdaSymbol{)}%
\>[49]\AgdaSymbol{→}\AgdaSpace{}%
\AgdaDatatype{Bool}\<%
\\
%
\>[1]\AgdaFunction{cmpMultiSigs}\AgdaSpace{}%
\AgdaBound{msg}%
\>[19]\AgdaInductiveConstructor{[]}%
\>[36]\AgdaBound{pubkeys}%
\>[47]\AgdaSymbol{=}%
\>[50]\AgdaInductiveConstructor{true}\<%
\\
%
\>[1]\AgdaFunction{cmpMultiSigs}\AgdaSpace{}%
\AgdaBound{msg}%
\>[19]\AgdaSymbol{(}\AgdaBound{sig}\AgdaSpace{}%
\AgdaOperator{\AgdaInductiveConstructor{∷}}\AgdaSpace{}%
\AgdaBound{sigs}\AgdaSymbol{)}%
\>[33]\AgdaInductiveConstructor{[]}%
\>[47]\AgdaSymbol{=}%
\>[50]\AgdaInductiveConstructor{false}\<%
\\
%
\>[1]\AgdaFunction{cmpMultiSigs}\AgdaSpace{}%
\AgdaBound{msg}%
\>[19]\AgdaSymbol{(}\AgdaBound{sig}\AgdaSpace{}%
\AgdaOperator{\AgdaInductiveConstructor{∷}}\AgdaSpace{}%
\AgdaBound{sigs}\AgdaSymbol{)}%
\>[33]\AgdaSymbol{(}\AgdaBound{pbk}\AgdaSpace{}%
\AgdaOperator{\AgdaInductiveConstructor{∷}}\AgdaSpace{}%
\AgdaBound{pbks}\AgdaSymbol{)}%
\>[47]\AgdaSymbol{=}\AgdaSpace{}%
\AgdaFunction{cmpMultiSigsAux}\AgdaSpace{}%
\AgdaBound{msg}\AgdaSpace{}%
\AgdaBound{sigs}\AgdaSpace{}%
\AgdaBound{pbks}\AgdaSpace{}%
\AgdaBound{sig}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaFunction{isSigned}\AgdaSpace{}%
\AgdaBound{msg}\AgdaSpace{}%
\AgdaBound{sig}\AgdaSpace{}%
\AgdaBound{pbk}\AgdaSymbol{)}\<%
\\
%
\\[\AgdaEmptyExtraSkip]%
%
\>[1]\AgdaFunction{cmpMultiSigsAux}\AgdaSpace{}%
\AgdaSymbol{:}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaBound{msg}\AgdaSpace{}%
\AgdaSymbol{:}\AgdaSpace{}%
\AgdaDatatype{Msg}\AgdaSymbol{)(}\AgdaBound{sigs}\AgdaSpace{}%
\AgdaBound{pbks}\AgdaSpace{}%
\AgdaSymbol{:}\AgdaSpace{}%
\AgdaDatatype{List}\AgdaSpace{}%
\AgdaDatatype{ℕ}\AgdaSymbol{)(}\AgdaBound{sig}\AgdaSpace{}%
\AgdaSymbol{:}\AgdaSpace{}%
\AgdaDatatype{ℕ}\AgdaSymbol{)(}\AgdaBound{testRes}\AgdaSpace{}%
\AgdaSymbol{:}\AgdaSpace{}%
\AgdaDatatype{Bool}\AgdaSymbol{)}\AgdaSpace{}%
\AgdaSymbol{→}\AgdaSpace{}%
\AgdaDatatype{Bool}\<%
\\
%
\>[1]\AgdaFunction{cmpMultiSigsAux}%
\>[18]\AgdaBound{msg}%
\>[23]\AgdaBound{sigs}%
\>[29]\AgdaBound{pbks}%
\>[35]\AgdaBound{sig}%
\>[40]\AgdaInductiveConstructor{false}%
\>[47]\AgdaSymbol{=}%
\>[50]\AgdaFunction{cmpMultiSigs}%
\>[64]\AgdaBound{msg}%
\>[69]\AgdaSymbol{(}\AgdaBound{sig}\AgdaSpace{}%
\AgdaOperator{\AgdaInductiveConstructor{∷}}\AgdaSpace{}%
\AgdaBound{sigs}\AgdaSymbol{)}%
\>[83]\AgdaBound{pbks}\<%
\\
%
\>[1]\AgdaFunction{cmpMultiSigsAux}%
\>[18]\AgdaBound{msg}%
\>[23]\AgdaBound{sigs}%
\>[29]\AgdaBound{pbks}%
\>[35]\AgdaBound{sig}%
\>[40]\AgdaInductiveConstructor{true}%
\>[47]\AgdaSymbol{=}%
\>[50]\AgdaFunction{cmpMultiSigs}%
\>[64]\AgdaBound{msg}%
\>[69]\AgdaBound{sigs}%
\>[86]\AgdaBound{pbks}\<%
\end{code}
} % END newcommand

\AgdaHide{
\begin{code}%
\>[0]\<%
\\
\>[0]\AgdaComment{--\textbackslash{}semanticBasicOperationsForTypeSettingexecuteMultiSigThree}\<%
\end{code}
} % END AgdaHide

\newcommand{\semanticBasicOperationsForTypeSettingexecuteMultiSigThree}{
\begin{code}%
\>[0]\AgdaFunction{executeMultiSig3}\AgdaSpace{}%
\AgdaSymbol{:}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaBound{msg}\AgdaSpace{}%
\AgdaSymbol{:}\AgdaSpace{}%
\AgdaDatatype{Msg}\AgdaSymbol{)(}\AgdaBound{pbks}\AgdaSpace{}%
\AgdaSymbol{:}\AgdaSpace{}%
\AgdaDatatype{List}\AgdaSpace{}%
\AgdaDatatype{ℕ}\AgdaSymbol{)(}\AgdaBound{numSigs}\AgdaSpace{}%
\AgdaSymbol{:}\AgdaSpace{}%
\AgdaDatatype{ℕ}\AgdaSymbol{)(}\AgdaBound{st}\AgdaSpace{}%
\AgdaSymbol{:}\AgdaSpace{}%
\AgdaFunction{Stack}\AgdaSymbol{)(}\AgdaBound{sigs}\AgdaSpace{}%
\AgdaSymbol{:}\AgdaSpace{}%
\AgdaDatatype{List}\AgdaSpace{}%
\AgdaDatatype{ℕ}\AgdaSymbol{)}\AgdaSpace{}%
\AgdaSymbol{→}\AgdaSpace{}%
\AgdaDatatype{Maybe}\AgdaSpace{}%
\AgdaFunction{Stack}\<%
\\
\>[0]\AgdaFunction{executeMultiSig3}%
\>[18]\AgdaBound{msg}%
\>[23]\AgdaBound{pbks}%
\>[29]\AgdaSymbol{\AgdaUnderscore{}}%
\>[43]\AgdaInductiveConstructor{[]}\AgdaSpace{}%
\AgdaBound{sigs}%
\>[65]\AgdaSymbol{=}%
\>[68]\AgdaInductiveConstructor{nothing}\<%
\\
\>[0]\AgdaFunction{executeMultiSig3}%
\>[18]\AgdaBound{msg}%
\>[23]\AgdaBound{pbks}%
\>[29]\AgdaInductiveConstructor{zero}%
\>[43]\AgdaSymbol{(}\AgdaBound{x}\AgdaSpace{}%
\AgdaOperator{\AgdaInductiveConstructor{∷}}\AgdaSpace{}%
\AgdaBound{restStack}\AgdaSymbol{)}\AgdaSpace{}%
\AgdaBound{sigs}\<%
\\
%
\>[18]\AgdaSymbol{=}%
\>[21]\AgdaInductiveConstructor{just}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaFunction{boolToNat}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaFunction{cmpMultiSigs}\AgdaSpace{}%
\AgdaBound{msg}\AgdaSpace{}%
\AgdaBound{sigs}\AgdaSpace{}%
\AgdaBound{pbks}\AgdaSymbol{)}\AgdaSpace{}%
\AgdaOperator{\AgdaInductiveConstructor{∷}}\AgdaSpace{}%
\AgdaBound{restStack}\AgdaSymbol{)}\<%
\\
\>[0]\AgdaFunction{executeMultiSig3}%
\>[18]\AgdaBound{msg}%
\>[23]\AgdaBound{pbks}%
\>[29]\AgdaSymbol{(}\AgdaInductiveConstructor{suc}\AgdaSpace{}%
\AgdaBound{numSigs}\AgdaSymbol{)}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaBound{sig}\AgdaSpace{}%
\AgdaOperator{\AgdaInductiveConstructor{∷}}\AgdaSpace{}%
\AgdaBound{rest}\AgdaSymbol{)}\AgdaSpace{}%
\AgdaBound{sigs}\<%
\\
%
\>[18]\AgdaSymbol{=}%
\>[21]\AgdaFunction{executeMultiSig3}\AgdaSpace{}%
\AgdaBound{msg}\AgdaSpace{}%
\AgdaBound{pbks}\AgdaSpace{}%
\AgdaBound{numSigs}\AgdaSpace{}%
\AgdaBound{rest}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaBound{sig}\AgdaSpace{}%
\AgdaOperator{\AgdaInductiveConstructor{∷}}\AgdaSpace{}%
\AgdaBound{sigs}\AgdaSymbol{)}\<%
\end{code}
} % END newcommand

\AgdaHide{
\begin{code}%
\>[0]\<%
\\
\>[0]\AgdaFunction{coreExecuteMultiSigThree}\AgdaSpace{}%
\AgdaSymbol{:}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaBound{msg}\AgdaSpace{}%
\AgdaSymbol{:}\AgdaSpace{}%
\AgdaDatatype{Msg}\AgdaSymbol{)(}\AgdaBound{sigs}\AgdaSpace{}%
\AgdaSymbol{:}\AgdaSpace{}%
\AgdaDatatype{List}\AgdaSpace{}%
\AgdaDatatype{ℕ}\AgdaSymbol{)(}\AgdaBound{pbks}\AgdaSpace{}%
\AgdaSymbol{:}\AgdaSpace{}%
\AgdaDatatype{List}\AgdaSpace{}%
\AgdaDatatype{ℕ}\AgdaSymbol{)(}\AgdaBound{restStack}\AgdaSpace{}%
\AgdaSymbol{:}\AgdaSpace{}%
\AgdaFunction{Stack}\AgdaSymbol{)}\AgdaSpace{}%
\AgdaSymbol{→}\AgdaSpace{}%
\AgdaDatatype{Maybe}\AgdaSpace{}%
\AgdaFunction{Stack}\<%
\\
\>[0]\AgdaFunction{coreExecuteMultiSigThree}\AgdaSpace{}%
\AgdaBound{msg}\AgdaSpace{}%
\AgdaBound{sigs}\AgdaSpace{}%
\AgdaBound{pbks}\AgdaSpace{}%
\AgdaBound{restStack}\AgdaSpace{}%
\AgdaSymbol{=}\<%
\\
\>[0]\AgdaComment{--\textbackslash{}semanticBasicOperationsForTypeSettingcoreExecuteMultiSigThree}\<%
\end{code}
} % END AgdaHide

\newcommand{\semanticBasicOperationsForTypeSettingcoreExecuteMultiSigThree}{
\begin{code}[inline]%
\>[0][@{}l@{\AgdaIndent{1}}]%
\>[2]\AgdaInductiveConstructor{just}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaFunction{boolToNat}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaFunction{cmpMultiSigs}\AgdaSpace{}%
\AgdaBound{msg}\AgdaSpace{}%
\AgdaBound{sigs}\AgdaSpace{}%
\AgdaBound{pbks}\AgdaSymbol{)}\AgdaSpace{}%
\AgdaOperator{\AgdaInductiveConstructor{∷}}\AgdaSpace{}%
\AgdaBound{restStack}\AgdaSymbol{)}\<%
\end{code}
} % END newcommand

\AgdaHide{
\begin{code}%
\>[0]\<%
\\
\>[0]\AgdaComment{--\textbackslash{}semanticBasicOperationsForTypeSettingexecuteMultiSigTwo}\<%
\end{code}
} % END AgdaHide

\newcommand{\semanticBasicOperationsForTypeSettingexecuteMultiSigTwo}{
\begin{code}%
\>[0]\AgdaFunction{executeMultiSig2}\AgdaSpace{}%
\AgdaSymbol{:}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaBound{msg}\AgdaSpace{}%
\AgdaSymbol{:}\AgdaSpace{}%
\AgdaDatatype{Msg}\AgdaSymbol{)(}\AgdaBound{numPbks}\AgdaSpace{}%
\AgdaSymbol{:}\AgdaSpace{}%
\AgdaDatatype{ℕ}\AgdaSymbol{)(}\AgdaBound{st}\AgdaSpace{}%
\AgdaSymbol{:}%
\>[51]\AgdaFunction{Stack}\AgdaSymbol{)(}\AgdaBound{pbks}\AgdaSpace{}%
\AgdaSymbol{:}\AgdaSpace{}%
\AgdaDatatype{List}\AgdaSpace{}%
\AgdaDatatype{ℕ}\AgdaSymbol{)}\AgdaSpace{}%
\AgdaSymbol{→}\AgdaSpace{}%
\AgdaDatatype{Maybe}\AgdaSpace{}%
\AgdaFunction{Stack}\<%
\\
\>[0]\AgdaFunction{executeMultiSig2}%
\>[18]\AgdaBound{msg}%
\>[23]\AgdaSymbol{\AgdaUnderscore{}}%
\>[32]\AgdaInductiveConstructor{[]}%
\>[50]\AgdaBound{pbks}%
\>[56]\AgdaSymbol{=}%
\>[59]\AgdaInductiveConstructor{nothing}\<%
\\
\>[0]\AgdaFunction{executeMultiSig2}%
\>[18]\AgdaBound{msg}%
\>[23]\AgdaInductiveConstructor{zero}%
\>[32]\AgdaSymbol{(}\AgdaBound{numSigs}\AgdaSpace{}%
\AgdaOperator{\AgdaInductiveConstructor{∷}}\AgdaSpace{}%
\AgdaBound{rest}\AgdaSymbol{)}%
\>[50]\AgdaBound{pbks}%
\>[56]\AgdaSymbol{=}%
\>[59]\AgdaFunction{executeMultiSig3}\AgdaSpace{}%
\AgdaBound{msg}\AgdaSpace{}%
\AgdaBound{pbks}\AgdaSpace{}%
\AgdaBound{numSigs}\AgdaSpace{}%
\AgdaBound{rest}\AgdaSpace{}%
\AgdaInductiveConstructor{[]}\<%
\\
\>[0]\AgdaFunction{executeMultiSig2}%
\>[18]\AgdaBound{msg}%
\>[23]\AgdaSymbol{(}\AgdaInductiveConstructor{suc}\AgdaSpace{}%
\AgdaBound{n}\AgdaSymbol{)}%
\>[32]\AgdaSymbol{(}\AgdaBound{pbk}\AgdaSpace{}%
\AgdaOperator{\AgdaInductiveConstructor{∷}}\AgdaSpace{}%
\AgdaBound{rest}\AgdaSymbol{)}%
\>[50]\AgdaBound{pbks}%
\>[56]\AgdaSymbol{=}%
\>[59]\AgdaFunction{executeMultiSig2}\AgdaSpace{}%
\AgdaBound{msg}\AgdaSpace{}%
\AgdaBound{n}\AgdaSpace{}%
\AgdaBound{rest}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaBound{pbk}\AgdaSpace{}%
\AgdaOperator{\AgdaInductiveConstructor{∷}}\AgdaSpace{}%
\AgdaBound{pbks}\AgdaSymbol{)}\<%
\end{code}
} % END newcommand

\AgdaHide{
\begin{code}%
\>[0]\AgdaComment{--open\ import\ addition10}\<%
\\
%
\\[\AgdaEmptyExtraSkip]%
%
\\[\AgdaEmptyExtraSkip]%
\>[0]\AgdaComment{--\ Add\ the\ notes\ to\ a\ file\ \ notes\ in\ notes}\<%
\\
\>[0]\AgdaComment{--\ next\ steps}\<%
\\
\>[0]\AgdaComment{--\ move\ executeMultiSig\ to\ semanticsInstructions.agda}\<%
\\
\>[0]\AgdaComment{--\ add\ opMultiSig\ to\ the\ instructions}\<%
\\
\>[0]\AgdaComment{--\ define\ ⟦\ OpMultiSig\ ⟧s\ =\ liftMsgStackToStateTransformerDepIfStack'\ executeMultiSig}\<%
\\
\>[0]\AgdaComment{--\ in\ semanticsInstructions}\<%
\\
\>[0]\AgdaComment{--\ define\ in\ addition4.agda}\<%
\\
\>[0]\AgdaComment{--\ \ \ ⟦\ OpMultiSig\ \ \ ⟧stacks\ time₁\ msg\ =\ \ executeMultiSig\ msg}\<%
\\
%
\\[\AgdaEmptyExtraSkip]%
%
\\[\AgdaEmptyExtraSkip]%
\>[0]\AgdaComment{--\ Try\ out\ evaluatings\ scripts\ as\ in\ scriptInterpreter.agda\ \ whether\ it\ works\ as\ intended}\<%
\\
\>[0]\AgdaComment{--\ \ \ write\ some\ multisignature\ script\ and\ a\ scriptsig\ \ and\ check\ whether\ they\ work\ correctly}\<%
\\
%
\\[\AgdaEmptyExtraSkip]%
\>[0]\AgdaComment{--\ Try\ out\ experiments\ like\ stackfunP2PKH\ \ \ in\ additionAntonExperiments.agda}\<%
\\
\>[0]\AgdaComment{--\ for}\<%
\\
\>[0]\AgdaComment{--\ ⟦\ (opPush\ 2)\ ∷\ (opPush\ pbk1)\ ∷\ \ (opPush\ pbk2)\ ∷\ \ (opPush\ pbk3)\ ∷\ \ (opPush\ 3)\ ∷\ \ opMultiSig\ ∷\ \ []\ \ \ \ \ ⟧stack\ time\ msg\ stack}\<%
\\
\>[0]\AgdaComment{--\ whether\ this\ is\ equal\ to}\<%
\\
\>[0]\AgdaComment{--\ executeMultiSig3\ msg\ (pbk1\ ∷\ pbk2\ ∷\ pbk3\ ∷\ [])\ 2\ stack\ []}\<%
\\
\>[0]\AgdaComment{--\ similarly\ as\ in\ lemma1\ by\ postulating\ \ \ pbk1,..,pbk3,time,msg,stack}\<%
\\
%
\\[\AgdaEmptyExtraSkip]%
\>[0]\AgdaComment{--\ if\ yes\ then\ the}\<%
\\
\>[0]\AgdaComment{--\ weakest\ precondtion\ for\ the\ multisig\ script\ would\ be:}\<%
\\
\>[0]\AgdaComment{--\ stack\ needs\ to\ have\ size\ at\ least\ 2\ and\ the\ for\ signatures\ sig1\ sig2\ on\ the\ stack\ we\ have}\<%
\\
\>[0]\AgdaComment{--\ cmpMultiSigs\ \ msg\ (sig1\ ∷\ [\ sig2\ ])\ (pbk1\ ∷\ pbk2\ ∷\ [\ pbk3\ ]\ )\ =\ true}\<%
\\
%
\\[\AgdaEmptyExtraSkip]%
\>[0]\AgdaComment{--\textbackslash{}semanticBasicOperationsForTypeSettingcheckpubk}\<%
\end{code}
} % END AgdaHide

\newcommand{\semanticBasicOperationsForTypeSettingexecuteMultiSig}{
\begin{code}%
\>[0]\AgdaFunction{executeMultiSig}\AgdaSpace{}%
\AgdaSymbol{:}\AgdaSpace{}%
\AgdaDatatype{Msg}\AgdaSpace{}%
\AgdaSymbol{→}%
\>[25]\AgdaFunction{Stack}\AgdaSpace{}%
\AgdaSymbol{→}%
\>[34]\AgdaDatatype{Maybe}\AgdaSpace{}%
\AgdaFunction{Stack}\<%
\\
\>[0]\AgdaFunction{executeMultiSig}\AgdaSpace{}%
\AgdaBound{msg}\AgdaSpace{}%
\AgdaInductiveConstructor{[]}\AgdaSpace{}%
\AgdaSymbol{=}\AgdaSpace{}%
\AgdaInductiveConstructor{nothing}\<%
\\
\>[0]\AgdaFunction{executeMultiSig}\AgdaSpace{}%
\AgdaBound{msg}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaBound{numberOfPbks}\AgdaSpace{}%
\AgdaOperator{\AgdaInductiveConstructor{∷}}\AgdaSpace{}%
\AgdaBound{st}\AgdaSymbol{)}\AgdaSpace{}%
\AgdaSymbol{=}\AgdaSpace{}%
\AgdaFunction{executeMultiSig2}\AgdaSpace{}%
\AgdaBound{msg}\AgdaSpace{}%
\AgdaBound{numberOfPbks}\AgdaSpace{}%
\AgdaBound{st}\AgdaSpace{}%
\AgdaInductiveConstructor{[]}\<%
\end{code}
} % END newcommand

\AgdaHide{
\begin{code}%
\>[0]\<%
\end{code}
} % END AgdaHide


==> latex-before-sed/paperTypes2021PostProceed/stackVerificationP2PKHsymbolicExecutionPaperVersion.tex <==
%% This file has been generated automatically by mkLagda.awk
%% DO NOT EDIT! ALL YOUR CHANGES WILL BE LOST!

\AgdaHide{
\begin{code}%
\>[0]\AgdaComment{--\ \textbackslash{}stackVerificationPtoPKHsymbolicExecution}\<%
\\
\>[0]\AgdaKeyword{open}\AgdaSpace{}%
\AgdaKeyword{import}\AgdaSpace{}%
\AgdaModule{basicBitcoinDataType}\<%
\\
%
\\[\AgdaEmptyExtraSkip]%
\>[0]\AgdaKeyword{module}\AgdaSpace{}%
\AgdaModule{paperTypes2021PostProceed.stackVerificationP2PKHsymbolicExecutionPaperVersion}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaBound{param}\AgdaSpace{}%
\AgdaSymbol{:}\AgdaSpace{}%
\AgdaRecord{GlobalParameters}\AgdaSymbol{)}%
\>[113]\AgdaKeyword{where}\<%
\\
%
\\[\AgdaEmptyExtraSkip]%
\>[0]\AgdaKeyword{open}\AgdaSpace{}%
\AgdaKeyword{import}\AgdaSpace{}%
\AgdaModule{Data.Nat}%
\>[22]\AgdaKeyword{hiding}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaOperator{\AgdaDatatype{\AgdaUnderscore{}≤\AgdaUnderscore{}}}\AgdaSymbol{)}\<%
\\
\>[0]\AgdaKeyword{open}\AgdaSpace{}%
\AgdaKeyword{import}\AgdaSpace{}%
\AgdaModule{Data.List}\AgdaSpace{}%
\AgdaKeyword{hiding}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaOperator{\AgdaFunction{\AgdaUnderscore{}++\AgdaUnderscore{}}}\AgdaSymbol{)}\<%
\\
\>[0]\AgdaKeyword{open}\AgdaSpace{}%
\AgdaKeyword{import}\AgdaSpace{}%
\AgdaModule{Data.Unit}%
\>[23]\AgdaKeyword{hiding}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaOperator{\AgdaRecord{\AgdaUnderscore{}≤\AgdaUnderscore{}}}\AgdaSymbol{)}\<%
\\
\>[0]\AgdaKeyword{open}\AgdaSpace{}%
\AgdaKeyword{import}\AgdaSpace{}%
\AgdaModule{Data.Empty}\<%
\\
\>[0]\AgdaKeyword{open}\AgdaSpace{}%
\AgdaKeyword{import}\AgdaSpace{}%
\AgdaModule{Data.Sum}\<%
\\
\>[0]\AgdaKeyword{open}\AgdaSpace{}%
\AgdaKeyword{import}\AgdaSpace{}%
\AgdaModule{Data.Bool}%
\>[23]\AgdaKeyword{hiding}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaOperator{\AgdaDatatype{\AgdaUnderscore{}≤\AgdaUnderscore{}}}\AgdaSpace{}%
\AgdaSymbol{;}\AgdaSpace{}%
\AgdaOperator{\AgdaFunction{if\AgdaUnderscore{}then\AgdaUnderscore{}else\AgdaUnderscore{}}}\AgdaSpace{}%
\AgdaSymbol{)}\AgdaSpace{}%
\AgdaKeyword{renaming}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaOperator{\AgdaFunction{\AgdaUnderscore{}∧\AgdaUnderscore{}}}\AgdaSpace{}%
\AgdaSymbol{to}\AgdaSpace{}%
\AgdaOperator{\AgdaFunction{\AgdaUnderscore{}∧b\AgdaUnderscore{}}}\AgdaSpace{}%
\AgdaSymbol{;}\AgdaSpace{}%
\AgdaOperator{\AgdaFunction{\AgdaUnderscore{}∨\AgdaUnderscore{}}}\AgdaSpace{}%
\AgdaSymbol{to}\AgdaSpace{}%
\AgdaOperator{\AgdaFunction{\AgdaUnderscore{}∨b\AgdaUnderscore{}}}\AgdaSpace{}%
\AgdaSymbol{;}\AgdaSpace{}%
\AgdaFunction{T}\AgdaSpace{}%
\AgdaSymbol{to}\AgdaSpace{}%
\AgdaFunction{True}\AgdaSymbol{)}\<%
\\
\>[0]\AgdaKeyword{open}\AgdaSpace{}%
\AgdaKeyword{import}\AgdaSpace{}%
\AgdaModule{Data.Product}\AgdaSpace{}%
\AgdaKeyword{renaming}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaOperator{\AgdaInductiveConstructor{\AgdaUnderscore{},\AgdaUnderscore{}}}\AgdaSpace{}%
\AgdaSymbol{to}\AgdaSpace{}%
\AgdaOperator{\AgdaInductiveConstructor{\AgdaUnderscore{},,\AgdaUnderscore{}}}\AgdaSpace{}%
\AgdaSymbol{)}\<%
\\
\>[0]\AgdaKeyword{open}\AgdaSpace{}%
\AgdaKeyword{import}\AgdaSpace{}%
\AgdaModule{Data.Nat.Base}\AgdaSpace{}%
\AgdaKeyword{hiding}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaOperator{\AgdaDatatype{\AgdaUnderscore{}≤\AgdaUnderscore{}}}\AgdaSymbol{)}\<%
\\
\>[0]\AgdaKeyword{open}\AgdaSpace{}%
\AgdaKeyword{import}\AgdaSpace{}%
\AgdaModule{Data.List.NonEmpty}\AgdaSpace{}%
\AgdaKeyword{hiding}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaField{head}\AgdaSpace{}%
\AgdaSymbol{;}\AgdaSpace{}%
\AgdaOperator{\AgdaFunction{[\AgdaUnderscore{}]}}\AgdaSpace{}%
\AgdaSymbol{)}\<%
\\
\>[0]\AgdaKeyword{open}\AgdaSpace{}%
\AgdaKeyword{import}\AgdaSpace{}%
\AgdaModule{Data.Maybe}\<%
\\
\>[0]\AgdaKeyword{open}\AgdaSpace{}%
\AgdaKeyword{import}\AgdaSpace{}%
\AgdaModule{Relation.Nullary}\<%
\\
%
\\[\AgdaEmptyExtraSkip]%
\>[0]\AgdaKeyword{import}\AgdaSpace{}%
\AgdaModule{Relation.Binary.PropositionalEquality}\AgdaSpace{}%
\AgdaSymbol{as}\AgdaSpace{}%
\AgdaModule{Eq}\<%
\\
\>[0]\AgdaKeyword{open}\AgdaSpace{}%
\AgdaModule{Eq}\AgdaSpace{}%
\AgdaKeyword{using}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaOperator{\AgdaDatatype{\AgdaUnderscore{}≡\AgdaUnderscore{}}}\AgdaSymbol{;}\AgdaSpace{}%
\AgdaInductiveConstructor{refl}\AgdaSymbol{;}\AgdaSpace{}%
\AgdaFunction{cong}\AgdaSymbol{;}\AgdaSpace{}%
\AgdaKeyword{module}\AgdaSpace{}%
\AgdaModule{≡-Reasoning}\AgdaSymbol{;}\AgdaSpace{}%
\AgdaFunction{sym}\AgdaSymbol{)}\<%
\\
\>[0]\AgdaKeyword{open}\AgdaSpace{}%
\AgdaModule{≡-Reasoning}\<%
\\
\>[0]\AgdaKeyword{open}\AgdaSpace{}%
\AgdaKeyword{import}\AgdaSpace{}%
\AgdaModule{Agda.Builtin.Equality}\<%
\\
%
\\[\AgdaEmptyExtraSkip]%
%
\\[\AgdaEmptyExtraSkip]%
\>[0]\AgdaComment{--our\ libraries}\<%
\\
\>[0]\AgdaKeyword{open}\AgdaSpace{}%
\AgdaKeyword{import}\AgdaSpace{}%
\AgdaModule{libraries.listLib}\<%
\\
\>[0]\AgdaKeyword{open}\AgdaSpace{}%
\AgdaKeyword{import}\AgdaSpace{}%
\AgdaModule{libraries.equalityLib}\<%
\\
\>[0]\AgdaKeyword{open}\AgdaSpace{}%
\AgdaKeyword{import}\AgdaSpace{}%
\AgdaModule{libraries.natLib}\<%
\\
\>[0]\AgdaKeyword{open}\AgdaSpace{}%
\AgdaKeyword{import}\AgdaSpace{}%
\AgdaModule{libraries.boolLib}\<%
\\
\>[0]\AgdaKeyword{open}\AgdaSpace{}%
\AgdaKeyword{import}\AgdaSpace{}%
\AgdaModule{libraries.emptyLib}\<%
\\
\>[0]\AgdaKeyword{open}\AgdaSpace{}%
\AgdaKeyword{import}\AgdaSpace{}%
\AgdaModule{libraries.andLib}\<%
\\
\>[0]\AgdaKeyword{open}\AgdaSpace{}%
\AgdaKeyword{import}\AgdaSpace{}%
\AgdaModule{libraries.miscLib}\<%
\\
\>[0]\AgdaKeyword{open}\AgdaSpace{}%
\AgdaKeyword{import}\AgdaSpace{}%
\AgdaModule{libraries.maybeLib}\<%
\\
%
\\[\AgdaEmptyExtraSkip]%
\>[0]\AgdaKeyword{open}\AgdaSpace{}%
\AgdaKeyword{import}\AgdaSpace{}%
\AgdaModule{stack}\<%
\\
\>[0]\AgdaKeyword{open}\AgdaSpace{}%
\AgdaKeyword{import}\AgdaSpace{}%
\AgdaModule{stackPredicate}\<%
\\
\>[0]\AgdaKeyword{open}\AgdaSpace{}%
\AgdaKeyword{import}\AgdaSpace{}%
\AgdaModule{semanticBasicOperations}\AgdaSpace{}%
\AgdaBound{param}\<%
\\
\>[0]\AgdaKeyword{open}\AgdaSpace{}%
\AgdaKeyword{import}\AgdaSpace{}%
\AgdaModule{hoareTripleStack}\AgdaSpace{}%
\AgdaBound{param}\<%
\\
\>[0]\AgdaKeyword{open}\AgdaSpace{}%
\AgdaKeyword{import}\AgdaSpace{}%
\AgdaModule{instruction}\<%
\\
\>[0]\AgdaKeyword{open}\AgdaSpace{}%
\AgdaKeyword{import}\AgdaSpace{}%
\AgdaModule{verificationStackScripts.stackState}\<%
\\
\>[0]\AgdaKeyword{open}\AgdaSpace{}%
\AgdaKeyword{import}\AgdaSpace{}%
\AgdaModule{verificationStackScripts.sPredicate}\<%
\\
\>[0]\AgdaKeyword{open}\AgdaSpace{}%
\AgdaKeyword{import}\AgdaSpace{}%
\AgdaModule{verificationStackScripts.stackHoareTriple}\AgdaSpace{}%
\AgdaBound{param}\<%
\\
\>[0]\AgdaKeyword{open}\AgdaSpace{}%
\AgdaKeyword{import}\AgdaSpace{}%
\AgdaModule{verificationStackScripts.stackVerificationLemmas}\AgdaSpace{}%
\AgdaBound{param}\<%
\\
\>[0]\AgdaKeyword{open}\AgdaSpace{}%
\AgdaKeyword{import}\AgdaSpace{}%
\AgdaModule{verificationStackScripts.stackSemanticsInstructionsBasic}\AgdaSpace{}%
\AgdaBound{param}\<%
\\
\>[0]\AgdaKeyword{open}\AgdaSpace{}%
\AgdaKeyword{import}\AgdaSpace{}%
\AgdaModule{verificationStackScripts.semanticsStackInstructions}\AgdaSpace{}%
\AgdaBound{param}\<%
\\
\>[0]\AgdaKeyword{open}\AgdaSpace{}%
\AgdaKeyword{import}\AgdaSpace{}%
\AgdaModule{verificationStackScripts.stackVerificationP2PKH}\AgdaSpace{}%
\AgdaBound{param}\<%
\\
\>[0]\AgdaKeyword{open}\AgdaSpace{}%
\AgdaKeyword{import}\AgdaSpace{}%
\AgdaModule{verificationStackScripts.stackVerificationP2PKHindexed}\AgdaSpace{}%
\AgdaBound{param}\<%
\\
%
\\[\AgdaEmptyExtraSkip]%
\>[0]\AgdaComment{-------------------------------------------------------------}\<%
\\
\>[0]\AgdaComment{--\ \ \ This\ file\ explores\ the\ symoblic\ execution\ of\ the\ P2PKH\ program}\<%
\\
\>[0]\AgdaComment{--\ \ \ \ \ in\ order\ to\ determine\ the\ case\ distinction}\<%
\\
\>[0]\AgdaComment{--\ \ \ \ \ and\ extract\ a\ program\ from\ it}\<%
\\
\>[0]\AgdaComment{--}\<%
\\
\>[0]\AgdaComment{--\ \ \ This\ is\ done\ by\ postulating\ parameters\ and\ applying\ ⟦\ scriptP2PKHᵇ\ pbkh\ ⟧ˢ}\<%
\\
\>[0]\AgdaComment{--\ \ \ \ \ to\ parameters}\<%
\\
\>[0]\AgdaComment{--------------------------------------------------------------------------------}\<%
\\
%
\\[\AgdaEmptyExtraSkip]%
\>[0]\AgdaKeyword{private}\<%
\\
\>[0][@{}l@{\AgdaIndent{0}}]%
\>[2]\AgdaKeyword{postulate}\AgdaSpace{}%
\AgdaPostulate{time₁}\AgdaSpace{}%
\AgdaSymbol{:}\AgdaSpace{}%
\AgdaFunction{Time}\<%
\\
%
\>[2]\AgdaKeyword{postulate}\AgdaSpace{}%
\AgdaPostulate{msg₁}\AgdaSpace{}%
\AgdaSymbol{:}\AgdaSpace{}%
\AgdaDatatype{Msg}\<%
\\
%
\>[2]\AgdaKeyword{postulate}\AgdaSpace{}%
\AgdaPostulate{stack₁}\AgdaSpace{}%
\AgdaSymbol{:}\AgdaSpace{}%
\AgdaFunction{Stack}\<%
\\
%
\>[2]\AgdaKeyword{postulate}\AgdaSpace{}%
\AgdaPostulate{pbkh}\AgdaSpace{}%
\AgdaSymbol{:}\AgdaSpace{}%
\AgdaDatatype{ℕ}\<%
\\
%
\>[2]\AgdaKeyword{postulate}\AgdaSpace{}%
\AgdaPostulate{pbk}\AgdaSpace{}%
\AgdaSymbol{:}\AgdaSpace{}%
\AgdaDatatype{ℕ}\<%
\\
%
\>[2]\AgdaKeyword{postulate}\AgdaSpace{}%
\AgdaPostulate{x₁}\AgdaSpace{}%
\AgdaSymbol{:}\AgdaSpace{}%
\AgdaDatatype{ℕ}\<%
\\
%
\>[2]\AgdaKeyword{postulate}\AgdaSpace{}%
\AgdaPostulate{sig₁}\AgdaSpace{}%
\AgdaSymbol{:}\AgdaSpace{}%
\AgdaDatatype{ℕ}\<%
\\
%
\\[\AgdaEmptyExtraSkip]%
%
\\[\AgdaEmptyExtraSkip]%
\>[0]\AgdaComment{\{-\ We\ first\ create\ a\ symbolic\ execution\ of\ the\ scriptP2PKHᵇ\ pbkh\ to\ see\ what\ kind}\<%
\\
\>[0]\AgdaComment{\ \ \ of\ case\ distinction\ happens\ -\}}\<%
\\
%
\\[\AgdaEmptyExtraSkip]%
\>[0]\AgdaFunction{check}\AgdaSpace{}%
\AgdaSymbol{=}\AgdaSpace{}%
\AgdaFunction{scriptP2PKHᵇ}\<%
\\
%
\\[\AgdaEmptyExtraSkip]%
\>[0]\AgdaFunction{testP2PKHscript}\AgdaSpace{}%
\AgdaSymbol{:}\AgdaSpace{}%
\AgdaDatatype{Maybe}\AgdaSpace{}%
\AgdaFunction{Stack}\<%
\\
\>[0]\AgdaFunction{testP2PKHscript}\AgdaSpace{}%
\AgdaSymbol{=}\<%
\\
\>[0]\AgdaComment{--\ \textbackslash{}stackVerificationPtoPKHsymbolicExecutiontestPtoP}\<%
\end{code}
} % END AgdaHide

\newcommand{\stackVerificationPtoPKHsymbolicExecutiontestPtoP}{
\begin{code}[inline]%
\>[0][@{}l@{\AgdaIndent{1}}]%
\>[1]\AgdaOperator{\AgdaFunction{⟦}}\AgdaSpace{}%
\AgdaFunction{scriptP2PKHᵇ}\AgdaSpace{}%
\AgdaPostulate{pbkh}\AgdaSpace{}%
\AgdaOperator{\AgdaFunction{⟧ˢ}}\AgdaSpace{}%
\AgdaPostulate{time₁}\AgdaSpace{}%
\AgdaPostulate{msg₁}\AgdaSpace{}%
\AgdaPostulate{stack₁}\<%
\end{code}
} % END newcommand

\AgdaHide{
\begin{code}%
\>[0]\<%
\\
%
\\[\AgdaEmptyExtraSkip]%
%
\\[\AgdaEmptyExtraSkip]%
\>[0]\AgdaComment{--⟦\ scriptP2PKHᵇ\ pbkh\ ⟧ˢ\ time₁\ msg₁\ stack}\<%
\\
%
\\[\AgdaEmptyExtraSkip]%
\>[0]\AgdaComment{\{-\ evaluation\ gives}\<%
\\
\>[0]\<%
\\
\>[0]\AgdaComment{executeStackDup\ stack₁\ >>=}\<%
\\
\>[0]\AgdaComment{(λ\ stack₂\ →}\<%
\\
\>[0]\AgdaComment{\ \ \ executeOpHash\ stack₂\ >>=}\<%
\\
\>[0]\AgdaComment{\ \ \ (λ\ stack₃\ →}\<%
\\
\>[0]\AgdaComment{\ \ \ \ \ \ executeStackEquality\ (pbkh\ ∷\ stack₃)\ >>=}\<%
\\
\>[0]\AgdaComment{\ \ \ \ \ \ (λ\ stack₄\ →}\<%
\\
\>[0]\AgdaComment{\ \ \ \ \ \ \ \ \ executeStackVerify\ stack₄\ >>=}\<%
\\
\>[0]\AgdaComment{\ \ \ \ \ \ \ \ \ (λ\ stack₅\ →\ executeStackCheckSig\ msg₁\ stack₅))))}\<%
\\
\>[0]\<%
\\
\>[0]\AgdaComment{Improved\ layout}\<%
\\
\>[0]\AgdaComment{executeStackDup\ stack₁\ >>=\ (λ\ stack₂\ →\ \ executeOpHash\ stack₂\ >>=}\<%
\\
\>[0]\AgdaComment{\ \ \ (λ\ stack₃\ →\ \ executeStackEquality\ (pbkh\ ∷\ stack₃)\ >>=}\<%
\\
\>[0]\AgdaComment{\ \ \ (λ\ stack₄\ →\ \ executeStackVerify\ stack₄\ >>=}\<%
\\
\>[0]\AgdaComment{\ \ \ (λ\ stack₅\ →\ executeStackCheckSig\ msg₁\ stack₅))))}\<%
\\
\>[0]\<%
\\
\>[0]\<%
\\
\>[0]\<%
\\
\>[0]\AgdaComment{--\ old\ version\ was}\<%
\\
\>[0]\<%
\\
\>[0]\AgdaComment{lift2Maybe}\<%
\\
\>[0]\AgdaComment{(λ\ stack₂\ →}\<%
\\
\>[0]\AgdaComment{\ \ \ lift2Maybe}\<%
\\
\>[0]\AgdaComment{\ \ \ (λ\ stack₃\ →}\<%
\\
\>[0]\AgdaComment{\ \ \ \ \ \ lift2Maybe}\<%
\\
\>[0]\AgdaComment{\ \ \ \ \ \ (λ\ stack₄\ →}\<%
\\
\>[0]\AgdaComment{\ \ \ \ \ \ \ \ \ lift2Maybe\ (λ\ stack₅\ →\ executeStackCheckSig\ msg₁\ stack₅)}\<%
\\
\>[0]\AgdaComment{\ \ \ \ \ \ \ \ \ (executeStackVerify\ stack₄))}\<%
\\
\>[0]\AgdaComment{\ \ \ \ \ \ (executeStackEquality\ (pbkh\ ∷\ stack₃)))}\<%
\\
\>[0]\AgdaComment{\ \ \ (executeOpHash\ stack₂))}\<%
\\
\>[0]\AgdaComment{(executeStackDup\ stack₁)}\<%
\\
\>[0]\<%
\\
\>[0]\AgdaComment{-\}}\<%
\\
%
\\[\AgdaEmptyExtraSkip]%
\>[0]\AgdaComment{--\ We\ define\ a\ term\ giving\ the\ result\ of\ the\ evaluation}\<%
\\
%
\\[\AgdaEmptyExtraSkip]%
\>[0]\AgdaFunction{testP2PKHscript2}\AgdaSpace{}%
\AgdaSymbol{:}\AgdaSpace{}%
\AgdaDatatype{Maybe}\AgdaSpace{}%
\AgdaFunction{Stack}\<%
\\
\>[0]\AgdaFunction{testP2PKHscript2}\AgdaSpace{}%
\AgdaSymbol{=}\<%
\\
\>[0]\AgdaComment{--\ \textbackslash{}stackVerificationPtoPKHsymbolicExecutiontestPtoPKHscripttwo}\<%
\end{code}
} % END AgdaHide

\newcommand{\stackVerificationPtoPKHsymbolicExecutiontestPtoPKHscripttwo}{
\begin{code}%
\>[0][@{}l@{\AgdaIndent{1}}]%
\>[1]\AgdaFunction{executeStackDup}\AgdaSpace{}%
\AgdaPostulate{stack₁}%
\>[39]\AgdaOperator{\AgdaFunction{>>=}}%
\>[44]\AgdaSymbol{λ}\AgdaSpace{}%
\AgdaBound{stack₂}\AgdaSpace{}%
\AgdaSymbol{→}%
\>[56]\AgdaFunction{executeOpHash}\AgdaSpace{}%
\AgdaBound{stack₂}%
\>[83]\AgdaOperator{\AgdaFunction{>>=}}\AgdaSpace{}%
\AgdaSymbol{λ}\AgdaSpace{}%
\AgdaBound{stack₃}\AgdaSpace{}%
\AgdaSymbol{→}\<%
\\
%
\>[1]\AgdaFunction{executeStackEquality}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaPostulate{pbkh}\AgdaSpace{}%
\AgdaOperator{\AgdaInductiveConstructor{∷}}\AgdaSpace{}%
\AgdaBound{stack₃}\AgdaSymbol{)}%
\>[39]\AgdaOperator{\AgdaFunction{>>=}}%
\>[44]\AgdaSymbol{λ}\AgdaSpace{}%
\AgdaBound{stack₄}\AgdaSpace{}%
\AgdaSymbol{→}%
\>[56]\AgdaFunction{executeStackVerify}\AgdaSpace{}%
\AgdaBound{stack₄}%
\>[83]\AgdaOperator{\AgdaFunction{>>=}}\AgdaSpace{}%
\AgdaSymbol{λ}\AgdaSpace{}%
\AgdaBound{stack₅}\AgdaSpace{}%
\AgdaSymbol{→}\<%
\\
%
\>[1]\AgdaFunction{executeStackCheckSig}\AgdaSpace{}%
\AgdaPostulate{msg₁}\AgdaSpace{}%
\AgdaBound{stack₅}\<%
\end{code}
} % END newcommand

\AgdaHide{
\begin{code}%
\>[0]\<%
\\
\>[0]\AgdaFunction{testP2PKHscript2UsingMoreSpace}\AgdaSpace{}%
\AgdaSymbol{=}\<%
\\
\>[0]\AgdaComment{--\ \textbackslash{}stackVerificationPtoPKHsymbolicExecutiontestPtoPKHscripttwoUsingMoreSpace}\<%
\end{code}
} % END AgdaHide

\newcommand{\stackVerificationPtoPKHsymbolicExecutiontestPtoPKHscripttwoUsingMoreSpace}{
\begin{code}%
\>[0][@{}l@{\AgdaIndent{1}}]%
\>[1]\AgdaFunction{executeStackDup}\AgdaSpace{}%
\AgdaPostulate{stack₁}%
\>[52]\AgdaOperator{\AgdaFunction{>>=}}\<%
\\
%
\>[1]\AgdaSymbol{λ}\AgdaSpace{}%
\AgdaBound{stack₂}\AgdaSpace{}%
\AgdaSymbol{→}%
\>[13]\AgdaFunction{executeOpHash}\AgdaSpace{}%
\AgdaBound{stack₂}%
\>[52]\AgdaOperator{\AgdaFunction{>>=}}\<%
\\
%
\>[1]\AgdaSymbol{λ}\AgdaSpace{}%
\AgdaBound{stack₃}\AgdaSpace{}%
\AgdaSymbol{→}%
\>[13]\AgdaFunction{executeStackEquality}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaPostulate{pbkh}\AgdaSpace{}%
\AgdaOperator{\AgdaInductiveConstructor{∷}}\AgdaSpace{}%
\AgdaBound{stack₃}\AgdaSymbol{)}%
\>[52]\AgdaOperator{\AgdaFunction{>>=}}\<%
\\
%
\>[1]\AgdaSymbol{λ}\AgdaSpace{}%
\AgdaBound{stack₄}\AgdaSpace{}%
\AgdaSymbol{→}%
\>[13]\AgdaFunction{executeStackVerify}\AgdaSpace{}%
\AgdaBound{stack₄}%
\>[52]\AgdaOperator{\AgdaFunction{>>=}}\<%
\\
%
\>[1]\AgdaSymbol{λ}\AgdaSpace{}%
\AgdaBound{stack₅}\AgdaSpace{}%
\AgdaSymbol{→}%
\>[13]\AgdaFunction{executeStackCheckSig}\AgdaSpace{}%
\AgdaPostulate{msg₁}\AgdaSpace{}%
\AgdaBound{stack₅}\<%
\end{code}
} % END newcommand

\AgdaHide{
\begin{code}%
\>[0]\<%
\\
%
\\[\AgdaEmptyExtraSkip]%
\>[0]\AgdaFunction{testP2PKHscript2UsingMoreSpaceUsingDo}\AgdaSpace{}%
\AgdaSymbol{=}\<%
\\
\>[0]\AgdaComment{--\ \textbackslash{}stackVerificationPtoPKHsymbolicExecutiontestPtoPKHscripttwoUsingDo}\<%
\end{code}
} % END AgdaHide

\newcommand{\stackVerificationPtoPKHsymbolicExecutiontestPtoPKHscripttwoUsingDo}{
\begin{code}%
\>[0][@{}l@{\AgdaIndent{1}}]%
\>[1]\AgdaKeyword{do}%
\>[5]\AgdaBound{stack₂}\AgdaSpace{}%
\AgdaOperator{\AgdaFunction{←}}\AgdaSpace{}%
\AgdaFunction{executeStackDup}\AgdaSpace{}%
\AgdaPostulate{stack₁}\<%
\\
%
\>[5]\AgdaBound{stack₃}\AgdaSpace{}%
\AgdaOperator{\AgdaFunction{←}}\AgdaSpace{}%
\AgdaFunction{executeOpHash}\AgdaSpace{}%
\AgdaBound{stack₂}\<%
\\
%
\>[5]\AgdaBound{stack₄}\AgdaSpace{}%
\AgdaOperator{\AgdaFunction{←}}\AgdaSpace{}%
\AgdaFunction{executeStackEquality}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaPostulate{pbkh}\AgdaSpace{}%
\AgdaOperator{\AgdaInductiveConstructor{∷}}\AgdaSpace{}%
\AgdaBound{stack₃}\AgdaSymbol{)}\<%
\\
%
\>[5]\AgdaBound{stack₅}\AgdaSpace{}%
\AgdaOperator{\AgdaFunction{←}}\AgdaSpace{}%
\AgdaFunction{executeStackVerify}\AgdaSpace{}%
\AgdaBound{stack₄}\<%
\\
%
\>[5]\AgdaFunction{executeStackCheckSig}\AgdaSpace{}%
\AgdaPostulate{msg₁}\AgdaSpace{}%
\AgdaBound{stack₅}\<%
\end{code}
} % END newcommand

\AgdaHide{
\begin{code}%
\>[0]\<%
\\
%
\\[\AgdaEmptyExtraSkip]%
\>[0]\AgdaComment{\{-\ in\ imperative\ programming\ we\ would\ write}\<%
\\
\>[0]\<%
\\
\>[0]\AgdaComment{\ \ \ stack₂\ :=\ executeStackDup\ stack₁;}\<%
\\
\>[0]\AgdaComment{\ \ \ stack₃\ :=\ executeOpHash\ stack₂;}\<%
\\
\>[0]\AgdaComment{\ \ \ stack₄\ :=\ executeStackEquality\ (pbkh\ ∷\ stack₃);}\<%
\\
\>[0]\AgdaComment{\ \ \ stack₅\ :=\ executeStackVerify\ stack₄;}\<%
\\
\>[0]\AgdaComment{\ \ \ executeStackCheckSig\ msg₁\ stack₅;}\<%
\\
\>[0]\<%
\\
\>[0]\AgdaComment{-\}}\<%
\\
%
\\[\AgdaEmptyExtraSkip]%
%
\\[\AgdaEmptyExtraSkip]%
%
\\[\AgdaEmptyExtraSkip]%
%
\\[\AgdaEmptyExtraSkip]%
%
\\[\AgdaEmptyExtraSkip]%
\>[0]\AgdaComment{\{-}\<%
\\
\>[0]\AgdaComment{If\ we\ execute\ the\ first\ line}\<%
\\
\>[0]\AgdaComment{(executeStackDup\ stack₁)}\<%
\\
\>[0]\<%
\\
\>[0]\AgdaComment{we\ see\ it\ will\ give}\<%
\\
\>[0]\AgdaComment{nothing\ if\ stack₁\ =\ []}\<%
\\
\>[0]\AgdaComment{just\ something\ if\ stack₁\ is\ nonempty}\<%
\\
\>[0]\<%
\\
\>[0]\AgdaComment{So\ let's\ check\ what\ happens\ if\ stack₁\ =\ []}\<%
\\
\>[0]\AgdaComment{-\}}\<%
\\
%
\\[\AgdaEmptyExtraSkip]%
%
\\[\AgdaEmptyExtraSkip]%
\>[0]\AgdaFunction{testP2PKHscriptEmpty}\AgdaSpace{}%
\AgdaSymbol{:}\AgdaSpace{}%
\AgdaDatatype{Maybe}\AgdaSpace{}%
\AgdaFunction{Stack}\<%
\\
\>[0]\AgdaFunction{testP2PKHscriptEmpty}\AgdaSpace{}%
\AgdaSymbol{=}\<%
\\
\>[0]\AgdaComment{--\ \textbackslash{}stackVerificationPtoPKHsymbolicExecutionEmpty}\<%
\end{code}
} % END AgdaHide

\newcommand{\stackVerificationPtoPKHsymbolicExecutionEmpty}{
\begin{code}[inline]%
\>[0][@{}l@{\AgdaIndent{1}}]%
\>[1]\AgdaOperator{\AgdaFunction{⟦}}\AgdaSpace{}%
\AgdaFunction{scriptP2PKHᵇ}\AgdaSpace{}%
\AgdaPostulate{pbkh}\AgdaSpace{}%
\AgdaOperator{\AgdaFunction{⟧ˢ}}\AgdaSpace{}%
\AgdaPostulate{time₁}\AgdaSpace{}%
\AgdaPostulate{msg₁}\AgdaSpace{}%
\AgdaInductiveConstructor{[]}\<%
\end{code}
} % END newcommand

\AgdaHide{
\begin{code}%
\>[0]\<%
\\
%
\\[\AgdaEmptyExtraSkip]%
\>[0]\AgdaComment{--⟦\ scriptP2PKHᵇ\ pbkh\ ⟧ˢ\ time₁\ msg₁\ []}\<%
\\
%
\\[\AgdaEmptyExtraSkip]%
%
\\[\AgdaEmptyExtraSkip]%
%
\\[\AgdaEmptyExtraSkip]%
\>[0]\AgdaComment{\{-\ if\ we\ evaluate\ it\ we\ get:}\<%
\\
\>[0]\<%
\\
\>[0]\AgdaComment{nothing}\<%
\\
\>[0]\<%
\\
\>[0]\AgdaComment{So\ now\ get\ the\ first\ (trivial)\ theorem}\<%
\\
\>[0]\AgdaComment{(without\ the\ postulated\ parameters)}\<%
\\
\>[0]\AgdaComment{-\}}\<%
\\
%
\\[\AgdaEmptyExtraSkip]%
\>[0]\<%
\end{code}
} % END AgdaHide

\newcommand{\stackVerificationPtoPKHsymbolicExecutionnothing}{
\begin{code}%
\>[0]\AgdaFunction{stackfunP2PKHemptyIsNothing}\AgdaSpace{}%
\AgdaSymbol{:}%
\>[224I]\AgdaSymbol{(}\AgdaBound{pubKeyHash}\AgdaSpace{}%
\AgdaSymbol{:}\AgdaSpace{}%
\AgdaDatatype{ℕ}\AgdaSymbol{)(}\AgdaBound{time₁}\AgdaSpace{}%
\AgdaSymbol{:}\AgdaSpace{}%
\AgdaFunction{Time}\AgdaSymbol{)(}\AgdaBound{msg₁}\AgdaSpace{}%
\AgdaSymbol{:}\AgdaSpace{}%
\AgdaDatatype{Msg}\AgdaSymbol{)}\<%
\\
\>[.][@{}l@{}]\<[224I]%
\>[30]\AgdaSymbol{→}\AgdaSpace{}%
\AgdaOperator{\AgdaFunction{⟦}}\AgdaSpace{}%
\AgdaFunction{scriptP2PKHᵇ}\AgdaSpace{}%
\AgdaBound{pubKeyHash}\AgdaSpace{}%
\AgdaOperator{\AgdaFunction{⟧ˢ}}\AgdaSpace{}%
\AgdaBound{time₁}\AgdaSpace{}%
\AgdaBound{msg₁}\AgdaSpace{}%
\AgdaInductiveConstructor{[]}\AgdaSpace{}%
\AgdaOperator{\AgdaDatatype{≡}}\AgdaSpace{}%
\AgdaInductiveConstructor{nothing}\<%
\\
\>[0]\AgdaFunction{stackfunP2PKHemptyIsNothing}\AgdaSpace{}%
\AgdaBound{pubKeyHash}\AgdaSpace{}%
\AgdaBound{time₁}\AgdaSpace{}%
\AgdaBound{msg₁}\AgdaSpace{}%
\AgdaSymbol{=}\AgdaSpace{}%
\AgdaInductiveConstructor{refl}\<%
\end{code}
} % END newcommand

\AgdaHide{
\begin{code}%
\>[0]\<%
\\
%
\\[\AgdaEmptyExtraSkip]%
%
\\[\AgdaEmptyExtraSkip]%
\>[0]\AgdaComment{\{-\ Now\ we\ look\ at\ what\ happens\ if\ the\ stack\ is\ non\ empty}\<%
\\
\>[0]\<%
\\
\>[0]\AgdaComment{lets\ a\ test\ for\ symbolic\ execution\ -\}}\<%
\\
%
\\[\AgdaEmptyExtraSkip]%
%
\\[\AgdaEmptyExtraSkip]%
\>[0]\AgdaFunction{teststackfunP2PKHNonEmptyStack}\AgdaSpace{}%
\AgdaSymbol{:}%
\>[34]\AgdaDatatype{Maybe}\AgdaSpace{}%
\AgdaFunction{Stack}\<%
\\
\>[0]\AgdaFunction{teststackfunP2PKHNonEmptyStack}\AgdaSpace{}%
\AgdaSymbol{=}\<%
\\
\>[0]\AgdaComment{--\ \textbackslash{}stackVerificationPtoPKHsymbolicExecutionnonestack}\<%
\end{code}
} % END AgdaHide

\newcommand{\stackVerificationPtoPKHsymbolicExecutionnonestack}{
\begin{code}[inline]%
\>[0][@{}l@{\AgdaIndent{1}}]%
\>[2]\AgdaOperator{\AgdaFunction{⟦}}\AgdaSpace{}%
\AgdaFunction{scriptP2PKHᵇ}\AgdaSpace{}%
\AgdaPostulate{pbkh}\AgdaSpace{}%
\AgdaOperator{\AgdaFunction{⟧ˢ}}\AgdaSpace{}%
\AgdaPostulate{time₁}\AgdaSpace{}%
\AgdaPostulate{msg₁}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaPostulate{pbk}\AgdaSpace{}%
\AgdaOperator{\AgdaInductiveConstructor{∷}}\AgdaSpace{}%
\AgdaPostulate{stack₁}\AgdaSymbol{)}\<%
\end{code}
} % END newcommand

\AgdaHide{
\begin{code}%
\>[0]\<%
\\
\>[0]\AgdaComment{\{-\ If\ we\ compute\ it\ we\ get}\<%
\\
\>[0]\AgdaComment{executeStackVerify\ (compareNaturals\ pbkh\ (param\ .hash\ pbk)\ ∷\ pbk\ ∷\ stack₁)}\<%
\\
\>[0]\AgdaComment{>>=\ (λ\ stack₂\ →\ executeStackCheckSig\ msg₁\ stack₂)}\<%
\\
\>[0]\<%
\\
\>[0]\AgdaComment{--\ older\ version\ was}\<%
\\
\>[0]\AgdaComment{lift2Maybe\ (λ\ stack₂\ →\ executeStackCheckSig\ msg₁\ stack₂)}\<%
\\
\>[0]\AgdaComment{(executeStackVerify}\<%
\\
\>[0]\AgdaComment{\ (compareNaturals\ pbkh\ (hashFun\ pbk)\ ∷\ pbk\ ∷\ stack₁))}\<%
\\
\>[0]\AgdaComment{-\}}\<%
\\
%
\\[\AgdaEmptyExtraSkip]%
\>[0]\AgdaFunction{stackfunP2PKHNonEmptyStackNormalForm}\AgdaSpace{}%
\AgdaSymbol{:}%
\>[40]\AgdaDatatype{Maybe}\AgdaSpace{}%
\AgdaFunction{Stack}\<%
\\
\>[0]\AgdaFunction{stackfunP2PKHNonEmptyStackNormalForm}\AgdaSpace{}%
\AgdaSymbol{=}\<%
\\
\>[0]\AgdaComment{--\ \textbackslash{}stackVerificationPtoPKHsymbolicExecutionNonEmptyStackNormalForm}\<%
\end{code}
} % END AgdaHide

\newcommand{\stackVerificationPtoPKHsymbolicExecutionNonEmptyStackNormalForm}{
\begin{code}%
\>[0][@{}l@{\AgdaIndent{1}}]%
\>[1]\AgdaFunction{executeStackVerify}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaFunction{compareNaturals}\AgdaSpace{}%
\AgdaPostulate{pbkh}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaFunction{hashFun}\AgdaSpace{}%
\AgdaPostulate{pbk}\AgdaSymbol{)}\AgdaSpace{}%
\AgdaOperator{\AgdaInductiveConstructor{∷}}\AgdaSpace{}%
\AgdaPostulate{pbk}\AgdaSpace{}%
\AgdaOperator{\AgdaInductiveConstructor{∷}}\AgdaSpace{}%
\AgdaPostulate{stack₁}\AgdaSymbol{)}\AgdaSpace{}%
\AgdaOperator{\AgdaFunction{>>=}}\<%
\\
%
\>[1]\AgdaFunction{executeStackCheckSig}\AgdaSpace{}%
\AgdaPostulate{msg₁}\<%
\end{code}
} % END newcommand

\AgdaHide{
\begin{code}%
\>[0]\<%
\\
\>[0]\AgdaFunction{stackfunP2PKHNonEmptyStackNormalFormDo}\AgdaSpace{}%
\AgdaSymbol{:}%
\>[42]\AgdaDatatype{Maybe}\AgdaSpace{}%
\AgdaFunction{Stack}\<%
\\
\>[0]\AgdaFunction{stackfunP2PKHNonEmptyStackNormalFormDo}\AgdaSpace{}%
\AgdaSymbol{=}\<%
\\
\>[0]\AgdaComment{--\ \textbackslash{}stackVerificationPtoPKHsymbolicExecutionNonEmptyStackNormalForm}\<%
\end{code}
} % END AgdaHide

\newcommand{\stackVerificationPtoPKHsymbolicExecutionNonEmptyStackNormalFormUsingDo}{
\begin{code}%
\>[0][@{}l@{\AgdaIndent{1}}]%
\>[1]\AgdaKeyword{do}%
\>[6]\AgdaBound{stack₅}\AgdaSpace{}%
\AgdaOperator{\AgdaFunction{←}}\AgdaSpace{}%
\AgdaFunction{executeStackVerify}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaFunction{compareNaturals}\AgdaSpace{}%
\AgdaPostulate{pbkh}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaFunction{hashFun}\AgdaSpace{}%
\AgdaPostulate{pbk}\AgdaSymbol{)}\AgdaSpace{}%
\AgdaOperator{\AgdaInductiveConstructor{∷}}\AgdaSpace{}%
\AgdaPostulate{pbk}\AgdaSpace{}%
\AgdaOperator{\AgdaInductiveConstructor{∷}}\AgdaSpace{}%
\AgdaPostulate{stack₁}\AgdaSymbol{)}\<%
\\
%
\>[6]\AgdaFunction{executeStackCheckSig}\AgdaSpace{}%
\AgdaPostulate{msg₁}\AgdaSpace{}%
\AgdaBound{stack₅}\<%
\end{code}
} % END newcommand

\AgdaHide{
\begin{code}%
\>[0]\<%
\\
%
\\[\AgdaEmptyExtraSkip]%
%
\\[\AgdaEmptyExtraSkip]%
%
\\[\AgdaEmptyExtraSkip]%
\>[0]\AgdaFunction{stackfunP2PKHNonEmptyStackNormalFormFirstPart}\AgdaSpace{}%
\AgdaSymbol{:}%
\>[49]\AgdaDatatype{Maybe}\AgdaSpace{}%
\AgdaFunction{Stack}\<%
\\
\>[0]\AgdaFunction{stackfunP2PKHNonEmptyStackNormalFormFirstPart}\AgdaSpace{}%
\AgdaSymbol{=}\<%
\\
\>[0]\AgdaComment{--\ \textbackslash{}stackVerificationPtoPKHsymbolicExecutionNonEmptyStackNormalFormFirstPart}\<%
\end{code}
} % END AgdaHide

\newcommand{\stackVerificationPtoPKHsymbolicExecutionNonEmptyStackNormalFormFirstPart}{
\begin{code}[inline]%
\>[0][@{}l@{\AgdaIndent{1}}]%
\>[1]\AgdaFunction{executeStackVerify}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaFunction{compareNaturals}\AgdaSpace{}%
\AgdaPostulate{pbkh}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaFunction{hashFun}\AgdaSpace{}%
\AgdaPostulate{pbk}\AgdaSymbol{)}\AgdaSpace{}%
\AgdaOperator{\AgdaInductiveConstructor{∷}}\AgdaSpace{}%
\AgdaPostulate{pbk}\AgdaSpace{}%
\AgdaOperator{\AgdaInductiveConstructor{∷}}\AgdaSpace{}%
\AgdaPostulate{stack₁}\AgdaSymbol{)}\<%
\end{code}
} % END newcommand

\AgdaHide{
\begin{code}%
\>[0]\<%
\\
\>[0]\AgdaFunction{stackfunP2PKHNonEmptyStackNormalFormFirstPartZoomedIn}\AgdaSpace{}%
\AgdaSymbol{:}%
\>[57]\AgdaDatatype{ℕ}\<%
\\
\>[0]\AgdaFunction{stackfunP2PKHNonEmptyStackNormalFormFirstPartZoomedIn}\AgdaSpace{}%
\AgdaSymbol{=}\<%
\\
\>[0]\AgdaComment{--\ \textbackslash{}stackVerificationPtoPKHsymbolicExecutionNonEmptyStackNormalFormFirstPartZoomedIn}\<%
\end{code}
} % END AgdaHide

\newcommand{\stackVerificationPtoPKHsymbolicExecutionNonEmptyStackNormalFormFirstPartZoomedIn}{
\begin{code}[inline]%
\>[0][@{}l@{\AgdaIndent{1}}]%
\>[1]\AgdaFunction{compareNaturals}\AgdaSpace{}%
\AgdaPostulate{pbkh}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaFunction{hashFun}\AgdaSpace{}%
\AgdaPostulate{pbk}\AgdaSymbol{)}\<%
\end{code}
} % END newcommand

\AgdaHide{
\begin{code}%
\>[0]\<%
\\
%
\\[\AgdaEmptyExtraSkip]%
%
\\[\AgdaEmptyExtraSkip]%
%
\\[\AgdaEmptyExtraSkip]%
\>[0]\AgdaComment{\{-}\<%
\\
\>[0]\AgdaComment{We\ see\ that}\<%
\\
\>[0]\<%
\\
\>[0]\AgdaComment{(λ\ stack₂\ →\ executeStackCheckSig\ msg₁\ stack₂)\ =\ executeStackCheckSig\ msg₁}\<%
\\
\>[0]\<%
\\
\>[0]\AgdaComment{and\ can\ therefore\ use}\<%
\\
\>[0]\<%
\\
\>[0]\AgdaComment{executeStackVerify\ (compareNaturals\ pbkh\ (param\ .hash\ pbk)\ ∷\ pbk\ ∷\ stack₁)}\<%
\\
\>[0]\AgdaComment{>>=\ executeStackCheckSig\ msg₁}\<%
\\
\>[0]\<%
\\
\>[0]\AgdaComment{--\ older\ version}\<%
\\
\>[0]\AgdaComment{lift2Maybe\ (executeStackCheckSig\ msg₁)}\<%
\\
\>[0]\AgdaComment{(executeStackVerify}\<%
\\
\>[0]\AgdaComment{\ (compareNaturals\ pbkh\ (hashFun\ pbk)\ ∷\ pbk\ ∷\ stack₁))}\<%
\\
\>[0]\<%
\\
\>[0]\AgdaComment{\ -\}}\<%
\\
%
\\[\AgdaEmptyExtraSkip]%
%
\\[\AgdaEmptyExtraSkip]%
\>[0]\<%
\end{code}
} % END AgdaHide

\newcommand{\stackVerificationPtoPKHsymbolicExecutionstackempty}{
\begin{code}%
\>[0]\AgdaFunction{stackfunP2PKHNonEmptyStack}\AgdaSpace{}%
\AgdaSymbol{:}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaBound{pubKeyHash}\AgdaSpace{}%
\AgdaSymbol{:}\AgdaSpace{}%
\AgdaDatatype{ℕ}\AgdaSymbol{)(}\AgdaBound{msg₁}\AgdaSpace{}%
\AgdaSymbol{:}\AgdaSpace{}%
\AgdaDatatype{Msg}\AgdaSymbol{)(}\AgdaBound{pbk}\AgdaSpace{}%
\AgdaSymbol{:}\AgdaSpace{}%
\AgdaDatatype{ℕ}\AgdaSymbol{)(}\AgdaBound{stack₂}\AgdaSpace{}%
\AgdaSymbol{:}\AgdaSpace{}%
\AgdaFunction{Stack}\AgdaSymbol{)}\AgdaSpace{}%
\AgdaSymbol{→}\AgdaSpace{}%
\AgdaDatatype{Maybe}\AgdaSpace{}%
\AgdaFunction{Stack}\<%
\\
\>[0]\AgdaFunction{stackfunP2PKHNonEmptyStack}\AgdaSpace{}%
\AgdaBound{pubKeyHash}\AgdaSpace{}%
\AgdaBound{msg₁}\AgdaSpace{}%
\AgdaBound{pbk}\AgdaSpace{}%
\AgdaBound{stack₂}\<%
\\
\>[0][@{}l@{\AgdaIndent{0}}]%
\>[14]\AgdaSymbol{=}%
\>[317I]\AgdaFunction{executeStackVerify}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaFunction{compareNaturals}\AgdaSpace{}%
\AgdaBound{pubKeyHash}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaFunction{hashFun}\AgdaSpace{}%
\AgdaBound{pbk}\AgdaSymbol{)}\AgdaSpace{}%
\AgdaOperator{\AgdaInductiveConstructor{∷}}\AgdaSpace{}%
\AgdaBound{pbk}\AgdaSpace{}%
\AgdaOperator{\AgdaInductiveConstructor{∷}}\AgdaSpace{}%
\AgdaBound{stack₂}\AgdaSymbol{)}\<%
\\
\>[317I][@{}l@{\AgdaIndent{0}}]%
\>[17]\AgdaOperator{\AgdaFunction{>>=}}\AgdaSpace{}%
\AgdaFunction{executeStackCheckSig}\AgdaSpace{}%
\AgdaBound{msg₁}\<%
\\
%
\\[\AgdaEmptyExtraSkip]%
\>[0]\<%
\end{code}
} % END newcommand

\AgdaHide{
\begin{code}%
\>[0]\<%
\\
\>[0]\AgdaComment{\{-}\<%
\\
\>[0]\AgdaComment{and\ check\ that\ this\ is\ correct}\<%
\\
\>[0]\AgdaComment{-\}}\<%
\\
%
\\[\AgdaEmptyExtraSkip]%
\>[0]\AgdaFunction{stackfunP2PKHemptyNonEmptyStackCorrect}\AgdaSpace{}%
\AgdaSymbol{:}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaBound{pubKeyHash}\AgdaSpace{}%
\AgdaSymbol{:}\AgdaSpace{}%
\AgdaDatatype{ℕ}\AgdaSymbol{)(}\AgdaBound{time₁}\AgdaSpace{}%
\AgdaSymbol{:}\AgdaSpace{}%
\AgdaFunction{Time}\AgdaSymbol{)(}\AgdaBound{msg₁}\AgdaSpace{}%
\AgdaSymbol{:}\AgdaSpace{}%
\AgdaDatatype{Msg}\AgdaSymbol{)(}\AgdaBound{pbk}\AgdaSpace{}%
\AgdaSymbol{:}\AgdaSpace{}%
\AgdaDatatype{ℕ}\AgdaSymbol{)(}\AgdaBound{stack₂}\AgdaSpace{}%
\AgdaSymbol{:}\AgdaSpace{}%
\AgdaFunction{Stack}\AgdaSymbol{)}\<%
\\
\>[0][@{}l@{\AgdaIndent{0}}]%
\>[8]\AgdaSymbol{→}\AgdaSpace{}%
\AgdaOperator{\AgdaFunction{⟦}}\AgdaSpace{}%
\AgdaFunction{scriptP2PKHᵇ}\AgdaSpace{}%
\AgdaBound{pubKeyHash}%
\>[37]\AgdaOperator{\AgdaFunction{⟧ˢ}}\AgdaSpace{}%
\AgdaBound{time₁}\AgdaSpace{}%
\AgdaBound{msg₁}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaBound{pbk}\AgdaSpace{}%
\AgdaOperator{\AgdaInductiveConstructor{∷}}\AgdaSpace{}%
\AgdaBound{stack₂}\AgdaSymbol{)}\AgdaSpace{}%
\AgdaOperator{\AgdaDatatype{≡}}\AgdaSpace{}%
\AgdaFunction{stackfunP2PKHNonEmptyStack}\AgdaSpace{}%
\AgdaBound{pubKeyHash}\AgdaSpace{}%
\AgdaBound{msg₁}%
\>[112]\AgdaBound{pbk}\AgdaSpace{}%
\AgdaBound{stack₂}\<%
\\
\>[0]\AgdaFunction{stackfunP2PKHemptyNonEmptyStackCorrect}\AgdaSpace{}%
\AgdaBound{pubKeyHash}\AgdaSpace{}%
\AgdaBound{time₁}\AgdaSpace{}%
\AgdaBound{msg₁}\AgdaSpace{}%
\AgdaBound{pbk}\AgdaSpace{}%
\AgdaBound{stack₂}\AgdaSpace{}%
\AgdaSymbol{=}\AgdaSpace{}%
\AgdaInductiveConstructor{refl}\<%
\\
%
\\[\AgdaEmptyExtraSkip]%
%
\\[\AgdaEmptyExtraSkip]%
%
\\[\AgdaEmptyExtraSkip]%
\>[0]\AgdaComment{\{-\ We\ see\ now\ the\ case\ distinction\ depends\ on}\<%
\\
\>[0]\AgdaComment{\ \ \ compres\ :=\ compareNaturals\ pbkh\ (hashFun\ pbk)}\<%
\\
\>[0]\<%
\\
\>[0]\AgdaComment{since}\<%
\\
\>[0]\<%
\\
\>[0]\AgdaComment{executeStackVerify\ \ \ \ (compres\ ∷\ \ pbk\ ∷\ stack₁)}\<%
\\
\>[0]\<%
\\
\>[0]\AgdaComment{will\ depend\ on\ whether\ compres\ is\ 0\ or\ \ suc\ x'}\<%
\\
\>[0]\<%
\\
\>[0]\AgdaComment{so\ we\ abstract\ from}\<%
\\
\>[0]\<%
\\
\>[0]\AgdaComment{compres\ =\ compareNaturals\ pubKeyHash\ (hashFun\ pbk)}\<%
\\
\>[0]\<%
\\
\>[0]\AgdaComment{-\}}\<%
\\
%
\\[\AgdaEmptyExtraSkip]%
\>[0]\AgdaComment{--\ This\ function\ will\ be\ repeated\ in\ stackVerificationP2PKHextractedProgram.agda}\<%
\\
\>[0]\AgdaComment{--\ and\ therefore\ is\ kept\ private\ in\ this\ section\ in\ order\ to\ avoid\ a\ conflict}\<%
\\
\>[0]\AgdaComment{--\ \textbackslash{}stackVerificationPtoPKHsymbolicExecutionabstract}\<%
\end{code}
} % END AgdaHide

\newcommand{\stackVerificationPtoPKHsymbolicExecutionabstract}{
\begin{code}%
\>[0]\AgdaFunction{p2PKHNonEmptyStackAbstr'}\AgdaSpace{}%
\AgdaSymbol{:}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaBound{msg₁}\AgdaSpace{}%
\AgdaSymbol{:}\AgdaSpace{}%
\AgdaDatatype{Msg}\AgdaSymbol{)(}\AgdaBound{pbk}\AgdaSpace{}%
\AgdaSymbol{:}\AgdaSpace{}%
\AgdaDatatype{ℕ}\AgdaSymbol{)(}\AgdaBound{stack₁}\AgdaSpace{}%
\AgdaSymbol{:}\AgdaSpace{}%
\AgdaFunction{Stack}\AgdaSymbol{)(}\AgdaBound{cmp}\AgdaSpace{}%
\AgdaSymbol{:}\AgdaSpace{}%
\AgdaDatatype{ℕ}\AgdaSymbol{)}\AgdaSpace{}%
\AgdaSymbol{→}\AgdaSpace{}%
\AgdaDatatype{Maybe}\AgdaSpace{}%
\AgdaFunction{Stack}\<%
\\
\>[0]\AgdaFunction{p2PKHNonEmptyStackAbstr'}\AgdaSpace{}%
\AgdaBound{msg₁}\AgdaSpace{}%
\AgdaBound{pbk}\AgdaSpace{}%
\AgdaBound{stack₁}\AgdaSpace{}%
\AgdaBound{cmp}\AgdaSpace{}%
\AgdaSymbol{=}%
\>[48]\AgdaFunction{executeStackVerify}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaBound{cmp}\AgdaSpace{}%
\AgdaOperator{\AgdaInductiveConstructor{∷}}%
\>[75]\AgdaBound{pbk}\AgdaSpace{}%
\AgdaOperator{\AgdaInductiveConstructor{∷}}\AgdaSpace{}%
\AgdaBound{stack₁}\AgdaSymbol{)}\AgdaSpace{}%
\AgdaOperator{\AgdaFunction{>>=}}\<%
\\
%
\>[48]\AgdaFunction{executeStackCheckSig}\AgdaSpace{}%
\AgdaBound{msg₁}\<%
\end{code}
} % END newcommand

\AgdaHide{
\begin{code}%
\>[0]\<%
\\
\>[0]\AgdaComment{--\ \textbackslash{}stackVerificationPtoPKHsymbolicExecutionabstract}\<%
\end{code}
} % END AgdaHide

\newcommand{\stackVerificationPtoPKHsymbolicExecutionabstractUsingVar}{
\begin{code}%
\>[0]\AgdaFunction{abstrFun}\AgdaSpace{}%
\AgdaSymbol{:}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaBound{stack₁}\AgdaSpace{}%
\AgdaSymbol{:}\AgdaSpace{}%
\AgdaFunction{Stack}\AgdaSymbol{)(}\AgdaBound{cmp}\AgdaSpace{}%
\AgdaSymbol{:}\AgdaSpace{}%
\AgdaDatatype{ℕ}\AgdaSymbol{)}\AgdaSpace{}%
\AgdaSymbol{→}\AgdaSpace{}%
\AgdaDatatype{Maybe}\AgdaSpace{}%
\AgdaFunction{Stack}\<%
\\
\>[0]\AgdaFunction{abstrFun}\AgdaSpace{}%
\AgdaBound{stack₁}\AgdaSpace{}%
\AgdaBound{cmp}\AgdaSpace{}%
\AgdaSymbol{=}%
\>[23]\AgdaKeyword{do}%
\>[27]\AgdaBound{stack₅}\AgdaSpace{}%
\AgdaOperator{\AgdaFunction{←}}\AgdaSpace{}%
\AgdaFunction{executeStackVerify}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaBound{cmp}\AgdaSpace{}%
\AgdaOperator{\AgdaInductiveConstructor{∷}}%
\>[63]\AgdaPostulate{pbk}\AgdaSpace{}%
\AgdaOperator{\AgdaInductiveConstructor{∷}}\AgdaSpace{}%
\AgdaBound{stack₁}\AgdaSymbol{)}\<%
\\
%
\>[27]\AgdaFunction{executeStackCheckSig}\AgdaSpace{}%
\AgdaPostulate{msg₁}\AgdaSpace{}%
\AgdaBound{stack₅}\<%
\end{code}
} % END newcommand

\AgdaHide{
\begin{code}%
\>[0]\<%
\\
%
\\[\AgdaEmptyExtraSkip]%
%
\\[\AgdaEmptyExtraSkip]%
\>[0]\AgdaFunction{stackfunP2PKHNonEmptyStackNormalFormUsingAbstractedFun}\AgdaSpace{}%
\AgdaSymbol{:}\AgdaSpace{}%
\AgdaDatatype{Maybe}\AgdaSpace{}%
\AgdaFunction{Stack}\<%
\\
\>[0]\AgdaFunction{stackfunP2PKHNonEmptyStackNormalFormUsingAbstractedFun}\AgdaSpace{}%
\AgdaSymbol{=}\<%
\\
\>[0]\AgdaComment{--\ \textbackslash{}stackVerificationPtoPKHsymbolicExecutionnonEmptyStackNormalFormWithAbstractedFun}\<%
\end{code}
} % END AgdaHide

\newcommand{\stackVerificationPtoPKHsymbolicExecutionnonEmptyStackNormalFormWithAbstractedFun}{
\begin{code}[inline]%
\>[0][@{}l@{\AgdaIndent{1}}]%
\>[2]\AgdaFunction{abstrFun}\AgdaSpace{}%
\AgdaPostulate{stack₁}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaFunction{compareNaturals}\AgdaSpace{}%
\AgdaPostulate{pbkh}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaFunction{hashFun}\AgdaSpace{}%
\AgdaPostulate{pbk}\AgdaSymbol{))}\<%
\end{code}
} % END newcommand

\AgdaHide{
\begin{code}%
\>[0]\<%
\\
\>[0]\AgdaFunction{stackfunP2PKHNonEmptyStackNormalFormUsingAbstractedFunTest}\AgdaSpace{}%
\AgdaSymbol{:}\<%
\\
\>[0][@{}l@{\AgdaIndent{0}}]%
\>[4]\AgdaFunction{stackfunP2PKHNonEmptyStackNormalForm}\AgdaSpace{}%
\AgdaOperator{\AgdaDatatype{≡}}\AgdaSpace{}%
\AgdaFunction{stackfunP2PKHNonEmptyStackNormalFormUsingAbstractedFun}\<%
\\
\>[0]\AgdaFunction{stackfunP2PKHNonEmptyStackNormalFormUsingAbstractedFunTest}%
\>[60]\AgdaSymbol{=}\AgdaSpace{}%
\AgdaInductiveConstructor{refl}\<%
\\
%
\\[\AgdaEmptyExtraSkip]%
\>[0]\AgdaComment{\{-\ and\ we\ show\ that\ this\ is\ the\ right\ function}\<%
\\
\>[0]\AgdaComment{-\}}\<%
\\
%
\\[\AgdaEmptyExtraSkip]%
\>[0]\AgdaComment{--\ This\ function\ will\ be\ repeated\ in\ stackVerificationP2PKHextractedProgram.agda}\<%
\\
\>[0]\AgdaComment{--\ and\ therefore\ is\ kept\ private\ in\ this\ section\ in\ order\ to\ avoid\ a\ conflict}\<%
\\
\>[0]\AgdaKeyword{private}\<%
\\
\>[0][@{}l@{\AgdaIndent{0}}]%
\>[2]\AgdaFunction{stackfunP2PKHNonEmptyStackAbstractedCor}\AgdaSpace{}%
\AgdaSymbol{:}%
\>[45]\AgdaSymbol{(}\AgdaBound{pubKeyHash}\AgdaSpace{}%
\AgdaSymbol{:}\AgdaSpace{}%
\AgdaDatatype{ℕ}\AgdaSymbol{)(}\AgdaBound{time₁}\AgdaSpace{}%
\AgdaSymbol{:}\AgdaSpace{}%
\AgdaFunction{Time}\AgdaSymbol{)(}\AgdaBound{msg₁}\AgdaSpace{}%
\AgdaSymbol{:}\AgdaSpace{}%
\AgdaDatatype{Msg}\AgdaSymbol{)(}\AgdaBound{pbk}\AgdaSpace{}%
\AgdaSymbol{:}\AgdaSpace{}%
\AgdaDatatype{ℕ}\AgdaSymbol{)(}\AgdaBound{stack₂}\AgdaSpace{}%
\AgdaSymbol{:}\AgdaSpace{}%
\AgdaFunction{Stack}\AgdaSymbol{)}\<%
\\
\>[2][@{}l@{\AgdaIndent{0}}]%
\>[18]\AgdaSymbol{→}%
\>[428I]\AgdaOperator{\AgdaFunction{⟦}}\AgdaSpace{}%
\AgdaFunction{scriptP2PKHᵇ}\AgdaSpace{}%
\AgdaBound{pubKeyHash}\AgdaSpace{}%
\AgdaOperator{\AgdaFunction{⟧ˢ}}\AgdaSpace{}%
\AgdaBound{time₁}\AgdaSpace{}%
\AgdaBound{msg₁}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaBound{pbk}\AgdaSpace{}%
\AgdaOperator{\AgdaInductiveConstructor{∷}}\AgdaSpace{}%
\AgdaBound{stack₂}\AgdaSymbol{)}\<%
\\
\>[428I][@{}l@{\AgdaIndent{0}}]%
\>[21]\AgdaOperator{\AgdaDatatype{≡}}%
\>[437I]\AgdaFunction{p2PKHNonEmptyStackAbstr'}%
\>[49]\AgdaBound{msg₁}\AgdaSpace{}%
\AgdaBound{pbk}\AgdaSpace{}%
\AgdaBound{stack₂}\<%
\\
\>[437I][@{}l@{\AgdaIndent{0}}]%
\>[29]\AgdaSymbol{(}\AgdaFunction{compareNaturals}\AgdaSpace{}%
\AgdaBound{pubKeyHash}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaFunction{hashFun}\AgdaSpace{}%
\AgdaBound{pbk}\AgdaSymbol{))}\<%
\\
%
\>[2]\AgdaFunction{stackfunP2PKHNonEmptyStackAbstractedCor}\AgdaSpace{}%
\AgdaBound{pubKeyHash}\AgdaSpace{}%
\AgdaBound{time₁}\AgdaSpace{}%
\AgdaBound{msg₁}\AgdaSpace{}%
\AgdaBound{pbk}\AgdaSpace{}%
\AgdaBound{stack₂}\AgdaSpace{}%
\AgdaSymbol{=}\AgdaSpace{}%
\AgdaInductiveConstructor{refl}\<%
\\
%
\\[\AgdaEmptyExtraSkip]%
%
\\[\AgdaEmptyExtraSkip]%
\>[0]\AgdaComment{\{-\ Now\ we\ investigate\ what\ \ p2PKHNonEmptyStackAbstr'}\<%
\\
\>[0]\AgdaComment{When\ looking\ at\ it\ and\ see\ that}\<%
\\
\>[0]\<%
\\
\>[0]\AgdaComment{\ p2PKHNonEmptyStackAbstr'\ msg₁\ pbk\ stack₂\ cmp}\<%
\\
\>[0]\<%
\\
\>[0]\AgdaComment{will\ execute}\<%
\\
\>[0]\AgdaComment{executeStackVerify\ (cmp\ ∷\ \ pbk\ ∷\ stack₂)}\<%
\\
\>[0]\AgdaComment{which\ will\ in\ turn\ make\ a\ case\ disctintion\ on\ whether\ cmp\ is\ 0\ or\ \ not\ zero}\<%
\\
\>[0]\<%
\\
\>[0]\AgdaComment{(that\ corresponds\ to\ what\ the\ original\ function\ does\ because\ it\ makes\ this\ comparison}\<%
\\
\>[0]\AgdaComment{\ \ \ compareNaturals\ pubKeyHash\ (hashFun\ pbk)}\<%
\\
\>[0]\AgdaComment{\ \ which\ checks\ \ whether\ the\ pbk\ provided\ \ by\ the\ user\ hashes\ to\ the\ pubKeyHash\ of\ the\ locking\ script}\<%
\\
\>[0]\AgdaComment{\ \ \ \ if\ it\ \ is\ 0\ it\ should\ fail,\ and\ if\ it\ is\ 1\ it\ should\ succeed.}\<%
\\
\>[0]\<%
\\
\>[0]\AgdaComment{So\ lets\ make\ the\ test}\<%
\\
\>[0]\AgdaComment{-\}}\<%
\\
%
\\[\AgdaEmptyExtraSkip]%
\>[0]\AgdaFunction{testStackfunP2PKHNonEmptyStackAbstractedCompre0}\AgdaSpace{}%
\AgdaSymbol{:}\AgdaSpace{}%
\AgdaDatatype{Maybe}\AgdaSpace{}%
\AgdaFunction{Stack}\<%
\\
\>[0]\AgdaFunction{testStackfunP2PKHNonEmptyStackAbstractedCompre0}\AgdaSpace{}%
\AgdaSymbol{=}\AgdaSpace{}%
\AgdaFunction{p2PKHNonEmptyStackAbstr'}\AgdaSpace{}%
\AgdaPostulate{msg₁}\AgdaSpace{}%
\AgdaPostulate{pbk}\AgdaSpace{}%
\AgdaPostulate{stack₁}\AgdaSpace{}%
\AgdaNumber{0}\<%
\\
%
\\[\AgdaEmptyExtraSkip]%
\>[0]\AgdaComment{\{-\ if\ we\ evaluate\ it\ we\ get}\<%
\\
\>[0]\<%
\\
\>[0]\AgdaComment{nothing}\<%
\\
\>[0]\AgdaComment{-\}}\<%
\\
%
\\[\AgdaEmptyExtraSkip]%
\>[0]\AgdaComment{--\ we\ evaluate\ now}\<%
\\
\>[0]\AgdaFunction{abstrFunZeroCase}\AgdaSpace{}%
\AgdaSymbol{:}\AgdaSpace{}%
\AgdaDatatype{Maybe}\AgdaSpace{}%
\AgdaFunction{Stack}\<%
\\
\>[0]\AgdaFunction{abstrFunZeroCase}\AgdaSpace{}%
\AgdaSymbol{=}\<%
\\
\>[0]\AgdaComment{--\ \textbackslash{}stackVerificationPtoPKHsymbolicExecutionabstrFunZeroCase}\<%
\end{code}
} % END AgdaHide

\newcommand{\stackVerificationPtoPKHsymbolicExecutionabstrFunZeroCase}{
\begin{code}[inline]%
\>[0][@{}l@{\AgdaIndent{1}}]%
\>[1]\AgdaFunction{abstrFun}\AgdaSpace{}%
\AgdaPostulate{stack₁}\AgdaSpace{}%
\AgdaNumber{0}\<%
\end{code}
} % END newcommand

\AgdaHide{
\begin{code}%
\>[0]\<%
\\
%
\\[\AgdaEmptyExtraSkip]%
\>[0]\AgdaComment{\{-}\<%
\\
\>[0]\<%
\\
\>[0]\AgdaComment{We\ \ show\ now\ this\ is\ always\ the\ case}\<%
\\
\>[0]\<%
\\
\>[0]\AgdaComment{-\}}\<%
\\
%
\\[\AgdaEmptyExtraSkip]%
\>[0]\AgdaComment{--\ This\ function\ will\ be\ repeated\ in\ stackVerificationP2PKHextractedProgram.agda}\<%
\\
\>[0]\AgdaComment{--\ and\ therefore\ is\ kept\ private\ in\ this\ section\ in\ order\ to\ avoid\ a\ conflict}\<%
\\
\>[0]\AgdaKeyword{private}\<%
\\
\>[0][@{}l@{\AgdaIndent{0}}]%
\>[2]\AgdaFunction{stackfunP2PKHNonEmptyStackAbstractedCorCompr0IsNothing}\AgdaSpace{}%
\AgdaSymbol{:}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaBound{msg₁}\AgdaSpace{}%
\AgdaSymbol{:}\AgdaSpace{}%
\AgdaDatatype{Msg}\AgdaSymbol{)(}\AgdaBound{pbk}\AgdaSpace{}%
\AgdaSymbol{:}\AgdaSpace{}%
\AgdaDatatype{ℕ}\AgdaSymbol{)(}\AgdaBound{stack₂}\AgdaSpace{}%
\AgdaSymbol{:}\AgdaSpace{}%
\AgdaFunction{Stack}\AgdaSymbol{)}\<%
\\
\>[2][@{}l@{\AgdaIndent{0}}]%
\>[8]\AgdaSymbol{→}%
\>[11]\AgdaFunction{p2PKHNonEmptyStackAbstr'}\AgdaSpace{}%
\AgdaBound{msg₁}\AgdaSpace{}%
\AgdaBound{pbk}\AgdaSpace{}%
\AgdaBound{stack₂}\AgdaSpace{}%
\AgdaNumber{0}\AgdaSpace{}%
\AgdaOperator{\AgdaDatatype{≡}}\AgdaSpace{}%
\AgdaInductiveConstructor{nothing}\<%
\\
%
\>[2]\AgdaFunction{stackfunP2PKHNonEmptyStackAbstractedCorCompr0IsNothing}\AgdaSpace{}%
\AgdaBound{msg₁}\AgdaSpace{}%
\AgdaBound{pbk}\AgdaSpace{}%
\AgdaBound{stack₂}\AgdaSpace{}%
\AgdaSymbol{=}\AgdaSpace{}%
\AgdaInductiveConstructor{refl}\<%
\\
%
\\[\AgdaEmptyExtraSkip]%
%
\\[\AgdaEmptyExtraSkip]%
\>[0]\AgdaComment{\{-\ Now\ we\ look\ at\ what\ happens\ \ if\ the\ value\ is\ non\ zero\ -\}}\<%
\\
%
\\[\AgdaEmptyExtraSkip]%
%
\\[\AgdaEmptyExtraSkip]%
\>[0]\AgdaFunction{testStackfunP2PKHNonEmptyStackAbstractedCompreSucCase}\AgdaSpace{}%
\AgdaSymbol{:}\AgdaSpace{}%
\AgdaDatatype{Maybe}\AgdaSpace{}%
\AgdaFunction{Stack}\<%
\\
\>[0]\AgdaFunction{testStackfunP2PKHNonEmptyStackAbstractedCompreSucCase}\AgdaSpace{}%
\AgdaSymbol{=}\AgdaSpace{}%
\AgdaFunction{p2PKHNonEmptyStackAbstr'}\AgdaSpace{}%
\AgdaPostulate{msg₁}\AgdaSpace{}%
\AgdaPostulate{pbk}\AgdaSpace{}%
\AgdaPostulate{stack₁}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaInductiveConstructor{suc}\AgdaSpace{}%
\AgdaPostulate{x₁}\AgdaSymbol{)}\<%
\\
%
\\[\AgdaEmptyExtraSkip]%
%
\\[\AgdaEmptyExtraSkip]%
\>[0]\AgdaComment{--\ We\ evaluate}\<%
\\
%
\\[\AgdaEmptyExtraSkip]%
\>[0]\AgdaComment{--\ we\ evaluate\ now}\<%
\\
\>[0]\AgdaFunction{abstrFunSucCase}\AgdaSpace{}%
\AgdaSymbol{:}\AgdaSpace{}%
\AgdaDatatype{Maybe}\AgdaSpace{}%
\AgdaFunction{Stack}\<%
\\
\>[0]\AgdaFunction{abstrFunSucCase}\AgdaSpace{}%
\AgdaSymbol{=}\<%
\\
\>[0]\AgdaComment{--\ \textbackslash{}stackVerificationPtoPKHsymbolicExecutionabstrFunSucCase}\<%
\end{code}
} % END AgdaHide

\newcommand{\stackVerificationPtoPKHsymbolicExecutionabstrFunSucCase}{
\begin{code}[inline]%
\>[0][@{}l@{\AgdaIndent{1}}]%
\>[1]\AgdaFunction{abstrFun}\AgdaSpace{}%
\AgdaPostulate{stack₁}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaInductiveConstructor{suc}\AgdaSpace{}%
\AgdaPostulate{x₁}\AgdaSymbol{)}\<%
\end{code}
} % END newcommand

\AgdaHide{
\begin{code}%
\>[0]\<%
\\
\>[0]\AgdaComment{--\ we\ obtain}\<%
\\
%
\\[\AgdaEmptyExtraSkip]%
\>[0]\AgdaFunction{abstrFunSucCaseNormal}\AgdaSpace{}%
\AgdaSymbol{:}\AgdaSpace{}%
\AgdaDatatype{Maybe}\AgdaSpace{}%
\AgdaFunction{Stack}\<%
\\
\>[0]\AgdaFunction{abstrFunSucCaseNormal}\AgdaSpace{}%
\AgdaSymbol{=}\<%
\\
\>[0]\AgdaComment{--\ \textbackslash{}stackVerificationPtoPKHsymbolicExecutionabstrFunSucCaseNormal}\<%
\end{code}
} % END AgdaHide

\newcommand{\stackVerificationPtoPKHsymbolicExecutionabstrFunSucCaseNormal}{
\begin{code}[inline]%
\>[0][@{}l@{\AgdaIndent{1}}]%
\>[1]\AgdaFunction{executeStackCheckSig}\AgdaSpace{}%
\AgdaPostulate{msg₁}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaPostulate{pbk}\AgdaSpace{}%
\AgdaOperator{\AgdaInductiveConstructor{∷}}\AgdaSpace{}%
\AgdaPostulate{stack₁}\AgdaSymbol{)}\<%
\end{code}
} % END newcommand

\AgdaHide{
\begin{code}%
\>[0]\<%
\\
\>[0]\AgdaComment{\{-}\<%
\\
\>[0]\AgdaComment{executeStackCheckSig\ msg₁\ (pbk\ ∷\ stack₁)}\<%
\\
\>[0]\AgdaComment{-\}}\<%
\\
%
\\[\AgdaEmptyExtraSkip]%
%
\\[\AgdaEmptyExtraSkip]%
\>[0]\AgdaComment{\{-\ if\ we\ evalute}\<%
\\
\>[0]\AgdaComment{\ \ \ \ \ testStackfunP2PKHNonEmptyStackAbstractedCompreSucCase}\<%
\\
\>[0]\AgdaComment{\ \ \ \ we\ get}\<%
\\
\>[0]\<%
\\
\>[0]\AgdaComment{executeStackCheckSig\ msg₁\ (pbk\ ∷\ stack₁)}\<%
\\
\>[0]\<%
\\
\>[0]\<%
\\
\>[0]\AgdaComment{This\ corresponds\ to\ the\ situation\ where}\<%
\\
\>[0]\AgdaComment{the\ original\ stack₁\ was\ non\ empty,\ and\ the\ comparision\ of\ the\ pbk\ with\ the\ pbkhash}\<%
\\
\>[0]\AgdaComment{got\ a\ result\ >\ 0}\<%
\\
\>[0]\<%
\\
\>[0]\<%
\\
\>[0]\<%
\\
\>[0]\AgdaComment{If\ we\ look\ at}\<%
\\
\>[0]\AgdaComment{executeStackCheckSig}\<%
\\
\>[0]\<%
\\
\>[0]\AgdaComment{we\ see\ that\ it\ gives\ nothing\ when\ the\ stack\ has\ height\ <\ 2}\<%
\\
\>[0]\AgdaComment{and\ otherwise\ does\ something,}\<%
\\
\>[0]\<%
\\
\>[0]\AgdaComment{so\ we\ can\ \ make\ a\ case\ distinction\ on\ whether\ in}\<%
\\
\>[0]\<%
\\
\>[0]\AgdaComment{p2PKHNonEmptyStackAbstr'\ msg₁\ pbk\ stack₁\ x}\<%
\\
\>[0]\<%
\\
\>[0]\AgdaComment{stack₁\ is\ []\ or\ nonempty}\<%
\\
\>[0]\<%
\\
\>[0]\AgdaComment{So\ lets\ look\ at\ the\ easy\ case\ []}\<%
\\
\>[0]\<%
\\
\>[0]\AgdaComment{\ \ \ \ -\}}\<%
\\
%
\\[\AgdaEmptyExtraSkip]%
%
\\[\AgdaEmptyExtraSkip]%
\>[0]\AgdaComment{--\ we\ evaluate\ now}\<%
\\
\>[0]\AgdaFunction{abstrFunSucCaseEmpty}\AgdaSpace{}%
\AgdaSymbol{:}\AgdaSpace{}%
\AgdaDatatype{Maybe}\AgdaSpace{}%
\AgdaFunction{Stack}\<%
\\
\>[0]\AgdaFunction{abstrFunSucCaseEmpty}\AgdaSpace{}%
\AgdaSymbol{=}\<%
\\
\>[0]\AgdaComment{--\ \textbackslash{}stackVerificationPtoPKHsymbolicExecutionabstrFunSucCaseEmpty}\<%
\end{code}
} % END AgdaHide

\newcommand{\stackVerificationPtoPKHsymbolicExecutionabstrFunSucCaseEmpty}{
\begin{code}[inline]%
\>[0][@{}l@{\AgdaIndent{1}}]%
\>[1]\AgdaFunction{abstrFun}\AgdaSpace{}%
\AgdaInductiveConstructor{[]}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaInductiveConstructor{suc}\AgdaSpace{}%
\AgdaPostulate{x₁}\AgdaSymbol{)}\<%
\end{code}
} % END newcommand

\AgdaHide{
\begin{code}%
\>[0]\<%
\\
\>[0]\AgdaComment{--\ and\ obtain\ nothing}\<%
\\
\>[0]\AgdaFunction{abstrFunSucCaseEmptyCheck}\AgdaSpace{}%
\AgdaSymbol{:}%
\>[29]\AgdaFunction{abstrFunSucCaseEmpty}\AgdaSpace{}%
\AgdaOperator{\AgdaDatatype{≡}}\AgdaSpace{}%
\AgdaInductiveConstructor{nothing}\<%
\\
\>[0]\AgdaFunction{abstrFunSucCaseEmptyCheck}\AgdaSpace{}%
\AgdaSymbol{=}\AgdaSpace{}%
\AgdaInductiveConstructor{refl}\<%
\\
%
\\[\AgdaEmptyExtraSkip]%
\>[0]\AgdaComment{--\ we\ evaluate\ now}\<%
\\
\>[0]\AgdaFunction{abstrFunSucCaseNonEmpty}\AgdaSpace{}%
\AgdaSymbol{:}\AgdaSpace{}%
\AgdaDatatype{Maybe}\AgdaSpace{}%
\AgdaFunction{Stack}\<%
\\
\>[0]\AgdaFunction{abstrFunSucCaseNonEmpty}\AgdaSpace{}%
\AgdaSymbol{=}\<%
\\
\>[0]\AgdaComment{--\ \textbackslash{}stackVerificationPtoPKHsymbolicExecutionabstrFunSucCaseNonEmpty}\<%
\end{code}
} % END AgdaHide

\newcommand{\stackVerificationPtoPKHsymbolicExecutionabstrFunSucCaseNonEmpty}{
\begin{code}[inline]%
\>[0][@{}l@{\AgdaIndent{1}}]%
\>[1]\AgdaFunction{abstrFun}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaPostulate{sig₁}\AgdaSpace{}%
\AgdaOperator{\AgdaInductiveConstructor{∷}}\AgdaSpace{}%
\AgdaPostulate{stack₁}\AgdaSymbol{)}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaInductiveConstructor{suc}\AgdaSpace{}%
\AgdaPostulate{x₁}\AgdaSymbol{)}\<%
\end{code}
} % END newcommand

\AgdaHide{
\begin{code}%
\>[0]\<%
\\
%
\\[\AgdaEmptyExtraSkip]%
\>[0]\AgdaFunction{abstrFunSucCaseNonEmptyNormal}\AgdaSpace{}%
\AgdaSymbol{:}\AgdaSpace{}%
\AgdaDatatype{Maybe}\AgdaSpace{}%
\AgdaFunction{Stack}\<%
\\
\>[0]\AgdaFunction{abstrFunSucCaseNonEmptyNormal}\AgdaSpace{}%
\AgdaSymbol{=}\<%
\\
\>[0]\AgdaComment{--\ \textbackslash{}stackVerificationPtoPKHsymbolicExecutionabstrFunSucCaseNonEmptyNormal}\<%
\end{code}
} % END AgdaHide

\newcommand{\stackVerificationPtoPKHsymbolicExecutionabstrFunSucCaseNonEmptyNormal}{
\begin{code}[inline]%
\>[0][@{}l@{\AgdaIndent{1}}]%
\>[1]\AgdaInductiveConstructor{just}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaFunction{boolToNat}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaFunction{isSigned}\AgdaSpace{}%
\AgdaPostulate{msg₁}\AgdaSpace{}%
\AgdaPostulate{sig₁}\AgdaSpace{}%
\AgdaPostulate{pbk}\AgdaSymbol{)}\AgdaSpace{}%
\AgdaOperator{\AgdaInductiveConstructor{∷}}\AgdaSpace{}%
\AgdaPostulate{stack₁}\AgdaSymbol{)}\<%
\end{code}
} % END newcommand

\AgdaHide{
\begin{code}%
\>[0]\<%
\\
\>[0]\AgdaFunction{abstrFunSucCaseNonEmptyCheck}\AgdaSpace{}%
\AgdaSymbol{:}\AgdaSpace{}%
\AgdaFunction{abstrFunSucCaseNonEmpty}\AgdaSpace{}%
\AgdaOperator{\AgdaDatatype{≡}}\AgdaSpace{}%
\AgdaFunction{abstrFunSucCaseNonEmptyNormal}\<%
\\
\>[0]\AgdaFunction{abstrFunSucCaseNonEmptyCheck}\AgdaSpace{}%
\AgdaSymbol{=}\AgdaSpace{}%
\AgdaInductiveConstructor{refl}\<%
\\
\>[0]\<%
\end{code}
} % END AgdaHide

\newcommand{\stackVerificationPtoPKHsymbolicExecutioneasycase}{
\begin{code}%
\>[0]\AgdaFunction{testStackfunP2PKHNonEmptyStackAbstractedCompreSucEmpty}\AgdaSpace{}%
\AgdaSymbol{:}\AgdaSpace{}%
\AgdaDatatype{Maybe}\AgdaSpace{}%
\AgdaFunction{Stack}\<%
\\
\>[0]\AgdaFunction{testStackfunP2PKHNonEmptyStackAbstractedCompreSucEmpty}\AgdaSpace{}%
\AgdaSymbol{=}\<%
\\
\>[0][@{}l@{\AgdaIndent{0}}]%
\>[27]\AgdaFunction{p2PKHNonEmptyStackAbstr'}\AgdaSpace{}%
\AgdaPostulate{msg₁}\AgdaSpace{}%
\AgdaPostulate{pbk}\AgdaSpace{}%
\AgdaInductiveConstructor{[]}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaInductiveConstructor{suc}\AgdaSpace{}%
\AgdaPostulate{x₁}\AgdaSymbol{)}\<%
\end{code}
} % END newcommand

\AgdaHide{
\begin{code}%
\>[0]\<%
\\
\>[0]\AgdaComment{\{-\ if\ we\ evaluate\ it\ we\ get\ \ result}\<%
\\
\>[0]\<%
\\
\>[0]\AgdaComment{nothing}\<%
\\
\>[0]\<%
\\
\>[0]\AgdaComment{we\ check\ that\ this\ always\ holds}\<%
\\
\>[0]\AgdaComment{-\}}\<%
\\
%
\\[\AgdaEmptyExtraSkip]%
%
\\[\AgdaEmptyExtraSkip]%
\>[0]\AgdaFunction{stackfunP2PKHNonEmptyStackAbstractedCorComprSucStackEmpty}\AgdaSpace{}%
\AgdaSymbol{:}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaBound{msg₁}\AgdaSpace{}%
\AgdaSymbol{:}\AgdaSpace{}%
\AgdaDatatype{Msg}\AgdaSymbol{)(}\AgdaBound{pbk}\AgdaSpace{}%
\AgdaSymbol{:}\AgdaSpace{}%
\AgdaDatatype{ℕ}\AgdaSymbol{)(}\AgdaBound{x}\AgdaSpace{}%
\AgdaSymbol{:}\AgdaSpace{}%
\AgdaDatatype{ℕ}\AgdaSymbol{)}\<%
\\
\>[0][@{}l@{\AgdaIndent{0}}]%
\>[13]\AgdaSymbol{→}\AgdaSpace{}%
\AgdaFunction{p2PKHNonEmptyStackAbstr'}\AgdaSpace{}%
\AgdaBound{msg₁}\AgdaSpace{}%
\AgdaBound{pbk}\AgdaSpace{}%
\AgdaInductiveConstructor{[]}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaInductiveConstructor{suc}\AgdaSpace{}%
\AgdaBound{x}\AgdaSymbol{)}\AgdaSpace{}%
\AgdaOperator{\AgdaDatatype{≡}}\AgdaSpace{}%
\AgdaInductiveConstructor{nothing}\<%
\\
\>[0]\AgdaFunction{stackfunP2PKHNonEmptyStackAbstractedCorComprSucStackEmpty}\AgdaSpace{}%
\AgdaBound{msg₁}\AgdaSpace{}%
\AgdaBound{pbk}\AgdaSpace{}%
\AgdaBound{x}%
\>[70]\AgdaSymbol{=}\AgdaSpace{}%
\AgdaInductiveConstructor{refl}\<%
\\
%
\\[\AgdaEmptyExtraSkip]%
\>[0]\AgdaComment{\{-\ \ Intermezzo:\ we\ can\ see\ that\ the\ fanction\ gives\ always\ nothing\ if\ the\ stack\ is\ empty}\<%
\\
\>[0]\AgdaComment{\ \ \ independent\ of\ the\ result}\<%
\\
\>[0]\<%
\\
\>[0]\AgdaComment{But\ this\ result\ is\ not\ really\ needed\ (so\ can\ be\ probably\ be\ ommitted\ in\ the\ paper)}\<%
\\
\>[0]\AgdaComment{\ \ \ -\}}\<%
\\
%
\\[\AgdaEmptyExtraSkip]%
\>[0]\AgdaComment{--\ This\ function\ will\ be\ repeated\ in\ stackVerificationP2PKHextractedProgram.agda}\<%
\\
\>[0]\AgdaComment{--\ and\ therefore\ is\ kept\ private\ in\ this\ section\ in\ order\ to\ avoid\ a\ conflict}\<%
\\
\>[0]\AgdaKeyword{private}\<%
\\
\>[0][@{}l@{\AgdaIndent{0}}]%
\>[2]\AgdaFunction{stackfunP2PKHNonEmptyStackAbstractedCorEmptysNothing}\AgdaSpace{}%
\AgdaSymbol{:}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaBound{msg₁}\AgdaSpace{}%
\AgdaSymbol{:}\AgdaSpace{}%
\AgdaDatatype{Msg}\AgdaSymbol{)(}\AgdaBound{pbk}\AgdaSpace{}%
\AgdaSymbol{:}\AgdaSpace{}%
\AgdaDatatype{ℕ}\AgdaSymbol{)(}\AgdaBound{x}\AgdaSpace{}%
\AgdaSymbol{:}\AgdaSpace{}%
\AgdaDatatype{ℕ}\AgdaSymbol{)}\<%
\\
\>[2][@{}l@{\AgdaIndent{0}}]%
\>[8]\AgdaSymbol{→}%
\>[11]\AgdaFunction{p2PKHNonEmptyStackAbstr'}\AgdaSpace{}%
\AgdaBound{msg₁}\AgdaSpace{}%
\AgdaBound{pbk}\AgdaSpace{}%
\AgdaInductiveConstructor{[]}\AgdaSpace{}%
\AgdaBound{x}\AgdaSpace{}%
\AgdaOperator{\AgdaDatatype{≡}}\AgdaSpace{}%
\AgdaInductiveConstructor{nothing}\<%
\\
%
\\[\AgdaEmptyExtraSkip]%
%
\>[2]\AgdaFunction{stackfunP2PKHNonEmptyStackAbstractedCorEmptysNothing}\AgdaSpace{}%
\AgdaBound{msg₁}\AgdaSpace{}%
\AgdaBound{pbk₁}\AgdaSpace{}%
\AgdaInductiveConstructor{zero}\AgdaSpace{}%
\AgdaSymbol{=}\AgdaSpace{}%
\AgdaInductiveConstructor{refl}\<%
\\
%
\>[2]\AgdaFunction{stackfunP2PKHNonEmptyStackAbstractedCorEmptysNothing}\AgdaSpace{}%
\AgdaBound{msg₁}\AgdaSpace{}%
\AgdaBound{pbk₁}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaInductiveConstructor{suc}\AgdaSpace{}%
\AgdaBound{x}\AgdaSymbol{)}\AgdaSpace{}%
\AgdaSymbol{=}\AgdaSpace{}%
\AgdaInductiveConstructor{refl}\<%
\\
%
\\[\AgdaEmptyExtraSkip]%
\>[0]\AgdaComment{\{-\ Now\ we\ look\ at\ what\ happens\ if\ we\ have\ non\ empty\ stack₁\ and\ comparision\ >\ 0}\<%
\\
\>[0]\AgdaComment{-\}}\<%
\\
%
\\[\AgdaEmptyExtraSkip]%
\>[0]\AgdaComment{\{-\ if\ we\ evaluate\ it\ we\ get}\<%
\\
\>[0]\<%
\\
\>[0]\AgdaComment{just\ (boolToNat\ (isSigned\ \ msg₁\ sig₁\ pbk)\ ∷\ stack₁)}\<%
\\
\>[0]\<%
\\
\>[0]\<%
\\
\>[0]\<%
\\
\>[0]\AgdaComment{and\ we\ show\ that\ this\ is\ the\ case}\<%
\\
\>[0]\<%
\\
\>[0]\AgdaComment{-\}}\<%
\\
\>[0]\<%
\end{code}
} % END AgdaHide

\newcommand{\stackVerificationPtoPKHsymbolicExecutionstacknonempty}{
\begin{code}%
\>[0]\AgdaFunction{testStackfunP2PKHNonEmptyStackAbstractedCompreSucNonEmpty}\AgdaSpace{}%
\AgdaSymbol{:}\AgdaSpace{}%
\AgdaDatatype{Maybe}\AgdaSpace{}%
\AgdaFunction{Stack}\<%
\\
\>[0]\AgdaFunction{testStackfunP2PKHNonEmptyStackAbstractedCompreSucNonEmpty}\AgdaSpace{}%
\AgdaSymbol{=}\AgdaSpace{}%
\AgdaFunction{p2PKHNonEmptyStackAbstr'}\AgdaSpace{}%
\AgdaPostulate{msg₁}\AgdaSpace{}%
\AgdaPostulate{pbk}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaPostulate{sig₁}%
\>[101]\AgdaOperator{\AgdaInductiveConstructor{∷}}\AgdaSpace{}%
\AgdaPostulate{stack₁}\AgdaSymbol{)}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaInductiveConstructor{suc}\AgdaSpace{}%
\AgdaPostulate{x₁}\AgdaSymbol{)}\<%
\end{code}
} % END newcommand

\AgdaHide{
\begin{code}%
\>[0]\<%
\\
%
\\[\AgdaEmptyExtraSkip]%
\>[0]\AgdaFunction{stackfunP2PKHNonEmptyStackAbstractedCorComprSucStackNonEmptyCor}\AgdaSpace{}%
\AgdaSymbol{:}\<%
\\
\>[0][@{}l@{\AgdaIndent{0}}]%
\>[7]\AgdaSymbol{(}\AgdaBound{msg₁}\AgdaSpace{}%
\AgdaSymbol{:}\AgdaSpace{}%
\AgdaDatatype{Msg}\AgdaSymbol{)(}\AgdaBound{pbk}\AgdaSpace{}%
\AgdaSymbol{:}\AgdaSpace{}%
\AgdaDatatype{ℕ}\AgdaSymbol{)(}\AgdaBound{x}\AgdaSpace{}%
\AgdaSymbol{:}\AgdaSpace{}%
\AgdaDatatype{ℕ}\AgdaSymbol{)(}\AgdaBound{sig₁}\AgdaSpace{}%
\AgdaSymbol{:}\AgdaSpace{}%
\AgdaDatatype{ℕ}\AgdaSymbol{)(}\AgdaBound{stack₂}\AgdaSpace{}%
\AgdaSymbol{:}\AgdaSpace{}%
\AgdaFunction{Stack}\AgdaSymbol{)}\<%
\\
%
\>[7]\AgdaSymbol{→}%
\>[623I]\AgdaFunction{p2PKHNonEmptyStackAbstr'}\AgdaSpace{}%
\AgdaBound{msg₁}\AgdaSpace{}%
\AgdaBound{pbk}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaBound{sig₁}%
\>[50]\AgdaOperator{\AgdaInductiveConstructor{∷}}\AgdaSpace{}%
\AgdaBound{stack₂}\AgdaSymbol{)}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaInductiveConstructor{suc}\AgdaSpace{}%
\AgdaBound{x}\AgdaSymbol{)}\<%
\\
\>[623I][@{}l@{\AgdaIndent{0}}]%
\>[10]\AgdaOperator{\AgdaDatatype{≡}}%
\>[13]\AgdaInductiveConstructor{just}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaFunction{boolToNat}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaFunction{isSigned}%
\>[40]\AgdaBound{msg₁}\AgdaSpace{}%
\AgdaBound{sig₁}\AgdaSpace{}%
\AgdaBound{pbk}\AgdaSymbol{)}\AgdaSpace{}%
\AgdaOperator{\AgdaInductiveConstructor{∷}}\AgdaSpace{}%
\AgdaBound{stack₂}\AgdaSymbol{)}\<%
\\
\>[0]\AgdaFunction{stackfunP2PKHNonEmptyStackAbstractedCorComprSucStackNonEmptyCor}\AgdaSpace{}%
\AgdaBound{msg₂}\AgdaSpace{}%
\AgdaBound{pbk₁}\AgdaSpace{}%
\AgdaBound{sig₁}\AgdaSpace{}%
\AgdaBound{x}\AgdaSpace{}%
\AgdaBound{stack₃}\AgdaSpace{}%
\AgdaSymbol{=}\AgdaSpace{}%
\AgdaInductiveConstructor{refl}\<%
\\
%
\\[\AgdaEmptyExtraSkip]%
\>[0]\AgdaComment{\{-\ the\ following\ can\ be\ ommitted\ probably}\<%
\\
\>[0]\AgdaComment{\ \ \ since\ we\ have\ digged\ out\ the\ function\ completely}\<%
\\
\>[0]\AgdaComment{\ \ \ but\ here\ is\ anyway\ a\ theorem\ that\ the\ original\ function\ gives\ you\ nothing}\<%
\\
\>[0]\AgdaComment{\ \ \ \ \ \ \ \ \ if\ the\ stack\ has\ hight\ 1\ only}\<%
\\
\>[0]\<%
\\
\>[0]\AgdaComment{-\}}\<%
\\
%
\\[\AgdaEmptyExtraSkip]%
%
\\[\AgdaEmptyExtraSkip]%
\>[0]\AgdaComment{\{-\ this\ function\ is\ obolete\ but\ an\ interesting\ observation\ -\}}\<%
\\
%
\\[\AgdaEmptyExtraSkip]%
\>[0]\AgdaFunction{stackfunP2PKHemptySingleStackIsNothing}\AgdaSpace{}%
\AgdaSymbol{:}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaBound{pubKeyHash}\AgdaSpace{}%
\AgdaSymbol{:}\AgdaSpace{}%
\AgdaDatatype{ℕ}\AgdaSymbol{)(}\AgdaBound{time₁}\AgdaSpace{}%
\AgdaSymbol{:}\AgdaSpace{}%
\AgdaFunction{Time}\AgdaSymbol{)(}\AgdaBound{msg₁}\AgdaSpace{}%
\AgdaSymbol{:}\AgdaSpace{}%
\AgdaDatatype{Msg}\AgdaSymbol{)(}\AgdaBound{pbk}\AgdaSpace{}%
\AgdaSymbol{:}\AgdaSpace{}%
\AgdaDatatype{ℕ}\AgdaSymbol{)}\<%
\\
\>[0][@{}l@{\AgdaIndent{0}}]%
\>[8]\AgdaSymbol{→}\AgdaSpace{}%
\AgdaOperator{\AgdaFunction{⟦}}\AgdaSpace{}%
\AgdaFunction{scriptP2PKHᵇ}\AgdaSpace{}%
\AgdaBound{pubKeyHash}\AgdaSpace{}%
\AgdaOperator{\AgdaFunction{⟧ˢ}}\AgdaSpace{}%
\AgdaBound{time₁}\AgdaSpace{}%
\AgdaBound{msg₁}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaBound{pbk}\AgdaSpace{}%
\AgdaOperator{\AgdaInductiveConstructor{∷}}\AgdaSpace{}%
\AgdaInductiveConstructor{[]}\AgdaSymbol{)}\AgdaSpace{}%
\AgdaOperator{\AgdaDatatype{≡}}\AgdaSpace{}%
\AgdaInductiveConstructor{nothing}\<%
\\
\>[0]\AgdaFunction{stackfunP2PKHemptySingleStackIsNothing}%
\>[40]\AgdaBound{pubKeyHash}\AgdaSpace{}%
\AgdaBound{time₁}\AgdaSpace{}%
\AgdaBound{msg₁}\AgdaSpace{}%
\AgdaBound{pbk}\<%
\\
\>[0][@{}l@{\AgdaIndent{0}}]%
\>[2]\AgdaSymbol{=}%
\>[5]\AgdaOperator{\AgdaFunction{⟦}}%
\>[667I]\AgdaFunction{scriptP2PKHᵇ}\AgdaSpace{}%
\AgdaBound{pubKeyHash}\AgdaSpace{}%
\AgdaOperator{\AgdaFunction{⟧ˢ}}\AgdaSpace{}%
\AgdaBound{time₁}\AgdaSpace{}%
\AgdaBound{msg₁}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaBound{pbk}\AgdaSpace{}%
\AgdaOperator{\AgdaInductiveConstructor{∷}}\AgdaSpace{}%
\AgdaInductiveConstructor{[]}\AgdaSymbol{)}\<%
\\
\>[667I][@{}l@{\AgdaIndent{0}}]%
\>[15]\AgdaFunction{≡⟨}\AgdaSpace{}%
\AgdaFunction{stackfunP2PKHNonEmptyStackAbstractedCor}\AgdaSpace{}%
\AgdaBound{pubKeyHash}\AgdaSpace{}%
\AgdaBound{time₁}\AgdaSpace{}%
\AgdaBound{msg₁}\AgdaSpace{}%
\AgdaBound{pbk}\AgdaSpace{}%
\AgdaInductiveConstructor{[]}%
\>[89]\AgdaFunction{⟩}\<%
\\
%
\>[5]\AgdaFunction{p2PKHNonEmptyStackAbstr'}\AgdaSpace{}%
\AgdaBound{msg₁}\AgdaSpace{}%
\AgdaBound{pbk}\AgdaSpace{}%
\AgdaInductiveConstructor{[]}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaFunction{compareNaturals}\AgdaSpace{}%
\AgdaBound{pubKeyHash}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaFunction{hashFun}\AgdaSpace{}%
\AgdaBound{pbk}\AgdaSymbol{))}\<%
\\
\>[5][@{}l@{\AgdaIndent{0}}]%
\>[15]\AgdaFunction{≡⟨}\AgdaSpace{}%
\AgdaFunction{stackfunP2PKHNonEmptyStackAbstractedCorEmptysNothing}\AgdaSpace{}%
\AgdaBound{msg₁}\AgdaSpace{}%
\AgdaBound{pbk}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaFunction{compareNaturals}\AgdaSpace{}%
\AgdaBound{pubKeyHash}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaFunction{hashFun}\AgdaSpace{}%
\AgdaBound{pbk}\AgdaSymbol{))}%
\>[125]\AgdaFunction{⟩}\<%
\\
%
\>[5]\AgdaInductiveConstructor{nothing}\<%
\\
%
\>[5]\AgdaOperator{\AgdaFunction{∎}}\<%
\\
%
\\[\AgdaEmptyExtraSkip]%
\>[0]\AgdaFunction{abstrFunSucCaseNonEmptyNormalSubTerm1}\AgdaSpace{}%
\AgdaSymbol{:}\AgdaSpace{}%
\AgdaDatatype{ℕ}\<%
\\
\>[0]\AgdaFunction{abstrFunSucCaseNonEmptyNormalSubTerm1}\AgdaSpace{}%
\AgdaSymbol{=}\<%
\\
\>[0]\AgdaComment{--\ \textbackslash{}stackVerificationPtoPKHsymbolicExecutionabstrFunSucCaseNonEmptySubTermOne}\<%
\end{code}
} % END AgdaHide

\newcommand{\stackVerificationPtoPKHsymbolicExecutionabstrFunSucCaseNonEmptySubTermOne}{
\begin{code}[inline]%
\>[0][@{}l@{\AgdaIndent{1}}]%
\>[1]\AgdaFunction{boolToNat}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaFunction{isSigned}\AgdaSpace{}%
\AgdaPostulate{msg₁}\AgdaSpace{}%
\AgdaPostulate{sig₁}\AgdaSpace{}%
\AgdaPostulate{pbk}\AgdaSymbol{)}\<%
\end{code}
} % END newcommand

\AgdaHide{
\begin{code}%
\>[0]\<%
\\
\>[0]\AgdaFunction{abstrFunSucCaseNonEmptyNormalSubTerm2}\AgdaSpace{}%
\AgdaSymbol{:}\AgdaSpace{}%
\AgdaDatatype{Bool}\<%
\\
\>[0]\AgdaFunction{abstrFunSucCaseNonEmptyNormalSubTerm2}\AgdaSpace{}%
\AgdaSymbol{=}\<%
\\
\>[0]\AgdaComment{--\ \textbackslash{}stackVerificationPtoPKHsymbolicExecutionabstrFunSucCaseNonEmptySubTermTwo}\<%
\end{code}
} % END AgdaHide

\newcommand{\stackVerificationPtoPKHsymbolicExecutionabstrFunSucCaseNonEmptySubTermTwo}{
\begin{code}[inline]%
\>[0][@{}l@{\AgdaIndent{1}}]%
\>[1]\AgdaFunction{isSigned}\AgdaSpace{}%
\AgdaPostulate{msg₁}\AgdaSpace{}%
\AgdaPostulate{sig₁}\AgdaSpace{}%
\AgdaPostulate{pbk}\<%
\end{code}
} % END newcommand

\AgdaHide{
\begin{code}%
\>[0]\<%
\\
%
\\[\AgdaEmptyExtraSkip]%
\>[0]\AgdaComment{--\ uncomment\ to\ be\ able\ to\ evaluate}\<%
\\
\>[0]\AgdaComment{--\ test\ :\ Set}\<%
\\
\>[0]\AgdaComment{--\ test\ =\ \{!!\}}\<%
\end{code}
} % END AgdaHide


==> latex-before-sed/paperTypes2021PostProceed/stackVerificationP2PKHsymbolicExecutionPaperVersionPart2.tex <==
%% This file has been generated automatically by mkLagda.awk
%% DO NOT EDIT! ALL YOUR CHANGES WILL BE LOST!

\AgdaHide{
\begin{code}%
\>[0]\AgdaComment{--\ \textbackslash{}stackVerificationPtoPKHsymbolicExecutionPartTwo}\<%
\\
\>[0]\AgdaKeyword{open}\AgdaSpace{}%
\AgdaKeyword{import}\AgdaSpace{}%
\AgdaModule{basicBitcoinDataType}\<%
\\
%
\\[\AgdaEmptyExtraSkip]%
\>[0]\AgdaKeyword{module}\AgdaSpace{}%
\AgdaModule{paperTypes2021PostProceed.stackVerificationP2PKHsymbolicExecutionPaperVersionPart2}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaBound{param}\AgdaSpace{}%
\AgdaSymbol{:}\AgdaSpace{}%
\AgdaRecord{GlobalParameters}\AgdaSymbol{)}%
\>[118]\AgdaKeyword{where}\<%
\\
%
\\[\AgdaEmptyExtraSkip]%
\>[0]\AgdaKeyword{open}\AgdaSpace{}%
\AgdaKeyword{import}\AgdaSpace{}%
\AgdaModule{Data.Nat}%
\>[22]\AgdaKeyword{hiding}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaOperator{\AgdaDatatype{\AgdaUnderscore{}≤\AgdaUnderscore{}}}\AgdaSymbol{)}\<%
\\
\>[0]\AgdaKeyword{open}\AgdaSpace{}%
\AgdaKeyword{import}\AgdaSpace{}%
\AgdaModule{Data.List}\AgdaSpace{}%
\AgdaKeyword{hiding}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaOperator{\AgdaFunction{\AgdaUnderscore{}++\AgdaUnderscore{}}}\AgdaSymbol{)}\<%
\\
\>[0]\AgdaKeyword{open}\AgdaSpace{}%
\AgdaKeyword{import}\AgdaSpace{}%
\AgdaModule{Data.Unit}%
\>[23]\AgdaKeyword{hiding}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaOperator{\AgdaRecord{\AgdaUnderscore{}≤\AgdaUnderscore{}}}\AgdaSymbol{)}\<%
\\
\>[0]\AgdaKeyword{open}\AgdaSpace{}%
\AgdaKeyword{import}\AgdaSpace{}%
\AgdaModule{Data.Empty}\<%
\\
\>[0]\AgdaKeyword{open}\AgdaSpace{}%
\AgdaKeyword{import}\AgdaSpace{}%
\AgdaModule{Data.Sum}\<%
\\
\>[0]\AgdaKeyword{open}\AgdaSpace{}%
\AgdaKeyword{import}\AgdaSpace{}%
\AgdaModule{Data.Bool}%
\>[23]\AgdaKeyword{hiding}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaOperator{\AgdaDatatype{\AgdaUnderscore{}≤\AgdaUnderscore{}}}\AgdaSpace{}%
\AgdaSymbol{;}\AgdaSpace{}%
\AgdaOperator{\AgdaFunction{if\AgdaUnderscore{}then\AgdaUnderscore{}else\AgdaUnderscore{}}}\AgdaSpace{}%
\AgdaSymbol{)}\AgdaSpace{}%
\AgdaKeyword{renaming}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaOperator{\AgdaFunction{\AgdaUnderscore{}∧\AgdaUnderscore{}}}\AgdaSpace{}%
\AgdaSymbol{to}\AgdaSpace{}%
\AgdaOperator{\AgdaFunction{\AgdaUnderscore{}∧b\AgdaUnderscore{}}}\AgdaSpace{}%
\AgdaSymbol{;}\AgdaSpace{}%
\AgdaOperator{\AgdaFunction{\AgdaUnderscore{}∨\AgdaUnderscore{}}}\AgdaSpace{}%
\AgdaSymbol{to}\AgdaSpace{}%
\AgdaOperator{\AgdaFunction{\AgdaUnderscore{}∨b\AgdaUnderscore{}}}\AgdaSpace{}%
\AgdaSymbol{;}\AgdaSpace{}%
\AgdaFunction{T}\AgdaSpace{}%
\AgdaSymbol{to}\AgdaSpace{}%
\AgdaFunction{True}\AgdaSymbol{)}\<%
\\
\>[0]\AgdaKeyword{open}\AgdaSpace{}%
\AgdaKeyword{import}\AgdaSpace{}%
\AgdaModule{Data.Product}\AgdaSpace{}%
\AgdaKeyword{renaming}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaOperator{\AgdaInductiveConstructor{\AgdaUnderscore{},\AgdaUnderscore{}}}\AgdaSpace{}%
\AgdaSymbol{to}\AgdaSpace{}%
\AgdaOperator{\AgdaInductiveConstructor{\AgdaUnderscore{},,\AgdaUnderscore{}}}\AgdaSpace{}%
\AgdaSymbol{)}\<%
\\
\>[0]\AgdaKeyword{open}\AgdaSpace{}%
\AgdaKeyword{import}\AgdaSpace{}%
\AgdaModule{Data.Nat.Base}\AgdaSpace{}%
\AgdaKeyword{hiding}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaOperator{\AgdaDatatype{\AgdaUnderscore{}≤\AgdaUnderscore{}}}\AgdaSymbol{)}\<%
\\
\>[0]\AgdaKeyword{open}\AgdaSpace{}%
\AgdaKeyword{import}\AgdaSpace{}%
\AgdaModule{Data.List.NonEmpty}\AgdaSpace{}%
\AgdaKeyword{hiding}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaField{head}\AgdaSpace{}%
\AgdaSymbol{;}\AgdaSpace{}%
\AgdaOperator{\AgdaFunction{[\AgdaUnderscore{}]}}\AgdaSpace{}%
\AgdaSymbol{)}\<%
\\
\>[0]\AgdaKeyword{open}\AgdaSpace{}%
\AgdaKeyword{import}\AgdaSpace{}%
\AgdaModule{Data.Maybe}\<%
\\
\>[0]\AgdaKeyword{open}\AgdaSpace{}%
\AgdaKeyword{import}\AgdaSpace{}%
\AgdaModule{Relation.Nullary}\<%
\\
%
\\[\AgdaEmptyExtraSkip]%
\>[0]\AgdaKeyword{import}\AgdaSpace{}%
\AgdaModule{Relation.Binary.PropositionalEquality}\AgdaSpace{}%
\AgdaSymbol{as}\AgdaSpace{}%
\AgdaModule{Eq}\<%
\\
\>[0]\AgdaKeyword{open}\AgdaSpace{}%
\AgdaModule{Eq}\AgdaSpace{}%
\AgdaKeyword{using}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaOperator{\AgdaDatatype{\AgdaUnderscore{}≡\AgdaUnderscore{}}}\AgdaSymbol{;}\AgdaSpace{}%
\AgdaInductiveConstructor{refl}\AgdaSymbol{;}\AgdaSpace{}%
\AgdaFunction{cong}\AgdaSymbol{;}\AgdaSpace{}%
\AgdaKeyword{module}\AgdaSpace{}%
\AgdaModule{≡-Reasoning}\AgdaSymbol{;}\AgdaSpace{}%
\AgdaFunction{sym}\AgdaSymbol{)}\<%
\\
\>[0]\AgdaKeyword{open}\AgdaSpace{}%
\AgdaModule{≡-Reasoning}\<%
\\
\>[0]\AgdaKeyword{open}\AgdaSpace{}%
\AgdaKeyword{import}\AgdaSpace{}%
\AgdaModule{Agda.Builtin.Equality}\<%
\\
%
\\[\AgdaEmptyExtraSkip]%
%
\\[\AgdaEmptyExtraSkip]%
\>[0]\AgdaComment{--our\ libraries}\<%
\\
\>[0]\AgdaKeyword{open}\AgdaSpace{}%
\AgdaKeyword{import}\AgdaSpace{}%
\AgdaModule{libraries.listLib}\<%
\\
\>[0]\AgdaKeyword{open}\AgdaSpace{}%
\AgdaKeyword{import}\AgdaSpace{}%
\AgdaModule{libraries.equalityLib}\<%
\\
\>[0]\AgdaKeyword{open}\AgdaSpace{}%
\AgdaKeyword{import}\AgdaSpace{}%
\AgdaModule{libraries.natLib}\<%
\\
\>[0]\AgdaKeyword{open}\AgdaSpace{}%
\AgdaKeyword{import}\AgdaSpace{}%
\AgdaModule{libraries.boolLib}\<%
\\
\>[0]\AgdaKeyword{open}\AgdaSpace{}%
\AgdaKeyword{import}\AgdaSpace{}%
\AgdaModule{libraries.emptyLib}\<%
\\
\>[0]\AgdaKeyword{open}\AgdaSpace{}%
\AgdaKeyword{import}\AgdaSpace{}%
\AgdaModule{libraries.andLib}\<%
\\
\>[0]\AgdaKeyword{open}\AgdaSpace{}%
\AgdaKeyword{import}\AgdaSpace{}%
\AgdaModule{libraries.miscLib}\<%
\\
\>[0]\AgdaKeyword{open}\AgdaSpace{}%
\AgdaKeyword{import}\AgdaSpace{}%
\AgdaModule{libraries.maybeLib}\<%
\\
%
\\[\AgdaEmptyExtraSkip]%
\>[0]\AgdaKeyword{open}\AgdaSpace{}%
\AgdaKeyword{import}\AgdaSpace{}%
\AgdaModule{stack}\<%
\\
\>[0]\AgdaKeyword{open}\AgdaSpace{}%
\AgdaKeyword{import}\AgdaSpace{}%
\AgdaModule{stackPredicate}\<%
\\
\>[0]\AgdaKeyword{open}\AgdaSpace{}%
\AgdaKeyword{import}\AgdaSpace{}%
\AgdaModule{semanticBasicOperations}\AgdaSpace{}%
\AgdaBound{param}\<%
\\
\>[0]\AgdaKeyword{open}\AgdaSpace{}%
\AgdaKeyword{import}\AgdaSpace{}%
\AgdaModule{hoareTripleStack}\AgdaSpace{}%
\AgdaBound{param}\<%
\\
\>[0]\AgdaKeyword{open}\AgdaSpace{}%
\AgdaKeyword{import}\AgdaSpace{}%
\AgdaModule{instruction}\<%
\\
\>[0]\AgdaKeyword{open}\AgdaSpace{}%
\AgdaKeyword{import}\AgdaSpace{}%
\AgdaModule{verificationStackScripts.stackState}\<%
\\
\>[0]\AgdaKeyword{open}\AgdaSpace{}%
\AgdaKeyword{import}\AgdaSpace{}%
\AgdaModule{verificationStackScripts.sPredicate}\<%
\\
\>[0]\AgdaKeyword{open}\AgdaSpace{}%
\AgdaKeyword{import}\AgdaSpace{}%
\AgdaModule{verificationStackScripts.stackHoareTriple}\AgdaSpace{}%
\AgdaBound{param}\<%
\\
\>[0]\AgdaKeyword{open}\AgdaSpace{}%
\AgdaKeyword{import}\AgdaSpace{}%
\AgdaModule{verificationStackScripts.stackVerificationLemmas}\AgdaSpace{}%
\AgdaBound{param}\<%
\\
\>[0]\AgdaKeyword{open}\AgdaSpace{}%
\AgdaKeyword{import}\AgdaSpace{}%
\AgdaModule{verificationStackScripts.stackSemanticsInstructionsBasic}\AgdaSpace{}%
\AgdaBound{param}\<%
\\
\>[0]\AgdaKeyword{open}\AgdaSpace{}%
\AgdaKeyword{import}\AgdaSpace{}%
\AgdaModule{verificationStackScripts.semanticsStackInstructions}\AgdaSpace{}%
\AgdaBound{param}\<%
\\
\>[0]\AgdaKeyword{open}\AgdaSpace{}%
\AgdaKeyword{import}\AgdaSpace{}%
\AgdaModule{verificationStackScripts.stackVerificationP2PKH}\AgdaSpace{}%
\AgdaBound{param}\<%
\\
\>[0]\AgdaKeyword{open}\AgdaSpace{}%
\AgdaKeyword{import}\AgdaSpace{}%
\AgdaModule{verificationStackScripts.stackVerificationP2PKHindexed}\AgdaSpace{}%
\AgdaBound{param}\<%
\\
\>[0]\AgdaKeyword{open}\AgdaSpace{}%
\AgdaKeyword{import}\AgdaSpace{}%
\AgdaModule{verificationStackScripts.stackVerificationP2PKHindexed}\AgdaSpace{}%
\AgdaBound{param}\<%
\\
\>[0]\AgdaKeyword{open}\AgdaSpace{}%
\AgdaKeyword{import}\AgdaSpace{}%
\AgdaModule{paperTypes2021PostProceed.stackVerificationP2PKHsymbolicExecutionPaperVersion}\AgdaSpace{}%
\AgdaBound{param}\<%
\\
%
\\[\AgdaEmptyExtraSkip]%
%
\\[\AgdaEmptyExtraSkip]%
\>[0]\AgdaComment{-------------------------------------------}\<%
\\
\>[0]\AgdaComment{--\ \ Currently\ empty}\<%
\\
\>[0]\AgdaComment{--}\<%
\\
\>[0]\AgdaComment{--\ \ Used\ to\ work\ independently\ on\ that\ part}\<%
\\
\>[0]\AgdaComment{--\ \ To\ be\ kept\ until\ paper\ is\ finished}\<%
\\
\>[0]\AgdaComment{----------------------------------------------}\<%
\end{code}
} % END AgdaHide


==> latex-before-sed/paperTypes2021PostProceed/verificationMultiSigBasicSymbolicExecutionPaper.tex <==
%% This file has been generated automatically by mkLagda.awk
%% DO NOT EDIT! ALL YOUR CHANGES WILL BE LOST!

\AgdaHide{
\begin{code}%
\>[0]\AgdaComment{--\textbackslash{}verificationMultiSigBasicSymbolicExecutionPaper}\<%
\\
\>[0]\AgdaKeyword{open}\AgdaSpace{}%
\AgdaKeyword{import}\AgdaSpace{}%
\AgdaModule{basicBitcoinDataType}\<%
\\
%
\\[\AgdaEmptyExtraSkip]%
\>[0]\AgdaKeyword{module}\AgdaSpace{}%
\AgdaModule{paperTypes2021PostProceed.verificationMultiSigBasicSymbolicExecutionPaper}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaBound{param}\AgdaSpace{}%
\AgdaSymbol{:}\AgdaSpace{}%
\AgdaRecord{GlobalParameters}\AgdaSymbol{)}\AgdaSpace{}%
\AgdaKeyword{where}\<%
\\
%
\\[\AgdaEmptyExtraSkip]%
%
\\[\AgdaEmptyExtraSkip]%
\>[0]\AgdaKeyword{open}\AgdaSpace{}%
\AgdaKeyword{import}\AgdaSpace{}%
\AgdaModule{Data.List.Base}\AgdaSpace{}%
\AgdaKeyword{hiding}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaOperator{\AgdaFunction{\AgdaUnderscore{}++\AgdaUnderscore{}}}\AgdaSpace{}%
\AgdaSymbol{)}\<%
\\
\>[0]\AgdaKeyword{open}\AgdaSpace{}%
\AgdaKeyword{import}\AgdaSpace{}%
\AgdaModule{Data.Nat}%
\>[22]\AgdaKeyword{renaming}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaOperator{\AgdaDatatype{\AgdaUnderscore{}≤\AgdaUnderscore{}}}\AgdaSpace{}%
\AgdaSymbol{to}\AgdaSpace{}%
\AgdaOperator{\AgdaDatatype{\AgdaUnderscore{}≤'\AgdaUnderscore{}}}\AgdaSpace{}%
\AgdaSymbol{;}\AgdaSpace{}%
\AgdaOperator{\AgdaFunction{\AgdaUnderscore{}<\AgdaUnderscore{}}}\AgdaSpace{}%
\AgdaSymbol{to}\AgdaSpace{}%
\AgdaOperator{\AgdaFunction{\AgdaUnderscore{}<'\AgdaUnderscore{}}}\AgdaSymbol{)}\<%
\\
\>[0]\AgdaKeyword{open}\AgdaSpace{}%
\AgdaKeyword{import}\AgdaSpace{}%
\AgdaModule{Data.List}\AgdaSpace{}%
\AgdaKeyword{hiding}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaOperator{\AgdaFunction{\AgdaUnderscore{}++\AgdaUnderscore{}}}%
\>[36]\AgdaSymbol{)}\<%
\\
\>[0]\AgdaKeyword{open}\AgdaSpace{}%
\AgdaKeyword{import}\AgdaSpace{}%
\AgdaModule{Data.Sum}\<%
\\
\>[0]\AgdaKeyword{open}\AgdaSpace{}%
\AgdaKeyword{import}\AgdaSpace{}%
\AgdaModule{Data.Unit}%
\>[23]\AgdaKeyword{hiding}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaOperator{\AgdaRecord{\AgdaUnderscore{}≤\AgdaUnderscore{}}}\AgdaSymbol{)}\<%
\\
\>[0]\AgdaKeyword{open}\AgdaSpace{}%
\AgdaKeyword{import}\AgdaSpace{}%
\AgdaModule{Data.Empty}\<%
\\
\>[0]\AgdaKeyword{open}\AgdaSpace{}%
\AgdaKeyword{import}\AgdaSpace{}%
\AgdaModule{Data.Maybe}\<%
\\
\>[0]\AgdaKeyword{open}\AgdaSpace{}%
\AgdaKeyword{import}\AgdaSpace{}%
\AgdaModule{Data.Bool}%
\>[23]\AgdaKeyword{hiding}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaOperator{\AgdaDatatype{\AgdaUnderscore{}≤\AgdaUnderscore{}}}\AgdaSpace{}%
\AgdaSymbol{;}\AgdaSpace{}%
\AgdaOperator{\AgdaDatatype{\AgdaUnderscore{}<\AgdaUnderscore{}}}\AgdaSpace{}%
\AgdaSymbol{;}\AgdaSpace{}%
\AgdaOperator{\AgdaFunction{if\AgdaUnderscore{}then\AgdaUnderscore{}else\AgdaUnderscore{}}}%
\>[58]\AgdaSymbol{)}%
\>[61]\AgdaKeyword{renaming}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaOperator{\AgdaFunction{\AgdaUnderscore{}∧\AgdaUnderscore{}}}\AgdaSpace{}%
\AgdaSymbol{to}\AgdaSpace{}%
\AgdaOperator{\AgdaFunction{\AgdaUnderscore{}∧b\AgdaUnderscore{}}}\AgdaSpace{}%
\AgdaSymbol{;}\AgdaSpace{}%
\AgdaOperator{\AgdaFunction{\AgdaUnderscore{}∨\AgdaUnderscore{}}}\AgdaSpace{}%
\AgdaSymbol{to}\AgdaSpace{}%
\AgdaOperator{\AgdaFunction{\AgdaUnderscore{}∨b\AgdaUnderscore{}}}\AgdaSpace{}%
\AgdaSymbol{;}\AgdaSpace{}%
\AgdaFunction{T}\AgdaSpace{}%
\AgdaSymbol{to}\AgdaSpace{}%
\AgdaFunction{True}\AgdaSymbol{)}\<%
\\
\>[0]\AgdaKeyword{open}\AgdaSpace{}%
\AgdaKeyword{import}\AgdaSpace{}%
\AgdaModule{Data.Product}\AgdaSpace{}%
\AgdaKeyword{renaming}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaOperator{\AgdaInductiveConstructor{\AgdaUnderscore{},\AgdaUnderscore{}}}\AgdaSpace{}%
\AgdaSymbol{to}\AgdaSpace{}%
\AgdaOperator{\AgdaInductiveConstructor{\AgdaUnderscore{},,\AgdaUnderscore{}}}\AgdaSpace{}%
\AgdaSymbol{)}\<%
\\
\>[0]\AgdaKeyword{open}\AgdaSpace{}%
\AgdaKeyword{import}\AgdaSpace{}%
\AgdaModule{Data.Nat.Base}\AgdaSpace{}%
\AgdaKeyword{hiding}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaOperator{\AgdaDatatype{\AgdaUnderscore{}≤\AgdaUnderscore{}}}\AgdaSpace{}%
\AgdaSymbol{;}\AgdaSpace{}%
\AgdaOperator{\AgdaFunction{\AgdaUnderscore{}<\AgdaUnderscore{}}}\AgdaSymbol{)}\<%
\\
\>[0]\AgdaKeyword{open}\AgdaSpace{}%
\AgdaKeyword{import}\AgdaSpace{}%
\AgdaModule{Data.List.NonEmpty}\AgdaSpace{}%
\AgdaKeyword{hiding}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaField{head}\AgdaSymbol{;}\AgdaSpace{}%
\AgdaOperator{\AgdaFunction{[\AgdaUnderscore{}]}}\AgdaSymbol{)}\<%
\\
\>[0]\AgdaKeyword{open}\AgdaSpace{}%
\AgdaKeyword{import}\AgdaSpace{}%
\AgdaModule{Data.Nat}\AgdaSpace{}%
\AgdaKeyword{using}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaDatatype{ℕ}\AgdaSymbol{;}\AgdaSpace{}%
\AgdaOperator{\AgdaPrimitive{\AgdaUnderscore{}+\AgdaUnderscore{}}}\AgdaSymbol{;}\AgdaSpace{}%
\AgdaOperator{\AgdaFunction{\AgdaUnderscore{}≥\AgdaUnderscore{}}}\AgdaSymbol{;}\AgdaSpace{}%
\AgdaOperator{\AgdaFunction{\AgdaUnderscore{}>\AgdaUnderscore{}}}\AgdaSymbol{;}\AgdaSpace{}%
\AgdaInductiveConstructor{zero}\AgdaSymbol{;}\AgdaSpace{}%
\AgdaInductiveConstructor{suc}\AgdaSymbol{;}\AgdaSpace{}%
\AgdaInductiveConstructor{s≤s}\AgdaSymbol{;}\AgdaSpace{}%
\AgdaInductiveConstructor{z≤n}\AgdaSymbol{)}\<%
\\
\>[0]\AgdaKeyword{import}\AgdaSpace{}%
\AgdaModule{Relation.Binary.PropositionalEquality}\AgdaSpace{}%
\AgdaSymbol{as}\AgdaSpace{}%
\AgdaModule{Eq}\<%
\\
\>[0]\AgdaKeyword{open}\AgdaSpace{}%
\AgdaModule{Eq}\AgdaSpace{}%
\AgdaKeyword{using}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaOperator{\AgdaDatatype{\AgdaUnderscore{}≡\AgdaUnderscore{}}}\AgdaSymbol{;}\AgdaSpace{}%
\AgdaInductiveConstructor{refl}\AgdaSymbol{;}\AgdaSpace{}%
\AgdaFunction{cong}\AgdaSymbol{;}\AgdaSpace{}%
\AgdaKeyword{module}\AgdaSpace{}%
\AgdaModule{≡-Reasoning}\AgdaSymbol{;}\AgdaSpace{}%
\AgdaFunction{sym}\AgdaSymbol{)}\<%
\\
\>[0]\AgdaKeyword{open}\AgdaSpace{}%
\AgdaModule{≡-Reasoning}\<%
\\
\>[0]\AgdaKeyword{open}\AgdaSpace{}%
\AgdaKeyword{import}\AgdaSpace{}%
\AgdaModule{Agda.Builtin.Equality}\<%
\\
%
\\[\AgdaEmptyExtraSkip]%
%
\\[\AgdaEmptyExtraSkip]%
\>[0]\AgdaComment{--our\ libraries}\<%
\\
\>[0]\AgdaKeyword{open}\AgdaSpace{}%
\AgdaKeyword{import}\AgdaSpace{}%
\AgdaModule{libraries.listLib}\<%
\\
\>[0]\AgdaKeyword{open}\AgdaSpace{}%
\AgdaKeyword{import}\AgdaSpace{}%
\AgdaModule{libraries.emptyLib}\<%
\\
\>[0]\AgdaKeyword{open}\AgdaSpace{}%
\AgdaKeyword{import}\AgdaSpace{}%
\AgdaModule{libraries.natLib}\<%
\\
\>[0]\AgdaKeyword{open}\AgdaSpace{}%
\AgdaKeyword{import}\AgdaSpace{}%
\AgdaModule{libraries.boolLib}\<%
\\
\>[0]\AgdaKeyword{open}\AgdaSpace{}%
\AgdaKeyword{import}\AgdaSpace{}%
\AgdaModule{libraries.equalityLib}\<%
\\
\>[0]\AgdaKeyword{open}\AgdaSpace{}%
\AgdaKeyword{import}\AgdaSpace{}%
\AgdaModule{libraries.andLib}\<%
\\
\>[0]\AgdaKeyword{open}\AgdaSpace{}%
\AgdaKeyword{import}\AgdaSpace{}%
\AgdaModule{libraries.miscLib}\<%
\\
\>[0]\AgdaKeyword{open}\AgdaSpace{}%
\AgdaKeyword{import}\AgdaSpace{}%
\AgdaModule{libraries.maybeLib}\<%
\\
%
\\[\AgdaEmptyExtraSkip]%
\>[0]\AgdaKeyword{open}\AgdaSpace{}%
\AgdaKeyword{import}\AgdaSpace{}%
\AgdaModule{stack}\<%
\\
\>[0]\AgdaKeyword{open}\AgdaSpace{}%
\AgdaKeyword{import}\AgdaSpace{}%
\AgdaModule{stackPredicate}\<%
\\
\>[0]\AgdaKeyword{open}\AgdaSpace{}%
\AgdaKeyword{import}\AgdaSpace{}%
\AgdaModule{semanticBasicOperations}\AgdaSpace{}%
\AgdaBound{param}\<%
\\
\>[0][@{}l@{\AgdaIndent{0}}]%
\>[3]\AgdaKeyword{renaming}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaFunction{compareSigsMultiSigAux}\AgdaSpace{}%
\AgdaSymbol{to}\AgdaSpace{}%
\AgdaFunction{cmpMultiSigsAux}\AgdaSymbol{)}\AgdaSpace{}%
\AgdaComment{--cmpMultiSigsAux)}\<%
\\
\>[0]\AgdaKeyword{open}\AgdaSpace{}%
\AgdaKeyword{import}\AgdaSpace{}%
\AgdaModule{instructionBasic}\<%
\\
\>[0]\AgdaKeyword{open}\AgdaSpace{}%
\AgdaKeyword{import}\AgdaSpace{}%
\AgdaModule{verificationMultiSig}\AgdaSpace{}%
\AgdaBound{param}%
\>[40]\AgdaKeyword{hiding}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaFunction{multiSigScript2-4ᵇ}\AgdaSymbol{)}\<%
\\
\>[0]\AgdaKeyword{open}\AgdaSpace{}%
\AgdaKeyword{import}\AgdaSpace{}%
\AgdaModule{verificationStackScripts.semanticsStackInstructions}\AgdaSpace{}%
\AgdaBound{param}\<%
\\
\>[0]\AgdaKeyword{open}\AgdaSpace{}%
\AgdaKeyword{import}\AgdaSpace{}%
\AgdaModule{verificationStackScripts.stackVerificationLemmas}\AgdaSpace{}%
\AgdaBound{param}\<%
\\
\>[0]\AgdaKeyword{open}\AgdaSpace{}%
\AgdaKeyword{import}\AgdaSpace{}%
\AgdaModule{verificationStackScripts.stackHoareTriple}\AgdaSpace{}%
\AgdaBound{param}\<%
\\
\>[0]\AgdaKeyword{open}\AgdaSpace{}%
\AgdaKeyword{import}\AgdaSpace{}%
\AgdaModule{verificationStackScripts.sPredicate}\<%
\\
\>[0]\AgdaKeyword{open}\AgdaSpace{}%
\AgdaKeyword{import}\AgdaSpace{}%
\AgdaModule{verificationStackScripts.hoareTripleStackBasic}\AgdaSpace{}%
\AgdaBound{param}\<%
\\
\>[0]\AgdaKeyword{open}\AgdaSpace{}%
\AgdaKeyword{import}\AgdaSpace{}%
\AgdaModule{verificationStackScripts.stackState}\<%
\\
\>[0]\AgdaKeyword{open}\AgdaSpace{}%
\AgdaKeyword{import}\AgdaSpace{}%
\AgdaModule{verificationStackScripts.stackSemanticsInstructionsBasic}\AgdaSpace{}%
\AgdaBound{param}\<%
\\
\>[0]\AgdaKeyword{open}\AgdaSpace{}%
\AgdaKeyword{import}\AgdaSpace{}%
\AgdaModule{verificationStackScripts.verificationMultiSigBasic}\AgdaSpace{}%
\AgdaBound{param}\<%
\\
%
\\[\AgdaEmptyExtraSkip]%
\>[0]\AgdaKeyword{private}\<%
\\
\>[0][@{}l@{\AgdaIndent{0}}]%
\>[2]\AgdaKeyword{postulate}\AgdaSpace{}%
\AgdaPostulate{pbk₁}\AgdaSpace{}%
\AgdaPostulate{pbk₂}\AgdaSpace{}%
\AgdaPostulate{pbk₃}\AgdaSpace{}%
\AgdaPostulate{pbk₄}\AgdaSpace{}%
\AgdaSymbol{:}%
\>[35]\AgdaDatatype{ℕ}\<%
\\
%
\>[2]\AgdaKeyword{postulate}\AgdaSpace{}%
\AgdaPostulate{time₁}\AgdaSpace{}%
\AgdaSymbol{:}\AgdaSpace{}%
\AgdaFunction{Time}\<%
\\
%
\>[2]\AgdaKeyword{postulate}\AgdaSpace{}%
\AgdaPostulate{msg₁}\AgdaSpace{}%
\AgdaSymbol{:}\AgdaSpace{}%
\AgdaDatatype{Msg}\<%
\\
%
\>[2]\AgdaKeyword{postulate}\AgdaSpace{}%
\AgdaPostulate{stack₁}\AgdaSpace{}%
\AgdaSymbol{:}\AgdaSpace{}%
\AgdaDatatype{List}\AgdaSpace{}%
\AgdaDatatype{ℕ}\<%
\\
%
\>[2]\AgdaKeyword{postulate}\AgdaSpace{}%
\AgdaPostulate{sig₂}\AgdaSpace{}%
\AgdaPostulate{sig₁}\AgdaSpace{}%
\AgdaPostulate{dummy}\AgdaSpace{}%
\AgdaSymbol{:}\AgdaSpace{}%
\AgdaDatatype{ℕ}\<%
\\
\>[0]\AgdaFunction{multiSigScript2-4ᵇ}\AgdaSpace{}%
\AgdaSymbol{:}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaBound{pbk1}\AgdaSpace{}%
\AgdaBound{pbk2}\AgdaSpace{}%
\AgdaBound{pbk3}\AgdaSpace{}%
\AgdaBound{pbk4}\AgdaSpace{}%
\AgdaSymbol{:}%
\>[45]\AgdaDatatype{ℕ}\AgdaSymbol{)}\AgdaSpace{}%
\AgdaSymbol{→}\AgdaSpace{}%
\AgdaFunction{BitcoinScriptBasic}\<%
\\
\>[0]\AgdaComment{--\textbackslash{}verificationMultiSigBasicSymbolicExecutionPapercomplexmultisig}\<%
\end{code}
} % END AgdaHide

\newcommand{\verificationMultiSigBasicSymbolicExecutionPapercomplexmultisig}{
\begin{code}%
\>[0]\AgdaFunction{multiSigScript2-4ᵇ}%
\>[20]\AgdaBound{pbk1}\AgdaSpace{}%
\AgdaBound{pbk2}\AgdaSpace{}%
\AgdaBound{pbk3}\AgdaSpace{}%
\AgdaBound{pbk4}\AgdaSpace{}%
\AgdaSymbol{=}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaInductiveConstructor{opPush}\AgdaSpace{}%
\AgdaNumber{2}\AgdaSymbol{)}%
\>[57]\AgdaOperator{\AgdaInductiveConstructor{∷}}%
\>[60]\AgdaSymbol{(}\AgdaInductiveConstructor{opPush}\AgdaSpace{}%
\AgdaBound{pbk1}\AgdaSymbol{)}%
\>[75]\AgdaOperator{\AgdaInductiveConstructor{∷}}%
\>[78]\AgdaSymbol{(}\AgdaInductiveConstructor{opPush}\AgdaSpace{}%
\AgdaBound{pbk2}\AgdaSymbol{)}\AgdaSpace{}%
\AgdaOperator{\AgdaInductiveConstructor{∷}}\<%
\\
\>[0][@{}l@{\AgdaIndent{0}}]%
\>[2]\AgdaSymbol{(}\AgdaInductiveConstructor{opPush}\AgdaSpace{}%
\AgdaBound{pbk3}\AgdaSymbol{)}\AgdaSpace{}%
\AgdaOperator{\AgdaInductiveConstructor{∷}}%
\>[23]\AgdaSymbol{(}\AgdaInductiveConstructor{opPush}\AgdaSpace{}%
\AgdaBound{pbk4}\AgdaSymbol{)}%
\>[38]\AgdaOperator{\AgdaInductiveConstructor{∷}}%
\>[41]\AgdaSymbol{(}\AgdaInductiveConstructor{opPush}\AgdaSpace{}%
\AgdaNumber{4}\AgdaSymbol{)}%
\>[56]\AgdaOperator{\AgdaInductiveConstructor{∷}}%
\>[59]\AgdaOperator{\AgdaFunction{[}}\AgdaSpace{}%
\AgdaInductiveConstructor{opMultiSig}\AgdaSpace{}%
\AgdaOperator{\AgdaFunction{]}}\<%
\end{code}
} % END newcommand

\AgdaHide{
\begin{code}%
\>[0]\<%
\\
%
\\[\AgdaEmptyExtraSkip]%
\>[0]\AgdaFunction{multisigScript-2-4-symbolic}\AgdaSpace{}%
\AgdaSymbol{=}\<%
\\
\>[0]\AgdaComment{--\textbackslash{}verificationMultiSigBasicSymbolicExecutionPaper}\<%
\end{code}
} % END AgdaHide

\newcommand{\verificationMultiSigBasicSymbolicExecutionPapermultisigsymbolic}{
\begin{code}[inline]%
\>[0][@{}l@{\AgdaIndent{1}}]%
\>[8]\AgdaOperator{\AgdaFunction{⟦}}\AgdaSpace{}%
\AgdaFunction{multiSigScript2-4ᵇ}\AgdaSpace{}%
\AgdaPostulate{pbk₁}\AgdaSpace{}%
\AgdaPostulate{pbk₂}\AgdaSpace{}%
\AgdaPostulate{pbk₃}\AgdaSpace{}%
\AgdaPostulate{pbk₄}\AgdaSpace{}%
\AgdaOperator{\AgdaFunction{⟧ˢ}}\AgdaSpace{}%
\AgdaPostulate{time₁}\AgdaSpace{}%
\AgdaPostulate{msg₁}\AgdaSpace{}%
\AgdaPostulate{stack₁}\<%
\end{code}
} % END newcommand

\AgdaHide{
\begin{code}%
\>[0]\AgdaComment{\{-\ evaluated\ we\ get}\<%
\\
\>[0]\<%
\\
\>[0]\AgdaComment{executeMultiSig3\ msg₁\ (pbk₁\ ∷\ pbk₂\ ∷\ pbk₃\ ∷\ [\ pbk₄\ ])\ 2\ stack₁\ []}\<%
\\
\>[0]\<%
\\
\>[0]\AgdaComment{-\}}\<%
\\
%
\\[\AgdaEmptyExtraSkip]%
\>[0]\AgdaFunction{test2}\AgdaSpace{}%
\AgdaSymbol{:}\AgdaSpace{}%
\AgdaDatatype{Maybe}\AgdaSpace{}%
\AgdaFunction{Stack}\<%
\\
\>[0]\AgdaFunction{test2}%
\>[206I]\AgdaSymbol{=}\<%
\end{code}
} % END AgdaHide

\newcommand{\verificationMultiSigBasicSymbolicExecutionPaperresultmultisig}{
\begin{code}[inline]%
\>[.][@{}l@{}]\<[206I]%
\>[6]\AgdaFunction{executeMultiSig3}\AgdaSpace{}%
\AgdaPostulate{msg₁}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaPostulate{pbk₁}\AgdaSpace{}%
\AgdaOperator{\AgdaInductiveConstructor{∷}}\AgdaSpace{}%
\AgdaPostulate{pbk₂}\AgdaSpace{}%
\AgdaOperator{\AgdaInductiveConstructor{∷}}\AgdaSpace{}%
\AgdaPostulate{pbk₃}\AgdaSpace{}%
\AgdaOperator{\AgdaInductiveConstructor{∷}}\AgdaSpace{}%
\AgdaOperator{\AgdaFunction{[}}\AgdaSpace{}%
\AgdaPostulate{pbk₄}\AgdaSpace{}%
\AgdaOperator{\AgdaFunction{]}}\AgdaSymbol{)}\AgdaSpace{}%
\AgdaNumber{2}\AgdaSpace{}%
\AgdaPostulate{stack₁}\AgdaSpace{}%
\AgdaInductiveConstructor{[]}\<%
\end{code}
} % END newcommand

\AgdaHide{
\begin{code}%
\>[0]\<%
\\
\>[0]\AgdaComment{--\ now\ we\ try\ out\ stack₁\ =\ []}\<%
\\
%
\\[\AgdaEmptyExtraSkip]%
\>[0]\AgdaFunction{multisigScript-2-4-symbolic-empty}\AgdaSpace{}%
\AgdaSymbol{=}\AgdaSpace{}%
\AgdaOperator{\AgdaFunction{⟦}}\AgdaSpace{}%
\AgdaFunction{multiSigScript2-4ᵇ}\AgdaSpace{}%
\AgdaPostulate{pbk₁}\AgdaSpace{}%
\AgdaPostulate{pbk₂}\AgdaSpace{}%
\AgdaPostulate{pbk₃}\AgdaSpace{}%
\AgdaPostulate{pbk₄}\AgdaSpace{}%
\AgdaOperator{\AgdaFunction{⟧ˢ}}\AgdaSpace{}%
\AgdaPostulate{time₁}\AgdaSpace{}%
\AgdaPostulate{msg₁}\AgdaSpace{}%
\AgdaInductiveConstructor{[]}\<%
\\
%
\\[\AgdaEmptyExtraSkip]%
\>[0]\AgdaComment{\{-}\<%
\\
\>[0]\AgdaComment{result\ nothing}\<%
\\
\>[0]\AgdaComment{-\}}\<%
\\
%
\\[\AgdaEmptyExtraSkip]%
\>[0]\AgdaFunction{multisigScript-2-4-symbolic-1stackelement}\AgdaSpace{}%
\AgdaSymbol{=}\AgdaSpace{}%
\AgdaOperator{\AgdaFunction{⟦}}\AgdaSpace{}%
\AgdaFunction{multiSigScript2-4ᵇ}\AgdaSpace{}%
\AgdaPostulate{pbk₁}\AgdaSpace{}%
\AgdaPostulate{pbk₂}\AgdaSpace{}%
\AgdaPostulate{pbk₃}\AgdaSpace{}%
\AgdaPostulate{pbk₄}\AgdaSpace{}%
\AgdaOperator{\AgdaFunction{⟧ˢ}}\AgdaSpace{}%
\AgdaPostulate{time₁}\AgdaSpace{}%
\AgdaPostulate{msg₁}\AgdaSpace{}%
\AgdaOperator{\AgdaFunction{[}}\AgdaSpace{}%
\AgdaPostulate{sig₂}\AgdaSpace{}%
\AgdaOperator{\AgdaFunction{]}}\<%
\\
%
\\[\AgdaEmptyExtraSkip]%
\>[0]\AgdaComment{\{-}\<%
\\
\>[0]\AgdaComment{result\ nothing}\<%
\\
\>[0]\AgdaComment{-\}}\<%
\\
%
\\[\AgdaEmptyExtraSkip]%
\>[0]\AgdaFunction{multisigScript-2-4-symbolic-2stackelement}\AgdaSpace{}%
\AgdaSymbol{=}\AgdaSpace{}%
\AgdaOperator{\AgdaFunction{⟦}}\AgdaSpace{}%
\AgdaFunction{multiSigScript2-4ᵇ}\AgdaSpace{}%
\AgdaPostulate{pbk₁}\AgdaSpace{}%
\AgdaPostulate{pbk₂}\AgdaSpace{}%
\AgdaPostulate{pbk₃}\AgdaSpace{}%
\AgdaPostulate{pbk₄}\AgdaSpace{}%
\AgdaOperator{\AgdaFunction{⟧ˢ}}\AgdaSpace{}%
\AgdaPostulate{time₁}\AgdaSpace{}%
\AgdaPostulate{msg₁}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaPostulate{sig₂}\AgdaSpace{}%
\AgdaOperator{\AgdaInductiveConstructor{∷}}\AgdaSpace{}%
\AgdaOperator{\AgdaFunction{[}}\AgdaSpace{}%
\AgdaPostulate{sig₁}\AgdaSpace{}%
\AgdaOperator{\AgdaFunction{]}}\AgdaSymbol{)}\<%
\\
%
\\[\AgdaEmptyExtraSkip]%
\>[0]\AgdaComment{\{-}\<%
\\
\>[0]\AgdaComment{result\ nothing}\<%
\\
\>[0]\AgdaComment{-\}}\<%
\\
%
\\[\AgdaEmptyExtraSkip]%
\>[0]\AgdaFunction{stackNeededFirstStepMultiSig}\AgdaSpace{}%
\AgdaSymbol{:}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaBound{sig₂}\AgdaSpace{}%
\AgdaBound{sig₁}\AgdaSpace{}%
\AgdaBound{dummy}\AgdaSpace{}%
\AgdaSymbol{:}\AgdaSpace{}%
\AgdaDatatype{ℕ}\AgdaSymbol{)(}\AgdaBound{stack₁}\AgdaSpace{}%
\AgdaSymbol{:}\AgdaSpace{}%
\AgdaFunction{Stack}\AgdaSymbol{)}\AgdaSpace{}%
\AgdaSymbol{→}\AgdaSpace{}%
\AgdaFunction{Stack}\<%
\\
\>[0]\AgdaFunction{stackNeededFirstStepMultiSig}\AgdaSpace{}%
\AgdaBound{sig₂}\AgdaSpace{}%
\AgdaBound{sig₁}\AgdaSpace{}%
\AgdaBound{dummy}\AgdaSpace{}%
\AgdaBound{stack₁}\AgdaSpace{}%
\AgdaSymbol{=}\<%
\\
\>[0][@{}l@{\AgdaIndent{0}}]%
\>[2]\AgdaBound{sig₂}\AgdaSpace{}%
\AgdaOperator{\AgdaInductiveConstructor{∷}}\AgdaSpace{}%
\AgdaBound{sig₁}\AgdaSpace{}%
\AgdaOperator{\AgdaInductiveConstructor{∷}}\AgdaSpace{}%
\AgdaBound{dummy}\AgdaSpace{}%
\AgdaOperator{\AgdaInductiveConstructor{∷}}\AgdaSpace{}%
\AgdaBound{stack₁}\<%
\\
%
\\[\AgdaEmptyExtraSkip]%
%
\\[\AgdaEmptyExtraSkip]%
\>[0]\AgdaFunction{stackNeededFirstStepMultiSig'}\AgdaSpace{}%
\AgdaSymbol{:}\AgdaSpace{}%
\AgdaFunction{Stack}\<%
\\
\>[0]\AgdaFunction{stackNeededFirstStepMultiSig'}\AgdaSpace{}%
\AgdaSymbol{=}\<%
\\
\>[0]\AgdaComment{--\textbackslash{}verificationMultiSigBasicSymbolicExecutionPaperstackNeededFirstStepMultiSig}\<%
\end{code}
} % END AgdaHide

\newcommand{\verificationMultiSigBasicSymbolicExecutionPaperstackNeededFirstStepMultiSig}{
\begin{code}[inline]%
\>[0][@{}l@{\AgdaIndent{1}}]%
\>[2]\AgdaPostulate{sig₂}\AgdaSpace{}%
\AgdaOperator{\AgdaInductiveConstructor{∷}}\AgdaSpace{}%
\AgdaPostulate{sig₁}\AgdaSpace{}%
\AgdaOperator{\AgdaInductiveConstructor{∷}}\AgdaSpace{}%
\AgdaPostulate{dummy}\AgdaSpace{}%
\AgdaOperator{\AgdaInductiveConstructor{∷}}\AgdaSpace{}%
\AgdaPostulate{stack₁}\<%
\end{code}
} % END newcommand

\AgdaHide{
\begin{code}%
\>[0]\<%
\\
%
\\[\AgdaEmptyExtraSkip]%
\>[0]\AgdaFunction{multisigScript-2-4-symbolic-3stackelement}\AgdaSpace{}%
\AgdaSymbol{=}\<%
\end{code}
} % END AgdaHide

\newcommand{\verificationMultiSigBasicSymbolicExecutionPaperstackhasthreeelement}{
\begin{code}[inline]%
\>[0][@{}l@{\AgdaIndent{1}}]%
\>[2]\AgdaOperator{\AgdaFunction{⟦}}\AgdaSpace{}%
\AgdaFunction{multiSigScript2-4ᵇ}\AgdaSpace{}%
\AgdaPostulate{pbk₁}\AgdaSpace{}%
\AgdaPostulate{pbk₂}\AgdaSpace{}%
\AgdaPostulate{pbk₃}\AgdaSpace{}%
\AgdaPostulate{pbk₄}\AgdaSpace{}%
\AgdaOperator{\AgdaFunction{⟧ˢ}}\AgdaSpace{}%
\AgdaPostulate{time₁}\AgdaSpace{}%
\AgdaPostulate{msg₁}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaPostulate{sig₂}\AgdaSpace{}%
\AgdaOperator{\AgdaInductiveConstructor{∷}}\AgdaSpace{}%
\AgdaPostulate{sig₁}\AgdaSpace{}%
\AgdaOperator{\AgdaInductiveConstructor{∷}}\AgdaSpace{}%
\AgdaPostulate{dummy}\AgdaSpace{}%
\AgdaOperator{\AgdaInductiveConstructor{∷}}\AgdaSpace{}%
\AgdaPostulate{stack₁}\AgdaSymbol{)}\<%
\end{code}
} % END newcommand

\AgdaHide{
\begin{code}%
\>[0]\AgdaComment{\{-}\<%
\\
\>[0]\AgdaComment{just}\<%
\\
\>[0]\AgdaComment{(boolToNat}\<%
\\
\>[0]\AgdaComment{\ (cmpMultiSigsAux\ msg₁\ [\ sig₂\ ]\ (pbk₂\ ∷\ pbk₃\ ∷\ [\ pbk₄\ ])\ sig₁\ \ (isSigned\ msg₁\ sig₁\ pbk₁))}\<%
\\
\>[0]\AgdaComment{\ ∷\ \ stack₁)}\<%
\\
\>[0]\AgdaComment{-\}}\<%
\\
%
\\[\AgdaEmptyExtraSkip]%
\>[0]\AgdaFunction{multisigScript-2-4-symbolic-3stackelementNormalised}\AgdaSpace{}%
\AgdaSymbol{:}\AgdaSpace{}%
\AgdaDatatype{Maybe}\AgdaSpace{}%
\AgdaFunction{Stack}\<%
\\
\>[0]\AgdaFunction{multisigScript-2-4-symbolic-3stackelementNormalised}\AgdaSpace{}%
\AgdaSymbol{=}\<%
\\
\>[0]\AgdaComment{--\textbackslash{}verificationMultiSigBasicSymbolicExecutionPaperstackhasthreeelementNormalised}\<%
\end{code}
} % END AgdaHide

\newcommand{\verificationMultiSigBasicSymbolicExecutionPaperstackhasthreeelementNormalised}{
\begin{code}%
\>[0][@{}l@{\AgdaIndent{1}}]%
\>[2]\AgdaInductiveConstructor{just}%
\>[8]\AgdaSymbol{(}\AgdaFunction{boolToNat}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaFunction{cmpMultiSigsAux}\AgdaSpace{}%
\AgdaPostulate{msg₁}\AgdaSpace{}%
\AgdaOperator{\AgdaFunction{[}}\AgdaSpace{}%
\AgdaPostulate{sig₂}\AgdaSpace{}%
\AgdaOperator{\AgdaFunction{]}}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaPostulate{pbk₂}\AgdaSpace{}%
\AgdaOperator{\AgdaInductiveConstructor{∷}}\AgdaSpace{}%
\AgdaPostulate{pbk₃}\AgdaSpace{}%
\AgdaOperator{\AgdaInductiveConstructor{∷}}\AgdaSpace{}%
\AgdaOperator{\AgdaFunction{[}}\AgdaSpace{}%
\AgdaPostulate{pbk₄}\AgdaSpace{}%
\AgdaOperator{\AgdaFunction{]}}\AgdaSymbol{)}\AgdaSpace{}%
\AgdaPostulate{sig₁}\<%
\\
%
\>[8]\AgdaSymbol{(}\AgdaFunction{isSigned}\AgdaSpace{}%
\AgdaPostulate{msg₁}\AgdaSpace{}%
\AgdaPostulate{sig₁}\AgdaSpace{}%
\AgdaPostulate{pbk₁}\AgdaSymbol{))}\AgdaSpace{}%
\AgdaOperator{\AgdaInductiveConstructor{∷}}%
\>[38]\AgdaPostulate{stack₁}\AgdaSymbol{)}\<%
\end{code}
} % END newcommand

\AgdaHide{
\begin{code}%
\>[0]\<%
\\
%
\\[\AgdaEmptyExtraSkip]%
\>[0]\AgdaComment{\{-}\<%
\\
\>[0]\AgdaComment{So\ the\ program\ succeeds\ (we\ obtain\ result\ just)\ and\ all\ we\ need\ to\ check\ is\ whether\ the\ top\ element\ is}\<%
\\
\>[0]\<%
\\
\>[0]\AgdaComment{(boolToNat}\<%
\\
\>[0]\AgdaComment{\ (cmpMultiSigsAux\ msg₁\ [\ sig₂\ ]\ (pbk₂\ ∷\ pbk₃\ ∷\ [\ pbk₄\ ])\ sig₁\ \ (isSigned\ msg₁\ sig₁\ pbk₁))}\<%
\\
\>[0]\<%
\\
\>[0]\AgdaComment{is\ >\ 0}\<%
\\
\>[0]\<%
\\
\>[0]\<%
\\
\>[0]\AgdaComment{which\ is\ the\ case\ if}\<%
\\
\>[0]\AgdaComment{(cmpMultiSigsAux\ msg₁\ [\ sig₂\ ]\ (pbk₂\ ∷\ pbk₃\ ∷\ [\ pbk₄\ ])\ sig₁\ \ (isSigned\ msg₁\ sig₁\ pbk₁))}\<%
\\
\>[0]\<%
\\
\>[0]\AgdaComment{is\ true}\<%
\\
\>[0]\<%
\\
\>[0]\<%
\\
\>[0]\AgdaComment{so\ we\ symbolically\ evaluate}\<%
\\
\>[0]\<%
\\
\>[0]\AgdaComment{cmpMultiSigsAux\ msg₁\ [\ sig₂\ ]\ (pbk₂\ ∷\ pbk₃\ ∷\ [\ pbk₄\ ])\ sig₁\ \ (isSigned\ msg₁\ sig₁\ pbk₁)}\<%
\\
\>[0]\<%
\\
\>[0]\AgdaComment{-\}}\<%
\\
%
\\[\AgdaEmptyExtraSkip]%
\>[0]\AgdaFunction{topElementMultisigScript-2-4-symbolic-3'}\AgdaSpace{}%
\AgdaSymbol{:}\AgdaSpace{}%
\AgdaDatatype{Bool}\<%
\\
\>[0]\AgdaFunction{topElementMultisigScript-2-4-symbolic-3'}\AgdaSpace{}%
\AgdaSymbol{=}\<%
\\
\>[0][@{}l@{\AgdaIndent{0}}]%
\>[3]\AgdaFunction{cmpMultiSigsAux}\AgdaSpace{}%
\AgdaPostulate{msg₁}\AgdaSpace{}%
\AgdaOperator{\AgdaFunction{[}}\AgdaSpace{}%
\AgdaPostulate{sig₂}\AgdaSpace{}%
\AgdaOperator{\AgdaFunction{]}}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaPostulate{pbk₂}\AgdaSpace{}%
\AgdaOperator{\AgdaInductiveConstructor{∷}}\AgdaSpace{}%
\AgdaPostulate{pbk₃}\AgdaSpace{}%
\AgdaOperator{\AgdaInductiveConstructor{∷}}\AgdaSpace{}%
\AgdaOperator{\AgdaFunction{[}}\AgdaSpace{}%
\AgdaPostulate{pbk₄}\AgdaSpace{}%
\AgdaOperator{\AgdaFunction{]}}\AgdaSymbol{)}\AgdaSpace{}%
\AgdaPostulate{sig₁}%
\>[64]\AgdaSymbol{(}\AgdaBound{param}\AgdaSpace{}%
\AgdaSymbol{.}\AgdaField{signed}\AgdaSpace{}%
\AgdaPostulate{msg₁}\AgdaSpace{}%
\AgdaPostulate{sig₁}\AgdaSpace{}%
\AgdaPostulate{pbk₁}\AgdaSymbol{)}\<%
\\
%
\\[\AgdaEmptyExtraSkip]%
\>[0]\AgdaFunction{topElementMultisigScript-2-4-symbolic-3}\AgdaSpace{}%
\AgdaSymbol{:}\AgdaSpace{}%
\AgdaDatatype{Bool}\<%
\\
\>[0]\AgdaFunction{topElementMultisigScript-2-4-symbolic-3}\AgdaSpace{}%
\AgdaSymbol{=}\<%
\end{code}
} % END AgdaHide

\newcommand{\verificationMultiSigBasicSymbolicExecutionPapercompareSigmulti}{
\begin{code}[inline]%
\>[0][@{}l@{\AgdaIndent{1}}]%
\>[3]\AgdaFunction{cmpMultiSigsAux}\AgdaSpace{}%
\AgdaPostulate{msg₁}\AgdaSpace{}%
\AgdaOperator{\AgdaFunction{[}}\AgdaSpace{}%
\AgdaPostulate{sig₂}\AgdaSpace{}%
\AgdaOperator{\AgdaFunction{]}}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaPostulate{pbk₂}\AgdaSpace{}%
\AgdaOperator{\AgdaInductiveConstructor{∷}}\AgdaSpace{}%
\AgdaPostulate{pbk₃}\AgdaSpace{}%
\AgdaOperator{\AgdaInductiveConstructor{∷}}\AgdaSpace{}%
\AgdaOperator{\AgdaFunction{[}}\AgdaSpace{}%
\AgdaPostulate{pbk₄}\AgdaSpace{}%
\AgdaOperator{\AgdaFunction{]}}\AgdaSymbol{)}\AgdaSpace{}%
\AgdaPostulate{sig₁}%
\>[64]\AgdaSymbol{(}\AgdaFunction{isSigned}\AgdaSpace{}%
\AgdaPostulate{msg₁}\AgdaSpace{}%
\AgdaPostulate{sig₁}\AgdaSpace{}%
\AgdaPostulate{pbk₁}\AgdaSymbol{)}\<%
\end{code}
} % END newcommand

\AgdaHide{
\begin{code}%
\>[0]\<%
\\
\>[0]\AgdaFunction{subExpTopElementMultisigScript-2-4-symbolic-3}\AgdaSpace{}%
\AgdaSymbol{:}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaBound{msg₁}\AgdaSpace{}%
\AgdaSymbol{:}\AgdaSpace{}%
\AgdaDatatype{Msg}\AgdaSymbol{)(}\AgdaBound{sig₁}\AgdaSpace{}%
\AgdaBound{pbk₁}\AgdaSpace{}%
\AgdaSymbol{:}\AgdaSpace{}%
\AgdaDatatype{ℕ}\AgdaSymbol{)}\AgdaSpace{}%
\AgdaSymbol{→}\AgdaSpace{}%
\AgdaDatatype{Bool}\<%
\\
\>[0]\AgdaFunction{subExpTopElementMultisigScript-2-4-symbolic-3}\AgdaSpace{}%
\AgdaBound{msg₁}\AgdaSpace{}%
\AgdaBound{sig₁}\AgdaSpace{}%
\AgdaBound{pbk₁}\AgdaSpace{}%
\AgdaSymbol{=}\<%
\\
\>[0][@{}l@{\AgdaIndent{0}}]%
\>[1]\AgdaFunction{isSigned}\AgdaSpace{}%
\AgdaBound{msg₁}\AgdaSpace{}%
\AgdaBound{sig₁}\AgdaSpace{}%
\AgdaBound{pbk₁}\<%
\\
%
\\[\AgdaEmptyExtraSkip]%
\>[0]\AgdaFunction{subExpTopElementMultisigScript-2-4-symbolic-3'}\AgdaSpace{}%
\AgdaSymbol{:}\AgdaSpace{}%
\AgdaDatatype{Bool}\<%
\\
\>[0]\AgdaFunction{subExpTopElementMultisigScript-2-4-symbolic-3'}\AgdaSpace{}%
\AgdaSymbol{=}\<%
\\
\>[0]\AgdaComment{--\textbackslash{}verificationMultiSigBasicSymbolicExecutionPapersubexTopElementOne}\<%
\end{code}
} % END AgdaHide

\newcommand{\verificationMultiSigBasicSymbolicExecutionPapersubexTopElementOne}{
\begin{code}[inline]%
\>[0][@{}l@{\AgdaIndent{1}}]%
\>[1]\AgdaFunction{isSigned}\AgdaSpace{}%
\AgdaPostulate{msg₁}\AgdaSpace{}%
\AgdaPostulate{sig₁}\AgdaSpace{}%
\AgdaPostulate{pbk₁}\<%
\end{code}
} % END newcommand

\AgdaHide{
\begin{code}%
\>[0]\<%
\\
%
\\[\AgdaEmptyExtraSkip]%
%
\\[\AgdaEmptyExtraSkip]%
\>[0]\AgdaFunction{testEqual}\AgdaSpace{}%
\AgdaSymbol{:}\AgdaSpace{}%
\AgdaFunction{topElementMultisigScript-2-4-symbolic-3'}\AgdaSpace{}%
\AgdaOperator{\AgdaDatatype{≡}}\AgdaSpace{}%
\AgdaFunction{topElementMultisigScript-2-4-symbolic-3}\<%
\\
\>[0]\AgdaFunction{testEqual}\AgdaSpace{}%
\AgdaSymbol{=}\AgdaSpace{}%
\AgdaInductiveConstructor{refl}\<%
\\
%
\\[\AgdaEmptyExtraSkip]%
\>[0]\AgdaComment{\{-\ So\ we\ can\ always\ write}\<%
\\
\>[0]\<%
\\
\>[0]\AgdaComment{isSigned\ \ \ instead\ of\ \ \ \ \ param\ .signed}\<%
\\
\>[0]\<%
\\
\>[0]\AgdaComment{-\}}\<%
\\
%
\\[\AgdaEmptyExtraSkip]%
%
\\[\AgdaEmptyExtraSkip]%
%
\\[\AgdaEmptyExtraSkip]%
%
\\[\AgdaEmptyExtraSkip]%
\>[0]\AgdaComment{\{-}\<%
\\
\>[0]\AgdaComment{We\ now\ make\ a\ casedistinction\ on\ (isSigned\ msg₁\ sig₁\ pbk₁)}\<%
\\
\>[0]\<%
\\
\>[0]\<%
\\
\>[0]\AgdaComment{-\}}\<%
\\
%
\\[\AgdaEmptyExtraSkip]%
%
\\[\AgdaEmptyExtraSkip]%
%
\\[\AgdaEmptyExtraSkip]%
%
\\[\AgdaEmptyExtraSkip]%
\>[0]\AgdaFunction{multisigAuxStep1True}\AgdaSpace{}%
\AgdaSymbol{=}\AgdaSpace{}%
\AgdaFunction{cmpMultiSigsAux}\AgdaSpace{}%
\AgdaPostulate{msg₁}\AgdaSpace{}%
\AgdaOperator{\AgdaFunction{[}}\AgdaSpace{}%
\AgdaPostulate{sig₂}\AgdaSpace{}%
\AgdaOperator{\AgdaFunction{]}}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaPostulate{pbk₂}\AgdaSpace{}%
\AgdaOperator{\AgdaInductiveConstructor{∷}}\AgdaSpace{}%
\AgdaPostulate{pbk₃}\AgdaSpace{}%
\AgdaOperator{\AgdaInductiveConstructor{∷}}\AgdaSpace{}%
\AgdaOperator{\AgdaFunction{[}}\AgdaSpace{}%
\AgdaPostulate{pbk₄}\AgdaSpace{}%
\AgdaOperator{\AgdaFunction{]}}\AgdaSymbol{)}\AgdaSpace{}%
\AgdaPostulate{sig₁}\AgdaSpace{}%
\AgdaInductiveConstructor{true}\<%
\\
\>[0]\AgdaComment{\{-}\<%
\\
\>[0]\AgdaComment{\ \ compareSigsMultiSigAux\ msg₁\ []\ (pbk₃\ ∷\ [\ pbk₄\ ])\ sig₂\ (isSigned\ msg₁\ sig₂\ pbk₂)}\<%
\\
\>[0]\AgdaComment{-\}}\<%
\\
%
\\[\AgdaEmptyExtraSkip]%
\>[0]\AgdaFunction{resultMultisigAuxStep1True}\AgdaSpace{}%
\AgdaSymbol{:}\AgdaSpace{}%
\AgdaDatatype{Bool}\<%
\\
\>[0]\AgdaFunction{resultMultisigAuxStep1True}\AgdaSpace{}%
\AgdaSymbol{=}\<%
\\
\>[0]\AgdaComment{--\textbackslash{}verificationMultiSigBasicSymbolicExecutionPaperresultStepOnetrue}\<%
\end{code}
} % END AgdaHide

\newcommand{\verificationMultiSigBasicSymbolicExecutionPaperresultStepOnetrue}{
\begin{code}[inline]%
\>[0][@{}l@{\AgdaIndent{1}}]%
\>[2]\AgdaFunction{cmpMultiSigsAux}\AgdaSpace{}%
\AgdaPostulate{msg₁}\AgdaSpace{}%
\AgdaInductiveConstructor{[]}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaPostulate{pbk₃}\AgdaSpace{}%
\AgdaOperator{\AgdaInductiveConstructor{∷}}\AgdaSpace{}%
\AgdaOperator{\AgdaFunction{[}}\AgdaSpace{}%
\AgdaPostulate{pbk₄}\AgdaSpace{}%
\AgdaOperator{\AgdaFunction{]}}\AgdaSymbol{)}\AgdaSpace{}%
\AgdaPostulate{sig₂}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaFunction{isSigned}\AgdaSpace{}%
\AgdaPostulate{msg₁}\AgdaSpace{}%
\AgdaPostulate{sig₂}\AgdaSpace{}%
\AgdaPostulate{pbk₂}\AgdaSymbol{)}\<%
\end{code}
} % END newcommand

\AgdaHide{
\begin{code}%
\>[0]\<%
\\
\>[0]\AgdaFunction{resultMultisigAuxStep1TrueSubExp}\AgdaSpace{}%
\AgdaSymbol{:}\AgdaSpace{}%
\AgdaDatatype{Bool}\<%
\\
\>[0]\AgdaFunction{resultMultisigAuxStep1TrueSubExp}\AgdaSpace{}%
\AgdaSymbol{=}\<%
\\
\>[0]\AgdaComment{--\textbackslash{}verificationMultiSigBasicSymbolicExecutionPaperresultStepOnetrueSubExp}\<%
\end{code}
} % END AgdaHide

\newcommand{\verificationMultiSigBasicSymbolicExecutionPaperresultStepOnetrueSubExp}{
\begin{code}[inline]%
\>[0][@{}l@{\AgdaIndent{1}}]%
\>[2]\AgdaFunction{isSigned}\AgdaSpace{}%
\AgdaPostulate{msg₁}\AgdaSpace{}%
\AgdaPostulate{sig₂}\AgdaSpace{}%
\AgdaPostulate{pbk₂}\<%
\end{code}
} % END newcommand

\AgdaHide{
\begin{code}%
\>[0]\<%
\\
%
\\[\AgdaEmptyExtraSkip]%
\>[0]\AgdaFunction{multisigAuxStep1TrueStep2True}\AgdaSpace{}%
\AgdaSymbol{=}\AgdaSpace{}%
\AgdaFunction{cmpMultiSigsAux}\AgdaSpace{}%
\AgdaPostulate{msg₁}\AgdaSpace{}%
\AgdaInductiveConstructor{[]}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaPostulate{pbk₃}\AgdaSpace{}%
\AgdaOperator{\AgdaInductiveConstructor{∷}}\AgdaSpace{}%
\AgdaOperator{\AgdaFunction{[}}\AgdaSpace{}%
\AgdaPostulate{pbk₄}\AgdaSpace{}%
\AgdaOperator{\AgdaFunction{]}}\AgdaSymbol{)}\AgdaSpace{}%
\AgdaPostulate{sig₂}\AgdaSpace{}%
\AgdaInductiveConstructor{true}\<%
\\
%
\\[\AgdaEmptyExtraSkip]%
\>[0]\AgdaComment{\{-\ returns\ true\ -\}}\<%
\\
%
\\[\AgdaEmptyExtraSkip]%
%
\\[\AgdaEmptyExtraSkip]%
\>[0]\AgdaFunction{multisigAuxStep1TrueStep2False}\AgdaSpace{}%
\AgdaSymbol{=}\AgdaSpace{}%
\AgdaFunction{cmpMultiSigsAux}\AgdaSpace{}%
\AgdaPostulate{msg₁}\AgdaSpace{}%
\AgdaInductiveConstructor{[]}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaPostulate{pbk₃}\AgdaSpace{}%
\AgdaOperator{\AgdaInductiveConstructor{∷}}\AgdaSpace{}%
\AgdaOperator{\AgdaFunction{[}}\AgdaSpace{}%
\AgdaPostulate{pbk₄}\AgdaSpace{}%
\AgdaOperator{\AgdaFunction{]}}\AgdaSymbol{)}\AgdaSpace{}%
\AgdaPostulate{sig₂}\AgdaSpace{}%
\AgdaInductiveConstructor{false}\<%
\\
%
\\[\AgdaEmptyExtraSkip]%
\>[0]\AgdaComment{\{-\ returns}\<%
\\
\>[0]\AgdaComment{\ \ \ compareSigsMultiSigAux\ msg₁\ []\ [\ pbk₄\ ]\ sig₂\ (isSigned\ msg₁\ sig₂\ pbk₃)}\<%
\\
\>[0]\AgdaComment{-\}}\<%
\\
%
\\[\AgdaEmptyExtraSkip]%
\>[0]\AgdaFunction{resultMultisigAuxStep1Step2False}\AgdaSpace{}%
\AgdaSymbol{:}\AgdaSpace{}%
\AgdaDatatype{Bool}\<%
\\
\>[0]\AgdaFunction{resultMultisigAuxStep1Step2False}\AgdaSpace{}%
\AgdaSymbol{=}\<%
\\
\>[0]\AgdaComment{--\textbackslash{}verificationMultiSigBasicSymbolicExecutionPaperresultStepOnetrueStepTwoFalse}\<%
\end{code}
} % END AgdaHide

\newcommand{\verificationMultiSigBasicSymbolicExecutionPaperresultStepOnetrueStepTwoFalse}{
\begin{code}[inline]%
\>[0][@{}l@{\AgdaIndent{1}}]%
\>[1]\AgdaFunction{cmpMultiSigsAux}\AgdaSpace{}%
\AgdaPostulate{msg₁}\AgdaSpace{}%
\AgdaInductiveConstructor{[]}\AgdaSpace{}%
\AgdaOperator{\AgdaFunction{[}}\AgdaSpace{}%
\AgdaPostulate{pbk₄}\AgdaSpace{}%
\AgdaOperator{\AgdaFunction{]}}\AgdaSpace{}%
\AgdaPostulate{sig₂}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaFunction{isSigned}\AgdaSpace{}%
\AgdaPostulate{msg₁}\AgdaSpace{}%
\AgdaPostulate{sig₂}\AgdaSpace{}%
\AgdaPostulate{pbk₃}\AgdaSymbol{)}\<%
\end{code}
} % END newcommand

\AgdaHide{
\begin{code}%
\>[0]\<%
\\
\>[0]\AgdaFunction{resultMultisigAuxStep1Step2FalseCoreExp}\AgdaSpace{}%
\AgdaSymbol{:}\AgdaSpace{}%
\AgdaDatatype{Bool}\<%
\\
\>[0]\AgdaFunction{resultMultisigAuxStep1Step2FalseCoreExp}\AgdaSpace{}%
\AgdaSymbol{=}\<%
\\
\>[0]\AgdaComment{--\textbackslash{}verificationMultiSigBasicSymbolicExecutionPaperresultStepOnetrueStepTwoFalseCore}\<%
\end{code}
} % END AgdaHide

\newcommand{\verificationMultiSigBasicSymbolicExecutionPaperresultStepOnetrueStepTwoFalseCore}{
\begin{code}[inline]%
\>[0][@{}l@{\AgdaIndent{1}}]%
\>[1]\AgdaFunction{isSigned}\AgdaSpace{}%
\AgdaPostulate{msg₁}\AgdaSpace{}%
\AgdaPostulate{sig₂}\AgdaSpace{}%
\AgdaPostulate{pbk₃}\<%
\end{code}
} % END newcommand

\AgdaHide{
\begin{code}%
\>[0]\<%
\\
\>[0]\AgdaFunction{multisigAuxStep1TrueStep2FalseStep3True}\AgdaSpace{}%
\AgdaSymbol{=}\AgdaSpace{}%
\AgdaFunction{cmpMultiSigsAux}\AgdaSpace{}%
\AgdaPostulate{msg₁}\AgdaSpace{}%
\AgdaInductiveConstructor{[]}\AgdaSpace{}%
\AgdaOperator{\AgdaFunction{[}}\AgdaSpace{}%
\AgdaPostulate{pbk₄}\AgdaSpace{}%
\AgdaOperator{\AgdaFunction{]}}\AgdaSpace{}%
\AgdaPostulate{sig₂}\AgdaSpace{}%
\AgdaInductiveConstructor{true}\<%
\\
%
\\[\AgdaEmptyExtraSkip]%
%
\\[\AgdaEmptyExtraSkip]%
\>[0]\AgdaComment{\{-\ returns\ true\ -\}}\<%
\\
%
\\[\AgdaEmptyExtraSkip]%
\>[0]\AgdaFunction{multisigAuxStep1TrueStep2FalseStep3False}\AgdaSpace{}%
\AgdaSymbol{=}\AgdaSpace{}%
\AgdaFunction{cmpMultiSigsAux}\AgdaSpace{}%
\AgdaPostulate{msg₁}\AgdaSpace{}%
\AgdaInductiveConstructor{[]}\AgdaSpace{}%
\AgdaOperator{\AgdaFunction{[}}\AgdaSpace{}%
\AgdaPostulate{pbk₄}\AgdaSpace{}%
\AgdaOperator{\AgdaFunction{]}}\AgdaSpace{}%
\AgdaPostulate{sig₂}\AgdaSpace{}%
\AgdaInductiveConstructor{false}\<%
\\
%
\\[\AgdaEmptyExtraSkip]%
\>[0]\AgdaComment{\{-\ returns}\<%
\\
\>[0]\AgdaComment{\ \ \ \ cmpMultiSigsAux\ msg₁\ []\ []\ sig₂\ (isSigned\ msg₁\ sig₂\ pbk₄)}\<%
\\
\>[0]\AgdaComment{-\}}\<%
\\
%
\\[\AgdaEmptyExtraSkip]%
%
\\[\AgdaEmptyExtraSkip]%
%
\\[\AgdaEmptyExtraSkip]%
\>[0]\AgdaFunction{multisigAuxStep1TrueStep2FalseStep3FalseStep4True}\AgdaSpace{}%
\AgdaSymbol{=}\AgdaSpace{}%
\AgdaFunction{cmpMultiSigsAux}\AgdaSpace{}%
\AgdaPostulate{msg₁}\AgdaSpace{}%
\AgdaInductiveConstructor{[]}\AgdaSpace{}%
\AgdaInductiveConstructor{[]}\AgdaSpace{}%
\AgdaPostulate{sig₂}\AgdaSpace{}%
\AgdaInductiveConstructor{true}\<%
\\
%
\\[\AgdaEmptyExtraSkip]%
\>[0]\AgdaComment{\{-\ returns\ true\ -\}}\<%
\\
%
\\[\AgdaEmptyExtraSkip]%
\>[0]\AgdaFunction{multisigAuxStep1TrueStep2FalseStep3FalseStep4False}\AgdaSpace{}%
\AgdaSymbol{=}\AgdaSpace{}%
\AgdaFunction{cmpMultiSigsAux}\AgdaSpace{}%
\AgdaPostulate{msg₁}\AgdaSpace{}%
\AgdaInductiveConstructor{[]}\AgdaSpace{}%
\AgdaInductiveConstructor{[]}\AgdaSpace{}%
\AgdaPostulate{sig₂}\AgdaSpace{}%
\AgdaInductiveConstructor{false}\<%
\\
%
\\[\AgdaEmptyExtraSkip]%
\>[0]\AgdaComment{\{-\ returns\ false\ -\}}\<%
\\
%
\\[\AgdaEmptyExtraSkip]%
\>[0]\AgdaFunction{multisigAuxStep1False}\AgdaSpace{}%
\AgdaSymbol{=}\AgdaSpace{}%
\AgdaFunction{cmpMultiSigsAux}\AgdaSpace{}%
\AgdaPostulate{msg₁}\AgdaSpace{}%
\AgdaOperator{\AgdaFunction{[}}\AgdaSpace{}%
\AgdaPostulate{sig₂}\AgdaSpace{}%
\AgdaOperator{\AgdaFunction{]}}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaPostulate{pbk₂}\AgdaSpace{}%
\AgdaOperator{\AgdaInductiveConstructor{∷}}\AgdaSpace{}%
\AgdaPostulate{pbk₃}\AgdaSpace{}%
\AgdaOperator{\AgdaInductiveConstructor{∷}}\AgdaSpace{}%
\AgdaOperator{\AgdaFunction{[}}\AgdaSpace{}%
\AgdaPostulate{pbk₄}\AgdaSpace{}%
\AgdaOperator{\AgdaFunction{]}}\AgdaSymbol{)}\AgdaSpace{}%
\AgdaPostulate{sig₁}\AgdaSpace{}%
\AgdaInductiveConstructor{false}\<%
\\
%
\\[\AgdaEmptyExtraSkip]%
\>[0]\AgdaComment{\{-\ returns}\<%
\\
\>[0]\<%
\\
\>[0]\AgdaComment{\ \ \ cmpMultiSigsAux\ msg₁\ [\ sig₂\ ]\ (pbk₃\ ∷\ [\ pbk₄\ ])\ sig₁\ (isSigned\ msg₁\ sig₁\ pbk₂)}\<%
\\
\>[0]\<%
\\
\>[0]\AgdaComment{-\}}\<%
\\
%
\\[\AgdaEmptyExtraSkip]%
\>[0]\AgdaFunction{multisigAuxStep1FalseStep2True}%
\>[32]\AgdaSymbol{=}\AgdaSpace{}%
\AgdaFunction{cmpMultiSigsAux}\AgdaSpace{}%
\AgdaPostulate{msg₁}\AgdaSpace{}%
\AgdaOperator{\AgdaFunction{[}}\AgdaSpace{}%
\AgdaPostulate{sig₂}\AgdaSpace{}%
\AgdaOperator{\AgdaFunction{]}}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaPostulate{pbk₃}\AgdaSpace{}%
\AgdaOperator{\AgdaInductiveConstructor{∷}}\AgdaSpace{}%
\AgdaOperator{\AgdaFunction{[}}\AgdaSpace{}%
\AgdaPostulate{pbk₄}\AgdaSpace{}%
\AgdaOperator{\AgdaFunction{]}}\AgdaSymbol{)}\AgdaSpace{}%
\AgdaPostulate{sig₁}\AgdaSpace{}%
\AgdaInductiveConstructor{true}\<%
\\
%
\\[\AgdaEmptyExtraSkip]%
\>[0]\AgdaComment{\{-\ returns}\<%
\\
\>[0]\AgdaComment{\ \ \ \ \ cmpMultiSigsAux\ msg₁\ []\ [\ pbk₄\ ]\ sig₂\ (isSigned\ msg₁\ sig₂\ pbk₃)}\<%
\\
\>[0]\AgdaComment{-\}}\<%
\\
%
\\[\AgdaEmptyExtraSkip]%
\>[0]\AgdaFunction{multisigAuxStep1FalseStep2TrueStep3True}%
\>[41]\AgdaSymbol{=}\AgdaSpace{}%
\AgdaFunction{cmpMultiSigsAux}\AgdaSpace{}%
\AgdaPostulate{msg₁}\AgdaSpace{}%
\AgdaInductiveConstructor{[]}\AgdaSpace{}%
\AgdaOperator{\AgdaFunction{[}}\AgdaSpace{}%
\AgdaPostulate{pbk₄}\AgdaSpace{}%
\AgdaOperator{\AgdaFunction{]}}\AgdaSpace{}%
\AgdaPostulate{sig₂}\AgdaSpace{}%
\AgdaInductiveConstructor{true}\<%
\\
%
\\[\AgdaEmptyExtraSkip]%
\>[0]\AgdaComment{\{-\ returns\ true\ -\}}\<%
\\
%
\\[\AgdaEmptyExtraSkip]%
\>[0]\AgdaFunction{multisigAuxStep1FalseStep2TrueStep3False}%
\>[42]\AgdaSymbol{=}\AgdaSpace{}%
\AgdaFunction{cmpMultiSigsAux}\AgdaSpace{}%
\AgdaPostulate{msg₁}\AgdaSpace{}%
\AgdaInductiveConstructor{[]}\AgdaSpace{}%
\AgdaOperator{\AgdaFunction{[}}\AgdaSpace{}%
\AgdaPostulate{pbk₄}\AgdaSpace{}%
\AgdaOperator{\AgdaFunction{]}}\AgdaSpace{}%
\AgdaPostulate{sig₂}\AgdaSpace{}%
\AgdaInductiveConstructor{false}\<%
\\
%
\\[\AgdaEmptyExtraSkip]%
\>[0]\AgdaComment{\{-\ returns}\<%
\\
\>[0]\AgdaComment{\ \ \ cmpMultiSigsAux\ msg₁\ []\ []\ sig₂\ (isSigned\ msg₁\ sig₂\ pbk₄)}\<%
\\
\>[0]\AgdaComment{-\}}\<%
\\
%
\\[\AgdaEmptyExtraSkip]%
\>[0]\AgdaFunction{multisigAuxStep1FalseStep2TrueStep3FalseStep4True}%
\>[51]\AgdaSymbol{=}\AgdaSpace{}%
\AgdaFunction{cmpMultiSigsAux}\AgdaSpace{}%
\AgdaPostulate{msg₁}\AgdaSpace{}%
\AgdaInductiveConstructor{[]}\AgdaSpace{}%
\AgdaInductiveConstructor{[]}\AgdaSpace{}%
\AgdaPostulate{sig₂}\AgdaSpace{}%
\AgdaInductiveConstructor{true}\<%
\\
%
\\[\AgdaEmptyExtraSkip]%
\>[0]\AgdaComment{\{-\ returns\ true\ -\}}\<%
\\
%
\\[\AgdaEmptyExtraSkip]%
\>[0]\AgdaFunction{multisigAuxStep1FalseStep2TrueStep3FalseStepFalse}%
\>[51]\AgdaSymbol{=}\AgdaSpace{}%
\AgdaFunction{cmpMultiSigsAux}\AgdaSpace{}%
\AgdaPostulate{msg₁}\AgdaSpace{}%
\AgdaInductiveConstructor{[]}\AgdaSpace{}%
\AgdaInductiveConstructor{[]}\AgdaSpace{}%
\AgdaPostulate{sig₂}\AgdaSpace{}%
\AgdaInductiveConstructor{false}\<%
\\
%
\\[\AgdaEmptyExtraSkip]%
\>[0]\AgdaComment{\{-\ returns\ false\ -\}}\<%
\\
%
\\[\AgdaEmptyExtraSkip]%
%
\\[\AgdaEmptyExtraSkip]%
\>[0]\AgdaFunction{multisigAuxStep1FalseStep2False}%
\>[33]\AgdaSymbol{=}\AgdaSpace{}%
\AgdaFunction{cmpMultiSigsAux}\AgdaSpace{}%
\AgdaPostulate{msg₁}\AgdaSpace{}%
\AgdaOperator{\AgdaFunction{[}}\AgdaSpace{}%
\AgdaPostulate{sig₂}\AgdaSpace{}%
\AgdaOperator{\AgdaFunction{]}}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaPostulate{pbk₃}\AgdaSpace{}%
\AgdaOperator{\AgdaInductiveConstructor{∷}}\AgdaSpace{}%
\AgdaOperator{\AgdaFunction{[}}\AgdaSpace{}%
\AgdaPostulate{pbk₄}\AgdaSpace{}%
\AgdaOperator{\AgdaFunction{]}}\AgdaSymbol{)}\AgdaSpace{}%
\AgdaPostulate{sig₁}\AgdaSpace{}%
\AgdaInductiveConstructor{false}\<%
\\
%
\\[\AgdaEmptyExtraSkip]%
\>[0]\AgdaComment{\{-returns}\<%
\\
\>[0]\<%
\\
\>[0]\AgdaComment{\ \ cmpMultiSigsAux\ msg₁\ [\ sig₂\ ]\ [\ pbk₄\ ]\ sig₁\ (isSigned\ msg₁\ sig₁\ pbk₃)}\<%
\\
\>[0]\AgdaComment{-\}}\<%
\\
%
\\[\AgdaEmptyExtraSkip]%
\>[0]\AgdaFunction{multisigAuxStep1FalseStep2FalseStep3True}%
\>[42]\AgdaSymbol{=}\AgdaSpace{}%
\AgdaFunction{cmpMultiSigsAux}\AgdaSpace{}%
\AgdaPostulate{msg₁}\AgdaSpace{}%
\AgdaOperator{\AgdaFunction{[}}\AgdaSpace{}%
\AgdaPostulate{sig₂}\AgdaSpace{}%
\AgdaOperator{\AgdaFunction{]}}\AgdaSpace{}%
\AgdaOperator{\AgdaFunction{[}}\AgdaSpace{}%
\AgdaPostulate{pbk₄}\AgdaSpace{}%
\AgdaOperator{\AgdaFunction{]}}\AgdaSpace{}%
\AgdaPostulate{sig₁}\AgdaSpace{}%
\AgdaInductiveConstructor{true}\<%
\\
%
\\[\AgdaEmptyExtraSkip]%
\>[0]\AgdaComment{\{-\ returns}\<%
\\
\>[0]\AgdaComment{\ \ \ cmpMultiSigsAux\ msg₁\ []\ []\ sig₂\ (isSigned\ msg₁\ sig₂\ pbk₄)}\<%
\\
\>[0]\AgdaComment{-\}}\<%
\\
%
\\[\AgdaEmptyExtraSkip]%
\>[0]\AgdaFunction{multisigAuxStep1FalseStep2FalseStep3TrueStep4True}%
\>[51]\AgdaSymbol{=}\AgdaSpace{}%
\AgdaFunction{cmpMultiSigsAux}\AgdaSpace{}%
\AgdaPostulate{msg₁}\AgdaSpace{}%
\AgdaInductiveConstructor{[]}\AgdaSpace{}%
\AgdaInductiveConstructor{[]}\AgdaSpace{}%
\AgdaPostulate{sig₂}\AgdaSpace{}%
\AgdaInductiveConstructor{true}\<%
\\
%
\\[\AgdaEmptyExtraSkip]%
\>[0]\AgdaComment{\{-\ returns\ true\ -\}}\<%
\\
%
\\[\AgdaEmptyExtraSkip]%
\>[0]\AgdaFunction{multisigAuxStep1FalseStep2FalseStep3TrueStep4False}%
\>[52]\AgdaSymbol{=}\AgdaSpace{}%
\AgdaFunction{cmpMultiSigsAux}\AgdaSpace{}%
\AgdaPostulate{msg₁}\AgdaSpace{}%
\AgdaInductiveConstructor{[]}\AgdaSpace{}%
\AgdaInductiveConstructor{[]}\AgdaSpace{}%
\AgdaPostulate{sig₂}\AgdaSpace{}%
\AgdaInductiveConstructor{false}\<%
\\
%
\\[\AgdaEmptyExtraSkip]%
\>[0]\AgdaComment{\{-\ returns\ false\ -\}}\<%
\\
%
\\[\AgdaEmptyExtraSkip]%
%
\\[\AgdaEmptyExtraSkip]%
%
\\[\AgdaEmptyExtraSkip]%
%
\\[\AgdaEmptyExtraSkip]%
\>[0]\AgdaFunction{multisigAuxStep1FalseStep2FalseStep3False}%
\>[43]\AgdaSymbol{=}\AgdaSpace{}%
\AgdaFunction{cmpMultiSigsAux}\AgdaSpace{}%
\AgdaPostulate{msg₁}\AgdaSpace{}%
\AgdaOperator{\AgdaFunction{[}}\AgdaSpace{}%
\AgdaPostulate{sig₂}\AgdaSpace{}%
\AgdaOperator{\AgdaFunction{]}}\AgdaSpace{}%
\AgdaOperator{\AgdaFunction{[}}\AgdaSpace{}%
\AgdaPostulate{pbk₄}\AgdaSpace{}%
\AgdaOperator{\AgdaFunction{]}}\AgdaSpace{}%
\AgdaPostulate{sig₁}\AgdaSpace{}%
\AgdaInductiveConstructor{false}\<%
\\
%
\\[\AgdaEmptyExtraSkip]%
\>[0]\AgdaComment{\{-\ returns}\<%
\\
\>[0]\AgdaComment{\ \ \ \ cmpMultiSigsAux\ msg₁\ [\ sig₂\ ]\ []\ sig₁\ (isSigned\ msg₁\ sig₁\ pbk₄)}\<%
\\
\>[0]\AgdaComment{-\}}\<%
\\
%
\\[\AgdaEmptyExtraSkip]%
\>[0]\AgdaFunction{multisigAuxStep1FalseStep2FalseStep3FalseStep4True}%
\>[52]\AgdaSymbol{=}\AgdaSpace{}%
\AgdaFunction{cmpMultiSigsAux}\AgdaSpace{}%
\AgdaPostulate{msg₁}\AgdaSpace{}%
\AgdaOperator{\AgdaFunction{[}}\AgdaSpace{}%
\AgdaPostulate{sig₂}\AgdaSpace{}%
\AgdaOperator{\AgdaFunction{]}}\AgdaSpace{}%
\AgdaInductiveConstructor{[]}\AgdaSpace{}%
\AgdaPostulate{sig₁}\AgdaSpace{}%
\AgdaInductiveConstructor{true}\<%
\\
%
\\[\AgdaEmptyExtraSkip]%
\>[0]\AgdaComment{\{-\ returns\ false\ -\}}\<%
\\
%
\\[\AgdaEmptyExtraSkip]%
\>[0]\AgdaFunction{multisigAuxStep1FalseStep2FalseStep3FalseStep4False}%
\>[53]\AgdaSymbol{=}\AgdaSpace{}%
\AgdaFunction{cmpMultiSigsAux}\AgdaSpace{}%
\AgdaPostulate{msg₁}\AgdaSpace{}%
\AgdaOperator{\AgdaFunction{[}}\AgdaSpace{}%
\AgdaPostulate{sig₂}\AgdaSpace{}%
\AgdaOperator{\AgdaFunction{]}}\AgdaSpace{}%
\AgdaInductiveConstructor{[]}\AgdaSpace{}%
\AgdaPostulate{sig₁}\AgdaSpace{}%
\AgdaInductiveConstructor{false}\<%
\\
%
\\[\AgdaEmptyExtraSkip]%
\>[0]\AgdaComment{\{-\ returns\ false\ -\}}\<%
\\
%
\\[\AgdaEmptyExtraSkip]%
%
\\[\AgdaEmptyExtraSkip]%
\>[0]\AgdaComment{\{-\ So\ we\ see\ that\ that}\<%
\\
\>[0]\<%
\\
\>[0]\AgdaComment{(cmpMultiSigsAux\ msg₁\ [\ sig₂\ ]\ (pbk₂\ ∷\ pbk₃\ ∷\ [\ pbk₄\ ])\ sig₁\ \ (isSigned\ msg₁\ sig₁\ pbk₁))}\<%
\\
\>[0]\<%
\\
\>[0]\<%
\\
\>[0]\AgdaComment{returns\ true\ iff}\<%
\\
\>[0]\<%
\\
\>[0]\AgdaComment{(isSigned\ msg₁\ sig₂\ pbk₂)\ \ \ and\ (isSigned\ msg₁\ sig₂\ pbk₂)}\<%
\\
\>[0]\AgdaComment{or}\<%
\\
\>[0]\AgdaComment{(isSigned\ msg₁\ sig₂\ pbk₂)\ \ \ and\ ¬\ (isSigned\ msg₁\ sig₂\ pbk₂)\ \ and\ (isSigned\ msg₁\ sig₂\ pbk₃)}\<%
\\
\>[0]\AgdaComment{or}\<%
\\
\>[0]\AgdaComment{(isSigned\ msg₁\ sig₂\ pbk₂)\ \ \ and\ ¬\ (isSigned\ msg₁\ sig₂\ pbk₂)\ \ and\ ¬\ (isSigned\ msg₁\ sig₂\ pbk₃)\ and\ (isSigned\ msg₁\ sig₂\ pbk₄)}\<%
\\
\>[0]\AgdaComment{or}\<%
\\
\>[0]\AgdaComment{¬\ (isSigned\ msg₁\ sig₂\ pbk₂)\ \ and\ (isSigned\ msg₁\ sig₁\ pbk₂)\ and\ (isSigned\ msg₁\ sig₂\ pbk₃)}\<%
\\
\>[0]\AgdaComment{or}\<%
\\
\>[0]\AgdaComment{¬\ (isSigned\ msg₁\ sig₂\ pbk₂)\ \ and\ (isSigned\ msg₁\ sig₁\ pbk₂)\ and\ ¬\ (isSigned\ msg₁\ sig₂\ pbk₃)\ and\ (isSigned\ msg₁\ sig₂\ pbk₄)}\<%
\\
\>[0]\AgdaComment{or}\<%
\\
\>[0]\AgdaComment{¬\ (isSigned\ msg₁\ sig₂\ pbk₂)\ \ and\ ¬\ (isSigned\ msg₁\ sig₁\ pbk₂)\ \ and\ (isSigned\ msg₁\ sig₁\ pbk₃)\ \ and\ (isSigned\ msg₁\ sig₂\ pbk₄)}\<%
\\
\>[0]\<%
\\
\>[0]\<%
\\
\>[0]\<%
\\
\>[0]\AgdaComment{we\ simplify\ it\ to:}\<%
\\
\>[0]\<%
\\
\>[0]\AgdaComment{(isSigned\ msg₁\ sig₂\ pbk₂)\ \ \ and\ (isSigned\ msg₁\ sig₂\ pbk₂)}\<%
\\
\>[0]\AgdaComment{or}\<%
\\
\>[0]\AgdaComment{(isSigned\ msg₁\ sig₂\ pbk₂)\ \ \ and\ (isSigned\ msg₁\ sig₂\ pbk₃)}\<%
\\
\>[0]\AgdaComment{or}\<%
\\
\>[0]\AgdaComment{(isSigned\ msg₁\ sig₂\ pbk₂)\ \ \ and\ \ (isSigned\ msg₁\ sig₂\ pbk₄)}\<%
\\
\>[0]\AgdaComment{or}\<%
\\
\>[0]\AgdaComment{(isSigned\ msg₁\ sig₁\ pbk₂)\ and\ (isSigned\ msg₁\ sig₂\ pbk₃)}\<%
\\
\>[0]\AgdaComment{or}\<%
\\
\>[0]\AgdaComment{(isSigned\ msg₁\ sig₁\ pbk₂)\ and\ (isSigned\ msg₁\ sig₂\ pbk₄)}\<%
\\
\>[0]\AgdaComment{or}\<%
\\
\>[0]\AgdaComment{(isSigned\ msg₁\ sig₁\ pbk₃)\ \ and\ (isSigned\ msg₁\ sig₂\ pbk₄)}\<%
\\
\>[0]\<%
\\
\>[0]\<%
\\
\>[0]\<%
\\
\>[0]\AgdaComment{so\ the\ full\ script\ is\ accepted\ if\ and\ only\ if\ the\ stack\ has\ hight\ at\ least\ 3\ and}\<%
\\
\>[0]\AgdaComment{if\ the\ top\ elements\ are\ sig₁\ sig₂\ \ dummy}\<%
\\
\>[0]\AgdaComment{then\ \ the\ above\ condition\ holds}\<%
\\
\>[0]\<%
\\
\>[0]\AgdaComment{so\ the\ weakest\ precondition\ is\ ...\ \ name\ for\ weakest\ precondition}\<%
\\
\>[0]\<%
\\
\>[0]\<%
\\
\>[0]\AgdaComment{-\}}\<%
\\
%
\\[\AgdaEmptyExtraSkip]%
%
\\[\AgdaEmptyExtraSkip]%
%
\\[\AgdaEmptyExtraSkip]%
%
\\[\AgdaEmptyExtraSkip]%
\>[0]\AgdaComment{\{-}\<%
\\
\>[0]\AgdaComment{test\ :\ Set}\<%
\\
\>[0]\AgdaComment{test\ =\ \{!!\}}\<%
\\
\>[0]\AgdaComment{-\}}\<%
\end{code}
} % END AgdaHide


==> latex-before-sed/stack.tex <==
%% This file has been generated automatically by mkLagda.awk
%% DO NOT EDIT! ALL YOUR CHANGES WILL BE LOST!

\AgdaHide{
\begin{code}%
\>[0]\AgdaKeyword{module}\AgdaSpace{}%
\AgdaModule{stack}\AgdaSpace{}%
\AgdaKeyword{where}\<%
\\
%
\\[\AgdaEmptyExtraSkip]%
\>[0]\AgdaKeyword{open}\AgdaSpace{}%
\AgdaKeyword{import}\AgdaSpace{}%
\AgdaModule{Data.Nat}%
\>[22]\AgdaKeyword{hiding}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaOperator{\AgdaDatatype{\AgdaUnderscore{}≤\AgdaUnderscore{}}}\AgdaSymbol{)}\<%
\\
\>[0]\AgdaKeyword{open}\AgdaSpace{}%
\AgdaKeyword{import}\AgdaSpace{}%
\AgdaModule{Data.List}\AgdaSpace{}%
\AgdaKeyword{hiding}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaOperator{\AgdaFunction{\AgdaUnderscore{}++\AgdaUnderscore{}}}\AgdaSymbol{)}\<%
\\
\>[0]\AgdaKeyword{open}\AgdaSpace{}%
\AgdaKeyword{import}\AgdaSpace{}%
\AgdaModule{Data.Unit}%
\>[23]\AgdaKeyword{hiding}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaOperator{\AgdaRecord{\AgdaUnderscore{}≤\AgdaUnderscore{}}}\AgdaSymbol{)}\<%
\\
\>[0]\AgdaKeyword{open}\AgdaSpace{}%
\AgdaKeyword{import}\AgdaSpace{}%
\AgdaModule{Data.Empty}\<%
\\
\>[0]\AgdaKeyword{open}\AgdaSpace{}%
\AgdaKeyword{import}\AgdaSpace{}%
\AgdaModule{Data.Maybe}\<%
\\
\>[0]\AgdaKeyword{open}\AgdaSpace{}%
\AgdaKeyword{import}\AgdaSpace{}%
\AgdaModule{Data.Bool}%
\>[23]\AgdaKeyword{hiding}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaOperator{\AgdaDatatype{\AgdaUnderscore{}≤\AgdaUnderscore{}}}\AgdaSpace{}%
\AgdaSymbol{;}\AgdaSpace{}%
\AgdaOperator{\AgdaFunction{if\AgdaUnderscore{}then\AgdaUnderscore{}else\AgdaUnderscore{}}}\AgdaSpace{}%
\AgdaSymbol{)}\AgdaSpace{}%
\AgdaKeyword{renaming}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaOperator{\AgdaFunction{\AgdaUnderscore{}∧\AgdaUnderscore{}}}\AgdaSpace{}%
\AgdaSymbol{to}\AgdaSpace{}%
\AgdaOperator{\AgdaFunction{\AgdaUnderscore{}∧b\AgdaUnderscore{}}}\AgdaSpace{}%
\AgdaSymbol{;}\AgdaSpace{}%
\AgdaOperator{\AgdaFunction{\AgdaUnderscore{}∨\AgdaUnderscore{}}}\AgdaSpace{}%
\AgdaSymbol{to}\AgdaSpace{}%
\AgdaOperator{\AgdaFunction{\AgdaUnderscore{}∨b\AgdaUnderscore{}}}\AgdaSpace{}%
\AgdaSymbol{;}\AgdaSpace{}%
\AgdaFunction{T}\AgdaSpace{}%
\AgdaSymbol{to}\AgdaSpace{}%
\AgdaFunction{True}\AgdaSymbol{)}\<%
\\
\>[0]\AgdaKeyword{open}\AgdaSpace{}%
\AgdaKeyword{import}\AgdaSpace{}%
\AgdaModule{Data.Bool.Base}\AgdaSpace{}%
\AgdaKeyword{hiding}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaOperator{\AgdaDatatype{\AgdaUnderscore{}≤\AgdaUnderscore{}}}\AgdaSpace{}%
\AgdaSymbol{;}\AgdaSpace{}%
\AgdaOperator{\AgdaFunction{if\AgdaUnderscore{}then\AgdaUnderscore{}else\AgdaUnderscore{}}}\AgdaSpace{}%
\AgdaSymbol{)}\AgdaSpace{}%
\AgdaKeyword{renaming}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaOperator{\AgdaFunction{\AgdaUnderscore{}∧\AgdaUnderscore{}}}\AgdaSpace{}%
\AgdaSymbol{to}\AgdaSpace{}%
\AgdaOperator{\AgdaFunction{\AgdaUnderscore{}∧b\AgdaUnderscore{}}}\AgdaSpace{}%
\AgdaSymbol{;}\AgdaSpace{}%
\AgdaOperator{\AgdaFunction{\AgdaUnderscore{}∨\AgdaUnderscore{}}}\AgdaSpace{}%
\AgdaSymbol{to}\AgdaSpace{}%
\AgdaOperator{\AgdaFunction{\AgdaUnderscore{}∨b\AgdaUnderscore{}}}\AgdaSpace{}%
\AgdaSymbol{;}\AgdaSpace{}%
\AgdaFunction{T}\AgdaSpace{}%
\AgdaSymbol{to}\AgdaSpace{}%
\AgdaFunction{True}\AgdaSymbol{)}\<%
\\
\>[0]\AgdaKeyword{open}\AgdaSpace{}%
\AgdaKeyword{import}\AgdaSpace{}%
\AgdaModule{Data.Product}\AgdaSpace{}%
\AgdaKeyword{renaming}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaOperator{\AgdaInductiveConstructor{\AgdaUnderscore{},\AgdaUnderscore{}}}\AgdaSpace{}%
\AgdaSymbol{to}\AgdaSpace{}%
\AgdaOperator{\AgdaInductiveConstructor{\AgdaUnderscore{},,\AgdaUnderscore{}}}\AgdaSpace{}%
\AgdaSymbol{)}\<%
\\
\>[0]\AgdaKeyword{open}\AgdaSpace{}%
\AgdaKeyword{import}\AgdaSpace{}%
\AgdaModule{Data.Nat.Base}\AgdaSpace{}%
\AgdaKeyword{hiding}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaOperator{\AgdaDatatype{\AgdaUnderscore{}≤\AgdaUnderscore{}}}\AgdaSymbol{)}\<%
\\
\>[0]\AgdaKeyword{open}\AgdaSpace{}%
\AgdaKeyword{import}\AgdaSpace{}%
\AgdaModule{Data.List.NonEmpty}\AgdaSpace{}%
\AgdaKeyword{hiding}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaField{head}\AgdaSymbol{)}\<%
\\
%
\\[\AgdaEmptyExtraSkip]%
\>[0]\AgdaKeyword{open}\AgdaSpace{}%
\AgdaKeyword{import}\AgdaSpace{}%
\AgdaModule{libraries.listLib}\<%
\\
\>[0]\AgdaKeyword{open}\AgdaSpace{}%
\AgdaKeyword{import}\AgdaSpace{}%
\AgdaModule{libraries.natLib}\<%
\\
\>[0]\AgdaKeyword{open}\AgdaSpace{}%
\AgdaKeyword{import}\AgdaSpace{}%
\AgdaModule{libraries.boolLib}\<%
\\
%
\\[\AgdaEmptyExtraSkip]%
\>[0]\AgdaKeyword{open}\AgdaSpace{}%
\AgdaKeyword{import}\AgdaSpace{}%
\AgdaModule{libraries.andLib}\<%
\\
\>[0]\AgdaKeyword{open}\AgdaSpace{}%
\AgdaKeyword{import}\AgdaSpace{}%
\AgdaModule{libraries.miscLib}\<%
\\
\>[0]\AgdaKeyword{open}\AgdaSpace{}%
\AgdaKeyword{import}\AgdaSpace{}%
\AgdaModule{libraries.maybeLib}\<%
\\
%
\\[\AgdaEmptyExtraSkip]%
\>[0]\AgdaKeyword{open}\AgdaSpace{}%
\AgdaKeyword{import}\AgdaSpace{}%
\AgdaModule{basicBitcoinDataType}\<%
\\
\>[0]\<%
\end{code}
} % END AgdaHide

\newcommand{\stackexamplestackdef}{
\begin{code}%
\>[0]\AgdaFunction{Stack}\AgdaSpace{}%
\AgdaSymbol{:}\AgdaSpace{}%
\AgdaPrimitive{Set}\<%
\\
\>[0]\AgdaFunction{Stack}\AgdaSpace{}%
\AgdaSymbol{=}\AgdaSpace{}%
\AgdaDatatype{List}\AgdaSpace{}%
\AgdaDatatype{ℕ}\<%
\end{code}
} % END newcommand

\AgdaHide{
\begin{code}%
\>[0]\<%
\\
\>[0]\AgdaFunction{stackHasSingletonTop}%
\>[22]\AgdaSymbol{:}\AgdaSpace{}%
\AgdaDatatype{ℕ}\AgdaSpace{}%
\AgdaSymbol{→}%
\>[30]\AgdaDatatype{Maybe}\AgdaSpace{}%
\AgdaFunction{Stack}\AgdaSpace{}%
\AgdaSymbol{→}%
\>[45]\AgdaDatatype{Bool}\<%
\\
\>[0]\AgdaFunction{stackHasSingletonTop}\AgdaSpace{}%
\AgdaBound{l}\AgdaSpace{}%
\AgdaInductiveConstructor{nothing}\AgdaSpace{}%
\AgdaSymbol{=}\AgdaSpace{}%
\AgdaInductiveConstructor{false}\<%
\\
\>[0]\AgdaFunction{stackHasSingletonTop}\AgdaSpace{}%
\AgdaBound{l}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaInductiveConstructor{just}\AgdaSpace{}%
\AgdaInductiveConstructor{[]}\AgdaSymbol{)}\AgdaSpace{}%
\AgdaSymbol{=}\AgdaSpace{}%
\AgdaInductiveConstructor{false}\<%
\\
\>[0]\AgdaFunction{stackHasSingletonTop}\AgdaSpace{}%
\AgdaBound{l}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaInductiveConstructor{just}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaBound{z}\AgdaSpace{}%
\AgdaOperator{\AgdaInductiveConstructor{∷}}\AgdaSpace{}%
\AgdaBound{y}\AgdaSymbol{))}\AgdaSpace{}%
\AgdaSymbol{=}%
\>[41]\AgdaBound{l}%
\>[44]\AgdaOperator{\AgdaFunction{==b}}\AgdaSpace{}%
\AgdaBound{z}\<%
\\
%
\\[\AgdaEmptyExtraSkip]%
%
\\[\AgdaEmptyExtraSkip]%
\>[0]\AgdaFunction{stackHasTop}%
\>[13]\AgdaSymbol{:}%
\>[17]\AgdaDatatype{List}\AgdaSpace{}%
\AgdaDatatype{ℕ}\AgdaSpace{}%
\AgdaSymbol{→}%
\>[27]\AgdaDatatype{Maybe}%
\>[34]\AgdaFunction{Stack}\AgdaSpace{}%
\AgdaSymbol{→}\AgdaSpace{}%
\AgdaPrimitive{Set}\<%
\\
\>[0]\AgdaFunction{stackHasTop}\AgdaSpace{}%
\AgdaInductiveConstructor{[]}\AgdaSpace{}%
\AgdaBound{m}\AgdaSpace{}%
\AgdaSymbol{=}\AgdaSpace{}%
\AgdaRecord{⊤}\<%
\\
\>[0]\AgdaFunction{stackHasTop}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaBound{y}\AgdaSpace{}%
\AgdaOperator{\AgdaInductiveConstructor{∷}}\AgdaSpace{}%
\AgdaBound{n}\AgdaSymbol{)}\AgdaSpace{}%
\AgdaBound{m}\AgdaSpace{}%
\AgdaSymbol{=}\AgdaSpace{}%
\AgdaFunction{True}\AgdaSymbol{(}\AgdaFunction{stackHasSingletonTop}\AgdaSpace{}%
\AgdaBound{y}\AgdaSpace{}%
\AgdaBound{m}\AgdaSymbol{)}\<%
\\
%
\\[\AgdaEmptyExtraSkip]%
\>[0]\AgdaFunction{stackAuxFunction}\AgdaSpace{}%
\AgdaSymbol{:}%
\>[20]\AgdaFunction{Stack}\AgdaSpace{}%
\AgdaSymbol{→}\AgdaSpace{}%
\AgdaDatatype{Bool}\AgdaSpace{}%
\AgdaSymbol{→}\AgdaSpace{}%
\AgdaDatatype{Maybe}\AgdaSpace{}%
\AgdaFunction{Stack}\<%
\\
\>[0]\AgdaFunction{stackAuxFunction}\AgdaSpace{}%
\AgdaBound{s}\AgdaSpace{}%
\AgdaBound{b}\AgdaSpace{}%
\AgdaSymbol{=}\AgdaSpace{}%
\AgdaInductiveConstructor{just}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaFunction{boolToNat}\AgdaSpace{}%
\AgdaBound{b}\AgdaSpace{}%
\AgdaOperator{\AgdaInductiveConstructor{∷}}\AgdaSpace{}%
\AgdaBound{s}\AgdaSymbol{)}\<%
\\
%
\\[\AgdaEmptyExtraSkip]%
%
\\[\AgdaEmptyExtraSkip]%
\>[0]\AgdaComment{--\ Stack\ transformer}\<%
\\
\>[0]\AgdaFunction{StackTransformer}\AgdaSpace{}%
\AgdaSymbol{:}\AgdaSpace{}%
\AgdaPrimitive{Set}\<%
\\
\>[0]\AgdaFunction{StackTransformer}\AgdaSpace{}%
\AgdaSymbol{=}\AgdaSpace{}%
\AgdaFunction{Time}\AgdaSpace{}%
\AgdaSymbol{→}\AgdaSpace{}%
\AgdaDatatype{Msg}\AgdaSpace{}%
\AgdaSymbol{→}\AgdaSpace{}%
\AgdaFunction{Stack}\AgdaSpace{}%
\AgdaSymbol{→}\AgdaSpace{}%
\AgdaDatatype{Maybe}\AgdaSpace{}%
\AgdaFunction{Stack}\<%
\\
%
\\[\AgdaEmptyExtraSkip]%
\>[0]\AgdaComment{--\ function\ that\ checking\ if\ the\ stack\ is\ empty\ or\ the\ top\ element\ is\ false}\<%
\\
\>[0]\AgdaFunction{checkStackAux}\AgdaSpace{}%
\AgdaSymbol{:}\AgdaSpace{}%
\AgdaFunction{Stack}\AgdaSpace{}%
\AgdaSymbol{→}\AgdaSpace{}%
\AgdaDatatype{Bool}\<%
\\
\>[0]\AgdaFunction{checkStackAux}\AgdaSpace{}%
\AgdaInductiveConstructor{[]}%
\>[18]\AgdaSymbol{=}\AgdaSpace{}%
\AgdaInductiveConstructor{false}\<%
\\
\>[0]\AgdaFunction{checkStackAux}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaInductiveConstructor{zero}\AgdaSpace{}%
\AgdaOperator{\AgdaInductiveConstructor{∷}}\AgdaSpace{}%
\AgdaBound{bitcoinStack₁}\AgdaSymbol{)}%
\>[38]\AgdaSymbol{=}\AgdaSpace{}%
\AgdaInductiveConstructor{false}\<%
\\
\>[0]\AgdaFunction{checkStackAux}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaInductiveConstructor{suc}\AgdaSpace{}%
\AgdaBound{x}\AgdaSpace{}%
\AgdaOperator{\AgdaInductiveConstructor{∷}}\AgdaSpace{}%
\AgdaBound{bitcoinStack₁}\AgdaSymbol{)}%
\>[39]\AgdaSymbol{=}\AgdaSpace{}%
\AgdaInductiveConstructor{true}\<%
\\
%
\\[\AgdaEmptyExtraSkip]%
\>[0]\AgdaComment{--\ lifting\ the\ checkStackAux\ to\ Maybe\ StackIfStack\ data\ type}\<%
\\
\>[0]\AgdaFunction{checkStack}\AgdaSpace{}%
\AgdaSymbol{:}%
\>[14]\AgdaDatatype{Maybe}\AgdaSpace{}%
\AgdaFunction{Stack}%
\>[28]\AgdaSymbol{→}\AgdaSpace{}%
\AgdaDatatype{Bool}\<%
\\
\>[0]\AgdaFunction{checkStack}\AgdaSpace{}%
\AgdaInductiveConstructor{nothing}\AgdaSpace{}%
\AgdaSymbol{=}\AgdaSpace{}%
\AgdaInductiveConstructor{false}\<%
\\
\>[0]\AgdaFunction{checkStack}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaInductiveConstructor{just}\AgdaSpace{}%
\AgdaBound{x}\AgdaSymbol{)}\AgdaSpace{}%
\AgdaSymbol{=}\AgdaSpace{}%
\AgdaFunction{checkStackAux}\AgdaSpace{}%
\AgdaBound{x}\<%
\end{code}
} % END AgdaHide


==> latex-before-sed/stackPredicate.tex <==
%% This file has been generated automatically by mkLagda.awk
%% DO NOT EDIT! ALL YOUR CHANGES WILL BE LOST!

\AgdaHide{
\begin{code}%
\>[0]\AgdaComment{--\textbackslash{}stackPredicate}\<%
\\
\>[0]\AgdaKeyword{module}\AgdaSpace{}%
\AgdaModule{stackPredicate}\AgdaSpace{}%
\AgdaKeyword{where}\<%
\\
%
\\[\AgdaEmptyExtraSkip]%
\>[0]\AgdaKeyword{open}\AgdaSpace{}%
\AgdaKeyword{import}\AgdaSpace{}%
\AgdaModule{Data.Nat}%
\>[22]\AgdaKeyword{hiding}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaOperator{\AgdaDatatype{\AgdaUnderscore{}≤\AgdaUnderscore{}}}\AgdaSymbol{)}\<%
\\
\>[0]\AgdaKeyword{open}\AgdaSpace{}%
\AgdaKeyword{import}\AgdaSpace{}%
\AgdaModule{Data.List}\AgdaSpace{}%
\AgdaKeyword{hiding}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaOperator{\AgdaFunction{\AgdaUnderscore{}++\AgdaUnderscore{}}}\AgdaSymbol{)}\<%
\\
\>[0]\AgdaKeyword{open}\AgdaSpace{}%
\AgdaKeyword{import}\AgdaSpace{}%
\AgdaModule{Data.Unit}%
\>[23]\AgdaKeyword{hiding}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaOperator{\AgdaRecord{\AgdaUnderscore{}≤\AgdaUnderscore{}}}\AgdaSymbol{)}\<%
\\
\>[0]\AgdaKeyword{open}\AgdaSpace{}%
\AgdaKeyword{import}\AgdaSpace{}%
\AgdaModule{Data.Empty}\<%
\\
\>[0]\AgdaKeyword{open}\AgdaSpace{}%
\AgdaKeyword{import}\AgdaSpace{}%
\AgdaModule{Data.Sum}\<%
\\
\>[0]\AgdaKeyword{open}\AgdaSpace{}%
\AgdaKeyword{import}\AgdaSpace{}%
\AgdaModule{Data.Maybe}\<%
\\
\>[0]\AgdaKeyword{open}\AgdaSpace{}%
\AgdaKeyword{import}\AgdaSpace{}%
\AgdaModule{Data.Bool}%
\>[23]\AgdaKeyword{hiding}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaOperator{\AgdaDatatype{\AgdaUnderscore{}≤\AgdaUnderscore{}}}\AgdaSpace{}%
\AgdaSymbol{;}\AgdaSpace{}%
\AgdaOperator{\AgdaFunction{if\AgdaUnderscore{}then\AgdaUnderscore{}else\AgdaUnderscore{}}}\AgdaSpace{}%
\AgdaSymbol{)}\AgdaSpace{}%
\AgdaKeyword{renaming}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaOperator{\AgdaFunction{\AgdaUnderscore{}∧\AgdaUnderscore{}}}\AgdaSpace{}%
\AgdaSymbol{to}\AgdaSpace{}%
\AgdaOperator{\AgdaFunction{\AgdaUnderscore{}∧b\AgdaUnderscore{}}}\AgdaSpace{}%
\AgdaSymbol{;}\AgdaSpace{}%
\AgdaOperator{\AgdaFunction{\AgdaUnderscore{}∨\AgdaUnderscore{}}}\AgdaSpace{}%
\AgdaSymbol{to}\AgdaSpace{}%
\AgdaOperator{\AgdaFunction{\AgdaUnderscore{}∨b\AgdaUnderscore{}}}\AgdaSpace{}%
\AgdaSymbol{;}\AgdaSpace{}%
\AgdaFunction{T}\AgdaSpace{}%
\AgdaSymbol{to}\AgdaSpace{}%
\AgdaFunction{True}\AgdaSymbol{)}\<%
\\
\>[0]\AgdaKeyword{open}\AgdaSpace{}%
\AgdaKeyword{import}\AgdaSpace{}%
\AgdaModule{Data.Bool.Base}\AgdaSpace{}%
\AgdaKeyword{hiding}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaOperator{\AgdaDatatype{\AgdaUnderscore{}≤\AgdaUnderscore{}}}\AgdaSpace{}%
\AgdaSymbol{;}\AgdaSpace{}%
\AgdaOperator{\AgdaFunction{if\AgdaUnderscore{}then\AgdaUnderscore{}else\AgdaUnderscore{}}}\AgdaSpace{}%
\AgdaSymbol{)}\AgdaSpace{}%
\AgdaKeyword{renaming}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaOperator{\AgdaFunction{\AgdaUnderscore{}∧\AgdaUnderscore{}}}\AgdaSpace{}%
\AgdaSymbol{to}\AgdaSpace{}%
\AgdaOperator{\AgdaFunction{\AgdaUnderscore{}∧b\AgdaUnderscore{}}}\AgdaSpace{}%
\AgdaSymbol{;}\AgdaSpace{}%
\AgdaOperator{\AgdaFunction{\AgdaUnderscore{}∨\AgdaUnderscore{}}}\AgdaSpace{}%
\AgdaSymbol{to}\AgdaSpace{}%
\AgdaOperator{\AgdaFunction{\AgdaUnderscore{}∨b\AgdaUnderscore{}}}\AgdaSpace{}%
\AgdaSymbol{;}\AgdaSpace{}%
\AgdaFunction{T}\AgdaSpace{}%
\AgdaSymbol{to}\AgdaSpace{}%
\AgdaFunction{True}\AgdaSymbol{)}\<%
\\
\>[0]\AgdaKeyword{open}\AgdaSpace{}%
\AgdaKeyword{import}\AgdaSpace{}%
\AgdaModule{Data.Product}\AgdaSpace{}%
\AgdaKeyword{renaming}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaOperator{\AgdaInductiveConstructor{\AgdaUnderscore{},\AgdaUnderscore{}}}\AgdaSpace{}%
\AgdaSymbol{to}\AgdaSpace{}%
\AgdaOperator{\AgdaInductiveConstructor{\AgdaUnderscore{},,\AgdaUnderscore{}}}\AgdaSpace{}%
\AgdaSymbol{)}\<%
\\
\>[0]\AgdaKeyword{open}\AgdaSpace{}%
\AgdaKeyword{import}\AgdaSpace{}%
\AgdaModule{Data.Nat.Base}\AgdaSpace{}%
\AgdaKeyword{hiding}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaOperator{\AgdaDatatype{\AgdaUnderscore{}≤\AgdaUnderscore{}}}\AgdaSymbol{)}\<%
\\
\>[0]\AgdaKeyword{open}\AgdaSpace{}%
\AgdaKeyword{import}\AgdaSpace{}%
\AgdaModule{Data.List.NonEmpty}\AgdaSpace{}%
\AgdaKeyword{hiding}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaField{head}\AgdaSymbol{)}\<%
\\
\>[0]\AgdaKeyword{import}\AgdaSpace{}%
\AgdaModule{Relation.Binary.PropositionalEquality}\AgdaSpace{}%
\AgdaSymbol{as}\AgdaSpace{}%
\AgdaModule{Eq}\<%
\\
\>[0]\AgdaKeyword{open}\AgdaSpace{}%
\AgdaModule{Eq}\AgdaSpace{}%
\AgdaKeyword{using}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaOperator{\AgdaDatatype{\AgdaUnderscore{}≡\AgdaUnderscore{}}}\AgdaSymbol{;}\AgdaSpace{}%
\AgdaInductiveConstructor{refl}\AgdaSymbol{;}\AgdaSpace{}%
\AgdaFunction{cong}\AgdaSymbol{;}\AgdaSpace{}%
\AgdaKeyword{module}\AgdaSpace{}%
\AgdaModule{≡-Reasoning}\AgdaSymbol{;}\AgdaSpace{}%
\AgdaFunction{sym}\AgdaSymbol{)}\<%
\\
\>[0]\AgdaKeyword{open}\AgdaSpace{}%
\AgdaModule{≡-Reasoning}\<%
\\
\>[0]\AgdaKeyword{open}\AgdaSpace{}%
\AgdaKeyword{import}\AgdaSpace{}%
\AgdaModule{Agda.Builtin.Equality}\<%
\\
%
\\[\AgdaEmptyExtraSkip]%
\>[0]\AgdaKeyword{open}\AgdaSpace{}%
\AgdaKeyword{import}\AgdaSpace{}%
\AgdaModule{libraries.listLib}\<%
\\
\>[0]\AgdaKeyword{open}\AgdaSpace{}%
\AgdaKeyword{import}\AgdaSpace{}%
\AgdaModule{libraries.natLib}\<%
\\
\>[0]\AgdaKeyword{open}\AgdaSpace{}%
\AgdaKeyword{import}\AgdaSpace{}%
\AgdaModule{libraries.boolLib}\<%
\\
\>[0]\AgdaKeyword{open}\AgdaSpace{}%
\AgdaKeyword{import}\AgdaSpace{}%
\AgdaModule{libraries.andLib}\<%
\\
\>[0]\AgdaKeyword{open}\AgdaSpace{}%
\AgdaKeyword{import}\AgdaSpace{}%
\AgdaModule{libraries.miscLib}\<%
\\
\>[0]\AgdaKeyword{open}\AgdaSpace{}%
\AgdaKeyword{import}\AgdaSpace{}%
\AgdaModule{libraries.maybeLib}\<%
\\
%
\\[\AgdaEmptyExtraSkip]%
%
\\[\AgdaEmptyExtraSkip]%
\>[0]\AgdaKeyword{open}\AgdaSpace{}%
\AgdaKeyword{import}\AgdaSpace{}%
\AgdaModule{stack}\<%
\\
\>[0]\AgdaKeyword{open}\AgdaSpace{}%
\AgdaKeyword{import}\AgdaSpace{}%
\AgdaModule{basicBitcoinDataType}\<%
\\
%
\\[\AgdaEmptyExtraSkip]%
%
\\[\AgdaEmptyExtraSkip]%
\>[0]\AgdaFunction{StackPredicate}\AgdaSpace{}%
\AgdaSymbol{:}\AgdaSpace{}%
\AgdaPrimitive{Set₁}\<%
\\
\>[0]\AgdaComment{--\textbackslash{}stackPredicateStackPred}\<%
\end{code}
} % END AgdaHide

\newcommand{\stackPredicateStackPred}{
\begin{code}[inline]%
\>[0]\AgdaFunction{StackPredicate}\AgdaSpace{}%
\AgdaSymbol{=}\AgdaSpace{}%
\AgdaFunction{Time}\AgdaSpace{}%
\AgdaSymbol{→}\AgdaSpace{}%
\AgdaDatatype{Msg}\AgdaSpace{}%
\AgdaSymbol{→}\AgdaSpace{}%
\AgdaFunction{Stack}\AgdaSpace{}%
\AgdaSymbol{→}\AgdaSpace{}%
\AgdaPrimitive{Set}\<%
\end{code}
} % END newcommand

\AgdaHide{
\begin{code}%
\>[0]\<%
\\
\>[0]\AgdaOperator{\AgdaFunction{\AgdaUnderscore{}⊎sp\AgdaUnderscore{}}}%
\>[8]\AgdaSymbol{:}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaBound{φ}\AgdaSpace{}%
\AgdaBound{ψ}\AgdaSpace{}%
\AgdaSymbol{:}\AgdaSpace{}%
\AgdaFunction{StackPredicate}\AgdaSymbol{)}\AgdaSpace{}%
\AgdaSymbol{→}\AgdaSpace{}%
\AgdaFunction{StackPredicate}\<%
\\
\>[0]\AgdaSymbol{(}\AgdaBound{φ}%
\>[4]\AgdaOperator{\AgdaFunction{⊎sp}}%
\>[9]\AgdaBound{ψ}\AgdaSymbol{)}%
\>[13]\AgdaBound{t}\AgdaSpace{}%
\AgdaBound{m}\AgdaSpace{}%
\AgdaBound{st}\AgdaSpace{}%
\AgdaSymbol{=}\AgdaSpace{}%
\AgdaBound{φ}%
\>[25]\AgdaBound{t}\AgdaSpace{}%
\AgdaBound{m}\AgdaSpace{}%
\AgdaBound{st}%
\>[33]\AgdaOperator{\AgdaDatatype{⊎}}\AgdaSpace{}%
\AgdaBound{ψ}%
\>[38]\AgdaBound{t}\AgdaSpace{}%
\AgdaBound{m}\AgdaSpace{}%
\AgdaBound{st}\<%
\\
%
\\[\AgdaEmptyExtraSkip]%
\>[0]\AgdaOperator{\AgdaFunction{\AgdaUnderscore{}∧sp\AgdaUnderscore{}}}\AgdaSpace{}%
\AgdaSymbol{:}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaSpace{}%
\AgdaBound{φ}\AgdaSpace{}%
\AgdaBound{ψ}%
\>[15]\AgdaSymbol{:}\AgdaSpace{}%
\AgdaFunction{StackPredicate}\AgdaSpace{}%
\AgdaSymbol{)}\AgdaSpace{}%
\AgdaSymbol{→}\AgdaSpace{}%
\AgdaFunction{StackPredicate}\<%
\\
\>[0]\AgdaSymbol{(}\AgdaBound{φ}\AgdaSpace{}%
\AgdaOperator{\AgdaFunction{∧sp}}\AgdaSpace{}%
\AgdaBound{ψ}\AgdaSpace{}%
\AgdaSymbol{)}\AgdaSpace{}%
\AgdaBound{t}\AgdaSpace{}%
\AgdaBound{m}\AgdaSpace{}%
\AgdaBound{s}%
\>[19]\AgdaSymbol{=}%
\>[22]\AgdaBound{φ}\AgdaSpace{}%
\AgdaBound{t}\AgdaSpace{}%
\AgdaBound{m}\AgdaSpace{}%
\AgdaBound{s}%
\>[31]\AgdaOperator{\AgdaRecord{∧}}%
\>[34]\AgdaBound{ψ}\AgdaSpace{}%
\AgdaBound{t}\AgdaSpace{}%
\AgdaBound{m}\AgdaSpace{}%
\AgdaBound{s}\<%
\\
%
\\[\AgdaEmptyExtraSkip]%
%
\\[\AgdaEmptyExtraSkip]%
\>[0]\AgdaFunction{truePredaux}\AgdaSpace{}%
\AgdaSymbol{:}\AgdaSpace{}%
\AgdaFunction{StackPredicate}\AgdaSpace{}%
\AgdaSymbol{→}\AgdaSpace{}%
\AgdaFunction{StackPredicate}\<%
\\
\>[0]\AgdaFunction{truePredaux}\AgdaSpace{}%
\AgdaBound{φ}\AgdaSpace{}%
\AgdaBound{time}\AgdaSpace{}%
\AgdaBound{msg}\AgdaSpace{}%
\AgdaInductiveConstructor{[]}\AgdaSpace{}%
\AgdaSymbol{=}\AgdaSpace{}%
\AgdaDatatype{⊥}\<%
\\
\>[0]\AgdaFunction{truePredaux}\AgdaSpace{}%
\AgdaBound{φ}\AgdaSpace{}%
\AgdaBound{time}\AgdaSpace{}%
\AgdaBound{msg}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaInductiveConstructor{zero}\AgdaSpace{}%
\AgdaOperator{\AgdaInductiveConstructor{∷}}\AgdaSpace{}%
\AgdaBound{st}\AgdaSymbol{)}\AgdaSpace{}%
\AgdaSymbol{=}\AgdaSpace{}%
\AgdaDatatype{⊥}\<%
\\
\>[0]\AgdaFunction{truePredaux}\AgdaSpace{}%
\AgdaBound{φ}\AgdaSpace{}%
\AgdaBound{time}\AgdaSpace{}%
\AgdaBound{msg}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaInductiveConstructor{suc}\AgdaSpace{}%
\AgdaBound{x}\AgdaSpace{}%
\AgdaOperator{\AgdaInductiveConstructor{∷}}\AgdaSpace{}%
\AgdaBound{st}\AgdaSymbol{)}\AgdaSpace{}%
\AgdaSymbol{=}\AgdaSpace{}%
\AgdaBound{φ}\AgdaSpace{}%
\AgdaBound{time}\AgdaSpace{}%
\AgdaBound{msg}%
\>[50]\AgdaBound{st}\<%
\\
%
\\[\AgdaEmptyExtraSkip]%
\>[0]\AgdaComment{--\ acceptingBasic\ :\ Time\ →\ Msg\ →\ Stack\ →\ Bool}\<%
\\
\>[0]\AgdaComment{--\ acceptingBasic\ time\ msg₁\ []\ =\ false}\<%
\\
\>[0]\AgdaComment{--\ acceptingBasic\ time\ msg₁\ (x\ ∷\ stack₁)\ =\ notFalse\ x}\<%
\\
%
\\[\AgdaEmptyExtraSkip]%
\>[0]\AgdaComment{--\textbackslash{}stackPredicateacceptState}\<%
\end{code}
} % END AgdaHide

\newcommand{\stackPredicateacceptState}{
\begin{code}%
\>[0]\AgdaFunction{acceptStateˢ}\AgdaSpace{}%
\AgdaSymbol{:}\AgdaSpace{}%
\AgdaFunction{StackPredicate}\<%
\\
\>[0]\AgdaFunction{acceptStateˢ}%
\>[14]\AgdaBound{time}%
\>[20]\AgdaBound{msg₁}%
\>[26]\AgdaInductiveConstructor{[]}%
\>[40]\AgdaSymbol{=}%
\>[43]\AgdaDatatype{⊥}\<%
\\
\>[0]\AgdaFunction{acceptStateˢ}%
\>[14]\AgdaBound{time}%
\>[20]\AgdaBound{msg₁}%
\>[26]\AgdaSymbol{(}\AgdaBound{x}\AgdaSpace{}%
\AgdaOperator{\AgdaInductiveConstructor{∷}}\AgdaSpace{}%
\AgdaBound{stack₁}\AgdaSymbol{)}%
\>[40]\AgdaSymbol{=}%
\>[43]\AgdaFunction{NotFalse}\AgdaSpace{}%
\AgdaBound{x}\<%
\\
\>[0]\<%
\end{code}
} % END newcommand

\AgdaHide{
\begin{code}%
\>[0]\<%
\end{code}
} % END AgdaHide


==> latex-before-sed/verificationMultiSig.tex <==
%% This file has been generated automatically by mkLagda.awk
%% DO NOT EDIT! ALL YOUR CHANGES WILL BE LOST!

\AgdaHide{
\begin{code}%
\>[0]\AgdaComment{--\textbackslash{}multisig}\<%
\\
%
\\[\AgdaEmptyExtraSkip]%
\>[0]\AgdaComment{\{-\ OPTIONS\ --allow-unsolved-metas\ \#-\}}\<%
\\
%
\\[\AgdaEmptyExtraSkip]%
\>[0]\AgdaKeyword{open}\AgdaSpace{}%
\AgdaKeyword{import}\AgdaSpace{}%
\AgdaModule{basicBitcoinDataType}\<%
\\
%
\\[\AgdaEmptyExtraSkip]%
\>[0]\AgdaKeyword{module}\AgdaSpace{}%
\AgdaModule{verificationMultiSig}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaBound{param}\AgdaSpace{}%
\AgdaSymbol{:}\AgdaSpace{}%
\AgdaRecord{GlobalParameters}\AgdaSymbol{)}\AgdaSpace{}%
\AgdaKeyword{where}\<%
\\
%
\\[\AgdaEmptyExtraSkip]%
%
\\[\AgdaEmptyExtraSkip]%
\>[0]\AgdaKeyword{open}\AgdaSpace{}%
\AgdaKeyword{import}\AgdaSpace{}%
\AgdaModule{Data.List.Base}\AgdaSpace{}%
\AgdaKeyword{hiding}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaOperator{\AgdaFunction{\AgdaUnderscore{}++\AgdaUnderscore{}}}\AgdaSpace{}%
\AgdaSymbol{)}\<%
\\
\>[0]\AgdaKeyword{open}\AgdaSpace{}%
\AgdaKeyword{import}\AgdaSpace{}%
\AgdaModule{Data.Nat}%
\>[22]\AgdaKeyword{renaming}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaOperator{\AgdaDatatype{\AgdaUnderscore{}≤\AgdaUnderscore{}}}\AgdaSpace{}%
\AgdaSymbol{to}\AgdaSpace{}%
\AgdaOperator{\AgdaDatatype{\AgdaUnderscore{}≤'\AgdaUnderscore{}}}\AgdaSymbol{)}\AgdaSpace{}%
\AgdaComment{--\ \ \AgdaUnderscore{}<\AgdaUnderscore{}\ to\ \AgdaUnderscore{}<'\AgdaUnderscore{})}\<%
\\
\>[0]\AgdaKeyword{open}\AgdaSpace{}%
\AgdaKeyword{import}\AgdaSpace{}%
\AgdaModule{Data.List}\AgdaSpace{}%
\AgdaKeyword{hiding}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaOperator{\AgdaFunction{\AgdaUnderscore{}++\AgdaUnderscore{}}}%
\>[36]\AgdaSymbol{)}\<%
\\
\>[0]\AgdaKeyword{open}\AgdaSpace{}%
\AgdaKeyword{import}\AgdaSpace{}%
\AgdaModule{Data.Sum}\<%
\\
\>[0]\AgdaKeyword{open}\AgdaSpace{}%
\AgdaKeyword{import}\AgdaSpace{}%
\AgdaModule{Data.Unit}%
\>[23]\AgdaKeyword{hiding}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaOperator{\AgdaRecord{\AgdaUnderscore{}≤\AgdaUnderscore{}}}\AgdaSymbol{)}\<%
\\
\>[0]\AgdaKeyword{open}\AgdaSpace{}%
\AgdaKeyword{import}\AgdaSpace{}%
\AgdaModule{Data.Empty}\<%
\\
\>[0]\AgdaKeyword{open}\AgdaSpace{}%
\AgdaKeyword{import}\AgdaSpace{}%
\AgdaModule{Data.Maybe}\<%
\\
\>[0]\AgdaComment{--open\ import\ Data.List.Base}\<%
\\
\>[0]\AgdaKeyword{open}\AgdaSpace{}%
\AgdaKeyword{import}\AgdaSpace{}%
\AgdaModule{Data.Bool}%
\>[23]\AgdaKeyword{hiding}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaOperator{\AgdaDatatype{\AgdaUnderscore{}≤\AgdaUnderscore{}}}\AgdaSpace{}%
\AgdaSymbol{;}\AgdaSpace{}%
\AgdaOperator{\AgdaDatatype{\AgdaUnderscore{}<\AgdaUnderscore{}}}\AgdaSpace{}%
\AgdaSymbol{;}\AgdaSpace{}%
\AgdaOperator{\AgdaFunction{if\AgdaUnderscore{}then\AgdaUnderscore{}else\AgdaUnderscore{}}}%
\>[58]\AgdaSymbol{)}%
\>[61]\AgdaKeyword{renaming}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaOperator{\AgdaFunction{\AgdaUnderscore{}∧\AgdaUnderscore{}}}\AgdaSpace{}%
\AgdaSymbol{to}\AgdaSpace{}%
\AgdaOperator{\AgdaFunction{\AgdaUnderscore{}∧b\AgdaUnderscore{}}}\AgdaSpace{}%
\AgdaSymbol{;}\AgdaSpace{}%
\AgdaOperator{\AgdaFunction{\AgdaUnderscore{}∨\AgdaUnderscore{}}}\AgdaSpace{}%
\AgdaSymbol{to}\AgdaSpace{}%
\AgdaOperator{\AgdaFunction{\AgdaUnderscore{}∨b\AgdaUnderscore{}}}\AgdaSpace{}%
\AgdaSymbol{;}\AgdaSpace{}%
\AgdaFunction{T}\AgdaSpace{}%
\AgdaSymbol{to}\AgdaSpace{}%
\AgdaFunction{True}\AgdaSymbol{)}\<%
\\
\>[0]\AgdaKeyword{open}\AgdaSpace{}%
\AgdaKeyword{import}\AgdaSpace{}%
\AgdaModule{Data.Product}\AgdaSpace{}%
\AgdaKeyword{renaming}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaOperator{\AgdaInductiveConstructor{\AgdaUnderscore{},\AgdaUnderscore{}}}\AgdaSpace{}%
\AgdaSymbol{to}\AgdaSpace{}%
\AgdaOperator{\AgdaInductiveConstructor{\AgdaUnderscore{},,\AgdaUnderscore{}}}\AgdaSpace{}%
\AgdaSymbol{)}\<%
\\
\>[0]\AgdaKeyword{open}\AgdaSpace{}%
\AgdaKeyword{import}\AgdaSpace{}%
\AgdaModule{Data.Nat.Base}\AgdaSpace{}%
\AgdaKeyword{hiding}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaOperator{\AgdaDatatype{\AgdaUnderscore{}≤\AgdaUnderscore{}}}\AgdaSpace{}%
\AgdaSymbol{;}\AgdaSpace{}%
\AgdaOperator{\AgdaFunction{\AgdaUnderscore{}<\AgdaUnderscore{}}}\AgdaSymbol{)}\<%
\\
\>[0]\AgdaKeyword{open}\AgdaSpace{}%
\AgdaKeyword{import}\AgdaSpace{}%
\AgdaModule{Data.List.NonEmpty}\AgdaSpace{}%
\AgdaKeyword{hiding}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaField{head}\AgdaSymbol{;}\AgdaSpace{}%
\AgdaOperator{\AgdaFunction{[\AgdaUnderscore{}]}}\AgdaSymbol{;}\AgdaSpace{}%
\AgdaFunction{length}\AgdaSymbol{)}\<%
\\
\>[0]\AgdaKeyword{open}\AgdaSpace{}%
\AgdaKeyword{import}\AgdaSpace{}%
\AgdaModule{Data.Nat}\AgdaSpace{}%
\AgdaKeyword{using}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaDatatype{ℕ}\AgdaSymbol{;}\AgdaSpace{}%
\AgdaOperator{\AgdaPrimitive{\AgdaUnderscore{}+\AgdaUnderscore{}}}\AgdaSymbol{;}\AgdaSpace{}%
\AgdaOperator{\AgdaFunction{\AgdaUnderscore{}≥\AgdaUnderscore{}}}\AgdaSymbol{;}\AgdaSpace{}%
\AgdaOperator{\AgdaFunction{\AgdaUnderscore{}>\AgdaUnderscore{}}}\AgdaSymbol{;}\AgdaSpace{}%
\AgdaInductiveConstructor{zero}\AgdaSymbol{;}\AgdaSpace{}%
\AgdaInductiveConstructor{suc}\AgdaSymbol{;}\AgdaSpace{}%
\AgdaInductiveConstructor{s≤s}\AgdaSymbol{;}\AgdaSpace{}%
\AgdaInductiveConstructor{z≤n}\AgdaSymbol{)}\<%
\\
\>[0]\AgdaKeyword{import}\AgdaSpace{}%
\AgdaModule{Relation.Binary.PropositionalEquality}\AgdaSpace{}%
\AgdaSymbol{as}\AgdaSpace{}%
\AgdaModule{Eq}\<%
\\
\>[0]\AgdaKeyword{open}\AgdaSpace{}%
\AgdaModule{Eq}\AgdaSpace{}%
\AgdaKeyword{using}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaOperator{\AgdaDatatype{\AgdaUnderscore{}≡\AgdaUnderscore{}}}\AgdaSymbol{;}\AgdaSpace{}%
\AgdaInductiveConstructor{refl}\AgdaSymbol{;}\AgdaSpace{}%
\AgdaFunction{cong}\AgdaSymbol{;}\AgdaSpace{}%
\AgdaKeyword{module}\AgdaSpace{}%
\AgdaModule{≡-Reasoning}\AgdaSymbol{;}\AgdaSpace{}%
\AgdaFunction{sym}\AgdaSymbol{)}\<%
\\
\>[0]\AgdaKeyword{open}\AgdaSpace{}%
\AgdaModule{≡-Reasoning}\<%
\\
\>[0]\AgdaKeyword{open}\AgdaSpace{}%
\AgdaKeyword{import}\AgdaSpace{}%
\AgdaModule{Agda.Builtin.Equality}\<%
\\
\>[0]\AgdaComment{--open\ import\ Agda.Builtin.Equality.Rewrite}\<%
\\
%
\\[\AgdaEmptyExtraSkip]%
\>[0]\AgdaKeyword{open}\AgdaSpace{}%
\AgdaKeyword{import}\AgdaSpace{}%
\AgdaModule{libraries.listLib}\<%
\\
\>[0]\AgdaKeyword{open}\AgdaSpace{}%
\AgdaKeyword{import}\AgdaSpace{}%
\AgdaModule{libraries.emptyLib}\<%
\\
\>[0]\AgdaKeyword{open}\AgdaSpace{}%
\AgdaKeyword{import}\AgdaSpace{}%
\AgdaModule{libraries.natLib}\<%
\\
\>[0]\AgdaKeyword{open}\AgdaSpace{}%
\AgdaKeyword{import}\AgdaSpace{}%
\AgdaModule{libraries.boolLib}\<%
\\
\>[0]\AgdaKeyword{open}\AgdaSpace{}%
\AgdaKeyword{import}\AgdaSpace{}%
\AgdaModule{libraries.equalityLib}\<%
\\
%
\\[\AgdaEmptyExtraSkip]%
%
\\[\AgdaEmptyExtraSkip]%
%
\\[\AgdaEmptyExtraSkip]%
\>[0]\AgdaKeyword{open}\AgdaSpace{}%
\AgdaKeyword{import}\AgdaSpace{}%
\AgdaModule{libraries.andLib}\<%
\\
\>[0]\AgdaKeyword{open}\AgdaSpace{}%
\AgdaKeyword{import}\AgdaSpace{}%
\AgdaModule{libraries.miscLib}\<%
\\
\>[0]\AgdaKeyword{open}\AgdaSpace{}%
\AgdaKeyword{import}\AgdaSpace{}%
\AgdaModule{libraries.maybeLib}\<%
\\
%
\\[\AgdaEmptyExtraSkip]%
\>[0]\AgdaKeyword{open}\AgdaSpace{}%
\AgdaKeyword{import}\AgdaSpace{}%
\AgdaModule{stack}\<%
\\
\>[0]\AgdaKeyword{open}\AgdaSpace{}%
\AgdaKeyword{import}\AgdaSpace{}%
\AgdaModule{stackPredicate}\<%
\\
\>[0]\AgdaKeyword{open}\AgdaSpace{}%
\AgdaKeyword{import}\AgdaSpace{}%
\AgdaModule{instructionBasic}\<%
\\
\>[0]\AgdaKeyword{open}\AgdaSpace{}%
\AgdaKeyword{import}\AgdaSpace{}%
\AgdaModule{semanticBasicOperations}\AgdaSpace{}%
\AgdaBound{param}\<%
\\
\>[0]\AgdaKeyword{open}\AgdaSpace{}%
\AgdaKeyword{import}\AgdaSpace{}%
\AgdaModule{stackSemanticsInstructions}\AgdaSpace{}%
\AgdaBound{param}\<%
\\
\>[0]\AgdaKeyword{open}\AgdaSpace{}%
\AgdaKeyword{import}\AgdaSpace{}%
\AgdaModule{hoareTripleStack}\AgdaSpace{}%
\AgdaBound{param}\<%
\\
%
\\[\AgdaEmptyExtraSkip]%
\>[0]\AgdaComment{-------------------------------------------------------}\<%
\\
\>[0]\AgdaComment{--\ Verification\ of\ the\ Multisig\ script\ both\ for\ active\ and\ nonactive\ ifStack}\<%
\\
\>[0]\AgdaComment{--\ \ theoremCorrectnessMultiSig-2-3\ \ \ proves\ correctness\ for\ active\ ifStack}\<%
\\
\>[0]\AgdaComment{--\ \ theoremCorrectnessMultiSig-2-3-nonactive\ proves\ correctness\ for\ nonactive\ ifStack}\<%
\\
\>[0]\AgdaComment{-----------------------------------------------------------------}\<%
\\
%
\\[\AgdaEmptyExtraSkip]%
%
\\[\AgdaEmptyExtraSkip]%
%
\\[\AgdaEmptyExtraSkip]%
%
\\[\AgdaEmptyExtraSkip]%
%
\\[\AgdaEmptyExtraSkip]%
%
\\[\AgdaEmptyExtraSkip]%
\>[0]\AgdaFunction{weakestPreCondMultiSig-2-3-bas}\AgdaSpace{}%
\AgdaSymbol{:}%
\>[125I]\AgdaSymbol{(}\AgdaBound{pbk1}\AgdaSpace{}%
\AgdaBound{pbk2}\AgdaSpace{}%
\AgdaBound{pbk3}\AgdaSpace{}%
\AgdaSymbol{:}%
\>[52]\AgdaDatatype{ℕ}\AgdaSymbol{)}\<%
\\
\>[125I][@{}l@{\AgdaIndent{0}}]%
\>[38]\AgdaSymbol{→}\AgdaSpace{}%
\AgdaFunction{StackPredicate}\<%
\\
\>[0]\AgdaFunction{weakestPreCondMultiSig-2-3-bas}\AgdaSpace{}%
\AgdaBound{pbk1}\AgdaSpace{}%
\AgdaBound{pbk2}\AgdaSpace{}%
\AgdaBound{pbk3}\AgdaSpace{}%
\AgdaBound{time}\AgdaSpace{}%
\AgdaBound{msg₁}\AgdaSpace{}%
\AgdaInductiveConstructor{[]}\AgdaSpace{}%
\AgdaSymbol{=}\AgdaSpace{}%
\AgdaDatatype{⊥}\<%
\\
\>[0]\AgdaFunction{weakestPreCondMultiSig-2-3-bas}\AgdaSpace{}%
\AgdaBound{pbk1}\AgdaSpace{}%
\AgdaBound{pbk2}\AgdaSpace{}%
\AgdaBound{pbk3}\AgdaSpace{}%
\AgdaBound{time}\AgdaSpace{}%
\AgdaBound{msg₁}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaBound{x}\AgdaSpace{}%
\AgdaOperator{\AgdaInductiveConstructor{∷}}\AgdaSpace{}%
\AgdaInductiveConstructor{[]}\AgdaSymbol{)}\AgdaSpace{}%
\AgdaSymbol{=}\AgdaSpace{}%
\AgdaDatatype{⊥}\<%
\\
\>[0]\AgdaFunction{weakestPreCondMultiSig-2-3-bas}\AgdaSpace{}%
\AgdaBound{pbk1}\AgdaSpace{}%
\AgdaBound{pbk2}\AgdaSpace{}%
\AgdaBound{pbk3}\AgdaSpace{}%
\AgdaBound{time}\AgdaSpace{}%
\AgdaBound{msg₁}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaBound{x}\AgdaSpace{}%
\AgdaOperator{\AgdaInductiveConstructor{∷}}\AgdaSpace{}%
\AgdaBound{y}\AgdaSpace{}%
\AgdaOperator{\AgdaInductiveConstructor{∷}}\AgdaSpace{}%
\AgdaInductiveConstructor{[]}\AgdaSymbol{)}\AgdaSpace{}%
\AgdaSymbol{=}\AgdaSpace{}%
\AgdaDatatype{⊥}\<%
\\
\>[0]\AgdaFunction{weakestPreCondMultiSig-2-3-bas}\AgdaSpace{}%
\AgdaBound{pbk1}\AgdaSpace{}%
\AgdaBound{pbk2}\AgdaSpace{}%
\AgdaBound{pbk3}\AgdaSpace{}%
\AgdaBound{time}\AgdaSpace{}%
\AgdaBound{msg₁}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaBound{sig2}\AgdaSpace{}%
\AgdaOperator{\AgdaInductiveConstructor{∷}}\AgdaSpace{}%
\AgdaBound{sig1}\AgdaSpace{}%
\AgdaOperator{\AgdaInductiveConstructor{∷}}\AgdaSpace{}%
\AgdaBound{dummy}\AgdaSpace{}%
\AgdaOperator{\AgdaInductiveConstructor{∷}}\AgdaSpace{}%
\AgdaBound{stack₁}\AgdaSymbol{)}\AgdaSpace{}%
\AgdaSymbol{=}\<%
\\
\>[0][@{}l@{\AgdaIndent{0}}]%
\>[9]\AgdaSymbol{(}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaFunction{IsSigned}\AgdaSpace{}%
\AgdaBound{msg₁}\AgdaSpace{}%
\AgdaBound{sig1}\AgdaSpace{}%
\AgdaBound{pbk1}\AgdaSpace{}%
\AgdaOperator{\AgdaRecord{∧}}%
\>[39]\AgdaFunction{IsSigned}\AgdaSpace{}%
\AgdaBound{msg₁}\AgdaSpace{}%
\AgdaBound{sig2}\AgdaSpace{}%
\AgdaBound{pbk2}\AgdaSymbol{)}\AgdaSpace{}%
\AgdaOperator{\AgdaDatatype{⊎}}\<%
\\
\>[9][@{}l@{\AgdaIndent{0}}]%
\>[10]\AgdaSymbol{(}\AgdaFunction{IsSigned}\AgdaSpace{}%
\AgdaBound{msg₁}\AgdaSpace{}%
\AgdaBound{sig1}\AgdaSpace{}%
\AgdaBound{pbk1}\AgdaSpace{}%
\AgdaOperator{\AgdaRecord{∧}}%
\>[38]\AgdaFunction{IsSigned}\AgdaSpace{}%
\AgdaBound{msg₁}\AgdaSpace{}%
\AgdaBound{sig2}\AgdaSpace{}%
\AgdaBound{pbk3}\AgdaSymbol{)}\AgdaSpace{}%
\AgdaOperator{\AgdaDatatype{⊎}}\<%
\\
%
\>[10]\AgdaSymbol{(}\AgdaFunction{IsSigned}\AgdaSpace{}%
\AgdaBound{msg₁}\AgdaSpace{}%
\AgdaBound{sig1}\AgdaSpace{}%
\AgdaBound{pbk2}\AgdaSpace{}%
\AgdaOperator{\AgdaRecord{∧}}%
\>[38]\AgdaFunction{IsSigned}\AgdaSpace{}%
\AgdaBound{msg₁}\AgdaSpace{}%
\AgdaBound{sig2}\AgdaSpace{}%
\AgdaBound{pbk3}\AgdaSpace{}%
\AgdaSymbol{))}\<%
\\
%
\\[\AgdaEmptyExtraSkip]%
%
\\[\AgdaEmptyExtraSkip]%
\>[0]\AgdaFunction{multiSigScript-2-3-b}\AgdaSpace{}%
\AgdaSymbol{:}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaBound{pbk1}\AgdaSpace{}%
\AgdaBound{pbk2}\AgdaSpace{}%
\AgdaBound{pbk3}\AgdaSpace{}%
\AgdaSymbol{:}%
\>[42]\AgdaDatatype{ℕ}\AgdaSymbol{)}\AgdaSpace{}%
\AgdaSymbol{→}\AgdaSpace{}%
\AgdaFunction{BitcoinScriptBasic}\<%
\\
\>[0]\AgdaFunction{multiSigScript-2-3-b}\AgdaSpace{}%
\AgdaBound{pbk1}\AgdaSpace{}%
\AgdaBound{pbk2}\AgdaSpace{}%
\AgdaBound{pbk3}\AgdaSpace{}%
\AgdaSymbol{=}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaInductiveConstructor{opPush}\AgdaSpace{}%
\AgdaNumber{2}\AgdaSymbol{)}\AgdaSpace{}%
\AgdaOperator{\AgdaInductiveConstructor{∷}}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaInductiveConstructor{opPush}\AgdaSpace{}%
\AgdaBound{pbk1}\AgdaSymbol{)}\AgdaSpace{}%
\AgdaOperator{\AgdaInductiveConstructor{∷}}%
\>[68]\AgdaSymbol{(}\AgdaInductiveConstructor{opPush}\AgdaSpace{}%
\AgdaBound{pbk2}\AgdaSymbol{)}\AgdaSpace{}%
\AgdaOperator{\AgdaInductiveConstructor{∷}}%
\>[85]\AgdaSymbol{(}\AgdaInductiveConstructor{opPush}\AgdaSpace{}%
\AgdaBound{pbk3}\AgdaSymbol{)}\AgdaSpace{}%
\AgdaOperator{\AgdaInductiveConstructor{∷}}%
\>[102]\AgdaSymbol{(}\AgdaInductiveConstructor{opPush}\AgdaSpace{}%
\AgdaNumber{3}\AgdaSymbol{)}\AgdaSpace{}%
\AgdaOperator{\AgdaInductiveConstructor{∷}}%
\>[117]\AgdaInductiveConstructor{opMultiSig}\AgdaSpace{}%
\AgdaOperator{\AgdaInductiveConstructor{∷}}\AgdaSpace{}%
\AgdaInductiveConstructor{[]}\<%
\\
%
\\[\AgdaEmptyExtraSkip]%
\>[0]\AgdaFunction{lemmaHoareTripleStackGeAux'1}%
\>[223I]\AgdaSymbol{:}%
\>[224I]\AgdaSymbol{(}\AgdaBound{msg₂}\AgdaSpace{}%
\AgdaSymbol{:}\AgdaSpace{}%
\AgdaDatatype{Msg}\AgdaSymbol{)}\<%
\\
\>[.][@{}l@{}]\<[224I]%
\>[31]\AgdaSymbol{(}\AgdaBound{pbk1}\AgdaSpace{}%
\AgdaBound{pbk2}\AgdaSpace{}%
\AgdaBound{pbk3}\AgdaSpace{}%
\AgdaBound{sig1}\AgdaSpace{}%
\AgdaBound{sig2}\AgdaSpace{}%
\AgdaSymbol{:}\AgdaSpace{}%
\AgdaDatatype{ℕ}\AgdaSymbol{)}\<%
\\
%
\>[31]\AgdaSymbol{→}\AgdaSpace{}%
\AgdaFunction{True}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaFunction{isSigned}%
\>[49]\AgdaBound{msg₂}\AgdaSpace{}%
\AgdaBound{sig1}\AgdaSpace{}%
\AgdaBound{pbk1}\AgdaSymbol{)}\<%
\\
\>[223I][@{}l@{\AgdaIndent{0}}]%
\>[30]\AgdaSymbol{→}%
\>[33]\AgdaFunction{True}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaFunction{isSigned}%
\>[49]\AgdaBound{msg₂}\AgdaSpace{}%
\AgdaBound{sig2}\AgdaSpace{}%
\AgdaBound{pbk2}\AgdaSymbol{)}\<%
\\
\>[30][@{}l@{\AgdaIndent{0}}]%
\>[31]\AgdaSymbol{→}\AgdaSpace{}%
\AgdaFunction{True}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaFunction{compareSigsMultiSig}\AgdaSpace{}%
\AgdaBound{msg₂}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaSpace{}%
\AgdaBound{sig1}\AgdaSpace{}%
\AgdaOperator{\AgdaInductiveConstructor{∷}}\AgdaSpace{}%
\AgdaBound{sig2}\AgdaSpace{}%
\AgdaOperator{\AgdaInductiveConstructor{∷}}\AgdaSpace{}%
\AgdaInductiveConstructor{[]}\AgdaSymbol{)}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaBound{pbk1}\AgdaSpace{}%
\AgdaOperator{\AgdaInductiveConstructor{∷}}\AgdaSpace{}%
\AgdaBound{pbk2}\AgdaSpace{}%
\AgdaOperator{\AgdaInductiveConstructor{∷}}\AgdaSpace{}%
\AgdaBound{pbk3}\AgdaSpace{}%
\AgdaOperator{\AgdaInductiveConstructor{∷}}\AgdaSpace{}%
\AgdaInductiveConstructor{[]}\AgdaSymbol{))}\<%
\\
%
\\[\AgdaEmptyExtraSkip]%
\>[0]\AgdaFunction{lemmaHoareTripleStackGeAux'1}\AgdaSpace{}%
\AgdaBound{msg₂}\AgdaSpace{}%
\AgdaBound{pbk1}\AgdaSpace{}%
\AgdaBound{pbk2}\AgdaSpace{}%
\AgdaBound{pbk3}\AgdaSpace{}%
\AgdaBound{sig1}\AgdaSpace{}%
\AgdaBound{sig2}\AgdaSpace{}%
\AgdaBound{x}\AgdaSpace{}%
\AgdaBound{x₁}\AgdaSpace{}%
\AgdaKeyword{with}%
\>[70]\AgdaSymbol{(}\AgdaFunction{isSigned}%
\>[81]\AgdaBound{msg₂}\AgdaSpace{}%
\AgdaBound{sig1}\AgdaSpace{}%
\AgdaBound{pbk1}\AgdaSymbol{)}\<%
\\
\>[0]\AgdaFunction{lemmaHoareTripleStackGeAux'1}\AgdaSpace{}%
\AgdaBound{msg₂}\AgdaSpace{}%
\AgdaBound{pbk1}\AgdaSpace{}%
\AgdaBound{pbk2}\AgdaSpace{}%
\AgdaBound{pbk3}\AgdaSpace{}%
\AgdaBound{sig1}\AgdaSpace{}%
\AgdaBound{sig2}\AgdaSpace{}%
\AgdaBound{x}\AgdaSpace{}%
\AgdaBound{x₁}\AgdaSpace{}%
\AgdaSymbol{|}\AgdaSpace{}%
\AgdaInductiveConstructor{true}%
\>[72]\AgdaKeyword{with}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaFunction{isSigned}%
\>[88]\AgdaBound{msg₂}\AgdaSpace{}%
\AgdaBound{sig2}\AgdaSpace{}%
\AgdaBound{pbk2}\AgdaSymbol{)}\<%
\\
\>[0]\AgdaFunction{lemmaHoareTripleStackGeAux'1}\AgdaSpace{}%
\AgdaBound{msg₂}\AgdaSpace{}%
\AgdaBound{pbk1}\AgdaSpace{}%
\AgdaBound{pbk2}\AgdaSpace{}%
\AgdaBound{pbk3}\AgdaSpace{}%
\AgdaBound{sig1}\AgdaSpace{}%
\AgdaBound{sig2}\AgdaSpace{}%
\AgdaBound{x}\AgdaSpace{}%
\AgdaBound{x₁}\AgdaSpace{}%
\AgdaSymbol{|}\AgdaSpace{}%
\AgdaInductiveConstructor{true}\AgdaSpace{}%
\AgdaSymbol{|}\AgdaSpace{}%
\AgdaInductiveConstructor{true}\AgdaSpace{}%
\AgdaSymbol{=}\AgdaSpace{}%
\AgdaInductiveConstructor{tt}\<%
\\
%
\\[\AgdaEmptyExtraSkip]%
%
\\[\AgdaEmptyExtraSkip]%
%
\\[\AgdaEmptyExtraSkip]%
%
\\[\AgdaEmptyExtraSkip]%
\>[0]\AgdaFunction{lemmaHoareTripleStackGeAux'2}%
\>[294I]\AgdaSymbol{:}%
\>[295I]\AgdaSymbol{(}\AgdaBound{msg₂}\AgdaSpace{}%
\AgdaSymbol{:}\AgdaSpace{}%
\AgdaDatatype{Msg}\AgdaSymbol{)}\<%
\\
\>[.][@{}l@{}]\<[295I]%
\>[31]\AgdaSymbol{(}\AgdaBound{pbk1}\AgdaSpace{}%
\AgdaBound{pbk2}\AgdaSpace{}%
\AgdaBound{pbk3}\AgdaSpace{}%
\AgdaBound{sig1}\AgdaSpace{}%
\AgdaBound{sig2}\AgdaSpace{}%
\AgdaSymbol{:}\AgdaSpace{}%
\AgdaDatatype{ℕ}\AgdaSymbol{)}\<%
\\
%
\>[31]\AgdaSymbol{→}\AgdaSpace{}%
\AgdaFunction{True}%
\>[39]\AgdaSymbol{(}\AgdaFunction{isSigned}%
\>[50]\AgdaBound{msg₂}\AgdaSpace{}%
\AgdaBound{sig1}\AgdaSpace{}%
\AgdaBound{pbk1}\AgdaSymbol{)}\<%
\\
\>[294I][@{}l@{\AgdaIndent{0}}]%
\>[30]\AgdaSymbol{→}%
\>[33]\AgdaFunction{True}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaFunction{isSigned}%
\>[49]\AgdaBound{msg₂}\AgdaSpace{}%
\AgdaBound{sig2}\AgdaSpace{}%
\AgdaBound{pbk3}\AgdaSymbol{)}\<%
\\
\>[30][@{}l@{\AgdaIndent{0}}]%
\>[31]\AgdaSymbol{→}\AgdaSpace{}%
\AgdaFunction{True}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaFunction{compareSigsMultiSig}\AgdaSpace{}%
\AgdaBound{msg₂}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaSpace{}%
\AgdaBound{sig1}\AgdaSpace{}%
\AgdaOperator{\AgdaInductiveConstructor{∷}}\AgdaSpace{}%
\AgdaBound{sig2}\AgdaSpace{}%
\AgdaOperator{\AgdaInductiveConstructor{∷}}\AgdaSpace{}%
\AgdaInductiveConstructor{[]}\AgdaSymbol{)}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaBound{pbk1}\AgdaSpace{}%
\AgdaOperator{\AgdaInductiveConstructor{∷}}\AgdaSpace{}%
\AgdaBound{pbk2}\AgdaSpace{}%
\AgdaOperator{\AgdaInductiveConstructor{∷}}\AgdaSpace{}%
\AgdaBound{pbk3}\AgdaSpace{}%
\AgdaOperator{\AgdaInductiveConstructor{∷}}\AgdaSpace{}%
\AgdaInductiveConstructor{[]}\AgdaSymbol{))}\<%
\\
\>[0]\AgdaFunction{lemmaHoareTripleStackGeAux'2}\AgdaSpace{}%
\AgdaBound{msg₂}\AgdaSpace{}%
\AgdaBound{pbk1}\AgdaSpace{}%
\AgdaBound{pbk2}\AgdaSpace{}%
\AgdaBound{pbk3}\AgdaSpace{}%
\AgdaBound{sig1}\AgdaSpace{}%
\AgdaBound{sig2}\AgdaSpace{}%
\AgdaBound{x}\AgdaSpace{}%
\AgdaBound{x₁}\AgdaSpace{}%
\AgdaKeyword{with}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaFunction{isSigned}%
\>[80]\AgdaBound{msg₂}\AgdaSpace{}%
\AgdaBound{sig1}\AgdaSpace{}%
\AgdaBound{pbk1}\AgdaSymbol{)}\<%
\\
\>[0]\AgdaFunction{lemmaHoareTripleStackGeAux'2}\AgdaSpace{}%
\AgdaBound{msg₂}\AgdaSpace{}%
\AgdaBound{pbk1}\AgdaSpace{}%
\AgdaBound{pbk2}\AgdaSpace{}%
\AgdaBound{pbk3}\AgdaSpace{}%
\AgdaBound{sig1}\AgdaSpace{}%
\AgdaBound{sig2}\AgdaSpace{}%
\AgdaBound{x}\AgdaSpace{}%
\AgdaBound{x₁}\AgdaSpace{}%
\AgdaSymbol{|}\AgdaSpace{}%
\AgdaInductiveConstructor{true}\AgdaSpace{}%
\AgdaKeyword{with}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaFunction{isSigned}%
\>[87]\AgdaBound{msg₂}\AgdaSpace{}%
\AgdaBound{sig2}\AgdaSpace{}%
\AgdaBound{pbk2}\AgdaSymbol{)}\<%
\\
\>[0]\AgdaFunction{lemmaHoareTripleStackGeAux'2}\AgdaSpace{}%
\AgdaBound{msg₂}\AgdaSpace{}%
\AgdaBound{pbk1}\AgdaSpace{}%
\AgdaBound{pbk2}\AgdaSpace{}%
\AgdaBound{pbk3}\AgdaSpace{}%
\AgdaBound{sig1}\AgdaSpace{}%
\AgdaBound{sig2}\AgdaSpace{}%
\AgdaBound{x}\AgdaSpace{}%
\AgdaBound{x₁}\AgdaSpace{}%
\AgdaSymbol{|}\AgdaSpace{}%
\AgdaInductiveConstructor{true}\AgdaSpace{}%
\AgdaSymbol{|}\AgdaSpace{}%
\AgdaInductiveConstructor{false}\AgdaSpace{}%
\AgdaKeyword{with}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaFunction{isSigned}%
\>[95]\AgdaBound{msg₂}\AgdaSpace{}%
\AgdaBound{sig2}\AgdaSpace{}%
\AgdaBound{pbk3}\AgdaSymbol{)}\<%
\\
\>[0]\AgdaFunction{lemmaHoareTripleStackGeAux'2}\AgdaSpace{}%
\AgdaBound{msg₂}\AgdaSpace{}%
\AgdaBound{pbk1}\AgdaSpace{}%
\AgdaBound{pbk2}\AgdaSpace{}%
\AgdaBound{pbk3}\AgdaSpace{}%
\AgdaBound{sig1}\AgdaSpace{}%
\AgdaBound{sig2}\AgdaSpace{}%
\AgdaBound{x}\AgdaSpace{}%
\AgdaBound{x₁}\AgdaSpace{}%
\AgdaSymbol{|}\AgdaSpace{}%
\AgdaInductiveConstructor{true}\AgdaSpace{}%
\AgdaSymbol{|}\AgdaSpace{}%
\AgdaInductiveConstructor{false}\AgdaSpace{}%
\AgdaSymbol{|}\AgdaSpace{}%
\AgdaInductiveConstructor{true}\AgdaSpace{}%
\AgdaSymbol{=}\AgdaSpace{}%
\AgdaInductiveConstructor{tt}\<%
\\
\>[0]\AgdaFunction{lemmaHoareTripleStackGeAux'2}\AgdaSpace{}%
\AgdaBound{msg₂}\AgdaSpace{}%
\AgdaBound{pbk1}\AgdaSpace{}%
\AgdaBound{pbk2}\AgdaSpace{}%
\AgdaBound{pbk3}\AgdaSpace{}%
\AgdaBound{sig1}\AgdaSpace{}%
\AgdaBound{sig2}\AgdaSpace{}%
\AgdaBound{x}\AgdaSpace{}%
\AgdaBound{x₁}\AgdaSpace{}%
\AgdaSymbol{|}\AgdaSpace{}%
\AgdaInductiveConstructor{true}\AgdaSpace{}%
\AgdaSymbol{|}\AgdaSpace{}%
\AgdaInductiveConstructor{true}\AgdaSpace{}%
\AgdaSymbol{=}\AgdaSpace{}%
\AgdaInductiveConstructor{tt}\<%
\\
%
\\[\AgdaEmptyExtraSkip]%
%
\\[\AgdaEmptyExtraSkip]%
%
\\[\AgdaEmptyExtraSkip]%
\>[0]\AgdaFunction{lemmaHoareTripleStackGeAux'3}%
\>[398I]\AgdaSymbol{:}%
\>[399I]\AgdaSymbol{(}\AgdaBound{msg₂}\AgdaSpace{}%
\AgdaSymbol{:}\AgdaSpace{}%
\AgdaDatatype{Msg}\AgdaSymbol{)}\<%
\\
\>[.][@{}l@{}]\<[399I]%
\>[31]\AgdaSymbol{(}\AgdaBound{pbk1}\AgdaSpace{}%
\AgdaBound{pbk2}\AgdaSpace{}%
\AgdaBound{pbk3}\AgdaSpace{}%
\AgdaBound{sig1}\AgdaSpace{}%
\AgdaBound{sig2}\AgdaSpace{}%
\AgdaSymbol{:}\AgdaSpace{}%
\AgdaDatatype{ℕ}\AgdaSymbol{)}\<%
\\
%
\>[31]\AgdaSymbol{→}\AgdaSpace{}%
\AgdaFunction{True}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaFunction{isSigned}%
\>[49]\AgdaBound{msg₂}\AgdaSpace{}%
\AgdaBound{sig1}\AgdaSpace{}%
\AgdaBound{pbk2}\AgdaSymbol{)}\<%
\\
\>[398I][@{}l@{\AgdaIndent{0}}]%
\>[30]\AgdaSymbol{→}%
\>[33]\AgdaFunction{True}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaFunction{isSigned}%
\>[49]\AgdaBound{msg₂}\AgdaSpace{}%
\AgdaBound{sig2}\AgdaSpace{}%
\AgdaBound{pbk3}\AgdaSymbol{)}\<%
\\
\>[30][@{}l@{\AgdaIndent{0}}]%
\>[31]\AgdaSymbol{→}\AgdaSpace{}%
\AgdaFunction{True}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaFunction{compareSigsMultiSig}\AgdaSpace{}%
\AgdaBound{msg₂}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaSpace{}%
\AgdaBound{sig1}\AgdaSpace{}%
\AgdaOperator{\AgdaInductiveConstructor{∷}}\AgdaSpace{}%
\AgdaBound{sig2}\AgdaSpace{}%
\AgdaOperator{\AgdaInductiveConstructor{∷}}\AgdaSpace{}%
\AgdaInductiveConstructor{[]}\AgdaSymbol{)}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaBound{pbk1}\AgdaSpace{}%
\AgdaOperator{\AgdaInductiveConstructor{∷}}\AgdaSpace{}%
\AgdaBound{pbk2}\AgdaSpace{}%
\AgdaOperator{\AgdaInductiveConstructor{∷}}\AgdaSpace{}%
\AgdaBound{pbk3}\AgdaSpace{}%
\AgdaOperator{\AgdaInductiveConstructor{∷}}\AgdaSpace{}%
\AgdaInductiveConstructor{[]}\AgdaSymbol{))}\<%
\\
\>[0]\AgdaFunction{lemmaHoareTripleStackGeAux'3}\AgdaSpace{}%
\AgdaBound{msg₂}\AgdaSpace{}%
\AgdaBound{pbk1}\AgdaSpace{}%
\AgdaBound{pbk2}\AgdaSpace{}%
\AgdaBound{pbk3}\AgdaSpace{}%
\AgdaBound{sig1}\AgdaSpace{}%
\AgdaBound{sig2}\AgdaSpace{}%
\AgdaBound{x}\AgdaSpace{}%
\AgdaBound{x₁}%
\>[65]\AgdaKeyword{with}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaFunction{isSigned}%
\>[81]\AgdaBound{msg₂}\AgdaSpace{}%
\AgdaBound{sig1}\AgdaSpace{}%
\AgdaBound{pbk1}\AgdaSpace{}%
\AgdaSymbol{)}\<%
\\
\>[0]\AgdaFunction{lemmaHoareTripleStackGeAux'3}\AgdaSpace{}%
\AgdaBound{msg₂}\AgdaSpace{}%
\AgdaBound{pbk1}\AgdaSpace{}%
\AgdaBound{pbk2}\AgdaSpace{}%
\AgdaBound{pbk3}\AgdaSpace{}%
\AgdaBound{sig1}\AgdaSpace{}%
\AgdaBound{sig2}\AgdaSpace{}%
\AgdaBound{x}\AgdaSpace{}%
\AgdaBound{x₁}\AgdaSpace{}%
\AgdaSymbol{|}\AgdaSpace{}%
\AgdaInductiveConstructor{false}\AgdaSpace{}%
\AgdaKeyword{with}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaFunction{isSigned}%
\>[88]\AgdaBound{msg₂}\AgdaSpace{}%
\AgdaBound{sig1}\AgdaSpace{}%
\AgdaBound{pbk2}\AgdaSymbol{)}\<%
\\
\>[0]\AgdaFunction{lemmaHoareTripleStackGeAux'3}\AgdaSpace{}%
\AgdaBound{msg₂}\AgdaSpace{}%
\AgdaBound{pbk1}\AgdaSpace{}%
\AgdaBound{pbk2}\AgdaSpace{}%
\AgdaBound{pbk3}\AgdaSpace{}%
\AgdaBound{sig1}\AgdaSpace{}%
\AgdaBound{sig2}\AgdaSpace{}%
\AgdaBound{x}\AgdaSpace{}%
\AgdaBound{x₁}\AgdaSpace{}%
\AgdaSymbol{|}\AgdaSpace{}%
\AgdaInductiveConstructor{false}\AgdaSpace{}%
\AgdaSymbol{|}\AgdaSpace{}%
\AgdaInductiveConstructor{true}\AgdaSpace{}%
\AgdaKeyword{with}\AgdaSpace{}%
\AgdaFunction{isSigned}%
\>[94]\AgdaBound{msg₂}\AgdaSpace{}%
\AgdaBound{sig2}\AgdaSpace{}%
\AgdaBound{pbk3}\<%
\\
\>[0]\AgdaFunction{lemmaHoareTripleStackGeAux'3}\AgdaSpace{}%
\AgdaBound{msg₂}\AgdaSpace{}%
\AgdaBound{pbk1}\AgdaSpace{}%
\AgdaBound{pbk2}\AgdaSpace{}%
\AgdaBound{pbk3}\AgdaSpace{}%
\AgdaBound{sig1}\AgdaSpace{}%
\AgdaBound{sig2}\AgdaSpace{}%
\AgdaBound{x}\AgdaSpace{}%
\AgdaBound{x₁}\AgdaSpace{}%
\AgdaSymbol{|}\AgdaSpace{}%
\AgdaInductiveConstructor{false}\AgdaSpace{}%
\AgdaSymbol{|}\AgdaSpace{}%
\AgdaInductiveConstructor{true}\AgdaSpace{}%
\AgdaSymbol{|}\AgdaSpace{}%
\AgdaInductiveConstructor{true}\AgdaSpace{}%
\AgdaSymbol{=}\AgdaSpace{}%
\AgdaInductiveConstructor{tt}\<%
\\
\>[0]\AgdaFunction{lemmaHoareTripleStackGeAux'3}\AgdaSpace{}%
\AgdaBound{msg₂}\AgdaSpace{}%
\AgdaBound{pbk1}\AgdaSpace{}%
\AgdaBound{pbk2}\AgdaSpace{}%
\AgdaBound{pbk3}\AgdaSpace{}%
\AgdaBound{sig1}\AgdaSpace{}%
\AgdaBound{sig2}\AgdaSpace{}%
\AgdaBound{x}\AgdaSpace{}%
\AgdaBound{x₁}\AgdaSpace{}%
\AgdaSymbol{|}\AgdaSpace{}%
\AgdaInductiveConstructor{true}\AgdaSpace{}%
\AgdaKeyword{with}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaFunction{isSigned}%
\>[87]\AgdaBound{msg₂}\AgdaSpace{}%
\AgdaBound{sig2}\AgdaSpace{}%
\AgdaBound{pbk2}\AgdaSymbol{)}\<%
\\
\>[0]\AgdaFunction{lemmaHoareTripleStackGeAux'3}\AgdaSpace{}%
\AgdaBound{msg₂}\AgdaSpace{}%
\AgdaBound{pbk1}\AgdaSpace{}%
\AgdaBound{pbk2}\AgdaSpace{}%
\AgdaBound{pbk3}\AgdaSpace{}%
\AgdaBound{sig1}\AgdaSpace{}%
\AgdaBound{sig2}\AgdaSpace{}%
\AgdaBound{x}\AgdaSpace{}%
\AgdaBound{x₁}\AgdaSpace{}%
\AgdaSymbol{|}\AgdaSpace{}%
\AgdaInductiveConstructor{true}\AgdaSpace{}%
\AgdaSymbol{|}\AgdaSpace{}%
\AgdaInductiveConstructor{false}\AgdaSpace{}%
\AgdaKeyword{with}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaFunction{isSigned}%
\>[95]\AgdaBound{msg₂}\AgdaSpace{}%
\AgdaBound{sig2}\AgdaSpace{}%
\AgdaBound{pbk3}\AgdaSymbol{)}\<%
\\
\>[0]\AgdaFunction{lemmaHoareTripleStackGeAux'3}\AgdaSpace{}%
\AgdaBound{msg₂}\AgdaSpace{}%
\AgdaBound{pbk1}\AgdaSpace{}%
\AgdaBound{pbk2}\AgdaSpace{}%
\AgdaBound{pbk3}\AgdaSpace{}%
\AgdaBound{sig1}\AgdaSpace{}%
\AgdaBound{sig2}\AgdaSpace{}%
\AgdaBound{x}\AgdaSpace{}%
\AgdaBound{x₁}\AgdaSpace{}%
\AgdaSymbol{|}\AgdaSpace{}%
\AgdaInductiveConstructor{true}\AgdaSpace{}%
\AgdaSymbol{|}\AgdaSpace{}%
\AgdaInductiveConstructor{false}\AgdaSpace{}%
\AgdaSymbol{|}\AgdaSpace{}%
\AgdaInductiveConstructor{true}\AgdaSpace{}%
\AgdaSymbol{=}\AgdaSpace{}%
\AgdaInductiveConstructor{tt}\<%
\\
\>[0]\AgdaFunction{lemmaHoareTripleStackGeAux'3}\AgdaSpace{}%
\AgdaBound{msg₂}\AgdaSpace{}%
\AgdaBound{pbk1}\AgdaSpace{}%
\AgdaBound{pbk2}\AgdaSpace{}%
\AgdaBound{pbk3}\AgdaSpace{}%
\AgdaBound{sig1}\AgdaSpace{}%
\AgdaBound{sig2}\AgdaSpace{}%
\AgdaBound{x}\AgdaSpace{}%
\AgdaBound{x₁}\AgdaSpace{}%
\AgdaSymbol{|}\AgdaSpace{}%
\AgdaInductiveConstructor{true}\AgdaSpace{}%
\AgdaSymbol{|}\AgdaSpace{}%
\AgdaInductiveConstructor{true}\AgdaSpace{}%
\AgdaSymbol{=}\AgdaSpace{}%
\AgdaInductiveConstructor{tt}\<%
\\
%
\\[\AgdaEmptyExtraSkip]%
\>[0]\AgdaComment{\{-}\<%
\\
\>[0]\AgdaComment{For\ the\ other\ direction\ we\ get\ the\ goal}\<%
\\
\>[0]\<%
\\
\>[0]\<%
\\
\>[0]\AgdaComment{Goal:\ (True\ (isSigned\ \ msg₂\ sig1\ pbk1\ )\ ∧}\<%
\\
\>[0]\AgdaComment{\ \ \ \ \ \ \ True\ (isSigned\ \ msg₂\ sig2\ pbk2))}\<%
\\
\>[0]\AgdaComment{\ \ \ \ \ \ ⊎}\<%
\\
\>[0]\AgdaComment{\ \ \ \ \ \ (True\ (isSigned\ \ msg₂\ sig1\ pbk1\ )\ ∧}\<%
\\
\>[0]\AgdaComment{\ \ \ \ \ \ \ True\ (isSigned\ \ msg₂\ sig2\ pbk3))}\<%
\\
\>[0]\AgdaComment{\ \ \ \ \ \ ⊎}\<%
\\
\>[0]\AgdaComment{\ \ \ \ \ \ (True\ (isSigned\ \ msg₂\ sig1\ pbk2)\ ∧}\<%
\\
\>[0]\AgdaComment{\ \ \ \ \ \ \ True\ (isSigned\ \ msg₂\ sig2\ pbk3))}\<%
\\
\>[0]\AgdaComment{————————————————————————————————————————————————————————————}\<%
\\
\>[0]\AgdaComment{x\ \ \ \ \ :\ True}\<%
\\
\>[0]\AgdaComment{\ \ \ \ \ \ \ \ (notFalse}\<%
\\
\>[0]\AgdaComment{\ \ \ \ \ \ \ \ \ (boolToNat}\<%
\\
\>[0]\AgdaComment{\ \ \ \ \ \ \ \ \ \ (compareSigsMultiSigAux\ msg₂\ (sig2\ ∷\ [])\ (pbk2\ ∷\ pbk3\ ∷\ [])\ sig1}\<%
\\
\>[0]\AgdaComment{\ \ \ \ \ \ \ \ \ \ \ (isSigned\ \ msg₂\ sig1\ pbk1\ ))))}\<%
\\
\>[0]\<%
\\
\>[0]\<%
\\
\>[0]\<%
\\
\>[0]\AgdaComment{Again\ we\ use\ the\ boolToNatNotFalseLemma2\ lemma\ to\ get\ rid\ of\ the}\<%
\\
\>[0]\AgdaComment{True(notFalse\ (boolToNat}\<%
\\
\>[0]\<%
\\
\>[0]\AgdaComment{and\ show}\<%
\\
\>[0]\AgdaComment{lemmaHoareTripleStackGeAux'4}\<%
\\
\>[0]\<%
\\
\>[0]\AgdaComment{we\ see\ that\ now\ the\ x\ ends\ with}\<%
\\
\>[0]\AgdaComment{(isSigned\ \ msg₂\ sig1\ pbk1\ )}\<%
\\
\>[0]\AgdaComment{so\ we\ start\ with\ the\ with\ pattern\ with\ a\ case\ distinction\ on\ this}\<%
\\
\>[0]\AgdaComment{and\ continue\ making\ casedistintion\ on\ the\ last\ formula\ in\ x}\<%
\\
\>[0]\<%
\\
\>[0]\<%
\\
\>[0]\<%
\\
\>[0]\AgdaComment{-\}}\<%
\\
%
\\[\AgdaEmptyExtraSkip]%
\>[0]\AgdaFunction{lemmaHoareTripleStackGeAux'4}\AgdaSpace{}%
\AgdaSymbol{:}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaBound{msg₂}\AgdaSpace{}%
\AgdaSymbol{:}\AgdaSpace{}%
\AgdaDatatype{Msg}\AgdaSymbol{)}\<%
\\
\>[0][@{}l@{\AgdaIndent{0}}]%
\>[9]\AgdaSymbol{(}\AgdaBound{pbk1}\AgdaSpace{}%
\AgdaBound{pbk2}\AgdaSpace{}%
\AgdaBound{pbk3}\AgdaSpace{}%
\AgdaBound{sig1}\AgdaSpace{}%
\AgdaBound{sig2}\AgdaSpace{}%
\AgdaSymbol{:}\AgdaSpace{}%
\AgdaDatatype{ℕ}\AgdaSymbol{)}\<%
\\
\>[9][@{}l@{\AgdaIndent{0}}]%
\>[10]\AgdaSymbol{→}\AgdaSpace{}%
\AgdaFunction{True}%
\>[560I]\AgdaSymbol{(}\AgdaFunction{compareSigsMultiSigAux}\AgdaSpace{}%
\AgdaBound{msg₂}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaBound{sig2}\AgdaSpace{}%
\AgdaOperator{\AgdaInductiveConstructor{∷}}\AgdaSpace{}%
\AgdaInductiveConstructor{[]}\AgdaSymbol{)}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaBound{pbk2}\AgdaSpace{}%
\AgdaOperator{\AgdaInductiveConstructor{∷}}\AgdaSpace{}%
\AgdaBound{pbk3}\AgdaSpace{}%
\AgdaOperator{\AgdaInductiveConstructor{∷}}\AgdaSpace{}%
\AgdaInductiveConstructor{[]}\AgdaSymbol{)}%
\>[78]\AgdaBound{sig1}\<%
\\
\>[.][@{}l@{}]\<[560I]%
\>[17]\AgdaSymbol{(}\AgdaFunction{isSigned}%
\>[28]\AgdaBound{msg₂}\AgdaSpace{}%
\AgdaBound{sig1}\AgdaSpace{}%
\AgdaBound{pbk1}\AgdaSpace{}%
\AgdaSymbol{))}\<%
\\
%
\>[10]\AgdaSymbol{→}%
\>[16]\AgdaSymbol{(}\AgdaFunction{True}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaFunction{isSigned}%
\>[33]\AgdaBound{msg₂}\AgdaSpace{}%
\AgdaBound{sig1}\AgdaSpace{}%
\AgdaBound{pbk1}\AgdaSpace{}%
\AgdaSymbol{)}\AgdaSpace{}%
\AgdaOperator{\AgdaRecord{∧}}\AgdaSpace{}%
\AgdaFunction{True}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaFunction{isSigned}%
\>[68]\AgdaBound{msg₂}\AgdaSpace{}%
\AgdaBound{sig2}\AgdaSpace{}%
\AgdaBound{pbk2}\AgdaSymbol{))}\<%
\\
\>[10][@{}l@{\AgdaIndent{0}}]%
\>[13]\AgdaOperator{\AgdaDatatype{⊎}}%
\>[16]\AgdaSymbol{(}\AgdaFunction{True}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaFunction{isSigned}%
\>[33]\AgdaBound{msg₂}\AgdaSpace{}%
\AgdaBound{sig1}\AgdaSpace{}%
\AgdaBound{pbk1}\AgdaSpace{}%
\AgdaSymbol{)}\AgdaSpace{}%
\AgdaOperator{\AgdaRecord{∧}}%
\>[53]\AgdaFunction{True}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaFunction{isSigned}%
\>[69]\AgdaBound{msg₂}\AgdaSpace{}%
\AgdaBound{sig2}\AgdaSpace{}%
\AgdaBound{pbk3}\AgdaSymbol{))}\<%
\\
%
\>[13]\AgdaOperator{\AgdaDatatype{⊎}}%
\>[16]\AgdaSymbol{(}\AgdaFunction{True}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaFunction{isSigned}%
\>[33]\AgdaBound{msg₂}\AgdaSpace{}%
\AgdaBound{sig1}\AgdaSpace{}%
\AgdaBound{pbk2}\AgdaSymbol{)}\AgdaSpace{}%
\AgdaOperator{\AgdaRecord{∧}}\AgdaSpace{}%
\AgdaFunction{True}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaFunction{isSigned}%
\>[67]\AgdaBound{msg₂}\AgdaSpace{}%
\AgdaBound{sig2}\AgdaSpace{}%
\AgdaBound{pbk3}\AgdaSymbol{))}\<%
\\
\>[0]\AgdaFunction{lemmaHoareTripleStackGeAux'4}\AgdaSpace{}%
\AgdaBound{msg₂}\AgdaSpace{}%
\AgdaBound{pbk1}\AgdaSpace{}%
\AgdaBound{pbk2}\AgdaSpace{}%
\AgdaBound{pbk3}\AgdaSpace{}%
\AgdaBound{sig1}\AgdaSpace{}%
\AgdaBound{sig2}\AgdaSpace{}%
\AgdaSymbol{\AgdaUnderscore{}}\AgdaSpace{}%
\AgdaKeyword{with}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaFunction{isSigned}%
\>[77]\AgdaBound{msg₂}\AgdaSpace{}%
\AgdaBound{sig1}\AgdaSpace{}%
\AgdaBound{pbk1}\AgdaSpace{}%
\AgdaSymbol{)}\<%
\\
\>[0]\AgdaFunction{lemmaHoareTripleStackGeAux'4}\AgdaSpace{}%
\AgdaBound{msg₂}\AgdaSpace{}%
\AgdaBound{pbk1}\AgdaSpace{}%
\AgdaBound{pbk2}\AgdaSpace{}%
\AgdaBound{pbk3}\AgdaSpace{}%
\AgdaBound{sig1}\AgdaSpace{}%
\AgdaBound{sig2}\AgdaSpace{}%
\AgdaSymbol{\AgdaUnderscore{}}\AgdaSpace{}%
\AgdaSymbol{|}\AgdaSpace{}%
\AgdaInductiveConstructor{false}\AgdaSpace{}%
\AgdaKeyword{with}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaFunction{isSigned}%
\>[85]\AgdaBound{msg₂}\AgdaSpace{}%
\AgdaBound{sig1}\AgdaSpace{}%
\AgdaBound{pbk2}\AgdaSymbol{)}\<%
\\
\>[0]\AgdaFunction{lemmaHoareTripleStackGeAux'4}\AgdaSpace{}%
\AgdaBound{msg₂}\AgdaSpace{}%
\AgdaBound{pbk1}\AgdaSpace{}%
\AgdaBound{pbk2}\AgdaSpace{}%
\AgdaBound{pbk3}\AgdaSpace{}%
\AgdaBound{sig1}\AgdaSpace{}%
\AgdaBound{sig2}\AgdaSpace{}%
\AgdaSymbol{\AgdaUnderscore{}}\AgdaSpace{}%
\AgdaSymbol{|}\AgdaSpace{}%
\AgdaInductiveConstructor{false}\AgdaSpace{}%
\AgdaSymbol{|}\AgdaSpace{}%
\AgdaInductiveConstructor{false}\AgdaSpace{}%
\AgdaKeyword{with}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaFunction{isSigned}%
\>[93]\AgdaBound{msg₂}\AgdaSpace{}%
\AgdaBound{sig1}\AgdaSpace{}%
\AgdaBound{pbk3}\AgdaSymbol{)}\<%
\\
\>[0]\AgdaFunction{lemmaHoareTripleStackGeAux'4}\AgdaSpace{}%
\AgdaBound{msg₂}\AgdaSpace{}%
\AgdaBound{pbk1}\AgdaSpace{}%
\AgdaBound{pbk2}\AgdaSpace{}%
\AgdaBound{pbk3}\AgdaSpace{}%
\AgdaBound{sig1}\AgdaSpace{}%
\AgdaBound{sig2}\AgdaSpace{}%
\AgdaSymbol{()}\AgdaSpace{}%
\AgdaSymbol{|}\AgdaSpace{}%
\AgdaInductiveConstructor{false}\AgdaSpace{}%
\AgdaSymbol{|}\AgdaSpace{}%
\AgdaInductiveConstructor{false}\AgdaSpace{}%
\AgdaSymbol{|}\AgdaSpace{}%
\AgdaInductiveConstructor{false}\<%
\\
\>[0]\AgdaFunction{lemmaHoareTripleStackGeAux'4}\AgdaSpace{}%
\AgdaBound{msg₂}\AgdaSpace{}%
\AgdaBound{pbk1}\AgdaSpace{}%
\AgdaBound{pbk2}\AgdaSpace{}%
\AgdaBound{pbk3}\AgdaSpace{}%
\AgdaBound{sig1}\AgdaSpace{}%
\AgdaBound{sig2}\AgdaSpace{}%
\AgdaSymbol{()}\AgdaSpace{}%
\AgdaSymbol{|}\AgdaSpace{}%
\AgdaInductiveConstructor{false}\AgdaSpace{}%
\AgdaSymbol{|}\AgdaSpace{}%
\AgdaInductiveConstructor{false}\AgdaSpace{}%
\AgdaSymbol{|}\AgdaSpace{}%
\AgdaInductiveConstructor{true}\<%
\\
\>[0]\AgdaFunction{lemmaHoareTripleStackGeAux'4}\AgdaSpace{}%
\AgdaBound{msg₂}\AgdaSpace{}%
\AgdaBound{pbk1}\AgdaSpace{}%
\AgdaBound{pbk2}\AgdaSpace{}%
\AgdaBound{pbk3}\AgdaSpace{}%
\AgdaBound{sig1}\AgdaSpace{}%
\AgdaBound{sig2}\AgdaSpace{}%
\AgdaSymbol{\AgdaUnderscore{}}\AgdaSpace{}%
\AgdaSymbol{|}\AgdaSpace{}%
\AgdaInductiveConstructor{false}\AgdaSpace{}%
\AgdaSymbol{|}\AgdaSpace{}%
\AgdaInductiveConstructor{true}\AgdaSpace{}%
\AgdaKeyword{with}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaFunction{isSigned}%
\>[92]\AgdaBound{msg₂}\AgdaSpace{}%
\AgdaBound{sig2}\AgdaSpace{}%
\AgdaBound{pbk3}\AgdaSymbol{)}\<%
\\
\>[0]\AgdaFunction{lemmaHoareTripleStackGeAux'4}\AgdaSpace{}%
\AgdaBound{msg₂}\AgdaSpace{}%
\AgdaBound{pbk1}\AgdaSpace{}%
\AgdaBound{pbk2}\AgdaSpace{}%
\AgdaBound{pbk3}\AgdaSpace{}%
\AgdaBound{sig1}\AgdaSpace{}%
\AgdaBound{sig2}\AgdaSpace{}%
\AgdaSymbol{\AgdaUnderscore{}}\AgdaSpace{}%
\AgdaSymbol{|}\AgdaSpace{}%
\AgdaInductiveConstructor{false}\AgdaSpace{}%
\AgdaSymbol{|}\AgdaSpace{}%
\AgdaInductiveConstructor{true}\AgdaSpace{}%
\AgdaSymbol{|}\AgdaSpace{}%
\AgdaInductiveConstructor{true}\AgdaSpace{}%
\AgdaSymbol{=}\AgdaSpace{}%
\AgdaInductiveConstructor{inj₂}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaInductiveConstructor{inj₂}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaInductiveConstructor{conj}\AgdaSpace{}%
\AgdaInductiveConstructor{tt}\AgdaSpace{}%
\AgdaInductiveConstructor{tt}\AgdaSymbol{))}\<%
\\
\>[0]\AgdaFunction{lemmaHoareTripleStackGeAux'4}\AgdaSpace{}%
\AgdaBound{msg₂}\AgdaSpace{}%
\AgdaBound{pbk1}\AgdaSpace{}%
\AgdaBound{pbk2}\AgdaSpace{}%
\AgdaBound{pbk3}\AgdaSpace{}%
\AgdaBound{sig1}\AgdaSpace{}%
\AgdaBound{sig2}\AgdaSpace{}%
\AgdaSymbol{\AgdaUnderscore{}}\AgdaSpace{}%
\AgdaSymbol{|}\AgdaSpace{}%
\AgdaInductiveConstructor{true}%
\>[69]\AgdaKeyword{with}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaFunction{isSigned}%
\>[85]\AgdaBound{msg₂}\AgdaSpace{}%
\AgdaBound{sig2}\AgdaSpace{}%
\AgdaBound{pbk2}\AgdaSymbol{)}\<%
\\
\>[0]\AgdaFunction{lemmaHoareTripleStackGeAux'4}\AgdaSpace{}%
\AgdaBound{msg₂}\AgdaSpace{}%
\AgdaBound{pbk1}\AgdaSpace{}%
\AgdaBound{pbk2}\AgdaSpace{}%
\AgdaBound{pbk3}\AgdaSpace{}%
\AgdaBound{sig1}\AgdaSpace{}%
\AgdaBound{sig2}\AgdaSpace{}%
\AgdaSymbol{\AgdaUnderscore{}}\AgdaSpace{}%
\AgdaSymbol{|}\AgdaSpace{}%
\AgdaInductiveConstructor{true}\AgdaSpace{}%
\AgdaSymbol{|}\AgdaSpace{}%
\AgdaInductiveConstructor{false}\AgdaSpace{}%
\AgdaKeyword{with}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaFunction{isSigned}%
\>[92]\AgdaBound{msg₂}\AgdaSpace{}%
\AgdaBound{sig2}\AgdaSpace{}%
\AgdaBound{pbk3}\AgdaSymbol{)}\<%
\\
\>[0]\AgdaFunction{lemmaHoareTripleStackGeAux'4}\AgdaSpace{}%
\AgdaBound{msg₂}\AgdaSpace{}%
\AgdaBound{pbk1}\AgdaSpace{}%
\AgdaBound{pbk2}\AgdaSpace{}%
\AgdaBound{pbk3}\AgdaSpace{}%
\AgdaBound{sig1}\AgdaSpace{}%
\AgdaBound{sig2}\AgdaSpace{}%
\AgdaSymbol{\AgdaUnderscore{}}\AgdaSpace{}%
\AgdaSymbol{|}\AgdaSpace{}%
\AgdaInductiveConstructor{true}\AgdaSpace{}%
\AgdaSymbol{|}\AgdaSpace{}%
\AgdaInductiveConstructor{false}\AgdaSpace{}%
\AgdaSymbol{|}\AgdaSpace{}%
\AgdaInductiveConstructor{true}\AgdaSpace{}%
\AgdaSymbol{=}\AgdaSpace{}%
\AgdaInductiveConstructor{inj₂}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaInductiveConstructor{inj₁}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaInductiveConstructor{conj}\AgdaSpace{}%
\AgdaInductiveConstructor{tt}\AgdaSpace{}%
\AgdaInductiveConstructor{tt}\AgdaSymbol{))}\<%
\\
\>[0]\AgdaFunction{lemmaHoareTripleStackGeAux'4}\AgdaSpace{}%
\AgdaBound{msg₂}\AgdaSpace{}%
\AgdaBound{pbk1}\AgdaSpace{}%
\AgdaBound{pbk2}\AgdaSpace{}%
\AgdaBound{pbk3}\AgdaSpace{}%
\AgdaBound{sig1}\AgdaSpace{}%
\AgdaBound{sig2}\AgdaSpace{}%
\AgdaSymbol{\AgdaUnderscore{}}\AgdaSpace{}%
\AgdaSymbol{|}\AgdaSpace{}%
\AgdaInductiveConstructor{true}\AgdaSpace{}%
\AgdaSymbol{|}\AgdaSpace{}%
\AgdaInductiveConstructor{true}\AgdaSpace{}%
\AgdaSymbol{=}\AgdaSpace{}%
\AgdaInductiveConstructor{inj₁}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaInductiveConstructor{conj}\AgdaSpace{}%
\AgdaInductiveConstructor{tt}\AgdaSpace{}%
\AgdaInductiveConstructor{tt}\AgdaSymbol{)}\<%
\\
%
\\[\AgdaEmptyExtraSkip]%
%
\\[\AgdaEmptyExtraSkip]%
%
\\[\AgdaEmptyExtraSkip]%
%
\\[\AgdaEmptyExtraSkip]%
\>[0]\AgdaComment{--\textbackslash{}multisigweakestPreCondTwoFour}\<%
\end{code}
} % END AgdaHide

\newcommand{\multisigweakestPreCondTwoFour}{
\begin{code}%
\>[0]\AgdaFunction{weakestPreCondMultiSig-2-4ˢ}\AgdaSpace{}%
\AgdaSymbol{:}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaBound{pbk1}\AgdaSpace{}%
\AgdaBound{pbk2}\AgdaSpace{}%
\AgdaBound{pbk3}\AgdaSpace{}%
\AgdaBound{pbk4}\AgdaSpace{}%
\AgdaSymbol{:}%
\>[54]\AgdaDatatype{ℕ}\AgdaSymbol{)}\AgdaSpace{}%
\AgdaSymbol{→}\AgdaSpace{}%
\AgdaFunction{StackPredicate}\<%
\\
\>[0]\AgdaFunction{weakestPreCondMultiSig-2-4ˢ}\AgdaSpace{}%
\AgdaBound{pbk1}\AgdaSpace{}%
\AgdaBound{pbk2}\AgdaSpace{}%
\AgdaBound{pbk3}\AgdaSpace{}%
\AgdaBound{pbk4}\AgdaSpace{}%
\AgdaBound{time}%
\>[54]\AgdaBound{msg₁}\AgdaSpace{}%
\AgdaInductiveConstructor{[]}\AgdaSpace{}%
\AgdaSymbol{=}\AgdaSpace{}%
\AgdaDatatype{⊥}\<%
\\
\>[0]\AgdaFunction{weakestPreCondMultiSig-2-4ˢ}\AgdaSpace{}%
\AgdaBound{pbk1}\AgdaSpace{}%
\AgdaBound{pbk2}\AgdaSpace{}%
\AgdaBound{pbk3}\AgdaSpace{}%
\AgdaBound{pbk4}\AgdaSpace{}%
\AgdaBound{time}%
\>[54]\AgdaBound{msg₁}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaBound{x}\AgdaSpace{}%
\AgdaOperator{\AgdaInductiveConstructor{∷}}\AgdaSpace{}%
\AgdaInductiveConstructor{[]}\AgdaSymbol{)}\AgdaSpace{}%
\AgdaSymbol{=}\AgdaSpace{}%
\AgdaDatatype{⊥}\<%
\\
\>[0]\AgdaFunction{weakestPreCondMultiSig-2-4ˢ}\AgdaSpace{}%
\AgdaBound{pbk1}\AgdaSpace{}%
\AgdaBound{pbk2}\AgdaSpace{}%
\AgdaBound{pbk3}\AgdaSpace{}%
\AgdaBound{pbk4}\AgdaSpace{}%
\AgdaBound{time}%
\>[54]\AgdaBound{msg₁}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaBound{x}\AgdaSpace{}%
\AgdaOperator{\AgdaInductiveConstructor{∷}}\AgdaSpace{}%
\AgdaBound{y}\AgdaSpace{}%
\AgdaOperator{\AgdaInductiveConstructor{∷}}\AgdaSpace{}%
\AgdaInductiveConstructor{[]}\AgdaSymbol{)}\AgdaSpace{}%
\AgdaSymbol{=}\AgdaSpace{}%
\AgdaDatatype{⊥}\<%
\\
\>[0]\AgdaFunction{weakestPreCondMultiSig-2-4ˢ}\AgdaSpace{}%
\AgdaBound{pbk1}\AgdaSpace{}%
\AgdaBound{pbk2}\AgdaSpace{}%
\AgdaBound{pbk3}\AgdaSpace{}%
\AgdaBound{pbk4}\AgdaSpace{}%
\AgdaBound{time}%
\>[54]\AgdaBound{msg₁}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaSpace{}%
\AgdaBound{sig2}\AgdaSpace{}%
\AgdaOperator{\AgdaInductiveConstructor{∷}}\AgdaSpace{}%
\AgdaBound{sig1}\AgdaSpace{}%
\AgdaOperator{\AgdaInductiveConstructor{∷}}\AgdaSpace{}%
\AgdaBound{dummy}\AgdaSpace{}%
\AgdaOperator{\AgdaInductiveConstructor{∷}}\AgdaSpace{}%
\AgdaBound{stack₁}\AgdaSymbol{)}\AgdaSpace{}%
\AgdaSymbol{=}\<%
\\
\>[0][@{}l@{\AgdaIndent{0}}]%
\>[7]\AgdaSymbol{(}%
\>[10]\AgdaSymbol{(}\AgdaFunction{IsSigned}\AgdaSpace{}%
\AgdaBound{msg₁}\AgdaSpace{}%
\AgdaBound{sig1}\AgdaSpace{}%
\AgdaBound{pbk1}\AgdaSpace{}%
\AgdaOperator{\AgdaRecord{∧}}%
\>[38]\AgdaFunction{IsSigned}\AgdaSpace{}%
\AgdaBound{msg₁}\AgdaSpace{}%
\AgdaBound{sig2}\AgdaSpace{}%
\AgdaBound{pbk2}\AgdaSymbol{)}\AgdaSpace{}%
\AgdaOperator{\AgdaDatatype{⊎}}\<%
\\
%
\>[10]\AgdaSymbol{(}\AgdaFunction{IsSigned}\AgdaSpace{}%
\AgdaBound{msg₁}\AgdaSpace{}%
\AgdaBound{sig1}\AgdaSpace{}%
\AgdaBound{pbk1}\AgdaSpace{}%
\AgdaOperator{\AgdaRecord{∧}}%
\>[38]\AgdaFunction{IsSigned}\AgdaSpace{}%
\AgdaBound{msg₁}\AgdaSpace{}%
\AgdaBound{sig2}\AgdaSpace{}%
\AgdaBound{pbk3}\AgdaSymbol{)}\AgdaSpace{}%
\AgdaOperator{\AgdaDatatype{⊎}}\<%
\\
%
\>[10]\AgdaSymbol{(}\AgdaFunction{IsSigned}\AgdaSpace{}%
\AgdaBound{msg₁}\AgdaSpace{}%
\AgdaBound{sig1}\AgdaSpace{}%
\AgdaBound{pbk1}\AgdaSpace{}%
\AgdaOperator{\AgdaRecord{∧}}%
\>[38]\AgdaFunction{IsSigned}\AgdaSpace{}%
\AgdaBound{msg₁}\AgdaSpace{}%
\AgdaBound{sig2}\AgdaSpace{}%
\AgdaBound{pbk4}\AgdaSymbol{)}\AgdaSpace{}%
\AgdaOperator{\AgdaDatatype{⊎}}\<%
\\
%
\>[10]\AgdaSymbol{(}\AgdaFunction{IsSigned}\AgdaSpace{}%
\AgdaBound{msg₁}\AgdaSpace{}%
\AgdaBound{sig1}\AgdaSpace{}%
\AgdaBound{pbk2}\AgdaSpace{}%
\AgdaOperator{\AgdaRecord{∧}}%
\>[38]\AgdaFunction{IsSigned}\AgdaSpace{}%
\AgdaBound{msg₁}\AgdaSpace{}%
\AgdaBound{sig2}\AgdaSpace{}%
\AgdaBound{pbk3}\AgdaSymbol{)}\AgdaSpace{}%
\AgdaOperator{\AgdaDatatype{⊎}}\<%
\\
%
\>[10]\AgdaSymbol{(}\AgdaFunction{IsSigned}\AgdaSpace{}%
\AgdaBound{msg₁}\AgdaSpace{}%
\AgdaBound{sig1}\AgdaSpace{}%
\AgdaBound{pbk2}\AgdaSpace{}%
\AgdaOperator{\AgdaRecord{∧}}%
\>[38]\AgdaFunction{IsSigned}\AgdaSpace{}%
\AgdaBound{msg₁}\AgdaSpace{}%
\AgdaBound{sig2}\AgdaSpace{}%
\AgdaBound{pbk4}\AgdaSymbol{)}\AgdaSpace{}%
\AgdaOperator{\AgdaDatatype{⊎}}\<%
\\
%
\>[10]\AgdaSymbol{(}\AgdaFunction{IsSigned}\AgdaSpace{}%
\AgdaBound{msg₁}\AgdaSpace{}%
\AgdaBound{sig1}\AgdaSpace{}%
\AgdaBound{pbk3}\AgdaSpace{}%
\AgdaOperator{\AgdaRecord{∧}}%
\>[38]\AgdaFunction{IsSigned}\AgdaSpace{}%
\AgdaBound{msg₁}\AgdaSpace{}%
\AgdaBound{sig2}\AgdaSpace{}%
\AgdaBound{pbk4}\AgdaSymbol{))}\<%
\end{code}
} % END newcommand

\AgdaHide{
\begin{code}%
\>[0]\<%
\\
%
\\[\AgdaEmptyExtraSkip]%
%
\\[\AgdaEmptyExtraSkip]%
%
\\[\AgdaEmptyExtraSkip]%
\>[0]\AgdaFunction{HoareTripleStackGeAux'}\AgdaSpace{}%
\AgdaSymbol{:}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaBound{msg₁}\AgdaSpace{}%
\AgdaSymbol{:}\AgdaSpace{}%
\AgdaDatatype{Msg}\AgdaSymbol{)(}\AgdaBound{pbk1}\AgdaSpace{}%
\AgdaBound{pbk2}\AgdaSpace{}%
\AgdaBound{pbk3}\AgdaSpace{}%
\AgdaSymbol{:}\AgdaSpace{}%
\AgdaDatatype{ℕ}\AgdaSymbol{)}\AgdaSpace{}%
\AgdaSymbol{→}\<%
\\
\>[0][@{}l@{\AgdaIndent{0}}]%
\>[17]\AgdaOperator{\AgdaRecord{<}}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaFunction{weakestPreCondMultiSig-2-3-bas}\AgdaSpace{}%
\AgdaBound{pbk1}\AgdaSpace{}%
\AgdaBound{pbk2}\AgdaSpace{}%
\AgdaBound{pbk3}\AgdaSymbol{)}\AgdaSpace{}%
\AgdaOperator{\AgdaRecord{>gˢ}}\<%
\\
%
\>[17]\AgdaSymbol{(λ}%
\>[873I]\AgdaBound{time₁}\AgdaSpace{}%
\AgdaBound{msg₁}\AgdaSpace{}%
\AgdaBound{stack}\AgdaSpace{}%
\AgdaSymbol{→}\<%
\\
\>[.][@{}l@{}]\<[873I]%
\>[20]\AgdaFunction{executeMultiSig3}\AgdaSpace{}%
\AgdaBound{msg₁}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaBound{pbk1}\AgdaSpace{}%
\AgdaOperator{\AgdaInductiveConstructor{∷}}\AgdaSpace{}%
\AgdaBound{pbk2}\AgdaSpace{}%
\AgdaOperator{\AgdaInductiveConstructor{∷}}\AgdaSpace{}%
\AgdaBound{pbk3}\AgdaSpace{}%
\AgdaOperator{\AgdaInductiveConstructor{∷}}\AgdaSpace{}%
\AgdaInductiveConstructor{[]}\AgdaSymbol{)}\AgdaSpace{}%
\AgdaNumber{2}\AgdaSpace{}%
\AgdaBound{stack}\AgdaSpace{}%
\AgdaInductiveConstructor{[]}\AgdaSymbol{)}\<%
\\
%
\>[17]\AgdaOperator{\AgdaRecord{<}}\AgdaSpace{}%
\AgdaSymbol{(λ}\AgdaSpace{}%
\AgdaBound{time₁}\AgdaSpace{}%
\AgdaBound{msg₁}\AgdaSpace{}%
\AgdaBound{stack}\AgdaSpace{}%
\AgdaSymbol{→}\AgdaSpace{}%
\AgdaFunction{acceptStateˢ}\AgdaSpace{}%
\AgdaBound{time₁}\AgdaSpace{}%
\AgdaBound{msg₁}\AgdaSpace{}%
\AgdaBound{stack}\AgdaSymbol{)}\AgdaSpace{}%
\AgdaOperator{\AgdaRecord{>}}\<%
\\
\>[0]\AgdaFunction{HoareTripleStackGeAux'}\AgdaSpace{}%
\AgdaBound{msg₁}\AgdaSpace{}%
\AgdaBound{pbk1}\AgdaSpace{}%
\AgdaBound{pbk2}\AgdaSpace{}%
\AgdaBound{pbk3}\AgdaSpace{}%
\AgdaSymbol{.}\AgdaField{==>stg}\AgdaSpace{}%
\AgdaBound{time}\AgdaSpace{}%
\AgdaBound{msg₂}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaBound{sig2}\AgdaSpace{}%
\AgdaOperator{\AgdaInductiveConstructor{∷}}\AgdaSpace{}%
\AgdaBound{sig1}\AgdaSpace{}%
\AgdaOperator{\AgdaInductiveConstructor{∷}}\AgdaSpace{}%
\AgdaBound{dummy}\AgdaSpace{}%
\AgdaOperator{\AgdaInductiveConstructor{∷}}\AgdaSpace{}%
\AgdaBound{s}\AgdaSymbol{)}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaInductiveConstructor{inj₁}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaInductiveConstructor{conj}\AgdaSpace{}%
\AgdaBound{and3}\AgdaSpace{}%
\AgdaBound{and4}\AgdaSymbol{))}\<%
\\
\>[0][@{}l@{\AgdaIndent{0}}]%
\>[10]\AgdaSymbol{=}%
\>[916I]\AgdaFunction{boolToNatNotFalseLemma}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaFunction{compareSigsMultiSigAux}\AgdaSpace{}%
\AgdaBound{msg₂}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaBound{sig2}\AgdaSpace{}%
\AgdaOperator{\AgdaInductiveConstructor{∷}}\AgdaSpace{}%
\AgdaInductiveConstructor{[]}\AgdaSymbol{)}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaBound{pbk2}\AgdaSpace{}%
\AgdaOperator{\AgdaInductiveConstructor{∷}}\AgdaSpace{}%
\AgdaBound{pbk3}\AgdaSpace{}%
\AgdaOperator{\AgdaInductiveConstructor{∷}}\AgdaSpace{}%
\AgdaInductiveConstructor{[]}\AgdaSymbol{)}\AgdaSpace{}%
\AgdaBound{sig1}\<%
\\
\>[.][@{}l@{}]\<[916I]%
\>[12]\AgdaSymbol{(}\AgdaFunction{isSigned}%
\>[23]\AgdaBound{msg₂}\AgdaSpace{}%
\AgdaBound{sig1}\AgdaSpace{}%
\AgdaBound{pbk1}\AgdaSymbol{))}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaFunction{lemmaHoareTripleStackGeAux'1}\AgdaSpace{}%
\AgdaBound{msg₂}\AgdaSpace{}%
\AgdaBound{pbk1}\AgdaSpace{}%
\AgdaBound{pbk2}\AgdaSpace{}%
\AgdaBound{pbk3}\AgdaSpace{}%
\AgdaBound{sig1}\AgdaSpace{}%
\AgdaBound{sig2}\AgdaSpace{}%
\AgdaBound{and3}\AgdaSpace{}%
\AgdaBound{and4}\AgdaSymbol{)}\<%
\\
%
\\[\AgdaEmptyExtraSkip]%
\>[0]\AgdaFunction{HoareTripleStackGeAux'}\AgdaSpace{}%
\AgdaBound{msg₁}\AgdaSpace{}%
\AgdaBound{pbk1}\AgdaSpace{}%
\AgdaBound{pbk2}\AgdaSpace{}%
\AgdaBound{pbk3}\AgdaSpace{}%
\AgdaSymbol{.}\AgdaField{==>stg}\AgdaSpace{}%
\AgdaBound{time}\AgdaSpace{}%
\AgdaBound{msg₂}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaBound{sig2}\AgdaSpace{}%
\AgdaOperator{\AgdaInductiveConstructor{∷}}\AgdaSpace{}%
\AgdaBound{sig1}\AgdaSpace{}%
\AgdaOperator{\AgdaInductiveConstructor{∷}}\AgdaSpace{}%
\AgdaBound{dummy}\AgdaSpace{}%
\AgdaOperator{\AgdaInductiveConstructor{∷}}\AgdaSpace{}%
\AgdaBound{s}\AgdaSymbol{)}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaInductiveConstructor{inj₂}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaInductiveConstructor{inj₁}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaInductiveConstructor{conj}\AgdaSpace{}%
\AgdaBound{and3}\AgdaSpace{}%
\AgdaBound{and4}\AgdaSymbol{)))}\<%
\\
\>[0][@{}l@{\AgdaIndent{0}}]%
\>[10]\AgdaSymbol{=}%
\>[958I]\AgdaFunction{boolToNatNotFalseLemma}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaFunction{compareSigsMultiSigAux}\AgdaSpace{}%
\AgdaBound{msg₂}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaBound{sig2}\AgdaSpace{}%
\AgdaOperator{\AgdaInductiveConstructor{∷}}\AgdaSpace{}%
\AgdaInductiveConstructor{[]}\AgdaSymbol{)}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaBound{pbk2}\AgdaSpace{}%
\AgdaOperator{\AgdaInductiveConstructor{∷}}\AgdaSpace{}%
\AgdaBound{pbk3}\AgdaSpace{}%
\AgdaOperator{\AgdaInductiveConstructor{∷}}\AgdaSpace{}%
\AgdaInductiveConstructor{[]}\AgdaSymbol{)}\AgdaSpace{}%
\AgdaBound{sig1}\<%
\\
\>[958I][@{}l@{\AgdaIndent{0}}]%
\>[13]\AgdaSymbol{(}\AgdaFunction{isSigned}%
\>[24]\AgdaBound{msg₂}\AgdaSpace{}%
\AgdaBound{sig1}\AgdaSpace{}%
\AgdaBound{pbk1}\AgdaSymbol{))}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaFunction{lemmaHoareTripleStackGeAux'2}%
\>[72]\AgdaBound{msg₂}\AgdaSpace{}%
\AgdaBound{pbk1}\AgdaSpace{}%
\AgdaBound{pbk2}\AgdaSpace{}%
\AgdaBound{pbk3}\AgdaSpace{}%
\AgdaBound{sig1}\AgdaSpace{}%
\AgdaBound{sig2}\AgdaSpace{}%
\AgdaBound{and3}\AgdaSpace{}%
\AgdaBound{and4}\AgdaSymbol{)}\<%
\\
%
\\[\AgdaEmptyExtraSkip]%
\>[0]\AgdaFunction{HoareTripleStackGeAux'}\AgdaSpace{}%
\AgdaBound{msg₁}\AgdaSpace{}%
\AgdaBound{pbk1}\AgdaSpace{}%
\AgdaBound{pbk2}\AgdaSpace{}%
\AgdaBound{pbk3}\AgdaSpace{}%
\AgdaSymbol{.}\AgdaField{==>stg}\AgdaSpace{}%
\AgdaBound{time}\AgdaSpace{}%
\AgdaBound{msg₂}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaBound{sig2}\AgdaSpace{}%
\AgdaOperator{\AgdaInductiveConstructor{∷}}\AgdaSpace{}%
\AgdaBound{sig1}\AgdaSpace{}%
\AgdaOperator{\AgdaInductiveConstructor{∷}}\AgdaSpace{}%
\AgdaBound{dummy}\AgdaSpace{}%
\AgdaOperator{\AgdaInductiveConstructor{∷}}\AgdaSpace{}%
\AgdaBound{s}\AgdaSymbol{)}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaInductiveConstructor{inj₂}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaInductiveConstructor{inj₂}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaInductiveConstructor{conj}\AgdaSpace{}%
\AgdaBound{and1}\AgdaSpace{}%
\AgdaBound{and2}\AgdaSymbol{)))}\<%
\\
\>[0][@{}l@{\AgdaIndent{0}}]%
\>[10]\AgdaSymbol{=}\AgdaSpace{}%
\AgdaFunction{boolToNatNotFalseLemma}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaFunction{compareSigsMultiSigAux}\AgdaSpace{}%
\AgdaBound{msg₂}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaBound{sig2}\AgdaSpace{}%
\AgdaOperator{\AgdaInductiveConstructor{∷}}\AgdaSpace{}%
\AgdaInductiveConstructor{[]}\AgdaSymbol{)}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaBound{pbk2}\AgdaSpace{}%
\AgdaOperator{\AgdaInductiveConstructor{∷}}\AgdaSpace{}%
\AgdaBound{pbk3}\AgdaSpace{}%
\AgdaOperator{\AgdaInductiveConstructor{∷}}\AgdaSpace{}%
\AgdaInductiveConstructor{[]}\AgdaSymbol{)}\AgdaSpace{}%
\AgdaBound{sig1}\<%
\\
\>[10][@{}l@{\AgdaIndent{0}}]%
\>[11]\AgdaSymbol{(}\AgdaFunction{isSigned}%
\>[22]\AgdaBound{msg₂}\AgdaSpace{}%
\AgdaBound{sig1}\AgdaSpace{}%
\AgdaBound{pbk1}\AgdaSpace{}%
\AgdaSymbol{))}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaFunction{lemmaHoareTripleStackGeAux'3}\AgdaSpace{}%
\AgdaBound{msg₂}\AgdaSpace{}%
\AgdaBound{pbk1}\AgdaSpace{}%
\AgdaBound{pbk2}\AgdaSpace{}%
\AgdaBound{pbk3}\AgdaSpace{}%
\AgdaBound{sig1}\AgdaSpace{}%
\AgdaBound{sig2}\AgdaSpace{}%
\AgdaBound{and1}\AgdaSpace{}%
\AgdaBound{and2}\AgdaSymbol{)}\<%
\\
%
\\[\AgdaEmptyExtraSkip]%
\>[0]\AgdaFunction{HoareTripleStackGeAux'}\AgdaSpace{}%
\AgdaBound{msg₁}\AgdaSpace{}%
\AgdaBound{pbk1}\AgdaSpace{}%
\AgdaBound{pbk2}\AgdaSpace{}%
\AgdaBound{pbk3}\AgdaSpace{}%
\AgdaComment{\{-numsig\ stack\ time₁-\}}\AgdaSpace{}%
\AgdaSymbol{.}\AgdaField{<==stg}\AgdaSpace{}%
\AgdaBound{time}\AgdaSpace{}%
\AgdaBound{msg₂}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaBound{sig2}\AgdaSpace{}%
\AgdaOperator{\AgdaInductiveConstructor{∷}}\AgdaSpace{}%
\AgdaBound{sig1}\AgdaSpace{}%
\AgdaOperator{\AgdaInductiveConstructor{∷}}\AgdaSpace{}%
\AgdaBound{dummy}\AgdaSpace{}%
\AgdaOperator{\AgdaInductiveConstructor{∷}}\AgdaSpace{}%
\AgdaBound{s}\AgdaSymbol{)}\AgdaSpace{}%
\AgdaBound{x}\<%
\\
\>[0][@{}l@{\AgdaIndent{0}}]%
\>[4]\AgdaSymbol{=}%
\>[1039I]\AgdaFunction{lemmaHoareTripleStackGeAux'4}\AgdaSpace{}%
\AgdaBound{msg₂}\AgdaSpace{}%
\AgdaBound{pbk1}\AgdaSpace{}%
\AgdaBound{pbk2}\AgdaSpace{}%
\AgdaBound{pbk3}\AgdaSpace{}%
\AgdaBound{sig1}\AgdaSpace{}%
\AgdaBound{sig2}\<%
\\
\>[1039I][@{}l@{\AgdaIndent{0}}]%
\>[8]\AgdaSymbol{(}\AgdaFunction{boolToNatNotFalseLemma2}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaFunction{compareSigsMultiSigAux}\AgdaSpace{}%
\AgdaBound{msg₂}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaBound{sig2}\AgdaSpace{}%
\AgdaOperator{\AgdaInductiveConstructor{∷}}\AgdaSpace{}%
\AgdaInductiveConstructor{[]}\AgdaSymbol{)}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaBound{pbk2}\AgdaSpace{}%
\AgdaOperator{\AgdaInductiveConstructor{∷}}\AgdaSpace{}%
\AgdaBound{pbk3}\AgdaSpace{}%
\AgdaOperator{\AgdaInductiveConstructor{∷}}\AgdaSpace{}%
\AgdaInductiveConstructor{[]}\AgdaSymbol{)}\AgdaSpace{}%
\AgdaBound{sig1}\<%
\\
\>[8][@{}l@{\AgdaIndent{0}}]%
\>[11]\AgdaSymbol{(}\AgdaFunction{isSigned}%
\>[22]\AgdaBound{msg₂}\AgdaSpace{}%
\AgdaBound{sig1}\AgdaSpace{}%
\AgdaBound{pbk1}\AgdaSpace{}%
\AgdaSymbol{))}\AgdaSpace{}%
\AgdaBound{x}\AgdaSymbol{)}\<%
\\
%
\\[\AgdaEmptyExtraSkip]%
%
\\[\AgdaEmptyExtraSkip]%
\>[0]\AgdaFunction{lemmaHoareTripleStackGeAux'7}%
\>[1061I]\AgdaSymbol{:}%
\>[1062I]\AgdaSymbol{(}\AgdaBound{msg₂}\AgdaSpace{}%
\AgdaSymbol{:}\AgdaSpace{}%
\AgdaDatatype{Msg}\AgdaSymbol{)}\<%
\\
\>[.][@{}l@{}]\<[1062I]%
\>[31]\AgdaSymbol{(}\AgdaBound{pbk1}\AgdaSpace{}%
\AgdaBound{pbk2}\AgdaSpace{}%
\AgdaBound{pbk3}\AgdaSpace{}%
\AgdaBound{pbk4}\AgdaSpace{}%
\AgdaBound{sig1}\AgdaSpace{}%
\AgdaBound{sig2}\AgdaSpace{}%
\AgdaSymbol{:}\AgdaSpace{}%
\AgdaDatatype{ℕ}\AgdaSymbol{)}\<%
\\
%
\>[31]\AgdaSymbol{→}\AgdaSpace{}%
\AgdaFunction{True}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaFunction{isSigned}%
\>[49]\AgdaBound{msg₂}\AgdaSpace{}%
\AgdaBound{sig1}\AgdaSpace{}%
\AgdaBound{pbk1}\AgdaSymbol{)}\<%
\\
\>[1061I][@{}l@{\AgdaIndent{0}}]%
\>[30]\AgdaSymbol{→}%
\>[33]\AgdaFunction{True}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaFunction{isSigned}%
\>[49]\AgdaBound{msg₂}\AgdaSpace{}%
\AgdaBound{sig2}\AgdaSpace{}%
\AgdaBound{pbk2}\AgdaSymbol{)}\<%
\\
\>[30][@{}l@{\AgdaIndent{0}}]%
\>[31]\AgdaSymbol{→}\AgdaSpace{}%
\AgdaFunction{True}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaFunction{compareSigsMultiSig}\AgdaSpace{}%
\AgdaBound{msg₂}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaSpace{}%
\AgdaBound{sig1}\AgdaSpace{}%
\AgdaOperator{\AgdaInductiveConstructor{∷}}\AgdaSpace{}%
\AgdaBound{sig2}\AgdaSpace{}%
\AgdaOperator{\AgdaInductiveConstructor{∷}}\AgdaSpace{}%
\AgdaInductiveConstructor{[]}\AgdaSymbol{)}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaBound{pbk1}\AgdaSpace{}%
\AgdaOperator{\AgdaInductiveConstructor{∷}}\AgdaSpace{}%
\AgdaBound{pbk2}\AgdaSpace{}%
\AgdaOperator{\AgdaInductiveConstructor{∷}}\AgdaSpace{}%
\AgdaBound{pbk3}\AgdaSpace{}%
\AgdaOperator{\AgdaInductiveConstructor{∷}}\AgdaSpace{}%
\AgdaBound{pbk4}\AgdaSpace{}%
\AgdaOperator{\AgdaInductiveConstructor{∷}}%
\>[114]\AgdaInductiveConstructor{[]}\AgdaSymbol{))}\<%
\\
%
\\[\AgdaEmptyExtraSkip]%
\>[0]\AgdaFunction{lemmaHoareTripleStackGeAux'7}\AgdaSpace{}%
\AgdaBound{msg₂}\AgdaSpace{}%
\AgdaBound{pbk1}\AgdaSpace{}%
\AgdaBound{pbk2}\AgdaSpace{}%
\AgdaBound{pbk3}\AgdaSpace{}%
\AgdaBound{pbk4}\AgdaSpace{}%
\AgdaBound{sig1}\AgdaSpace{}%
\AgdaBound{sig2}\AgdaSpace{}%
\AgdaBound{x}\AgdaSpace{}%
\AgdaBound{x₁}\AgdaSpace{}%
\AgdaKeyword{with}%
\>[75]\AgdaSymbol{(}\AgdaFunction{isSigned}%
\>[86]\AgdaBound{msg₂}\AgdaSpace{}%
\AgdaBound{sig1}\AgdaSpace{}%
\AgdaBound{pbk1}\AgdaSymbol{)}\<%
\\
\>[0]\AgdaFunction{lemmaHoareTripleStackGeAux'7}\AgdaSpace{}%
\AgdaBound{msg₂}\AgdaSpace{}%
\AgdaBound{pbk1}\AgdaSpace{}%
\AgdaBound{pbk2}\AgdaSpace{}%
\AgdaBound{pbk3}\AgdaSpace{}%
\AgdaBound{pbk4}\AgdaSpace{}%
\AgdaBound{sig1}\AgdaSpace{}%
\AgdaBound{sig2}\AgdaSpace{}%
\AgdaBound{x}\AgdaSpace{}%
\AgdaBound{x₁}\AgdaSpace{}%
\AgdaSymbol{|}\AgdaSpace{}%
\AgdaInductiveConstructor{true}\AgdaSpace{}%
\AgdaKeyword{with}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaFunction{isSigned}%
\>[92]\AgdaBound{msg₂}\AgdaSpace{}%
\AgdaBound{sig2}\AgdaSpace{}%
\AgdaBound{pbk2}\AgdaSymbol{)}\<%
\\
\>[0]\AgdaFunction{lemmaHoareTripleStackGeAux'7}\AgdaSpace{}%
\AgdaBound{msg₂}\AgdaSpace{}%
\AgdaBound{pbk1}\AgdaSpace{}%
\AgdaBound{pbk2}\AgdaSpace{}%
\AgdaBound{pbk3}\AgdaSpace{}%
\AgdaBound{pbk4}\AgdaSpace{}%
\AgdaBound{sig1}\AgdaSpace{}%
\AgdaBound{sig2}\AgdaSpace{}%
\AgdaBound{x}\AgdaSpace{}%
\AgdaBound{x₁}\AgdaSpace{}%
\AgdaSymbol{|}\AgdaSpace{}%
\AgdaInductiveConstructor{true}\AgdaSpace{}%
\AgdaSymbol{|}\AgdaSpace{}%
\AgdaInductiveConstructor{true}\AgdaSpace{}%
\AgdaSymbol{=}\AgdaSpace{}%
\AgdaInductiveConstructor{tt}\<%
\\
%
\\[\AgdaEmptyExtraSkip]%
%
\\[\AgdaEmptyExtraSkip]%
\>[0]\AgdaFunction{lemmaHoareTripleStackGeAux'8}%
\>[1138I]\AgdaSymbol{:}%
\>[1139I]\AgdaSymbol{(}\AgdaBound{msg₂}\AgdaSpace{}%
\AgdaSymbol{:}\AgdaSpace{}%
\AgdaDatatype{Msg}\AgdaSymbol{)}\<%
\\
\>[.][@{}l@{}]\<[1139I]%
\>[31]\AgdaSymbol{(}\AgdaBound{pbk1}\AgdaSpace{}%
\AgdaBound{pbk2}\AgdaSpace{}%
\AgdaBound{pbk3}\AgdaSpace{}%
\AgdaBound{pbk4}\AgdaSpace{}%
\AgdaBound{sig1}\AgdaSpace{}%
\AgdaBound{sig2}\AgdaSpace{}%
\AgdaSymbol{:}\AgdaSpace{}%
\AgdaDatatype{ℕ}\AgdaSymbol{)}\<%
\\
%
\>[31]\AgdaSymbol{→}\AgdaSpace{}%
\AgdaFunction{True}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaFunction{isSigned}%
\>[49]\AgdaBound{msg₂}\AgdaSpace{}%
\AgdaBound{sig1}\AgdaSpace{}%
\AgdaBound{pbk1}\AgdaSymbol{)}\<%
\\
\>[1138I][@{}l@{\AgdaIndent{0}}]%
\>[30]\AgdaSymbol{→}%
\>[33]\AgdaFunction{True}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaFunction{isSigned}%
\>[49]\AgdaBound{msg₂}\AgdaSpace{}%
\AgdaBound{sig2}\AgdaSpace{}%
\AgdaBound{pbk3}\AgdaSymbol{)}\<%
\\
\>[30][@{}l@{\AgdaIndent{0}}]%
\>[31]\AgdaSymbol{→}\AgdaSpace{}%
\AgdaFunction{True}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaFunction{compareSigsMultiSig}\AgdaSpace{}%
\AgdaBound{msg₂}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaSpace{}%
\AgdaBound{sig1}\AgdaSpace{}%
\AgdaOperator{\AgdaInductiveConstructor{∷}}\AgdaSpace{}%
\AgdaBound{sig2}\AgdaSpace{}%
\AgdaOperator{\AgdaInductiveConstructor{∷}}\AgdaSpace{}%
\AgdaInductiveConstructor{[]}\AgdaSymbol{)}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaBound{pbk1}\AgdaSpace{}%
\AgdaOperator{\AgdaInductiveConstructor{∷}}\AgdaSpace{}%
\AgdaBound{pbk2}\AgdaSpace{}%
\AgdaOperator{\AgdaInductiveConstructor{∷}}\AgdaSpace{}%
\AgdaBound{pbk3}\AgdaSpace{}%
\AgdaOperator{\AgdaInductiveConstructor{∷}}\AgdaSpace{}%
\AgdaBound{pbk4}\AgdaSpace{}%
\AgdaOperator{\AgdaInductiveConstructor{∷}}%
\>[114]\AgdaInductiveConstructor{[]}\AgdaSymbol{))}\<%
\\
%
\\[\AgdaEmptyExtraSkip]%
\>[0]\AgdaFunction{lemmaHoareTripleStackGeAux'8}\AgdaSpace{}%
\AgdaBound{msg₂}\AgdaSpace{}%
\AgdaBound{pbk1}\AgdaSpace{}%
\AgdaBound{pbk2}\AgdaSpace{}%
\AgdaBound{pbk3}\AgdaSpace{}%
\AgdaBound{pbk4}\AgdaSpace{}%
\AgdaBound{sig1}\AgdaSpace{}%
\AgdaBound{sig2}\AgdaSpace{}%
\AgdaBound{x}\AgdaSpace{}%
\AgdaBound{x₁}\AgdaSpace{}%
\AgdaKeyword{with}%
\>[75]\AgdaSymbol{(}\AgdaFunction{isSigned}%
\>[86]\AgdaBound{msg₂}\AgdaSpace{}%
\AgdaBound{sig2}\AgdaSpace{}%
\AgdaBound{pbk1}\AgdaSymbol{)}\<%
\\
\>[0]\AgdaFunction{lemmaHoareTripleStackGeAux'8}\AgdaSpace{}%
\AgdaBound{msg₂}\AgdaSpace{}%
\AgdaBound{pbk1}\AgdaSpace{}%
\AgdaBound{pbk2}\AgdaSpace{}%
\AgdaBound{pbk3}\AgdaSpace{}%
\AgdaBound{pbk4}\AgdaSpace{}%
\AgdaBound{sig1}\AgdaSpace{}%
\AgdaBound{sig2}\AgdaSpace{}%
\AgdaBound{x}\AgdaSpace{}%
\AgdaBound{x₁}\AgdaSpace{}%
\AgdaSymbol{|}\AgdaSpace{}%
\AgdaInductiveConstructor{false}\AgdaSpace{}%
\AgdaKeyword{with}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaFunction{isSigned}%
\>[93]\AgdaBound{msg₂}\AgdaSpace{}%
\AgdaBound{sig1}\AgdaSpace{}%
\AgdaBound{pbk1}\AgdaSymbol{)}\<%
\\
\>[0]\AgdaFunction{lemmaHoareTripleStackGeAux'8}\AgdaSpace{}%
\AgdaBound{msg₂}\AgdaSpace{}%
\AgdaBound{pbk1}\AgdaSpace{}%
\AgdaBound{pbk2}\AgdaSpace{}%
\AgdaBound{pbk3}\AgdaSpace{}%
\AgdaBound{pbk4}\AgdaSpace{}%
\AgdaBound{sig1}\AgdaSpace{}%
\AgdaBound{sig2}\AgdaSpace{}%
\AgdaBound{x}\AgdaSpace{}%
\AgdaBound{x₁}\AgdaSpace{}%
\AgdaSymbol{|}\AgdaSpace{}%
\AgdaInductiveConstructor{false}\AgdaSpace{}%
\AgdaSymbol{|}\AgdaSpace{}%
\AgdaInductiveConstructor{true}\AgdaSpace{}%
\AgdaKeyword{with}%
\>[90]\AgdaSymbol{(}\AgdaFunction{isSigned}%
\>[101]\AgdaBound{msg₂}\AgdaSpace{}%
\AgdaBound{sig2}\AgdaSpace{}%
\AgdaBound{pbk2}\AgdaSymbol{)}\<%
\\
\>[0]\AgdaFunction{lemmaHoareTripleStackGeAux'8}\AgdaSpace{}%
\AgdaBound{msg₂}\AgdaSpace{}%
\AgdaBound{pbk1}\AgdaSpace{}%
\AgdaBound{pbk2}\AgdaSpace{}%
\AgdaBound{pbk3}\AgdaSpace{}%
\AgdaBound{pbk4}\AgdaSpace{}%
\AgdaBound{sig1}\AgdaSpace{}%
\AgdaBound{sig2}\AgdaSpace{}%
\AgdaBound{x}\AgdaSpace{}%
\AgdaBound{x₁}\AgdaSpace{}%
\AgdaSymbol{|}\AgdaSpace{}%
\AgdaInductiveConstructor{false}\AgdaSpace{}%
\AgdaSymbol{|}\AgdaSpace{}%
\AgdaInductiveConstructor{true}\AgdaSpace{}%
\AgdaSymbol{|}\AgdaSpace{}%
\AgdaInductiveConstructor{false}\AgdaSpace{}%
\AgdaKeyword{with}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaFunction{isSigned}%
\>[108]\AgdaBound{msg₂}\AgdaSpace{}%
\AgdaBound{sig2}\AgdaSpace{}%
\AgdaBound{pbk3}\AgdaSymbol{)}\<%
\\
\>[0]\AgdaFunction{lemmaHoareTripleStackGeAux'8}\AgdaSpace{}%
\AgdaBound{msg₂}\AgdaSpace{}%
\AgdaBound{pbk1}\AgdaSpace{}%
\AgdaBound{pbk2}\AgdaSpace{}%
\AgdaBound{pbk3}\AgdaSpace{}%
\AgdaBound{pbk4}\AgdaSpace{}%
\AgdaBound{sig1}\AgdaSpace{}%
\AgdaBound{sig2}\AgdaSpace{}%
\AgdaBound{x}\AgdaSpace{}%
\AgdaBound{x₁}\AgdaSpace{}%
\AgdaSymbol{|}\AgdaSpace{}%
\AgdaInductiveConstructor{false}\AgdaSpace{}%
\AgdaSymbol{|}\AgdaSpace{}%
\AgdaInductiveConstructor{true}\AgdaSpace{}%
\AgdaSymbol{|}\AgdaSpace{}%
\AgdaInductiveConstructor{false}\AgdaSpace{}%
\AgdaSymbol{|}\AgdaSpace{}%
\AgdaInductiveConstructor{true}\AgdaSpace{}%
\AgdaSymbol{=}\AgdaSpace{}%
\AgdaInductiveConstructor{tt}\<%
\\
\>[0]\AgdaFunction{lemmaHoareTripleStackGeAux'8}\AgdaSpace{}%
\AgdaBound{msg₂}\AgdaSpace{}%
\AgdaBound{pbk1}\AgdaSpace{}%
\AgdaBound{pbk2}\AgdaSpace{}%
\AgdaBound{pbk3}\AgdaSpace{}%
\AgdaBound{pbk4}\AgdaSpace{}%
\AgdaBound{sig1}\AgdaSpace{}%
\AgdaBound{sig2}\AgdaSpace{}%
\AgdaBound{x}\AgdaSpace{}%
\AgdaBound{x₁}\AgdaSpace{}%
\AgdaSymbol{|}\AgdaSpace{}%
\AgdaInductiveConstructor{false}\AgdaSpace{}%
\AgdaSymbol{|}\AgdaSpace{}%
\AgdaInductiveConstructor{true}\AgdaSpace{}%
\AgdaSymbol{|}\AgdaSpace{}%
\AgdaInductiveConstructor{true}\AgdaSpace{}%
\AgdaSymbol{=}\AgdaSpace{}%
\AgdaInductiveConstructor{tt}\<%
\\
\>[0]\AgdaFunction{lemmaHoareTripleStackGeAux'8}\AgdaSpace{}%
\AgdaBound{msg₂}\AgdaSpace{}%
\AgdaBound{pbk1}\AgdaSpace{}%
\AgdaBound{pbk2}\AgdaSpace{}%
\AgdaBound{pbk3}\AgdaSpace{}%
\AgdaBound{pbk4}\AgdaSpace{}%
\AgdaBound{sig1}\AgdaSpace{}%
\AgdaBound{sig2}\AgdaSpace{}%
\AgdaBound{x}\AgdaSpace{}%
\AgdaBound{x₁}\AgdaSpace{}%
\AgdaSymbol{|}\AgdaSpace{}%
\AgdaInductiveConstructor{true}%
\>[77]\AgdaKeyword{with}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaFunction{isSigned}%
\>[93]\AgdaBound{msg₂}\AgdaSpace{}%
\AgdaBound{sig1}\AgdaSpace{}%
\AgdaBound{pbk1}\AgdaSymbol{)}\<%
\\
\>[0]\AgdaFunction{lemmaHoareTripleStackGeAux'8}\AgdaSpace{}%
\AgdaBound{msg₂}\AgdaSpace{}%
\AgdaBound{pbk1}\AgdaSpace{}%
\AgdaBound{pbk2}\AgdaSpace{}%
\AgdaBound{pbk3}\AgdaSpace{}%
\AgdaBound{pbk4}\AgdaSpace{}%
\AgdaBound{sig1}\AgdaSpace{}%
\AgdaBound{sig2}\AgdaSpace{}%
\AgdaBound{x}\AgdaSpace{}%
\AgdaBound{x₁}\AgdaSpace{}%
\AgdaSymbol{|}\AgdaSpace{}%
\AgdaInductiveConstructor{true}\AgdaSpace{}%
\AgdaSymbol{|}\AgdaSpace{}%
\AgdaInductiveConstructor{true}\AgdaSpace{}%
\AgdaKeyword{with}%
\>[89]\AgdaSymbol{(}\AgdaFunction{isSigned}%
\>[100]\AgdaBound{msg₂}\AgdaSpace{}%
\AgdaBound{sig2}\AgdaSpace{}%
\AgdaBound{pbk2}\AgdaSymbol{)}\<%
\\
\>[0]\AgdaFunction{lemmaHoareTripleStackGeAux'8}\AgdaSpace{}%
\AgdaBound{msg₂}\AgdaSpace{}%
\AgdaBound{pbk1}\AgdaSpace{}%
\AgdaBound{pbk2}\AgdaSpace{}%
\AgdaBound{pbk3}\AgdaSpace{}%
\AgdaBound{pbk4}\AgdaSpace{}%
\AgdaBound{sig1}\AgdaSpace{}%
\AgdaBound{sig2}\AgdaSpace{}%
\AgdaBound{x}\AgdaSpace{}%
\AgdaBound{x₁}\AgdaSpace{}%
\AgdaSymbol{|}\AgdaSpace{}%
\AgdaInductiveConstructor{true}\AgdaSpace{}%
\AgdaSymbol{|}\AgdaSpace{}%
\AgdaInductiveConstructor{true}\AgdaSpace{}%
\AgdaSymbol{|}\AgdaSpace{}%
\AgdaInductiveConstructor{false}\AgdaSpace{}%
\AgdaKeyword{with}%
\>[97]\AgdaSymbol{(}\AgdaFunction{isSigned}%
\>[108]\AgdaBound{msg₂}\AgdaSpace{}%
\AgdaBound{sig2}\AgdaSpace{}%
\AgdaBound{pbk3}\AgdaSymbol{)}\<%
\\
\>[0]\AgdaFunction{lemmaHoareTripleStackGeAux'8}\AgdaSpace{}%
\AgdaBound{msg₂}\AgdaSpace{}%
\AgdaBound{pbk1}\AgdaSpace{}%
\AgdaBound{pbk2}\AgdaSpace{}%
\AgdaBound{pbk3}\AgdaSpace{}%
\AgdaBound{pbk4}\AgdaSpace{}%
\AgdaBound{sig1}\AgdaSpace{}%
\AgdaBound{sig2}\AgdaSpace{}%
\AgdaBound{x}\AgdaSpace{}%
\AgdaBound{x₁}\AgdaSpace{}%
\AgdaSymbol{|}\AgdaSpace{}%
\AgdaInductiveConstructor{true}\AgdaSpace{}%
\AgdaSymbol{|}\AgdaSpace{}%
\AgdaInductiveConstructor{true}\AgdaSpace{}%
\AgdaSymbol{|}\AgdaSpace{}%
\AgdaInductiveConstructor{false}\AgdaSpace{}%
\AgdaSymbol{|}\AgdaSpace{}%
\AgdaInductiveConstructor{true}\AgdaSpace{}%
\AgdaSymbol{=}\AgdaSpace{}%
\AgdaInductiveConstructor{tt}\<%
\\
\>[0]\AgdaFunction{lemmaHoareTripleStackGeAux'8}\AgdaSpace{}%
\AgdaBound{msg₂}\AgdaSpace{}%
\AgdaBound{pbk1}\AgdaSpace{}%
\AgdaBound{pbk2}\AgdaSpace{}%
\AgdaBound{pbk3}\AgdaSpace{}%
\AgdaBound{pbk4}\AgdaSpace{}%
\AgdaBound{sig1}\AgdaSpace{}%
\AgdaBound{sig2}\AgdaSpace{}%
\AgdaBound{x}\AgdaSpace{}%
\AgdaBound{x₁}\AgdaSpace{}%
\AgdaSymbol{|}\AgdaSpace{}%
\AgdaInductiveConstructor{true}\AgdaSpace{}%
\AgdaSymbol{|}\AgdaSpace{}%
\AgdaInductiveConstructor{true}\AgdaSpace{}%
\AgdaSymbol{|}\AgdaSpace{}%
\AgdaInductiveConstructor{true}\AgdaSpace{}%
\AgdaSymbol{=}\AgdaSpace{}%
\AgdaInductiveConstructor{tt}\<%
\\
%
\\[\AgdaEmptyExtraSkip]%
%
\\[\AgdaEmptyExtraSkip]%
\>[0]\AgdaFunction{lemmaHoareTripleStackGeAux'9}%
\>[1355I]\AgdaSymbol{:}%
\>[1356I]\AgdaSymbol{(}\AgdaBound{msg₂}\AgdaSpace{}%
\AgdaSymbol{:}\AgdaSpace{}%
\AgdaDatatype{Msg}\AgdaSymbol{)}\<%
\\
\>[.][@{}l@{}]\<[1356I]%
\>[31]\AgdaSymbol{(}\AgdaBound{pbk1}\AgdaSpace{}%
\AgdaBound{pbk2}\AgdaSpace{}%
\AgdaBound{pbk3}\AgdaSpace{}%
\AgdaBound{pbk4}\AgdaSpace{}%
\AgdaBound{sig1}\AgdaSpace{}%
\AgdaBound{sig2}\AgdaSpace{}%
\AgdaSymbol{:}\AgdaSpace{}%
\AgdaDatatype{ℕ}\AgdaSymbol{)}\<%
\\
%
\>[31]\AgdaSymbol{→}\AgdaSpace{}%
\AgdaFunction{True}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaFunction{isSigned}%
\>[49]\AgdaBound{msg₂}\AgdaSpace{}%
\AgdaBound{sig1}\AgdaSpace{}%
\AgdaBound{pbk1}\AgdaSymbol{)}\<%
\\
\>[1355I][@{}l@{\AgdaIndent{0}}]%
\>[30]\AgdaSymbol{→}%
\>[33]\AgdaFunction{True}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaFunction{isSigned}%
\>[49]\AgdaBound{msg₂}\AgdaSpace{}%
\AgdaBound{sig2}\AgdaSpace{}%
\AgdaBound{pbk4}\AgdaSymbol{)}\<%
\\
\>[30][@{}l@{\AgdaIndent{0}}]%
\>[31]\AgdaSymbol{→}\AgdaSpace{}%
\AgdaFunction{True}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaFunction{compareSigsMultiSig}\AgdaSpace{}%
\AgdaBound{msg₂}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaSpace{}%
\AgdaBound{sig1}\AgdaSpace{}%
\AgdaOperator{\AgdaInductiveConstructor{∷}}\AgdaSpace{}%
\AgdaBound{sig2}\AgdaSpace{}%
\AgdaOperator{\AgdaInductiveConstructor{∷}}\AgdaSpace{}%
\AgdaInductiveConstructor{[]}\AgdaSymbol{)}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaBound{pbk1}\AgdaSpace{}%
\AgdaOperator{\AgdaInductiveConstructor{∷}}\AgdaSpace{}%
\AgdaBound{pbk2}\AgdaSpace{}%
\AgdaOperator{\AgdaInductiveConstructor{∷}}\AgdaSpace{}%
\AgdaBound{pbk3}\AgdaSpace{}%
\AgdaOperator{\AgdaInductiveConstructor{∷}}\AgdaSpace{}%
\AgdaBound{pbk4}\AgdaSpace{}%
\AgdaOperator{\AgdaInductiveConstructor{∷}}%
\>[114]\AgdaInductiveConstructor{[]}\AgdaSymbol{))}\<%
\\
%
\\[\AgdaEmptyExtraSkip]%
\>[0]\AgdaFunction{lemmaHoareTripleStackGeAux'9}\AgdaSpace{}%
\AgdaBound{msg₂}\AgdaSpace{}%
\AgdaBound{pbk1}\AgdaSpace{}%
\AgdaBound{pbk2}\AgdaSpace{}%
\AgdaBound{pbk3}\AgdaSpace{}%
\AgdaBound{pbk4}\AgdaSpace{}%
\AgdaBound{sig1}\AgdaSpace{}%
\AgdaBound{sig2}\AgdaSpace{}%
\AgdaBound{x}\AgdaSpace{}%
\AgdaBound{x₁}\AgdaSpace{}%
\AgdaKeyword{with}%
\>[75]\AgdaSymbol{(}\AgdaFunction{isSigned}%
\>[86]\AgdaBound{msg₂}\AgdaSpace{}%
\AgdaBound{sig1}\AgdaSpace{}%
\AgdaBound{pbk1}\AgdaSymbol{)}\<%
\\
\>[0]\AgdaFunction{lemmaHoareTripleStackGeAux'9}\AgdaSpace{}%
\AgdaBound{msg₂}\AgdaSpace{}%
\AgdaBound{pbk1}\AgdaSpace{}%
\AgdaBound{pbk2}\AgdaSpace{}%
\AgdaBound{pbk3}\AgdaSpace{}%
\AgdaBound{pbk4}\AgdaSpace{}%
\AgdaBound{sig1}\AgdaSpace{}%
\AgdaBound{sig2}\AgdaSpace{}%
\AgdaBound{x}\AgdaSpace{}%
\AgdaBound{x₁}\AgdaSpace{}%
\AgdaSymbol{|}\AgdaSpace{}%
\AgdaInductiveConstructor{true}\AgdaSpace{}%
\AgdaKeyword{with}%
\>[82]\AgdaSymbol{(}\AgdaFunction{isSigned}%
\>[93]\AgdaBound{msg₂}\AgdaSpace{}%
\AgdaBound{sig2}\AgdaSpace{}%
\AgdaBound{pbk2}\AgdaSymbol{)}\<%
\\
\>[0]\AgdaFunction{lemmaHoareTripleStackGeAux'9}\AgdaSpace{}%
\AgdaBound{msg₂}\AgdaSpace{}%
\AgdaBound{pbk1}\AgdaSpace{}%
\AgdaBound{pbk2}\AgdaSpace{}%
\AgdaBound{pbk3}\AgdaSpace{}%
\AgdaBound{pbk4}\AgdaSpace{}%
\AgdaBound{sig1}\AgdaSpace{}%
\AgdaBound{sig2}\AgdaSpace{}%
\AgdaBound{x}\AgdaSpace{}%
\AgdaBound{x₁}\AgdaSpace{}%
\AgdaSymbol{|}\AgdaSpace{}%
\AgdaInductiveConstructor{true}\AgdaSpace{}%
\AgdaSymbol{|}\AgdaSpace{}%
\AgdaInductiveConstructor{false}\AgdaSpace{}%
\AgdaKeyword{with}%
\>[90]\AgdaSymbol{(}\AgdaFunction{isSigned}%
\>[101]\AgdaBound{msg₂}\AgdaSpace{}%
\AgdaBound{sig2}\AgdaSpace{}%
\AgdaBound{pbk3}\AgdaSymbol{)}\<%
\\
\>[0]\AgdaFunction{lemmaHoareTripleStackGeAux'9}\AgdaSpace{}%
\AgdaBound{msg₂}\AgdaSpace{}%
\AgdaBound{pbk1}\AgdaSpace{}%
\AgdaBound{pbk2}\AgdaSpace{}%
\AgdaBound{pbk3}\AgdaSpace{}%
\AgdaBound{pbk4}\AgdaSpace{}%
\AgdaBound{sig1}\AgdaSpace{}%
\AgdaBound{sig2}\AgdaSpace{}%
\AgdaBound{x}\AgdaSpace{}%
\AgdaBound{x₁}\AgdaSpace{}%
\AgdaSymbol{|}\AgdaSpace{}%
\AgdaInductiveConstructor{true}\AgdaSpace{}%
\AgdaSymbol{|}\AgdaSpace{}%
\AgdaInductiveConstructor{false}\AgdaSpace{}%
\AgdaSymbol{|}\AgdaSpace{}%
\AgdaInductiveConstructor{false}\AgdaSpace{}%
\AgdaKeyword{with}%
\>[98]\AgdaSymbol{(}\AgdaFunction{isSigned}%
\>[109]\AgdaBound{msg₂}\AgdaSpace{}%
\AgdaBound{sig2}\AgdaSpace{}%
\AgdaBound{pbk4}\AgdaSymbol{)}\<%
\\
\>[0]\AgdaFunction{lemmaHoareTripleStackGeAux'9}\AgdaSpace{}%
\AgdaBound{msg₂}\AgdaSpace{}%
\AgdaBound{pbk1}\AgdaSpace{}%
\AgdaBound{pbk2}\AgdaSpace{}%
\AgdaBound{pbk3}\AgdaSpace{}%
\AgdaBound{pbk4}\AgdaSpace{}%
\AgdaBound{sig1}\AgdaSpace{}%
\AgdaBound{sig2}\AgdaSpace{}%
\AgdaBound{x}\AgdaSpace{}%
\AgdaBound{x₁}\AgdaSpace{}%
\AgdaSymbol{|}\AgdaSpace{}%
\AgdaInductiveConstructor{true}\AgdaSpace{}%
\AgdaSymbol{|}\AgdaSpace{}%
\AgdaInductiveConstructor{false}\AgdaSpace{}%
\AgdaSymbol{|}\AgdaSpace{}%
\AgdaInductiveConstructor{false}\AgdaSpace{}%
\AgdaSymbol{|}\AgdaSpace{}%
\AgdaInductiveConstructor{true}\AgdaSpace{}%
\AgdaSymbol{=}\AgdaSpace{}%
\AgdaInductiveConstructor{tt}\<%
\\
\>[0]\AgdaFunction{lemmaHoareTripleStackGeAux'9}\AgdaSpace{}%
\AgdaBound{msg₂}\AgdaSpace{}%
\AgdaBound{pbk1}\AgdaSpace{}%
\AgdaBound{pbk2}\AgdaSpace{}%
\AgdaBound{pbk3}\AgdaSpace{}%
\AgdaBound{pbk4}\AgdaSpace{}%
\AgdaBound{sig1}\AgdaSpace{}%
\AgdaBound{sig2}\AgdaSpace{}%
\AgdaBound{x}\AgdaSpace{}%
\AgdaBound{x₁}\AgdaSpace{}%
\AgdaSymbol{|}\AgdaSpace{}%
\AgdaInductiveConstructor{true}\AgdaSpace{}%
\AgdaSymbol{|}\AgdaSpace{}%
\AgdaInductiveConstructor{false}\AgdaSpace{}%
\AgdaSymbol{|}\AgdaSpace{}%
\AgdaInductiveConstructor{true}\AgdaSpace{}%
\AgdaSymbol{=}\AgdaSpace{}%
\AgdaInductiveConstructor{tt}\<%
\\
\>[0]\AgdaFunction{lemmaHoareTripleStackGeAux'9}\AgdaSpace{}%
\AgdaBound{msg₂}\AgdaSpace{}%
\AgdaBound{pbk1}\AgdaSpace{}%
\AgdaBound{pbk2}\AgdaSpace{}%
\AgdaBound{pbk3}\AgdaSpace{}%
\AgdaBound{pbk4}\AgdaSpace{}%
\AgdaBound{sig1}\AgdaSpace{}%
\AgdaBound{sig2}\AgdaSpace{}%
\AgdaBound{x}\AgdaSpace{}%
\AgdaBound{x₁}\AgdaSpace{}%
\AgdaSymbol{|}\AgdaSpace{}%
\AgdaInductiveConstructor{true}\AgdaSpace{}%
\AgdaSymbol{|}\AgdaSpace{}%
\AgdaInductiveConstructor{true}\AgdaSpace{}%
\AgdaSymbol{=}\AgdaSpace{}%
\AgdaInductiveConstructor{tt}\<%
\\
%
\\[\AgdaEmptyExtraSkip]%
%
\\[\AgdaEmptyExtraSkip]%
%
\\[\AgdaEmptyExtraSkip]%
%
\\[\AgdaEmptyExtraSkip]%
\>[0]\AgdaFunction{lemmaHoareTripleStackGeAux'10}%
\>[1501I]\AgdaSymbol{:}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaBound{msg₂}\AgdaSpace{}%
\AgdaSymbol{:}\AgdaSpace{}%
\AgdaDatatype{Msg}\AgdaSymbol{)}\<%
\\
\>[1501I][@{}l@{\AgdaIndent{0}}]%
\>[31]\AgdaSymbol{(}\AgdaBound{pbk1}\AgdaSpace{}%
\AgdaBound{pbk2}\AgdaSpace{}%
\AgdaBound{pbk3}\AgdaSpace{}%
\AgdaBound{pbk4}\AgdaSpace{}%
\AgdaBound{sig1}\AgdaSpace{}%
\AgdaBound{sig2}\AgdaSpace{}%
\AgdaSymbol{:}\AgdaSpace{}%
\AgdaDatatype{ℕ}\AgdaSymbol{)}\<%
\\
%
\>[31]\AgdaSymbol{→}\AgdaSpace{}%
\AgdaFunction{True}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaFunction{isSigned}%
\>[49]\AgdaBound{msg₂}\AgdaSpace{}%
\AgdaBound{sig1}\AgdaSpace{}%
\AgdaBound{pbk2}\AgdaSymbol{)}\<%
\\
\>[.][@{}l@{}]\<[1501I]%
\>[30]\AgdaSymbol{→}%
\>[33]\AgdaFunction{True}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaFunction{isSigned}%
\>[49]\AgdaBound{msg₂}\AgdaSpace{}%
\AgdaBound{sig2}\AgdaSpace{}%
\AgdaBound{pbk3}\AgdaSymbol{)}\<%
\\
\>[30][@{}l@{\AgdaIndent{0}}]%
\>[31]\AgdaSymbol{→}\AgdaSpace{}%
\AgdaFunction{True}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaFunction{compareSigsMultiSig}\AgdaSpace{}%
\AgdaBound{msg₂}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaSpace{}%
\AgdaBound{sig1}\AgdaSpace{}%
\AgdaOperator{\AgdaInductiveConstructor{∷}}\AgdaSpace{}%
\AgdaBound{sig2}\AgdaSpace{}%
\AgdaOperator{\AgdaInductiveConstructor{∷}}\AgdaSpace{}%
\AgdaInductiveConstructor{[]}\AgdaSymbol{)}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaBound{pbk1}\AgdaSpace{}%
\AgdaOperator{\AgdaInductiveConstructor{∷}}\AgdaSpace{}%
\AgdaBound{pbk2}\AgdaSpace{}%
\AgdaOperator{\AgdaInductiveConstructor{∷}}\AgdaSpace{}%
\AgdaBound{pbk3}\AgdaSpace{}%
\AgdaOperator{\AgdaInductiveConstructor{∷}}\AgdaSpace{}%
\AgdaBound{pbk4}\AgdaSpace{}%
\AgdaOperator{\AgdaInductiveConstructor{∷}}%
\>[114]\AgdaInductiveConstructor{[]}\AgdaSymbol{))}\<%
\\
%
\\[\AgdaEmptyExtraSkip]%
\>[0]\AgdaFunction{lemmaHoareTripleStackGeAux'10}\AgdaSpace{}%
\AgdaBound{msg₂}\AgdaSpace{}%
\AgdaBound{pbk1}\AgdaSpace{}%
\AgdaBound{pbk2}\AgdaSpace{}%
\AgdaBound{pbk3}\AgdaSpace{}%
\AgdaBound{pbk4}\AgdaSpace{}%
\AgdaBound{sig1}\AgdaSpace{}%
\AgdaBound{sig2}\AgdaSpace{}%
\AgdaBound{x}\AgdaSpace{}%
\AgdaBound{x₁}\AgdaSpace{}%
\AgdaKeyword{with}%
\>[76]\AgdaSymbol{(}\AgdaFunction{isSigned}%
\>[87]\AgdaBound{msg₂}\AgdaSpace{}%
\AgdaBound{sig1}\AgdaSpace{}%
\AgdaBound{pbk1}\AgdaSymbol{)}\<%
\\
\>[0]\AgdaFunction{lemmaHoareTripleStackGeAux'10}\AgdaSpace{}%
\AgdaBound{msg₂}\AgdaSpace{}%
\AgdaBound{pbk1}\AgdaSpace{}%
\AgdaBound{pbk2}\AgdaSpace{}%
\AgdaBound{pbk3}\AgdaSpace{}%
\AgdaBound{pbk4}\AgdaSpace{}%
\AgdaBound{sig1}\AgdaSpace{}%
\AgdaBound{sig2}\AgdaSpace{}%
\AgdaBound{x}\AgdaSpace{}%
\AgdaBound{x₁}\AgdaSpace{}%
\AgdaSymbol{|}\AgdaSpace{}%
\AgdaInductiveConstructor{false}\AgdaSpace{}%
\AgdaKeyword{with}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaFunction{isSigned}%
\>[94]\AgdaBound{msg₂}\AgdaSpace{}%
\AgdaBound{sig1}\AgdaSpace{}%
\AgdaBound{pbk2}\AgdaSymbol{)}\<%
\\
\>[0]\AgdaFunction{lemmaHoareTripleStackGeAux'10}\AgdaSpace{}%
\AgdaBound{msg₂}\AgdaSpace{}%
\AgdaBound{pbk1}\AgdaSpace{}%
\AgdaBound{pbk2}\AgdaSpace{}%
\AgdaBound{pbk3}\AgdaSpace{}%
\AgdaBound{pbk4}\AgdaSpace{}%
\AgdaBound{sig1}\AgdaSpace{}%
\AgdaBound{sig2}\AgdaSpace{}%
\AgdaBound{x}\AgdaSpace{}%
\AgdaBound{x₁}\AgdaSpace{}%
\AgdaSymbol{|}\AgdaSpace{}%
\AgdaInductiveConstructor{false}\AgdaSpace{}%
\AgdaSymbol{|}\AgdaSpace{}%
\AgdaInductiveConstructor{true}\AgdaSpace{}%
\AgdaKeyword{with}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaFunction{isSigned}%
\>[101]\AgdaBound{msg₂}\AgdaSpace{}%
\AgdaBound{sig2}\AgdaSpace{}%
\AgdaBound{pbk3}\AgdaSymbol{)}\<%
\\
\>[0]\AgdaFunction{lemmaHoareTripleStackGeAux'10}\AgdaSpace{}%
\AgdaBound{msg₂}\AgdaSpace{}%
\AgdaBound{pbk1}\AgdaSpace{}%
\AgdaBound{pbk2}\AgdaSpace{}%
\AgdaBound{pbk3}\AgdaSpace{}%
\AgdaBound{pbk4}\AgdaSpace{}%
\AgdaBound{sig1}\AgdaSpace{}%
\AgdaBound{sig2}\AgdaSpace{}%
\AgdaBound{x}\AgdaSpace{}%
\AgdaBound{x₁}\AgdaSpace{}%
\AgdaSymbol{|}\AgdaSpace{}%
\AgdaInductiveConstructor{false}\AgdaSpace{}%
\AgdaSymbol{|}\AgdaSpace{}%
\AgdaInductiveConstructor{true}\AgdaSpace{}%
\AgdaSymbol{|}\AgdaSpace{}%
\AgdaInductiveConstructor{true}\AgdaSpace{}%
\AgdaSymbol{=}\AgdaSpace{}%
\AgdaInductiveConstructor{tt}\<%
\\
\>[0]\AgdaFunction{lemmaHoareTripleStackGeAux'10}\AgdaSpace{}%
\AgdaBound{msg₂}\AgdaSpace{}%
\AgdaBound{pbk1}\AgdaSpace{}%
\AgdaBound{pbk2}\AgdaSpace{}%
\AgdaBound{pbk3}\AgdaSpace{}%
\AgdaBound{pbk4}\AgdaSpace{}%
\AgdaBound{sig1}\AgdaSpace{}%
\AgdaBound{sig2}\AgdaSpace{}%
\AgdaBound{x}\AgdaSpace{}%
\AgdaBound{x₁}\AgdaSpace{}%
\AgdaSymbol{|}\AgdaSpace{}%
\AgdaInductiveConstructor{true}\AgdaSpace{}%
\AgdaKeyword{with}%
\>[83]\AgdaSymbol{(}\AgdaFunction{isSigned}%
\>[94]\AgdaBound{msg₂}\AgdaSpace{}%
\AgdaBound{sig2}\AgdaSpace{}%
\AgdaBound{pbk2}\AgdaSymbol{)}\<%
\\
\>[0]\AgdaFunction{lemmaHoareTripleStackGeAux'10}\AgdaSpace{}%
\AgdaBound{msg₂}\AgdaSpace{}%
\AgdaBound{pbk1}\AgdaSpace{}%
\AgdaBound{pbk2}\AgdaSpace{}%
\AgdaBound{pbk3}\AgdaSpace{}%
\AgdaBound{pbk4}\AgdaSpace{}%
\AgdaBound{sig1}\AgdaSpace{}%
\AgdaBound{sig2}\AgdaSpace{}%
\AgdaBound{x}\AgdaSpace{}%
\AgdaBound{x₁}\AgdaSpace{}%
\AgdaSymbol{|}\AgdaSpace{}%
\AgdaInductiveConstructor{true}\AgdaSpace{}%
\AgdaSymbol{|}\AgdaSpace{}%
\AgdaInductiveConstructor{false}\AgdaSpace{}%
\AgdaKeyword{with}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaFunction{isSigned}%
\>[101]\AgdaBound{msg₂}\AgdaSpace{}%
\AgdaBound{sig2}\AgdaSpace{}%
\AgdaBound{pbk3}\AgdaSymbol{)}\<%
\\
\>[0]\AgdaFunction{lemmaHoareTripleStackGeAux'10}\AgdaSpace{}%
\AgdaBound{msg₂}\AgdaSpace{}%
\AgdaBound{pbk1}\AgdaSpace{}%
\AgdaBound{pbk2}\AgdaSpace{}%
\AgdaBound{pbk3}\AgdaSpace{}%
\AgdaBound{pbk4}\AgdaSpace{}%
\AgdaBound{sig1}\AgdaSpace{}%
\AgdaBound{sig2}\AgdaSpace{}%
\AgdaBound{x}\AgdaSpace{}%
\AgdaBound{x₁}\AgdaSpace{}%
\AgdaSymbol{|}\AgdaSpace{}%
\AgdaInductiveConstructor{true}\AgdaSpace{}%
\AgdaSymbol{|}\AgdaSpace{}%
\AgdaInductiveConstructor{false}\AgdaSpace{}%
\AgdaSymbol{|}\AgdaSpace{}%
\AgdaInductiveConstructor{true}\AgdaSpace{}%
\AgdaSymbol{=}\AgdaSpace{}%
\AgdaInductiveConstructor{tt}\<%
\\
\>[0]\AgdaFunction{lemmaHoareTripleStackGeAux'10}\AgdaSpace{}%
\AgdaBound{msg₂}\AgdaSpace{}%
\AgdaBound{pbk1}\AgdaSpace{}%
\AgdaBound{pbk2}\AgdaSpace{}%
\AgdaBound{pbk3}\AgdaSpace{}%
\AgdaBound{pbk4}\AgdaSpace{}%
\AgdaBound{sig1}\AgdaSpace{}%
\AgdaBound{sig2}\AgdaSpace{}%
\AgdaBound{x}\AgdaSpace{}%
\AgdaBound{x₁}\AgdaSpace{}%
\AgdaSymbol{|}\AgdaSpace{}%
\AgdaInductiveConstructor{true}\AgdaSpace{}%
\AgdaSymbol{|}\AgdaSpace{}%
\AgdaInductiveConstructor{true}\AgdaSpace{}%
\AgdaSymbol{=}\AgdaSpace{}%
\AgdaInductiveConstructor{tt}\<%
\\
%
\\[\AgdaEmptyExtraSkip]%
%
\\[\AgdaEmptyExtraSkip]%
\>[0]\AgdaFunction{lemmaHoareTripleStackGeAux'11}%
\>[1660I]\AgdaSymbol{:}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaBound{msg₂}\AgdaSpace{}%
\AgdaSymbol{:}\AgdaSpace{}%
\AgdaDatatype{Msg}\AgdaSymbol{)}\<%
\\
\>[1660I][@{}l@{\AgdaIndent{0}}]%
\>[31]\AgdaSymbol{(}\AgdaBound{pbk1}\AgdaSpace{}%
\AgdaBound{pbk2}\AgdaSpace{}%
\AgdaBound{pbk3}\AgdaSpace{}%
\AgdaBound{pbk4}\AgdaSpace{}%
\AgdaBound{sig1}\AgdaSpace{}%
\AgdaBound{sig2}\AgdaSpace{}%
\AgdaSymbol{:}\AgdaSpace{}%
\AgdaDatatype{ℕ}\AgdaSymbol{)}\<%
\\
%
\>[31]\AgdaSymbol{→}\AgdaSpace{}%
\AgdaFunction{True}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaFunction{isSigned}%
\>[49]\AgdaBound{msg₂}\AgdaSpace{}%
\AgdaBound{sig1}\AgdaSpace{}%
\AgdaBound{pbk2}\AgdaSymbol{)}\<%
\\
\>[.][@{}l@{}]\<[1660I]%
\>[30]\AgdaSymbol{→}%
\>[33]\AgdaFunction{True}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaFunction{isSigned}%
\>[49]\AgdaBound{msg₂}\AgdaSpace{}%
\AgdaBound{sig2}\AgdaSpace{}%
\AgdaBound{pbk4}\AgdaSymbol{)}\<%
\\
\>[30][@{}l@{\AgdaIndent{0}}]%
\>[31]\AgdaSymbol{→}\AgdaSpace{}%
\AgdaFunction{True}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaFunction{compareSigsMultiSig}\AgdaSpace{}%
\AgdaBound{msg₂}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaSpace{}%
\AgdaBound{sig1}\AgdaSpace{}%
\AgdaOperator{\AgdaInductiveConstructor{∷}}\AgdaSpace{}%
\AgdaBound{sig2}\AgdaSpace{}%
\AgdaOperator{\AgdaInductiveConstructor{∷}}\AgdaSpace{}%
\AgdaInductiveConstructor{[]}\AgdaSymbol{)}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaBound{pbk1}\AgdaSpace{}%
\AgdaOperator{\AgdaInductiveConstructor{∷}}\AgdaSpace{}%
\AgdaBound{pbk2}\AgdaSpace{}%
\AgdaOperator{\AgdaInductiveConstructor{∷}}\AgdaSpace{}%
\AgdaBound{pbk3}\AgdaSpace{}%
\AgdaOperator{\AgdaInductiveConstructor{∷}}\AgdaSpace{}%
\AgdaBound{pbk4}\AgdaSpace{}%
\AgdaOperator{\AgdaInductiveConstructor{∷}}%
\>[114]\AgdaInductiveConstructor{[]}\AgdaSymbol{))}\<%
\\
%
\\[\AgdaEmptyExtraSkip]%
\>[0]\AgdaFunction{lemmaHoareTripleStackGeAux'11}\AgdaSpace{}%
\AgdaBound{msg₂}\AgdaSpace{}%
\AgdaBound{pbk1}\AgdaSpace{}%
\AgdaBound{pbk2}\AgdaSpace{}%
\AgdaBound{pbk3}\AgdaSpace{}%
\AgdaBound{pbk4}\AgdaSpace{}%
\AgdaBound{sig1}\AgdaSpace{}%
\AgdaBound{sig2}\AgdaSpace{}%
\AgdaBound{x}\AgdaSpace{}%
\AgdaBound{x₁}\AgdaSpace{}%
\AgdaKeyword{with}%
\>[76]\AgdaSymbol{(}\AgdaFunction{isSigned}%
\>[87]\AgdaBound{msg₂}\AgdaSpace{}%
\AgdaBound{sig1}\AgdaSpace{}%
\AgdaBound{pbk1}\AgdaSymbol{)}\<%
\\
\>[0]\AgdaFunction{lemmaHoareTripleStackGeAux'11}\AgdaSpace{}%
\AgdaBound{msg₂}\AgdaSpace{}%
\AgdaBound{pbk1}\AgdaSpace{}%
\AgdaBound{pbk2}\AgdaSpace{}%
\AgdaBound{pbk3}\AgdaSpace{}%
\AgdaBound{pbk4}\AgdaSpace{}%
\AgdaBound{sig1}\AgdaSpace{}%
\AgdaBound{sig2}\AgdaSpace{}%
\AgdaBound{x}\AgdaSpace{}%
\AgdaBound{x₁}\AgdaSpace{}%
\AgdaSymbol{|}\AgdaSpace{}%
\AgdaInductiveConstructor{false}\AgdaSpace{}%
\AgdaKeyword{with}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaFunction{isSigned}%
\>[94]\AgdaBound{msg₂}\AgdaSpace{}%
\AgdaBound{sig1}\AgdaSpace{}%
\AgdaBound{pbk2}\AgdaSymbol{)}\<%
\\
\>[0]\AgdaFunction{lemmaHoareTripleStackGeAux'11}\AgdaSpace{}%
\AgdaBound{msg₂}\AgdaSpace{}%
\AgdaBound{pbk1}\AgdaSpace{}%
\AgdaBound{pbk2}\AgdaSpace{}%
\AgdaBound{pbk3}\AgdaSpace{}%
\AgdaBound{pbk4}\AgdaSpace{}%
\AgdaBound{sig1}\AgdaSpace{}%
\AgdaBound{sig2}\AgdaSpace{}%
\AgdaBound{x}\AgdaSpace{}%
\AgdaBound{x₁}\AgdaSpace{}%
\AgdaSymbol{|}\AgdaSpace{}%
\AgdaInductiveConstructor{false}\AgdaSpace{}%
\AgdaSymbol{|}\AgdaSpace{}%
\AgdaInductiveConstructor{true}\AgdaSpace{}%
\AgdaKeyword{with}%
\>[92]\AgdaSymbol{(}\AgdaFunction{isSigned}%
\>[103]\AgdaBound{msg₂}\AgdaSpace{}%
\AgdaBound{sig2}\AgdaSpace{}%
\AgdaBound{pbk3}\AgdaSymbol{)}\<%
\\
\>[0]\AgdaFunction{lemmaHoareTripleStackGeAux'11}\AgdaSpace{}%
\AgdaBound{msg₂}\AgdaSpace{}%
\AgdaBound{pbk1}\AgdaSpace{}%
\AgdaBound{pbk2}\AgdaSpace{}%
\AgdaBound{pbk3}\AgdaSpace{}%
\AgdaBound{pbk4}\AgdaSpace{}%
\AgdaBound{sig1}\AgdaSpace{}%
\AgdaBound{sig2}\AgdaSpace{}%
\AgdaBound{x}\AgdaSpace{}%
\AgdaBound{x₁}\AgdaSpace{}%
\AgdaSymbol{|}\AgdaSpace{}%
\AgdaInductiveConstructor{false}\AgdaSpace{}%
\AgdaSymbol{|}\AgdaSpace{}%
\AgdaInductiveConstructor{true}\AgdaSpace{}%
\AgdaSymbol{|}\AgdaSpace{}%
\AgdaInductiveConstructor{false}\AgdaSpace{}%
\AgdaKeyword{with}%
\>[99]\AgdaSymbol{(}\AgdaFunction{isSigned}%
\>[110]\AgdaBound{msg₂}\AgdaSpace{}%
\AgdaBound{sig2}\AgdaSpace{}%
\AgdaBound{pbk4}\AgdaSymbol{)}\<%
\\
\>[0]\AgdaFunction{lemmaHoareTripleStackGeAux'11}\AgdaSpace{}%
\AgdaBound{msg₂}\AgdaSpace{}%
\AgdaBound{pbk1}\AgdaSpace{}%
\AgdaBound{pbk2}\AgdaSpace{}%
\AgdaBound{pbk3}\AgdaSpace{}%
\AgdaBound{pbk4}\AgdaSpace{}%
\AgdaBound{sig1}\AgdaSpace{}%
\AgdaBound{sig2}\AgdaSpace{}%
\AgdaBound{x}\AgdaSpace{}%
\AgdaBound{x₁}\AgdaSpace{}%
\AgdaSymbol{|}\AgdaSpace{}%
\AgdaInductiveConstructor{false}\AgdaSpace{}%
\AgdaSymbol{|}\AgdaSpace{}%
\AgdaInductiveConstructor{true}\AgdaSpace{}%
\AgdaSymbol{|}\AgdaSpace{}%
\AgdaInductiveConstructor{false}\AgdaSpace{}%
\AgdaSymbol{|}\AgdaSpace{}%
\AgdaInductiveConstructor{true}\AgdaSpace{}%
\AgdaSymbol{=}\AgdaSpace{}%
\AgdaInductiveConstructor{tt}\<%
\\
\>[0]\AgdaFunction{lemmaHoareTripleStackGeAux'11}\AgdaSpace{}%
\AgdaBound{msg₂}\AgdaSpace{}%
\AgdaBound{pbk1}\AgdaSpace{}%
\AgdaBound{pbk2}\AgdaSpace{}%
\AgdaBound{pbk3}\AgdaSpace{}%
\AgdaBound{pbk4}\AgdaSpace{}%
\AgdaBound{sig1}\AgdaSpace{}%
\AgdaBound{sig2}\AgdaSpace{}%
\AgdaBound{x}\AgdaSpace{}%
\AgdaBound{x₁}\AgdaSpace{}%
\AgdaSymbol{|}\AgdaSpace{}%
\AgdaInductiveConstructor{false}\AgdaSpace{}%
\AgdaSymbol{|}\AgdaSpace{}%
\AgdaInductiveConstructor{true}\AgdaSpace{}%
\AgdaSymbol{|}\AgdaSpace{}%
\AgdaInductiveConstructor{true}\AgdaSpace{}%
\AgdaSymbol{=}\AgdaSpace{}%
\AgdaInductiveConstructor{tt}\<%
\\
\>[0]\AgdaFunction{lemmaHoareTripleStackGeAux'11}\AgdaSpace{}%
\AgdaBound{msg₂}\AgdaSpace{}%
\AgdaBound{pbk1}\AgdaSpace{}%
\AgdaBound{pbk2}\AgdaSpace{}%
\AgdaBound{pbk3}\AgdaSpace{}%
\AgdaBound{pbk4}\AgdaSpace{}%
\AgdaBound{sig1}\AgdaSpace{}%
\AgdaBound{sig2}\AgdaSpace{}%
\AgdaBound{x}\AgdaSpace{}%
\AgdaBound{x₁}\AgdaSpace{}%
\AgdaSymbol{|}\AgdaSpace{}%
\AgdaInductiveConstructor{true}\AgdaSpace{}%
\AgdaKeyword{with}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaFunction{isSigned}%
\>[93]\AgdaBound{msg₂}\AgdaSpace{}%
\AgdaBound{sig2}\AgdaSpace{}%
\AgdaBound{pbk2}\AgdaSymbol{)}\<%
\\
\>[0]\AgdaFunction{lemmaHoareTripleStackGeAux'11}\AgdaSpace{}%
\AgdaBound{msg₂}\AgdaSpace{}%
\AgdaBound{pbk1}\AgdaSpace{}%
\AgdaBound{pbk2}\AgdaSpace{}%
\AgdaBound{pbk3}\AgdaSpace{}%
\AgdaBound{pbk4}\AgdaSpace{}%
\AgdaBound{sig1}\AgdaSpace{}%
\AgdaBound{sig2}\AgdaSpace{}%
\AgdaBound{x}\AgdaSpace{}%
\AgdaBound{x₁}\AgdaSpace{}%
\AgdaSymbol{|}\AgdaSpace{}%
\AgdaInductiveConstructor{true}\AgdaSpace{}%
\AgdaSymbol{|}\AgdaSpace{}%
\AgdaInductiveConstructor{false}\AgdaSpace{}%
\AgdaKeyword{with}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaFunction{isSigned}%
\>[101]\AgdaBound{msg₂}\AgdaSpace{}%
\AgdaBound{sig2}\AgdaSpace{}%
\AgdaBound{pbk3}\AgdaSymbol{)}\<%
\\
\>[0]\AgdaFunction{lemmaHoareTripleStackGeAux'11}\AgdaSpace{}%
\AgdaBound{msg₂}\AgdaSpace{}%
\AgdaBound{pbk1}\AgdaSpace{}%
\AgdaBound{pbk2}\AgdaSpace{}%
\AgdaBound{pbk3}\AgdaSpace{}%
\AgdaBound{pbk4}\AgdaSpace{}%
\AgdaBound{sig1}\AgdaSpace{}%
\AgdaBound{sig2}\AgdaSpace{}%
\AgdaBound{x}\AgdaSpace{}%
\AgdaBound{x₁}\AgdaSpace{}%
\AgdaSymbol{|}\AgdaSpace{}%
\AgdaInductiveConstructor{true}\AgdaSpace{}%
\AgdaSymbol{|}\AgdaSpace{}%
\AgdaInductiveConstructor{false}\AgdaSpace{}%
\AgdaSymbol{|}\AgdaSpace{}%
\AgdaInductiveConstructor{false}\AgdaSpace{}%
\AgdaKeyword{with}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaFunction{isSigned}%
\>[109]\AgdaBound{msg₂}\AgdaSpace{}%
\AgdaBound{sig2}\AgdaSpace{}%
\AgdaBound{pbk4}\AgdaSymbol{)}\<%
\\
\>[0]\AgdaFunction{lemmaHoareTripleStackGeAux'11}\AgdaSpace{}%
\AgdaBound{msg₂}\AgdaSpace{}%
\AgdaBound{pbk1}\AgdaSpace{}%
\AgdaBound{pbk2}\AgdaSpace{}%
\AgdaBound{pbk3}\AgdaSpace{}%
\AgdaBound{pbk4}\AgdaSpace{}%
\AgdaBound{sig1}\AgdaSpace{}%
\AgdaBound{sig2}\AgdaSpace{}%
\AgdaBound{x}\AgdaSpace{}%
\AgdaBound{x₁}\AgdaSpace{}%
\AgdaSymbol{|}\AgdaSpace{}%
\AgdaInductiveConstructor{true}\AgdaSpace{}%
\AgdaSymbol{|}\AgdaSpace{}%
\AgdaInductiveConstructor{false}\AgdaSpace{}%
\AgdaSymbol{|}\AgdaSpace{}%
\AgdaInductiveConstructor{false}\AgdaSpace{}%
\AgdaSymbol{|}\AgdaSpace{}%
\AgdaInductiveConstructor{true}\AgdaSpace{}%
\AgdaSymbol{=}\AgdaSpace{}%
\AgdaInductiveConstructor{tt}\<%
\\
\>[0]\AgdaFunction{lemmaHoareTripleStackGeAux'11}\AgdaSpace{}%
\AgdaBound{msg₂}\AgdaSpace{}%
\AgdaBound{pbk1}\AgdaSpace{}%
\AgdaBound{pbk2}\AgdaSpace{}%
\AgdaBound{pbk3}\AgdaSpace{}%
\AgdaBound{pbk4}\AgdaSpace{}%
\AgdaBound{sig1}\AgdaSpace{}%
\AgdaBound{sig2}\AgdaSpace{}%
\AgdaBound{x}\AgdaSpace{}%
\AgdaBound{x₁}\AgdaSpace{}%
\AgdaSymbol{|}\AgdaSpace{}%
\AgdaInductiveConstructor{true}\AgdaSpace{}%
\AgdaSymbol{|}\AgdaSpace{}%
\AgdaInductiveConstructor{false}\AgdaSpace{}%
\AgdaSymbol{|}\AgdaSpace{}%
\AgdaInductiveConstructor{true}\AgdaSpace{}%
\AgdaSymbol{=}\AgdaSpace{}%
\AgdaInductiveConstructor{tt}\<%
\\
\>[0]\AgdaFunction{lemmaHoareTripleStackGeAux'11}\AgdaSpace{}%
\AgdaBound{msg₂}\AgdaSpace{}%
\AgdaBound{pbk1}\AgdaSpace{}%
\AgdaBound{pbk2}\AgdaSpace{}%
\AgdaBound{pbk3}\AgdaSpace{}%
\AgdaBound{pbk4}\AgdaSpace{}%
\AgdaBound{sig1}\AgdaSpace{}%
\AgdaBound{sig2}\AgdaSpace{}%
\AgdaBound{x}\AgdaSpace{}%
\AgdaBound{x₁}\AgdaSpace{}%
\AgdaSymbol{|}\AgdaSpace{}%
\AgdaInductiveConstructor{true}\AgdaSpace{}%
\AgdaSymbol{|}\AgdaSpace{}%
\AgdaInductiveConstructor{true}\AgdaSpace{}%
\AgdaSymbol{=}\AgdaSpace{}%
\AgdaInductiveConstructor{tt}\<%
\\
%
\\[\AgdaEmptyExtraSkip]%
\>[0]\AgdaFunction{lemmaHoareTripleStackGeAux'12}%
\>[1894I]\AgdaSymbol{:}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaBound{msg₂}\AgdaSpace{}%
\AgdaSymbol{:}\AgdaSpace{}%
\AgdaDatatype{Msg}\AgdaSymbol{)}\<%
\\
\>[1894I][@{}l@{\AgdaIndent{0}}]%
\>[31]\AgdaSymbol{(}\AgdaBound{pbk1}\AgdaSpace{}%
\AgdaBound{pbk2}\AgdaSpace{}%
\AgdaBound{pbk3}\AgdaSpace{}%
\AgdaBound{pbk4}\AgdaSpace{}%
\AgdaBound{sig1}\AgdaSpace{}%
\AgdaBound{sig2}\AgdaSpace{}%
\AgdaSymbol{:}\AgdaSpace{}%
\AgdaDatatype{ℕ}\AgdaSymbol{)}\<%
\\
%
\>[31]\AgdaSymbol{→}\AgdaSpace{}%
\AgdaFunction{True}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaFunction{isSigned}%
\>[49]\AgdaBound{msg₂}\AgdaSpace{}%
\AgdaBound{sig1}\AgdaSpace{}%
\AgdaBound{pbk3}\AgdaSymbol{)}\<%
\\
\>[.][@{}l@{}]\<[1894I]%
\>[30]\AgdaSymbol{→}%
\>[33]\AgdaFunction{True}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaFunction{isSigned}%
\>[49]\AgdaBound{msg₂}\AgdaSpace{}%
\AgdaBound{sig2}\AgdaSpace{}%
\AgdaBound{pbk4}\AgdaSymbol{)}\<%
\\
\>[30][@{}l@{\AgdaIndent{0}}]%
\>[31]\AgdaSymbol{→}\AgdaSpace{}%
\AgdaFunction{True}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaFunction{compareSigsMultiSig}\AgdaSpace{}%
\AgdaBound{msg₂}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaSpace{}%
\AgdaBound{sig1}\AgdaSpace{}%
\AgdaOperator{\AgdaInductiveConstructor{∷}}\AgdaSpace{}%
\AgdaBound{sig2}\AgdaSpace{}%
\AgdaOperator{\AgdaInductiveConstructor{∷}}\AgdaSpace{}%
\AgdaInductiveConstructor{[]}\AgdaSymbol{)}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaBound{pbk1}\AgdaSpace{}%
\AgdaOperator{\AgdaInductiveConstructor{∷}}\AgdaSpace{}%
\AgdaBound{pbk2}\AgdaSpace{}%
\AgdaOperator{\AgdaInductiveConstructor{∷}}\AgdaSpace{}%
\AgdaBound{pbk3}\AgdaSpace{}%
\AgdaOperator{\AgdaInductiveConstructor{∷}}\AgdaSpace{}%
\AgdaBound{pbk4}\AgdaSpace{}%
\AgdaOperator{\AgdaInductiveConstructor{∷}}%
\>[114]\AgdaInductiveConstructor{[]}\AgdaSymbol{))}\<%
\\
%
\\[\AgdaEmptyExtraSkip]%
\>[0]\AgdaFunction{lemmaHoareTripleStackGeAux'12}\AgdaSpace{}%
\AgdaBound{msg₂}\AgdaSpace{}%
\AgdaBound{pbk1}\AgdaSpace{}%
\AgdaBound{pbk2}\AgdaSpace{}%
\AgdaBound{pbk3}\AgdaSpace{}%
\AgdaBound{pbk4}\AgdaSpace{}%
\AgdaBound{sig1}\AgdaSpace{}%
\AgdaBound{sig2}\AgdaSpace{}%
\AgdaBound{x}\AgdaSpace{}%
\AgdaBound{x₁}\AgdaSpace{}%
\AgdaKeyword{with}%
\>[76]\AgdaSymbol{(}\AgdaFunction{isSigned}%
\>[87]\AgdaBound{msg₂}\AgdaSpace{}%
\AgdaBound{sig1}\AgdaSpace{}%
\AgdaBound{pbk1}\AgdaSymbol{)}\<%
\\
\>[0]\AgdaFunction{lemmaHoareTripleStackGeAux'12}\AgdaSpace{}%
\AgdaBound{msg₂}\AgdaSpace{}%
\AgdaBound{pbk1}\AgdaSpace{}%
\AgdaBound{pbk2}\AgdaSpace{}%
\AgdaBound{pbk3}\AgdaSpace{}%
\AgdaBound{pbk4}\AgdaSpace{}%
\AgdaBound{sig1}\AgdaSpace{}%
\AgdaBound{sig2}\AgdaSpace{}%
\AgdaBound{x}\AgdaSpace{}%
\AgdaBound{x₁}\AgdaSpace{}%
\AgdaSymbol{|}\AgdaSpace{}%
\AgdaInductiveConstructor{false}\AgdaSpace{}%
\AgdaKeyword{with}%
\>[84]\AgdaSymbol{(}\AgdaFunction{isSigned}%
\>[95]\AgdaBound{msg₂}\AgdaSpace{}%
\AgdaBound{sig1}\AgdaSpace{}%
\AgdaBound{pbk2}\AgdaSymbol{)}\<%
\\
\>[0]\AgdaFunction{lemmaHoareTripleStackGeAux'12}\AgdaSpace{}%
\AgdaBound{msg₂}\AgdaSpace{}%
\AgdaBound{pbk1}\AgdaSpace{}%
\AgdaBound{pbk2}\AgdaSpace{}%
\AgdaBound{pbk3}\AgdaSpace{}%
\AgdaBound{pbk4}\AgdaSpace{}%
\AgdaBound{sig1}\AgdaSpace{}%
\AgdaBound{sig2}\AgdaSpace{}%
\AgdaBound{x}\AgdaSpace{}%
\AgdaBound{x₁}\AgdaSpace{}%
\AgdaSymbol{|}\AgdaSpace{}%
\AgdaInductiveConstructor{false}\AgdaSpace{}%
\AgdaSymbol{|}\AgdaSpace{}%
\AgdaInductiveConstructor{false}\AgdaSpace{}%
\AgdaKeyword{with}%
\>[92]\AgdaSymbol{(}\AgdaFunction{isSigned}%
\>[103]\AgdaBound{msg₂}\AgdaSpace{}%
\AgdaBound{sig1}\AgdaSpace{}%
\AgdaBound{pbk3}\AgdaSymbol{)}\<%
\\
\>[0]\AgdaFunction{lemmaHoareTripleStackGeAux'12}\AgdaSpace{}%
\AgdaBound{msg₂}\AgdaSpace{}%
\AgdaBound{pbk1}\AgdaSpace{}%
\AgdaBound{pbk2}\AgdaSpace{}%
\AgdaBound{pbk3}\AgdaSpace{}%
\AgdaBound{pbk4}\AgdaSpace{}%
\AgdaBound{sig1}\AgdaSpace{}%
\AgdaBound{sig2}\AgdaSpace{}%
\AgdaBound{x}\AgdaSpace{}%
\AgdaBound{x₁}\AgdaSpace{}%
\AgdaSymbol{|}\AgdaSpace{}%
\AgdaInductiveConstructor{false}\AgdaSpace{}%
\AgdaSymbol{|}\AgdaSpace{}%
\AgdaInductiveConstructor{false}\AgdaSpace{}%
\AgdaSymbol{|}\AgdaSpace{}%
\AgdaInductiveConstructor{true}\AgdaSpace{}%
\AgdaKeyword{with}%
\>[99]\AgdaSymbol{(}\AgdaFunction{isSigned}%
\>[110]\AgdaBound{msg₂}\AgdaSpace{}%
\AgdaBound{sig2}\AgdaSpace{}%
\AgdaBound{pbk4}\AgdaSymbol{)}\<%
\\
\>[0]\AgdaFunction{lemmaHoareTripleStackGeAux'12}\AgdaSpace{}%
\AgdaBound{msg₂}\AgdaSpace{}%
\AgdaBound{pbk1}\AgdaSpace{}%
\AgdaBound{pbk2}\AgdaSpace{}%
\AgdaBound{pbk3}\AgdaSpace{}%
\AgdaBound{pbk4}\AgdaSpace{}%
\AgdaBound{sig1}\AgdaSpace{}%
\AgdaBound{sig2}\AgdaSpace{}%
\AgdaBound{x}\AgdaSpace{}%
\AgdaBound{x₁}\AgdaSpace{}%
\AgdaSymbol{|}\AgdaSpace{}%
\AgdaInductiveConstructor{false}\AgdaSpace{}%
\AgdaSymbol{|}\AgdaSpace{}%
\AgdaInductiveConstructor{false}\AgdaSpace{}%
\AgdaSymbol{|}\AgdaSpace{}%
\AgdaInductiveConstructor{true}\AgdaSpace{}%
\AgdaSymbol{|}\AgdaSpace{}%
\AgdaInductiveConstructor{true}\AgdaSpace{}%
\AgdaSymbol{=}\AgdaSpace{}%
\AgdaInductiveConstructor{tt}\<%
\\
\>[0]\AgdaFunction{lemmaHoareTripleStackGeAux'12}\AgdaSpace{}%
\AgdaBound{msg₂}\AgdaSpace{}%
\AgdaBound{pbk1}\AgdaSpace{}%
\AgdaBound{pbk2}\AgdaSpace{}%
\AgdaBound{pbk3}\AgdaSpace{}%
\AgdaBound{pbk4}\AgdaSpace{}%
\AgdaBound{sig1}\AgdaSpace{}%
\AgdaBound{sig2}\AgdaSpace{}%
\AgdaBound{x}\AgdaSpace{}%
\AgdaBound{x₁}\AgdaSpace{}%
\AgdaSymbol{|}\AgdaSpace{}%
\AgdaInductiveConstructor{false}\AgdaSpace{}%
\AgdaSymbol{|}\AgdaSpace{}%
\AgdaInductiveConstructor{true}\AgdaSpace{}%
\AgdaKeyword{with}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaFunction{isSigned}%
\>[101]\AgdaBound{msg₂}\AgdaSpace{}%
\AgdaBound{sig2}\AgdaSpace{}%
\AgdaBound{pbk3}\AgdaSymbol{)}\<%
\\
\>[0]\AgdaFunction{lemmaHoareTripleStackGeAux'12}\AgdaSpace{}%
\AgdaBound{msg₂}\AgdaSpace{}%
\AgdaBound{pbk1}\AgdaSpace{}%
\AgdaBound{pbk2}\AgdaSpace{}%
\AgdaBound{pbk3}\AgdaSpace{}%
\AgdaBound{pbk4}\AgdaSpace{}%
\AgdaBound{sig1}\AgdaSpace{}%
\AgdaBound{sig2}\AgdaSpace{}%
\AgdaBound{x}\AgdaSpace{}%
\AgdaBound{x₁}\AgdaSpace{}%
\AgdaSymbol{|}\AgdaSpace{}%
\AgdaInductiveConstructor{false}\AgdaSpace{}%
\AgdaSymbol{|}\AgdaSpace{}%
\AgdaInductiveConstructor{true}\AgdaSpace{}%
\AgdaSymbol{|}\AgdaSpace{}%
\AgdaInductiveConstructor{false}\AgdaSpace{}%
\AgdaKeyword{with}%
\>[99]\AgdaSymbol{(}\AgdaFunction{isSigned}%
\>[110]\AgdaBound{msg₂}\AgdaSpace{}%
\AgdaBound{sig2}\AgdaSpace{}%
\AgdaBound{pbk4}\AgdaSymbol{)}\<%
\\
\>[0]\AgdaFunction{lemmaHoareTripleStackGeAux'12}\AgdaSpace{}%
\AgdaBound{msg₂}\AgdaSpace{}%
\AgdaBound{pbk1}\AgdaSpace{}%
\AgdaBound{pbk2}\AgdaSpace{}%
\AgdaBound{pbk3}\AgdaSpace{}%
\AgdaBound{pbk4}\AgdaSpace{}%
\AgdaBound{sig1}\AgdaSpace{}%
\AgdaBound{sig2}\AgdaSpace{}%
\AgdaBound{x}\AgdaSpace{}%
\AgdaBound{x₁}\AgdaSpace{}%
\AgdaSymbol{|}\AgdaSpace{}%
\AgdaInductiveConstructor{false}\AgdaSpace{}%
\AgdaSymbol{|}\AgdaSpace{}%
\AgdaInductiveConstructor{true}\AgdaSpace{}%
\AgdaSymbol{|}\AgdaSpace{}%
\AgdaInductiveConstructor{false}\AgdaSpace{}%
\AgdaSymbol{|}\AgdaSpace{}%
\AgdaInductiveConstructor{true}\AgdaSpace{}%
\AgdaSymbol{=}\AgdaSpace{}%
\AgdaInductiveConstructor{tt}\<%
\\
\>[0]\AgdaFunction{lemmaHoareTripleStackGeAux'12}\AgdaSpace{}%
\AgdaBound{msg₂}\AgdaSpace{}%
\AgdaBound{pbk1}\AgdaSpace{}%
\AgdaBound{pbk2}\AgdaSpace{}%
\AgdaBound{pbk3}\AgdaSpace{}%
\AgdaBound{pbk4}\AgdaSpace{}%
\AgdaBound{sig1}\AgdaSpace{}%
\AgdaBound{sig2}\AgdaSpace{}%
\AgdaBound{x}\AgdaSpace{}%
\AgdaBound{x₁}\AgdaSpace{}%
\AgdaSymbol{|}\AgdaSpace{}%
\AgdaInductiveConstructor{false}\AgdaSpace{}%
\AgdaSymbol{|}\AgdaSpace{}%
\AgdaInductiveConstructor{true}\AgdaSpace{}%
\AgdaSymbol{|}\AgdaSpace{}%
\AgdaInductiveConstructor{true}\AgdaSpace{}%
\AgdaSymbol{=}\AgdaSpace{}%
\AgdaInductiveConstructor{tt}\<%
\\
\>[0]\AgdaFunction{lemmaHoareTripleStackGeAux'12}\AgdaSpace{}%
\AgdaBound{msg₂}\AgdaSpace{}%
\AgdaBound{pbk1}\AgdaSpace{}%
\AgdaBound{pbk2}\AgdaSpace{}%
\AgdaBound{pbk3}\AgdaSpace{}%
\AgdaBound{pbk4}\AgdaSpace{}%
\AgdaBound{sig1}\AgdaSpace{}%
\AgdaBound{sig2}\AgdaSpace{}%
\AgdaBound{x}\AgdaSpace{}%
\AgdaBound{x₁}\AgdaSpace{}%
\AgdaSymbol{|}\AgdaSpace{}%
\AgdaInductiveConstructor{true}\AgdaSpace{}%
\AgdaKeyword{with}%
\>[83]\AgdaSymbol{(}\AgdaFunction{isSigned}%
\>[94]\AgdaBound{msg₂}\AgdaSpace{}%
\AgdaBound{sig2}\AgdaSpace{}%
\AgdaBound{pbk2}\AgdaSymbol{)}\<%
\\
\>[0]\AgdaFunction{lemmaHoareTripleStackGeAux'12}\AgdaSpace{}%
\AgdaBound{msg₂}\AgdaSpace{}%
\AgdaBound{pbk1}\AgdaSpace{}%
\AgdaBound{pbk2}\AgdaSpace{}%
\AgdaBound{pbk3}\AgdaSpace{}%
\AgdaBound{pbk4}\AgdaSpace{}%
\AgdaBound{sig1}\AgdaSpace{}%
\AgdaBound{sig2}\AgdaSpace{}%
\AgdaBound{x}\AgdaSpace{}%
\AgdaBound{x₁}\AgdaSpace{}%
\AgdaSymbol{|}\AgdaSpace{}%
\AgdaInductiveConstructor{true}\AgdaSpace{}%
\AgdaSymbol{|}\AgdaSpace{}%
\AgdaInductiveConstructor{false}\AgdaSpace{}%
\AgdaKeyword{with}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaFunction{isSigned}%
\>[101]\AgdaBound{msg₂}\AgdaSpace{}%
\AgdaBound{sig2}\AgdaSpace{}%
\AgdaBound{pbk3}\AgdaSymbol{)}\<%
\\
\>[0]\AgdaFunction{lemmaHoareTripleStackGeAux'12}\AgdaSpace{}%
\AgdaBound{msg₂}\AgdaSpace{}%
\AgdaBound{pbk1}\AgdaSpace{}%
\AgdaBound{pbk2}\AgdaSpace{}%
\AgdaBound{pbk3}\AgdaSpace{}%
\AgdaBound{pbk4}\AgdaSpace{}%
\AgdaBound{sig1}\AgdaSpace{}%
\AgdaBound{sig2}\AgdaSpace{}%
\AgdaBound{x}\AgdaSpace{}%
\AgdaBound{x₁}\AgdaSpace{}%
\AgdaSymbol{|}\AgdaSpace{}%
\AgdaInductiveConstructor{true}\AgdaSpace{}%
\AgdaSymbol{|}\AgdaSpace{}%
\AgdaInductiveConstructor{false}\AgdaSpace{}%
\AgdaSymbol{|}\AgdaSpace{}%
\AgdaInductiveConstructor{false}\AgdaSpace{}%
\AgdaKeyword{with}%
\>[99]\AgdaSymbol{(}\AgdaFunction{isSigned}%
\>[110]\AgdaBound{msg₂}\AgdaSpace{}%
\AgdaBound{sig2}\AgdaSpace{}%
\AgdaBound{pbk4}\AgdaSymbol{)}\<%
\\
\>[0]\AgdaFunction{lemmaHoareTripleStackGeAux'12}\AgdaSpace{}%
\AgdaBound{msg₂}\AgdaSpace{}%
\AgdaBound{pbk1}\AgdaSpace{}%
\AgdaBound{pbk2}\AgdaSpace{}%
\AgdaBound{pbk3}\AgdaSpace{}%
\AgdaBound{pbk4}\AgdaSpace{}%
\AgdaBound{sig1}\AgdaSpace{}%
\AgdaBound{sig2}\AgdaSpace{}%
\AgdaBound{x}\AgdaSpace{}%
\AgdaBound{x₁}\AgdaSpace{}%
\AgdaSymbol{|}\AgdaSpace{}%
\AgdaInductiveConstructor{true}\AgdaSpace{}%
\AgdaSymbol{|}\AgdaSpace{}%
\AgdaInductiveConstructor{false}\AgdaSpace{}%
\AgdaSymbol{|}\AgdaSpace{}%
\AgdaInductiveConstructor{false}\AgdaSpace{}%
\AgdaSymbol{|}\AgdaSpace{}%
\AgdaInductiveConstructor{true}\AgdaSpace{}%
\AgdaSymbol{=}\AgdaSpace{}%
\AgdaInductiveConstructor{tt}\<%
\\
\>[0]\AgdaFunction{lemmaHoareTripleStackGeAux'12}\AgdaSpace{}%
\AgdaBound{msg₂}\AgdaSpace{}%
\AgdaBound{pbk1}\AgdaSpace{}%
\AgdaBound{pbk2}\AgdaSpace{}%
\AgdaBound{pbk3}\AgdaSpace{}%
\AgdaBound{pbk4}\AgdaSpace{}%
\AgdaBound{sig1}\AgdaSpace{}%
\AgdaBound{sig2}\AgdaSpace{}%
\AgdaBound{x}\AgdaSpace{}%
\AgdaBound{x₁}\AgdaSpace{}%
\AgdaSymbol{|}\AgdaSpace{}%
\AgdaInductiveConstructor{true}\AgdaSpace{}%
\AgdaSymbol{|}\AgdaSpace{}%
\AgdaInductiveConstructor{false}\AgdaSpace{}%
\AgdaSymbol{|}\AgdaSpace{}%
\AgdaInductiveConstructor{true}\AgdaSpace{}%
\AgdaSymbol{=}\AgdaSpace{}%
\AgdaInductiveConstructor{tt}\<%
\\
\>[0]\AgdaFunction{lemmaHoareTripleStackGeAux'12}\AgdaSpace{}%
\AgdaBound{msg₂}\AgdaSpace{}%
\AgdaBound{pbk1}\AgdaSpace{}%
\AgdaBound{pbk2}\AgdaSpace{}%
\AgdaBound{pbk3}\AgdaSpace{}%
\AgdaBound{pbk4}\AgdaSpace{}%
\AgdaBound{sig1}\AgdaSpace{}%
\AgdaBound{sig2}\AgdaSpace{}%
\AgdaBound{x}\AgdaSpace{}%
\AgdaBound{x₁}\AgdaSpace{}%
\AgdaSymbol{|}\AgdaSpace{}%
\AgdaInductiveConstructor{true}\AgdaSpace{}%
\AgdaSymbol{|}\AgdaSpace{}%
\AgdaInductiveConstructor{true}\AgdaSpace{}%
\AgdaSymbol{=}\AgdaSpace{}%
\AgdaInductiveConstructor{tt}\<%
\\
%
\\[\AgdaEmptyExtraSkip]%
\>[0]\AgdaFunction{lemmaHoareTripleStackGeAux'Comb2-4}\AgdaSpace{}%
\AgdaSymbol{:}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaBound{msg₂}\AgdaSpace{}%
\AgdaSymbol{:}\AgdaSpace{}%
\AgdaDatatype{Msg}\AgdaSymbol{)}\<%
\\
\>[0][@{}l@{\AgdaIndent{0}}]%
\>[9]\AgdaSymbol{(}\AgdaBound{pbk1}\AgdaSpace{}%
\AgdaBound{pbk2}\AgdaSpace{}%
\AgdaBound{pbk3}\AgdaSpace{}%
\AgdaBound{pbk4}\AgdaSpace{}%
\AgdaBound{sig1}\AgdaSpace{}%
\AgdaBound{sig2}\AgdaSpace{}%
\AgdaSymbol{:}\AgdaSpace{}%
\AgdaDatatype{ℕ}\AgdaSymbol{)}\<%
\\
\>[9][@{}l@{\AgdaIndent{0}}]%
\>[10]\AgdaSymbol{→}\AgdaSpace{}%
\AgdaFunction{True}%
\>[2191I]\AgdaSymbol{(}\AgdaFunction{compareSigsMultiSigAux}\AgdaSpace{}%
\AgdaBound{msg₂}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaBound{sig2}\AgdaSpace{}%
\AgdaOperator{\AgdaInductiveConstructor{∷}}\AgdaSpace{}%
\AgdaInductiveConstructor{[]}\AgdaSymbol{)}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaBound{pbk2}\AgdaSpace{}%
\AgdaOperator{\AgdaInductiveConstructor{∷}}\AgdaSpace{}%
\AgdaBound{pbk3}\AgdaSpace{}%
\AgdaOperator{\AgdaInductiveConstructor{∷}}%
\>[74]\AgdaBound{pbk4}\AgdaSpace{}%
\AgdaOperator{\AgdaInductiveConstructor{∷}}\AgdaSpace{}%
\AgdaInductiveConstructor{[]}\AgdaSymbol{)}%
\>[86]\AgdaBound{sig1}\<%
\\
\>[.][@{}l@{}]\<[2191I]%
\>[17]\AgdaSymbol{(}\AgdaFunction{isSigned}%
\>[28]\AgdaBound{msg₂}\AgdaSpace{}%
\AgdaBound{sig1}\AgdaSpace{}%
\AgdaBound{pbk1}\AgdaSpace{}%
\AgdaSymbol{))}\<%
\\
%
\>[10]\AgdaSymbol{→}%
\>[13]\AgdaSymbol{(}\AgdaFunction{True}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaFunction{isSigned}%
\>[30]\AgdaBound{msg₂}\AgdaSpace{}%
\AgdaBound{sig1}\AgdaSpace{}%
\AgdaBound{pbk1}\AgdaSymbol{)}\AgdaSpace{}%
\AgdaOperator{\AgdaRecord{∧}}\AgdaSpace{}%
\AgdaFunction{True}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaFunction{isSigned}%
\>[64]\AgdaBound{msg₂}\AgdaSpace{}%
\AgdaBound{sig2}\AgdaSpace{}%
\AgdaBound{pbk2}\AgdaSymbol{))}\AgdaSpace{}%
\AgdaOperator{\AgdaDatatype{⊎}}\<%
\\
%
\>[13]\AgdaSymbol{(}\AgdaFunction{True}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaFunction{isSigned}%
\>[30]\AgdaBound{msg₂}\AgdaSpace{}%
\AgdaBound{sig1}\AgdaSpace{}%
\AgdaBound{pbk1}\AgdaSymbol{)}\AgdaSpace{}%
\AgdaOperator{\AgdaRecord{∧}}\AgdaSpace{}%
\AgdaFunction{True}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaFunction{isSigned}%
\>[64]\AgdaBound{msg₂}\AgdaSpace{}%
\AgdaBound{sig2}\AgdaSpace{}%
\AgdaBound{pbk3}\AgdaSymbol{))}\AgdaSpace{}%
\AgdaOperator{\AgdaDatatype{⊎}}\<%
\\
%
\>[13]\AgdaSymbol{(}\AgdaFunction{True}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaFunction{isSigned}%
\>[30]\AgdaBound{msg₂}\AgdaSpace{}%
\AgdaBound{sig1}\AgdaSpace{}%
\AgdaBound{pbk1}\AgdaSymbol{)}\AgdaSpace{}%
\AgdaOperator{\AgdaRecord{∧}}\AgdaSpace{}%
\AgdaFunction{True}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaFunction{isSigned}%
\>[64]\AgdaBound{msg₂}\AgdaSpace{}%
\AgdaBound{sig2}\AgdaSpace{}%
\AgdaBound{pbk4}\AgdaSymbol{))}\AgdaSpace{}%
\AgdaOperator{\AgdaDatatype{⊎}}\<%
\\
%
\>[13]\AgdaSymbol{(}\AgdaFunction{True}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaFunction{isSigned}%
\>[30]\AgdaBound{msg₂}\AgdaSpace{}%
\AgdaBound{sig1}\AgdaSpace{}%
\AgdaBound{pbk2}\AgdaSymbol{)}\AgdaSpace{}%
\AgdaOperator{\AgdaRecord{∧}}\AgdaSpace{}%
\AgdaFunction{True}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaFunction{isSigned}%
\>[64]\AgdaBound{msg₂}\AgdaSpace{}%
\AgdaBound{sig2}\AgdaSpace{}%
\AgdaBound{pbk3}\AgdaSymbol{))}\AgdaSpace{}%
\AgdaOperator{\AgdaDatatype{⊎}}\<%
\\
%
\>[13]\AgdaSymbol{(}\AgdaFunction{True}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaFunction{isSigned}%
\>[30]\AgdaBound{msg₂}\AgdaSpace{}%
\AgdaBound{sig1}\AgdaSpace{}%
\AgdaBound{pbk2}\AgdaSymbol{)}\AgdaSpace{}%
\AgdaOperator{\AgdaRecord{∧}}\AgdaSpace{}%
\AgdaFunction{True}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaFunction{isSigned}%
\>[64]\AgdaBound{msg₂}\AgdaSpace{}%
\AgdaBound{sig2}\AgdaSpace{}%
\AgdaBound{pbk4}\AgdaSymbol{))}\AgdaSpace{}%
\AgdaOperator{\AgdaDatatype{⊎}}\<%
\\
%
\>[13]\AgdaSymbol{(}\AgdaFunction{True}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaFunction{isSigned}%
\>[30]\AgdaBound{msg₂}\AgdaSpace{}%
\AgdaBound{sig1}\AgdaSpace{}%
\AgdaBound{pbk3}\AgdaSymbol{)}\AgdaSpace{}%
\AgdaOperator{\AgdaRecord{∧}}\AgdaSpace{}%
\AgdaFunction{True}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaFunction{isSigned}%
\>[64]\AgdaBound{msg₂}\AgdaSpace{}%
\AgdaBound{sig2}\AgdaSpace{}%
\AgdaBound{pbk4}\AgdaSymbol{))}\<%
\\
\>[0]\AgdaFunction{lemmaHoareTripleStackGeAux'Comb2-4}\AgdaSpace{}%
\AgdaBound{msg₂}\AgdaSpace{}%
\AgdaBound{pbk1}\AgdaSpace{}%
\AgdaBound{pbk2}\AgdaSpace{}%
\AgdaBound{pbk3}\AgdaSpace{}%
\AgdaBound{pbk4}\AgdaSpace{}%
\AgdaBound{sig1}\AgdaSpace{}%
\AgdaBound{sig2}\AgdaSpace{}%
\AgdaBound{x}\AgdaSpace{}%
\AgdaKeyword{with}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaFunction{isSigned}%
\>[88]\AgdaBound{msg₂}\AgdaSpace{}%
\AgdaBound{sig1}\AgdaSpace{}%
\AgdaBound{pbk1}\AgdaSymbol{)}\<%
\\
\>[0]\AgdaFunction{lemmaHoareTripleStackGeAux'Comb2-4}\AgdaSpace{}%
\AgdaBound{msg₂}\AgdaSpace{}%
\AgdaBound{pbk1}\AgdaSpace{}%
\AgdaBound{pbk2}\AgdaSpace{}%
\AgdaBound{pbk3}\AgdaSpace{}%
\AgdaBound{pbk4}\AgdaSpace{}%
\AgdaBound{sig1}\AgdaSpace{}%
\AgdaBound{sig2}\AgdaSpace{}%
\AgdaBound{x}\AgdaSpace{}%
\AgdaSymbol{|}\AgdaSpace{}%
\AgdaInductiveConstructor{false}\AgdaSpace{}%
\AgdaKeyword{with}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaFunction{isSigned}%
\>[96]\AgdaBound{msg₂}\AgdaSpace{}%
\AgdaBound{sig1}\AgdaSpace{}%
\AgdaBound{pbk2}\AgdaSymbol{)}\<%
\\
\>[0]\AgdaFunction{lemmaHoareTripleStackGeAux'Comb2-4}\AgdaSpace{}%
\AgdaBound{msg₂}\AgdaSpace{}%
\AgdaBound{pbk1}\AgdaSpace{}%
\AgdaBound{pbk2}\AgdaSpace{}%
\AgdaBound{pbk3}\AgdaSpace{}%
\AgdaBound{pbk4}\AgdaSpace{}%
\AgdaBound{sig1}\AgdaSpace{}%
\AgdaBound{sig2}\AgdaSpace{}%
\AgdaBound{x}\AgdaSpace{}%
\AgdaSymbol{|}\AgdaSpace{}%
\AgdaInductiveConstructor{false}\AgdaSpace{}%
\AgdaSymbol{|}\AgdaSpace{}%
\AgdaInductiveConstructor{false}\AgdaSpace{}%
\AgdaKeyword{with}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaFunction{isSigned}%
\>[104]\AgdaBound{msg₂}\AgdaSpace{}%
\AgdaBound{sig1}\AgdaSpace{}%
\AgdaBound{pbk3}\AgdaSymbol{)}\<%
\\
\>[0]\AgdaFunction{lemmaHoareTripleStackGeAux'Comb2-4}\AgdaSpace{}%
\AgdaBound{msg₂}\AgdaSpace{}%
\AgdaBound{pbk1}\AgdaSpace{}%
\AgdaBound{pbk2}\AgdaSpace{}%
\AgdaBound{pbk3}\AgdaSpace{}%
\AgdaBound{pbk4}\AgdaSpace{}%
\AgdaBound{sig1}\AgdaSpace{}%
\AgdaBound{sig2}\AgdaSpace{}%
\AgdaBound{x}\AgdaSpace{}%
\AgdaSymbol{|}\AgdaSpace{}%
\AgdaInductiveConstructor{false}\AgdaSpace{}%
\AgdaSymbol{|}\AgdaSpace{}%
\AgdaInductiveConstructor{false}\AgdaSpace{}%
\AgdaSymbol{|}\AgdaSpace{}%
\AgdaInductiveConstructor{false}\AgdaSpace{}%
\AgdaKeyword{with}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaFunction{isSigned}%
\>[112]\AgdaBound{msg₂}\AgdaSpace{}%
\AgdaBound{sig1}\AgdaSpace{}%
\AgdaBound{pbk4}\AgdaSymbol{)}\<%
\\
\>[0]\AgdaFunction{lemmaHoareTripleStackGeAux'Comb2-4}\AgdaSpace{}%
\AgdaBound{msg₂}\AgdaSpace{}%
\AgdaBound{pbk1}\AgdaSpace{}%
\AgdaBound{pbk2}\AgdaSpace{}%
\AgdaBound{pbk3}\AgdaSpace{}%
\AgdaBound{pbk4}\AgdaSpace{}%
\AgdaBound{sig1}\AgdaSpace{}%
\AgdaBound{sig2}\AgdaSpace{}%
\AgdaSymbol{()}\AgdaSpace{}%
\AgdaSymbol{|}\AgdaSpace{}%
\AgdaInductiveConstructor{false}\AgdaSpace{}%
\AgdaSymbol{|}\AgdaSpace{}%
\AgdaInductiveConstructor{false}\AgdaSpace{}%
\AgdaSymbol{|}\AgdaSpace{}%
\AgdaInductiveConstructor{false}\AgdaSpace{}%
\AgdaSymbol{|}\AgdaSpace{}%
\AgdaInductiveConstructor{false}\<%
\\
\>[0]\AgdaFunction{lemmaHoareTripleStackGeAux'Comb2-4}\AgdaSpace{}%
\AgdaBound{msg₂}\AgdaSpace{}%
\AgdaBound{pbk1}\AgdaSpace{}%
\AgdaBound{pbk2}\AgdaSpace{}%
\AgdaBound{pbk3}\AgdaSpace{}%
\AgdaBound{pbk4}\AgdaSpace{}%
\AgdaBound{sig1}\AgdaSpace{}%
\AgdaBound{sig2}\AgdaSpace{}%
\AgdaSymbol{()}\AgdaSpace{}%
\AgdaSymbol{|}\AgdaSpace{}%
\AgdaInductiveConstructor{false}\AgdaSpace{}%
\AgdaSymbol{|}\AgdaSpace{}%
\AgdaInductiveConstructor{false}\AgdaSpace{}%
\AgdaSymbol{|}\AgdaSpace{}%
\AgdaInductiveConstructor{false}\AgdaSpace{}%
\AgdaSymbol{|}\AgdaSpace{}%
\AgdaInductiveConstructor{true}\<%
\\
\>[0]\AgdaFunction{lemmaHoareTripleStackGeAux'Comb2-4}\AgdaSpace{}%
\AgdaBound{msg₂}\AgdaSpace{}%
\AgdaBound{pbk1}\AgdaSpace{}%
\AgdaBound{pbk2}\AgdaSpace{}%
\AgdaBound{pbk3}\AgdaSpace{}%
\AgdaBound{pbk4}\AgdaSpace{}%
\AgdaBound{sig1}\AgdaSpace{}%
\AgdaBound{sig2}\AgdaSpace{}%
\AgdaBound{x}\AgdaSpace{}%
\AgdaSymbol{|}\AgdaSpace{}%
\AgdaInductiveConstructor{false}\AgdaSpace{}%
\AgdaSymbol{|}\AgdaSpace{}%
\AgdaInductiveConstructor{false}\AgdaSpace{}%
\AgdaSymbol{|}\AgdaSpace{}%
\AgdaInductiveConstructor{true}\AgdaSpace{}%
\AgdaKeyword{with}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaFunction{isSigned}%
\>[111]\AgdaBound{msg₂}\AgdaSpace{}%
\AgdaBound{sig2}\AgdaSpace{}%
\AgdaBound{pbk4}\AgdaSymbol{)}\<%
\\
\>[0]\AgdaFunction{lemmaHoareTripleStackGeAux'Comb2-4}\AgdaSpace{}%
\AgdaBound{msg₂}\AgdaSpace{}%
\AgdaBound{pbk1}\AgdaSpace{}%
\AgdaBound{pbk2}\AgdaSpace{}%
\AgdaBound{pbk3}\AgdaSpace{}%
\AgdaBound{pbk4}\AgdaSpace{}%
\AgdaBound{sig1}\AgdaSpace{}%
\AgdaBound{sig2}\AgdaSpace{}%
\AgdaInductiveConstructor{tt}\AgdaSpace{}%
\AgdaSymbol{|}\AgdaSpace{}%
\AgdaInductiveConstructor{false}\AgdaSpace{}%
\AgdaSymbol{|}\AgdaSpace{}%
\AgdaInductiveConstructor{false}\AgdaSpace{}%
\AgdaSymbol{|}\AgdaSpace{}%
\AgdaInductiveConstructor{true}\AgdaSpace{}%
\AgdaSymbol{|}\AgdaSpace{}%
\AgdaInductiveConstructor{true}\AgdaSpace{}%
\AgdaKeyword{with}%
\>[109]\AgdaSymbol{(}\AgdaFunction{isSigned}%
\>[120]\AgdaBound{msg₂}\AgdaSpace{}%
\AgdaBound{sig2}\AgdaSpace{}%
\AgdaBound{pbk3}\AgdaSymbol{)}\<%
\\
\>[0]\AgdaFunction{lemmaHoareTripleStackGeAux'Comb2-4}\AgdaSpace{}%
\AgdaBound{msg₂}\AgdaSpace{}%
\AgdaBound{pbk1}\AgdaSpace{}%
\AgdaBound{pbk2}\AgdaSpace{}%
\AgdaBound{pbk3}\AgdaSpace{}%
\AgdaBound{pbk4}\AgdaSpace{}%
\AgdaBound{sig1}\AgdaSpace{}%
\AgdaBound{sig2}\AgdaSpace{}%
\AgdaInductiveConstructor{tt}\AgdaSpace{}%
\AgdaSymbol{|}\AgdaSpace{}%
\AgdaInductiveConstructor{false}\AgdaSpace{}%
\AgdaSymbol{|}\AgdaSpace{}%
\AgdaInductiveConstructor{false}\AgdaSpace{}%
\AgdaSymbol{|}\AgdaSpace{}%
\AgdaInductiveConstructor{true}\AgdaSpace{}%
\AgdaSymbol{|}\AgdaSpace{}%
\AgdaInductiveConstructor{true}\AgdaSpace{}%
\AgdaSymbol{|}\AgdaSpace{}%
\AgdaInductiveConstructor{false}\AgdaSpace{}%
\AgdaKeyword{with}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaFunction{isSigned}%
\>[127]\AgdaBound{msg₂}\AgdaSpace{}%
\AgdaBound{sig2}\AgdaSpace{}%
\AgdaBound{pbk2}\AgdaSymbol{)}\<%
\\
\>[0]\AgdaFunction{lemmaHoareTripleStackGeAux'Comb2-4}\AgdaSpace{}%
\AgdaBound{msg₂}\AgdaSpace{}%
\AgdaBound{pbk1}\AgdaSpace{}%
\AgdaBound{pbk2}\AgdaSpace{}%
\AgdaBound{pbk3}\AgdaSpace{}%
\AgdaBound{pbk4}\AgdaSpace{}%
\AgdaBound{sig1}\AgdaSpace{}%
\AgdaBound{sig2}\AgdaSpace{}%
\AgdaInductiveConstructor{tt}\AgdaSpace{}%
\AgdaSymbol{|}\AgdaSpace{}%
\AgdaInductiveConstructor{false}\AgdaSpace{}%
\AgdaSymbol{|}\AgdaSpace{}%
\AgdaInductiveConstructor{false}\AgdaSpace{}%
\AgdaSymbol{|}\AgdaSpace{}%
\AgdaInductiveConstructor{true}\AgdaSpace{}%
\AgdaSymbol{|}\AgdaSpace{}%
\AgdaInductiveConstructor{true}\AgdaSpace{}%
\AgdaSymbol{|}\AgdaSpace{}%
\AgdaInductiveConstructor{false}\AgdaSpace{}%
\AgdaSymbol{|}\AgdaSpace{}%
\AgdaInductiveConstructor{false}\AgdaSpace{}%
\AgdaSymbol{=}\AgdaSpace{}%
\AgdaInductiveConstructor{inj₂}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaInductiveConstructor{inj₂}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaInductiveConstructor{inj₂}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaInductiveConstructor{inj₂}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaInductiveConstructor{inj₂}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaInductiveConstructor{conj}\AgdaSpace{}%
\AgdaInductiveConstructor{tt}\AgdaSpace{}%
\AgdaInductiveConstructor{tt}\AgdaSymbol{)))))}\<%
\\
\>[0]\AgdaFunction{lemmaHoareTripleStackGeAux'Comb2-4}\AgdaSpace{}%
\AgdaBound{msg₂}\AgdaSpace{}%
\AgdaBound{pbk1}\AgdaSpace{}%
\AgdaBound{pbk2}\AgdaSpace{}%
\AgdaBound{pbk3}\AgdaSpace{}%
\AgdaBound{pbk4}\AgdaSpace{}%
\AgdaBound{sig1}\AgdaSpace{}%
\AgdaBound{sig2}\AgdaSpace{}%
\AgdaInductiveConstructor{tt}\AgdaSpace{}%
\AgdaSymbol{|}\AgdaSpace{}%
\AgdaInductiveConstructor{false}\AgdaSpace{}%
\AgdaSymbol{|}\AgdaSpace{}%
\AgdaInductiveConstructor{false}\AgdaSpace{}%
\AgdaSymbol{|}\AgdaSpace{}%
\AgdaInductiveConstructor{true}\AgdaSpace{}%
\AgdaSymbol{|}\AgdaSpace{}%
\AgdaInductiveConstructor{true}\AgdaSpace{}%
\AgdaSymbol{|}\AgdaSpace{}%
\AgdaInductiveConstructor{false}\AgdaSpace{}%
\AgdaSymbol{|}\AgdaSpace{}%
\AgdaInductiveConstructor{true}\AgdaSpace{}%
\AgdaSymbol{=}\AgdaSpace{}%
\AgdaInductiveConstructor{inj₂}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaInductiveConstructor{inj₂}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaInductiveConstructor{inj₂}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaInductiveConstructor{inj₂}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaInductiveConstructor{inj₂}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaInductiveConstructor{conj}\AgdaSpace{}%
\AgdaInductiveConstructor{tt}\AgdaSpace{}%
\AgdaInductiveConstructor{tt}\AgdaSymbol{)))))}\<%
\\
\>[0]\AgdaFunction{lemmaHoareTripleStackGeAux'Comb2-4}\AgdaSpace{}%
\AgdaBound{msg₂}\AgdaSpace{}%
\AgdaBound{pbk1}\AgdaSpace{}%
\AgdaBound{pbk2}\AgdaSpace{}%
\AgdaBound{pbk3}\AgdaSpace{}%
\AgdaBound{pbk4}\AgdaSpace{}%
\AgdaBound{sig1}\AgdaSpace{}%
\AgdaBound{sig2}\AgdaSpace{}%
\AgdaInductiveConstructor{tt}\AgdaSpace{}%
\AgdaSymbol{|}\AgdaSpace{}%
\AgdaInductiveConstructor{false}\AgdaSpace{}%
\AgdaSymbol{|}\AgdaSpace{}%
\AgdaInductiveConstructor{false}\AgdaSpace{}%
\AgdaSymbol{|}\AgdaSpace{}%
\AgdaInductiveConstructor{true}\AgdaSpace{}%
\AgdaSymbol{|}\AgdaSpace{}%
\AgdaInductiveConstructor{true}\AgdaSpace{}%
\AgdaSymbol{|}\AgdaSpace{}%
\AgdaInductiveConstructor{true}\AgdaSpace{}%
\AgdaKeyword{with}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaFunction{isSigned}%
\>[126]\AgdaBound{msg₂}\AgdaSpace{}%
\AgdaBound{sig2}\AgdaSpace{}%
\AgdaBound{pbk2}\AgdaSymbol{)}\<%
\\
\>[0]\AgdaFunction{lemmaHoareTripleStackGeAux'Comb2-4}\AgdaSpace{}%
\AgdaBound{msg₂}\AgdaSpace{}%
\AgdaBound{pbk1}\AgdaSpace{}%
\AgdaBound{pbk2}\AgdaSpace{}%
\AgdaBound{pbk3}\AgdaSpace{}%
\AgdaBound{pbk4}\AgdaSpace{}%
\AgdaBound{sig1}\AgdaSpace{}%
\AgdaBound{sig2}\AgdaSpace{}%
\AgdaInductiveConstructor{tt}\AgdaSpace{}%
\AgdaSymbol{|}\AgdaSpace{}%
\AgdaInductiveConstructor{false}\AgdaSpace{}%
\AgdaSymbol{|}\AgdaSpace{}%
\AgdaInductiveConstructor{false}\AgdaSpace{}%
\AgdaSymbol{|}\AgdaSpace{}%
\AgdaInductiveConstructor{true}\AgdaSpace{}%
\AgdaSymbol{|}\AgdaSpace{}%
\AgdaInductiveConstructor{true}\AgdaSpace{}%
\AgdaSymbol{|}\AgdaSpace{}%
\AgdaInductiveConstructor{true}\AgdaSpace{}%
\AgdaSymbol{|}\AgdaSpace{}%
\AgdaInductiveConstructor{false}\AgdaSpace{}%
\AgdaSymbol{=}\AgdaSpace{}%
\AgdaInductiveConstructor{inj₂}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaInductiveConstructor{inj₂}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaInductiveConstructor{inj₂}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaInductiveConstructor{inj₂}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaInductiveConstructor{inj₂}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaInductiveConstructor{conj}\AgdaSpace{}%
\AgdaInductiveConstructor{tt}\AgdaSpace{}%
\AgdaInductiveConstructor{tt}\AgdaSymbol{)))))}\<%
\\
\>[0]\AgdaFunction{lemmaHoareTripleStackGeAux'Comb2-4}\AgdaSpace{}%
\AgdaBound{msg₂}\AgdaSpace{}%
\AgdaBound{pbk1}\AgdaSpace{}%
\AgdaBound{pbk2}\AgdaSpace{}%
\AgdaBound{pbk3}\AgdaSpace{}%
\AgdaBound{pbk4}\AgdaSpace{}%
\AgdaBound{sig1}\AgdaSpace{}%
\AgdaBound{sig2}\AgdaSpace{}%
\AgdaInductiveConstructor{tt}\AgdaSpace{}%
\AgdaSymbol{|}\AgdaSpace{}%
\AgdaInductiveConstructor{false}\AgdaSpace{}%
\AgdaSymbol{|}\AgdaSpace{}%
\AgdaInductiveConstructor{false}\AgdaSpace{}%
\AgdaSymbol{|}\AgdaSpace{}%
\AgdaInductiveConstructor{true}\AgdaSpace{}%
\AgdaSymbol{|}\AgdaSpace{}%
\AgdaInductiveConstructor{true}\AgdaSpace{}%
\AgdaSymbol{|}\AgdaSpace{}%
\AgdaInductiveConstructor{true}\AgdaSpace{}%
\AgdaSymbol{|}\AgdaSpace{}%
\AgdaInductiveConstructor{true}\AgdaSpace{}%
\AgdaSymbol{=}\AgdaSpace{}%
\AgdaInductiveConstructor{inj₂}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaInductiveConstructor{inj₂}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaInductiveConstructor{inj₂}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaInductiveConstructor{inj₂}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaInductiveConstructor{inj₂}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaInductiveConstructor{conj}\AgdaSpace{}%
\AgdaInductiveConstructor{tt}\AgdaSpace{}%
\AgdaInductiveConstructor{tt}\AgdaSymbol{)))))}\<%
\\
\>[0]\AgdaFunction{lemmaHoareTripleStackGeAux'Comb2-4}\AgdaSpace{}%
\AgdaBound{msg₂}\AgdaSpace{}%
\AgdaBound{pbk1}\AgdaSpace{}%
\AgdaBound{pbk2}\AgdaSpace{}%
\AgdaBound{pbk3}\AgdaSpace{}%
\AgdaBound{pbk4}\AgdaSpace{}%
\AgdaBound{sig1}\AgdaSpace{}%
\AgdaBound{sig2}\AgdaSpace{}%
\AgdaBound{x}\AgdaSpace{}%
\AgdaSymbol{|}\AgdaSpace{}%
\AgdaInductiveConstructor{false}\AgdaSpace{}%
\AgdaSymbol{|}\AgdaSpace{}%
\AgdaInductiveConstructor{true}\AgdaSpace{}%
\AgdaKeyword{with}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaFunction{isSigned}%
\>[103]\AgdaBound{msg₂}\AgdaSpace{}%
\AgdaBound{sig2}\AgdaSpace{}%
\AgdaBound{pbk3}\AgdaSymbol{)}\<%
\\
\>[0]\AgdaFunction{lemmaHoareTripleStackGeAux'Comb2-4}\AgdaSpace{}%
\AgdaBound{msg₂}\AgdaSpace{}%
\AgdaBound{pbk1}\AgdaSpace{}%
\AgdaBound{pbk2}\AgdaSpace{}%
\AgdaBound{pbk3}\AgdaSpace{}%
\AgdaBound{pbk4}\AgdaSpace{}%
\AgdaBound{sig1}\AgdaSpace{}%
\AgdaBound{sig2}\AgdaSpace{}%
\AgdaBound{x}\AgdaSpace{}%
\AgdaSymbol{|}\AgdaSpace{}%
\AgdaInductiveConstructor{false}\AgdaSpace{}%
\AgdaSymbol{|}\AgdaSpace{}%
\AgdaInductiveConstructor{true}\AgdaSpace{}%
\AgdaSymbol{|}\AgdaSpace{}%
\AgdaInductiveConstructor{false}\AgdaSpace{}%
\AgdaKeyword{with}%
\>[101]\AgdaSymbol{(}\AgdaFunction{isSigned}%
\>[112]\AgdaBound{msg₂}\AgdaSpace{}%
\AgdaBound{sig2}\AgdaSpace{}%
\AgdaBound{pbk4}\AgdaSymbol{)}\<%
\\
\>[0]\AgdaFunction{lemmaHoareTripleStackGeAux'Comb2-4}\AgdaSpace{}%
\AgdaBound{msg₂}\AgdaSpace{}%
\AgdaBound{pbk1}\AgdaSpace{}%
\AgdaBound{pbk2}\AgdaSpace{}%
\AgdaBound{pbk3}\AgdaSpace{}%
\AgdaBound{pbk4}\AgdaSpace{}%
\AgdaBound{sig1}\AgdaSpace{}%
\AgdaBound{sig2}\AgdaSpace{}%
\AgdaBound{x}\AgdaSpace{}%
\AgdaSymbol{|}\AgdaSpace{}%
\AgdaInductiveConstructor{false}\AgdaSpace{}%
\AgdaSymbol{|}\AgdaSpace{}%
\AgdaInductiveConstructor{true}\AgdaSpace{}%
\AgdaSymbol{|}\AgdaSpace{}%
\AgdaInductiveConstructor{false}\AgdaSpace{}%
\AgdaSymbol{|}\AgdaSpace{}%
\AgdaInductiveConstructor{true}\AgdaSpace{}%
\AgdaKeyword{with}\AgdaSpace{}%
\AgdaFunction{isSigned}%
\>[117]\AgdaBound{msg₂}\AgdaSpace{}%
\AgdaBound{sig1}\AgdaSpace{}%
\AgdaBound{pbk3}\<%
\\
\>[0]\AgdaFunction{lemmaHoareTripleStackGeAux'Comb2-4}\AgdaSpace{}%
\AgdaBound{msg₂}\AgdaSpace{}%
\AgdaBound{pbk1}\AgdaSpace{}%
\AgdaBound{pbk2}\AgdaSpace{}%
\AgdaBound{pbk3}\AgdaSpace{}%
\AgdaBound{pbk4}\AgdaSpace{}%
\AgdaBound{sig1}\AgdaSpace{}%
\AgdaBound{sig2}\AgdaSpace{}%
\AgdaBound{x}\AgdaSpace{}%
\AgdaSymbol{|}\AgdaSpace{}%
\AgdaInductiveConstructor{false}\AgdaSpace{}%
\AgdaSymbol{|}\AgdaSpace{}%
\AgdaInductiveConstructor{true}\AgdaSpace{}%
\AgdaSymbol{|}\AgdaSpace{}%
\AgdaInductiveConstructor{false}\AgdaSpace{}%
\AgdaSymbol{|}\AgdaSpace{}%
\AgdaInductiveConstructor{true}\AgdaSpace{}%
\AgdaSymbol{|}\AgdaSpace{}%
\AgdaInductiveConstructor{false}\AgdaSpace{}%
\AgdaKeyword{with}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaFunction{isSigned}%
\>[126]\AgdaBound{msg₂}\AgdaSpace{}%
\AgdaBound{sig2}\AgdaSpace{}%
\AgdaBound{pbk2}\AgdaSymbol{)}\<%
\\
\>[0]\AgdaFunction{lemmaHoareTripleStackGeAux'Comb2-4}\AgdaSpace{}%
\AgdaBound{msg₂}\AgdaSpace{}%
\AgdaBound{pbk1}\AgdaSpace{}%
\AgdaBound{pbk2}\AgdaSpace{}%
\AgdaBound{pbk3}\AgdaSpace{}%
\AgdaBound{pbk4}\AgdaSpace{}%
\AgdaBound{sig1}\AgdaSpace{}%
\AgdaBound{sig2}\AgdaSpace{}%
\AgdaBound{x}\AgdaSpace{}%
\AgdaSymbol{|}\AgdaSpace{}%
\AgdaInductiveConstructor{false}\AgdaSpace{}%
\AgdaSymbol{|}\AgdaSpace{}%
\AgdaInductiveConstructor{true}\AgdaSpace{}%
\AgdaSymbol{|}\AgdaSpace{}%
\AgdaInductiveConstructor{false}\AgdaSpace{}%
\AgdaSymbol{|}\AgdaSpace{}%
\AgdaInductiveConstructor{true}\AgdaSpace{}%
\AgdaSymbol{|}\AgdaSpace{}%
\AgdaInductiveConstructor{false}\AgdaSpace{}%
\AgdaSymbol{|}\AgdaSpace{}%
\AgdaInductiveConstructor{false}\AgdaSpace{}%
\AgdaSymbol{=}\AgdaSpace{}%
\AgdaInductiveConstructor{inj₂}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaInductiveConstructor{inj₂}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaInductiveConstructor{inj₂}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaInductiveConstructor{inj₂}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaInductiveConstructor{inj₁}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaInductiveConstructor{conj}\AgdaSpace{}%
\AgdaInductiveConstructor{tt}\AgdaSpace{}%
\AgdaInductiveConstructor{tt}\AgdaSymbol{)))))}\<%
\\
\>[0]\AgdaFunction{lemmaHoareTripleStackGeAux'Comb2-4}\AgdaSpace{}%
\AgdaBound{msg₂}\AgdaSpace{}%
\AgdaBound{pbk1}\AgdaSpace{}%
\AgdaBound{pbk2}\AgdaSpace{}%
\AgdaBound{pbk3}\AgdaSpace{}%
\AgdaBound{pbk4}\AgdaSpace{}%
\AgdaBound{sig1}\AgdaSpace{}%
\AgdaBound{sig2}\AgdaSpace{}%
\AgdaBound{x}\AgdaSpace{}%
\AgdaSymbol{|}\AgdaSpace{}%
\AgdaInductiveConstructor{false}\AgdaSpace{}%
\AgdaSymbol{|}\AgdaSpace{}%
\AgdaInductiveConstructor{true}\AgdaSpace{}%
\AgdaSymbol{|}\AgdaSpace{}%
\AgdaInductiveConstructor{false}\AgdaSpace{}%
\AgdaSymbol{|}\AgdaSpace{}%
\AgdaInductiveConstructor{true}\AgdaSpace{}%
\AgdaSymbol{|}\AgdaSpace{}%
\AgdaInductiveConstructor{false}\AgdaSpace{}%
\AgdaSymbol{|}\AgdaSpace{}%
\AgdaInductiveConstructor{true}\AgdaSpace{}%
\AgdaSymbol{=}\AgdaSpace{}%
\AgdaInductiveConstructor{inj₂}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaInductiveConstructor{inj₂}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaInductiveConstructor{inj₂}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaInductiveConstructor{inj₂}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaInductiveConstructor{inj₁}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaInductiveConstructor{conj}\AgdaSpace{}%
\AgdaInductiveConstructor{tt}\AgdaSpace{}%
\AgdaInductiveConstructor{tt}\AgdaSymbol{)))))}\<%
\\
\>[0]\AgdaFunction{lemmaHoareTripleStackGeAux'Comb2-4}\AgdaSpace{}%
\AgdaBound{msg₂}\AgdaSpace{}%
\AgdaBound{pbk1}\AgdaSpace{}%
\AgdaBound{pbk2}\AgdaSpace{}%
\AgdaBound{pbk3}\AgdaSpace{}%
\AgdaBound{pbk4}\AgdaSpace{}%
\AgdaBound{sig1}\AgdaSpace{}%
\AgdaBound{sig2}\AgdaSpace{}%
\AgdaBound{x}\AgdaSpace{}%
\AgdaSymbol{|}\AgdaSpace{}%
\AgdaInductiveConstructor{false}\AgdaSpace{}%
\AgdaSymbol{|}\AgdaSpace{}%
\AgdaInductiveConstructor{true}\AgdaSpace{}%
\AgdaSymbol{|}\AgdaSpace{}%
\AgdaInductiveConstructor{false}\AgdaSpace{}%
\AgdaSymbol{|}\AgdaSpace{}%
\AgdaInductiveConstructor{true}\AgdaSpace{}%
\AgdaSymbol{|}\AgdaSpace{}%
\AgdaInductiveConstructor{true}\AgdaSpace{}%
\AgdaKeyword{with}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaFunction{isSigned}%
\>[125]\AgdaBound{msg₂}\AgdaSpace{}%
\AgdaBound{sig2}\AgdaSpace{}%
\AgdaBound{pbk2}\AgdaSymbol{)}\<%
\\
\>[0]\AgdaFunction{lemmaHoareTripleStackGeAux'Comb2-4}\AgdaSpace{}%
\AgdaBound{msg₂}\AgdaSpace{}%
\AgdaBound{pbk1}\AgdaSpace{}%
\AgdaBound{pbk2}\AgdaSpace{}%
\AgdaBound{pbk3}\AgdaSpace{}%
\AgdaBound{pbk4}\AgdaSpace{}%
\AgdaBound{sig1}\AgdaSpace{}%
\AgdaBound{sig2}\AgdaSpace{}%
\AgdaBound{x}\AgdaSpace{}%
\AgdaSymbol{|}\AgdaSpace{}%
\AgdaInductiveConstructor{false}\AgdaSpace{}%
\AgdaSymbol{|}\AgdaSpace{}%
\AgdaInductiveConstructor{true}\AgdaSpace{}%
\AgdaSymbol{|}\AgdaSpace{}%
\AgdaInductiveConstructor{false}\AgdaSpace{}%
\AgdaSymbol{|}\AgdaSpace{}%
\AgdaInductiveConstructor{true}\AgdaSpace{}%
\AgdaSymbol{|}\AgdaSpace{}%
\AgdaInductiveConstructor{true}\AgdaSpace{}%
\AgdaSymbol{|}\AgdaSpace{}%
\AgdaInductiveConstructor{false}\AgdaSpace{}%
\AgdaSymbol{=}\AgdaSpace{}%
\AgdaInductiveConstructor{inj₂}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaInductiveConstructor{inj₂}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaInductiveConstructor{inj₂}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaInductiveConstructor{inj₂}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaInductiveConstructor{inj₁}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaInductiveConstructor{conj}\AgdaSpace{}%
\AgdaInductiveConstructor{tt}\AgdaSpace{}%
\AgdaInductiveConstructor{tt}\AgdaSymbol{)))))}\<%
\\
\>[0]\AgdaFunction{lemmaHoareTripleStackGeAux'Comb2-4}\AgdaSpace{}%
\AgdaBound{msg₂}\AgdaSpace{}%
\AgdaBound{pbk1}\AgdaSpace{}%
\AgdaBound{pbk2}\AgdaSpace{}%
\AgdaBound{pbk3}\AgdaSpace{}%
\AgdaBound{pbk4}\AgdaSpace{}%
\AgdaBound{sig1}\AgdaSpace{}%
\AgdaBound{sig2}\AgdaSpace{}%
\AgdaBound{x}\AgdaSpace{}%
\AgdaSymbol{|}\AgdaSpace{}%
\AgdaInductiveConstructor{false}\AgdaSpace{}%
\AgdaSymbol{|}\AgdaSpace{}%
\AgdaInductiveConstructor{true}\AgdaSpace{}%
\AgdaSymbol{|}\AgdaSpace{}%
\AgdaInductiveConstructor{false}\AgdaSpace{}%
\AgdaSymbol{|}\AgdaSpace{}%
\AgdaInductiveConstructor{true}\AgdaSpace{}%
\AgdaSymbol{|}\AgdaSpace{}%
\AgdaInductiveConstructor{true}\AgdaSpace{}%
\AgdaSymbol{|}\AgdaSpace{}%
\AgdaInductiveConstructor{true}\AgdaSpace{}%
\AgdaSymbol{=}\AgdaSpace{}%
\AgdaInductiveConstructor{inj₂}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaInductiveConstructor{inj₂}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaInductiveConstructor{inj₂}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaInductiveConstructor{inj₂}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaInductiveConstructor{inj₁}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaInductiveConstructor{conj}\AgdaSpace{}%
\AgdaInductiveConstructor{tt}\AgdaSpace{}%
\AgdaInductiveConstructor{tt}\AgdaSymbol{)))))}\<%
\\
\>[0]\AgdaFunction{lemmaHoareTripleStackGeAux'Comb2-4}\AgdaSpace{}%
\AgdaBound{msg₂}\AgdaSpace{}%
\AgdaBound{pbk1}\AgdaSpace{}%
\AgdaBound{pbk2}\AgdaSpace{}%
\AgdaBound{pbk3}\AgdaSpace{}%
\AgdaBound{pbk4}\AgdaSpace{}%
\AgdaBound{sig1}\AgdaSpace{}%
\AgdaBound{sig2}\AgdaSpace{}%
\AgdaBound{x}\AgdaSpace{}%
\AgdaSymbol{|}\AgdaSpace{}%
\AgdaInductiveConstructor{false}\AgdaSpace{}%
\AgdaSymbol{|}\AgdaSpace{}%
\AgdaInductiveConstructor{true}\AgdaSpace{}%
\AgdaSymbol{|}\AgdaSpace{}%
\AgdaInductiveConstructor{true}\AgdaSpace{}%
\AgdaKeyword{with}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaFunction{isSigned}%
\>[110]\AgdaBound{msg₂}\AgdaSpace{}%
\AgdaBound{sig2}\AgdaSpace{}%
\AgdaBound{pbk4}\AgdaSymbol{)}\<%
\\
\>[0]\AgdaFunction{lemmaHoareTripleStackGeAux'Comb2-4}\AgdaSpace{}%
\AgdaBound{msg₂}\AgdaSpace{}%
\AgdaBound{pbk1}\AgdaSpace{}%
\AgdaBound{pbk2}\AgdaSpace{}%
\AgdaBound{pbk3}\AgdaSpace{}%
\AgdaBound{pbk4}\AgdaSpace{}%
\AgdaBound{sig1}\AgdaSpace{}%
\AgdaBound{sig2}\AgdaSpace{}%
\AgdaBound{x}\AgdaSpace{}%
\AgdaSymbol{|}\AgdaSpace{}%
\AgdaInductiveConstructor{false}\AgdaSpace{}%
\AgdaSymbol{|}\AgdaSpace{}%
\AgdaInductiveConstructor{true}\AgdaSpace{}%
\AgdaSymbol{|}\AgdaSpace{}%
\AgdaInductiveConstructor{true}\AgdaSpace{}%
\AgdaSymbol{|}\AgdaSpace{}%
\AgdaInductiveConstructor{false}\AgdaSpace{}%
\AgdaKeyword{with}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaFunction{isSigned}%
\>[118]\AgdaBound{msg₂}\AgdaSpace{}%
\AgdaBound{sig1}\AgdaSpace{}%
\AgdaBound{pbk3}\AgdaSymbol{)}\<%
\\
\>[0]\AgdaFunction{lemmaHoareTripleStackGeAux'Comb2-4}\AgdaSpace{}%
\AgdaBound{msg₂}\AgdaSpace{}%
\AgdaBound{pbk1}\AgdaSpace{}%
\AgdaBound{pbk2}\AgdaSpace{}%
\AgdaBound{pbk3}\AgdaSpace{}%
\AgdaBound{pbk4}\AgdaSpace{}%
\AgdaBound{sig1}\AgdaSpace{}%
\AgdaBound{sig2}\AgdaSpace{}%
\AgdaBound{x}\AgdaSpace{}%
\AgdaSymbol{|}\AgdaSpace{}%
\AgdaInductiveConstructor{false}\AgdaSpace{}%
\AgdaSymbol{|}\AgdaSpace{}%
\AgdaInductiveConstructor{true}\AgdaSpace{}%
\AgdaSymbol{|}\AgdaSpace{}%
\AgdaInductiveConstructor{true}\AgdaSpace{}%
\AgdaSymbol{|}\AgdaSpace{}%
\AgdaInductiveConstructor{false}\AgdaSpace{}%
\AgdaSymbol{|}\AgdaSpace{}%
\AgdaInductiveConstructor{false}\AgdaSpace{}%
\AgdaKeyword{with}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaFunction{isSigned}%
\>[126]\AgdaBound{msg₂}\AgdaSpace{}%
\AgdaBound{sig2}\AgdaSpace{}%
\AgdaBound{pbk2}\AgdaSymbol{)}\<%
\\
\>[0]\AgdaFunction{lemmaHoareTripleStackGeAux'Comb2-4}\AgdaSpace{}%
\AgdaBound{msg₂}\AgdaSpace{}%
\AgdaBound{pbk1}\AgdaSpace{}%
\AgdaBound{pbk2}\AgdaSpace{}%
\AgdaBound{pbk3}\AgdaSpace{}%
\AgdaBound{pbk4}\AgdaSpace{}%
\AgdaBound{sig1}\AgdaSpace{}%
\AgdaBound{sig2}\AgdaSpace{}%
\AgdaBound{x}\AgdaSpace{}%
\AgdaSymbol{|}\AgdaSpace{}%
\AgdaInductiveConstructor{false}\AgdaSpace{}%
\AgdaSymbol{|}\AgdaSpace{}%
\AgdaInductiveConstructor{true}\AgdaSpace{}%
\AgdaSymbol{|}\AgdaSpace{}%
\AgdaInductiveConstructor{true}\AgdaSpace{}%
\AgdaSymbol{|}\AgdaSpace{}%
\AgdaInductiveConstructor{false}\AgdaSpace{}%
\AgdaSymbol{|}\AgdaSpace{}%
\AgdaInductiveConstructor{false}\AgdaSpace{}%
\AgdaSymbol{|}\AgdaSpace{}%
\AgdaInductiveConstructor{false}\AgdaSpace{}%
\AgdaSymbol{=}\AgdaSpace{}%
\AgdaInductiveConstructor{inj₂}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaInductiveConstructor{inj₂}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaInductiveConstructor{inj₂}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaInductiveConstructor{inj₁}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaInductiveConstructor{conj}\AgdaSpace{}%
\AgdaInductiveConstructor{tt}\AgdaSpace{}%
\AgdaInductiveConstructor{tt}\AgdaSymbol{))))}\<%
\\
\>[0]\AgdaFunction{lemmaHoareTripleStackGeAux'Comb2-4}\AgdaSpace{}%
\AgdaBound{msg₂}\AgdaSpace{}%
\AgdaBound{pbk1}\AgdaSpace{}%
\AgdaBound{pbk2}\AgdaSpace{}%
\AgdaBound{pbk3}\AgdaSpace{}%
\AgdaBound{pbk4}\AgdaSpace{}%
\AgdaBound{sig1}\AgdaSpace{}%
\AgdaBound{sig2}\AgdaSpace{}%
\AgdaBound{x}\AgdaSpace{}%
\AgdaSymbol{|}\AgdaSpace{}%
\AgdaInductiveConstructor{false}\AgdaSpace{}%
\AgdaSymbol{|}\AgdaSpace{}%
\AgdaInductiveConstructor{true}\AgdaSpace{}%
\AgdaSymbol{|}\AgdaSpace{}%
\AgdaInductiveConstructor{true}\AgdaSpace{}%
\AgdaSymbol{|}\AgdaSpace{}%
\AgdaInductiveConstructor{false}\AgdaSpace{}%
\AgdaSymbol{|}\AgdaSpace{}%
\AgdaInductiveConstructor{false}\AgdaSpace{}%
\AgdaSymbol{|}\AgdaSpace{}%
\AgdaInductiveConstructor{true}\AgdaSpace{}%
\AgdaSymbol{=}\AgdaSpace{}%
\AgdaInductiveConstructor{inj₂}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaInductiveConstructor{inj₂}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaInductiveConstructor{inj₂}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaInductiveConstructor{inj₁}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaInductiveConstructor{conj}\AgdaSpace{}%
\AgdaInductiveConstructor{tt}\AgdaSpace{}%
\AgdaInductiveConstructor{tt}\AgdaSymbol{))))}\<%
\\
\>[0]\AgdaFunction{lemmaHoareTripleStackGeAux'Comb2-4}\AgdaSpace{}%
\AgdaBound{msg₂}\AgdaSpace{}%
\AgdaBound{pbk1}\AgdaSpace{}%
\AgdaBound{pbk2}\AgdaSpace{}%
\AgdaBound{pbk3}\AgdaSpace{}%
\AgdaBound{pbk4}\AgdaSpace{}%
\AgdaBound{sig1}\AgdaSpace{}%
\AgdaBound{sig2}\AgdaSpace{}%
\AgdaBound{x}\AgdaSpace{}%
\AgdaSymbol{|}\AgdaSpace{}%
\AgdaInductiveConstructor{false}\AgdaSpace{}%
\AgdaSymbol{|}\AgdaSpace{}%
\AgdaInductiveConstructor{true}\AgdaSpace{}%
\AgdaSymbol{|}\AgdaSpace{}%
\AgdaInductiveConstructor{true}\AgdaSpace{}%
\AgdaSymbol{|}\AgdaSpace{}%
\AgdaInductiveConstructor{false}\AgdaSpace{}%
\AgdaSymbol{|}\AgdaSpace{}%
\AgdaInductiveConstructor{true}\AgdaSpace{}%
\AgdaSymbol{=}\AgdaSpace{}%
\AgdaInductiveConstructor{inj₂}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaInductiveConstructor{inj₂}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaInductiveConstructor{inj₂}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaInductiveConstructor{inj₁}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaInductiveConstructor{conj}\AgdaSpace{}%
\AgdaInductiveConstructor{tt}\AgdaSpace{}%
\AgdaInductiveConstructor{tt}\AgdaSymbol{))))}\<%
\\
\>[0]\AgdaFunction{lemmaHoareTripleStackGeAux'Comb2-4}\AgdaSpace{}%
\AgdaBound{msg₂}\AgdaSpace{}%
\AgdaBound{pbk1}\AgdaSpace{}%
\AgdaBound{pbk2}\AgdaSpace{}%
\AgdaBound{pbk3}\AgdaSpace{}%
\AgdaBound{pbk4}\AgdaSpace{}%
\AgdaBound{sig1}\AgdaSpace{}%
\AgdaBound{sig2}\AgdaSpace{}%
\AgdaBound{x}\AgdaSpace{}%
\AgdaSymbol{|}\AgdaSpace{}%
\AgdaInductiveConstructor{false}\AgdaSpace{}%
\AgdaSymbol{|}\AgdaSpace{}%
\AgdaInductiveConstructor{true}\AgdaSpace{}%
\AgdaSymbol{|}\AgdaSpace{}%
\AgdaInductiveConstructor{true}\AgdaSpace{}%
\AgdaSymbol{|}\AgdaSpace{}%
\AgdaInductiveConstructor{true}\AgdaSpace{}%
\AgdaSymbol{=}\AgdaSpace{}%
\AgdaInductiveConstructor{inj₂}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaInductiveConstructor{inj₂}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaInductiveConstructor{inj₂}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaInductiveConstructor{inj₁}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaInductiveConstructor{conj}\AgdaSpace{}%
\AgdaInductiveConstructor{tt}\AgdaSpace{}%
\AgdaInductiveConstructor{tt}\AgdaSymbol{))))}\<%
\\
\>[0]\AgdaFunction{lemmaHoareTripleStackGeAux'Comb2-4}\AgdaSpace{}%
\AgdaBound{msg₂}\AgdaSpace{}%
\AgdaBound{pbk1}\AgdaSpace{}%
\AgdaBound{pbk2}\AgdaSpace{}%
\AgdaBound{pbk3}\AgdaSpace{}%
\AgdaBound{pbk4}\AgdaSpace{}%
\AgdaBound{sig1}\AgdaSpace{}%
\AgdaBound{sig2}\AgdaSpace{}%
\AgdaBound{x}\AgdaSpace{}%
\AgdaSymbol{|}\AgdaSpace{}%
\AgdaInductiveConstructor{true}\AgdaSpace{}%
\AgdaKeyword{with}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaFunction{isSigned}%
\>[95]\AgdaBound{msg₂}\AgdaSpace{}%
\AgdaBound{sig2}\AgdaSpace{}%
\AgdaBound{pbk2}\AgdaSymbol{)}\<%
\\
\>[0]\AgdaFunction{lemmaHoareTripleStackGeAux'Comb2-4}\AgdaSpace{}%
\AgdaBound{msg₂}\AgdaSpace{}%
\AgdaBound{pbk1}\AgdaSpace{}%
\AgdaBound{pbk2}\AgdaSpace{}%
\AgdaBound{pbk3}\AgdaSpace{}%
\AgdaBound{pbk4}\AgdaSpace{}%
\AgdaBound{sig1}\AgdaSpace{}%
\AgdaBound{sig2}\AgdaSpace{}%
\AgdaBound{x}\AgdaSpace{}%
\AgdaSymbol{|}\AgdaSpace{}%
\AgdaInductiveConstructor{true}\AgdaSpace{}%
\AgdaSymbol{|}\AgdaSpace{}%
\AgdaInductiveConstructor{false}\AgdaSpace{}%
\AgdaKeyword{with}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaFunction{isSigned}%
\>[103]\AgdaBound{msg₂}\AgdaSpace{}%
\AgdaBound{sig2}\AgdaSpace{}%
\AgdaBound{pbk3}\AgdaSymbol{)}\<%
\\
\>[0]\AgdaFunction{lemmaHoareTripleStackGeAux'Comb2-4}\AgdaSpace{}%
\AgdaBound{msg₂}\AgdaSpace{}%
\AgdaBound{pbk1}\AgdaSpace{}%
\AgdaBound{pbk2}\AgdaSpace{}%
\AgdaBound{pbk3}\AgdaSpace{}%
\AgdaBound{pbk4}\AgdaSpace{}%
\AgdaBound{sig1}\AgdaSpace{}%
\AgdaBound{sig2}\AgdaSpace{}%
\AgdaBound{x}\AgdaSpace{}%
\AgdaSymbol{|}\AgdaSpace{}%
\AgdaInductiveConstructor{true}\AgdaSpace{}%
\AgdaSymbol{|}\AgdaSpace{}%
\AgdaInductiveConstructor{false}\AgdaSpace{}%
\AgdaSymbol{|}\AgdaSpace{}%
\AgdaInductiveConstructor{false}\AgdaSpace{}%
\AgdaKeyword{with}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaFunction{isSigned}%
\>[111]\AgdaBound{msg₂}\AgdaSpace{}%
\AgdaBound{sig2}\AgdaSpace{}%
\AgdaBound{pbk4}\AgdaSymbol{)}\<%
\\
\>[0]\AgdaFunction{lemmaHoareTripleStackGeAux'Comb2-4}\AgdaSpace{}%
\AgdaBound{msg₂}\AgdaSpace{}%
\AgdaBound{pbk1}\AgdaSpace{}%
\AgdaBound{pbk2}\AgdaSpace{}%
\AgdaBound{pbk3}\AgdaSpace{}%
\AgdaBound{pbk4}\AgdaSpace{}%
\AgdaBound{sig1}\AgdaSpace{}%
\AgdaBound{sig2}\AgdaSpace{}%
\AgdaBound{x}\AgdaSpace{}%
\AgdaSymbol{|}\AgdaSpace{}%
\AgdaInductiveConstructor{true}\AgdaSpace{}%
\AgdaSymbol{|}\AgdaSpace{}%
\AgdaInductiveConstructor{false}\AgdaSpace{}%
\AgdaSymbol{|}\AgdaSpace{}%
\AgdaInductiveConstructor{false}\AgdaSpace{}%
\AgdaSymbol{|}\AgdaSpace{}%
\AgdaInductiveConstructor{true}\AgdaSpace{}%
\AgdaSymbol{=}\AgdaSpace{}%
\AgdaInductiveConstructor{inj₂}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaInductiveConstructor{inj₂}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaInductiveConstructor{inj₁}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaInductiveConstructor{conj}\AgdaSpace{}%
\AgdaInductiveConstructor{tt}\AgdaSpace{}%
\AgdaInductiveConstructor{tt}\AgdaSymbol{)))}\<%
\\
\>[0]\AgdaFunction{lemmaHoareTripleStackGeAux'Comb2-4}\AgdaSpace{}%
\AgdaBound{msg₂}\AgdaSpace{}%
\AgdaBound{pbk1}\AgdaSpace{}%
\AgdaBound{pbk2}\AgdaSpace{}%
\AgdaBound{pbk3}\AgdaSpace{}%
\AgdaBound{pbk4}\AgdaSpace{}%
\AgdaBound{sig1}\AgdaSpace{}%
\AgdaBound{sig2}\AgdaSpace{}%
\AgdaBound{x}\AgdaSpace{}%
\AgdaSymbol{|}\AgdaSpace{}%
\AgdaInductiveConstructor{true}\AgdaSpace{}%
\AgdaSymbol{|}\AgdaSpace{}%
\AgdaInductiveConstructor{false}\AgdaSpace{}%
\AgdaSymbol{|}\AgdaSpace{}%
\AgdaInductiveConstructor{true}\AgdaSpace{}%
\AgdaSymbol{=}\AgdaSpace{}%
\AgdaInductiveConstructor{inj₂}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaInductiveConstructor{inj₁}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaInductiveConstructor{conj}\AgdaSpace{}%
\AgdaInductiveConstructor{tt}\AgdaSpace{}%
\AgdaInductiveConstructor{tt}\AgdaSymbol{))}\<%
\\
\>[0]\AgdaFunction{lemmaHoareTripleStackGeAux'Comb2-4}\AgdaSpace{}%
\AgdaBound{msg₂}\AgdaSpace{}%
\AgdaBound{pbk1}\AgdaSpace{}%
\AgdaBound{pbk2}\AgdaSpace{}%
\AgdaBound{pbk3}\AgdaSpace{}%
\AgdaBound{pbk4}\AgdaSpace{}%
\AgdaBound{sig1}\AgdaSpace{}%
\AgdaBound{sig2}\AgdaSpace{}%
\AgdaBound{x}\AgdaSpace{}%
\AgdaSymbol{|}\AgdaSpace{}%
\AgdaInductiveConstructor{true}\AgdaSpace{}%
\AgdaSymbol{|}\AgdaSpace{}%
\AgdaInductiveConstructor{true}\AgdaSpace{}%
\AgdaSymbol{=}\AgdaSpace{}%
\AgdaInductiveConstructor{inj₁}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaInductiveConstructor{conj}\AgdaSpace{}%
\AgdaInductiveConstructor{tt}\AgdaSpace{}%
\AgdaInductiveConstructor{tt}\AgdaSymbol{)}\<%
\\
%
\\[\AgdaEmptyExtraSkip]%
%
\\[\AgdaEmptyExtraSkip]%
%
\\[\AgdaEmptyExtraSkip]%
%
\\[\AgdaEmptyExtraSkip]%
%
\\[\AgdaEmptyExtraSkip]%
\>[0]\AgdaFunction{lemmaHoareTripleStackGeAux'14}%
\>[3034I]\AgdaSymbol{:}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaBound{msg}\AgdaSpace{}%
\AgdaSymbol{:}\AgdaSpace{}%
\AgdaDatatype{Msg}\AgdaSymbol{)}\<%
\\
\>[3034I][@{}l@{\AgdaIndent{0}}]%
\>[31]\AgdaSymbol{(}\AgdaBound{pbk1}\AgdaSpace{}%
\AgdaBound{pbk2}\AgdaSpace{}%
\AgdaBound{pbk3}\AgdaSpace{}%
\AgdaBound{pbk4}\AgdaSpace{}%
\AgdaBound{pbk5}\AgdaSpace{}%
\AgdaBound{sig1}\AgdaSpace{}%
\AgdaBound{sig2}\AgdaSpace{}%
\AgdaBound{sig3}\AgdaSpace{}%
\AgdaSymbol{:}\AgdaSpace{}%
\AgdaDatatype{ℕ}\AgdaSymbol{)}\<%
\\
\>[.][@{}l@{}]\<[3034I]%
\>[30]\AgdaSymbol{→}\AgdaSpace{}%
\AgdaFunction{True}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaFunction{isSigned}%
\>[48]\AgdaBound{msg}\AgdaSpace{}%
\AgdaBound{sig1}\AgdaSpace{}%
\AgdaBound{pbk1}\AgdaSymbol{)}\<%
\\
%
\>[30]\AgdaSymbol{→}\AgdaSpace{}%
\AgdaFunction{True}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaFunction{isSigned}%
\>[48]\AgdaBound{msg}\AgdaSpace{}%
\AgdaBound{sig3}\AgdaSpace{}%
\AgdaBound{pbk3}\AgdaSymbol{)}\<%
\\
%
\>[30]\AgdaSymbol{→}\AgdaSpace{}%
\AgdaFunction{True}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaFunction{isSigned}%
\>[48]\AgdaBound{msg}\AgdaSpace{}%
\AgdaBound{sig2}\AgdaSpace{}%
\AgdaBound{pbk2}\AgdaSymbol{)}\<%
\\
%
\>[30]\AgdaSymbol{→}\AgdaSpace{}%
\AgdaFunction{True}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaFunction{compareSigsMultiSig}\AgdaSpace{}%
\AgdaBound{msg}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaSpace{}%
\AgdaBound{sig1}\AgdaSpace{}%
\AgdaOperator{\AgdaInductiveConstructor{∷}}\AgdaSpace{}%
\AgdaBound{sig2}\AgdaSpace{}%
\AgdaOperator{\AgdaInductiveConstructor{∷}}\AgdaSpace{}%
\AgdaBound{sig3}\AgdaSpace{}%
\AgdaOperator{\AgdaInductiveConstructor{∷}}\AgdaSpace{}%
\AgdaInductiveConstructor{[]}\AgdaSymbol{)}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaBound{pbk1}\AgdaSpace{}%
\AgdaOperator{\AgdaInductiveConstructor{∷}}\AgdaSpace{}%
\AgdaBound{pbk2}\AgdaSpace{}%
\AgdaOperator{\AgdaInductiveConstructor{∷}}\AgdaSpace{}%
\AgdaBound{pbk3}\AgdaSpace{}%
\AgdaOperator{\AgdaInductiveConstructor{∷}}\AgdaSpace{}%
\AgdaBound{pbk4}\AgdaSpace{}%
\AgdaOperator{\AgdaInductiveConstructor{∷}}\AgdaSpace{}%
\AgdaBound{pbk5}\AgdaSpace{}%
\AgdaOperator{\AgdaInductiveConstructor{∷}}\AgdaSpace{}%
\AgdaInductiveConstructor{[]}\AgdaSymbol{))}\<%
\\
\>[0]\AgdaFunction{lemmaHoareTripleStackGeAux'14}\AgdaSpace{}%
\AgdaBound{msg}\AgdaSpace{}%
\AgdaBound{pbk1}\AgdaSpace{}%
\AgdaBound{pbk2}\AgdaSpace{}%
\AgdaBound{pbk3}\AgdaSpace{}%
\AgdaBound{pbk4}\AgdaSpace{}%
\AgdaBound{pbk5}\AgdaSpace{}%
\AgdaBound{sig1}\AgdaSpace{}%
\AgdaBound{sig2}\AgdaSpace{}%
\AgdaBound{sig3}\AgdaSpace{}%
\AgdaBound{x}\AgdaSpace{}%
\AgdaBound{x₁}\AgdaSpace{}%
\AgdaBound{x₂}\AgdaSpace{}%
\AgdaKeyword{with}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaFunction{isSigned}%
\>[98]\AgdaBound{msg}\AgdaSpace{}%
\AgdaBound{sig1}\AgdaSpace{}%
\AgdaBound{pbk1}\AgdaSymbol{)}\<%
\\
\>[0]\AgdaFunction{lemmaHoareTripleStackGeAux'14}\AgdaSpace{}%
\AgdaBound{msg}\AgdaSpace{}%
\AgdaBound{pbk1}\AgdaSpace{}%
\AgdaBound{pbk2}\AgdaSpace{}%
\AgdaBound{pbk3}\AgdaSpace{}%
\AgdaBound{pbk4}\AgdaSpace{}%
\AgdaBound{pbk5}\AgdaSpace{}%
\AgdaBound{sig1}\AgdaSpace{}%
\AgdaBound{sig2}\AgdaSpace{}%
\AgdaBound{sig3}\AgdaSpace{}%
\AgdaBound{x}\AgdaSpace{}%
\AgdaBound{x₁}\AgdaSpace{}%
\AgdaBound{x₂}\AgdaSpace{}%
\AgdaSymbol{|}\AgdaSpace{}%
\AgdaInductiveConstructor{true}%
\>[90]\AgdaKeyword{with}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaFunction{isSigned}%
\>[106]\AgdaBound{msg}\AgdaSpace{}%
\AgdaBound{sig2}\AgdaSpace{}%
\AgdaBound{pbk2}\AgdaSymbol{)}\<%
\\
\>[0]\AgdaFunction{lemmaHoareTripleStackGeAux'14}\AgdaSpace{}%
\AgdaBound{msg}\AgdaSpace{}%
\AgdaBound{pbk1}\AgdaSpace{}%
\AgdaBound{pbk2}\AgdaSpace{}%
\AgdaBound{pbk3}\AgdaSpace{}%
\AgdaBound{pbk4}\AgdaSpace{}%
\AgdaBound{pbk5}\AgdaSpace{}%
\AgdaBound{sig1}\AgdaSpace{}%
\AgdaBound{sig2}\AgdaSpace{}%
\AgdaBound{sig3}\AgdaSpace{}%
\AgdaBound{x}\AgdaSpace{}%
\AgdaBound{x₁}\AgdaSpace{}%
\AgdaBound{x₂}\AgdaSpace{}%
\AgdaSymbol{|}\AgdaSpace{}%
\AgdaInductiveConstructor{true}\AgdaSpace{}%
\AgdaSymbol{|}\AgdaSpace{}%
\AgdaInductiveConstructor{true}\AgdaSpace{}%
\AgdaKeyword{with}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaFunction{isSigned}%
\>[112]\AgdaBound{msg}\AgdaSpace{}%
\AgdaBound{sig3}\AgdaSpace{}%
\AgdaBound{pbk3}\AgdaSymbol{)}\<%
\\
\>[0]\AgdaFunction{lemmaHoareTripleStackGeAux'14}\AgdaSpace{}%
\AgdaBound{msg}\AgdaSpace{}%
\AgdaBound{pbk1}\AgdaSpace{}%
\AgdaBound{pbk2}\AgdaSpace{}%
\AgdaBound{pbk3}\AgdaSpace{}%
\AgdaBound{pbk4}\AgdaSpace{}%
\AgdaBound{pbk5}\AgdaSpace{}%
\AgdaBound{sig1}\AgdaSpace{}%
\AgdaBound{sig2}\AgdaSpace{}%
\AgdaBound{sig3}\AgdaSpace{}%
\AgdaBound{x}\AgdaSpace{}%
\AgdaBound{x₁}\AgdaSpace{}%
\AgdaBound{x₂}\AgdaSpace{}%
\AgdaSymbol{|}\AgdaSpace{}%
\AgdaInductiveConstructor{true}\AgdaSpace{}%
\AgdaSymbol{|}\AgdaSpace{}%
\AgdaInductiveConstructor{true}\AgdaSpace{}%
\AgdaSymbol{|}\AgdaSpace{}%
\AgdaInductiveConstructor{true}\AgdaSpace{}%
\AgdaSymbol{=}\AgdaSpace{}%
\AgdaInductiveConstructor{tt}\<%
\\
%
\\[\AgdaEmptyExtraSkip]%
%
\\[\AgdaEmptyExtraSkip]%
\>[0]\AgdaFunction{lemmaHoareTripleStackGeAux'15}%
\>[3154I]\AgdaSymbol{:}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaBound{msg}\AgdaSpace{}%
\AgdaSymbol{:}\AgdaSpace{}%
\AgdaDatatype{Msg}\AgdaSymbol{)}\<%
\\
\>[3154I][@{}l@{\AgdaIndent{0}}]%
\>[31]\AgdaSymbol{(}\AgdaBound{pbk1}\AgdaSpace{}%
\AgdaBound{pbk2}\AgdaSpace{}%
\AgdaBound{pbk3}\AgdaSpace{}%
\AgdaBound{pbk4}\AgdaSpace{}%
\AgdaBound{pbk5}\AgdaSpace{}%
\AgdaBound{sig1}\AgdaSpace{}%
\AgdaBound{sig2}\AgdaSpace{}%
\AgdaBound{sig3}\AgdaSpace{}%
\AgdaSymbol{:}\AgdaSpace{}%
\AgdaDatatype{ℕ}\AgdaSymbol{)}\<%
\\
%
\>[31]\AgdaSymbol{→}\AgdaSpace{}%
\AgdaFunction{True}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaFunction{isSigned}%
\>[49]\AgdaBound{msg}\AgdaSpace{}%
\AgdaBound{sig3}\AgdaSpace{}%
\AgdaBound{pbk4}\AgdaSymbol{)}\<%
\\
\>[.][@{}l@{}]\<[3154I]%
\>[30]\AgdaSymbol{→}%
\>[33]\AgdaFunction{True}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaFunction{isSigned}%
\>[49]\AgdaBound{msg}\AgdaSpace{}%
\AgdaBound{sig2}\AgdaSpace{}%
\AgdaBound{pbk2}\AgdaSymbol{)}\<%
\\
%
\>[30]\AgdaSymbol{→}%
\>[33]\AgdaFunction{True}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaFunction{isSigned}%
\>[49]\AgdaBound{msg}\AgdaSpace{}%
\AgdaBound{sig1}\AgdaSpace{}%
\AgdaBound{pbk1}\AgdaSymbol{)}\<%
\\
\>[30][@{}l@{\AgdaIndent{0}}]%
\>[31]\AgdaSymbol{→}\AgdaSpace{}%
\AgdaFunction{True}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaFunction{compareSigsMultiSig}\AgdaSpace{}%
\AgdaBound{msg}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaSpace{}%
\AgdaBound{sig1}\AgdaSpace{}%
\AgdaOperator{\AgdaInductiveConstructor{∷}}\AgdaSpace{}%
\AgdaBound{sig2}\AgdaSpace{}%
\AgdaOperator{\AgdaInductiveConstructor{∷}}\AgdaSpace{}%
\AgdaBound{sig3}\AgdaSpace{}%
\AgdaOperator{\AgdaInductiveConstructor{∷}}\AgdaSpace{}%
\AgdaInductiveConstructor{[]}\AgdaSymbol{)}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaBound{pbk1}\AgdaSpace{}%
\AgdaOperator{\AgdaInductiveConstructor{∷}}\AgdaSpace{}%
\AgdaBound{pbk2}\AgdaSpace{}%
\AgdaOperator{\AgdaInductiveConstructor{∷}}\AgdaSpace{}%
\AgdaBound{pbk3}\AgdaSpace{}%
\AgdaOperator{\AgdaInductiveConstructor{∷}}\AgdaSpace{}%
\AgdaBound{pbk4}\AgdaSpace{}%
\AgdaOperator{\AgdaInductiveConstructor{∷}}\AgdaSpace{}%
\AgdaBound{pbk5}\AgdaSpace{}%
\AgdaOperator{\AgdaInductiveConstructor{∷}}\AgdaSpace{}%
\AgdaInductiveConstructor{[]}\AgdaSymbol{))}\<%
\\
\>[0]\AgdaFunction{lemmaHoareTripleStackGeAux'15}\AgdaSpace{}%
\AgdaBound{msg₁}\AgdaSpace{}%
\AgdaBound{pbk1}\AgdaSpace{}%
\AgdaBound{pbk2}\AgdaSpace{}%
\AgdaBound{pbk3}\AgdaSpace{}%
\AgdaBound{pbk4}\AgdaSpace{}%
\AgdaBound{pbk5}\AgdaSpace{}%
\AgdaBound{sig1}\AgdaSpace{}%
\AgdaBound{sig2}\AgdaSpace{}%
\AgdaBound{sig3}\AgdaSpace{}%
\AgdaBound{x}\AgdaSpace{}%
\AgdaBound{x₁}\AgdaSpace{}%
\AgdaBound{x₂}\AgdaSpace{}%
\AgdaKeyword{with}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaFunction{isSigned}%
\>[99]\AgdaBound{msg₁}\AgdaSpace{}%
\AgdaBound{sig1}\AgdaSpace{}%
\AgdaBound{pbk1}\AgdaSymbol{)}\<%
\\
\>[0]\AgdaFunction{lemmaHoareTripleStackGeAux'15}\AgdaSpace{}%
\AgdaBound{msg₁}\AgdaSpace{}%
\AgdaBound{pbk1}\AgdaSpace{}%
\AgdaBound{pbk2}\AgdaSpace{}%
\AgdaBound{pbk3}\AgdaSpace{}%
\AgdaBound{pbk4}\AgdaSpace{}%
\AgdaBound{pbk5}\AgdaSpace{}%
\AgdaBound{sig1}\AgdaSpace{}%
\AgdaBound{sig2}\AgdaSpace{}%
\AgdaBound{sig3}\AgdaSpace{}%
\AgdaBound{x}\AgdaSpace{}%
\AgdaBound{x₁}\AgdaSpace{}%
\AgdaBound{x₂}\AgdaSpace{}%
\AgdaSymbol{|}\AgdaSpace{}%
\AgdaInductiveConstructor{true}\AgdaSpace{}%
\AgdaKeyword{with}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaFunction{isSigned}%
\>[106]\AgdaBound{msg₁}\AgdaSpace{}%
\AgdaBound{sig2}\AgdaSpace{}%
\AgdaBound{pbk2}\AgdaSymbol{)}\<%
\\
\>[0]\AgdaFunction{lemmaHoareTripleStackGeAux'15}\AgdaSpace{}%
\AgdaBound{msg₁}\AgdaSpace{}%
\AgdaBound{pbk1}\AgdaSpace{}%
\AgdaBound{pbk2}\AgdaSpace{}%
\AgdaBound{pbk3}\AgdaSpace{}%
\AgdaBound{pbk4}\AgdaSpace{}%
\AgdaBound{pbk5}\AgdaSpace{}%
\AgdaBound{sig1}\AgdaSpace{}%
\AgdaBound{sig2}\AgdaSpace{}%
\AgdaBound{sig3}\AgdaSpace{}%
\AgdaBound{x}\AgdaSpace{}%
\AgdaBound{x₁}\AgdaSpace{}%
\AgdaBound{x₂}\AgdaSpace{}%
\AgdaSymbol{|}\AgdaSpace{}%
\AgdaInductiveConstructor{true}\AgdaSpace{}%
\AgdaSymbol{|}\AgdaSpace{}%
\AgdaInductiveConstructor{true}\AgdaSpace{}%
\AgdaKeyword{with}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaFunction{isSigned}%
\>[113]\AgdaBound{msg₁}\AgdaSpace{}%
\AgdaBound{sig3}\AgdaSpace{}%
\AgdaBound{pbk3}\AgdaSymbol{)}\<%
\\
\>[0]\AgdaFunction{lemmaHoareTripleStackGeAux'15}\AgdaSpace{}%
\AgdaBound{msg₁}\AgdaSpace{}%
\AgdaBound{pbk1}\AgdaSpace{}%
\AgdaBound{pbk2}\AgdaSpace{}%
\AgdaBound{pbk3}\AgdaSpace{}%
\AgdaBound{pbk4}\AgdaSpace{}%
\AgdaBound{pbk5}\AgdaSpace{}%
\AgdaBound{sig1}\AgdaSpace{}%
\AgdaBound{sig2}\AgdaSpace{}%
\AgdaBound{sig3}\AgdaSpace{}%
\AgdaBound{x}\AgdaSpace{}%
\AgdaBound{x₁}\AgdaSpace{}%
\AgdaBound{x₂}\AgdaSpace{}%
\AgdaSymbol{|}\AgdaSpace{}%
\AgdaInductiveConstructor{true}\AgdaSpace{}%
\AgdaSymbol{|}\AgdaSpace{}%
\AgdaInductiveConstructor{true}\AgdaSpace{}%
\AgdaSymbol{|}\AgdaSpace{}%
\AgdaInductiveConstructor{false}\AgdaSpace{}%
\AgdaKeyword{with}%
\>[111]\AgdaSymbol{(}\AgdaFunction{isSigned}%
\>[122]\AgdaBound{msg₁}\AgdaSpace{}%
\AgdaBound{sig3}\AgdaSpace{}%
\AgdaBound{pbk4}\AgdaSymbol{)}\<%
\\
\>[0]\AgdaFunction{lemmaHoareTripleStackGeAux'15}\AgdaSpace{}%
\AgdaBound{msg₁}\AgdaSpace{}%
\AgdaBound{pbk1}\AgdaSpace{}%
\AgdaBound{pbk2}\AgdaSpace{}%
\AgdaBound{pbk3}\AgdaSpace{}%
\AgdaBound{pbk4}\AgdaSpace{}%
\AgdaBound{pbk5}\AgdaSpace{}%
\AgdaBound{sig1}\AgdaSpace{}%
\AgdaBound{sig2}\AgdaSpace{}%
\AgdaBound{sig3}\AgdaSpace{}%
\AgdaBound{x}\AgdaSpace{}%
\AgdaBound{x₁}\AgdaSpace{}%
\AgdaBound{x₂}\AgdaSpace{}%
\AgdaSymbol{|}\AgdaSpace{}%
\AgdaInductiveConstructor{true}\AgdaSpace{}%
\AgdaSymbol{|}\AgdaSpace{}%
\AgdaInductiveConstructor{true}\AgdaSpace{}%
\AgdaSymbol{|}\AgdaSpace{}%
\AgdaInductiveConstructor{false}\AgdaSpace{}%
\AgdaSymbol{|}\AgdaSpace{}%
\AgdaInductiveConstructor{true}\AgdaSpace{}%
\AgdaSymbol{=}\AgdaSpace{}%
\AgdaInductiveConstructor{tt}\<%
\\
\>[0]\AgdaFunction{lemmaHoareTripleStackGeAux'15}\AgdaSpace{}%
\AgdaBound{msg₁}\AgdaSpace{}%
\AgdaBound{pbk1}\AgdaSpace{}%
\AgdaBound{pbk2}\AgdaSpace{}%
\AgdaBound{pbk3}\AgdaSpace{}%
\AgdaBound{pbk4}\AgdaSpace{}%
\AgdaBound{pbk5}\AgdaSpace{}%
\AgdaBound{sig1}\AgdaSpace{}%
\AgdaBound{sig2}\AgdaSpace{}%
\AgdaBound{sig3}\AgdaSpace{}%
\AgdaBound{x}\AgdaSpace{}%
\AgdaBound{x₁}\AgdaSpace{}%
\AgdaBound{x₂}\AgdaSpace{}%
\AgdaSymbol{|}\AgdaSpace{}%
\AgdaInductiveConstructor{true}\AgdaSpace{}%
\AgdaSymbol{|}\AgdaSpace{}%
\AgdaInductiveConstructor{true}\AgdaSpace{}%
\AgdaSymbol{|}\AgdaSpace{}%
\AgdaInductiveConstructor{true}\AgdaSpace{}%
\AgdaSymbol{=}\AgdaSpace{}%
\AgdaInductiveConstructor{tt}\<%
\\
%
\\[\AgdaEmptyExtraSkip]%
%
\\[\AgdaEmptyExtraSkip]%
\>[0]\AgdaFunction{lemmaHoareTripleStackGeAux'16}%
\>[3316I]\AgdaSymbol{:}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaBound{msg}\AgdaSpace{}%
\AgdaSymbol{:}\AgdaSpace{}%
\AgdaDatatype{Msg}\AgdaSymbol{)}\<%
\\
\>[3316I][@{}l@{\AgdaIndent{0}}]%
\>[31]\AgdaSymbol{(}\AgdaBound{pbk1}\AgdaSpace{}%
\AgdaBound{pbk2}\AgdaSpace{}%
\AgdaBound{pbk3}\AgdaSpace{}%
\AgdaBound{pbk4}\AgdaSpace{}%
\AgdaBound{pbk5}\AgdaSpace{}%
\AgdaBound{sig1}\AgdaSpace{}%
\AgdaBound{sig2}\AgdaSpace{}%
\AgdaBound{sig3}\AgdaSpace{}%
\AgdaSymbol{:}\AgdaSpace{}%
\AgdaDatatype{ℕ}\AgdaSymbol{)}\<%
\\
%
\>[31]\AgdaSymbol{→}\AgdaSpace{}%
\AgdaFunction{True}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaFunction{isSigned}%
\>[49]\AgdaBound{msg}\AgdaSpace{}%
\AgdaBound{sig3}\AgdaSpace{}%
\AgdaBound{pbk5}\AgdaSymbol{)}\<%
\\
\>[.][@{}l@{}]\<[3316I]%
\>[30]\AgdaSymbol{→}%
\>[33]\AgdaFunction{True}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaFunction{isSigned}%
\>[49]\AgdaBound{msg}\AgdaSpace{}%
\AgdaBound{sig2}\AgdaSpace{}%
\AgdaBound{pbk2}\AgdaSymbol{)}\<%
\\
\>[30][@{}l@{\AgdaIndent{0}}]%
\>[31]\AgdaSymbol{→}%
\>[34]\AgdaFunction{True}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaFunction{isSigned}%
\>[50]\AgdaBound{msg}\AgdaSpace{}%
\AgdaBound{sig1}\AgdaSpace{}%
\AgdaBound{pbk1}\AgdaSymbol{)}\<%
\\
%
\>[31]\AgdaSymbol{→}\AgdaSpace{}%
\AgdaFunction{True}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaFunction{compareSigsMultiSig}\AgdaSpace{}%
\AgdaBound{msg}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaSpace{}%
\AgdaBound{sig1}\AgdaSpace{}%
\AgdaOperator{\AgdaInductiveConstructor{∷}}\AgdaSpace{}%
\AgdaBound{sig2}\AgdaSpace{}%
\AgdaOperator{\AgdaInductiveConstructor{∷}}\AgdaSpace{}%
\AgdaBound{sig3}\AgdaSpace{}%
\AgdaOperator{\AgdaInductiveConstructor{∷}}\AgdaSpace{}%
\AgdaInductiveConstructor{[]}\AgdaSymbol{)}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaBound{pbk1}\AgdaSpace{}%
\AgdaOperator{\AgdaInductiveConstructor{∷}}\AgdaSpace{}%
\AgdaBound{pbk2}\AgdaSpace{}%
\AgdaOperator{\AgdaInductiveConstructor{∷}}\AgdaSpace{}%
\AgdaBound{pbk3}\AgdaSpace{}%
\AgdaOperator{\AgdaInductiveConstructor{∷}}\AgdaSpace{}%
\AgdaBound{pbk4}\AgdaSpace{}%
\AgdaOperator{\AgdaInductiveConstructor{∷}}\AgdaSpace{}%
\AgdaBound{pbk5}\AgdaSpace{}%
\AgdaOperator{\AgdaInductiveConstructor{∷}}\AgdaSpace{}%
\AgdaInductiveConstructor{[]}\AgdaSymbol{))}\<%
\\
\>[0]\AgdaFunction{lemmaHoareTripleStackGeAux'16}\AgdaSpace{}%
\AgdaBound{msg₁}\AgdaSpace{}%
\AgdaBound{pbk1}\AgdaSpace{}%
\AgdaBound{pbk2}\AgdaSpace{}%
\AgdaBound{pbk3}\AgdaSpace{}%
\AgdaBound{pbk4}\AgdaSpace{}%
\AgdaBound{pbk5}\AgdaSpace{}%
\AgdaBound{sig1}\AgdaSpace{}%
\AgdaBound{sig2}\AgdaSpace{}%
\AgdaBound{sig3}\AgdaSpace{}%
\AgdaBound{x}\AgdaSpace{}%
\AgdaBound{x₁}\AgdaSpace{}%
\AgdaBound{x₂}\AgdaSpace{}%
\AgdaKeyword{with}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaFunction{isSigned}%
\>[99]\AgdaBound{msg₁}\AgdaSpace{}%
\AgdaBound{sig1}\AgdaSpace{}%
\AgdaBound{pbk1}\AgdaSymbol{)}\<%
\\
\>[0]\AgdaFunction{lemmaHoareTripleStackGeAux'16}\AgdaSpace{}%
\AgdaBound{msg₁}\AgdaSpace{}%
\AgdaBound{pbk1}\AgdaSpace{}%
\AgdaBound{pbk2}\AgdaSpace{}%
\AgdaBound{pbk3}\AgdaSpace{}%
\AgdaBound{pbk4}\AgdaSpace{}%
\AgdaBound{pbk5}\AgdaSpace{}%
\AgdaBound{sig1}\AgdaSpace{}%
\AgdaBound{sig2}\AgdaSpace{}%
\AgdaBound{sig3}\AgdaSpace{}%
\AgdaBound{x}\AgdaSpace{}%
\AgdaBound{x₁}\AgdaSpace{}%
\AgdaBound{x₂}\AgdaSpace{}%
\AgdaSymbol{|}\AgdaSpace{}%
\AgdaInductiveConstructor{true}\AgdaSpace{}%
\AgdaKeyword{with}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaFunction{isSigned}%
\>[106]\AgdaBound{msg₁}\AgdaSpace{}%
\AgdaBound{sig2}\AgdaSpace{}%
\AgdaBound{pbk2}\AgdaSymbol{)}\<%
\\
\>[0]\AgdaFunction{lemmaHoareTripleStackGeAux'16}\AgdaSpace{}%
\AgdaBound{msg₁}\AgdaSpace{}%
\AgdaBound{pbk1}\AgdaSpace{}%
\AgdaBound{pbk2}\AgdaSpace{}%
\AgdaBound{pbk3}\AgdaSpace{}%
\AgdaBound{pbk4}\AgdaSpace{}%
\AgdaBound{pbk5}\AgdaSpace{}%
\AgdaBound{sig1}\AgdaSpace{}%
\AgdaBound{sig2}\AgdaSpace{}%
\AgdaBound{sig3}\AgdaSpace{}%
\AgdaBound{x}\AgdaSpace{}%
\AgdaBound{x₁}\AgdaSpace{}%
\AgdaBound{x₂}\AgdaSpace{}%
\AgdaSymbol{|}\AgdaSpace{}%
\AgdaInductiveConstructor{true}\AgdaSpace{}%
\AgdaSymbol{|}\AgdaSpace{}%
\AgdaInductiveConstructor{true}\AgdaSpace{}%
\AgdaKeyword{with}%
\>[103]\AgdaSymbol{(}\AgdaFunction{isSigned}%
\>[114]\AgdaBound{msg₁}\AgdaSpace{}%
\AgdaBound{sig3}\AgdaSpace{}%
\AgdaBound{pbk3}\AgdaSymbol{)}\<%
\\
\>[0]\AgdaFunction{lemmaHoareTripleStackGeAux'16}\AgdaSpace{}%
\AgdaBound{msg₁}\AgdaSpace{}%
\AgdaBound{pbk1}\AgdaSpace{}%
\AgdaBound{pbk2}\AgdaSpace{}%
\AgdaBound{pbk3}\AgdaSpace{}%
\AgdaBound{pbk4}\AgdaSpace{}%
\AgdaBound{pbk5}\AgdaSpace{}%
\AgdaBound{sig1}\AgdaSpace{}%
\AgdaBound{sig2}\AgdaSpace{}%
\AgdaBound{sig3}\AgdaSpace{}%
\AgdaBound{x}\AgdaSpace{}%
\AgdaBound{x₁}\AgdaSpace{}%
\AgdaBound{x₂}\AgdaSpace{}%
\AgdaSymbol{|}\AgdaSpace{}%
\AgdaInductiveConstructor{true}\AgdaSpace{}%
\AgdaSymbol{|}\AgdaSpace{}%
\AgdaInductiveConstructor{true}\AgdaSpace{}%
\AgdaSymbol{|}\AgdaSpace{}%
\AgdaInductiveConstructor{false}\AgdaSpace{}%
\AgdaKeyword{with}%
\>[111]\AgdaSymbol{(}\AgdaFunction{isSigned}%
\>[122]\AgdaBound{msg₁}\AgdaSpace{}%
\AgdaBound{sig3}\AgdaSpace{}%
\AgdaBound{pbk4}\AgdaSymbol{)}\<%
\\
\>[0]\AgdaFunction{lemmaHoareTripleStackGeAux'16}\AgdaSpace{}%
\AgdaBound{msg₁}\AgdaSpace{}%
\AgdaBound{pbk1}\AgdaSpace{}%
\AgdaBound{pbk2}\AgdaSpace{}%
\AgdaBound{pbk3}\AgdaSpace{}%
\AgdaBound{pbk4}\AgdaSpace{}%
\AgdaBound{pbk5}\AgdaSpace{}%
\AgdaBound{sig1}\AgdaSpace{}%
\AgdaBound{sig2}\AgdaSpace{}%
\AgdaBound{sig3}\AgdaSpace{}%
\AgdaBound{x}\AgdaSpace{}%
\AgdaBound{x₁}\AgdaSpace{}%
\AgdaBound{x₂}\AgdaSpace{}%
\AgdaSymbol{|}\AgdaSpace{}%
\AgdaInductiveConstructor{true}\AgdaSpace{}%
\AgdaSymbol{|}\AgdaSpace{}%
\AgdaInductiveConstructor{true}\AgdaSpace{}%
\AgdaSymbol{|}\AgdaSpace{}%
\AgdaInductiveConstructor{false}\AgdaSpace{}%
\AgdaSymbol{|}\AgdaSpace{}%
\AgdaInductiveConstructor{false}\AgdaSpace{}%
\AgdaKeyword{with}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaFunction{isSigned}%
\>[129]\AgdaBound{msg₁}\AgdaSpace{}%
\AgdaBound{sig3}\AgdaSpace{}%
\AgdaBound{pbk5}\AgdaSymbol{)}\<%
\\
\>[0]\AgdaFunction{lemmaHoareTripleStackGeAux'16}\AgdaSpace{}%
\AgdaBound{msg₁}\AgdaSpace{}%
\AgdaBound{pbk1}\AgdaSpace{}%
\AgdaBound{pbk2}\AgdaSpace{}%
\AgdaBound{pbk3}\AgdaSpace{}%
\AgdaBound{pbk4}\AgdaSpace{}%
\AgdaBound{pbk5}\AgdaSpace{}%
\AgdaBound{sig1}\AgdaSpace{}%
\AgdaBound{sig2}\AgdaSpace{}%
\AgdaBound{sig3}\AgdaSpace{}%
\AgdaBound{x}\AgdaSpace{}%
\AgdaBound{x₁}\AgdaSpace{}%
\AgdaBound{x₂}\AgdaSpace{}%
\AgdaSymbol{|}\AgdaSpace{}%
\AgdaInductiveConstructor{true}\AgdaSpace{}%
\AgdaSymbol{|}\AgdaSpace{}%
\AgdaInductiveConstructor{true}\AgdaSpace{}%
\AgdaSymbol{|}\AgdaSpace{}%
\AgdaInductiveConstructor{false}\AgdaSpace{}%
\AgdaSymbol{|}\AgdaSpace{}%
\AgdaInductiveConstructor{false}\AgdaSpace{}%
\AgdaSymbol{|}\AgdaSpace{}%
\AgdaInductiveConstructor{true}\AgdaSpace{}%
\AgdaSymbol{=}\AgdaSpace{}%
\AgdaInductiveConstructor{tt}\<%
\\
\>[0]\AgdaFunction{lemmaHoareTripleStackGeAux'16}\AgdaSpace{}%
\AgdaBound{msg₁}\AgdaSpace{}%
\AgdaBound{pbk1}\AgdaSpace{}%
\AgdaBound{pbk2}\AgdaSpace{}%
\AgdaBound{pbk3}\AgdaSpace{}%
\AgdaBound{pbk4}\AgdaSpace{}%
\AgdaBound{pbk5}\AgdaSpace{}%
\AgdaBound{sig1}\AgdaSpace{}%
\AgdaBound{sig2}\AgdaSpace{}%
\AgdaBound{sig3}\AgdaSpace{}%
\AgdaBound{x}\AgdaSpace{}%
\AgdaBound{x₁}\AgdaSpace{}%
\AgdaBound{x₂}\AgdaSpace{}%
\AgdaSymbol{|}\AgdaSpace{}%
\AgdaInductiveConstructor{true}\AgdaSpace{}%
\AgdaSymbol{|}\AgdaSpace{}%
\AgdaInductiveConstructor{true}\AgdaSpace{}%
\AgdaSymbol{|}\AgdaSpace{}%
\AgdaInductiveConstructor{false}\AgdaSpace{}%
\AgdaSymbol{|}\AgdaSpace{}%
\AgdaInductiveConstructor{true}\AgdaSpace{}%
\AgdaSymbol{=}\AgdaSpace{}%
\AgdaInductiveConstructor{tt}\<%
\\
\>[0]\AgdaFunction{lemmaHoareTripleStackGeAux'16}\AgdaSpace{}%
\AgdaBound{msg₁}\AgdaSpace{}%
\AgdaBound{pbk1}\AgdaSpace{}%
\AgdaBound{pbk2}\AgdaSpace{}%
\AgdaBound{pbk3}\AgdaSpace{}%
\AgdaBound{pbk4}\AgdaSpace{}%
\AgdaBound{pbk5}\AgdaSpace{}%
\AgdaBound{sig1}\AgdaSpace{}%
\AgdaBound{sig2}\AgdaSpace{}%
\AgdaBound{sig3}\AgdaSpace{}%
\AgdaBound{x}\AgdaSpace{}%
\AgdaBound{x₁}\AgdaSpace{}%
\AgdaBound{x₂}\AgdaSpace{}%
\AgdaSymbol{|}\AgdaSpace{}%
\AgdaInductiveConstructor{true}\AgdaSpace{}%
\AgdaSymbol{|}\AgdaSpace{}%
\AgdaInductiveConstructor{true}\AgdaSpace{}%
\AgdaSymbol{|}\AgdaSpace{}%
\AgdaInductiveConstructor{true}\AgdaSpace{}%
\AgdaSymbol{=}\AgdaSpace{}%
\AgdaInductiveConstructor{tt}\<%
\\
%
\\[\AgdaEmptyExtraSkip]%
%
\\[\AgdaEmptyExtraSkip]%
\>[0]\AgdaFunction{lemmaHoareTripleStackGeAux'17}%
\>[3525I]\AgdaSymbol{:}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaBound{msg}\AgdaSpace{}%
\AgdaSymbol{:}\AgdaSpace{}%
\AgdaDatatype{Msg}\AgdaSymbol{)}\<%
\\
\>[3525I][@{}l@{\AgdaIndent{0}}]%
\>[31]\AgdaSymbol{(}\AgdaBound{pbk1}\AgdaSpace{}%
\AgdaBound{pbk2}\AgdaSpace{}%
\AgdaBound{pbk3}\AgdaSpace{}%
\AgdaBound{pbk4}\AgdaSpace{}%
\AgdaBound{pbk5}\AgdaSpace{}%
\AgdaBound{sig1}\AgdaSpace{}%
\AgdaBound{sig2}\AgdaSpace{}%
\AgdaBound{sig3}\AgdaSpace{}%
\AgdaSymbol{:}\AgdaSpace{}%
\AgdaDatatype{ℕ}\AgdaSymbol{)}\<%
\\
%
\>[31]\AgdaSymbol{→}\AgdaSpace{}%
\AgdaFunction{True}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaFunction{isSigned}%
\>[49]\AgdaBound{msg}\AgdaSpace{}%
\AgdaBound{sig3}\AgdaSpace{}%
\AgdaBound{pbk4}\AgdaSymbol{)}\<%
\\
\>[.][@{}l@{}]\<[3525I]%
\>[30]\AgdaSymbol{→}%
\>[33]\AgdaFunction{True}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaFunction{isSigned}%
\>[49]\AgdaBound{msg}\AgdaSpace{}%
\AgdaBound{sig2}\AgdaSpace{}%
\AgdaBound{pbk3}\AgdaSymbol{)}\<%
\\
\>[30][@{}l@{\AgdaIndent{0}}]%
\>[31]\AgdaSymbol{→}%
\>[34]\AgdaFunction{True}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaFunction{isSigned}%
\>[50]\AgdaBound{msg}\AgdaSpace{}%
\AgdaBound{sig1}\AgdaSpace{}%
\AgdaBound{pbk1}\AgdaSymbol{)}\<%
\\
%
\>[31]\AgdaSymbol{→}\AgdaSpace{}%
\AgdaFunction{True}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaFunction{compareSigsMultiSig}\AgdaSpace{}%
\AgdaBound{msg}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaSpace{}%
\AgdaBound{sig1}\AgdaSpace{}%
\AgdaOperator{\AgdaInductiveConstructor{∷}}\AgdaSpace{}%
\AgdaBound{sig2}\AgdaSpace{}%
\AgdaOperator{\AgdaInductiveConstructor{∷}}\AgdaSpace{}%
\AgdaBound{sig3}\AgdaSpace{}%
\AgdaOperator{\AgdaInductiveConstructor{∷}}\AgdaSpace{}%
\AgdaInductiveConstructor{[]}\AgdaSymbol{)}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaBound{pbk1}\AgdaSpace{}%
\AgdaOperator{\AgdaInductiveConstructor{∷}}\AgdaSpace{}%
\AgdaBound{pbk2}\AgdaSpace{}%
\AgdaOperator{\AgdaInductiveConstructor{∷}}\AgdaSpace{}%
\AgdaBound{pbk3}\AgdaSpace{}%
\AgdaOperator{\AgdaInductiveConstructor{∷}}\AgdaSpace{}%
\AgdaBound{pbk4}\AgdaSpace{}%
\AgdaOperator{\AgdaInductiveConstructor{∷}}\AgdaSpace{}%
\AgdaBound{pbk5}\AgdaSpace{}%
\AgdaOperator{\AgdaInductiveConstructor{∷}}\AgdaSpace{}%
\AgdaInductiveConstructor{[]}\AgdaSymbol{))}\<%
\\
\>[0]\AgdaFunction{lemmaHoareTripleStackGeAux'17}\AgdaSpace{}%
\AgdaBound{msg₁}\AgdaSpace{}%
\AgdaBound{pbk1}\AgdaSpace{}%
\AgdaBound{pbk2}\AgdaSpace{}%
\AgdaBound{pbk3}\AgdaSpace{}%
\AgdaBound{pbk4}\AgdaSpace{}%
\AgdaBound{pbk5}\AgdaSpace{}%
\AgdaBound{sig1}\AgdaSpace{}%
\AgdaBound{sig2}\AgdaSpace{}%
\AgdaBound{sig3}\AgdaSpace{}%
\AgdaBound{x}\AgdaSpace{}%
\AgdaBound{x₁}\AgdaSpace{}%
\AgdaBound{x₂}\AgdaSpace{}%
\AgdaKeyword{with}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaFunction{isSigned}%
\>[99]\AgdaBound{msg₁}\AgdaSpace{}%
\AgdaBound{sig1}\AgdaSpace{}%
\AgdaBound{pbk1}\AgdaSymbol{)}\<%
\\
\>[0]\AgdaFunction{lemmaHoareTripleStackGeAux'17}\AgdaSpace{}%
\AgdaBound{msg₁}\AgdaSpace{}%
\AgdaBound{pbk1}\AgdaSpace{}%
\AgdaBound{pbk2}\AgdaSpace{}%
\AgdaBound{pbk3}\AgdaSpace{}%
\AgdaBound{pbk4}\AgdaSpace{}%
\AgdaBound{pbk5}\AgdaSpace{}%
\AgdaBound{sig1}\AgdaSpace{}%
\AgdaBound{sig2}\AgdaSpace{}%
\AgdaBound{sig3}\AgdaSpace{}%
\AgdaBound{x}\AgdaSpace{}%
\AgdaBound{x₁}\AgdaSpace{}%
\AgdaBound{x₂}\AgdaSpace{}%
\AgdaSymbol{|}\AgdaSpace{}%
\AgdaInductiveConstructor{true}\AgdaSpace{}%
\AgdaKeyword{with}%
\>[96]\AgdaSymbol{(}\AgdaFunction{isSigned}%
\>[107]\AgdaBound{msg₁}\AgdaSpace{}%
\AgdaBound{sig2}\AgdaSpace{}%
\AgdaBound{pbk2}\AgdaSymbol{)}\<%
\\
\>[0]\AgdaFunction{lemmaHoareTripleStackGeAux'17}\AgdaSpace{}%
\AgdaBound{msg₁}\AgdaSpace{}%
\AgdaBound{pbk1}\AgdaSpace{}%
\AgdaBound{pbk2}\AgdaSpace{}%
\AgdaBound{pbk3}\AgdaSpace{}%
\AgdaBound{pbk4}\AgdaSpace{}%
\AgdaBound{pbk5}\AgdaSpace{}%
\AgdaBound{sig1}\AgdaSpace{}%
\AgdaBound{sig2}\AgdaSpace{}%
\AgdaBound{sig3}\AgdaSpace{}%
\AgdaBound{x}\AgdaSpace{}%
\AgdaBound{x₁}\AgdaSpace{}%
\AgdaBound{x₂}\AgdaSpace{}%
\AgdaSymbol{|}\AgdaSpace{}%
\AgdaInductiveConstructor{true}\AgdaSpace{}%
\AgdaSymbol{|}\AgdaSpace{}%
\AgdaInductiveConstructor{false}\AgdaSpace{}%
\AgdaKeyword{with}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaFunction{isSigned}%
\>[114]\AgdaBound{msg₁}\AgdaSpace{}%
\AgdaBound{sig2}\AgdaSpace{}%
\AgdaBound{pbk3}\AgdaSymbol{)}\<%
\\
\>[0]\AgdaFunction{lemmaHoareTripleStackGeAux'17}\AgdaSpace{}%
\AgdaBound{msg₁}\AgdaSpace{}%
\AgdaBound{pbk1}\AgdaSpace{}%
\AgdaBound{pbk2}\AgdaSpace{}%
\AgdaBound{pbk3}\AgdaSpace{}%
\AgdaBound{pbk4}\AgdaSpace{}%
\AgdaBound{pbk5}\AgdaSpace{}%
\AgdaBound{sig1}\AgdaSpace{}%
\AgdaBound{sig2}\AgdaSpace{}%
\AgdaBound{sig3}\AgdaSpace{}%
\AgdaBound{x}\AgdaSpace{}%
\AgdaBound{x₁}\AgdaSpace{}%
\AgdaBound{x₂}\AgdaSpace{}%
\AgdaSymbol{|}\AgdaSpace{}%
\AgdaInductiveConstructor{true}\AgdaSpace{}%
\AgdaSymbol{|}\AgdaSpace{}%
\AgdaInductiveConstructor{false}\AgdaSpace{}%
\AgdaSymbol{|}\AgdaSpace{}%
\AgdaInductiveConstructor{true}\AgdaSpace{}%
\AgdaKeyword{with}%
\>[111]\AgdaSymbol{(}\AgdaFunction{isSigned}%
\>[122]\AgdaBound{msg₁}\AgdaSpace{}%
\AgdaBound{sig3}\AgdaSpace{}%
\AgdaBound{pbk4}\AgdaSymbol{)}\<%
\\
\>[0]\AgdaFunction{lemmaHoareTripleStackGeAux'17}\AgdaSpace{}%
\AgdaBound{msg₁}\AgdaSpace{}%
\AgdaBound{pbk1}\AgdaSpace{}%
\AgdaBound{pbk2}\AgdaSpace{}%
\AgdaBound{pbk3}\AgdaSpace{}%
\AgdaBound{pbk4}\AgdaSpace{}%
\AgdaBound{pbk5}\AgdaSpace{}%
\AgdaBound{sig1}\AgdaSpace{}%
\AgdaBound{sig2}\AgdaSpace{}%
\AgdaBound{sig3}\AgdaSpace{}%
\AgdaBound{x}\AgdaSpace{}%
\AgdaBound{x₁}\AgdaSpace{}%
\AgdaBound{x₂}\AgdaSpace{}%
\AgdaSymbol{|}\AgdaSpace{}%
\AgdaInductiveConstructor{true}\AgdaSpace{}%
\AgdaSymbol{|}\AgdaSpace{}%
\AgdaInductiveConstructor{false}\AgdaSpace{}%
\AgdaSymbol{|}\AgdaSpace{}%
\AgdaInductiveConstructor{true}\AgdaSpace{}%
\AgdaSymbol{|}\AgdaSpace{}%
\AgdaInductiveConstructor{true}\AgdaSpace{}%
\AgdaSymbol{=}\AgdaSpace{}%
\AgdaInductiveConstructor{tt}\<%
\\
\>[0]\AgdaFunction{lemmaHoareTripleStackGeAux'17}\AgdaSpace{}%
\AgdaBound{msg₁}\AgdaSpace{}%
\AgdaBound{pbk1}\AgdaSpace{}%
\AgdaBound{pbk2}\AgdaSpace{}%
\AgdaBound{pbk3}\AgdaSpace{}%
\AgdaBound{pbk4}\AgdaSpace{}%
\AgdaBound{pbk5}\AgdaSpace{}%
\AgdaBound{sig1}\AgdaSpace{}%
\AgdaBound{sig2}\AgdaSpace{}%
\AgdaBound{sig3}\AgdaSpace{}%
\AgdaBound{x}\AgdaSpace{}%
\AgdaBound{x₁}\AgdaSpace{}%
\AgdaBound{x₂}\AgdaSpace{}%
\AgdaSymbol{|}\AgdaSpace{}%
\AgdaInductiveConstructor{true}\AgdaSpace{}%
\AgdaSymbol{|}\AgdaSpace{}%
\AgdaInductiveConstructor{true}\AgdaSpace{}%
\AgdaKeyword{with}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaFunction{isSigned}%
\>[113]\AgdaBound{msg₁}\AgdaSpace{}%
\AgdaBound{sig3}\AgdaSpace{}%
\AgdaBound{pbk3}\AgdaSymbol{)}\<%
\\
\>[0]\AgdaFunction{lemmaHoareTripleStackGeAux'17}\AgdaSpace{}%
\AgdaBound{msg₁}\AgdaSpace{}%
\AgdaBound{pbk1}\AgdaSpace{}%
\AgdaBound{pbk2}\AgdaSpace{}%
\AgdaBound{pbk3}\AgdaSpace{}%
\AgdaBound{pbk4}\AgdaSpace{}%
\AgdaBound{pbk5}\AgdaSpace{}%
\AgdaBound{sig1}\AgdaSpace{}%
\AgdaBound{sig2}\AgdaSpace{}%
\AgdaBound{sig3}\AgdaSpace{}%
\AgdaBound{x}\AgdaSpace{}%
\AgdaBound{x₁}\AgdaSpace{}%
\AgdaBound{x₂}\AgdaSpace{}%
\AgdaSymbol{|}\AgdaSpace{}%
\AgdaInductiveConstructor{true}\AgdaSpace{}%
\AgdaSymbol{|}\AgdaSpace{}%
\AgdaInductiveConstructor{true}\AgdaSpace{}%
\AgdaSymbol{|}\AgdaSpace{}%
\AgdaInductiveConstructor{false}\AgdaSpace{}%
\AgdaKeyword{with}%
\>[111]\AgdaSymbol{(}\AgdaFunction{isSigned}%
\>[122]\AgdaBound{msg₁}\AgdaSpace{}%
\AgdaBound{sig3}\AgdaSpace{}%
\AgdaBound{pbk4}\AgdaSymbol{)}\<%
\\
\>[0]\AgdaFunction{lemmaHoareTripleStackGeAux'17}\AgdaSpace{}%
\AgdaBound{msg₁}\AgdaSpace{}%
\AgdaBound{pbk1}\AgdaSpace{}%
\AgdaBound{pbk2}\AgdaSpace{}%
\AgdaBound{pbk3}\AgdaSpace{}%
\AgdaBound{pbk4}\AgdaSpace{}%
\AgdaBound{pbk5}\AgdaSpace{}%
\AgdaBound{sig1}\AgdaSpace{}%
\AgdaBound{sig2}\AgdaSpace{}%
\AgdaBound{sig3}\AgdaSpace{}%
\AgdaBound{x}\AgdaSpace{}%
\AgdaBound{x₁}\AgdaSpace{}%
\AgdaBound{x₂}\AgdaSpace{}%
\AgdaSymbol{|}\AgdaSpace{}%
\AgdaInductiveConstructor{true}\AgdaSpace{}%
\AgdaSymbol{|}\AgdaSpace{}%
\AgdaInductiveConstructor{true}\AgdaSpace{}%
\AgdaSymbol{|}\AgdaSpace{}%
\AgdaInductiveConstructor{false}\AgdaSpace{}%
\AgdaSymbol{|}\AgdaSpace{}%
\AgdaInductiveConstructor{true}\AgdaSpace{}%
\AgdaSymbol{=}\AgdaSpace{}%
\AgdaInductiveConstructor{tt}\<%
\\
\>[0]\AgdaFunction{lemmaHoareTripleStackGeAux'17}\AgdaSpace{}%
\AgdaBound{msg₁}\AgdaSpace{}%
\AgdaBound{pbk1}\AgdaSpace{}%
\AgdaBound{pbk2}\AgdaSpace{}%
\AgdaBound{pbk3}\AgdaSpace{}%
\AgdaBound{pbk4}\AgdaSpace{}%
\AgdaBound{pbk5}\AgdaSpace{}%
\AgdaBound{sig1}\AgdaSpace{}%
\AgdaBound{sig2}\AgdaSpace{}%
\AgdaBound{sig3}\AgdaSpace{}%
\AgdaBound{x}\AgdaSpace{}%
\AgdaBound{x₁}\AgdaSpace{}%
\AgdaBound{x₂}\AgdaSpace{}%
\AgdaSymbol{|}\AgdaSpace{}%
\AgdaInductiveConstructor{true}\AgdaSpace{}%
\AgdaSymbol{|}\AgdaSpace{}%
\AgdaInductiveConstructor{true}\AgdaSpace{}%
\AgdaSymbol{|}\AgdaSpace{}%
\AgdaInductiveConstructor{true}\AgdaSpace{}%
\AgdaSymbol{=}\AgdaSpace{}%
\AgdaInductiveConstructor{tt}\<%
\\
%
\\[\AgdaEmptyExtraSkip]%
%
\\[\AgdaEmptyExtraSkip]%
\>[0]\AgdaFunction{lemmaHoareTripleStackGeAux'18}%
\>[3749I]\AgdaSymbol{:}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaBound{msg}\AgdaSpace{}%
\AgdaSymbol{:}\AgdaSpace{}%
\AgdaDatatype{Msg}\AgdaSymbol{)}\<%
\\
\>[3749I][@{}l@{\AgdaIndent{0}}]%
\>[31]\AgdaSymbol{(}\AgdaBound{pbk1}\AgdaSpace{}%
\AgdaBound{pbk2}\AgdaSpace{}%
\AgdaBound{pbk3}\AgdaSpace{}%
\AgdaBound{pbk4}\AgdaSpace{}%
\AgdaBound{pbk5}\AgdaSpace{}%
\AgdaBound{sig1}\AgdaSpace{}%
\AgdaBound{sig2}\AgdaSpace{}%
\AgdaBound{sig3}\AgdaSpace{}%
\AgdaSymbol{:}\AgdaSpace{}%
\AgdaDatatype{ℕ}\AgdaSymbol{)}\<%
\\
%
\>[31]\AgdaSymbol{→}\AgdaSpace{}%
\AgdaFunction{True}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaFunction{isSigned}%
\>[49]\AgdaBound{msg}\AgdaSpace{}%
\AgdaBound{sig3}\AgdaSpace{}%
\AgdaBound{pbk5}\AgdaSymbol{)}\<%
\\
\>[.][@{}l@{}]\<[3749I]%
\>[30]\AgdaSymbol{→}%
\>[33]\AgdaFunction{True}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaFunction{isSigned}%
\>[49]\AgdaBound{msg}\AgdaSpace{}%
\AgdaBound{sig2}\AgdaSpace{}%
\AgdaBound{pbk3}\AgdaSymbol{)}\<%
\\
%
\>[30]\AgdaSymbol{→}%
\>[33]\AgdaFunction{True}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaFunction{isSigned}%
\>[49]\AgdaBound{msg}\AgdaSpace{}%
\AgdaBound{sig1}\AgdaSpace{}%
\AgdaBound{pbk1}\AgdaSymbol{)}\<%
\\
\>[30][@{}l@{\AgdaIndent{0}}]%
\>[31]\AgdaSymbol{→}\AgdaSpace{}%
\AgdaFunction{True}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaFunction{compareSigsMultiSig}\AgdaSpace{}%
\AgdaBound{msg}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaSpace{}%
\AgdaBound{sig1}\AgdaSpace{}%
\AgdaOperator{\AgdaInductiveConstructor{∷}}\AgdaSpace{}%
\AgdaBound{sig2}\AgdaSpace{}%
\AgdaOperator{\AgdaInductiveConstructor{∷}}\AgdaSpace{}%
\AgdaBound{sig3}\AgdaSpace{}%
\AgdaOperator{\AgdaInductiveConstructor{∷}}\AgdaSpace{}%
\AgdaInductiveConstructor{[]}\AgdaSymbol{)}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaBound{pbk1}\AgdaSpace{}%
\AgdaOperator{\AgdaInductiveConstructor{∷}}\AgdaSpace{}%
\AgdaBound{pbk2}\AgdaSpace{}%
\AgdaOperator{\AgdaInductiveConstructor{∷}}\AgdaSpace{}%
\AgdaBound{pbk3}\AgdaSpace{}%
\AgdaOperator{\AgdaInductiveConstructor{∷}}\AgdaSpace{}%
\AgdaBound{pbk4}\AgdaSpace{}%
\AgdaOperator{\AgdaInductiveConstructor{∷}}\AgdaSpace{}%
\AgdaBound{pbk5}\AgdaSpace{}%
\AgdaOperator{\AgdaInductiveConstructor{∷}}\AgdaSpace{}%
\AgdaInductiveConstructor{[]}\AgdaSymbol{))}\<%
\\
\>[0]\AgdaFunction{lemmaHoareTripleStackGeAux'18}\AgdaSpace{}%
\AgdaBound{msg₁}\AgdaSpace{}%
\AgdaBound{pbk1}\AgdaSpace{}%
\AgdaBound{pbk2}\AgdaSpace{}%
\AgdaBound{pbk3}\AgdaSpace{}%
\AgdaBound{pbk4}\AgdaSpace{}%
\AgdaBound{pbk5}\AgdaSpace{}%
\AgdaBound{sig1}\AgdaSpace{}%
\AgdaBound{sig2}\AgdaSpace{}%
\AgdaBound{sig3}\AgdaSpace{}%
\AgdaBound{x}\AgdaSpace{}%
\AgdaBound{x₁}\AgdaSpace{}%
\AgdaBound{x₂}\AgdaSpace{}%
\AgdaKeyword{with}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaFunction{isSigned}%
\>[99]\AgdaBound{msg₁}\AgdaSpace{}%
\AgdaBound{sig1}\AgdaSpace{}%
\AgdaBound{pbk1}\AgdaSymbol{)}\<%
\\
\>[0]\AgdaFunction{lemmaHoareTripleStackGeAux'18}\AgdaSpace{}%
\AgdaBound{msg₁}\AgdaSpace{}%
\AgdaBound{pbk1}\AgdaSpace{}%
\AgdaBound{pbk2}\AgdaSpace{}%
\AgdaBound{pbk3}\AgdaSpace{}%
\AgdaBound{pbk4}\AgdaSpace{}%
\AgdaBound{pbk5}\AgdaSpace{}%
\AgdaBound{sig1}\AgdaSpace{}%
\AgdaBound{sig2}\AgdaSpace{}%
\AgdaBound{sig3}\AgdaSpace{}%
\AgdaBound{x}\AgdaSpace{}%
\AgdaBound{x₁}\AgdaSpace{}%
\AgdaBound{x₂}\AgdaSpace{}%
\AgdaSymbol{|}\AgdaSpace{}%
\AgdaInductiveConstructor{true}\AgdaSpace{}%
\AgdaKeyword{with}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaFunction{isSigned}%
\>[106]\AgdaBound{msg₁}\AgdaSpace{}%
\AgdaBound{sig2}\AgdaSpace{}%
\AgdaBound{pbk2}\AgdaSymbol{)}\<%
\\
\>[0]\AgdaFunction{lemmaHoareTripleStackGeAux'18}\AgdaSpace{}%
\AgdaBound{msg₁}\AgdaSpace{}%
\AgdaBound{pbk1}\AgdaSpace{}%
\AgdaBound{pbk2}\AgdaSpace{}%
\AgdaBound{pbk3}\AgdaSpace{}%
\AgdaBound{pbk4}\AgdaSpace{}%
\AgdaBound{pbk5}\AgdaSpace{}%
\AgdaBound{sig1}\AgdaSpace{}%
\AgdaBound{sig2}\AgdaSpace{}%
\AgdaBound{sig3}\AgdaSpace{}%
\AgdaBound{x}\AgdaSpace{}%
\AgdaBound{x₁}\AgdaSpace{}%
\AgdaBound{x₂}\AgdaSpace{}%
\AgdaSymbol{|}\AgdaSpace{}%
\AgdaInductiveConstructor{true}\AgdaSpace{}%
\AgdaSymbol{|}\AgdaSpace{}%
\AgdaInductiveConstructor{false}\AgdaSpace{}%
\AgdaKeyword{with}%
\>[104]\AgdaSymbol{(}\AgdaFunction{isSigned}%
\>[115]\AgdaBound{msg₁}\AgdaSpace{}%
\AgdaBound{sig2}\AgdaSpace{}%
\AgdaBound{pbk3}\AgdaSymbol{)}\<%
\\
\>[0]\AgdaFunction{lemmaHoareTripleStackGeAux'18}\AgdaSpace{}%
\AgdaBound{msg₁}\AgdaSpace{}%
\AgdaBound{pbk1}\AgdaSpace{}%
\AgdaBound{pbk2}\AgdaSpace{}%
\AgdaBound{pbk3}\AgdaSpace{}%
\AgdaBound{pbk4}\AgdaSpace{}%
\AgdaBound{pbk5}\AgdaSpace{}%
\AgdaBound{sig1}\AgdaSpace{}%
\AgdaBound{sig2}\AgdaSpace{}%
\AgdaBound{sig3}\AgdaSpace{}%
\AgdaBound{x}\AgdaSpace{}%
\AgdaBound{x₁}\AgdaSpace{}%
\AgdaBound{x₂}\AgdaSpace{}%
\AgdaSymbol{|}\AgdaSpace{}%
\AgdaInductiveConstructor{true}\AgdaSpace{}%
\AgdaSymbol{|}\AgdaSpace{}%
\AgdaInductiveConstructor{false}\AgdaSpace{}%
\AgdaSymbol{|}\AgdaSpace{}%
\AgdaInductiveConstructor{true}\AgdaSpace{}%
\AgdaKeyword{with}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaFunction{isSigned}%
\>[121]\AgdaBound{msg₁}\AgdaSpace{}%
\AgdaBound{sig3}\AgdaSpace{}%
\AgdaBound{pbk4}\AgdaSymbol{)}\<%
\\
\>[0]\AgdaFunction{lemmaHoareTripleStackGeAux'18}\AgdaSpace{}%
\AgdaBound{msg₁}\AgdaSpace{}%
\AgdaBound{pbk1}\AgdaSpace{}%
\AgdaBound{pbk2}\AgdaSpace{}%
\AgdaBound{pbk3}\AgdaSpace{}%
\AgdaBound{pbk4}\AgdaSpace{}%
\AgdaBound{pbk5}\AgdaSpace{}%
\AgdaBound{sig1}\AgdaSpace{}%
\AgdaBound{sig2}\AgdaSpace{}%
\AgdaBound{sig3}\AgdaSpace{}%
\AgdaBound{x}\AgdaSpace{}%
\AgdaBound{x₁}\AgdaSpace{}%
\AgdaBound{x₂}\AgdaSpace{}%
\AgdaSymbol{|}\AgdaSpace{}%
\AgdaInductiveConstructor{true}\AgdaSpace{}%
\AgdaSymbol{|}\AgdaSpace{}%
\AgdaInductiveConstructor{false}\AgdaSpace{}%
\AgdaSymbol{|}\AgdaSpace{}%
\AgdaInductiveConstructor{true}\AgdaSpace{}%
\AgdaSymbol{|}\AgdaSpace{}%
\AgdaInductiveConstructor{false}\AgdaSpace{}%
\AgdaKeyword{with}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaFunction{isSigned}%
\>[129]\AgdaBound{msg₁}\AgdaSpace{}%
\AgdaBound{sig3}\AgdaSpace{}%
\AgdaBound{pbk5}\AgdaSymbol{)}\<%
\\
\>[0]\AgdaFunction{lemmaHoareTripleStackGeAux'18}\AgdaSpace{}%
\AgdaBound{msg₁}\AgdaSpace{}%
\AgdaBound{pbk1}\AgdaSpace{}%
\AgdaBound{pbk2}\AgdaSpace{}%
\AgdaBound{pbk3}\AgdaSpace{}%
\AgdaBound{pbk4}\AgdaSpace{}%
\AgdaBound{pbk5}\AgdaSpace{}%
\AgdaBound{sig1}\AgdaSpace{}%
\AgdaBound{sig2}\AgdaSpace{}%
\AgdaBound{sig3}\AgdaSpace{}%
\AgdaBound{x}\AgdaSpace{}%
\AgdaBound{x₁}\AgdaSpace{}%
\AgdaBound{x₂}\AgdaSpace{}%
\AgdaSymbol{|}\AgdaSpace{}%
\AgdaInductiveConstructor{true}\AgdaSpace{}%
\AgdaSymbol{|}\AgdaSpace{}%
\AgdaInductiveConstructor{false}\AgdaSpace{}%
\AgdaSymbol{|}\AgdaSpace{}%
\AgdaInductiveConstructor{true}\AgdaSpace{}%
\AgdaSymbol{|}\AgdaSpace{}%
\AgdaInductiveConstructor{false}\AgdaSpace{}%
\AgdaSymbol{|}\AgdaSpace{}%
\AgdaInductiveConstructor{true}\AgdaSpace{}%
\AgdaSymbol{=}\AgdaSpace{}%
\AgdaInductiveConstructor{tt}\<%
\\
\>[0]\AgdaFunction{lemmaHoareTripleStackGeAux'18}\AgdaSpace{}%
\AgdaBound{msg₁}\AgdaSpace{}%
\AgdaBound{pbk1}\AgdaSpace{}%
\AgdaBound{pbk2}\AgdaSpace{}%
\AgdaBound{pbk3}\AgdaSpace{}%
\AgdaBound{pbk4}\AgdaSpace{}%
\AgdaBound{pbk5}\AgdaSpace{}%
\AgdaBound{sig1}\AgdaSpace{}%
\AgdaBound{sig2}\AgdaSpace{}%
\AgdaBound{sig3}\AgdaSpace{}%
\AgdaBound{x}\AgdaSpace{}%
\AgdaBound{x₁}\AgdaSpace{}%
\AgdaBound{x₂}\AgdaSpace{}%
\AgdaSymbol{|}\AgdaSpace{}%
\AgdaInductiveConstructor{true}\AgdaSpace{}%
\AgdaSymbol{|}\AgdaSpace{}%
\AgdaInductiveConstructor{false}\AgdaSpace{}%
\AgdaSymbol{|}\AgdaSpace{}%
\AgdaInductiveConstructor{true}\AgdaSpace{}%
\AgdaSymbol{|}\AgdaSpace{}%
\AgdaInductiveConstructor{true}\AgdaSpace{}%
\AgdaSymbol{=}\AgdaSpace{}%
\AgdaInductiveConstructor{tt}\<%
\\
\>[0]\AgdaFunction{lemmaHoareTripleStackGeAux'18}\AgdaSpace{}%
\AgdaBound{msg₁}\AgdaSpace{}%
\AgdaBound{pbk1}\AgdaSpace{}%
\AgdaBound{pbk2}\AgdaSpace{}%
\AgdaBound{pbk3}\AgdaSpace{}%
\AgdaBound{pbk4}\AgdaSpace{}%
\AgdaBound{pbk5}\AgdaSpace{}%
\AgdaBound{sig1}\AgdaSpace{}%
\AgdaBound{sig2}\AgdaSpace{}%
\AgdaBound{sig3}\AgdaSpace{}%
\AgdaBound{x}\AgdaSpace{}%
\AgdaBound{x₁}\AgdaSpace{}%
\AgdaBound{x₂}\AgdaSpace{}%
\AgdaSymbol{|}\AgdaSpace{}%
\AgdaInductiveConstructor{true}\AgdaSpace{}%
\AgdaSymbol{|}\AgdaSpace{}%
\AgdaInductiveConstructor{true}\AgdaSpace{}%
\AgdaKeyword{with}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaFunction{isSigned}%
\>[113]\AgdaBound{msg₁}\AgdaSpace{}%
\AgdaBound{sig3}\AgdaSpace{}%
\AgdaBound{pbk3}\AgdaSymbol{)}\<%
\\
\>[0]\AgdaFunction{lemmaHoareTripleStackGeAux'18}\AgdaSpace{}%
\AgdaBound{msg₁}\AgdaSpace{}%
\AgdaBound{pbk1}\AgdaSpace{}%
\AgdaBound{pbk2}\AgdaSpace{}%
\AgdaBound{pbk3}\AgdaSpace{}%
\AgdaBound{pbk4}\AgdaSpace{}%
\AgdaBound{pbk5}\AgdaSpace{}%
\AgdaBound{sig1}\AgdaSpace{}%
\AgdaBound{sig2}\AgdaSpace{}%
\AgdaBound{sig3}\AgdaSpace{}%
\AgdaBound{x}\AgdaSpace{}%
\AgdaBound{x₁}\AgdaSpace{}%
\AgdaBound{x₂}\AgdaSpace{}%
\AgdaSymbol{|}\AgdaSpace{}%
\AgdaInductiveConstructor{true}\AgdaSpace{}%
\AgdaSymbol{|}\AgdaSpace{}%
\AgdaInductiveConstructor{true}\AgdaSpace{}%
\AgdaSymbol{|}\AgdaSpace{}%
\AgdaInductiveConstructor{false}\AgdaSpace{}%
\AgdaKeyword{with}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaFunction{isSigned}%
\>[121]\AgdaBound{msg₁}\AgdaSpace{}%
\AgdaBound{sig3}\AgdaSpace{}%
\AgdaBound{pbk4}\AgdaSymbol{)}\<%
\\
\>[0]\AgdaFunction{lemmaHoareTripleStackGeAux'18}\AgdaSpace{}%
\AgdaBound{msg₁}\AgdaSpace{}%
\AgdaBound{pbk1}\AgdaSpace{}%
\AgdaBound{pbk2}\AgdaSpace{}%
\AgdaBound{pbk3}\AgdaSpace{}%
\AgdaBound{pbk4}\AgdaSpace{}%
\AgdaBound{pbk5}\AgdaSpace{}%
\AgdaBound{sig1}\AgdaSpace{}%
\AgdaBound{sig2}\AgdaSpace{}%
\AgdaBound{sig3}\AgdaSpace{}%
\AgdaBound{x}\AgdaSpace{}%
\AgdaBound{x₁}\AgdaSpace{}%
\AgdaBound{x₂}\AgdaSpace{}%
\AgdaSymbol{|}\AgdaSpace{}%
\AgdaInductiveConstructor{true}\AgdaSpace{}%
\AgdaSymbol{|}\AgdaSpace{}%
\AgdaInductiveConstructor{true}\AgdaSpace{}%
\AgdaSymbol{|}\AgdaSpace{}%
\AgdaInductiveConstructor{false}\AgdaSpace{}%
\AgdaSymbol{|}\AgdaSpace{}%
\AgdaInductiveConstructor{false}\AgdaSpace{}%
\AgdaKeyword{with}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaFunction{isSigned}%
\>[129]\AgdaBound{msg₁}\AgdaSpace{}%
\AgdaBound{sig3}\AgdaSpace{}%
\AgdaBound{pbk5}\AgdaSymbol{)}\<%
\\
\>[0]\AgdaFunction{lemmaHoareTripleStackGeAux'18}\AgdaSpace{}%
\AgdaBound{msg₁}\AgdaSpace{}%
\AgdaBound{pbk1}\AgdaSpace{}%
\AgdaBound{pbk2}\AgdaSpace{}%
\AgdaBound{pbk3}\AgdaSpace{}%
\AgdaBound{pbk4}\AgdaSpace{}%
\AgdaBound{pbk5}\AgdaSpace{}%
\AgdaBound{sig1}\AgdaSpace{}%
\AgdaBound{sig2}\AgdaSpace{}%
\AgdaBound{sig3}\AgdaSpace{}%
\AgdaBound{x}\AgdaSpace{}%
\AgdaBound{x₁}\AgdaSpace{}%
\AgdaBound{x₂}\AgdaSpace{}%
\AgdaSymbol{|}\AgdaSpace{}%
\AgdaInductiveConstructor{true}\AgdaSpace{}%
\AgdaSymbol{|}\AgdaSpace{}%
\AgdaInductiveConstructor{true}\AgdaSpace{}%
\AgdaSymbol{|}\AgdaSpace{}%
\AgdaInductiveConstructor{false}\AgdaSpace{}%
\AgdaSymbol{|}\AgdaSpace{}%
\AgdaInductiveConstructor{false}\AgdaSpace{}%
\AgdaSymbol{|}\AgdaSpace{}%
\AgdaInductiveConstructor{true}\AgdaSpace{}%
\AgdaSymbol{=}\AgdaSpace{}%
\AgdaInductiveConstructor{tt}\<%
\\
\>[0]\AgdaFunction{lemmaHoareTripleStackGeAux'18}\AgdaSpace{}%
\AgdaBound{msg₁}\AgdaSpace{}%
\AgdaBound{pbk1}\AgdaSpace{}%
\AgdaBound{pbk2}\AgdaSpace{}%
\AgdaBound{pbk3}\AgdaSpace{}%
\AgdaBound{pbk4}\AgdaSpace{}%
\AgdaBound{pbk5}\AgdaSpace{}%
\AgdaBound{sig1}\AgdaSpace{}%
\AgdaBound{sig2}\AgdaSpace{}%
\AgdaBound{sig3}\AgdaSpace{}%
\AgdaBound{x}\AgdaSpace{}%
\AgdaBound{x₁}\AgdaSpace{}%
\AgdaBound{x₂}\AgdaSpace{}%
\AgdaSymbol{|}\AgdaSpace{}%
\AgdaInductiveConstructor{true}\AgdaSpace{}%
\AgdaSymbol{|}\AgdaSpace{}%
\AgdaInductiveConstructor{true}\AgdaSpace{}%
\AgdaSymbol{|}\AgdaSpace{}%
\AgdaInductiveConstructor{false}\AgdaSpace{}%
\AgdaSymbol{|}\AgdaSpace{}%
\AgdaInductiveConstructor{true}\AgdaSpace{}%
\AgdaSymbol{=}\AgdaSpace{}%
\AgdaInductiveConstructor{tt}\<%
\\
\>[0]\AgdaFunction{lemmaHoareTripleStackGeAux'18}\AgdaSpace{}%
\AgdaBound{msg₁}\AgdaSpace{}%
\AgdaBound{pbk1}\AgdaSpace{}%
\AgdaBound{pbk2}\AgdaSpace{}%
\AgdaBound{pbk3}\AgdaSpace{}%
\AgdaBound{pbk4}\AgdaSpace{}%
\AgdaBound{pbk5}\AgdaSpace{}%
\AgdaBound{sig1}\AgdaSpace{}%
\AgdaBound{sig2}\AgdaSpace{}%
\AgdaBound{sig3}\AgdaSpace{}%
\AgdaBound{x}\AgdaSpace{}%
\AgdaBound{x₁}\AgdaSpace{}%
\AgdaBound{x₂}\AgdaSpace{}%
\AgdaSymbol{|}\AgdaSpace{}%
\AgdaInductiveConstructor{true}\AgdaSpace{}%
\AgdaSymbol{|}\AgdaSpace{}%
\AgdaInductiveConstructor{true}\AgdaSpace{}%
\AgdaSymbol{|}\AgdaSpace{}%
\AgdaInductiveConstructor{true}\AgdaSpace{}%
\AgdaSymbol{=}\AgdaSpace{}%
\AgdaInductiveConstructor{tt}\<%
\\
%
\\[\AgdaEmptyExtraSkip]%
%
\\[\AgdaEmptyExtraSkip]%
\>[0]\AgdaFunction{lemmaHoareTripleStackGeAux'19}%
\>[4071I]\AgdaSymbol{:}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaBound{msg}\AgdaSpace{}%
\AgdaSymbol{:}\AgdaSpace{}%
\AgdaDatatype{Msg}\AgdaSymbol{)}\<%
\\
\>[4071I][@{}l@{\AgdaIndent{0}}]%
\>[31]\AgdaSymbol{(}\AgdaBound{pbk1}\AgdaSpace{}%
\AgdaBound{pbk2}\AgdaSpace{}%
\AgdaBound{pbk3}\AgdaSpace{}%
\AgdaBound{pbk4}\AgdaSpace{}%
\AgdaBound{pbk5}\AgdaSpace{}%
\AgdaBound{sig1}\AgdaSpace{}%
\AgdaBound{sig2}\AgdaSpace{}%
\AgdaBound{sig3}\AgdaSpace{}%
\AgdaSymbol{:}\AgdaSpace{}%
\AgdaDatatype{ℕ}\AgdaSymbol{)}\<%
\\
%
\>[31]\AgdaSymbol{→}\AgdaSpace{}%
\AgdaFunction{True}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaFunction{isSigned}%
\>[49]\AgdaBound{msg}\AgdaSpace{}%
\AgdaBound{sig3}\AgdaSpace{}%
\AgdaBound{pbk5}\AgdaSymbol{)}\<%
\\
\>[.][@{}l@{}]\<[4071I]%
\>[30]\AgdaSymbol{→}%
\>[33]\AgdaFunction{True}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaFunction{isSigned}%
\>[49]\AgdaBound{msg}\AgdaSpace{}%
\AgdaBound{sig2}\AgdaSpace{}%
\AgdaBound{pbk4}\AgdaSymbol{)}\<%
\\
\>[30][@{}l@{\AgdaIndent{0}}]%
\>[31]\AgdaSymbol{→}%
\>[34]\AgdaFunction{True}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaFunction{isSigned}%
\>[50]\AgdaBound{msg}\AgdaSpace{}%
\AgdaBound{sig1}\AgdaSpace{}%
\AgdaBound{pbk1}\AgdaSymbol{)}\<%
\\
%
\>[31]\AgdaSymbol{→}\AgdaSpace{}%
\AgdaFunction{True}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaFunction{compareSigsMultiSig}\AgdaSpace{}%
\AgdaBound{msg}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaSpace{}%
\AgdaBound{sig1}\AgdaSpace{}%
\AgdaOperator{\AgdaInductiveConstructor{∷}}\AgdaSpace{}%
\AgdaBound{sig2}\AgdaSpace{}%
\AgdaOperator{\AgdaInductiveConstructor{∷}}\AgdaSpace{}%
\AgdaBound{sig3}\AgdaSpace{}%
\AgdaOperator{\AgdaInductiveConstructor{∷}}\AgdaSpace{}%
\AgdaInductiveConstructor{[]}\AgdaSymbol{)}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaBound{pbk1}\AgdaSpace{}%
\AgdaOperator{\AgdaInductiveConstructor{∷}}\AgdaSpace{}%
\AgdaBound{pbk2}\AgdaSpace{}%
\AgdaOperator{\AgdaInductiveConstructor{∷}}\AgdaSpace{}%
\AgdaBound{pbk3}\AgdaSpace{}%
\AgdaOperator{\AgdaInductiveConstructor{∷}}\AgdaSpace{}%
\AgdaBound{pbk4}\AgdaSpace{}%
\AgdaOperator{\AgdaInductiveConstructor{∷}}\AgdaSpace{}%
\AgdaBound{pbk5}\AgdaSpace{}%
\AgdaOperator{\AgdaInductiveConstructor{∷}}\AgdaSpace{}%
\AgdaInductiveConstructor{[]}\AgdaSymbol{))}\<%
\\
\>[0]\AgdaFunction{lemmaHoareTripleStackGeAux'19}\AgdaSpace{}%
\AgdaBound{msg₁}\AgdaSpace{}%
\AgdaBound{pbk1}\AgdaSpace{}%
\AgdaBound{pbk2}\AgdaSpace{}%
\AgdaBound{pbk3}\AgdaSpace{}%
\AgdaBound{pbk4}\AgdaSpace{}%
\AgdaBound{pbk5}\AgdaSpace{}%
\AgdaBound{sig1}\AgdaSpace{}%
\AgdaBound{sig2}\AgdaSpace{}%
\AgdaBound{sig3}\AgdaSpace{}%
\AgdaBound{x}\AgdaSpace{}%
\AgdaBound{x₁}\AgdaSpace{}%
\AgdaBound{x₂}\AgdaSpace{}%
\AgdaKeyword{with}%
\>[89]\AgdaSymbol{(}\AgdaFunction{isSigned}%
\>[100]\AgdaBound{msg₁}\AgdaSpace{}%
\AgdaBound{sig1}\AgdaSpace{}%
\AgdaBound{pbk1}\AgdaSymbol{)}\<%
\\
\>[0]\AgdaFunction{lemmaHoareTripleStackGeAux'19}\AgdaSpace{}%
\AgdaBound{msg₁}\AgdaSpace{}%
\AgdaBound{pbk1}\AgdaSpace{}%
\AgdaBound{pbk2}\AgdaSpace{}%
\AgdaBound{pbk3}\AgdaSpace{}%
\AgdaBound{pbk4}\AgdaSpace{}%
\AgdaBound{pbk5}\AgdaSpace{}%
\AgdaBound{sig1}\AgdaSpace{}%
\AgdaBound{sig2}\AgdaSpace{}%
\AgdaBound{sig3}\AgdaSpace{}%
\AgdaBound{x}\AgdaSpace{}%
\AgdaBound{x₁}\AgdaSpace{}%
\AgdaBound{x₂}\AgdaSpace{}%
\AgdaSymbol{|}\AgdaSpace{}%
\AgdaInductiveConstructor{true}\AgdaSpace{}%
\AgdaKeyword{with}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaFunction{isSigned}%
\>[106]\AgdaBound{msg₁}\AgdaSpace{}%
\AgdaBound{sig2}\AgdaSpace{}%
\AgdaBound{pbk2}\AgdaSymbol{)}\<%
\\
\>[0]\AgdaFunction{lemmaHoareTripleStackGeAux'19}\AgdaSpace{}%
\AgdaBound{msg₁}\AgdaSpace{}%
\AgdaBound{pbk1}\AgdaSpace{}%
\AgdaBound{pbk2}\AgdaSpace{}%
\AgdaBound{pbk3}\AgdaSpace{}%
\AgdaBound{pbk4}\AgdaSpace{}%
\AgdaBound{pbk5}\AgdaSpace{}%
\AgdaBound{sig1}\AgdaSpace{}%
\AgdaBound{sig2}\AgdaSpace{}%
\AgdaBound{sig3}\AgdaSpace{}%
\AgdaBound{x}\AgdaSpace{}%
\AgdaBound{x₁}\AgdaSpace{}%
\AgdaBound{x₂}\AgdaSpace{}%
\AgdaSymbol{|}\AgdaSpace{}%
\AgdaInductiveConstructor{true}\AgdaSpace{}%
\AgdaSymbol{|}\AgdaSpace{}%
\AgdaInductiveConstructor{false}\AgdaSpace{}%
\AgdaKeyword{with}%
\>[104]\AgdaSymbol{(}\AgdaFunction{isSigned}%
\>[115]\AgdaBound{msg₁}\AgdaSpace{}%
\AgdaBound{sig2}\AgdaSpace{}%
\AgdaBound{pbk3}\AgdaSymbol{)}\<%
\\
\>[0]\AgdaFunction{lemmaHoareTripleStackGeAux'19}\AgdaSpace{}%
\AgdaBound{msg₁}\AgdaSpace{}%
\AgdaBound{pbk1}\AgdaSpace{}%
\AgdaBound{pbk2}\AgdaSpace{}%
\AgdaBound{pbk3}\AgdaSpace{}%
\AgdaBound{pbk4}\AgdaSpace{}%
\AgdaBound{pbk5}\AgdaSpace{}%
\AgdaBound{sig1}\AgdaSpace{}%
\AgdaBound{sig2}\AgdaSpace{}%
\AgdaBound{sig3}\AgdaSpace{}%
\AgdaBound{x}\AgdaSpace{}%
\AgdaBound{x₁}\AgdaSpace{}%
\AgdaBound{x₂}\AgdaSpace{}%
\AgdaSymbol{|}\AgdaSpace{}%
\AgdaInductiveConstructor{true}\AgdaSpace{}%
\AgdaSymbol{|}\AgdaSpace{}%
\AgdaInductiveConstructor{false}\AgdaSpace{}%
\AgdaSymbol{|}\AgdaSpace{}%
\AgdaInductiveConstructor{false}\AgdaSpace{}%
\AgdaKeyword{with}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaFunction{isSigned}%
\>[122]\AgdaBound{msg₁}\AgdaSpace{}%
\AgdaBound{sig2}\AgdaSpace{}%
\AgdaBound{pbk4}\AgdaSymbol{)}\<%
\\
\>[0]\AgdaFunction{lemmaHoareTripleStackGeAux'19}\AgdaSpace{}%
\AgdaBound{msg₁}\AgdaSpace{}%
\AgdaBound{pbk1}\AgdaSpace{}%
\AgdaBound{pbk2}\AgdaSpace{}%
\AgdaBound{pbk3}\AgdaSpace{}%
\AgdaBound{pbk4}\AgdaSpace{}%
\AgdaBound{pbk5}\AgdaSpace{}%
\AgdaBound{sig1}\AgdaSpace{}%
\AgdaBound{sig2}\AgdaSpace{}%
\AgdaBound{sig3}\AgdaSpace{}%
\AgdaBound{x}\AgdaSpace{}%
\AgdaBound{x₁}\AgdaSpace{}%
\AgdaBound{x₂}\AgdaSpace{}%
\AgdaSymbol{|}\AgdaSpace{}%
\AgdaInductiveConstructor{true}\AgdaSpace{}%
\AgdaSymbol{|}\AgdaSpace{}%
\AgdaInductiveConstructor{false}\AgdaSpace{}%
\AgdaSymbol{|}\AgdaSpace{}%
\AgdaInductiveConstructor{false}\AgdaSpace{}%
\AgdaSymbol{|}\AgdaSpace{}%
\AgdaInductiveConstructor{true}\AgdaSpace{}%
\AgdaKeyword{with}%
\>[119]\AgdaSymbol{(}\AgdaFunction{isSigned}%
\>[130]\AgdaBound{msg₁}\AgdaSpace{}%
\AgdaBound{sig3}\AgdaSpace{}%
\AgdaBound{pbk5}\AgdaSymbol{)}\<%
\\
\>[0]\AgdaFunction{lemmaHoareTripleStackGeAux'19}\AgdaSpace{}%
\AgdaBound{msg₁}\AgdaSpace{}%
\AgdaBound{pbk1}\AgdaSpace{}%
\AgdaBound{pbk2}\AgdaSpace{}%
\AgdaBound{pbk3}\AgdaSpace{}%
\AgdaBound{pbk4}\AgdaSpace{}%
\AgdaBound{pbk5}\AgdaSpace{}%
\AgdaBound{sig1}\AgdaSpace{}%
\AgdaBound{sig2}\AgdaSpace{}%
\AgdaBound{sig3}\AgdaSpace{}%
\AgdaBound{x}\AgdaSpace{}%
\AgdaBound{x₁}\AgdaSpace{}%
\AgdaBound{x₂}\AgdaSpace{}%
\AgdaSymbol{|}\AgdaSpace{}%
\AgdaInductiveConstructor{true}\AgdaSpace{}%
\AgdaSymbol{|}\AgdaSpace{}%
\AgdaInductiveConstructor{false}\AgdaSpace{}%
\AgdaSymbol{|}\AgdaSpace{}%
\AgdaInductiveConstructor{false}\AgdaSpace{}%
\AgdaSymbol{|}\AgdaSpace{}%
\AgdaInductiveConstructor{true}\AgdaSpace{}%
\AgdaSymbol{|}\AgdaSpace{}%
\AgdaInductiveConstructor{true}\AgdaSpace{}%
\AgdaSymbol{=}\AgdaSpace{}%
\AgdaInductiveConstructor{tt}\<%
\\
\>[0]\AgdaFunction{lemmaHoareTripleStackGeAux'19}\AgdaSpace{}%
\AgdaBound{msg₁}\AgdaSpace{}%
\AgdaBound{pbk1}\AgdaSpace{}%
\AgdaBound{pbk2}\AgdaSpace{}%
\AgdaBound{pbk3}\AgdaSpace{}%
\AgdaBound{pbk4}\AgdaSpace{}%
\AgdaBound{pbk5}\AgdaSpace{}%
\AgdaBound{sig1}\AgdaSpace{}%
\AgdaBound{sig2}\AgdaSpace{}%
\AgdaBound{sig3}\AgdaSpace{}%
\AgdaBound{x}\AgdaSpace{}%
\AgdaBound{x₁}\AgdaSpace{}%
\AgdaBound{x₂}\AgdaSpace{}%
\AgdaSymbol{|}\AgdaSpace{}%
\AgdaInductiveConstructor{true}\AgdaSpace{}%
\AgdaSymbol{|}\AgdaSpace{}%
\AgdaInductiveConstructor{false}\AgdaSpace{}%
\AgdaSymbol{|}\AgdaSpace{}%
\AgdaInductiveConstructor{true}\AgdaSpace{}%
\AgdaKeyword{with}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaFunction{isSigned}%
\>[121]\AgdaBound{msg₁}\AgdaSpace{}%
\AgdaBound{sig3}\AgdaSpace{}%
\AgdaBound{pbk4}\AgdaSymbol{)}\<%
\\
\>[0]\AgdaFunction{lemmaHoareTripleStackGeAux'19}\AgdaSpace{}%
\AgdaBound{msg₁}\AgdaSpace{}%
\AgdaBound{pbk1}\AgdaSpace{}%
\AgdaBound{pbk2}\AgdaSpace{}%
\AgdaBound{pbk3}\AgdaSpace{}%
\AgdaBound{pbk4}\AgdaSpace{}%
\AgdaBound{pbk5}\AgdaSpace{}%
\AgdaBound{sig1}\AgdaSpace{}%
\AgdaBound{sig2}\AgdaSpace{}%
\AgdaBound{sig3}\AgdaSpace{}%
\AgdaBound{x}\AgdaSpace{}%
\AgdaBound{x₁}\AgdaSpace{}%
\AgdaBound{x₂}\AgdaSpace{}%
\AgdaSymbol{|}\AgdaSpace{}%
\AgdaInductiveConstructor{true}\AgdaSpace{}%
\AgdaSymbol{|}\AgdaSpace{}%
\AgdaInductiveConstructor{false}\AgdaSpace{}%
\AgdaSymbol{|}\AgdaSpace{}%
\AgdaInductiveConstructor{true}\AgdaSpace{}%
\AgdaSymbol{|}\AgdaSpace{}%
\AgdaInductiveConstructor{false}\AgdaSpace{}%
\AgdaKeyword{with}%
\>[120]\AgdaSymbol{(}\AgdaFunction{isSigned}%
\>[131]\AgdaBound{msg₁}\AgdaSpace{}%
\AgdaBound{sig3}\AgdaSpace{}%
\AgdaBound{pbk5}\AgdaSymbol{)}\<%
\\
\>[0]\AgdaFunction{lemmaHoareTripleStackGeAux'19}\AgdaSpace{}%
\AgdaBound{msg₁}\AgdaSpace{}%
\AgdaBound{pbk1}\AgdaSpace{}%
\AgdaBound{pbk2}\AgdaSpace{}%
\AgdaBound{pbk3}\AgdaSpace{}%
\AgdaBound{pbk4}\AgdaSpace{}%
\AgdaBound{pbk5}\AgdaSpace{}%
\AgdaBound{sig1}\AgdaSpace{}%
\AgdaBound{sig2}\AgdaSpace{}%
\AgdaBound{sig3}\AgdaSpace{}%
\AgdaBound{x}\AgdaSpace{}%
\AgdaBound{x₁}\AgdaSpace{}%
\AgdaBound{x₂}\AgdaSpace{}%
\AgdaSymbol{|}\AgdaSpace{}%
\AgdaInductiveConstructor{true}\AgdaSpace{}%
\AgdaSymbol{|}\AgdaSpace{}%
\AgdaInductiveConstructor{false}\AgdaSpace{}%
\AgdaSymbol{|}\AgdaSpace{}%
\AgdaInductiveConstructor{true}\AgdaSpace{}%
\AgdaSymbol{|}\AgdaSpace{}%
\AgdaInductiveConstructor{false}\AgdaSpace{}%
\AgdaSymbol{|}\AgdaSpace{}%
\AgdaInductiveConstructor{true}\AgdaSpace{}%
\AgdaSymbol{=}\AgdaSpace{}%
\AgdaInductiveConstructor{tt}\<%
\\
\>[0]\AgdaFunction{lemmaHoareTripleStackGeAux'19}\AgdaSpace{}%
\AgdaBound{msg₁}\AgdaSpace{}%
\AgdaBound{pbk1}\AgdaSpace{}%
\AgdaBound{pbk2}\AgdaSpace{}%
\AgdaBound{pbk3}\AgdaSpace{}%
\AgdaBound{pbk4}\AgdaSpace{}%
\AgdaBound{pbk5}\AgdaSpace{}%
\AgdaBound{sig1}\AgdaSpace{}%
\AgdaBound{sig2}\AgdaSpace{}%
\AgdaBound{sig3}\AgdaSpace{}%
\AgdaBound{x}\AgdaSpace{}%
\AgdaBound{x₁}\AgdaSpace{}%
\AgdaBound{x₂}\AgdaSpace{}%
\AgdaSymbol{|}\AgdaSpace{}%
\AgdaInductiveConstructor{true}\AgdaSpace{}%
\AgdaSymbol{|}\AgdaSpace{}%
\AgdaInductiveConstructor{false}\AgdaSpace{}%
\AgdaSymbol{|}\AgdaSpace{}%
\AgdaInductiveConstructor{true}\AgdaSpace{}%
\AgdaSymbol{|}\AgdaSpace{}%
\AgdaInductiveConstructor{true}\AgdaSpace{}%
\AgdaSymbol{=}\AgdaSpace{}%
\AgdaInductiveConstructor{tt}\<%
\\
\>[0]\AgdaFunction{lemmaHoareTripleStackGeAux'19}\AgdaSpace{}%
\AgdaBound{msg₁}\AgdaSpace{}%
\AgdaBound{pbk1}\AgdaSpace{}%
\AgdaBound{pbk2}\AgdaSpace{}%
\AgdaBound{pbk3}\AgdaSpace{}%
\AgdaBound{pbk4}\AgdaSpace{}%
\AgdaBound{pbk5}\AgdaSpace{}%
\AgdaBound{sig1}\AgdaSpace{}%
\AgdaBound{sig2}\AgdaSpace{}%
\AgdaBound{sig3}\AgdaSpace{}%
\AgdaBound{x}\AgdaSpace{}%
\AgdaBound{x₁}\AgdaSpace{}%
\AgdaBound{x₂}\AgdaSpace{}%
\AgdaSymbol{|}\AgdaSpace{}%
\AgdaInductiveConstructor{true}\AgdaSpace{}%
\AgdaSymbol{|}\AgdaSpace{}%
\AgdaInductiveConstructor{true}\AgdaSpace{}%
\AgdaKeyword{with}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaFunction{isSigned}%
\>[113]\AgdaBound{msg₁}\AgdaSpace{}%
\AgdaBound{sig3}\AgdaSpace{}%
\AgdaBound{pbk3}\AgdaSymbol{)}\<%
\\
\>[0]\AgdaFunction{lemmaHoareTripleStackGeAux'19}\AgdaSpace{}%
\AgdaBound{msg₁}\AgdaSpace{}%
\AgdaBound{pbk1}\AgdaSpace{}%
\AgdaBound{pbk2}\AgdaSpace{}%
\AgdaBound{pbk3}\AgdaSpace{}%
\AgdaBound{pbk4}\AgdaSpace{}%
\AgdaBound{pbk5}\AgdaSpace{}%
\AgdaBound{sig1}\AgdaSpace{}%
\AgdaBound{sig2}\AgdaSpace{}%
\AgdaBound{sig3}\AgdaSpace{}%
\AgdaBound{x}\AgdaSpace{}%
\AgdaBound{x₁}\AgdaSpace{}%
\AgdaBound{x₂}\AgdaSpace{}%
\AgdaSymbol{|}\AgdaSpace{}%
\AgdaInductiveConstructor{true}\AgdaSpace{}%
\AgdaSymbol{|}\AgdaSpace{}%
\AgdaInductiveConstructor{true}\AgdaSpace{}%
\AgdaSymbol{|}\AgdaSpace{}%
\AgdaInductiveConstructor{false}\AgdaSpace{}%
\AgdaKeyword{with}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaFunction{isSigned}%
\>[121]\AgdaBound{msg₁}\AgdaSpace{}%
\AgdaBound{sig3}\AgdaSpace{}%
\AgdaBound{pbk4}\AgdaSymbol{)}\<%
\\
\>[0]\AgdaFunction{lemmaHoareTripleStackGeAux'19}\AgdaSpace{}%
\AgdaBound{msg₁}\AgdaSpace{}%
\AgdaBound{pbk1}\AgdaSpace{}%
\AgdaBound{pbk2}\AgdaSpace{}%
\AgdaBound{pbk3}\AgdaSpace{}%
\AgdaBound{pbk4}\AgdaSpace{}%
\AgdaBound{pbk5}\AgdaSpace{}%
\AgdaBound{sig1}\AgdaSpace{}%
\AgdaBound{sig2}\AgdaSpace{}%
\AgdaBound{sig3}\AgdaSpace{}%
\AgdaBound{x}\AgdaSpace{}%
\AgdaBound{x₁}\AgdaSpace{}%
\AgdaBound{x₂}\AgdaSpace{}%
\AgdaSymbol{|}\AgdaSpace{}%
\AgdaInductiveConstructor{true}\AgdaSpace{}%
\AgdaSymbol{|}\AgdaSpace{}%
\AgdaInductiveConstructor{true}\AgdaSpace{}%
\AgdaSymbol{|}\AgdaSpace{}%
\AgdaInductiveConstructor{false}\AgdaSpace{}%
\AgdaSymbol{|}\AgdaSpace{}%
\AgdaInductiveConstructor{false}\AgdaSpace{}%
\AgdaKeyword{with}%
\>[119]\AgdaSymbol{(}\AgdaFunction{isSigned}%
\>[130]\AgdaBound{msg₁}\AgdaSpace{}%
\AgdaBound{sig3}\AgdaSpace{}%
\AgdaBound{pbk5}\AgdaSymbol{)}\<%
\\
\>[0]\AgdaFunction{lemmaHoareTripleStackGeAux'19}\AgdaSpace{}%
\AgdaBound{msg₁}\AgdaSpace{}%
\AgdaBound{pbk1}\AgdaSpace{}%
\AgdaBound{pbk2}\AgdaSpace{}%
\AgdaBound{pbk3}\AgdaSpace{}%
\AgdaBound{pbk4}\AgdaSpace{}%
\AgdaBound{pbk5}\AgdaSpace{}%
\AgdaBound{sig1}\AgdaSpace{}%
\AgdaBound{sig2}\AgdaSpace{}%
\AgdaBound{sig3}\AgdaSpace{}%
\AgdaBound{x}\AgdaSpace{}%
\AgdaBound{x₁}\AgdaSpace{}%
\AgdaBound{x₂}\AgdaSpace{}%
\AgdaSymbol{|}\AgdaSpace{}%
\AgdaInductiveConstructor{true}\AgdaSpace{}%
\AgdaSymbol{|}\AgdaSpace{}%
\AgdaInductiveConstructor{true}\AgdaSpace{}%
\AgdaSymbol{|}\AgdaSpace{}%
\AgdaInductiveConstructor{false}\AgdaSpace{}%
\AgdaSymbol{|}\AgdaSpace{}%
\AgdaInductiveConstructor{false}\AgdaSpace{}%
\AgdaSymbol{|}\AgdaSpace{}%
\AgdaInductiveConstructor{true}\AgdaSpace{}%
\AgdaSymbol{=}\AgdaSpace{}%
\AgdaInductiveConstructor{tt}\<%
\\
\>[0]\AgdaFunction{lemmaHoareTripleStackGeAux'19}\AgdaSpace{}%
\AgdaBound{msg₁}\AgdaSpace{}%
\AgdaBound{pbk1}\AgdaSpace{}%
\AgdaBound{pbk2}\AgdaSpace{}%
\AgdaBound{pbk3}\AgdaSpace{}%
\AgdaBound{pbk4}\AgdaSpace{}%
\AgdaBound{pbk5}\AgdaSpace{}%
\AgdaBound{sig1}\AgdaSpace{}%
\AgdaBound{sig2}\AgdaSpace{}%
\AgdaBound{sig3}\AgdaSpace{}%
\AgdaBound{x}\AgdaSpace{}%
\AgdaBound{x₁}\AgdaSpace{}%
\AgdaBound{x₂}\AgdaSpace{}%
\AgdaSymbol{|}\AgdaSpace{}%
\AgdaInductiveConstructor{true}\AgdaSpace{}%
\AgdaSymbol{|}\AgdaSpace{}%
\AgdaInductiveConstructor{true}\AgdaSpace{}%
\AgdaSymbol{|}\AgdaSpace{}%
\AgdaInductiveConstructor{false}\AgdaSpace{}%
\AgdaSymbol{|}\AgdaSpace{}%
\AgdaInductiveConstructor{true}\AgdaSpace{}%
\AgdaSymbol{=}\AgdaSpace{}%
\AgdaInductiveConstructor{tt}\<%
\\
\>[0]\AgdaFunction{lemmaHoareTripleStackGeAux'19}\AgdaSpace{}%
\AgdaBound{msg₁}\AgdaSpace{}%
\AgdaBound{pbk1}\AgdaSpace{}%
\AgdaBound{pbk2}\AgdaSpace{}%
\AgdaBound{pbk3}\AgdaSpace{}%
\AgdaBound{pbk4}\AgdaSpace{}%
\AgdaBound{pbk5}\AgdaSpace{}%
\AgdaBound{sig1}\AgdaSpace{}%
\AgdaBound{sig2}\AgdaSpace{}%
\AgdaBound{sig3}\AgdaSpace{}%
\AgdaBound{x}\AgdaSpace{}%
\AgdaBound{x₁}\AgdaSpace{}%
\AgdaBound{x₂}\AgdaSpace{}%
\AgdaSymbol{|}\AgdaSpace{}%
\AgdaInductiveConstructor{true}\AgdaSpace{}%
\AgdaSymbol{|}\AgdaSpace{}%
\AgdaInductiveConstructor{true}\AgdaSpace{}%
\AgdaSymbol{|}\AgdaSpace{}%
\AgdaInductiveConstructor{true}\AgdaSpace{}%
\AgdaSymbol{=}\AgdaSpace{}%
\AgdaInductiveConstructor{tt}\<%
\\
%
\\[\AgdaEmptyExtraSkip]%
\>[0]\AgdaFunction{lemmaHoareTripleStackGeAux'20}%
\>[4459I]\AgdaSymbol{:}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaBound{msg}\AgdaSpace{}%
\AgdaSymbol{:}\AgdaSpace{}%
\AgdaDatatype{Msg}\AgdaSymbol{)}\<%
\\
\>[4459I][@{}l@{\AgdaIndent{0}}]%
\>[31]\AgdaSymbol{(}\AgdaBound{pbk1}\AgdaSpace{}%
\AgdaBound{pbk2}\AgdaSpace{}%
\AgdaBound{pbk3}\AgdaSpace{}%
\AgdaBound{pbk4}\AgdaSpace{}%
\AgdaBound{pbk5}\AgdaSpace{}%
\AgdaBound{sig1}\AgdaSpace{}%
\AgdaBound{sig2}\AgdaSpace{}%
\AgdaBound{sig3}\AgdaSpace{}%
\AgdaSymbol{:}\AgdaSpace{}%
\AgdaDatatype{ℕ}\AgdaSymbol{)}\<%
\\
%
\>[31]\AgdaSymbol{→}\AgdaSpace{}%
\AgdaFunction{True}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaFunction{isSigned}%
\>[49]\AgdaBound{msg}\AgdaSpace{}%
\AgdaBound{sig3}\AgdaSpace{}%
\AgdaBound{pbk4}\AgdaSymbol{)}\<%
\\
\>[.][@{}l@{}]\<[4459I]%
\>[30]\AgdaSymbol{→}%
\>[33]\AgdaFunction{True}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaFunction{isSigned}%
\>[49]\AgdaBound{msg}\AgdaSpace{}%
\AgdaBound{sig2}\AgdaSpace{}%
\AgdaBound{pbk3}\AgdaSymbol{)}\<%
\\
%
\>[30]\AgdaSymbol{→}%
\>[33]\AgdaFunction{True}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaFunction{isSigned}%
\>[49]\AgdaBound{msg}\AgdaSpace{}%
\AgdaBound{sig1}\AgdaSpace{}%
\AgdaBound{pbk2}\AgdaSymbol{)}\<%
\\
\>[30][@{}l@{\AgdaIndent{0}}]%
\>[31]\AgdaSymbol{→}\AgdaSpace{}%
\AgdaFunction{True}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaFunction{compareSigsMultiSig}\AgdaSpace{}%
\AgdaBound{msg}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaSpace{}%
\AgdaBound{sig1}\AgdaSpace{}%
\AgdaOperator{\AgdaInductiveConstructor{∷}}\AgdaSpace{}%
\AgdaBound{sig2}\AgdaSpace{}%
\AgdaOperator{\AgdaInductiveConstructor{∷}}\AgdaSpace{}%
\AgdaBound{sig3}\AgdaSpace{}%
\AgdaOperator{\AgdaInductiveConstructor{∷}}\AgdaSpace{}%
\AgdaInductiveConstructor{[]}\AgdaSymbol{)}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaBound{pbk1}\AgdaSpace{}%
\AgdaOperator{\AgdaInductiveConstructor{∷}}\AgdaSpace{}%
\AgdaBound{pbk2}\AgdaSpace{}%
\AgdaOperator{\AgdaInductiveConstructor{∷}}\AgdaSpace{}%
\AgdaBound{pbk3}\AgdaSpace{}%
\AgdaOperator{\AgdaInductiveConstructor{∷}}\AgdaSpace{}%
\AgdaBound{pbk4}\AgdaSpace{}%
\AgdaOperator{\AgdaInductiveConstructor{∷}}\AgdaSpace{}%
\AgdaBound{pbk5}\AgdaSpace{}%
\AgdaOperator{\AgdaInductiveConstructor{∷}}\AgdaSpace{}%
\AgdaInductiveConstructor{[]}\AgdaSymbol{))}\<%
\\
\>[0]\AgdaFunction{lemmaHoareTripleStackGeAux'20}\AgdaSpace{}%
\AgdaBound{msg₁}\AgdaSpace{}%
\AgdaBound{pbk1}\AgdaSpace{}%
\AgdaBound{pbk2}\AgdaSpace{}%
\AgdaBound{pbk3}\AgdaSpace{}%
\AgdaBound{pbk4}\AgdaSpace{}%
\AgdaBound{pbk5}\AgdaSpace{}%
\AgdaBound{sig1}\AgdaSpace{}%
\AgdaBound{sig2}\AgdaSpace{}%
\AgdaBound{sig3}\AgdaSpace{}%
\AgdaBound{x}\AgdaSpace{}%
\AgdaBound{x₁}\AgdaSpace{}%
\AgdaBound{x₂}\AgdaSpace{}%
\AgdaKeyword{with}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaFunction{isSigned}%
\>[99]\AgdaBound{msg₁}\AgdaSpace{}%
\AgdaBound{sig1}\AgdaSpace{}%
\AgdaBound{pbk1}\AgdaSymbol{)}\<%
\\
\>[0]\AgdaFunction{lemmaHoareTripleStackGeAux'20}\AgdaSpace{}%
\AgdaBound{msg₁}\AgdaSpace{}%
\AgdaBound{pbk1}\AgdaSpace{}%
\AgdaBound{pbk2}\AgdaSpace{}%
\AgdaBound{pbk3}\AgdaSpace{}%
\AgdaBound{pbk4}\AgdaSpace{}%
\AgdaBound{pbk5}\AgdaSpace{}%
\AgdaBound{sig1}\AgdaSpace{}%
\AgdaBound{sig2}\AgdaSpace{}%
\AgdaBound{sig3}\AgdaSpace{}%
\AgdaBound{x}\AgdaSpace{}%
\AgdaBound{x₁}\AgdaSpace{}%
\AgdaBound{x₂}\AgdaSpace{}%
\AgdaSymbol{|}\AgdaSpace{}%
\AgdaInductiveConstructor{false}\AgdaSpace{}%
\AgdaKeyword{with}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaFunction{isSigned}%
\>[107]\AgdaBound{msg₁}\AgdaSpace{}%
\AgdaBound{sig1}\AgdaSpace{}%
\AgdaBound{pbk2}\AgdaSymbol{)}\<%
\\
\>[0]\AgdaFunction{lemmaHoareTripleStackGeAux'20}\AgdaSpace{}%
\AgdaBound{msg₁}\AgdaSpace{}%
\AgdaBound{pbk1}\AgdaSpace{}%
\AgdaBound{pbk2}\AgdaSpace{}%
\AgdaBound{pbk3}\AgdaSpace{}%
\AgdaBound{pbk4}\AgdaSpace{}%
\AgdaBound{pbk5}\AgdaSpace{}%
\AgdaBound{sig1}\AgdaSpace{}%
\AgdaBound{sig2}\AgdaSpace{}%
\AgdaBound{sig3}\AgdaSpace{}%
\AgdaBound{x}\AgdaSpace{}%
\AgdaBound{x₁}\AgdaSpace{}%
\AgdaBound{x₂}\AgdaSpace{}%
\AgdaSymbol{|}\AgdaSpace{}%
\AgdaInductiveConstructor{false}\AgdaSpace{}%
\AgdaSymbol{|}\AgdaSpace{}%
\AgdaInductiveConstructor{true}\AgdaSpace{}%
\AgdaKeyword{with}%
\>[104]\AgdaSymbol{(}\AgdaFunction{isSigned}%
\>[115]\AgdaBound{msg₁}\AgdaSpace{}%
\AgdaBound{sig2}\AgdaSpace{}%
\AgdaBound{pbk3}\AgdaSymbol{)}\<%
\\
\>[0]\AgdaFunction{lemmaHoareTripleStackGeAux'20}\AgdaSpace{}%
\AgdaBound{msg₁}\AgdaSpace{}%
\AgdaBound{pbk1}\AgdaSpace{}%
\AgdaBound{pbk2}\AgdaSpace{}%
\AgdaBound{pbk3}\AgdaSpace{}%
\AgdaBound{pbk4}\AgdaSpace{}%
\AgdaBound{pbk5}\AgdaSpace{}%
\AgdaBound{sig1}\AgdaSpace{}%
\AgdaBound{sig2}\AgdaSpace{}%
\AgdaBound{sig3}\AgdaSpace{}%
\AgdaBound{x}\AgdaSpace{}%
\AgdaBound{x₁}\AgdaSpace{}%
\AgdaBound{x₂}\AgdaSpace{}%
\AgdaSymbol{|}\AgdaSpace{}%
\AgdaInductiveConstructor{false}\AgdaSpace{}%
\AgdaSymbol{|}\AgdaSpace{}%
\AgdaInductiveConstructor{true}\AgdaSpace{}%
\AgdaSymbol{|}\AgdaSpace{}%
\AgdaInductiveConstructor{true}\AgdaSpace{}%
\AgdaKeyword{with}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaFunction{isSigned}%
\>[121]\AgdaBound{msg₁}\AgdaSpace{}%
\AgdaBound{sig3}\AgdaSpace{}%
\AgdaBound{pbk4}\AgdaSymbol{)}\<%
\\
\>[0]\AgdaFunction{lemmaHoareTripleStackGeAux'20}\AgdaSpace{}%
\AgdaBound{msg₁}\AgdaSpace{}%
\AgdaBound{pbk1}\AgdaSpace{}%
\AgdaBound{pbk2}\AgdaSpace{}%
\AgdaBound{pbk3}\AgdaSpace{}%
\AgdaBound{pbk4}\AgdaSpace{}%
\AgdaBound{pbk5}\AgdaSpace{}%
\AgdaBound{sig1}\AgdaSpace{}%
\AgdaBound{sig2}\AgdaSpace{}%
\AgdaBound{sig3}\AgdaSpace{}%
\AgdaBound{x}\AgdaSpace{}%
\AgdaBound{x₁}\AgdaSpace{}%
\AgdaBound{x₂}\AgdaSpace{}%
\AgdaSymbol{|}\AgdaSpace{}%
\AgdaInductiveConstructor{false}\AgdaSpace{}%
\AgdaSymbol{|}\AgdaSpace{}%
\AgdaInductiveConstructor{true}\AgdaSpace{}%
\AgdaSymbol{|}\AgdaSpace{}%
\AgdaInductiveConstructor{true}\AgdaSpace{}%
\AgdaSymbol{|}\AgdaSpace{}%
\AgdaInductiveConstructor{true}\AgdaSpace{}%
\AgdaSymbol{=}\AgdaSpace{}%
\AgdaInductiveConstructor{tt}\<%
\\
\>[0]\AgdaFunction{lemmaHoareTripleStackGeAux'20}\AgdaSpace{}%
\AgdaBound{msg₁}\AgdaSpace{}%
\AgdaBound{pbk1}\AgdaSpace{}%
\AgdaBound{pbk2}\AgdaSpace{}%
\AgdaBound{pbk3}\AgdaSpace{}%
\AgdaBound{pbk4}\AgdaSpace{}%
\AgdaBound{pbk5}\AgdaSpace{}%
\AgdaBound{sig1}\AgdaSpace{}%
\AgdaBound{sig2}\AgdaSpace{}%
\AgdaBound{sig3}\AgdaSpace{}%
\AgdaBound{x}\AgdaSpace{}%
\AgdaBound{x₁}\AgdaSpace{}%
\AgdaBound{x₂}\AgdaSpace{}%
\AgdaSymbol{|}\AgdaSpace{}%
\AgdaInductiveConstructor{true}\AgdaSpace{}%
\AgdaKeyword{with}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaFunction{isSigned}%
\>[106]\AgdaBound{msg₁}\AgdaSpace{}%
\AgdaBound{sig2}\AgdaSpace{}%
\AgdaBound{pbk2}\AgdaSymbol{)}\<%
\\
\>[0]\AgdaFunction{lemmaHoareTripleStackGeAux'20}\AgdaSpace{}%
\AgdaBound{msg₁}\AgdaSpace{}%
\AgdaBound{pbk1}\AgdaSpace{}%
\AgdaBound{pbk2}\AgdaSpace{}%
\AgdaBound{pbk3}\AgdaSpace{}%
\AgdaBound{pbk4}\AgdaSpace{}%
\AgdaBound{pbk5}\AgdaSpace{}%
\AgdaBound{sig1}\AgdaSpace{}%
\AgdaBound{sig2}\AgdaSpace{}%
\AgdaBound{sig3}\AgdaSpace{}%
\AgdaBound{x}\AgdaSpace{}%
\AgdaBound{x₁}\AgdaSpace{}%
\AgdaBound{x₂}\AgdaSpace{}%
\AgdaSymbol{|}\AgdaSpace{}%
\AgdaInductiveConstructor{true}\AgdaSpace{}%
\AgdaSymbol{|}\AgdaSpace{}%
\AgdaInductiveConstructor{false}\AgdaSpace{}%
\AgdaKeyword{with}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaFunction{isSigned}%
\>[114]\AgdaBound{msg₁}\AgdaSpace{}%
\AgdaBound{sig2}\AgdaSpace{}%
\AgdaBound{pbk3}\AgdaSymbol{)}\<%
\\
\>[0]\AgdaFunction{lemmaHoareTripleStackGeAux'20}\AgdaSpace{}%
\AgdaBound{msg₁}\AgdaSpace{}%
\AgdaBound{pbk1}\AgdaSpace{}%
\AgdaBound{pbk2}\AgdaSpace{}%
\AgdaBound{pbk3}\AgdaSpace{}%
\AgdaBound{pbk4}\AgdaSpace{}%
\AgdaBound{pbk5}\AgdaSpace{}%
\AgdaBound{sig1}\AgdaSpace{}%
\AgdaBound{sig2}\AgdaSpace{}%
\AgdaBound{sig3}\AgdaSpace{}%
\AgdaBound{x}\AgdaSpace{}%
\AgdaBound{x₁}\AgdaSpace{}%
\AgdaBound{x₂}\AgdaSpace{}%
\AgdaSymbol{|}\AgdaSpace{}%
\AgdaInductiveConstructor{true}\AgdaSpace{}%
\AgdaSymbol{|}\AgdaSpace{}%
\AgdaInductiveConstructor{false}\AgdaSpace{}%
\AgdaSymbol{|}\AgdaSpace{}%
\AgdaInductiveConstructor{true}\AgdaSpace{}%
\AgdaKeyword{with}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaFunction{isSigned}%
\>[121]\AgdaBound{msg₁}\AgdaSpace{}%
\AgdaBound{sig3}\AgdaSpace{}%
\AgdaBound{pbk4}\AgdaSymbol{)}\<%
\\
\>[0]\AgdaFunction{lemmaHoareTripleStackGeAux'20}\AgdaSpace{}%
\AgdaBound{msg₁}\AgdaSpace{}%
\AgdaBound{pbk1}\AgdaSpace{}%
\AgdaBound{pbk2}\AgdaSpace{}%
\AgdaBound{pbk3}\AgdaSpace{}%
\AgdaBound{pbk4}\AgdaSpace{}%
\AgdaBound{pbk5}\AgdaSpace{}%
\AgdaBound{sig1}\AgdaSpace{}%
\AgdaBound{sig2}\AgdaSpace{}%
\AgdaBound{sig3}\AgdaSpace{}%
\AgdaBound{x}\AgdaSpace{}%
\AgdaBound{x₁}\AgdaSpace{}%
\AgdaBound{x₂}\AgdaSpace{}%
\AgdaSymbol{|}\AgdaSpace{}%
\AgdaInductiveConstructor{true}\AgdaSpace{}%
\AgdaSymbol{|}\AgdaSpace{}%
\AgdaInductiveConstructor{false}\AgdaSpace{}%
\AgdaSymbol{|}\AgdaSpace{}%
\AgdaInductiveConstructor{true}\AgdaSpace{}%
\AgdaSymbol{|}\AgdaSpace{}%
\AgdaInductiveConstructor{true}\AgdaSpace{}%
\AgdaSymbol{=}\AgdaSpace{}%
\AgdaInductiveConstructor{tt}\<%
\\
\>[0]\AgdaFunction{lemmaHoareTripleStackGeAux'20}\AgdaSpace{}%
\AgdaBound{msg₁}\AgdaSpace{}%
\AgdaBound{pbk1}\AgdaSpace{}%
\AgdaBound{pbk2}\AgdaSpace{}%
\AgdaBound{pbk3}\AgdaSpace{}%
\AgdaBound{pbk4}\AgdaSpace{}%
\AgdaBound{pbk5}\AgdaSpace{}%
\AgdaBound{sig1}\AgdaSpace{}%
\AgdaBound{sig2}\AgdaSpace{}%
\AgdaBound{sig3}\AgdaSpace{}%
\AgdaBound{x}\AgdaSpace{}%
\AgdaBound{x₁}\AgdaSpace{}%
\AgdaBound{x₂}\AgdaSpace{}%
\AgdaSymbol{|}\AgdaSpace{}%
\AgdaInductiveConstructor{true}\AgdaSpace{}%
\AgdaSymbol{|}\AgdaSpace{}%
\AgdaInductiveConstructor{true}\AgdaSpace{}%
\AgdaKeyword{with}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaFunction{isSigned}%
\>[113]\AgdaBound{msg₁}\AgdaSpace{}%
\AgdaBound{sig3}\AgdaSpace{}%
\AgdaBound{pbk3}\AgdaSymbol{)}\<%
\\
\>[0]\AgdaFunction{lemmaHoareTripleStackGeAux'20}\AgdaSpace{}%
\AgdaBound{msg₁}\AgdaSpace{}%
\AgdaBound{pbk1}\AgdaSpace{}%
\AgdaBound{pbk2}\AgdaSpace{}%
\AgdaBound{pbk3}\AgdaSpace{}%
\AgdaBound{pbk4}\AgdaSpace{}%
\AgdaBound{pbk5}\AgdaSpace{}%
\AgdaBound{sig1}\AgdaSpace{}%
\AgdaBound{sig2}\AgdaSpace{}%
\AgdaBound{sig3}\AgdaSpace{}%
\AgdaBound{x}\AgdaSpace{}%
\AgdaBound{x₁}\AgdaSpace{}%
\AgdaBound{x₂}\AgdaSpace{}%
\AgdaSymbol{|}\AgdaSpace{}%
\AgdaInductiveConstructor{true}\AgdaSpace{}%
\AgdaSymbol{|}\AgdaSpace{}%
\AgdaInductiveConstructor{true}\AgdaSpace{}%
\AgdaSymbol{|}\AgdaSpace{}%
\AgdaInductiveConstructor{false}\AgdaSpace{}%
\AgdaKeyword{with}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaFunction{isSigned}%
\>[121]\AgdaBound{msg₁}\AgdaSpace{}%
\AgdaBound{sig3}\AgdaSpace{}%
\AgdaBound{pbk4}\AgdaSymbol{)}\<%
\\
\>[0]\AgdaFunction{lemmaHoareTripleStackGeAux'20}\AgdaSpace{}%
\AgdaBound{msg₁}\AgdaSpace{}%
\AgdaBound{pbk1}\AgdaSpace{}%
\AgdaBound{pbk2}\AgdaSpace{}%
\AgdaBound{pbk3}\AgdaSpace{}%
\AgdaBound{pbk4}\AgdaSpace{}%
\AgdaBound{pbk5}\AgdaSpace{}%
\AgdaBound{sig1}\AgdaSpace{}%
\AgdaBound{sig2}\AgdaSpace{}%
\AgdaBound{sig3}\AgdaSpace{}%
\AgdaBound{x}\AgdaSpace{}%
\AgdaBound{x₁}\AgdaSpace{}%
\AgdaBound{x₂}\AgdaSpace{}%
\AgdaSymbol{|}\AgdaSpace{}%
\AgdaInductiveConstructor{true}\AgdaSpace{}%
\AgdaSymbol{|}\AgdaSpace{}%
\AgdaInductiveConstructor{true}\AgdaSpace{}%
\AgdaSymbol{|}\AgdaSpace{}%
\AgdaInductiveConstructor{false}\AgdaSpace{}%
\AgdaSymbol{|}\AgdaSpace{}%
\AgdaInductiveConstructor{true}\AgdaSpace{}%
\AgdaSymbol{=}\AgdaSpace{}%
\AgdaInductiveConstructor{tt}\<%
\\
\>[0]\AgdaFunction{lemmaHoareTripleStackGeAux'20}\AgdaSpace{}%
\AgdaBound{msg₁}\AgdaSpace{}%
\AgdaBound{pbk1}\AgdaSpace{}%
\AgdaBound{pbk2}\AgdaSpace{}%
\AgdaBound{pbk3}\AgdaSpace{}%
\AgdaBound{pbk4}\AgdaSpace{}%
\AgdaBound{pbk5}\AgdaSpace{}%
\AgdaBound{sig1}\AgdaSpace{}%
\AgdaBound{sig2}\AgdaSpace{}%
\AgdaBound{sig3}\AgdaSpace{}%
\AgdaBound{x}\AgdaSpace{}%
\AgdaBound{x₁}\AgdaSpace{}%
\AgdaBound{x₂}\AgdaSpace{}%
\AgdaSymbol{|}\AgdaSpace{}%
\AgdaInductiveConstructor{true}\AgdaSpace{}%
\AgdaSymbol{|}\AgdaSpace{}%
\AgdaInductiveConstructor{true}\AgdaSpace{}%
\AgdaSymbol{|}\AgdaSpace{}%
\AgdaInductiveConstructor{true}\AgdaSpace{}%
\AgdaSymbol{=}\AgdaSpace{}%
\AgdaInductiveConstructor{tt}\<%
\\
%
\\[\AgdaEmptyExtraSkip]%
%
\\[\AgdaEmptyExtraSkip]%
%
\\[\AgdaEmptyExtraSkip]%
\>[0]\AgdaFunction{lemmaHoareTripleStackGeAux'21}%
\>[4767I]\AgdaSymbol{:}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaBound{msg}\AgdaSpace{}%
\AgdaSymbol{:}\AgdaSpace{}%
\AgdaDatatype{Msg}\AgdaSymbol{)}\<%
\\
\>[4767I][@{}l@{\AgdaIndent{0}}]%
\>[31]\AgdaSymbol{(}\AgdaBound{pbk1}\AgdaSpace{}%
\AgdaBound{pbk2}\AgdaSpace{}%
\AgdaBound{pbk3}\AgdaSpace{}%
\AgdaBound{pbk4}\AgdaSpace{}%
\AgdaBound{pbk5}\AgdaSpace{}%
\AgdaBound{sig1}\AgdaSpace{}%
\AgdaBound{sig2}\AgdaSpace{}%
\AgdaBound{sig3}\AgdaSpace{}%
\AgdaSymbol{:}\AgdaSpace{}%
\AgdaDatatype{ℕ}\AgdaSymbol{)}\<%
\\
%
\>[31]\AgdaSymbol{→}\AgdaSpace{}%
\AgdaFunction{True}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaFunction{isSigned}%
\>[49]\AgdaBound{msg}\AgdaSpace{}%
\AgdaBound{sig3}\AgdaSpace{}%
\AgdaBound{pbk5}\AgdaSymbol{)}\<%
\\
\>[.][@{}l@{}]\<[4767I]%
\>[30]\AgdaSymbol{→}%
\>[33]\AgdaFunction{True}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaFunction{isSigned}%
\>[49]\AgdaBound{msg}\AgdaSpace{}%
\AgdaBound{sig2}\AgdaSpace{}%
\AgdaBound{pbk3}\AgdaSymbol{)}\<%
\\
%
\>[30]\AgdaSymbol{→}%
\>[33]\AgdaFunction{True}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaFunction{isSigned}%
\>[49]\AgdaBound{msg}\AgdaSpace{}%
\AgdaBound{sig1}\AgdaSpace{}%
\AgdaBound{pbk2}\AgdaSymbol{)}\<%
\\
\>[30][@{}l@{\AgdaIndent{0}}]%
\>[31]\AgdaSymbol{→}\AgdaSpace{}%
\AgdaFunction{True}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaFunction{compareSigsMultiSig}\AgdaSpace{}%
\AgdaBound{msg}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaSpace{}%
\AgdaBound{sig1}\AgdaSpace{}%
\AgdaOperator{\AgdaInductiveConstructor{∷}}\AgdaSpace{}%
\AgdaBound{sig2}\AgdaSpace{}%
\AgdaOperator{\AgdaInductiveConstructor{∷}}\AgdaSpace{}%
\AgdaBound{sig3}\AgdaSpace{}%
\AgdaOperator{\AgdaInductiveConstructor{∷}}\AgdaSpace{}%
\AgdaInductiveConstructor{[]}\AgdaSymbol{)}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaBound{pbk1}\AgdaSpace{}%
\AgdaOperator{\AgdaInductiveConstructor{∷}}\AgdaSpace{}%
\AgdaBound{pbk2}\AgdaSpace{}%
\AgdaOperator{\AgdaInductiveConstructor{∷}}\AgdaSpace{}%
\AgdaBound{pbk3}\AgdaSpace{}%
\AgdaOperator{\AgdaInductiveConstructor{∷}}\AgdaSpace{}%
\AgdaBound{pbk4}\AgdaSpace{}%
\AgdaOperator{\AgdaInductiveConstructor{∷}}\AgdaSpace{}%
\AgdaBound{pbk5}\AgdaSpace{}%
\AgdaOperator{\AgdaInductiveConstructor{∷}}\AgdaSpace{}%
\AgdaInductiveConstructor{[]}\AgdaSymbol{))}\<%
\\
\>[0]\AgdaFunction{lemmaHoareTripleStackGeAux'21}\AgdaSpace{}%
\AgdaBound{msg₁}\AgdaSpace{}%
\AgdaBound{pbk1}\AgdaSpace{}%
\AgdaBound{pbk2}\AgdaSpace{}%
\AgdaBound{pbk3}\AgdaSpace{}%
\AgdaBound{pbk4}\AgdaSpace{}%
\AgdaBound{pbk5}\AgdaSpace{}%
\AgdaBound{sig1}\AgdaSpace{}%
\AgdaBound{sig2}\AgdaSpace{}%
\AgdaBound{sig3}\AgdaSpace{}%
\AgdaBound{x}\AgdaSpace{}%
\AgdaBound{x₁}\AgdaSpace{}%
\AgdaBound{x₂}\AgdaSpace{}%
\AgdaKeyword{with}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaFunction{isSigned}%
\>[99]\AgdaBound{msg₁}\AgdaSpace{}%
\AgdaBound{sig1}\AgdaSpace{}%
\AgdaBound{pbk1}\AgdaSymbol{)}\<%
\\
\>[0]\AgdaFunction{lemmaHoareTripleStackGeAux'21}\AgdaSpace{}%
\AgdaBound{msg₁}\AgdaSpace{}%
\AgdaBound{pbk1}\AgdaSpace{}%
\AgdaBound{pbk2}\AgdaSpace{}%
\AgdaBound{pbk3}\AgdaSpace{}%
\AgdaBound{pbk4}\AgdaSpace{}%
\AgdaBound{pbk5}\AgdaSpace{}%
\AgdaBound{sig1}\AgdaSpace{}%
\AgdaBound{sig2}\AgdaSpace{}%
\AgdaBound{sig3}\AgdaSpace{}%
\AgdaBound{x}\AgdaSpace{}%
\AgdaBound{x₁}\AgdaSpace{}%
\AgdaBound{x₂}\AgdaSpace{}%
\AgdaSymbol{|}\AgdaSpace{}%
\AgdaInductiveConstructor{false}\AgdaSpace{}%
\AgdaKeyword{with}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaFunction{isSigned}%
\>[107]\AgdaBound{msg₁}\AgdaSpace{}%
\AgdaBound{sig1}\AgdaSpace{}%
\AgdaBound{pbk2}\AgdaSymbol{)}\<%
\\
\>[0]\AgdaFunction{lemmaHoareTripleStackGeAux'21}\AgdaSpace{}%
\AgdaBound{msg₁}\AgdaSpace{}%
\AgdaBound{pbk1}\AgdaSpace{}%
\AgdaBound{pbk2}\AgdaSpace{}%
\AgdaBound{pbk3}\AgdaSpace{}%
\AgdaBound{pbk4}\AgdaSpace{}%
\AgdaBound{pbk5}\AgdaSpace{}%
\AgdaBound{sig1}\AgdaSpace{}%
\AgdaBound{sig2}\AgdaSpace{}%
\AgdaBound{sig3}\AgdaSpace{}%
\AgdaBound{x}\AgdaSpace{}%
\AgdaBound{x₁}\AgdaSpace{}%
\AgdaBound{x₂}\AgdaSpace{}%
\AgdaSymbol{|}\AgdaSpace{}%
\AgdaInductiveConstructor{false}\AgdaSpace{}%
\AgdaSymbol{|}\AgdaSpace{}%
\AgdaInductiveConstructor{true}\AgdaSpace{}%
\AgdaKeyword{with}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaFunction{isSigned}%
\>[114]\AgdaBound{msg₁}\AgdaSpace{}%
\AgdaBound{sig2}\AgdaSpace{}%
\AgdaBound{pbk3}\AgdaSymbol{)}\<%
\\
\>[0]\AgdaFunction{lemmaHoareTripleStackGeAux'21}\AgdaSpace{}%
\AgdaBound{msg₁}\AgdaSpace{}%
\AgdaBound{pbk1}\AgdaSpace{}%
\AgdaBound{pbk2}\AgdaSpace{}%
\AgdaBound{pbk3}\AgdaSpace{}%
\AgdaBound{pbk4}\AgdaSpace{}%
\AgdaBound{pbk5}\AgdaSpace{}%
\AgdaBound{sig1}\AgdaSpace{}%
\AgdaBound{sig2}\AgdaSpace{}%
\AgdaBound{sig3}\AgdaSpace{}%
\AgdaBound{x}\AgdaSpace{}%
\AgdaBound{x₁}\AgdaSpace{}%
\AgdaBound{x₂}\AgdaSpace{}%
\AgdaSymbol{|}\AgdaSpace{}%
\AgdaInductiveConstructor{false}\AgdaSpace{}%
\AgdaSymbol{|}\AgdaSpace{}%
\AgdaInductiveConstructor{true}\AgdaSpace{}%
\AgdaSymbol{|}\AgdaSpace{}%
\AgdaInductiveConstructor{true}\AgdaSpace{}%
\AgdaKeyword{with}%
\>[111]\AgdaSymbol{(}\AgdaFunction{isSigned}%
\>[122]\AgdaBound{msg₁}\AgdaSpace{}%
\AgdaBound{sig3}\AgdaSpace{}%
\AgdaBound{pbk4}\AgdaSymbol{)}\<%
\\
\>[0]\AgdaFunction{lemmaHoareTripleStackGeAux'21}\AgdaSpace{}%
\AgdaBound{msg₁}\AgdaSpace{}%
\AgdaBound{pbk1}\AgdaSpace{}%
\AgdaBound{pbk2}\AgdaSpace{}%
\AgdaBound{pbk3}\AgdaSpace{}%
\AgdaBound{pbk4}\AgdaSpace{}%
\AgdaBound{pbk5}\AgdaSpace{}%
\AgdaBound{sig1}\AgdaSpace{}%
\AgdaBound{sig2}\AgdaSpace{}%
\AgdaBound{sig3}\AgdaSpace{}%
\AgdaBound{x}\AgdaSpace{}%
\AgdaBound{x₁}\AgdaSpace{}%
\AgdaBound{x₂}\AgdaSpace{}%
\AgdaSymbol{|}\AgdaSpace{}%
\AgdaInductiveConstructor{false}\AgdaSpace{}%
\AgdaSymbol{|}\AgdaSpace{}%
\AgdaInductiveConstructor{true}\AgdaSpace{}%
\AgdaSymbol{|}\AgdaSpace{}%
\AgdaInductiveConstructor{true}\AgdaSpace{}%
\AgdaSymbol{|}\AgdaSpace{}%
\AgdaInductiveConstructor{false}\AgdaSpace{}%
\AgdaKeyword{with}%
\>[119]\AgdaSymbol{(}\AgdaFunction{isSigned}%
\>[130]\AgdaBound{msg₁}\AgdaSpace{}%
\AgdaBound{sig3}\AgdaSpace{}%
\AgdaBound{pbk5}\AgdaSymbol{)}\<%
\\
\>[0]\AgdaFunction{lemmaHoareTripleStackGeAux'21}\AgdaSpace{}%
\AgdaBound{msg₁}\AgdaSpace{}%
\AgdaBound{pbk1}\AgdaSpace{}%
\AgdaBound{pbk2}\AgdaSpace{}%
\AgdaBound{pbk3}\AgdaSpace{}%
\AgdaBound{pbk4}\AgdaSpace{}%
\AgdaBound{pbk5}\AgdaSpace{}%
\AgdaBound{sig1}\AgdaSpace{}%
\AgdaBound{sig2}\AgdaSpace{}%
\AgdaBound{sig3}\AgdaSpace{}%
\AgdaBound{x}\AgdaSpace{}%
\AgdaBound{x₁}\AgdaSpace{}%
\AgdaBound{x₂}\AgdaSpace{}%
\AgdaSymbol{|}\AgdaSpace{}%
\AgdaInductiveConstructor{false}\AgdaSpace{}%
\AgdaSymbol{|}\AgdaSpace{}%
\AgdaInductiveConstructor{true}\AgdaSpace{}%
\AgdaSymbol{|}\AgdaSpace{}%
\AgdaInductiveConstructor{true}\AgdaSpace{}%
\AgdaSymbol{|}\AgdaSpace{}%
\AgdaInductiveConstructor{false}\AgdaSpace{}%
\AgdaSymbol{|}\AgdaSpace{}%
\AgdaInductiveConstructor{true}\AgdaSpace{}%
\AgdaSymbol{=}\AgdaSpace{}%
\AgdaInductiveConstructor{tt}\<%
\\
\>[0]\AgdaFunction{lemmaHoareTripleStackGeAux'21}\AgdaSpace{}%
\AgdaBound{msg₁}\AgdaSpace{}%
\AgdaBound{pbk1}\AgdaSpace{}%
\AgdaBound{pbk2}\AgdaSpace{}%
\AgdaBound{pbk3}\AgdaSpace{}%
\AgdaBound{pbk4}\AgdaSpace{}%
\AgdaBound{pbk5}\AgdaSpace{}%
\AgdaBound{sig1}\AgdaSpace{}%
\AgdaBound{sig2}\AgdaSpace{}%
\AgdaBound{sig3}\AgdaSpace{}%
\AgdaBound{x}\AgdaSpace{}%
\AgdaBound{x₁}\AgdaSpace{}%
\AgdaBound{x₂}\AgdaSpace{}%
\AgdaSymbol{|}\AgdaSpace{}%
\AgdaInductiveConstructor{false}\AgdaSpace{}%
\AgdaSymbol{|}\AgdaSpace{}%
\AgdaInductiveConstructor{true}\AgdaSpace{}%
\AgdaSymbol{|}\AgdaSpace{}%
\AgdaInductiveConstructor{true}\AgdaSpace{}%
\AgdaSymbol{|}\AgdaSpace{}%
\AgdaInductiveConstructor{true}\AgdaSpace{}%
\AgdaSymbol{=}\AgdaSpace{}%
\AgdaInductiveConstructor{tt}\<%
\\
\>[0]\AgdaFunction{lemmaHoareTripleStackGeAux'21}\AgdaSpace{}%
\AgdaBound{msg₁}\AgdaSpace{}%
\AgdaBound{pbk1}\AgdaSpace{}%
\AgdaBound{pbk2}\AgdaSpace{}%
\AgdaBound{pbk3}\AgdaSpace{}%
\AgdaBound{pbk4}\AgdaSpace{}%
\AgdaBound{pbk5}\AgdaSpace{}%
\AgdaBound{sig1}\AgdaSpace{}%
\AgdaBound{sig2}\AgdaSpace{}%
\AgdaBound{sig3}\AgdaSpace{}%
\AgdaBound{x}\AgdaSpace{}%
\AgdaBound{x₁}\AgdaSpace{}%
\AgdaBound{x₂}\AgdaSpace{}%
\AgdaSymbol{|}\AgdaSpace{}%
\AgdaInductiveConstructor{true}\AgdaSpace{}%
\AgdaKeyword{with}%
\>[96]\AgdaSymbol{(}\AgdaFunction{isSigned}%
\>[107]\AgdaBound{msg₁}\AgdaSpace{}%
\AgdaBound{sig2}\AgdaSpace{}%
\AgdaBound{pbk2}\AgdaSymbol{)}\<%
\\
\>[0]\AgdaFunction{lemmaHoareTripleStackGeAux'21}\AgdaSpace{}%
\AgdaBound{msg₁}\AgdaSpace{}%
\AgdaBound{pbk1}\AgdaSpace{}%
\AgdaBound{pbk2}\AgdaSpace{}%
\AgdaBound{pbk3}\AgdaSpace{}%
\AgdaBound{pbk4}\AgdaSpace{}%
\AgdaBound{pbk5}\AgdaSpace{}%
\AgdaBound{sig1}\AgdaSpace{}%
\AgdaBound{sig2}\AgdaSpace{}%
\AgdaBound{sig3}\AgdaSpace{}%
\AgdaBound{x}\AgdaSpace{}%
\AgdaBound{x₁}\AgdaSpace{}%
\AgdaBound{x₂}\AgdaSpace{}%
\AgdaSymbol{|}\AgdaSpace{}%
\AgdaInductiveConstructor{true}\AgdaSpace{}%
\AgdaSymbol{|}\AgdaSpace{}%
\AgdaInductiveConstructor{false}\AgdaSpace{}%
\AgdaKeyword{with}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaFunction{isSigned}%
\>[114]\AgdaBound{msg₁}\AgdaSpace{}%
\AgdaBound{sig2}\AgdaSpace{}%
\AgdaBound{pbk3}\AgdaSymbol{)}\<%
\\
\>[0]\AgdaFunction{lemmaHoareTripleStackGeAux'21}\AgdaSpace{}%
\AgdaBound{msg₁}\AgdaSpace{}%
\AgdaBound{pbk1}\AgdaSpace{}%
\AgdaBound{pbk2}\AgdaSpace{}%
\AgdaBound{pbk3}\AgdaSpace{}%
\AgdaBound{pbk4}\AgdaSpace{}%
\AgdaBound{pbk5}\AgdaSpace{}%
\AgdaBound{sig1}\AgdaSpace{}%
\AgdaBound{sig2}\AgdaSpace{}%
\AgdaBound{sig3}\AgdaSpace{}%
\AgdaBound{x}\AgdaSpace{}%
\AgdaBound{x₁}\AgdaSpace{}%
\AgdaBound{x₂}\AgdaSpace{}%
\AgdaSymbol{|}\AgdaSpace{}%
\AgdaInductiveConstructor{true}\AgdaSpace{}%
\AgdaSymbol{|}\AgdaSpace{}%
\AgdaInductiveConstructor{false}\AgdaSpace{}%
\AgdaSymbol{|}\AgdaSpace{}%
\AgdaInductiveConstructor{true}\AgdaSpace{}%
\AgdaKeyword{with}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaFunction{isSigned}%
\>[121]\AgdaBound{msg₁}\AgdaSpace{}%
\AgdaBound{sig3}\AgdaSpace{}%
\AgdaBound{pbk4}\AgdaSymbol{)}\<%
\\
\>[0]\AgdaFunction{lemmaHoareTripleStackGeAux'21}\AgdaSpace{}%
\AgdaBound{msg₁}\AgdaSpace{}%
\AgdaBound{pbk1}\AgdaSpace{}%
\AgdaBound{pbk2}\AgdaSpace{}%
\AgdaBound{pbk3}\AgdaSpace{}%
\AgdaBound{pbk4}\AgdaSpace{}%
\AgdaBound{pbk5}\AgdaSpace{}%
\AgdaBound{sig1}\AgdaSpace{}%
\AgdaBound{sig2}\AgdaSpace{}%
\AgdaBound{sig3}\AgdaSpace{}%
\AgdaBound{x}\AgdaSpace{}%
\AgdaBound{x₁}\AgdaSpace{}%
\AgdaBound{x₂}\AgdaSpace{}%
\AgdaSymbol{|}\AgdaSpace{}%
\AgdaInductiveConstructor{true}\AgdaSpace{}%
\AgdaSymbol{|}\AgdaSpace{}%
\AgdaInductiveConstructor{false}\AgdaSpace{}%
\AgdaSymbol{|}\AgdaSpace{}%
\AgdaInductiveConstructor{true}\AgdaSpace{}%
\AgdaSymbol{|}\AgdaSpace{}%
\AgdaInductiveConstructor{false}\AgdaSpace{}%
\AgdaKeyword{with}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaFunction{isSigned}%
\>[129]\AgdaBound{msg₁}\AgdaSpace{}%
\AgdaBound{sig3}\AgdaSpace{}%
\AgdaBound{pbk5}\AgdaSymbol{)}\<%
\\
\>[0]\AgdaFunction{lemmaHoareTripleStackGeAux'21}\AgdaSpace{}%
\AgdaBound{msg₁}\AgdaSpace{}%
\AgdaBound{pbk1}\AgdaSpace{}%
\AgdaBound{pbk2}\AgdaSpace{}%
\AgdaBound{pbk3}\AgdaSpace{}%
\AgdaBound{pbk4}\AgdaSpace{}%
\AgdaBound{pbk5}\AgdaSpace{}%
\AgdaBound{sig1}\AgdaSpace{}%
\AgdaBound{sig2}\AgdaSpace{}%
\AgdaBound{sig3}\AgdaSpace{}%
\AgdaBound{x}\AgdaSpace{}%
\AgdaBound{x₁}\AgdaSpace{}%
\AgdaBound{x₂}\AgdaSpace{}%
\AgdaSymbol{|}\AgdaSpace{}%
\AgdaInductiveConstructor{true}\AgdaSpace{}%
\AgdaSymbol{|}\AgdaSpace{}%
\AgdaInductiveConstructor{false}\AgdaSpace{}%
\AgdaSymbol{|}\AgdaSpace{}%
\AgdaInductiveConstructor{true}\AgdaSpace{}%
\AgdaSymbol{|}\AgdaSpace{}%
\AgdaInductiveConstructor{false}\AgdaSpace{}%
\AgdaSymbol{|}\AgdaSpace{}%
\AgdaInductiveConstructor{true}\AgdaSpace{}%
\AgdaSymbol{=}\AgdaSpace{}%
\AgdaInductiveConstructor{tt}\<%
\\
\>[0]\AgdaFunction{lemmaHoareTripleStackGeAux'21}\AgdaSpace{}%
\AgdaBound{msg₁}\AgdaSpace{}%
\AgdaBound{pbk1}\AgdaSpace{}%
\AgdaBound{pbk2}\AgdaSpace{}%
\AgdaBound{pbk3}\AgdaSpace{}%
\AgdaBound{pbk4}\AgdaSpace{}%
\AgdaBound{pbk5}\AgdaSpace{}%
\AgdaBound{sig1}\AgdaSpace{}%
\AgdaBound{sig2}\AgdaSpace{}%
\AgdaBound{sig3}\AgdaSpace{}%
\AgdaBound{x}\AgdaSpace{}%
\AgdaBound{x₁}\AgdaSpace{}%
\AgdaBound{x₂}\AgdaSpace{}%
\AgdaSymbol{|}\AgdaSpace{}%
\AgdaInductiveConstructor{true}\AgdaSpace{}%
\AgdaSymbol{|}\AgdaSpace{}%
\AgdaInductiveConstructor{false}\AgdaSpace{}%
\AgdaSymbol{|}\AgdaSpace{}%
\AgdaInductiveConstructor{true}\AgdaSpace{}%
\AgdaSymbol{|}\AgdaSpace{}%
\AgdaInductiveConstructor{true}\AgdaSpace{}%
\AgdaSymbol{=}\AgdaSpace{}%
\AgdaInductiveConstructor{tt}\<%
\\
\>[0]\AgdaFunction{lemmaHoareTripleStackGeAux'21}\AgdaSpace{}%
\AgdaBound{msg₁}\AgdaSpace{}%
\AgdaBound{pbk1}\AgdaSpace{}%
\AgdaBound{pbk2}\AgdaSpace{}%
\AgdaBound{pbk3}\AgdaSpace{}%
\AgdaBound{pbk4}\AgdaSpace{}%
\AgdaBound{pbk5}\AgdaSpace{}%
\AgdaBound{sig1}\AgdaSpace{}%
\AgdaBound{sig2}\AgdaSpace{}%
\AgdaBound{sig3}\AgdaSpace{}%
\AgdaBound{x}\AgdaSpace{}%
\AgdaBound{x₁}\AgdaSpace{}%
\AgdaBound{x₂}\AgdaSpace{}%
\AgdaSymbol{|}\AgdaSpace{}%
\AgdaInductiveConstructor{true}\AgdaSpace{}%
\AgdaSymbol{|}\AgdaSpace{}%
\AgdaInductiveConstructor{true}\AgdaSpace{}%
\AgdaKeyword{with}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaFunction{isSigned}%
\>[113]\AgdaBound{msg₁}\AgdaSpace{}%
\AgdaBound{sig3}\AgdaSpace{}%
\AgdaBound{pbk3}\AgdaSymbol{)}\<%
\\
\>[0]\AgdaFunction{lemmaHoareTripleStackGeAux'21}\AgdaSpace{}%
\AgdaBound{msg₁}\AgdaSpace{}%
\AgdaBound{pbk1}\AgdaSpace{}%
\AgdaBound{pbk2}\AgdaSpace{}%
\AgdaBound{pbk3}\AgdaSpace{}%
\AgdaBound{pbk4}\AgdaSpace{}%
\AgdaBound{pbk5}\AgdaSpace{}%
\AgdaBound{sig1}\AgdaSpace{}%
\AgdaBound{sig2}\AgdaSpace{}%
\AgdaBound{sig3}\AgdaSpace{}%
\AgdaBound{x}\AgdaSpace{}%
\AgdaBound{x₁}\AgdaSpace{}%
\AgdaBound{x₂}\AgdaSpace{}%
\AgdaSymbol{|}\AgdaSpace{}%
\AgdaInductiveConstructor{true}\AgdaSpace{}%
\AgdaSymbol{|}\AgdaSpace{}%
\AgdaInductiveConstructor{true}\AgdaSpace{}%
\AgdaSymbol{|}\AgdaSpace{}%
\AgdaInductiveConstructor{false}\AgdaSpace{}%
\AgdaKeyword{with}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaFunction{isSigned}%
\>[121]\AgdaBound{msg₁}\AgdaSpace{}%
\AgdaBound{sig3}\AgdaSpace{}%
\AgdaBound{pbk4}\AgdaSymbol{)}\<%
\\
\>[0]\AgdaFunction{lemmaHoareTripleStackGeAux'21}\AgdaSpace{}%
\AgdaBound{msg₁}\AgdaSpace{}%
\AgdaBound{pbk1}\AgdaSpace{}%
\AgdaBound{pbk2}\AgdaSpace{}%
\AgdaBound{pbk3}\AgdaSpace{}%
\AgdaBound{pbk4}\AgdaSpace{}%
\AgdaBound{pbk5}\AgdaSpace{}%
\AgdaBound{sig1}\AgdaSpace{}%
\AgdaBound{sig2}\AgdaSpace{}%
\AgdaBound{sig3}\AgdaSpace{}%
\AgdaBound{x}\AgdaSpace{}%
\AgdaBound{x₁}\AgdaSpace{}%
\AgdaBound{x₂}\AgdaSpace{}%
\AgdaSymbol{|}\AgdaSpace{}%
\AgdaInductiveConstructor{true}\AgdaSpace{}%
\AgdaSymbol{|}\AgdaSpace{}%
\AgdaInductiveConstructor{true}\AgdaSpace{}%
\AgdaSymbol{|}\AgdaSpace{}%
\AgdaInductiveConstructor{false}\AgdaSpace{}%
\AgdaSymbol{|}\AgdaSpace{}%
\AgdaInductiveConstructor{false}\AgdaSpace{}%
\AgdaKeyword{with}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaFunction{isSigned}%
\>[129]\AgdaBound{msg₁}\AgdaSpace{}%
\AgdaBound{sig3}\AgdaSpace{}%
\AgdaBound{pbk5}\AgdaSymbol{)}\<%
\\
\>[0]\AgdaFunction{lemmaHoareTripleStackGeAux'21}\AgdaSpace{}%
\AgdaBound{msg₁}\AgdaSpace{}%
\AgdaBound{pbk1}\AgdaSpace{}%
\AgdaBound{pbk2}\AgdaSpace{}%
\AgdaBound{pbk3}\AgdaSpace{}%
\AgdaBound{pbk4}\AgdaSpace{}%
\AgdaBound{pbk5}\AgdaSpace{}%
\AgdaBound{sig1}\AgdaSpace{}%
\AgdaBound{sig2}\AgdaSpace{}%
\AgdaBound{sig3}\AgdaSpace{}%
\AgdaBound{x}\AgdaSpace{}%
\AgdaBound{x₁}\AgdaSpace{}%
\AgdaBound{x₂}\AgdaSpace{}%
\AgdaSymbol{|}\AgdaSpace{}%
\AgdaInductiveConstructor{true}\AgdaSpace{}%
\AgdaSymbol{|}\AgdaSpace{}%
\AgdaInductiveConstructor{true}\AgdaSpace{}%
\AgdaSymbol{|}\AgdaSpace{}%
\AgdaInductiveConstructor{false}\AgdaSpace{}%
\AgdaSymbol{|}\AgdaSpace{}%
\AgdaInductiveConstructor{false}\AgdaSpace{}%
\AgdaSymbol{|}\AgdaSpace{}%
\AgdaInductiveConstructor{true}\AgdaSpace{}%
\AgdaSymbol{=}\AgdaSpace{}%
\AgdaInductiveConstructor{tt}\<%
\\
\>[0]\AgdaFunction{lemmaHoareTripleStackGeAux'21}\AgdaSpace{}%
\AgdaBound{msg₁}\AgdaSpace{}%
\AgdaBound{pbk1}\AgdaSpace{}%
\AgdaBound{pbk2}\AgdaSpace{}%
\AgdaBound{pbk3}\AgdaSpace{}%
\AgdaBound{pbk4}\AgdaSpace{}%
\AgdaBound{pbk5}\AgdaSpace{}%
\AgdaBound{sig1}\AgdaSpace{}%
\AgdaBound{sig2}\AgdaSpace{}%
\AgdaBound{sig3}\AgdaSpace{}%
\AgdaBound{x}\AgdaSpace{}%
\AgdaBound{x₁}\AgdaSpace{}%
\AgdaBound{x₂}\AgdaSpace{}%
\AgdaSymbol{|}\AgdaSpace{}%
\AgdaInductiveConstructor{true}\AgdaSpace{}%
\AgdaSymbol{|}\AgdaSpace{}%
\AgdaInductiveConstructor{true}\AgdaSpace{}%
\AgdaSymbol{|}\AgdaSpace{}%
\AgdaInductiveConstructor{false}\AgdaSpace{}%
\AgdaSymbol{|}\AgdaSpace{}%
\AgdaInductiveConstructor{true}\AgdaSpace{}%
\AgdaSymbol{=}\AgdaSpace{}%
\AgdaInductiveConstructor{tt}\<%
\\
\>[0]\AgdaFunction{lemmaHoareTripleStackGeAux'21}\AgdaSpace{}%
\AgdaBound{msg₁}\AgdaSpace{}%
\AgdaBound{pbk1}\AgdaSpace{}%
\AgdaBound{pbk2}\AgdaSpace{}%
\AgdaBound{pbk3}\AgdaSpace{}%
\AgdaBound{pbk4}\AgdaSpace{}%
\AgdaBound{pbk5}\AgdaSpace{}%
\AgdaBound{sig1}\AgdaSpace{}%
\AgdaBound{sig2}\AgdaSpace{}%
\AgdaBound{sig3}\AgdaSpace{}%
\AgdaBound{x}\AgdaSpace{}%
\AgdaBound{x₁}\AgdaSpace{}%
\AgdaBound{x₂}\AgdaSpace{}%
\AgdaSymbol{|}\AgdaSpace{}%
\AgdaInductiveConstructor{true}\AgdaSpace{}%
\AgdaSymbol{|}\AgdaSpace{}%
\AgdaInductiveConstructor{true}\AgdaSpace{}%
\AgdaSymbol{|}\AgdaSpace{}%
\AgdaInductiveConstructor{true}\AgdaSpace{}%
\AgdaSymbol{=}\AgdaSpace{}%
\AgdaInductiveConstructor{tt}\<%
\\
%
\\[\AgdaEmptyExtraSkip]%
%
\\[\AgdaEmptyExtraSkip]%
%
\\[\AgdaEmptyExtraSkip]%
%
\\[\AgdaEmptyExtraSkip]%
%
\\[\AgdaEmptyExtraSkip]%
\>[0]\AgdaFunction{lemmaHoareTripleStackGeAux'22}%
\>[5217I]\AgdaSymbol{:}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaBound{msg}\AgdaSpace{}%
\AgdaSymbol{:}\AgdaSpace{}%
\AgdaDatatype{Msg}\AgdaSymbol{)}\<%
\\
\>[5217I][@{}l@{\AgdaIndent{0}}]%
\>[31]\AgdaSymbol{(}\AgdaBound{pbk1}\AgdaSpace{}%
\AgdaBound{pbk2}\AgdaSpace{}%
\AgdaBound{pbk3}\AgdaSpace{}%
\AgdaBound{pbk4}\AgdaSpace{}%
\AgdaBound{pbk5}\AgdaSpace{}%
\AgdaBound{sig1}\AgdaSpace{}%
\AgdaBound{sig2}\AgdaSpace{}%
\AgdaBound{sig3}\AgdaSpace{}%
\AgdaSymbol{:}\AgdaSpace{}%
\AgdaDatatype{ℕ}\AgdaSymbol{)}\<%
\\
%
\>[31]\AgdaSymbol{→}\AgdaSpace{}%
\AgdaFunction{True}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaFunction{isSigned}%
\>[49]\AgdaBound{msg}\AgdaSpace{}%
\AgdaBound{sig3}\AgdaSpace{}%
\AgdaBound{pbk5}\AgdaSymbol{)}\<%
\\
\>[.][@{}l@{}]\<[5217I]%
\>[30]\AgdaSymbol{→}%
\>[33]\AgdaFunction{True}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaFunction{isSigned}%
\>[49]\AgdaBound{msg}\AgdaSpace{}%
\AgdaBound{sig2}\AgdaSpace{}%
\AgdaBound{pbk4}\AgdaSymbol{)}\<%
\\
%
\>[30]\AgdaSymbol{→}%
\>[33]\AgdaFunction{True}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaFunction{isSigned}%
\>[49]\AgdaBound{msg}\AgdaSpace{}%
\AgdaBound{sig1}\AgdaSpace{}%
\AgdaBound{pbk2}\AgdaSymbol{)}\<%
\\
\>[30][@{}l@{\AgdaIndent{0}}]%
\>[31]\AgdaSymbol{→}\AgdaSpace{}%
\AgdaFunction{True}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaFunction{compareSigsMultiSig}\AgdaSpace{}%
\AgdaBound{msg}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaSpace{}%
\AgdaBound{sig1}\AgdaSpace{}%
\AgdaOperator{\AgdaInductiveConstructor{∷}}\AgdaSpace{}%
\AgdaBound{sig2}\AgdaSpace{}%
\AgdaOperator{\AgdaInductiveConstructor{∷}}\AgdaSpace{}%
\AgdaBound{sig3}\AgdaSpace{}%
\AgdaOperator{\AgdaInductiveConstructor{∷}}\AgdaSpace{}%
\AgdaInductiveConstructor{[]}\AgdaSymbol{)}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaBound{pbk1}\AgdaSpace{}%
\AgdaOperator{\AgdaInductiveConstructor{∷}}\AgdaSpace{}%
\AgdaBound{pbk2}\AgdaSpace{}%
\AgdaOperator{\AgdaInductiveConstructor{∷}}\AgdaSpace{}%
\AgdaBound{pbk3}\AgdaSpace{}%
\AgdaOperator{\AgdaInductiveConstructor{∷}}\AgdaSpace{}%
\AgdaBound{pbk4}\AgdaSpace{}%
\AgdaOperator{\AgdaInductiveConstructor{∷}}\AgdaSpace{}%
\AgdaBound{pbk5}\AgdaSpace{}%
\AgdaOperator{\AgdaInductiveConstructor{∷}}\AgdaSpace{}%
\AgdaInductiveConstructor{[]}\AgdaSymbol{))}\<%
\\
\>[0]\AgdaFunction{lemmaHoareTripleStackGeAux'22}\AgdaSpace{}%
\AgdaBound{msg₁}\AgdaSpace{}%
\AgdaBound{pbk1}\AgdaSpace{}%
\AgdaBound{pbk2}\AgdaSpace{}%
\AgdaBound{pbk3}\AgdaSpace{}%
\AgdaBound{pbk4}\AgdaSpace{}%
\AgdaBound{pbk5}\AgdaSpace{}%
\AgdaBound{sig1}\AgdaSpace{}%
\AgdaBound{sig2}\AgdaSpace{}%
\AgdaBound{sig3}\AgdaSpace{}%
\AgdaBound{x}\AgdaSpace{}%
\AgdaBound{x₁}\AgdaSpace{}%
\AgdaBound{x₂}\AgdaSpace{}%
\AgdaKeyword{with}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaFunction{isSigned}%
\>[99]\AgdaBound{msg₁}\AgdaSpace{}%
\AgdaBound{sig1}\AgdaSpace{}%
\AgdaBound{pbk1}\AgdaSymbol{)}\<%
\\
\>[0]\AgdaFunction{lemmaHoareTripleStackGeAux'22}\AgdaSpace{}%
\AgdaBound{msg₁}\AgdaSpace{}%
\AgdaBound{pbk1}\AgdaSpace{}%
\AgdaBound{pbk2}\AgdaSpace{}%
\AgdaBound{pbk3}\AgdaSpace{}%
\AgdaBound{pbk4}\AgdaSpace{}%
\AgdaBound{pbk5}\AgdaSpace{}%
\AgdaBound{sig1}\AgdaSpace{}%
\AgdaBound{sig2}\AgdaSpace{}%
\AgdaBound{sig3}\AgdaSpace{}%
\AgdaBound{x}\AgdaSpace{}%
\AgdaBound{x₁}\AgdaSpace{}%
\AgdaBound{x₂}\AgdaSpace{}%
\AgdaSymbol{|}\AgdaSpace{}%
\AgdaInductiveConstructor{false}\AgdaSpace{}%
\AgdaKeyword{with}%
\>[97]\AgdaSymbol{(}\AgdaFunction{isSigned}%
\>[108]\AgdaBound{msg₁}\AgdaSpace{}%
\AgdaBound{sig1}\AgdaSpace{}%
\AgdaBound{pbk2}\AgdaSymbol{)}\<%
\\
\>[0]\AgdaFunction{lemmaHoareTripleStackGeAux'22}\AgdaSpace{}%
\AgdaBound{msg₁}\AgdaSpace{}%
\AgdaBound{pbk1}\AgdaSpace{}%
\AgdaBound{pbk2}\AgdaSpace{}%
\AgdaBound{pbk3}\AgdaSpace{}%
\AgdaBound{pbk4}\AgdaSpace{}%
\AgdaBound{pbk5}\AgdaSpace{}%
\AgdaBound{sig1}\AgdaSpace{}%
\AgdaBound{sig2}\AgdaSpace{}%
\AgdaBound{sig3}\AgdaSpace{}%
\AgdaBound{x}\AgdaSpace{}%
\AgdaBound{x₁}\AgdaSpace{}%
\AgdaBound{x₂}\AgdaSpace{}%
\AgdaSymbol{|}\AgdaSpace{}%
\AgdaInductiveConstructor{false}\AgdaSpace{}%
\AgdaSymbol{|}\AgdaSpace{}%
\AgdaInductiveConstructor{true}\AgdaSpace{}%
\AgdaKeyword{with}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaFunction{isSigned}%
\>[114]\AgdaBound{msg₁}\AgdaSpace{}%
\AgdaBound{sig2}\AgdaSpace{}%
\AgdaBound{pbk3}\AgdaSymbol{)}\<%
\\
\>[0]\AgdaFunction{lemmaHoareTripleStackGeAux'22}\AgdaSpace{}%
\AgdaBound{msg₁}\AgdaSpace{}%
\AgdaBound{pbk1}\AgdaSpace{}%
\AgdaBound{pbk2}\AgdaSpace{}%
\AgdaBound{pbk3}\AgdaSpace{}%
\AgdaBound{pbk4}\AgdaSpace{}%
\AgdaBound{pbk5}\AgdaSpace{}%
\AgdaBound{sig1}\AgdaSpace{}%
\AgdaBound{sig2}\AgdaSpace{}%
\AgdaBound{sig3}\AgdaSpace{}%
\AgdaBound{x}\AgdaSpace{}%
\AgdaBound{x₁}\AgdaSpace{}%
\AgdaBound{x₂}\AgdaSpace{}%
\AgdaSymbol{|}\AgdaSpace{}%
\AgdaInductiveConstructor{false}\AgdaSpace{}%
\AgdaSymbol{|}\AgdaSpace{}%
\AgdaInductiveConstructor{true}\AgdaSpace{}%
\AgdaSymbol{|}\AgdaSpace{}%
\AgdaInductiveConstructor{false}\AgdaSpace{}%
\AgdaKeyword{with}%
\>[112]\AgdaSymbol{(}\AgdaFunction{isSigned}%
\>[123]\AgdaBound{msg₁}\AgdaSpace{}%
\AgdaBound{sig2}\AgdaSpace{}%
\AgdaBound{pbk4}\AgdaSymbol{)}\<%
\\
\>[0]\AgdaFunction{lemmaHoareTripleStackGeAux'22}\AgdaSpace{}%
\AgdaBound{msg₁}\AgdaSpace{}%
\AgdaBound{pbk1}\AgdaSpace{}%
\AgdaBound{pbk2}\AgdaSpace{}%
\AgdaBound{pbk3}\AgdaSpace{}%
\AgdaBound{pbk4}\AgdaSpace{}%
\AgdaBound{pbk5}\AgdaSpace{}%
\AgdaBound{sig1}\AgdaSpace{}%
\AgdaBound{sig2}\AgdaSpace{}%
\AgdaBound{sig3}\AgdaSpace{}%
\AgdaBound{x}\AgdaSpace{}%
\AgdaBound{x₁}\AgdaSpace{}%
\AgdaBound{x₂}\AgdaSpace{}%
\AgdaSymbol{|}\AgdaSpace{}%
\AgdaInductiveConstructor{false}\AgdaSpace{}%
\AgdaSymbol{|}\AgdaSpace{}%
\AgdaInductiveConstructor{true}\AgdaSpace{}%
\AgdaSymbol{|}\AgdaSpace{}%
\AgdaInductiveConstructor{false}\AgdaSpace{}%
\AgdaSymbol{|}\AgdaSpace{}%
\AgdaInductiveConstructor{true}\AgdaSpace{}%
\AgdaKeyword{with}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaFunction{isSigned}%
\>[129]\AgdaBound{msg₁}\AgdaSpace{}%
\AgdaBound{sig3}\AgdaSpace{}%
\AgdaBound{pbk5}\AgdaSymbol{)}\<%
\\
\>[0]\AgdaFunction{lemmaHoareTripleStackGeAux'22}\AgdaSpace{}%
\AgdaBound{msg₁}\AgdaSpace{}%
\AgdaBound{pbk1}\AgdaSpace{}%
\AgdaBound{pbk2}\AgdaSpace{}%
\AgdaBound{pbk3}\AgdaSpace{}%
\AgdaBound{pbk4}\AgdaSpace{}%
\AgdaBound{pbk5}\AgdaSpace{}%
\AgdaBound{sig1}\AgdaSpace{}%
\AgdaBound{sig2}\AgdaSpace{}%
\AgdaBound{sig3}\AgdaSpace{}%
\AgdaBound{x}\AgdaSpace{}%
\AgdaBound{x₁}\AgdaSpace{}%
\AgdaBound{x₂}\AgdaSpace{}%
\AgdaSymbol{|}\AgdaSpace{}%
\AgdaInductiveConstructor{false}\AgdaSpace{}%
\AgdaSymbol{|}\AgdaSpace{}%
\AgdaInductiveConstructor{true}\AgdaSpace{}%
\AgdaSymbol{|}\AgdaSpace{}%
\AgdaInductiveConstructor{false}\AgdaSpace{}%
\AgdaSymbol{|}\AgdaSpace{}%
\AgdaInductiveConstructor{true}\AgdaSpace{}%
\AgdaSymbol{|}\AgdaSpace{}%
\AgdaInductiveConstructor{true}\AgdaSpace{}%
\AgdaSymbol{=}\AgdaSpace{}%
\AgdaInductiveConstructor{tt}\<%
\\
\>[0]\AgdaFunction{lemmaHoareTripleStackGeAux'22}\AgdaSpace{}%
\AgdaBound{msg₁}\AgdaSpace{}%
\AgdaBound{pbk1}\AgdaSpace{}%
\AgdaBound{pbk2}\AgdaSpace{}%
\AgdaBound{pbk3}\AgdaSpace{}%
\AgdaBound{pbk4}\AgdaSpace{}%
\AgdaBound{pbk5}\AgdaSpace{}%
\AgdaBound{sig1}\AgdaSpace{}%
\AgdaBound{sig2}\AgdaSpace{}%
\AgdaBound{sig3}\AgdaSpace{}%
\AgdaBound{x}\AgdaSpace{}%
\AgdaBound{x₁}\AgdaSpace{}%
\AgdaBound{x₂}\AgdaSpace{}%
\AgdaSymbol{|}\AgdaSpace{}%
\AgdaInductiveConstructor{false}\AgdaSpace{}%
\AgdaSymbol{|}\AgdaSpace{}%
\AgdaInductiveConstructor{true}\AgdaSpace{}%
\AgdaSymbol{|}\AgdaSpace{}%
\AgdaInductiveConstructor{true}\AgdaSpace{}%
\AgdaKeyword{with}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaFunction{isSigned}%
\>[121]\AgdaBound{msg₁}\AgdaSpace{}%
\AgdaBound{sig3}\AgdaSpace{}%
\AgdaBound{pbk4}\AgdaSymbol{)}\<%
\\
\>[0]\AgdaFunction{lemmaHoareTripleStackGeAux'22}\AgdaSpace{}%
\AgdaBound{msg₁}\AgdaSpace{}%
\AgdaBound{pbk1}\AgdaSpace{}%
\AgdaBound{pbk2}\AgdaSpace{}%
\AgdaBound{pbk3}\AgdaSpace{}%
\AgdaBound{pbk4}\AgdaSpace{}%
\AgdaBound{pbk5}\AgdaSpace{}%
\AgdaBound{sig1}\AgdaSpace{}%
\AgdaBound{sig2}\AgdaSpace{}%
\AgdaBound{sig3}\AgdaSpace{}%
\AgdaBound{x}\AgdaSpace{}%
\AgdaBound{x₁}\AgdaSpace{}%
\AgdaBound{x₂}\AgdaSpace{}%
\AgdaSymbol{|}\AgdaSpace{}%
\AgdaInductiveConstructor{false}\AgdaSpace{}%
\AgdaSymbol{|}\AgdaSpace{}%
\AgdaInductiveConstructor{true}\AgdaSpace{}%
\AgdaSymbol{|}\AgdaSpace{}%
\AgdaInductiveConstructor{true}\AgdaSpace{}%
\AgdaSymbol{|}\AgdaSpace{}%
\AgdaInductiveConstructor{false}\AgdaSpace{}%
\AgdaKeyword{with}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaFunction{isSigned}%
\>[129]\AgdaBound{msg₁}\AgdaSpace{}%
\AgdaBound{sig3}\AgdaSpace{}%
\AgdaBound{pbk5}\AgdaSymbol{)}\<%
\\
\>[0]\AgdaFunction{lemmaHoareTripleStackGeAux'22}\AgdaSpace{}%
\AgdaBound{msg₁}\AgdaSpace{}%
\AgdaBound{pbk1}\AgdaSpace{}%
\AgdaBound{pbk2}\AgdaSpace{}%
\AgdaBound{pbk3}\AgdaSpace{}%
\AgdaBound{pbk4}\AgdaSpace{}%
\AgdaBound{pbk5}\AgdaSpace{}%
\AgdaBound{sig1}\AgdaSpace{}%
\AgdaBound{sig2}\AgdaSpace{}%
\AgdaBound{sig3}\AgdaSpace{}%
\AgdaBound{x}\AgdaSpace{}%
\AgdaBound{x₁}\AgdaSpace{}%
\AgdaBound{x₂}\AgdaSpace{}%
\AgdaSymbol{|}\AgdaSpace{}%
\AgdaInductiveConstructor{false}\AgdaSpace{}%
\AgdaSymbol{|}\AgdaSpace{}%
\AgdaInductiveConstructor{true}\AgdaSpace{}%
\AgdaSymbol{|}\AgdaSpace{}%
\AgdaInductiveConstructor{true}\AgdaSpace{}%
\AgdaSymbol{|}\AgdaSpace{}%
\AgdaInductiveConstructor{false}\AgdaSpace{}%
\AgdaSymbol{|}\AgdaSpace{}%
\AgdaInductiveConstructor{true}\AgdaSpace{}%
\AgdaSymbol{=}\AgdaSpace{}%
\AgdaInductiveConstructor{tt}\<%
\\
\>[0]\AgdaFunction{lemmaHoareTripleStackGeAux'22}\AgdaSpace{}%
\AgdaBound{msg₁}\AgdaSpace{}%
\AgdaBound{pbk1}\AgdaSpace{}%
\AgdaBound{pbk2}\AgdaSpace{}%
\AgdaBound{pbk3}\AgdaSpace{}%
\AgdaBound{pbk4}\AgdaSpace{}%
\AgdaBound{pbk5}\AgdaSpace{}%
\AgdaBound{sig1}\AgdaSpace{}%
\AgdaBound{sig2}\AgdaSpace{}%
\AgdaBound{sig3}\AgdaSpace{}%
\AgdaBound{x}\AgdaSpace{}%
\AgdaBound{x₁}\AgdaSpace{}%
\AgdaBound{x₂}\AgdaSpace{}%
\AgdaSymbol{|}\AgdaSpace{}%
\AgdaInductiveConstructor{false}\AgdaSpace{}%
\AgdaSymbol{|}\AgdaSpace{}%
\AgdaInductiveConstructor{true}\AgdaSpace{}%
\AgdaSymbol{|}\AgdaSpace{}%
\AgdaInductiveConstructor{true}\AgdaSpace{}%
\AgdaSymbol{|}\AgdaSpace{}%
\AgdaInductiveConstructor{true}\AgdaSpace{}%
\AgdaSymbol{=}\AgdaSpace{}%
\AgdaInductiveConstructor{tt}\<%
\\
\>[0]\AgdaFunction{lemmaHoareTripleStackGeAux'22}\AgdaSpace{}%
\AgdaBound{msg₁}\AgdaSpace{}%
\AgdaBound{pbk1}\AgdaSpace{}%
\AgdaBound{pbk2}\AgdaSpace{}%
\AgdaBound{pbk3}\AgdaSpace{}%
\AgdaBound{pbk4}\AgdaSpace{}%
\AgdaBound{pbk5}\AgdaSpace{}%
\AgdaBound{sig1}\AgdaSpace{}%
\AgdaBound{sig2}\AgdaSpace{}%
\AgdaBound{sig3}\AgdaSpace{}%
\AgdaBound{x}\AgdaSpace{}%
\AgdaBound{x₁}\AgdaSpace{}%
\AgdaBound{x₂}\AgdaSpace{}%
\AgdaSymbol{|}\AgdaSpace{}%
\AgdaInductiveConstructor{true}\AgdaSpace{}%
\AgdaKeyword{with}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaFunction{isSigned}%
\>[106]\AgdaBound{msg₁}\AgdaSpace{}%
\AgdaBound{sig2}\AgdaSpace{}%
\AgdaBound{pbk2}\AgdaSymbol{)}\<%
\\
\>[0]\AgdaFunction{lemmaHoareTripleStackGeAux'22}\AgdaSpace{}%
\AgdaBound{msg₁}\AgdaSpace{}%
\AgdaBound{pbk1}\AgdaSpace{}%
\AgdaBound{pbk2}\AgdaSpace{}%
\AgdaBound{pbk3}\AgdaSpace{}%
\AgdaBound{pbk4}\AgdaSpace{}%
\AgdaBound{pbk5}\AgdaSpace{}%
\AgdaBound{sig1}\AgdaSpace{}%
\AgdaBound{sig2}\AgdaSpace{}%
\AgdaBound{sig3}\AgdaSpace{}%
\AgdaBound{x}\AgdaSpace{}%
\AgdaBound{x₁}\AgdaSpace{}%
\AgdaBound{x₂}\AgdaSpace{}%
\AgdaSymbol{|}\AgdaSpace{}%
\AgdaInductiveConstructor{true}\AgdaSpace{}%
\AgdaSymbol{|}\AgdaSpace{}%
\AgdaInductiveConstructor{false}\AgdaSpace{}%
\AgdaKeyword{with}%
\>[104]\AgdaSymbol{(}\AgdaFunction{isSigned}%
\>[115]\AgdaBound{msg₁}\AgdaSpace{}%
\AgdaBound{sig2}\AgdaSpace{}%
\AgdaBound{pbk3}\AgdaSymbol{)}\<%
\\
\>[0]\AgdaFunction{lemmaHoareTripleStackGeAux'22}\AgdaSpace{}%
\AgdaBound{msg₁}\AgdaSpace{}%
\AgdaBound{pbk1}\AgdaSpace{}%
\AgdaBound{pbk2}\AgdaSpace{}%
\AgdaBound{pbk3}\AgdaSpace{}%
\AgdaBound{pbk4}\AgdaSpace{}%
\AgdaBound{pbk5}\AgdaSpace{}%
\AgdaBound{sig1}\AgdaSpace{}%
\AgdaBound{sig2}\AgdaSpace{}%
\AgdaBound{sig3}\AgdaSpace{}%
\AgdaBound{x}\AgdaSpace{}%
\AgdaBound{x₁}\AgdaSpace{}%
\AgdaBound{x₂}\AgdaSpace{}%
\AgdaSymbol{|}\AgdaSpace{}%
\AgdaInductiveConstructor{true}\AgdaSpace{}%
\AgdaSymbol{|}\AgdaSpace{}%
\AgdaInductiveConstructor{false}\AgdaSpace{}%
\AgdaSymbol{|}\AgdaSpace{}%
\AgdaInductiveConstructor{false}\AgdaSpace{}%
\AgdaKeyword{with}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaFunction{isSigned}%
\>[122]\AgdaBound{msg₁}\AgdaSpace{}%
\AgdaBound{sig2}\AgdaSpace{}%
\AgdaBound{pbk4}\AgdaSymbol{)}\<%
\\
\>[0]\AgdaFunction{lemmaHoareTripleStackGeAux'22}\AgdaSpace{}%
\AgdaBound{msg₁}\AgdaSpace{}%
\AgdaBound{pbk1}\AgdaSpace{}%
\AgdaBound{pbk2}\AgdaSpace{}%
\AgdaBound{pbk3}\AgdaSpace{}%
\AgdaBound{pbk4}\AgdaSpace{}%
\AgdaBound{pbk5}\AgdaSpace{}%
\AgdaBound{sig1}\AgdaSpace{}%
\AgdaBound{sig2}\AgdaSpace{}%
\AgdaBound{sig3}\AgdaSpace{}%
\AgdaBound{x}\AgdaSpace{}%
\AgdaBound{x₁}\AgdaSpace{}%
\AgdaBound{x₂}\AgdaSpace{}%
\AgdaSymbol{|}\AgdaSpace{}%
\AgdaInductiveConstructor{true}\AgdaSpace{}%
\AgdaSymbol{|}\AgdaSpace{}%
\AgdaInductiveConstructor{false}\AgdaSpace{}%
\AgdaSymbol{|}\AgdaSpace{}%
\AgdaInductiveConstructor{false}\AgdaSpace{}%
\AgdaSymbol{|}\AgdaSpace{}%
\AgdaInductiveConstructor{true}\AgdaSpace{}%
\AgdaKeyword{with}%
\>[119]\AgdaSymbol{(}\AgdaFunction{isSigned}%
\>[130]\AgdaBound{msg₁}\AgdaSpace{}%
\AgdaBound{sig3}\AgdaSpace{}%
\AgdaBound{pbk5}\AgdaSymbol{)}\<%
\\
\>[0]\AgdaFunction{lemmaHoareTripleStackGeAux'22}\AgdaSpace{}%
\AgdaBound{msg₁}\AgdaSpace{}%
\AgdaBound{pbk1}\AgdaSpace{}%
\AgdaBound{pbk2}\AgdaSpace{}%
\AgdaBound{pbk3}\AgdaSpace{}%
\AgdaBound{pbk4}\AgdaSpace{}%
\AgdaBound{pbk5}\AgdaSpace{}%
\AgdaBound{sig1}\AgdaSpace{}%
\AgdaBound{sig2}\AgdaSpace{}%
\AgdaBound{sig3}\AgdaSpace{}%
\AgdaBound{x}\AgdaSpace{}%
\AgdaBound{x₁}\AgdaSpace{}%
\AgdaBound{x₂}\AgdaSpace{}%
\AgdaSymbol{|}\AgdaSpace{}%
\AgdaInductiveConstructor{true}\AgdaSpace{}%
\AgdaSymbol{|}\AgdaSpace{}%
\AgdaInductiveConstructor{false}\AgdaSpace{}%
\AgdaSymbol{|}\AgdaSpace{}%
\AgdaInductiveConstructor{false}\AgdaSpace{}%
\AgdaSymbol{|}\AgdaSpace{}%
\AgdaInductiveConstructor{true}\AgdaSpace{}%
\AgdaSymbol{|}\AgdaSpace{}%
\AgdaInductiveConstructor{true}\AgdaSpace{}%
\AgdaSymbol{=}\AgdaSpace{}%
\AgdaInductiveConstructor{tt}\<%
\\
\>[0]\AgdaFunction{lemmaHoareTripleStackGeAux'22}\AgdaSpace{}%
\AgdaBound{msg₁}\AgdaSpace{}%
\AgdaBound{pbk1}\AgdaSpace{}%
\AgdaBound{pbk2}\AgdaSpace{}%
\AgdaBound{pbk3}\AgdaSpace{}%
\AgdaBound{pbk4}\AgdaSpace{}%
\AgdaBound{pbk5}\AgdaSpace{}%
\AgdaBound{sig1}\AgdaSpace{}%
\AgdaBound{sig2}\AgdaSpace{}%
\AgdaBound{sig3}\AgdaSpace{}%
\AgdaBound{x}\AgdaSpace{}%
\AgdaBound{x₁}\AgdaSpace{}%
\AgdaBound{x₂}\AgdaSpace{}%
\AgdaSymbol{|}\AgdaSpace{}%
\AgdaInductiveConstructor{true}\AgdaSpace{}%
\AgdaSymbol{|}\AgdaSpace{}%
\AgdaInductiveConstructor{false}\AgdaSpace{}%
\AgdaSymbol{|}\AgdaSpace{}%
\AgdaInductiveConstructor{true}\AgdaSpace{}%
\AgdaKeyword{with}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaFunction{isSigned}%
\>[121]\AgdaBound{msg₁}\AgdaSpace{}%
\AgdaBound{sig3}\AgdaSpace{}%
\AgdaBound{pbk4}\AgdaSymbol{)}\<%
\\
\>[0]\AgdaFunction{lemmaHoareTripleStackGeAux'22}\AgdaSpace{}%
\AgdaBound{msg₁}\AgdaSpace{}%
\AgdaBound{pbk1}\AgdaSpace{}%
\AgdaBound{pbk2}\AgdaSpace{}%
\AgdaBound{pbk3}\AgdaSpace{}%
\AgdaBound{pbk4}\AgdaSpace{}%
\AgdaBound{pbk5}\AgdaSpace{}%
\AgdaBound{sig1}\AgdaSpace{}%
\AgdaBound{sig2}\AgdaSpace{}%
\AgdaBound{sig3}\AgdaSpace{}%
\AgdaBound{x}\AgdaSpace{}%
\AgdaBound{x₁}\AgdaSpace{}%
\AgdaBound{x₂}\AgdaSpace{}%
\AgdaSymbol{|}\AgdaSpace{}%
\AgdaInductiveConstructor{true}\AgdaSpace{}%
\AgdaSymbol{|}\AgdaSpace{}%
\AgdaInductiveConstructor{false}\AgdaSpace{}%
\AgdaSymbol{|}\AgdaSpace{}%
\AgdaInductiveConstructor{true}\AgdaSpace{}%
\AgdaSymbol{|}\AgdaSpace{}%
\AgdaInductiveConstructor{false}\AgdaSpace{}%
\AgdaKeyword{with}%
\>[119]\AgdaSymbol{(}\AgdaFunction{isSigned}%
\>[130]\AgdaBound{msg₁}\AgdaSpace{}%
\AgdaBound{sig3}\AgdaSpace{}%
\AgdaBound{pbk5}\AgdaSymbol{)}\<%
\\
\>[0]\AgdaFunction{lemmaHoareTripleStackGeAux'22}\AgdaSpace{}%
\AgdaBound{msg₁}\AgdaSpace{}%
\AgdaBound{pbk1}\AgdaSpace{}%
\AgdaBound{pbk2}\AgdaSpace{}%
\AgdaBound{pbk3}\AgdaSpace{}%
\AgdaBound{pbk4}\AgdaSpace{}%
\AgdaBound{pbk5}\AgdaSpace{}%
\AgdaBound{sig1}\AgdaSpace{}%
\AgdaBound{sig2}\AgdaSpace{}%
\AgdaBound{sig3}\AgdaSpace{}%
\AgdaBound{x}\AgdaSpace{}%
\AgdaBound{x₁}\AgdaSpace{}%
\AgdaBound{x₂}\AgdaSpace{}%
\AgdaSymbol{|}\AgdaSpace{}%
\AgdaInductiveConstructor{true}\AgdaSpace{}%
\AgdaSymbol{|}\AgdaSpace{}%
\AgdaInductiveConstructor{false}\AgdaSpace{}%
\AgdaSymbol{|}\AgdaSpace{}%
\AgdaInductiveConstructor{true}\AgdaSpace{}%
\AgdaSymbol{|}\AgdaSpace{}%
\AgdaInductiveConstructor{false}\AgdaSpace{}%
\AgdaSymbol{|}\AgdaSpace{}%
\AgdaInductiveConstructor{true}\AgdaSpace{}%
\AgdaSymbol{=}\AgdaSpace{}%
\AgdaInductiveConstructor{tt}\<%
\\
\>[0]\AgdaFunction{lemmaHoareTripleStackGeAux'22}\AgdaSpace{}%
\AgdaBound{msg₁}\AgdaSpace{}%
\AgdaBound{pbk1}\AgdaSpace{}%
\AgdaBound{pbk2}\AgdaSpace{}%
\AgdaBound{pbk3}\AgdaSpace{}%
\AgdaBound{pbk4}\AgdaSpace{}%
\AgdaBound{pbk5}\AgdaSpace{}%
\AgdaBound{sig1}\AgdaSpace{}%
\AgdaBound{sig2}\AgdaSpace{}%
\AgdaBound{sig3}\AgdaSpace{}%
\AgdaBound{x}\AgdaSpace{}%
\AgdaBound{x₁}\AgdaSpace{}%
\AgdaBound{x₂}\AgdaSpace{}%
\AgdaSymbol{|}\AgdaSpace{}%
\AgdaInductiveConstructor{true}\AgdaSpace{}%
\AgdaSymbol{|}\AgdaSpace{}%
\AgdaInductiveConstructor{false}\AgdaSpace{}%
\AgdaSymbol{|}\AgdaSpace{}%
\AgdaInductiveConstructor{true}\AgdaSpace{}%
\AgdaSymbol{|}\AgdaSpace{}%
\AgdaInductiveConstructor{true}\AgdaSpace{}%
\AgdaSymbol{=}\AgdaSpace{}%
\AgdaInductiveConstructor{tt}\<%
\\
\>[0]\AgdaFunction{lemmaHoareTripleStackGeAux'22}\AgdaSpace{}%
\AgdaBound{msg₁}\AgdaSpace{}%
\AgdaBound{pbk1}\AgdaSpace{}%
\AgdaBound{pbk2}\AgdaSpace{}%
\AgdaBound{pbk3}\AgdaSpace{}%
\AgdaBound{pbk4}\AgdaSpace{}%
\AgdaBound{pbk5}\AgdaSpace{}%
\AgdaBound{sig1}\AgdaSpace{}%
\AgdaBound{sig2}\AgdaSpace{}%
\AgdaBound{sig3}\AgdaSpace{}%
\AgdaBound{x}\AgdaSpace{}%
\AgdaBound{x₁}\AgdaSpace{}%
\AgdaBound{x₂}\AgdaSpace{}%
\AgdaSymbol{|}\AgdaSpace{}%
\AgdaInductiveConstructor{true}\AgdaSpace{}%
\AgdaSymbol{|}\AgdaSpace{}%
\AgdaInductiveConstructor{true}\AgdaSpace{}%
\AgdaKeyword{with}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaFunction{isSigned}%
\>[113]\AgdaBound{msg₁}\AgdaSpace{}%
\AgdaBound{sig3}\AgdaSpace{}%
\AgdaBound{pbk3}\AgdaSymbol{)}\<%
\\
\>[0]\AgdaFunction{lemmaHoareTripleStackGeAux'22}\AgdaSpace{}%
\AgdaBound{msg₁}\AgdaSpace{}%
\AgdaBound{pbk1}\AgdaSpace{}%
\AgdaBound{pbk2}\AgdaSpace{}%
\AgdaBound{pbk3}\AgdaSpace{}%
\AgdaBound{pbk4}\AgdaSpace{}%
\AgdaBound{pbk5}\AgdaSpace{}%
\AgdaBound{sig1}\AgdaSpace{}%
\AgdaBound{sig2}\AgdaSpace{}%
\AgdaBound{sig3}\AgdaSpace{}%
\AgdaBound{x}\AgdaSpace{}%
\AgdaBound{x₁}\AgdaSpace{}%
\AgdaBound{x₂}\AgdaSpace{}%
\AgdaSymbol{|}\AgdaSpace{}%
\AgdaInductiveConstructor{true}\AgdaSpace{}%
\AgdaSymbol{|}\AgdaSpace{}%
\AgdaInductiveConstructor{true}\AgdaSpace{}%
\AgdaSymbol{|}\AgdaSpace{}%
\AgdaInductiveConstructor{false}\AgdaSpace{}%
\AgdaKeyword{with}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaFunction{isSigned}%
\>[121]\AgdaBound{msg₁}\AgdaSpace{}%
\AgdaBound{sig3}\AgdaSpace{}%
\AgdaBound{pbk4}\AgdaSymbol{)}\<%
\\
\>[0]\AgdaFunction{lemmaHoareTripleStackGeAux'22}\AgdaSpace{}%
\AgdaBound{msg₁}\AgdaSpace{}%
\AgdaBound{pbk1}\AgdaSpace{}%
\AgdaBound{pbk2}\AgdaSpace{}%
\AgdaBound{pbk3}\AgdaSpace{}%
\AgdaBound{pbk4}\AgdaSpace{}%
\AgdaBound{pbk5}\AgdaSpace{}%
\AgdaBound{sig1}\AgdaSpace{}%
\AgdaBound{sig2}\AgdaSpace{}%
\AgdaBound{sig3}\AgdaSpace{}%
\AgdaBound{x}\AgdaSpace{}%
\AgdaBound{x₁}\AgdaSpace{}%
\AgdaBound{x₂}\AgdaSpace{}%
\AgdaSymbol{|}\AgdaSpace{}%
\AgdaInductiveConstructor{true}\AgdaSpace{}%
\AgdaSymbol{|}\AgdaSpace{}%
\AgdaInductiveConstructor{true}\AgdaSpace{}%
\AgdaSymbol{|}\AgdaSpace{}%
\AgdaInductiveConstructor{false}\AgdaSpace{}%
\AgdaSymbol{|}\AgdaSpace{}%
\AgdaInductiveConstructor{false}\AgdaSpace{}%
\AgdaKeyword{with}%
\>[119]\AgdaSymbol{(}\AgdaFunction{isSigned}%
\>[130]\AgdaBound{msg₁}\AgdaSpace{}%
\AgdaBound{sig3}\AgdaSpace{}%
\AgdaBound{pbk5}\AgdaSymbol{)}\<%
\\
\>[0]\AgdaFunction{lemmaHoareTripleStackGeAux'22}\AgdaSpace{}%
\AgdaBound{msg₁}\AgdaSpace{}%
\AgdaBound{pbk1}\AgdaSpace{}%
\AgdaBound{pbk2}\AgdaSpace{}%
\AgdaBound{pbk3}\AgdaSpace{}%
\AgdaBound{pbk4}\AgdaSpace{}%
\AgdaBound{pbk5}\AgdaSpace{}%
\AgdaBound{sig1}\AgdaSpace{}%
\AgdaBound{sig2}\AgdaSpace{}%
\AgdaBound{sig3}\AgdaSpace{}%
\AgdaBound{x}\AgdaSpace{}%
\AgdaBound{x₁}\AgdaSpace{}%
\AgdaBound{x₂}\AgdaSpace{}%
\AgdaSymbol{|}\AgdaSpace{}%
\AgdaInductiveConstructor{true}\AgdaSpace{}%
\AgdaSymbol{|}\AgdaSpace{}%
\AgdaInductiveConstructor{true}\AgdaSpace{}%
\AgdaSymbol{|}\AgdaSpace{}%
\AgdaInductiveConstructor{false}\AgdaSpace{}%
\AgdaSymbol{|}\AgdaSpace{}%
\AgdaInductiveConstructor{false}\AgdaSpace{}%
\AgdaSymbol{|}\AgdaSpace{}%
\AgdaInductiveConstructor{true}\AgdaSpace{}%
\AgdaSymbol{=}\AgdaSpace{}%
\AgdaInductiveConstructor{tt}\<%
\\
\>[0]\AgdaFunction{lemmaHoareTripleStackGeAux'22}\AgdaSpace{}%
\AgdaBound{msg₁}\AgdaSpace{}%
\AgdaBound{pbk1}\AgdaSpace{}%
\AgdaBound{pbk2}\AgdaSpace{}%
\AgdaBound{pbk3}\AgdaSpace{}%
\AgdaBound{pbk4}\AgdaSpace{}%
\AgdaBound{pbk5}\AgdaSpace{}%
\AgdaBound{sig1}\AgdaSpace{}%
\AgdaBound{sig2}\AgdaSpace{}%
\AgdaBound{sig3}\AgdaSpace{}%
\AgdaBound{x}\AgdaSpace{}%
\AgdaBound{x₁}\AgdaSpace{}%
\AgdaBound{x₂}\AgdaSpace{}%
\AgdaSymbol{|}\AgdaSpace{}%
\AgdaInductiveConstructor{true}\AgdaSpace{}%
\AgdaSymbol{|}\AgdaSpace{}%
\AgdaInductiveConstructor{true}\AgdaSpace{}%
\AgdaSymbol{|}\AgdaSpace{}%
\AgdaInductiveConstructor{false}\AgdaSpace{}%
\AgdaSymbol{|}\AgdaSpace{}%
\AgdaInductiveConstructor{true}\AgdaSpace{}%
\AgdaSymbol{=}\AgdaSpace{}%
\AgdaInductiveConstructor{tt}\<%
\\
\>[0]\AgdaFunction{lemmaHoareTripleStackGeAux'22}\AgdaSpace{}%
\AgdaBound{msg₁}\AgdaSpace{}%
\AgdaBound{pbk1}\AgdaSpace{}%
\AgdaBound{pbk2}\AgdaSpace{}%
\AgdaBound{pbk3}\AgdaSpace{}%
\AgdaBound{pbk4}\AgdaSpace{}%
\AgdaBound{pbk5}\AgdaSpace{}%
\AgdaBound{sig1}\AgdaSpace{}%
\AgdaBound{sig2}\AgdaSpace{}%
\AgdaBound{sig3}\AgdaSpace{}%
\AgdaBound{x}\AgdaSpace{}%
\AgdaBound{x₁}\AgdaSpace{}%
\AgdaBound{x₂}\AgdaSpace{}%
\AgdaSymbol{|}\AgdaSpace{}%
\AgdaInductiveConstructor{true}\AgdaSpace{}%
\AgdaSymbol{|}\AgdaSpace{}%
\AgdaInductiveConstructor{true}\AgdaSpace{}%
\AgdaSymbol{|}\AgdaSpace{}%
\AgdaInductiveConstructor{true}\AgdaSpace{}%
\AgdaSymbol{=}\AgdaSpace{}%
\AgdaInductiveConstructor{tt}\<%
\\
%
\\[\AgdaEmptyExtraSkip]%
%
\\[\AgdaEmptyExtraSkip]%
%
\\[\AgdaEmptyExtraSkip]%
\>[0]\AgdaFunction{lemmaHoareTripleStackGeAux'23}%
\>[5804I]\AgdaSymbol{:}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaBound{msg}\AgdaSpace{}%
\AgdaSymbol{:}\AgdaSpace{}%
\AgdaDatatype{Msg}\AgdaSymbol{)}\<%
\\
\>[5804I][@{}l@{\AgdaIndent{0}}]%
\>[31]\AgdaSymbol{(}\AgdaBound{pbk1}\AgdaSpace{}%
\AgdaBound{pbk2}\AgdaSpace{}%
\AgdaBound{pbk3}\AgdaSpace{}%
\AgdaBound{pbk4}\AgdaSpace{}%
\AgdaBound{pbk5}\AgdaSpace{}%
\AgdaBound{sig1}\AgdaSpace{}%
\AgdaBound{sig2}\AgdaSpace{}%
\AgdaBound{sig3}\AgdaSpace{}%
\AgdaSymbol{:}\AgdaSpace{}%
\AgdaDatatype{ℕ}\AgdaSymbol{)}\<%
\\
%
\>[31]\AgdaSymbol{→}\AgdaSpace{}%
\AgdaFunction{True}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaFunction{isSigned}%
\>[49]\AgdaBound{msg}\AgdaSpace{}%
\AgdaBound{sig3}\AgdaSpace{}%
\AgdaBound{pbk5}\AgdaSymbol{)}\<%
\\
\>[.][@{}l@{}]\<[5804I]%
\>[30]\AgdaSymbol{→}%
\>[33]\AgdaFunction{True}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaFunction{isSigned}%
\>[49]\AgdaBound{msg}\AgdaSpace{}%
\AgdaBound{sig2}\AgdaSpace{}%
\AgdaBound{pbk4}\AgdaSymbol{)}\<%
\\
%
\>[30]\AgdaSymbol{→}%
\>[33]\AgdaFunction{True}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaFunction{isSigned}%
\>[49]\AgdaBound{msg}\AgdaSpace{}%
\AgdaBound{sig1}\AgdaSpace{}%
\AgdaBound{pbk3}\AgdaSymbol{)}\<%
\\
\>[30][@{}l@{\AgdaIndent{0}}]%
\>[31]\AgdaSymbol{→}\AgdaSpace{}%
\AgdaFunction{True}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaFunction{compareSigsMultiSig}\AgdaSpace{}%
\AgdaBound{msg}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaSpace{}%
\AgdaBound{sig1}\AgdaSpace{}%
\AgdaOperator{\AgdaInductiveConstructor{∷}}\AgdaSpace{}%
\AgdaBound{sig2}\AgdaSpace{}%
\AgdaOperator{\AgdaInductiveConstructor{∷}}\AgdaSpace{}%
\AgdaBound{sig3}\AgdaSpace{}%
\AgdaOperator{\AgdaInductiveConstructor{∷}}\AgdaSpace{}%
\AgdaInductiveConstructor{[]}\AgdaSymbol{)}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaBound{pbk1}\AgdaSpace{}%
\AgdaOperator{\AgdaInductiveConstructor{∷}}\AgdaSpace{}%
\AgdaBound{pbk2}\AgdaSpace{}%
\AgdaOperator{\AgdaInductiveConstructor{∷}}\AgdaSpace{}%
\AgdaBound{pbk3}\AgdaSpace{}%
\AgdaOperator{\AgdaInductiveConstructor{∷}}\AgdaSpace{}%
\AgdaBound{pbk4}\AgdaSpace{}%
\AgdaOperator{\AgdaInductiveConstructor{∷}}\AgdaSpace{}%
\AgdaBound{pbk5}\AgdaSpace{}%
\AgdaOperator{\AgdaInductiveConstructor{∷}}\AgdaSpace{}%
\AgdaInductiveConstructor{[]}\AgdaSymbol{))}\<%
\\
\>[0]\AgdaFunction{lemmaHoareTripleStackGeAux'23}\AgdaSpace{}%
\AgdaBound{msg₁}\AgdaSpace{}%
\AgdaBound{pbk1}\AgdaSpace{}%
\AgdaBound{pbk2}\AgdaSpace{}%
\AgdaBound{pbk3}\AgdaSpace{}%
\AgdaBound{pbk4}\AgdaSpace{}%
\AgdaBound{pbk5}\AgdaSpace{}%
\AgdaBound{sig1}\AgdaSpace{}%
\AgdaBound{sig2}\AgdaSpace{}%
\AgdaBound{sig3}\AgdaSpace{}%
\AgdaBound{x}\AgdaSpace{}%
\AgdaBound{x₁}\AgdaSpace{}%
\AgdaBound{x₂}\AgdaSpace{}%
\AgdaKeyword{with}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaFunction{isSigned}%
\>[99]\AgdaBound{msg₁}\AgdaSpace{}%
\AgdaBound{sig1}\AgdaSpace{}%
\AgdaBound{pbk1}\AgdaSymbol{)}\<%
\\
\>[0]\AgdaFunction{lemmaHoareTripleStackGeAux'23}\AgdaSpace{}%
\AgdaBound{msg₁}\AgdaSpace{}%
\AgdaBound{pbk1}\AgdaSpace{}%
\AgdaBound{pbk2}\AgdaSpace{}%
\AgdaBound{pbk3}\AgdaSpace{}%
\AgdaBound{pbk4}\AgdaSpace{}%
\AgdaBound{pbk5}\AgdaSpace{}%
\AgdaBound{sig1}\AgdaSpace{}%
\AgdaBound{sig2}\AgdaSpace{}%
\AgdaBound{sig3}\AgdaSpace{}%
\AgdaBound{x}\AgdaSpace{}%
\AgdaBound{x₁}\AgdaSpace{}%
\AgdaBound{x₂}\AgdaSpace{}%
\AgdaSymbol{|}\AgdaSpace{}%
\AgdaInductiveConstructor{false}\AgdaSpace{}%
\AgdaKeyword{with}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaFunction{isSigned}%
\>[107]\AgdaBound{msg₁}\AgdaSpace{}%
\AgdaBound{sig1}\AgdaSpace{}%
\AgdaBound{pbk2}\AgdaSymbol{)}\<%
\\
\>[0]\AgdaFunction{lemmaHoareTripleStackGeAux'23}\AgdaSpace{}%
\AgdaBound{msg₁}\AgdaSpace{}%
\AgdaBound{pbk1}\AgdaSpace{}%
\AgdaBound{pbk2}\AgdaSpace{}%
\AgdaBound{pbk3}\AgdaSpace{}%
\AgdaBound{pbk4}\AgdaSpace{}%
\AgdaBound{pbk5}\AgdaSpace{}%
\AgdaBound{sig1}\AgdaSpace{}%
\AgdaBound{sig2}\AgdaSpace{}%
\AgdaBound{sig3}\AgdaSpace{}%
\AgdaBound{x}\AgdaSpace{}%
\AgdaBound{x₁}\AgdaSpace{}%
\AgdaBound{x₂}\AgdaSpace{}%
\AgdaSymbol{|}\AgdaSpace{}%
\AgdaInductiveConstructor{false}\AgdaSpace{}%
\AgdaSymbol{|}\AgdaSpace{}%
\AgdaInductiveConstructor{false}\AgdaSpace{}%
\AgdaKeyword{with}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaFunction{isSigned}%
\>[115]\AgdaBound{msg₁}\AgdaSpace{}%
\AgdaBound{sig1}\AgdaSpace{}%
\AgdaBound{pbk3}\AgdaSymbol{)}\<%
\\
\>[0]\AgdaFunction{lemmaHoareTripleStackGeAux'23}\AgdaSpace{}%
\AgdaBound{msg₁}\AgdaSpace{}%
\AgdaBound{pbk1}\AgdaSpace{}%
\AgdaBound{pbk2}\AgdaSpace{}%
\AgdaBound{pbk3}\AgdaSpace{}%
\AgdaBound{pbk4}\AgdaSpace{}%
\AgdaBound{pbk5}\AgdaSpace{}%
\AgdaBound{sig1}\AgdaSpace{}%
\AgdaBound{sig2}\AgdaSpace{}%
\AgdaBound{sig3}\AgdaSpace{}%
\AgdaBound{x}\AgdaSpace{}%
\AgdaBound{x₁}\AgdaSpace{}%
\AgdaBound{x₂}\AgdaSpace{}%
\AgdaSymbol{|}\AgdaSpace{}%
\AgdaInductiveConstructor{false}\AgdaSpace{}%
\AgdaSymbol{|}\AgdaSpace{}%
\AgdaInductiveConstructor{false}\AgdaSpace{}%
\AgdaSymbol{|}\AgdaSpace{}%
\AgdaInductiveConstructor{true}\AgdaSpace{}%
\AgdaKeyword{with}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaFunction{isSigned}%
\>[122]\AgdaBound{msg₁}\AgdaSpace{}%
\AgdaBound{sig2}\AgdaSpace{}%
\AgdaBound{pbk4}\AgdaSymbol{)}\<%
\\
\>[0]\AgdaFunction{lemmaHoareTripleStackGeAux'23}\AgdaSpace{}%
\AgdaBound{msg₁}\AgdaSpace{}%
\AgdaBound{pbk1}\AgdaSpace{}%
\AgdaBound{pbk2}\AgdaSpace{}%
\AgdaBound{pbk3}\AgdaSpace{}%
\AgdaBound{pbk4}\AgdaSpace{}%
\AgdaBound{pbk5}\AgdaSpace{}%
\AgdaBound{sig1}\AgdaSpace{}%
\AgdaBound{sig2}\AgdaSpace{}%
\AgdaBound{sig3}\AgdaSpace{}%
\AgdaBound{x}\AgdaSpace{}%
\AgdaBound{x₁}\AgdaSpace{}%
\AgdaBound{x₂}\AgdaSpace{}%
\AgdaSymbol{|}\AgdaSpace{}%
\AgdaInductiveConstructor{false}\AgdaSpace{}%
\AgdaSymbol{|}\AgdaSpace{}%
\AgdaInductiveConstructor{false}\AgdaSpace{}%
\AgdaSymbol{|}\AgdaSpace{}%
\AgdaInductiveConstructor{true}\AgdaSpace{}%
\AgdaSymbol{|}\AgdaSpace{}%
\AgdaInductiveConstructor{true}\AgdaSpace{}%
\AgdaKeyword{with}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaFunction{isSigned}%
\>[129]\AgdaBound{msg₁}\AgdaSpace{}%
\AgdaBound{sig3}\AgdaSpace{}%
\AgdaBound{pbk5}\AgdaSymbol{)}\<%
\\
\>[0]\AgdaFunction{lemmaHoareTripleStackGeAux'23}\AgdaSpace{}%
\AgdaBound{msg₁}\AgdaSpace{}%
\AgdaBound{pbk1}\AgdaSpace{}%
\AgdaBound{pbk2}\AgdaSpace{}%
\AgdaBound{pbk3}\AgdaSpace{}%
\AgdaBound{pbk4}\AgdaSpace{}%
\AgdaBound{pbk5}\AgdaSpace{}%
\AgdaBound{sig1}\AgdaSpace{}%
\AgdaBound{sig2}\AgdaSpace{}%
\AgdaBound{sig3}\AgdaSpace{}%
\AgdaBound{x}\AgdaSpace{}%
\AgdaBound{x₁}\AgdaSpace{}%
\AgdaBound{x₂}\AgdaSpace{}%
\AgdaSymbol{|}\AgdaSpace{}%
\AgdaInductiveConstructor{false}\AgdaSpace{}%
\AgdaSymbol{|}\AgdaSpace{}%
\AgdaInductiveConstructor{false}\AgdaSpace{}%
\AgdaSymbol{|}\AgdaSpace{}%
\AgdaInductiveConstructor{true}\AgdaSpace{}%
\AgdaSymbol{|}\AgdaSpace{}%
\AgdaInductiveConstructor{true}\AgdaSpace{}%
\AgdaSymbol{|}\AgdaSpace{}%
\AgdaInductiveConstructor{true}\AgdaSpace{}%
\AgdaSymbol{=}\AgdaSpace{}%
\AgdaInductiveConstructor{tt}\<%
\\
\>[0]\AgdaFunction{lemmaHoareTripleStackGeAux'23}\AgdaSpace{}%
\AgdaBound{msg₁}\AgdaSpace{}%
\AgdaBound{pbk1}\AgdaSpace{}%
\AgdaBound{pbk2}\AgdaSpace{}%
\AgdaBound{pbk3}\AgdaSpace{}%
\AgdaBound{pbk4}\AgdaSpace{}%
\AgdaBound{pbk5}\AgdaSpace{}%
\AgdaBound{sig1}\AgdaSpace{}%
\AgdaBound{sig2}\AgdaSpace{}%
\AgdaBound{sig3}\AgdaSpace{}%
\AgdaBound{x}\AgdaSpace{}%
\AgdaBound{x₁}\AgdaSpace{}%
\AgdaBound{x₂}\AgdaSpace{}%
\AgdaSymbol{|}\AgdaSpace{}%
\AgdaInductiveConstructor{false}\AgdaSpace{}%
\AgdaSymbol{|}\AgdaSpace{}%
\AgdaInductiveConstructor{true}\AgdaSpace{}%
\AgdaKeyword{with}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaFunction{isSigned}%
\>[114]\AgdaBound{msg₁}\AgdaSpace{}%
\AgdaBound{sig2}\AgdaSpace{}%
\AgdaBound{pbk3}\AgdaSymbol{)}\<%
\\
\>[0]\AgdaFunction{lemmaHoareTripleStackGeAux'23}\AgdaSpace{}%
\AgdaBound{msg₁}\AgdaSpace{}%
\AgdaBound{pbk1}\AgdaSpace{}%
\AgdaBound{pbk2}\AgdaSpace{}%
\AgdaBound{pbk3}\AgdaSpace{}%
\AgdaBound{pbk4}\AgdaSpace{}%
\AgdaBound{pbk5}\AgdaSpace{}%
\AgdaBound{sig1}\AgdaSpace{}%
\AgdaBound{sig2}\AgdaSpace{}%
\AgdaBound{sig3}\AgdaSpace{}%
\AgdaBound{x}\AgdaSpace{}%
\AgdaBound{x₁}\AgdaSpace{}%
\AgdaBound{x₂}\AgdaSpace{}%
\AgdaSymbol{|}\AgdaSpace{}%
\AgdaInductiveConstructor{false}\AgdaSpace{}%
\AgdaSymbol{|}\AgdaSpace{}%
\AgdaInductiveConstructor{true}\AgdaSpace{}%
\AgdaSymbol{|}\AgdaSpace{}%
\AgdaInductiveConstructor{false}\AgdaSpace{}%
\AgdaKeyword{with}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaFunction{isSigned}%
\>[122]\AgdaBound{msg₁}\AgdaSpace{}%
\AgdaBound{sig2}\AgdaSpace{}%
\AgdaBound{pbk4}\AgdaSymbol{)}\<%
\\
\>[0]\AgdaFunction{lemmaHoareTripleStackGeAux'23}\AgdaSpace{}%
\AgdaBound{msg₁}\AgdaSpace{}%
\AgdaBound{pbk1}\AgdaSpace{}%
\AgdaBound{pbk2}\AgdaSpace{}%
\AgdaBound{pbk3}\AgdaSpace{}%
\AgdaBound{pbk4}\AgdaSpace{}%
\AgdaBound{pbk5}\AgdaSpace{}%
\AgdaBound{sig1}\AgdaSpace{}%
\AgdaBound{sig2}\AgdaSpace{}%
\AgdaBound{sig3}\AgdaSpace{}%
\AgdaBound{x}\AgdaSpace{}%
\AgdaBound{x₁}\AgdaSpace{}%
\AgdaBound{x₂}\AgdaSpace{}%
\AgdaSymbol{|}\AgdaSpace{}%
\AgdaInductiveConstructor{false}\AgdaSpace{}%
\AgdaSymbol{|}\AgdaSpace{}%
\AgdaInductiveConstructor{true}\AgdaSpace{}%
\AgdaSymbol{|}\AgdaSpace{}%
\AgdaInductiveConstructor{false}\AgdaSpace{}%
\AgdaSymbol{|}\AgdaSpace{}%
\AgdaInductiveConstructor{true}\AgdaSpace{}%
\AgdaKeyword{with}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaFunction{isSigned}%
\>[129]\AgdaBound{msg₁}\AgdaSpace{}%
\AgdaBound{sig3}\AgdaSpace{}%
\AgdaBound{pbk5}\AgdaSymbol{)}\<%
\\
\>[0]\AgdaFunction{lemmaHoareTripleStackGeAux'23}\AgdaSpace{}%
\AgdaBound{msg₁}\AgdaSpace{}%
\AgdaBound{pbk1}\AgdaSpace{}%
\AgdaBound{pbk2}\AgdaSpace{}%
\AgdaBound{pbk3}\AgdaSpace{}%
\AgdaBound{pbk4}\AgdaSpace{}%
\AgdaBound{pbk5}\AgdaSpace{}%
\AgdaBound{sig1}\AgdaSpace{}%
\AgdaBound{sig2}\AgdaSpace{}%
\AgdaBound{sig3}\AgdaSpace{}%
\AgdaBound{x}\AgdaSpace{}%
\AgdaBound{x₁}\AgdaSpace{}%
\AgdaBound{x₂}\AgdaSpace{}%
\AgdaSymbol{|}\AgdaSpace{}%
\AgdaInductiveConstructor{false}\AgdaSpace{}%
\AgdaSymbol{|}\AgdaSpace{}%
\AgdaInductiveConstructor{true}\AgdaSpace{}%
\AgdaSymbol{|}\AgdaSpace{}%
\AgdaInductiveConstructor{false}\AgdaSpace{}%
\AgdaSymbol{|}\AgdaSpace{}%
\AgdaInductiveConstructor{true}\AgdaSpace{}%
\AgdaSymbol{|}\AgdaSpace{}%
\AgdaInductiveConstructor{true}\AgdaSpace{}%
\AgdaSymbol{=}\AgdaSpace{}%
\AgdaInductiveConstructor{tt}\<%
\\
\>[0]\AgdaFunction{lemmaHoareTripleStackGeAux'23}\AgdaSpace{}%
\AgdaBound{msg₁}\AgdaSpace{}%
\AgdaBound{pbk1}\AgdaSpace{}%
\AgdaBound{pbk2}\AgdaSpace{}%
\AgdaBound{pbk3}\AgdaSpace{}%
\AgdaBound{pbk4}\AgdaSpace{}%
\AgdaBound{pbk5}\AgdaSpace{}%
\AgdaBound{sig1}\AgdaSpace{}%
\AgdaBound{sig2}\AgdaSpace{}%
\AgdaBound{sig3}\AgdaSpace{}%
\AgdaBound{x}\AgdaSpace{}%
\AgdaBound{x₁}\AgdaSpace{}%
\AgdaBound{x₂}\AgdaSpace{}%
\AgdaSymbol{|}\AgdaSpace{}%
\AgdaInductiveConstructor{false}\AgdaSpace{}%
\AgdaSymbol{|}\AgdaSpace{}%
\AgdaInductiveConstructor{true}\AgdaSpace{}%
\AgdaSymbol{|}\AgdaSpace{}%
\AgdaInductiveConstructor{true}\AgdaSpace{}%
\AgdaKeyword{with}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaFunction{isSigned}%
\>[121]\AgdaBound{msg₁}\AgdaSpace{}%
\AgdaBound{sig3}\AgdaSpace{}%
\AgdaBound{pbk4}\AgdaSymbol{)}\<%
\\
\>[0]\AgdaFunction{lemmaHoareTripleStackGeAux'23}\AgdaSpace{}%
\AgdaBound{msg₁}\AgdaSpace{}%
\AgdaBound{pbk1}\AgdaSpace{}%
\AgdaBound{pbk2}\AgdaSpace{}%
\AgdaBound{pbk3}\AgdaSpace{}%
\AgdaBound{pbk4}\AgdaSpace{}%
\AgdaBound{pbk5}\AgdaSpace{}%
\AgdaBound{sig1}\AgdaSpace{}%
\AgdaBound{sig2}\AgdaSpace{}%
\AgdaBound{sig3}\AgdaSpace{}%
\AgdaBound{x}\AgdaSpace{}%
\AgdaBound{x₁}\AgdaSpace{}%
\AgdaBound{x₂}\AgdaSpace{}%
\AgdaSymbol{|}\AgdaSpace{}%
\AgdaInductiveConstructor{false}\AgdaSpace{}%
\AgdaSymbol{|}\AgdaSpace{}%
\AgdaInductiveConstructor{true}\AgdaSpace{}%
\AgdaSymbol{|}\AgdaSpace{}%
\AgdaInductiveConstructor{true}\AgdaSpace{}%
\AgdaSymbol{|}\AgdaSpace{}%
\AgdaInductiveConstructor{false}\AgdaSpace{}%
\AgdaKeyword{with}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaFunction{isSigned}%
\>[129]\AgdaBound{msg₁}\AgdaSpace{}%
\AgdaBound{sig3}\AgdaSpace{}%
\AgdaBound{pbk5}\AgdaSymbol{)}\<%
\\
\>[0]\AgdaFunction{lemmaHoareTripleStackGeAux'23}\AgdaSpace{}%
\AgdaBound{msg₁}\AgdaSpace{}%
\AgdaBound{pbk1}\AgdaSpace{}%
\AgdaBound{pbk2}\AgdaSpace{}%
\AgdaBound{pbk3}\AgdaSpace{}%
\AgdaBound{pbk4}\AgdaSpace{}%
\AgdaBound{pbk5}\AgdaSpace{}%
\AgdaBound{sig1}\AgdaSpace{}%
\AgdaBound{sig2}\AgdaSpace{}%
\AgdaBound{sig3}\AgdaSpace{}%
\AgdaBound{x}\AgdaSpace{}%
\AgdaBound{x₁}\AgdaSpace{}%
\AgdaBound{x₂}\AgdaSpace{}%
\AgdaSymbol{|}\AgdaSpace{}%
\AgdaInductiveConstructor{false}\AgdaSpace{}%
\AgdaSymbol{|}\AgdaSpace{}%
\AgdaInductiveConstructor{true}\AgdaSpace{}%
\AgdaSymbol{|}\AgdaSpace{}%
\AgdaInductiveConstructor{true}\AgdaSpace{}%
\AgdaSymbol{|}\AgdaSpace{}%
\AgdaInductiveConstructor{false}\AgdaSpace{}%
\AgdaSymbol{|}\AgdaSpace{}%
\AgdaInductiveConstructor{true}\AgdaSpace{}%
\AgdaSymbol{=}\AgdaSpace{}%
\AgdaInductiveConstructor{tt}\<%
\\
\>[0]\AgdaFunction{lemmaHoareTripleStackGeAux'23}\AgdaSpace{}%
\AgdaBound{msg₁}\AgdaSpace{}%
\AgdaBound{pbk1}\AgdaSpace{}%
\AgdaBound{pbk2}\AgdaSpace{}%
\AgdaBound{pbk3}\AgdaSpace{}%
\AgdaBound{pbk4}\AgdaSpace{}%
\AgdaBound{pbk5}\AgdaSpace{}%
\AgdaBound{sig1}\AgdaSpace{}%
\AgdaBound{sig2}\AgdaSpace{}%
\AgdaBound{sig3}\AgdaSpace{}%
\AgdaBound{x}\AgdaSpace{}%
\AgdaBound{x₁}\AgdaSpace{}%
\AgdaBound{x₂}\AgdaSpace{}%
\AgdaSymbol{|}\AgdaSpace{}%
\AgdaInductiveConstructor{false}\AgdaSpace{}%
\AgdaSymbol{|}\AgdaSpace{}%
\AgdaInductiveConstructor{true}\AgdaSpace{}%
\AgdaSymbol{|}\AgdaSpace{}%
\AgdaInductiveConstructor{true}\AgdaSpace{}%
\AgdaSymbol{|}\AgdaSpace{}%
\AgdaInductiveConstructor{true}\AgdaSpace{}%
\AgdaSymbol{=}\AgdaSpace{}%
\AgdaInductiveConstructor{tt}\<%
\\
\>[0]\AgdaFunction{lemmaHoareTripleStackGeAux'23}\AgdaSpace{}%
\AgdaBound{msg₁}\AgdaSpace{}%
\AgdaBound{pbk1}\AgdaSpace{}%
\AgdaBound{pbk2}\AgdaSpace{}%
\AgdaBound{pbk3}\AgdaSpace{}%
\AgdaBound{pbk4}\AgdaSpace{}%
\AgdaBound{pbk5}\AgdaSpace{}%
\AgdaBound{sig1}\AgdaSpace{}%
\AgdaBound{sig2}\AgdaSpace{}%
\AgdaBound{sig3}\AgdaSpace{}%
\AgdaBound{x}\AgdaSpace{}%
\AgdaBound{x₁}\AgdaSpace{}%
\AgdaBound{x₂}\AgdaSpace{}%
\AgdaSymbol{|}\AgdaSpace{}%
\AgdaInductiveConstructor{true}\AgdaSpace{}%
\AgdaKeyword{with}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaFunction{isSigned}%
\>[106]\AgdaBound{msg₁}\AgdaSpace{}%
\AgdaBound{sig2}\AgdaSpace{}%
\AgdaBound{pbk2}\AgdaSymbol{)}\<%
\\
\>[0]\AgdaFunction{lemmaHoareTripleStackGeAux'23}\AgdaSpace{}%
\AgdaBound{msg₁}\AgdaSpace{}%
\AgdaBound{pbk1}\AgdaSpace{}%
\AgdaBound{pbk2}\AgdaSpace{}%
\AgdaBound{pbk3}\AgdaSpace{}%
\AgdaBound{pbk4}\AgdaSpace{}%
\AgdaBound{pbk5}\AgdaSpace{}%
\AgdaBound{sig1}\AgdaSpace{}%
\AgdaBound{sig2}\AgdaSpace{}%
\AgdaBound{sig3}\AgdaSpace{}%
\AgdaBound{x}\AgdaSpace{}%
\AgdaBound{x₁}\AgdaSpace{}%
\AgdaBound{x₂}\AgdaSpace{}%
\AgdaSymbol{|}\AgdaSpace{}%
\AgdaInductiveConstructor{true}\AgdaSpace{}%
\AgdaSymbol{|}\AgdaSpace{}%
\AgdaInductiveConstructor{false}\AgdaSpace{}%
\AgdaKeyword{with}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaFunction{isSigned}%
\>[114]\AgdaBound{msg₁}\AgdaSpace{}%
\AgdaBound{sig2}\AgdaSpace{}%
\AgdaBound{pbk3}\AgdaSymbol{)}\<%
\\
\>[0]\AgdaFunction{lemmaHoareTripleStackGeAux'23}\AgdaSpace{}%
\AgdaBound{msg₁}\AgdaSpace{}%
\AgdaBound{pbk1}\AgdaSpace{}%
\AgdaBound{pbk2}\AgdaSpace{}%
\AgdaBound{pbk3}\AgdaSpace{}%
\AgdaBound{pbk4}\AgdaSpace{}%
\AgdaBound{pbk5}\AgdaSpace{}%
\AgdaBound{sig1}\AgdaSpace{}%
\AgdaBound{sig2}\AgdaSpace{}%
\AgdaBound{sig3}\AgdaSpace{}%
\AgdaBound{x}\AgdaSpace{}%
\AgdaBound{x₁}\AgdaSpace{}%
\AgdaBound{x₂}\AgdaSpace{}%
\AgdaSymbol{|}\AgdaSpace{}%
\AgdaInductiveConstructor{true}\AgdaSpace{}%
\AgdaSymbol{|}\AgdaSpace{}%
\AgdaInductiveConstructor{false}\AgdaSpace{}%
\AgdaSymbol{|}\AgdaSpace{}%
\AgdaInductiveConstructor{false}\AgdaSpace{}%
\AgdaKeyword{with}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaFunction{isSigned}%
\>[122]\AgdaBound{msg₁}\AgdaSpace{}%
\AgdaBound{sig2}\AgdaSpace{}%
\AgdaBound{pbk4}\AgdaSymbol{)}\<%
\\
\>[0]\AgdaFunction{lemmaHoareTripleStackGeAux'23}\AgdaSpace{}%
\AgdaBound{msg₁}\AgdaSpace{}%
\AgdaBound{pbk1}\AgdaSpace{}%
\AgdaBound{pbk2}\AgdaSpace{}%
\AgdaBound{pbk3}\AgdaSpace{}%
\AgdaBound{pbk4}\AgdaSpace{}%
\AgdaBound{pbk5}\AgdaSpace{}%
\AgdaBound{sig1}\AgdaSpace{}%
\AgdaBound{sig2}\AgdaSpace{}%
\AgdaBound{sig3}\AgdaSpace{}%
\AgdaBound{x}\AgdaSpace{}%
\AgdaBound{x₁}\AgdaSpace{}%
\AgdaBound{x₂}\AgdaSpace{}%
\AgdaSymbol{|}\AgdaSpace{}%
\AgdaInductiveConstructor{true}\AgdaSpace{}%
\AgdaSymbol{|}\AgdaSpace{}%
\AgdaInductiveConstructor{false}\AgdaSpace{}%
\AgdaSymbol{|}\AgdaSpace{}%
\AgdaInductiveConstructor{false}\AgdaSpace{}%
\AgdaSymbol{|}\AgdaSpace{}%
\AgdaInductiveConstructor{true}\AgdaSpace{}%
\AgdaKeyword{with}%
\>[119]\AgdaSymbol{(}\AgdaFunction{isSigned}%
\>[130]\AgdaBound{msg₁}\AgdaSpace{}%
\AgdaBound{sig3}\AgdaSpace{}%
\AgdaBound{pbk5}\AgdaSymbol{)}\<%
\\
\>[0]\AgdaFunction{lemmaHoareTripleStackGeAux'23}\AgdaSpace{}%
\AgdaBound{msg₁}\AgdaSpace{}%
\AgdaBound{pbk1}\AgdaSpace{}%
\AgdaBound{pbk2}\AgdaSpace{}%
\AgdaBound{pbk3}\AgdaSpace{}%
\AgdaBound{pbk4}\AgdaSpace{}%
\AgdaBound{pbk5}\AgdaSpace{}%
\AgdaBound{sig1}\AgdaSpace{}%
\AgdaBound{sig2}\AgdaSpace{}%
\AgdaBound{sig3}\AgdaSpace{}%
\AgdaBound{x}\AgdaSpace{}%
\AgdaBound{x₁}\AgdaSpace{}%
\AgdaBound{x₂}\AgdaSpace{}%
\AgdaSymbol{|}\AgdaSpace{}%
\AgdaInductiveConstructor{true}\AgdaSpace{}%
\AgdaSymbol{|}\AgdaSpace{}%
\AgdaInductiveConstructor{false}\AgdaSpace{}%
\AgdaSymbol{|}\AgdaSpace{}%
\AgdaInductiveConstructor{false}\AgdaSpace{}%
\AgdaSymbol{|}\AgdaSpace{}%
\AgdaInductiveConstructor{true}\AgdaSpace{}%
\AgdaSymbol{|}\AgdaSpace{}%
\AgdaInductiveConstructor{true}\AgdaSpace{}%
\AgdaSymbol{=}\AgdaSpace{}%
\AgdaInductiveConstructor{tt}\<%
\\
\>[0]\AgdaFunction{lemmaHoareTripleStackGeAux'23}\AgdaSpace{}%
\AgdaBound{msg₁}\AgdaSpace{}%
\AgdaBound{pbk1}\AgdaSpace{}%
\AgdaBound{pbk2}\AgdaSpace{}%
\AgdaBound{pbk3}\AgdaSpace{}%
\AgdaBound{pbk4}\AgdaSpace{}%
\AgdaBound{pbk5}\AgdaSpace{}%
\AgdaBound{sig1}\AgdaSpace{}%
\AgdaBound{sig2}\AgdaSpace{}%
\AgdaBound{sig3}\AgdaSpace{}%
\AgdaBound{x}\AgdaSpace{}%
\AgdaBound{x₁}\AgdaSpace{}%
\AgdaBound{x₂}\AgdaSpace{}%
\AgdaSymbol{|}\AgdaSpace{}%
\AgdaInductiveConstructor{true}\AgdaSpace{}%
\AgdaSymbol{|}\AgdaSpace{}%
\AgdaInductiveConstructor{false}\AgdaSpace{}%
\AgdaSymbol{|}\AgdaSpace{}%
\AgdaInductiveConstructor{true}\AgdaSpace{}%
\AgdaKeyword{with}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaFunction{isSigned}%
\>[121]\AgdaBound{msg₁}\AgdaSpace{}%
\AgdaBound{sig3}\AgdaSpace{}%
\AgdaBound{pbk4}\AgdaSymbol{)}\<%
\\
\>[0]\AgdaFunction{lemmaHoareTripleStackGeAux'23}\AgdaSpace{}%
\AgdaBound{msg₁}\AgdaSpace{}%
\AgdaBound{pbk1}\AgdaSpace{}%
\AgdaBound{pbk2}\AgdaSpace{}%
\AgdaBound{pbk3}\AgdaSpace{}%
\AgdaBound{pbk4}\AgdaSpace{}%
\AgdaBound{pbk5}\AgdaSpace{}%
\AgdaBound{sig1}\AgdaSpace{}%
\AgdaBound{sig2}\AgdaSpace{}%
\AgdaBound{sig3}\AgdaSpace{}%
\AgdaBound{x}\AgdaSpace{}%
\AgdaBound{x₁}\AgdaSpace{}%
\AgdaBound{x₂}\AgdaSpace{}%
\AgdaSymbol{|}\AgdaSpace{}%
\AgdaInductiveConstructor{true}\AgdaSpace{}%
\AgdaSymbol{|}\AgdaSpace{}%
\AgdaInductiveConstructor{false}\AgdaSpace{}%
\AgdaSymbol{|}\AgdaSpace{}%
\AgdaInductiveConstructor{true}\AgdaSpace{}%
\AgdaSymbol{|}\AgdaSpace{}%
\AgdaInductiveConstructor{false}\AgdaSpace{}%
\AgdaKeyword{with}%
\>[119]\AgdaSymbol{(}\AgdaFunction{isSigned}%
\>[130]\AgdaBound{msg₁}\AgdaSpace{}%
\AgdaBound{sig3}\AgdaSpace{}%
\AgdaBound{pbk5}\AgdaSymbol{)}\<%
\\
\>[0]\AgdaFunction{lemmaHoareTripleStackGeAux'23}\AgdaSpace{}%
\AgdaBound{msg₁}\AgdaSpace{}%
\AgdaBound{pbk1}\AgdaSpace{}%
\AgdaBound{pbk2}\AgdaSpace{}%
\AgdaBound{pbk3}\AgdaSpace{}%
\AgdaBound{pbk4}\AgdaSpace{}%
\AgdaBound{pbk5}\AgdaSpace{}%
\AgdaBound{sig1}\AgdaSpace{}%
\AgdaBound{sig2}\AgdaSpace{}%
\AgdaBound{sig3}\AgdaSpace{}%
\AgdaBound{x}\AgdaSpace{}%
\AgdaBound{x₁}\AgdaSpace{}%
\AgdaBound{x₂}\AgdaSpace{}%
\AgdaSymbol{|}\AgdaSpace{}%
\AgdaInductiveConstructor{true}\AgdaSpace{}%
\AgdaSymbol{|}\AgdaSpace{}%
\AgdaInductiveConstructor{false}\AgdaSpace{}%
\AgdaSymbol{|}\AgdaSpace{}%
\AgdaInductiveConstructor{true}\AgdaSpace{}%
\AgdaSymbol{|}\AgdaSpace{}%
\AgdaInductiveConstructor{false}\AgdaSpace{}%
\AgdaSymbol{|}\AgdaSpace{}%
\AgdaInductiveConstructor{true}\AgdaSpace{}%
\AgdaSymbol{=}\AgdaSpace{}%
\AgdaInductiveConstructor{tt}\<%
\\
\>[0]\AgdaFunction{lemmaHoareTripleStackGeAux'23}\AgdaSpace{}%
\AgdaBound{msg₁}\AgdaSpace{}%
\AgdaBound{pbk1}\AgdaSpace{}%
\AgdaBound{pbk2}\AgdaSpace{}%
\AgdaBound{pbk3}\AgdaSpace{}%
\AgdaBound{pbk4}\AgdaSpace{}%
\AgdaBound{pbk5}\AgdaSpace{}%
\AgdaBound{sig1}\AgdaSpace{}%
\AgdaBound{sig2}\AgdaSpace{}%
\AgdaBound{sig3}\AgdaSpace{}%
\AgdaBound{x}\AgdaSpace{}%
\AgdaBound{x₁}\AgdaSpace{}%
\AgdaBound{x₂}\AgdaSpace{}%
\AgdaSymbol{|}\AgdaSpace{}%
\AgdaInductiveConstructor{true}\AgdaSpace{}%
\AgdaSymbol{|}\AgdaSpace{}%
\AgdaInductiveConstructor{false}\AgdaSpace{}%
\AgdaSymbol{|}\AgdaSpace{}%
\AgdaInductiveConstructor{true}\AgdaSpace{}%
\AgdaSymbol{|}\AgdaSpace{}%
\AgdaInductiveConstructor{true}\AgdaSpace{}%
\AgdaSymbol{=}\AgdaSpace{}%
\AgdaInductiveConstructor{tt}\<%
\\
\>[0]\AgdaFunction{lemmaHoareTripleStackGeAux'23}\AgdaSpace{}%
\AgdaBound{msg₁}\AgdaSpace{}%
\AgdaBound{pbk1}\AgdaSpace{}%
\AgdaBound{pbk2}\AgdaSpace{}%
\AgdaBound{pbk3}\AgdaSpace{}%
\AgdaBound{pbk4}\AgdaSpace{}%
\AgdaBound{pbk5}\AgdaSpace{}%
\AgdaBound{sig1}\AgdaSpace{}%
\AgdaBound{sig2}\AgdaSpace{}%
\AgdaBound{sig3}\AgdaSpace{}%
\AgdaBound{x}\AgdaSpace{}%
\AgdaBound{x₁}\AgdaSpace{}%
\AgdaBound{x₂}\AgdaSpace{}%
\AgdaSymbol{|}\AgdaSpace{}%
\AgdaInductiveConstructor{true}\AgdaSpace{}%
\AgdaSymbol{|}\AgdaSpace{}%
\AgdaInductiveConstructor{true}\AgdaSpace{}%
\AgdaKeyword{with}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaFunction{isSigned}%
\>[113]\AgdaBound{msg₁}\AgdaSpace{}%
\AgdaBound{sig3}\AgdaSpace{}%
\AgdaBound{pbk3}\AgdaSymbol{)}\<%
\\
\>[0]\AgdaFunction{lemmaHoareTripleStackGeAux'23}\AgdaSpace{}%
\AgdaBound{msg₁}\AgdaSpace{}%
\AgdaBound{pbk1}\AgdaSpace{}%
\AgdaBound{pbk2}\AgdaSpace{}%
\AgdaBound{pbk3}\AgdaSpace{}%
\AgdaBound{pbk4}\AgdaSpace{}%
\AgdaBound{pbk5}\AgdaSpace{}%
\AgdaBound{sig1}\AgdaSpace{}%
\AgdaBound{sig2}\AgdaSpace{}%
\AgdaBound{sig3}\AgdaSpace{}%
\AgdaBound{x}\AgdaSpace{}%
\AgdaBound{x₁}\AgdaSpace{}%
\AgdaBound{x₂}\AgdaSpace{}%
\AgdaSymbol{|}\AgdaSpace{}%
\AgdaInductiveConstructor{true}\AgdaSpace{}%
\AgdaSymbol{|}\AgdaSpace{}%
\AgdaInductiveConstructor{true}\AgdaSpace{}%
\AgdaSymbol{|}\AgdaSpace{}%
\AgdaInductiveConstructor{false}\AgdaSpace{}%
\AgdaKeyword{with}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaFunction{isSigned}%
\>[121]\AgdaBound{msg₁}\AgdaSpace{}%
\AgdaBound{sig3}\AgdaSpace{}%
\AgdaBound{pbk4}\AgdaSymbol{)}\<%
\\
\>[0]\AgdaFunction{lemmaHoareTripleStackGeAux'23}\AgdaSpace{}%
\AgdaBound{msg₁}\AgdaSpace{}%
\AgdaBound{pbk1}\AgdaSpace{}%
\AgdaBound{pbk2}\AgdaSpace{}%
\AgdaBound{pbk3}\AgdaSpace{}%
\AgdaBound{pbk4}\AgdaSpace{}%
\AgdaBound{pbk5}\AgdaSpace{}%
\AgdaBound{sig1}\AgdaSpace{}%
\AgdaBound{sig2}\AgdaSpace{}%
\AgdaBound{sig3}\AgdaSpace{}%
\AgdaBound{x}\AgdaSpace{}%
\AgdaBound{x₁}\AgdaSpace{}%
\AgdaBound{x₂}\AgdaSpace{}%
\AgdaSymbol{|}\AgdaSpace{}%
\AgdaInductiveConstructor{true}\AgdaSpace{}%
\AgdaSymbol{|}\AgdaSpace{}%
\AgdaInductiveConstructor{true}\AgdaSpace{}%
\AgdaSymbol{|}\AgdaSpace{}%
\AgdaInductiveConstructor{false}\AgdaSpace{}%
\AgdaSymbol{|}\AgdaSpace{}%
\AgdaInductiveConstructor{false}\AgdaSpace{}%
\AgdaKeyword{with}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaFunction{isSigned}%
\>[129]\AgdaBound{msg₁}\AgdaSpace{}%
\AgdaBound{sig3}\AgdaSpace{}%
\AgdaBound{pbk5}\AgdaSymbol{)}\<%
\\
\>[0]\AgdaFunction{lemmaHoareTripleStackGeAux'23}\AgdaSpace{}%
\AgdaBound{msg₁}\AgdaSpace{}%
\AgdaBound{pbk1}\AgdaSpace{}%
\AgdaBound{pbk2}\AgdaSpace{}%
\AgdaBound{pbk3}\AgdaSpace{}%
\AgdaBound{pbk4}\AgdaSpace{}%
\AgdaBound{pbk5}\AgdaSpace{}%
\AgdaBound{sig1}\AgdaSpace{}%
\AgdaBound{sig2}\AgdaSpace{}%
\AgdaBound{sig3}\AgdaSpace{}%
\AgdaBound{x}\AgdaSpace{}%
\AgdaBound{x₁}\AgdaSpace{}%
\AgdaBound{x₂}\AgdaSpace{}%
\AgdaSymbol{|}\AgdaSpace{}%
\AgdaInductiveConstructor{true}\AgdaSpace{}%
\AgdaSymbol{|}\AgdaSpace{}%
\AgdaInductiveConstructor{true}\AgdaSpace{}%
\AgdaSymbol{|}\AgdaSpace{}%
\AgdaInductiveConstructor{false}\AgdaSpace{}%
\AgdaSymbol{|}\AgdaSpace{}%
\AgdaInductiveConstructor{false}\AgdaSpace{}%
\AgdaSymbol{|}\AgdaSpace{}%
\AgdaInductiveConstructor{true}\AgdaSpace{}%
\AgdaSymbol{=}\AgdaSpace{}%
\AgdaInductiveConstructor{tt}\<%
\\
\>[0]\AgdaFunction{lemmaHoareTripleStackGeAux'23}\AgdaSpace{}%
\AgdaBound{msg₁}\AgdaSpace{}%
\AgdaBound{pbk1}\AgdaSpace{}%
\AgdaBound{pbk2}\AgdaSpace{}%
\AgdaBound{pbk3}\AgdaSpace{}%
\AgdaBound{pbk4}\AgdaSpace{}%
\AgdaBound{pbk5}\AgdaSpace{}%
\AgdaBound{sig1}\AgdaSpace{}%
\AgdaBound{sig2}\AgdaSpace{}%
\AgdaBound{sig3}\AgdaSpace{}%
\AgdaBound{x}\AgdaSpace{}%
\AgdaBound{x₁}\AgdaSpace{}%
\AgdaBound{x₂}\AgdaSpace{}%
\AgdaSymbol{|}\AgdaSpace{}%
\AgdaInductiveConstructor{true}\AgdaSpace{}%
\AgdaSymbol{|}\AgdaSpace{}%
\AgdaInductiveConstructor{true}\AgdaSpace{}%
\AgdaSymbol{|}\AgdaSpace{}%
\AgdaInductiveConstructor{false}\AgdaSpace{}%
\AgdaSymbol{|}\AgdaSpace{}%
\AgdaInductiveConstructor{true}\AgdaSpace{}%
\AgdaSymbol{=}\AgdaSpace{}%
\AgdaInductiveConstructor{tt}\<%
\\
\>[0]\AgdaFunction{lemmaHoareTripleStackGeAux'23}\AgdaSpace{}%
\AgdaBound{msg₁}\AgdaSpace{}%
\AgdaBound{pbk1}\AgdaSpace{}%
\AgdaBound{pbk2}\AgdaSpace{}%
\AgdaBound{pbk3}\AgdaSpace{}%
\AgdaBound{pbk4}\AgdaSpace{}%
\AgdaBound{pbk5}\AgdaSpace{}%
\AgdaBound{sig1}\AgdaSpace{}%
\AgdaBound{sig2}\AgdaSpace{}%
\AgdaBound{sig3}\AgdaSpace{}%
\AgdaBound{x}\AgdaSpace{}%
\AgdaBound{x₁}\AgdaSpace{}%
\AgdaBound{x₂}\AgdaSpace{}%
\AgdaSymbol{|}\AgdaSpace{}%
\AgdaInductiveConstructor{true}\AgdaSpace{}%
\AgdaSymbol{|}\AgdaSpace{}%
\AgdaInductiveConstructor{true}\AgdaSpace{}%
\AgdaSymbol{|}\AgdaSpace{}%
\AgdaInductiveConstructor{true}\AgdaSpace{}%
\AgdaSymbol{=}\AgdaSpace{}%
\AgdaInductiveConstructor{tt}\<%
\\
%
\\[\AgdaEmptyExtraSkip]%
%
\\[\AgdaEmptyExtraSkip]%
%
\\[\AgdaEmptyExtraSkip]%
%
\\[\AgdaEmptyExtraSkip]%
%
\\[\AgdaEmptyExtraSkip]%
\>[0]\AgdaFunction{lemmaHoareTripleStackGeAux'Comb3-5}\AgdaSpace{}%
\AgdaSymbol{:}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaBound{msg₁}\AgdaSpace{}%
\AgdaSymbol{:}\AgdaSpace{}%
\AgdaDatatype{Msg}\AgdaSymbol{)}\<%
\\
\>[0][@{}l@{\AgdaIndent{0}}]%
\>[9]\AgdaSymbol{(}\AgdaBound{pbk1}\AgdaSpace{}%
\AgdaBound{pbk2}\AgdaSpace{}%
\AgdaBound{pbk3}\AgdaSpace{}%
\AgdaBound{pbk4}\AgdaSpace{}%
\AgdaBound{pbk5}\AgdaSpace{}%
\AgdaBound{sig1}\AgdaSpace{}%
\AgdaBound{sig2}\AgdaSpace{}%
\AgdaBound{sig3}\AgdaSpace{}%
\AgdaSymbol{:}\AgdaSpace{}%
\AgdaDatatype{ℕ}\AgdaSymbol{)}\<%
\\
\>[9][@{}l@{\AgdaIndent{0}}]%
\>[10]\AgdaSymbol{→}\AgdaSpace{}%
\AgdaFunction{True}%
\>[6499I]\AgdaSymbol{(}\AgdaFunction{compareSigsMultiSigAux}\AgdaSpace{}%
\AgdaBound{msg₁}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaBound{sig2}\AgdaSpace{}%
\AgdaOperator{\AgdaInductiveConstructor{∷}}\AgdaSpace{}%
\AgdaBound{sig3}\AgdaSpace{}%
\AgdaOperator{\AgdaInductiveConstructor{∷}}\AgdaSpace{}%
\AgdaInductiveConstructor{[]}\AgdaSymbol{)}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaSpace{}%
\AgdaBound{pbk2}\AgdaSpace{}%
\AgdaOperator{\AgdaInductiveConstructor{∷}}\AgdaSpace{}%
\AgdaBound{pbk3}\AgdaSpace{}%
\AgdaOperator{\AgdaInductiveConstructor{∷}}\AgdaSpace{}%
\AgdaBound{pbk4}\AgdaSpace{}%
\AgdaOperator{\AgdaInductiveConstructor{∷}}\AgdaSpace{}%
\AgdaBound{pbk5}\AgdaSpace{}%
\AgdaOperator{\AgdaInductiveConstructor{∷}}\AgdaSpace{}%
\AgdaInductiveConstructor{[]}\AgdaSymbol{)}%
\>[100]\AgdaBound{sig1}\<%
\\
\>[.][@{}l@{}]\<[6499I]%
\>[17]\AgdaSymbol{(}\AgdaFunction{isSigned}%
\>[28]\AgdaBound{msg₁}\AgdaSpace{}%
\AgdaBound{sig1}\AgdaSpace{}%
\AgdaBound{pbk1}\AgdaSpace{}%
\AgdaSymbol{))}\<%
\\
\>[0][@{}l@{\AgdaIndent{0}}]%
\>[6]\AgdaSymbol{→}%
\>[9]\AgdaSymbol{((}\AgdaFunction{True}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaFunction{isSigned}%
\>[27]\AgdaBound{msg₁}\AgdaSpace{}%
\AgdaBound{sig1}\AgdaSpace{}%
\AgdaBound{pbk1}\AgdaSymbol{)}\AgdaSpace{}%
\AgdaOperator{\AgdaRecord{∧}}\AgdaSpace{}%
\AgdaFunction{True}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaFunction{isSigned}%
\>[61]\AgdaBound{msg₁}\AgdaSpace{}%
\AgdaBound{sig2}\AgdaSpace{}%
\AgdaBound{pbk2}\AgdaSymbol{))}\AgdaSpace{}%
\AgdaOperator{\AgdaRecord{∧}}\AgdaSpace{}%
\AgdaFunction{True}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaFunction{isSigned}%
\>[96]\AgdaBound{msg₁}\AgdaSpace{}%
\AgdaBound{sig3}\AgdaSpace{}%
\AgdaBound{pbk3}\AgdaSymbol{))}\AgdaSpace{}%
\AgdaOperator{\AgdaDatatype{⊎}}\<%
\\
\>[9][@{}l@{\AgdaIndent{0}}]%
\>[10]\AgdaSymbol{((}\AgdaFunction{True}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaFunction{isSigned}%
\>[28]\AgdaBound{msg₁}\AgdaSpace{}%
\AgdaBound{sig1}\AgdaSpace{}%
\AgdaBound{pbk1}\AgdaSymbol{)}\AgdaSpace{}%
\AgdaOperator{\AgdaRecord{∧}}\AgdaSpace{}%
\AgdaFunction{True}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaFunction{isSigned}%
\>[62]\AgdaBound{msg₁}\AgdaSpace{}%
\AgdaBound{sig2}\AgdaSpace{}%
\AgdaBound{pbk2}\AgdaSymbol{))}\AgdaSpace{}%
\AgdaOperator{\AgdaRecord{∧}}\AgdaSpace{}%
\AgdaFunction{True}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaFunction{isSigned}%
\>[97]\AgdaBound{msg₁}\AgdaSpace{}%
\AgdaBound{sig3}\AgdaSpace{}%
\AgdaBound{pbk4}\AgdaSymbol{))}\AgdaSpace{}%
\AgdaOperator{\AgdaDatatype{⊎}}\<%
\\
%
\>[10]\AgdaSymbol{((}\AgdaFunction{True}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaFunction{isSigned}%
\>[28]\AgdaBound{msg₁}\AgdaSpace{}%
\AgdaBound{sig1}\AgdaSpace{}%
\AgdaBound{pbk1}\AgdaSymbol{)}\AgdaSpace{}%
\AgdaOperator{\AgdaRecord{∧}}\AgdaSpace{}%
\AgdaFunction{True}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaFunction{isSigned}%
\>[62]\AgdaBound{msg₁}\AgdaSpace{}%
\AgdaBound{sig2}\AgdaSpace{}%
\AgdaBound{pbk2}\AgdaSymbol{))}\AgdaSpace{}%
\AgdaOperator{\AgdaRecord{∧}}\AgdaSpace{}%
\AgdaFunction{True}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaFunction{isSigned}%
\>[97]\AgdaBound{msg₁}\AgdaSpace{}%
\AgdaBound{sig3}\AgdaSpace{}%
\AgdaBound{pbk5}\AgdaSymbol{))}\AgdaSpace{}%
\AgdaOperator{\AgdaDatatype{⊎}}\<%
\\
%
\>[10]\AgdaSymbol{((}\AgdaFunction{True}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaFunction{isSigned}%
\>[28]\AgdaBound{msg₁}\AgdaSpace{}%
\AgdaBound{sig1}\AgdaSpace{}%
\AgdaBound{pbk1}\AgdaSymbol{)}\AgdaSpace{}%
\AgdaOperator{\AgdaRecord{∧}}\AgdaSpace{}%
\AgdaFunction{True}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaFunction{isSigned}%
\>[62]\AgdaBound{msg₁}\AgdaSpace{}%
\AgdaBound{sig2}\AgdaSpace{}%
\AgdaBound{pbk3}\AgdaSymbol{))}\AgdaSpace{}%
\AgdaOperator{\AgdaRecord{∧}}\AgdaSpace{}%
\AgdaFunction{True}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaFunction{isSigned}%
\>[97]\AgdaBound{msg₁}\AgdaSpace{}%
\AgdaBound{sig3}\AgdaSpace{}%
\AgdaBound{pbk4}\AgdaSymbol{))}\AgdaSpace{}%
\AgdaOperator{\AgdaDatatype{⊎}}\<%
\\
%
\>[10]\AgdaSymbol{((}\AgdaFunction{True}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaFunction{isSigned}%
\>[28]\AgdaBound{msg₁}\AgdaSpace{}%
\AgdaBound{sig1}\AgdaSpace{}%
\AgdaBound{pbk1}\AgdaSymbol{)}\AgdaSpace{}%
\AgdaOperator{\AgdaRecord{∧}}\AgdaSpace{}%
\AgdaFunction{True}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaFunction{isSigned}%
\>[62]\AgdaBound{msg₁}\AgdaSpace{}%
\AgdaBound{sig2}\AgdaSpace{}%
\AgdaBound{pbk3}\AgdaSymbol{))}\AgdaSpace{}%
\AgdaOperator{\AgdaRecord{∧}}\AgdaSpace{}%
\AgdaFunction{True}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaFunction{isSigned}%
\>[97]\AgdaBound{msg₁}\AgdaSpace{}%
\AgdaBound{sig3}\AgdaSpace{}%
\AgdaBound{pbk5}\AgdaSymbol{))}\AgdaSpace{}%
\AgdaOperator{\AgdaDatatype{⊎}}\<%
\\
%
\>[10]\AgdaSymbol{((}\AgdaFunction{True}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaFunction{isSigned}%
\>[28]\AgdaBound{msg₁}\AgdaSpace{}%
\AgdaBound{sig1}\AgdaSpace{}%
\AgdaBound{pbk1}\AgdaSymbol{)}\AgdaSpace{}%
\AgdaOperator{\AgdaRecord{∧}}\AgdaSpace{}%
\AgdaFunction{True}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaFunction{isSigned}%
\>[62]\AgdaBound{msg₁}\AgdaSpace{}%
\AgdaBound{sig2}\AgdaSpace{}%
\AgdaBound{pbk4}\AgdaSymbol{))}\AgdaSpace{}%
\AgdaOperator{\AgdaRecord{∧}}\AgdaSpace{}%
\AgdaFunction{True}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaFunction{isSigned}%
\>[97]\AgdaBound{msg₁}\AgdaSpace{}%
\AgdaBound{sig3}\AgdaSpace{}%
\AgdaBound{pbk5}\AgdaSymbol{))}\AgdaSpace{}%
\AgdaOperator{\AgdaDatatype{⊎}}\<%
\\
%
\>[10]\AgdaSymbol{((}\AgdaFunction{True}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaFunction{isSigned}%
\>[28]\AgdaBound{msg₁}\AgdaSpace{}%
\AgdaBound{sig1}\AgdaSpace{}%
\AgdaBound{pbk2}\AgdaSymbol{)}\AgdaSpace{}%
\AgdaOperator{\AgdaRecord{∧}}\AgdaSpace{}%
\AgdaFunction{True}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaFunction{isSigned}%
\>[62]\AgdaBound{msg₁}\AgdaSpace{}%
\AgdaBound{sig2}\AgdaSpace{}%
\AgdaBound{pbk3}\AgdaSymbol{))}\AgdaSpace{}%
\AgdaOperator{\AgdaRecord{∧}}\AgdaSpace{}%
\AgdaFunction{True}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaFunction{isSigned}%
\>[97]\AgdaBound{msg₁}\AgdaSpace{}%
\AgdaBound{sig3}\AgdaSpace{}%
\AgdaBound{pbk4}\AgdaSymbol{))}\AgdaSpace{}%
\AgdaOperator{\AgdaDatatype{⊎}}\<%
\\
%
\>[10]\AgdaSymbol{((}\AgdaFunction{True}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaFunction{isSigned}%
\>[28]\AgdaBound{msg₁}\AgdaSpace{}%
\AgdaBound{sig1}\AgdaSpace{}%
\AgdaBound{pbk2}\AgdaSymbol{)}\AgdaSpace{}%
\AgdaOperator{\AgdaRecord{∧}}\AgdaSpace{}%
\AgdaFunction{True}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaFunction{isSigned}%
\>[62]\AgdaBound{msg₁}\AgdaSpace{}%
\AgdaBound{sig2}\AgdaSpace{}%
\AgdaBound{pbk3}\AgdaSymbol{))}\AgdaSpace{}%
\AgdaOperator{\AgdaRecord{∧}}\AgdaSpace{}%
\AgdaFunction{True}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaFunction{isSigned}%
\>[97]\AgdaBound{msg₁}\AgdaSpace{}%
\AgdaBound{sig3}\AgdaSpace{}%
\AgdaBound{pbk5}\AgdaSymbol{))}\AgdaSpace{}%
\AgdaOperator{\AgdaDatatype{⊎}}\<%
\\
%
\>[10]\AgdaSymbol{((}\AgdaFunction{True}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaFunction{isSigned}%
\>[28]\AgdaBound{msg₁}\AgdaSpace{}%
\AgdaBound{sig1}\AgdaSpace{}%
\AgdaBound{pbk2}\AgdaSymbol{)}\AgdaSpace{}%
\AgdaOperator{\AgdaRecord{∧}}\AgdaSpace{}%
\AgdaFunction{True}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaFunction{isSigned}%
\>[62]\AgdaBound{msg₁}\AgdaSpace{}%
\AgdaBound{sig2}\AgdaSpace{}%
\AgdaBound{pbk4}\AgdaSymbol{))}\AgdaSpace{}%
\AgdaOperator{\AgdaRecord{∧}}\AgdaSpace{}%
\AgdaFunction{True}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaFunction{isSigned}%
\>[97]\AgdaBound{msg₁}\AgdaSpace{}%
\AgdaBound{sig3}\AgdaSpace{}%
\AgdaBound{pbk5}\AgdaSymbol{))}\AgdaSpace{}%
\AgdaOperator{\AgdaDatatype{⊎}}\<%
\\
%
\>[10]\AgdaSymbol{((}\AgdaFunction{True}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaFunction{isSigned}%
\>[28]\AgdaBound{msg₁}\AgdaSpace{}%
\AgdaBound{sig1}\AgdaSpace{}%
\AgdaBound{pbk3}\AgdaSymbol{)}\AgdaSpace{}%
\AgdaOperator{\AgdaRecord{∧}}\AgdaSpace{}%
\AgdaFunction{True}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaFunction{isSigned}%
\>[62]\AgdaBound{msg₁}\AgdaSpace{}%
\AgdaBound{sig2}\AgdaSpace{}%
\AgdaBound{pbk4}\AgdaSymbol{))}\AgdaSpace{}%
\AgdaOperator{\AgdaRecord{∧}}\AgdaSpace{}%
\AgdaFunction{True}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaFunction{isSigned}%
\>[97]\AgdaBound{msg₁}\AgdaSpace{}%
\AgdaBound{sig3}\AgdaSpace{}%
\AgdaBound{pbk5}\AgdaSymbol{))}\<%
\\
%
\\[\AgdaEmptyExtraSkip]%
\>[0]\AgdaFunction{lemmaHoareTripleStackGeAux'Comb3-5}\AgdaSpace{}%
\AgdaBound{msg₁}\AgdaSpace{}%
\AgdaBound{pbk1}\AgdaSpace{}%
\AgdaBound{pbk2}\AgdaSpace{}%
\AgdaBound{pbk3}\AgdaSpace{}%
\AgdaBound{pbk4}\AgdaSpace{}%
\AgdaBound{pbk5}\AgdaSpace{}%
\AgdaBound{sig1}\AgdaSpace{}%
\AgdaBound{sig2}\AgdaSpace{}%
\AgdaBound{sig3}\AgdaSpace{}%
\AgdaBound{x}\AgdaSpace{}%
\AgdaKeyword{with}%
\>[88]\AgdaSymbol{(}\AgdaFunction{isSigned}%
\>[99]\AgdaBound{msg₁}\AgdaSpace{}%
\AgdaBound{sig1}\AgdaSpace{}%
\AgdaBound{pbk1}\AgdaSymbol{)}\<%
\\
\>[0]\AgdaFunction{lemmaHoareTripleStackGeAux'Comb3-5}\AgdaSpace{}%
\AgdaBound{msg₁}\AgdaSpace{}%
\AgdaBound{pbk1}\AgdaSpace{}%
\AgdaBound{pbk2}\AgdaSpace{}%
\AgdaBound{pbk3}\AgdaSpace{}%
\AgdaBound{pbk4}\AgdaSpace{}%
\AgdaBound{pbk5}\AgdaSpace{}%
\AgdaBound{sig1}\AgdaSpace{}%
\AgdaBound{sig2}\AgdaSpace{}%
\AgdaBound{sig3}\AgdaSpace{}%
\AgdaBound{x}\AgdaSpace{}%
\AgdaSymbol{|}\AgdaSpace{}%
\AgdaInductiveConstructor{false}\AgdaSpace{}%
\AgdaKeyword{with}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaFunction{isSigned}%
\>[106]\AgdaBound{msg₁}\AgdaSpace{}%
\AgdaBound{sig1}\AgdaSpace{}%
\AgdaBound{pbk2}\AgdaSymbol{)}\<%
\\
\>[0]\AgdaFunction{lemmaHoareTripleStackGeAux'Comb3-5}\AgdaSpace{}%
\AgdaBound{msg₁}\AgdaSpace{}%
\AgdaBound{pbk1}\AgdaSpace{}%
\AgdaBound{pbk2}\AgdaSpace{}%
\AgdaBound{pbk3}\AgdaSpace{}%
\AgdaBound{pbk4}\AgdaSpace{}%
\AgdaBound{pbk5}\AgdaSpace{}%
\AgdaBound{sig1}\AgdaSpace{}%
\AgdaBound{sig2}\AgdaSpace{}%
\AgdaBound{sig3}\AgdaSpace{}%
\AgdaBound{x}\AgdaSpace{}%
\AgdaSymbol{|}\AgdaSpace{}%
\AgdaInductiveConstructor{false}\AgdaSpace{}%
\AgdaSymbol{|}\AgdaSpace{}%
\AgdaInductiveConstructor{false}\AgdaSpace{}%
\AgdaKeyword{with}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaFunction{isSigned}%
\>[114]\AgdaBound{msg₁}\AgdaSpace{}%
\AgdaBound{sig1}\AgdaSpace{}%
\AgdaBound{pbk3}\AgdaSymbol{)}\<%
\\
\>[0]\AgdaFunction{lemmaHoareTripleStackGeAux'Comb3-5}\AgdaSpace{}%
\AgdaBound{msg₁}\AgdaSpace{}%
\AgdaBound{pbk1}\AgdaSpace{}%
\AgdaBound{pbk2}\AgdaSpace{}%
\AgdaBound{pbk3}\AgdaSpace{}%
\AgdaBound{pbk4}\AgdaSpace{}%
\AgdaBound{pbk5}\AgdaSpace{}%
\AgdaBound{sig1}\AgdaSpace{}%
\AgdaBound{sig2}\AgdaSpace{}%
\AgdaBound{sig3}\AgdaSpace{}%
\AgdaBound{x}\AgdaSpace{}%
\AgdaSymbol{|}\AgdaSpace{}%
\AgdaInductiveConstructor{false}\AgdaSpace{}%
\AgdaSymbol{|}\AgdaSpace{}%
\AgdaInductiveConstructor{false}\AgdaSpace{}%
\AgdaSymbol{|}\AgdaSpace{}%
\AgdaInductiveConstructor{false}\AgdaSpace{}%
\AgdaKeyword{with}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaFunction{isSigned}%
\>[122]\AgdaBound{msg₁}\AgdaSpace{}%
\AgdaBound{sig1}\AgdaSpace{}%
\AgdaBound{pbk4}\AgdaSymbol{)}\<%
\\
\>[0]\AgdaFunction{lemmaHoareTripleStackGeAux'Comb3-5}\AgdaSpace{}%
\AgdaBound{msg₁}\AgdaSpace{}%
\AgdaBound{pbk1}\AgdaSpace{}%
\AgdaBound{pbk2}\AgdaSpace{}%
\AgdaBound{pbk3}\AgdaSpace{}%
\AgdaBound{pbk4}\AgdaSpace{}%
\AgdaBound{pbk5}\AgdaSpace{}%
\AgdaBound{sig1}\AgdaSpace{}%
\AgdaBound{sig2}\AgdaSpace{}%
\AgdaBound{sig3}\AgdaSpace{}%
\AgdaBound{x}\AgdaSpace{}%
\AgdaSymbol{|}\AgdaSpace{}%
\AgdaInductiveConstructor{false}\AgdaSpace{}%
\AgdaSymbol{|}\AgdaSpace{}%
\AgdaInductiveConstructor{false}\AgdaSpace{}%
\AgdaSymbol{|}\AgdaSpace{}%
\AgdaInductiveConstructor{false}\AgdaSpace{}%
\AgdaSymbol{|}\AgdaSpace{}%
\AgdaInductiveConstructor{false}\AgdaSpace{}%
\AgdaKeyword{with}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaFunction{isSigned}%
\>[130]\AgdaBound{msg₁}\AgdaSpace{}%
\AgdaBound{sig1}\AgdaSpace{}%
\AgdaBound{pbk5}\AgdaSymbol{)}\<%
\\
\>[0]\AgdaFunction{lemmaHoareTripleStackGeAux'Comb3-5}\AgdaSpace{}%
\AgdaBound{msg₁}\AgdaSpace{}%
\AgdaBound{pbk1}\AgdaSpace{}%
\AgdaBound{pbk2}\AgdaSpace{}%
\AgdaBound{pbk3}\AgdaSpace{}%
\AgdaBound{pbk4}\AgdaSpace{}%
\AgdaBound{pbk5}\AgdaSpace{}%
\AgdaBound{sig1}\AgdaSpace{}%
\AgdaBound{sig2}\AgdaSpace{}%
\AgdaBound{sig3}\AgdaSpace{}%
\AgdaSymbol{()}\AgdaSpace{}%
\AgdaSymbol{|}\AgdaSpace{}%
\AgdaInductiveConstructor{false}\AgdaSpace{}%
\AgdaSymbol{|}\AgdaSpace{}%
\AgdaInductiveConstructor{false}\AgdaSpace{}%
\AgdaSymbol{|}\AgdaSpace{}%
\AgdaInductiveConstructor{false}\AgdaSpace{}%
\AgdaSymbol{|}\AgdaSpace{}%
\AgdaInductiveConstructor{false}\AgdaSpace{}%
\AgdaSymbol{|}\AgdaSpace{}%
\AgdaInductiveConstructor{false}\<%
\\
\>[0]\AgdaFunction{lemmaHoareTripleStackGeAux'Comb3-5}\AgdaSpace{}%
\AgdaBound{msg₁}\AgdaSpace{}%
\AgdaBound{pbk1}\AgdaSpace{}%
\AgdaBound{pbk2}\AgdaSpace{}%
\AgdaBound{pbk3}\AgdaSpace{}%
\AgdaBound{pbk4}\AgdaSpace{}%
\AgdaBound{pbk5}\AgdaSpace{}%
\AgdaBound{sig1}\AgdaSpace{}%
\AgdaBound{sig2}\AgdaSpace{}%
\AgdaBound{sig3}\AgdaSpace{}%
\AgdaSymbol{()}\AgdaSpace{}%
\AgdaSymbol{|}\AgdaSpace{}%
\AgdaInductiveConstructor{false}\AgdaSpace{}%
\AgdaSymbol{|}\AgdaSpace{}%
\AgdaInductiveConstructor{false}\AgdaSpace{}%
\AgdaSymbol{|}\AgdaSpace{}%
\AgdaInductiveConstructor{false}\AgdaSpace{}%
\AgdaSymbol{|}\AgdaSpace{}%
\AgdaInductiveConstructor{false}\AgdaSpace{}%
\AgdaSymbol{|}\AgdaSpace{}%
\AgdaInductiveConstructor{true}\<%
\\
\>[0]\AgdaFunction{lemmaHoareTripleStackGeAux'Comb3-5}\AgdaSpace{}%
\AgdaBound{msg₁}\AgdaSpace{}%
\AgdaBound{pbk1}\AgdaSpace{}%
\AgdaBound{pbk2}\AgdaSpace{}%
\AgdaBound{pbk3}\AgdaSpace{}%
\AgdaBound{pbk4}\AgdaSpace{}%
\AgdaBound{pbk5}\AgdaSpace{}%
\AgdaBound{sig1}\AgdaSpace{}%
\AgdaBound{sig2}\AgdaSpace{}%
\AgdaBound{sig3}\AgdaSpace{}%
\AgdaBound{x}\AgdaSpace{}%
\AgdaSymbol{|}\AgdaSpace{}%
\AgdaInductiveConstructor{false}\AgdaSpace{}%
\AgdaSymbol{|}\AgdaSpace{}%
\AgdaInductiveConstructor{false}\AgdaSpace{}%
\AgdaSymbol{|}\AgdaSpace{}%
\AgdaInductiveConstructor{false}\AgdaSpace{}%
\AgdaSymbol{|}\AgdaSpace{}%
\AgdaInductiveConstructor{true}\AgdaSpace{}%
\AgdaKeyword{with}%
\>[119]\AgdaSymbol{(}\AgdaFunction{isSigned}%
\>[130]\AgdaBound{msg₁}\AgdaSpace{}%
\AgdaBound{sig2}\AgdaSpace{}%
\AgdaBound{pbk5}\AgdaSymbol{)}\<%
\\
\>[0]\AgdaFunction{lemmaHoareTripleStackGeAux'Comb3-5}\AgdaSpace{}%
\AgdaBound{msg₁}\AgdaSpace{}%
\AgdaBound{pbk1}\AgdaSpace{}%
\AgdaBound{pbk2}\AgdaSpace{}%
\AgdaBound{pbk3}\AgdaSpace{}%
\AgdaBound{pbk4}\AgdaSpace{}%
\AgdaBound{pbk5}\AgdaSpace{}%
\AgdaBound{sig1}\AgdaSpace{}%
\AgdaBound{sig2}\AgdaSpace{}%
\AgdaBound{sig3}\AgdaSpace{}%
\AgdaSymbol{()}\AgdaSpace{}%
\AgdaSymbol{|}\AgdaSpace{}%
\AgdaInductiveConstructor{false}\AgdaSpace{}%
\AgdaSymbol{|}\AgdaSpace{}%
\AgdaInductiveConstructor{false}\AgdaSpace{}%
\AgdaSymbol{|}\AgdaSpace{}%
\AgdaInductiveConstructor{false}\AgdaSpace{}%
\AgdaSymbol{|}\AgdaSpace{}%
\AgdaInductiveConstructor{true}\AgdaSpace{}%
\AgdaSymbol{|}\AgdaSpace{}%
\AgdaInductiveConstructor{false}\<%
\\
\>[0]\AgdaFunction{lemmaHoareTripleStackGeAux'Comb3-5}\AgdaSpace{}%
\AgdaBound{msg₁}\AgdaSpace{}%
\AgdaBound{pbk1}\AgdaSpace{}%
\AgdaBound{pbk2}\AgdaSpace{}%
\AgdaBound{pbk3}\AgdaSpace{}%
\AgdaBound{pbk4}\AgdaSpace{}%
\AgdaBound{pbk5}\AgdaSpace{}%
\AgdaBound{sig1}\AgdaSpace{}%
\AgdaBound{sig2}\AgdaSpace{}%
\AgdaBound{sig3}\AgdaSpace{}%
\AgdaSymbol{()}\AgdaSpace{}%
\AgdaSymbol{|}\AgdaSpace{}%
\AgdaInductiveConstructor{false}\AgdaSpace{}%
\AgdaSymbol{|}\AgdaSpace{}%
\AgdaInductiveConstructor{false}\AgdaSpace{}%
\AgdaSymbol{|}\AgdaSpace{}%
\AgdaInductiveConstructor{false}\AgdaSpace{}%
\AgdaSymbol{|}\AgdaSpace{}%
\AgdaInductiveConstructor{true}\AgdaSpace{}%
\AgdaSymbol{|}\AgdaSpace{}%
\AgdaInductiveConstructor{true}\<%
\\
\>[0]\AgdaFunction{lemmaHoareTripleStackGeAux'Comb3-5}\AgdaSpace{}%
\AgdaBound{msg₁}\AgdaSpace{}%
\AgdaBound{pbk1}\AgdaSpace{}%
\AgdaBound{pbk2}\AgdaSpace{}%
\AgdaBound{pbk3}\AgdaSpace{}%
\AgdaBound{pbk4}\AgdaSpace{}%
\AgdaBound{pbk5}\AgdaSpace{}%
\AgdaBound{sig1}\AgdaSpace{}%
\AgdaBound{sig2}\AgdaSpace{}%
\AgdaBound{sig3}\AgdaSpace{}%
\AgdaBound{x}\AgdaSpace{}%
\AgdaSymbol{|}\AgdaSpace{}%
\AgdaInductiveConstructor{false}\AgdaSpace{}%
\AgdaSymbol{|}\AgdaSpace{}%
\AgdaInductiveConstructor{false}\AgdaSpace{}%
\AgdaSymbol{|}\AgdaSpace{}%
\AgdaInductiveConstructor{true}\AgdaSpace{}%
\AgdaKeyword{with}%
\>[111]\AgdaSymbol{(}\AgdaFunction{isSigned}%
\>[122]\AgdaBound{msg₁}\AgdaSpace{}%
\AgdaBound{sig2}\AgdaSpace{}%
\AgdaBound{pbk4}\AgdaSymbol{)}\<%
\\
\>[0]\AgdaFunction{lemmaHoareTripleStackGeAux'Comb3-5}\AgdaSpace{}%
\AgdaBound{msg₁}\AgdaSpace{}%
\AgdaBound{pbk1}\AgdaSpace{}%
\AgdaBound{pbk2}\AgdaSpace{}%
\AgdaBound{pbk3}\AgdaSpace{}%
\AgdaBound{pbk4}\AgdaSpace{}%
\AgdaBound{pbk5}\AgdaSpace{}%
\AgdaBound{sig1}\AgdaSpace{}%
\AgdaBound{sig2}\AgdaSpace{}%
\AgdaBound{sig3}\AgdaSpace{}%
\AgdaBound{x}\AgdaSpace{}%
\AgdaSymbol{|}\AgdaSpace{}%
\AgdaInductiveConstructor{false}\AgdaSpace{}%
\AgdaSymbol{|}\AgdaSpace{}%
\AgdaInductiveConstructor{false}\AgdaSpace{}%
\AgdaSymbol{|}\AgdaSpace{}%
\AgdaInductiveConstructor{true}\AgdaSpace{}%
\AgdaSymbol{|}\AgdaSpace{}%
\AgdaInductiveConstructor{false}\AgdaSpace{}%
\AgdaKeyword{with}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaFunction{isSigned}%
\>[129]\AgdaBound{msg₁}\AgdaSpace{}%
\AgdaBound{sig2}\AgdaSpace{}%
\AgdaBound{pbk5}\AgdaSymbol{)}\<%
\\
\>[0]\AgdaFunction{lemmaHoareTripleStackGeAux'Comb3-5}\AgdaSpace{}%
\AgdaBound{msg₁}\AgdaSpace{}%
\AgdaBound{pbk1}\AgdaSpace{}%
\AgdaBound{pbk2}\AgdaSpace{}%
\AgdaBound{pbk3}\AgdaSpace{}%
\AgdaBound{pbk4}\AgdaSpace{}%
\AgdaBound{pbk5}\AgdaSpace{}%
\AgdaBound{sig1}\AgdaSpace{}%
\AgdaBound{sig2}\AgdaSpace{}%
\AgdaBound{sig3}\AgdaSpace{}%
\AgdaSymbol{()}\AgdaSpace{}%
\AgdaSymbol{|}\AgdaSpace{}%
\AgdaInductiveConstructor{false}\AgdaSpace{}%
\AgdaSymbol{|}\AgdaSpace{}%
\AgdaInductiveConstructor{false}\AgdaSpace{}%
\AgdaSymbol{|}\AgdaSpace{}%
\AgdaInductiveConstructor{true}\AgdaSpace{}%
\AgdaSymbol{|}\AgdaSpace{}%
\AgdaInductiveConstructor{false}\AgdaSpace{}%
\AgdaSymbol{|}\AgdaSpace{}%
\AgdaInductiveConstructor{false}\<%
\\
\>[0]\AgdaFunction{lemmaHoareTripleStackGeAux'Comb3-5}\AgdaSpace{}%
\AgdaBound{msg₁}\AgdaSpace{}%
\AgdaBound{pbk1}\AgdaSpace{}%
\AgdaBound{pbk2}\AgdaSpace{}%
\AgdaBound{pbk3}\AgdaSpace{}%
\AgdaBound{pbk4}\AgdaSpace{}%
\AgdaBound{pbk5}\AgdaSpace{}%
\AgdaBound{sig1}\AgdaSpace{}%
\AgdaBound{sig2}\AgdaSpace{}%
\AgdaBound{sig3}\AgdaSpace{}%
\AgdaSymbol{()}\AgdaSpace{}%
\AgdaSymbol{|}\AgdaSpace{}%
\AgdaInductiveConstructor{false}\AgdaSpace{}%
\AgdaSymbol{|}\AgdaSpace{}%
\AgdaInductiveConstructor{false}\AgdaSpace{}%
\AgdaSymbol{|}\AgdaSpace{}%
\AgdaInductiveConstructor{true}\AgdaSpace{}%
\AgdaSymbol{|}\AgdaSpace{}%
\AgdaInductiveConstructor{false}\AgdaSpace{}%
\AgdaSymbol{|}\AgdaSpace{}%
\AgdaInductiveConstructor{true}\<%
\\
\>[0]\AgdaFunction{lemmaHoareTripleStackGeAux'Comb3-5}\AgdaSpace{}%
\AgdaBound{msg₁}\AgdaSpace{}%
\AgdaBound{pbk1}\AgdaSpace{}%
\AgdaBound{pbk2}\AgdaSpace{}%
\AgdaBound{pbk3}\AgdaSpace{}%
\AgdaBound{pbk4}\AgdaSpace{}%
\AgdaBound{pbk5}\AgdaSpace{}%
\AgdaBound{sig1}\AgdaSpace{}%
\AgdaBound{sig2}\AgdaSpace{}%
\AgdaBound{sig3}\AgdaSpace{}%
\AgdaBound{x}\AgdaSpace{}%
\AgdaSymbol{|}\AgdaSpace{}%
\AgdaInductiveConstructor{false}\AgdaSpace{}%
\AgdaSymbol{|}\AgdaSpace{}%
\AgdaInductiveConstructor{false}\AgdaSpace{}%
\AgdaSymbol{|}\AgdaSpace{}%
\AgdaInductiveConstructor{true}\AgdaSpace{}%
\AgdaSymbol{|}\AgdaSpace{}%
\AgdaInductiveConstructor{true}\AgdaSpace{}%
\AgdaKeyword{with}%
\>[118]\AgdaSymbol{(}\AgdaFunction{isSigned}%
\>[129]\AgdaBound{msg₁}\AgdaSpace{}%
\AgdaBound{sig3}\AgdaSpace{}%
\AgdaBound{pbk5}\AgdaSymbol{)}\<%
\\
\>[0]\AgdaFunction{lemmaHoareTripleStackGeAux'Comb3-5}\AgdaSpace{}%
\AgdaBound{msg₁}\AgdaSpace{}%
\AgdaBound{pbk1}\AgdaSpace{}%
\AgdaBound{pbk2}\AgdaSpace{}%
\AgdaBound{pbk3}\AgdaSpace{}%
\AgdaBound{pbk4}%
\>[6955I]\AgdaBound{pbk5}\AgdaSpace{}%
\AgdaBound{sig1}\AgdaSpace{}%
\AgdaBound{sig2}\AgdaSpace{}%
\AgdaBound{sig3}\AgdaSpace{}%
\AgdaBound{x}\AgdaSpace{}%
\AgdaSymbol{|}\AgdaSpace{}%
\AgdaInductiveConstructor{false}\AgdaSpace{}%
\AgdaSymbol{|}\AgdaSpace{}%
\AgdaInductiveConstructor{false}\AgdaSpace{}%
\AgdaSymbol{|}\AgdaSpace{}%
\AgdaInductiveConstructor{true}\AgdaSpace{}%
\AgdaSymbol{|}\AgdaSpace{}%
\AgdaInductiveConstructor{true}\AgdaSpace{}%
\AgdaSymbol{|}\AgdaSpace{}%
\AgdaInductiveConstructor{true}\<%
\\
\>[6955I][@{}l@{\AgdaIndent{0}}]%
\>[62]\AgdaSymbol{=}\AgdaSpace{}%
\AgdaInductiveConstructor{inj₂}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaInductiveConstructor{inj₂}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaInductiveConstructor{inj₂}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaInductiveConstructor{inj₂}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaInductiveConstructor{inj₂}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaInductiveConstructor{inj₂}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaInductiveConstructor{inj₂}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaInductiveConstructor{inj₂}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaInductiveConstructor{inj₂}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaInductiveConstructor{conj}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaInductiveConstructor{conj}\AgdaSpace{}%
\AgdaInductiveConstructor{tt}\AgdaSpace{}%
\AgdaInductiveConstructor{tt}\AgdaSymbol{)}\AgdaSpace{}%
\AgdaInductiveConstructor{tt}\AgdaSymbol{)))))))))}\<%
\\
\>[0]\AgdaFunction{lemmaHoareTripleStackGeAux'Comb3-5}\AgdaSpace{}%
\AgdaBound{msg₁}\AgdaSpace{}%
\AgdaBound{pbk1}\AgdaSpace{}%
\AgdaBound{pbk2}\AgdaSpace{}%
\AgdaBound{pbk3}\AgdaSpace{}%
\AgdaBound{pbk4}\AgdaSpace{}%
\AgdaBound{pbk5}\AgdaSpace{}%
\AgdaBound{sig1}\AgdaSpace{}%
\AgdaBound{sig2}\AgdaSpace{}%
\AgdaBound{sig3}\AgdaSpace{}%
\AgdaBound{x}\AgdaSpace{}%
\AgdaSymbol{|}\AgdaSpace{}%
\AgdaInductiveConstructor{false}\AgdaSpace{}%
\AgdaSymbol{|}\AgdaSpace{}%
\AgdaInductiveConstructor{true}\AgdaSpace{}%
\AgdaKeyword{with}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaFunction{isSigned}%
\>[113]\AgdaBound{msg₁}\AgdaSpace{}%
\AgdaBound{sig2}\AgdaSpace{}%
\AgdaBound{pbk3}\AgdaSymbol{)}\<%
\\
\>[0]\AgdaFunction{lemmaHoareTripleStackGeAux'Comb3-5}\AgdaSpace{}%
\AgdaBound{msg₁}\AgdaSpace{}%
\AgdaBound{pbk1}\AgdaSpace{}%
\AgdaBound{pbk2}\AgdaSpace{}%
\AgdaBound{pbk3}\AgdaSpace{}%
\AgdaBound{pbk4}\AgdaSpace{}%
\AgdaBound{pbk5}\AgdaSpace{}%
\AgdaBound{sig1}\AgdaSpace{}%
\AgdaBound{sig2}\AgdaSpace{}%
\AgdaBound{sig3}\AgdaSpace{}%
\AgdaBound{x}\AgdaSpace{}%
\AgdaSymbol{|}\AgdaSpace{}%
\AgdaInductiveConstructor{false}\AgdaSpace{}%
\AgdaSymbol{|}\AgdaSpace{}%
\AgdaInductiveConstructor{true}\AgdaSpace{}%
\AgdaSymbol{|}\AgdaSpace{}%
\AgdaInductiveConstructor{false}\AgdaSpace{}%
\AgdaKeyword{with}%
\>[111]\AgdaSymbol{(}\AgdaFunction{isSigned}%
\>[122]\AgdaBound{msg₁}\AgdaSpace{}%
\AgdaBound{sig2}\AgdaSpace{}%
\AgdaBound{pbk4}\AgdaSymbol{)}\<%
\\
\>[0]\AgdaFunction{lemmaHoareTripleStackGeAux'Comb3-5}\AgdaSpace{}%
\AgdaBound{msg₁}\AgdaSpace{}%
\AgdaBound{pbk1}\AgdaSpace{}%
\AgdaBound{pbk2}\AgdaSpace{}%
\AgdaBound{pbk3}\AgdaSpace{}%
\AgdaBound{pbk4}\AgdaSpace{}%
\AgdaBound{pbk5}\AgdaSpace{}%
\AgdaBound{sig1}\AgdaSpace{}%
\AgdaBound{sig2}\AgdaSpace{}%
\AgdaBound{sig3}\AgdaSpace{}%
\AgdaBound{x}\AgdaSpace{}%
\AgdaSymbol{|}\AgdaSpace{}%
\AgdaInductiveConstructor{false}\AgdaSpace{}%
\AgdaSymbol{|}\AgdaSpace{}%
\AgdaInductiveConstructor{true}\AgdaSpace{}%
\AgdaSymbol{|}\AgdaSpace{}%
\AgdaInductiveConstructor{false}\AgdaSpace{}%
\AgdaSymbol{|}\AgdaSpace{}%
\AgdaInductiveConstructor{false}\AgdaSpace{}%
\AgdaKeyword{with}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaFunction{isSigned}%
\>[129]\AgdaBound{msg₁}\AgdaSpace{}%
\AgdaBound{sig2}\AgdaSpace{}%
\AgdaBound{pbk5}\AgdaSymbol{)}\<%
\\
\>[0]\AgdaFunction{lemmaHoareTripleStackGeAux'Comb3-5}\AgdaSpace{}%
\AgdaBound{msg₁}\AgdaSpace{}%
\AgdaBound{pbk1}\AgdaSpace{}%
\AgdaBound{pbk2}\AgdaSpace{}%
\AgdaBound{pbk3}\AgdaSpace{}%
\AgdaBound{pbk4}\AgdaSpace{}%
\AgdaBound{pbk5}\AgdaSpace{}%
\AgdaBound{sig1}\AgdaSpace{}%
\AgdaBound{sig2}\AgdaSpace{}%
\AgdaBound{sig3}\AgdaSpace{}%
\AgdaSymbol{()}\AgdaSpace{}%
\AgdaSymbol{|}\AgdaSpace{}%
\AgdaInductiveConstructor{false}\AgdaSpace{}%
\AgdaSymbol{|}\AgdaSpace{}%
\AgdaInductiveConstructor{true}\AgdaSpace{}%
\AgdaSymbol{|}\AgdaSpace{}%
\AgdaInductiveConstructor{false}\AgdaSpace{}%
\AgdaSymbol{|}\AgdaSpace{}%
\AgdaInductiveConstructor{false}\AgdaSpace{}%
\AgdaSymbol{|}\AgdaSpace{}%
\AgdaInductiveConstructor{false}\<%
\\
\>[0]\AgdaFunction{lemmaHoareTripleStackGeAux'Comb3-5}\AgdaSpace{}%
\AgdaBound{msg₁}\AgdaSpace{}%
\AgdaBound{pbk1}\AgdaSpace{}%
\AgdaBound{pbk2}\AgdaSpace{}%
\AgdaBound{pbk3}\AgdaSpace{}%
\AgdaBound{pbk4}\AgdaSpace{}%
\AgdaBound{pbk5}\AgdaSpace{}%
\AgdaBound{sig1}\AgdaSpace{}%
\AgdaBound{sig2}\AgdaSpace{}%
\AgdaBound{sig3}\AgdaSpace{}%
\AgdaSymbol{()}\AgdaSpace{}%
\AgdaSymbol{|}\AgdaSpace{}%
\AgdaInductiveConstructor{false}\AgdaSpace{}%
\AgdaSymbol{|}\AgdaSpace{}%
\AgdaInductiveConstructor{true}\AgdaSpace{}%
\AgdaSymbol{|}\AgdaSpace{}%
\AgdaInductiveConstructor{false}\AgdaSpace{}%
\AgdaSymbol{|}\AgdaSpace{}%
\AgdaInductiveConstructor{false}\AgdaSpace{}%
\AgdaSymbol{|}\AgdaSpace{}%
\AgdaInductiveConstructor{true}\<%
\\
\>[0]\AgdaFunction{lemmaHoareTripleStackGeAux'Comb3-5}\AgdaSpace{}%
\AgdaBound{msg₁}\AgdaSpace{}%
\AgdaBound{pbk1}\AgdaSpace{}%
\AgdaBound{pbk2}\AgdaSpace{}%
\AgdaBound{pbk3}\AgdaSpace{}%
\AgdaBound{pbk4}\AgdaSpace{}%
\AgdaBound{pbk5}\AgdaSpace{}%
\AgdaBound{sig1}\AgdaSpace{}%
\AgdaBound{sig2}\AgdaSpace{}%
\AgdaBound{sig3}\AgdaSpace{}%
\AgdaBound{x}\AgdaSpace{}%
\AgdaSymbol{|}\AgdaSpace{}%
\AgdaInductiveConstructor{false}\AgdaSpace{}%
\AgdaSymbol{|}\AgdaSpace{}%
\AgdaInductiveConstructor{true}\AgdaSpace{}%
\AgdaSymbol{|}\AgdaSpace{}%
\AgdaInductiveConstructor{false}\AgdaSpace{}%
\AgdaSymbol{|}\AgdaSpace{}%
\AgdaInductiveConstructor{true}\AgdaSpace{}%
\AgdaKeyword{with}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaFunction{isSigned}%
\>[128]\AgdaBound{msg₁}\AgdaSpace{}%
\AgdaBound{sig3}\AgdaSpace{}%
\AgdaBound{pbk5}\AgdaSymbol{)}\<%
\\
\>[0]\AgdaFunction{lemmaHoareTripleStackGeAux'Comb3-5}\AgdaSpace{}%
\AgdaBound{msg₁}\AgdaSpace{}%
\AgdaBound{pbk1}\AgdaSpace{}%
\AgdaBound{pbk2}\AgdaSpace{}%
\AgdaBound{pbk3}%
\>[7109I]\AgdaBound{pbk4}\AgdaSpace{}%
\AgdaBound{pbk5}\AgdaSpace{}%
\AgdaBound{sig1}\AgdaSpace{}%
\AgdaBound{sig2}\AgdaSpace{}%
\AgdaBound{sig3}\AgdaSpace{}%
\AgdaBound{x}\AgdaSpace{}%
\AgdaSymbol{|}\AgdaSpace{}%
\AgdaInductiveConstructor{false}\AgdaSpace{}%
\AgdaSymbol{|}\AgdaSpace{}%
\AgdaInductiveConstructor{true}\AgdaSpace{}%
\AgdaSymbol{|}\AgdaSpace{}%
\AgdaInductiveConstructor{false}\AgdaSpace{}%
\AgdaSymbol{|}\AgdaSpace{}%
\AgdaInductiveConstructor{true}\AgdaSpace{}%
\AgdaSymbol{|}\AgdaSpace{}%
\AgdaInductiveConstructor{true}\<%
\\
\>[7109I][@{}l@{\AgdaIndent{0}}]%
\>[56]\AgdaSymbol{=}%
\>[59]\AgdaInductiveConstructor{inj₂}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaInductiveConstructor{inj₂}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaInductiveConstructor{inj₂}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaInductiveConstructor{inj₂}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaInductiveConstructor{inj₂}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaInductiveConstructor{inj₂}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaInductiveConstructor{inj₂}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaInductiveConstructor{inj₂}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaInductiveConstructor{inj₁}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaInductiveConstructor{conj}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaInductiveConstructor{conj}\AgdaSpace{}%
\AgdaInductiveConstructor{tt}\AgdaSpace{}%
\AgdaInductiveConstructor{tt}\AgdaSymbol{)}\AgdaSpace{}%
\AgdaInductiveConstructor{tt}\AgdaSymbol{)))))))))}\<%
\\
\>[0]\AgdaFunction{lemmaHoareTripleStackGeAux'Comb3-5}\AgdaSpace{}%
\AgdaBound{msg₁}\AgdaSpace{}%
\AgdaBound{pbk1}\AgdaSpace{}%
\AgdaBound{pbk2}\AgdaSpace{}%
\AgdaBound{pbk3}\AgdaSpace{}%
\AgdaBound{pbk4}\AgdaSpace{}%
\AgdaBound{pbk5}\AgdaSpace{}%
\AgdaBound{sig1}\AgdaSpace{}%
\AgdaBound{sig2}\AgdaSpace{}%
\AgdaBound{sig3}\AgdaSpace{}%
\AgdaBound{x}\AgdaSpace{}%
\AgdaSymbol{|}\AgdaSpace{}%
\AgdaInductiveConstructor{false}\AgdaSpace{}%
\AgdaSymbol{|}\AgdaSpace{}%
\AgdaInductiveConstructor{true}\AgdaSpace{}%
\AgdaSymbol{|}\AgdaSpace{}%
\AgdaInductiveConstructor{true}\AgdaSpace{}%
\AgdaKeyword{with}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaFunction{isSigned}%
\>[120]\AgdaBound{msg₁}\AgdaSpace{}%
\AgdaBound{sig3}\AgdaSpace{}%
\AgdaBound{pbk4}\AgdaSymbol{)}\<%
\\
\>[0]\AgdaFunction{lemmaHoareTripleStackGeAux'Comb3-5}\AgdaSpace{}%
\AgdaBound{msg₁}\AgdaSpace{}%
\AgdaBound{pbk1}\AgdaSpace{}%
\AgdaBound{pbk2}\AgdaSpace{}%
\AgdaBound{pbk3}\AgdaSpace{}%
\AgdaBound{pbk4}\AgdaSpace{}%
\AgdaBound{pbk5}\AgdaSpace{}%
\AgdaBound{sig1}\AgdaSpace{}%
\AgdaBound{sig2}\AgdaSpace{}%
\AgdaBound{sig3}\AgdaSpace{}%
\AgdaBound{x}\AgdaSpace{}%
\AgdaSymbol{|}\AgdaSpace{}%
\AgdaInductiveConstructor{false}\AgdaSpace{}%
\AgdaSymbol{|}\AgdaSpace{}%
\AgdaInductiveConstructor{true}\AgdaSpace{}%
\AgdaSymbol{|}\AgdaSpace{}%
\AgdaInductiveConstructor{true}\AgdaSpace{}%
\AgdaSymbol{|}\AgdaSpace{}%
\AgdaInductiveConstructor{false}\AgdaSpace{}%
\AgdaKeyword{with}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaFunction{isSigned}%
\>[128]\AgdaBound{msg₁}\AgdaSpace{}%
\AgdaBound{sig3}\AgdaSpace{}%
\AgdaBound{pbk5}\AgdaSymbol{)}\<%
\\
\>[0]\AgdaFunction{lemmaHoareTripleStackGeAux'Comb3-5}\AgdaSpace{}%
\AgdaBound{msg₁}\AgdaSpace{}%
\AgdaBound{pbk1}\AgdaSpace{}%
\AgdaBound{pbk2}\AgdaSpace{}%
\AgdaBound{pbk3}%
\>[7184I]\AgdaBound{pbk4}\AgdaSpace{}%
\AgdaBound{pbk5}\AgdaSpace{}%
\AgdaBound{sig1}\AgdaSpace{}%
\AgdaBound{sig2}\AgdaSpace{}%
\AgdaBound{sig3}\AgdaSpace{}%
\AgdaBound{x}\AgdaSpace{}%
\AgdaSymbol{|}\AgdaSpace{}%
\AgdaInductiveConstructor{false}\AgdaSpace{}%
\AgdaSymbol{|}\AgdaSpace{}%
\AgdaInductiveConstructor{true}\AgdaSpace{}%
\AgdaSymbol{|}\AgdaSpace{}%
\AgdaInductiveConstructor{true}\AgdaSpace{}%
\AgdaSymbol{|}\AgdaSpace{}%
\AgdaInductiveConstructor{false}\AgdaSpace{}%
\AgdaSymbol{|}\AgdaSpace{}%
\AgdaInductiveConstructor{true}\<%
\\
\>[7184I][@{}l@{\AgdaIndent{0}}]%
\>[56]\AgdaSymbol{=}\AgdaSpace{}%
\AgdaInductiveConstructor{inj₂}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaInductiveConstructor{inj₂}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaInductiveConstructor{inj₂}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaInductiveConstructor{inj₂}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaInductiveConstructor{inj₂}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaInductiveConstructor{inj₂}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaInductiveConstructor{inj₂}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaInductiveConstructor{inj₁}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaInductiveConstructor{conj}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaInductiveConstructor{conj}\AgdaSpace{}%
\AgdaInductiveConstructor{tt}\AgdaSpace{}%
\AgdaInductiveConstructor{tt}\AgdaSymbol{)}\AgdaSpace{}%
\AgdaInductiveConstructor{tt}\AgdaSymbol{))))))))}\<%
\\
\>[0]\AgdaFunction{lemmaHoareTripleStackGeAux'Comb3-5}\AgdaSpace{}%
\AgdaBound{msg₁}\AgdaSpace{}%
\AgdaBound{pbk1}\AgdaSpace{}%
\AgdaBound{pbk2}\AgdaSpace{}%
\AgdaBound{pbk3}%
\>[7217I]\AgdaBound{pbk4}\AgdaSpace{}%
\AgdaBound{pbk5}\AgdaSpace{}%
\AgdaBound{sig1}\AgdaSpace{}%
\AgdaBound{sig2}\AgdaSpace{}%
\AgdaBound{sig3}\AgdaSpace{}%
\AgdaBound{x}\AgdaSpace{}%
\AgdaSymbol{|}\AgdaSpace{}%
\AgdaInductiveConstructor{false}\AgdaSpace{}%
\AgdaSymbol{|}\AgdaSpace{}%
\AgdaInductiveConstructor{true}\AgdaSpace{}%
\AgdaSymbol{|}\AgdaSpace{}%
\AgdaInductiveConstructor{true}\AgdaSpace{}%
\AgdaSymbol{|}\AgdaSpace{}%
\AgdaInductiveConstructor{true}\<%
\\
\>[7217I][@{}l@{\AgdaIndent{0}}]%
\>[56]\AgdaSymbol{=}\AgdaSpace{}%
\AgdaInductiveConstructor{inj₂}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaInductiveConstructor{inj₂}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaInductiveConstructor{inj₂}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaInductiveConstructor{inj₂}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaInductiveConstructor{inj₂}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaInductiveConstructor{inj₂}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaInductiveConstructor{inj₁}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaInductiveConstructor{conj}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaInductiveConstructor{conj}\AgdaSpace{}%
\AgdaInductiveConstructor{tt}\AgdaSpace{}%
\AgdaInductiveConstructor{tt}\AgdaSymbol{)}\AgdaSpace{}%
\AgdaInductiveConstructor{tt}\AgdaSymbol{)))))))}\<%
\\
\>[0]\AgdaFunction{lemmaHoareTripleStackGeAux'Comb3-5}\AgdaSpace{}%
\AgdaBound{msg₁}\AgdaSpace{}%
\AgdaBound{pbk1}\AgdaSpace{}%
\AgdaBound{pbk2}\AgdaSpace{}%
\AgdaBound{pbk3}\AgdaSpace{}%
\AgdaBound{pbk4}\AgdaSpace{}%
\AgdaBound{pbk5}\AgdaSpace{}%
\AgdaBound{sig1}\AgdaSpace{}%
\AgdaBound{sig2}\AgdaSpace{}%
\AgdaBound{sig3}\AgdaSpace{}%
\AgdaBound{x}\AgdaSpace{}%
\AgdaSymbol{|}\AgdaSpace{}%
\AgdaInductiveConstructor{true}\AgdaSpace{}%
\AgdaKeyword{with}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaFunction{isSigned}%
\>[105]\AgdaBound{msg₁}\AgdaSpace{}%
\AgdaBound{sig2}\AgdaSpace{}%
\AgdaBound{pbk2}\AgdaSymbol{)}\<%
\\
\>[0]\AgdaFunction{lemmaHoareTripleStackGeAux'Comb3-5}\AgdaSpace{}%
\AgdaBound{msg₁}\AgdaSpace{}%
\AgdaBound{pbk1}\AgdaSpace{}%
\AgdaBound{pbk2}\AgdaSpace{}%
\AgdaBound{pbk3}\AgdaSpace{}%
\AgdaBound{pbk4}\AgdaSpace{}%
\AgdaBound{pbk5}\AgdaSpace{}%
\AgdaBound{sig1}\AgdaSpace{}%
\AgdaBound{sig2}\AgdaSpace{}%
\AgdaBound{sig3}\AgdaSpace{}%
\AgdaBound{x}\AgdaSpace{}%
\AgdaSymbol{|}\AgdaSpace{}%
\AgdaInductiveConstructor{true}\AgdaSpace{}%
\AgdaSymbol{|}\AgdaSpace{}%
\AgdaInductiveConstructor{false}\AgdaSpace{}%
\AgdaKeyword{with}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaFunction{isSigned}%
\>[113]\AgdaBound{msg₁}\AgdaSpace{}%
\AgdaBound{sig2}\AgdaSpace{}%
\AgdaBound{pbk3}\AgdaSymbol{)}\<%
\\
\>[0]\AgdaFunction{lemmaHoareTripleStackGeAux'Comb3-5}\AgdaSpace{}%
\AgdaBound{msg₁}\AgdaSpace{}%
\AgdaBound{pbk1}\AgdaSpace{}%
\AgdaBound{pbk2}\AgdaSpace{}%
\AgdaBound{pbk3}\AgdaSpace{}%
\AgdaBound{pbk4}\AgdaSpace{}%
\AgdaBound{pbk5}\AgdaSpace{}%
\AgdaBound{sig1}\AgdaSpace{}%
\AgdaBound{sig2}\AgdaSpace{}%
\AgdaBound{sig3}\AgdaSpace{}%
\AgdaBound{x}\AgdaSpace{}%
\AgdaSymbol{|}\AgdaSpace{}%
\AgdaInductiveConstructor{true}\AgdaSpace{}%
\AgdaSymbol{|}\AgdaSpace{}%
\AgdaInductiveConstructor{false}\AgdaSpace{}%
\AgdaSymbol{|}\AgdaSpace{}%
\AgdaInductiveConstructor{false}\AgdaSpace{}%
\AgdaKeyword{with}%
\>[111]\AgdaSymbol{(}\AgdaFunction{isSigned}%
\>[122]\AgdaBound{msg₁}\AgdaSpace{}%
\AgdaBound{sig2}\AgdaSpace{}%
\AgdaBound{pbk4}\AgdaSymbol{)}\<%
\\
\>[0]\AgdaFunction{lemmaHoareTripleStackGeAux'Comb3-5}\AgdaSpace{}%
\AgdaBound{msg₁}\AgdaSpace{}%
\AgdaBound{pbk1}\AgdaSpace{}%
\AgdaBound{pbk2}\AgdaSpace{}%
\AgdaBound{pbk3}\AgdaSpace{}%
\AgdaBound{pbk4}\AgdaSpace{}%
\AgdaBound{pbk5}\AgdaSpace{}%
\AgdaBound{sig1}\AgdaSpace{}%
\AgdaBound{sig2}\AgdaSpace{}%
\AgdaBound{sig3}\AgdaSpace{}%
\AgdaBound{x}\AgdaSpace{}%
\AgdaSymbol{|}\AgdaSpace{}%
\AgdaInductiveConstructor{true}\AgdaSpace{}%
\AgdaSymbol{|}\AgdaSpace{}%
\AgdaInductiveConstructor{false}\AgdaSpace{}%
\AgdaSymbol{|}\AgdaSpace{}%
\AgdaInductiveConstructor{false}\AgdaSpace{}%
\AgdaSymbol{|}\AgdaSpace{}%
\AgdaInductiveConstructor{false}\AgdaSpace{}%
\AgdaKeyword{with}%
\>[119]\AgdaSymbol{(}\AgdaFunction{isSigned}%
\>[130]\AgdaBound{msg₁}\AgdaSpace{}%
\AgdaBound{sig2}\AgdaSpace{}%
\AgdaBound{pbk5}\AgdaSymbol{)}\<%
\\
\>[0]\AgdaFunction{lemmaHoareTripleStackGeAux'Comb3-5}\AgdaSpace{}%
\AgdaBound{msg₁}\AgdaSpace{}%
\AgdaBound{pbk1}\AgdaSpace{}%
\AgdaBound{pbk2}\AgdaSpace{}%
\AgdaBound{pbk3}\AgdaSpace{}%
\AgdaBound{pbk4}\AgdaSpace{}%
\AgdaBound{pbk5}\AgdaSpace{}%
\AgdaBound{sig1}\AgdaSpace{}%
\AgdaBound{sig2}\AgdaSpace{}%
\AgdaBound{sig3}\AgdaSpace{}%
\AgdaSymbol{()}\AgdaSpace{}%
\AgdaSymbol{|}\AgdaSpace{}%
\AgdaInductiveConstructor{true}\AgdaSpace{}%
\AgdaSymbol{|}\AgdaSpace{}%
\AgdaInductiveConstructor{false}\AgdaSpace{}%
\AgdaSymbol{|}\AgdaSpace{}%
\AgdaInductiveConstructor{false}\AgdaSpace{}%
\AgdaSymbol{|}\AgdaSpace{}%
\AgdaInductiveConstructor{false}\AgdaSpace{}%
\AgdaSymbol{|}\AgdaSpace{}%
\AgdaInductiveConstructor{false}\<%
\\
\>[0]\AgdaFunction{lemmaHoareTripleStackGeAux'Comb3-5}\AgdaSpace{}%
\AgdaBound{msg₁}\AgdaSpace{}%
\AgdaBound{pbk1}\AgdaSpace{}%
\AgdaBound{pbk2}\AgdaSpace{}%
\AgdaBound{pbk3}\AgdaSpace{}%
\AgdaBound{pbk4}\AgdaSpace{}%
\AgdaBound{pbk5}\AgdaSpace{}%
\AgdaBound{sig1}\AgdaSpace{}%
\AgdaBound{sig2}\AgdaSpace{}%
\AgdaBound{sig3}\AgdaSpace{}%
\AgdaSymbol{()}\AgdaSpace{}%
\AgdaSymbol{|}\AgdaSpace{}%
\AgdaInductiveConstructor{true}\AgdaSpace{}%
\AgdaSymbol{|}\AgdaSpace{}%
\AgdaInductiveConstructor{false}\AgdaSpace{}%
\AgdaSymbol{|}\AgdaSpace{}%
\AgdaInductiveConstructor{false}\AgdaSpace{}%
\AgdaSymbol{|}\AgdaSpace{}%
\AgdaInductiveConstructor{false}\AgdaSpace{}%
\AgdaSymbol{|}\AgdaSpace{}%
\AgdaInductiveConstructor{true}\<%
\\
\>[0]\AgdaFunction{lemmaHoareTripleStackGeAux'Comb3-5}\AgdaSpace{}%
\AgdaBound{msg₁}\AgdaSpace{}%
\AgdaBound{pbk1}\AgdaSpace{}%
\AgdaBound{pbk2}\AgdaSpace{}%
\AgdaBound{pbk3}\AgdaSpace{}%
\AgdaBound{pbk4}\AgdaSpace{}%
\AgdaBound{pbk5}\AgdaSpace{}%
\AgdaBound{sig1}\AgdaSpace{}%
\AgdaBound{sig2}\AgdaSpace{}%
\AgdaBound{sig3}\AgdaSpace{}%
\AgdaBound{x}\AgdaSpace{}%
\AgdaSymbol{|}\AgdaSpace{}%
\AgdaInductiveConstructor{true}\AgdaSpace{}%
\AgdaSymbol{|}\AgdaSpace{}%
\AgdaInductiveConstructor{false}\AgdaSpace{}%
\AgdaSymbol{|}\AgdaSpace{}%
\AgdaInductiveConstructor{false}\AgdaSpace{}%
\AgdaSymbol{|}\AgdaSpace{}%
\AgdaInductiveConstructor{true}\AgdaSpace{}%
\AgdaKeyword{with}%
\>[118]\AgdaSymbol{(}\AgdaFunction{isSigned}%
\>[129]\AgdaBound{msg₁}\AgdaSpace{}%
\AgdaBound{sig3}\AgdaSpace{}%
\AgdaBound{pbk5}\AgdaSymbol{)}\<%
\\
\>[0]\AgdaFunction{lemmaHoareTripleStackGeAux'Comb3-5}\AgdaSpace{}%
\AgdaBound{msg₁}\AgdaSpace{}%
\AgdaBound{pbk1}\AgdaSpace{}%
\AgdaBound{pbk2}\AgdaSpace{}%
\AgdaBound{pbk3}%
\>[7382I]\AgdaBound{pbk4}\AgdaSpace{}%
\AgdaBound{pbk5}\AgdaSpace{}%
\AgdaBound{sig1}\AgdaSpace{}%
\AgdaBound{sig2}\AgdaSpace{}%
\AgdaBound{sig3}\AgdaSpace{}%
\AgdaBound{x}\AgdaSpace{}%
\AgdaSymbol{|}\AgdaSpace{}%
\AgdaInductiveConstructor{true}\AgdaSpace{}%
\AgdaSymbol{|}\AgdaSpace{}%
\AgdaInductiveConstructor{false}\AgdaSpace{}%
\AgdaSymbol{|}\AgdaSpace{}%
\AgdaInductiveConstructor{false}\AgdaSpace{}%
\AgdaSymbol{|}\AgdaSpace{}%
\AgdaInductiveConstructor{true}\AgdaSpace{}%
\AgdaSymbol{|}\AgdaSpace{}%
\AgdaInductiveConstructor{true}\<%
\\
\>[7382I][@{}l@{\AgdaIndent{0}}]%
\>[56]\AgdaSymbol{=}\AgdaSpace{}%
\AgdaInductiveConstructor{inj₂}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaInductiveConstructor{inj₂}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaInductiveConstructor{inj₂}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaInductiveConstructor{inj₂}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaInductiveConstructor{inj₂}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaInductiveConstructor{inj₁}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaInductiveConstructor{conj}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaInductiveConstructor{conj}\AgdaSpace{}%
\AgdaInductiveConstructor{tt}\AgdaSpace{}%
\AgdaInductiveConstructor{tt}\AgdaSymbol{)}\AgdaSpace{}%
\AgdaInductiveConstructor{tt}\AgdaSymbol{))))))}\<%
\\
\>[0]\AgdaFunction{lemmaHoareTripleStackGeAux'Comb3-5}\AgdaSpace{}%
\AgdaBound{msg₁}\AgdaSpace{}%
\AgdaBound{pbk1}\AgdaSpace{}%
\AgdaBound{pbk2}\AgdaSpace{}%
\AgdaBound{pbk3}\AgdaSpace{}%
\AgdaBound{pbk4}\AgdaSpace{}%
\AgdaBound{pbk5}\AgdaSpace{}%
\AgdaBound{sig1}\AgdaSpace{}%
\AgdaBound{sig2}\AgdaSpace{}%
\AgdaBound{sig3}\AgdaSpace{}%
\AgdaBound{x}\AgdaSpace{}%
\AgdaSymbol{|}\AgdaSpace{}%
\AgdaInductiveConstructor{true}\AgdaSpace{}%
\AgdaSymbol{|}\AgdaSpace{}%
\AgdaInductiveConstructor{false}\AgdaSpace{}%
\AgdaSymbol{|}\AgdaSpace{}%
\AgdaInductiveConstructor{true}\AgdaSpace{}%
\AgdaKeyword{with}%
\>[110]\AgdaSymbol{(}\AgdaFunction{isSigned}%
\>[121]\AgdaBound{msg₁}\AgdaSpace{}%
\AgdaBound{sig3}\AgdaSpace{}%
\AgdaBound{pbk4}\AgdaSymbol{)}\<%
\\
\>[0]\AgdaFunction{lemmaHoareTripleStackGeAux'Comb3-5}\AgdaSpace{}%
\AgdaBound{msg₁}\AgdaSpace{}%
\AgdaBound{pbk1}\AgdaSpace{}%
\AgdaBound{pbk2}\AgdaSpace{}%
\AgdaBound{pbk3}\AgdaSpace{}%
\AgdaBound{pbk4}\AgdaSpace{}%
\AgdaBound{pbk5}\AgdaSpace{}%
\AgdaBound{sig1}\AgdaSpace{}%
\AgdaBound{sig2}\AgdaSpace{}%
\AgdaBound{sig3}\AgdaSpace{}%
\AgdaBound{x}\AgdaSpace{}%
\AgdaSymbol{|}\AgdaSpace{}%
\AgdaInductiveConstructor{true}\AgdaSpace{}%
\AgdaSymbol{|}\AgdaSpace{}%
\AgdaInductiveConstructor{false}\AgdaSpace{}%
\AgdaSymbol{|}\AgdaSpace{}%
\AgdaInductiveConstructor{true}\AgdaSpace{}%
\AgdaSymbol{|}\AgdaSpace{}%
\AgdaInductiveConstructor{false}\AgdaSpace{}%
\AgdaKeyword{with}%
\>[118]\AgdaSymbol{(}\AgdaFunction{isSigned}%
\>[129]\AgdaBound{msg₁}\AgdaSpace{}%
\AgdaBound{sig3}\AgdaSpace{}%
\AgdaBound{pbk5}\AgdaSymbol{)}\<%
\\
\>[0]\AgdaFunction{lemmaHoareTripleStackGeAux'Comb3-5}\AgdaSpace{}%
\AgdaBound{msg₁}\AgdaSpace{}%
\AgdaBound{pbk1}\AgdaSpace{}%
\AgdaBound{pbk2}\AgdaSpace{}%
\AgdaBound{pbk3}%
\>[7453I]\AgdaBound{pbk4}\AgdaSpace{}%
\AgdaBound{pbk5}\AgdaSpace{}%
\AgdaBound{sig1}\AgdaSpace{}%
\AgdaBound{sig2}\AgdaSpace{}%
\AgdaBound{sig3}\AgdaSpace{}%
\AgdaBound{x}\AgdaSpace{}%
\AgdaSymbol{|}\AgdaSpace{}%
\AgdaInductiveConstructor{true}\AgdaSpace{}%
\AgdaSymbol{|}\AgdaSpace{}%
\AgdaInductiveConstructor{false}\AgdaSpace{}%
\AgdaSymbol{|}\AgdaSpace{}%
\AgdaInductiveConstructor{true}\AgdaSpace{}%
\AgdaSymbol{|}\AgdaSpace{}%
\AgdaInductiveConstructor{false}\AgdaSpace{}%
\AgdaSymbol{|}\AgdaSpace{}%
\AgdaInductiveConstructor{true}\<%
\\
\>[7453I][@{}l@{\AgdaIndent{0}}]%
\>[56]\AgdaSymbol{=}\AgdaSpace{}%
\AgdaInductiveConstructor{inj₂}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaInductiveConstructor{inj₂}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaInductiveConstructor{inj₂}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaInductiveConstructor{inj₂}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaInductiveConstructor{inj₁}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaInductiveConstructor{conj}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaInductiveConstructor{conj}\AgdaSpace{}%
\AgdaInductiveConstructor{tt}\AgdaSpace{}%
\AgdaInductiveConstructor{tt}\AgdaSymbol{)}\AgdaSpace{}%
\AgdaInductiveConstructor{tt}\AgdaSymbol{)))))}\<%
\\
\>[0]\AgdaFunction{lemmaHoareTripleStackGeAux'Comb3-5}\AgdaSpace{}%
\AgdaBound{msg₁}\AgdaSpace{}%
\AgdaBound{pbk1}\AgdaSpace{}%
\AgdaBound{pbk2}\AgdaSpace{}%
\AgdaBound{pbk3}%
\>[7483I]\AgdaBound{pbk4}\AgdaSpace{}%
\AgdaBound{pbk5}\AgdaSpace{}%
\AgdaBound{sig1}\AgdaSpace{}%
\AgdaBound{sig2}\AgdaSpace{}%
\AgdaBound{sig3}\AgdaSpace{}%
\AgdaBound{x}\AgdaSpace{}%
\AgdaSymbol{|}\AgdaSpace{}%
\AgdaInductiveConstructor{true}\AgdaSpace{}%
\AgdaSymbol{|}\AgdaSpace{}%
\AgdaInductiveConstructor{false}\AgdaSpace{}%
\AgdaSymbol{|}\AgdaSpace{}%
\AgdaInductiveConstructor{true}\AgdaSpace{}%
\AgdaSymbol{|}\AgdaSpace{}%
\AgdaInductiveConstructor{true}\<%
\\
\>[7483I][@{}l@{\AgdaIndent{0}}]%
\>[56]\AgdaSymbol{=}\AgdaSpace{}%
\AgdaInductiveConstructor{inj₂}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaInductiveConstructor{inj₂}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaInductiveConstructor{inj₂}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaInductiveConstructor{inj₁}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaInductiveConstructor{conj}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaInductiveConstructor{conj}\AgdaSpace{}%
\AgdaInductiveConstructor{tt}\AgdaSpace{}%
\AgdaInductiveConstructor{tt}\AgdaSymbol{)}\AgdaSpace{}%
\AgdaInductiveConstructor{tt}\AgdaSymbol{))))}\<%
\\
\>[0]\AgdaFunction{lemmaHoareTripleStackGeAux'Comb3-5}\AgdaSpace{}%
\AgdaBound{msg₁}\AgdaSpace{}%
\AgdaBound{pbk1}\AgdaSpace{}%
\AgdaBound{pbk2}\AgdaSpace{}%
\AgdaBound{pbk3}\AgdaSpace{}%
\AgdaBound{pbk4}\AgdaSpace{}%
\AgdaBound{pbk5}\AgdaSpace{}%
\AgdaBound{sig1}\AgdaSpace{}%
\AgdaBound{sig2}\AgdaSpace{}%
\AgdaBound{sig3}\AgdaSpace{}%
\AgdaBound{x}\AgdaSpace{}%
\AgdaSymbol{|}\AgdaSpace{}%
\AgdaInductiveConstructor{true}\AgdaSpace{}%
\AgdaSymbol{|}\AgdaSpace{}%
\AgdaInductiveConstructor{true}\AgdaSpace{}%
\AgdaKeyword{with}%
\>[102]\AgdaSymbol{(}\AgdaFunction{isSigned}%
\>[113]\AgdaBound{msg₁}\AgdaSpace{}%
\AgdaBound{sig3}\AgdaSpace{}%
\AgdaBound{pbk3}\AgdaSymbol{)}\<%
\\
\>[0]\AgdaFunction{lemmaHoareTripleStackGeAux'Comb3-5}\AgdaSpace{}%
\AgdaBound{msg₁}\AgdaSpace{}%
\AgdaBound{pbk1}\AgdaSpace{}%
\AgdaBound{pbk2}\AgdaSpace{}%
\AgdaBound{pbk3}\AgdaSpace{}%
\AgdaBound{pbk4}\AgdaSpace{}%
\AgdaBound{pbk5}\AgdaSpace{}%
\AgdaBound{sig1}\AgdaSpace{}%
\AgdaBound{sig2}\AgdaSpace{}%
\AgdaBound{sig3}\AgdaSpace{}%
\AgdaBound{x}\AgdaSpace{}%
\AgdaSymbol{|}\AgdaSpace{}%
\AgdaInductiveConstructor{true}\AgdaSpace{}%
\AgdaSymbol{|}\AgdaSpace{}%
\AgdaInductiveConstructor{true}\AgdaSpace{}%
\AgdaSymbol{|}\AgdaSpace{}%
\AgdaInductiveConstructor{false}\AgdaSpace{}%
\AgdaKeyword{with}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaFunction{isSigned}%
\>[120]\AgdaBound{msg₁}\AgdaSpace{}%
\AgdaBound{sig3}\AgdaSpace{}%
\AgdaBound{pbk4}\AgdaSymbol{)}\<%
\\
\>[0]\AgdaFunction{lemmaHoareTripleStackGeAux'Comb3-5}\AgdaSpace{}%
\AgdaBound{msg₁}\AgdaSpace{}%
\AgdaBound{pbk1}\AgdaSpace{}%
\AgdaBound{pbk2}\AgdaSpace{}%
\AgdaBound{pbk3}\AgdaSpace{}%
\AgdaBound{pbk4}\AgdaSpace{}%
\AgdaBound{pbk5}\AgdaSpace{}%
\AgdaBound{sig1}\AgdaSpace{}%
\AgdaBound{sig2}\AgdaSpace{}%
\AgdaBound{sig3}\AgdaSpace{}%
\AgdaBound{x}\AgdaSpace{}%
\AgdaSymbol{|}\AgdaSpace{}%
\AgdaInductiveConstructor{true}\AgdaSpace{}%
\AgdaSymbol{|}\AgdaSpace{}%
\AgdaInductiveConstructor{true}\AgdaSpace{}%
\AgdaSymbol{|}\AgdaSpace{}%
\AgdaInductiveConstructor{false}\AgdaSpace{}%
\AgdaSymbol{|}\AgdaSpace{}%
\AgdaInductiveConstructor{false}\AgdaSpace{}%
\AgdaKeyword{with}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaFunction{isSigned}%
\>[128]\AgdaBound{msg₁}\AgdaSpace{}%
\AgdaBound{sig3}\AgdaSpace{}%
\AgdaBound{pbk5}\AgdaSymbol{)}\<%
\\
\>[0]\AgdaFunction{lemmaHoareTripleStackGeAux'Comb3-5}\AgdaSpace{}%
\AgdaBound{msg₁}\AgdaSpace{}%
\AgdaBound{pbk1}\AgdaSpace{}%
\AgdaBound{pbk2}\AgdaSpace{}%
\AgdaBound{pbk3}%
\>[7569I]\AgdaBound{pbk4}\AgdaSpace{}%
\AgdaBound{pbk5}\AgdaSpace{}%
\AgdaBound{sig1}\AgdaSpace{}%
\AgdaBound{sig2}\AgdaSpace{}%
\AgdaBound{sig3}\AgdaSpace{}%
\AgdaBound{x}\AgdaSpace{}%
\AgdaSymbol{|}\AgdaSpace{}%
\AgdaInductiveConstructor{true}\AgdaSpace{}%
\AgdaSymbol{|}\AgdaSpace{}%
\AgdaInductiveConstructor{true}\AgdaSpace{}%
\AgdaSymbol{|}\AgdaSpace{}%
\AgdaInductiveConstructor{false}\AgdaSpace{}%
\AgdaSymbol{|}\AgdaSpace{}%
\AgdaInductiveConstructor{false}\AgdaSpace{}%
\AgdaSymbol{|}\AgdaSpace{}%
\AgdaInductiveConstructor{true}\<%
\\
\>[7569I][@{}l@{\AgdaIndent{0}}]%
\>[56]\AgdaSymbol{=}\AgdaSpace{}%
\AgdaInductiveConstructor{inj₂}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaInductiveConstructor{inj₂}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaInductiveConstructor{inj₁}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaInductiveConstructor{conj}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaInductiveConstructor{conj}\AgdaSpace{}%
\AgdaInductiveConstructor{tt}\AgdaSpace{}%
\AgdaInductiveConstructor{tt}\AgdaSymbol{)}\AgdaSpace{}%
\AgdaInductiveConstructor{tt}\AgdaSymbol{)))}\<%
\\
\>[0]\AgdaFunction{lemmaHoareTripleStackGeAux'Comb3-5}\AgdaSpace{}%
\AgdaBound{msg₁}\AgdaSpace{}%
\AgdaBound{pbk1}\AgdaSpace{}%
\AgdaBound{pbk2}\AgdaSpace{}%
\AgdaBound{pbk3}\AgdaSpace{}%
\AgdaBound{pbk4}\AgdaSpace{}%
\AgdaBound{pbk5}\AgdaSpace{}%
\AgdaBound{sig1}\AgdaSpace{}%
\AgdaBound{sig2}\AgdaSpace{}%
\AgdaBound{sig3}\AgdaSpace{}%
\AgdaBound{x}\AgdaSpace{}%
\AgdaSymbol{|}\AgdaSpace{}%
\AgdaInductiveConstructor{true}\AgdaSpace{}%
\AgdaSymbol{|}\AgdaSpace{}%
\AgdaInductiveConstructor{true}\AgdaSpace{}%
\AgdaSymbol{|}\AgdaSpace{}%
\AgdaInductiveConstructor{false}\AgdaSpace{}%
\AgdaSymbol{|}\AgdaSpace{}%
\AgdaInductiveConstructor{true}\AgdaSpace{}%
\AgdaSymbol{=}\AgdaSpace{}%
\AgdaInductiveConstructor{inj₂}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaInductiveConstructor{inj₁}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaInductiveConstructor{conj}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaInductiveConstructor{conj}\AgdaSpace{}%
\AgdaInductiveConstructor{tt}\AgdaSpace{}%
\AgdaInductiveConstructor{tt}\AgdaSymbol{)}\AgdaSpace{}%
\AgdaInductiveConstructor{tt}\AgdaSymbol{))}\<%
\\
\>[0]\AgdaFunction{lemmaHoareTripleStackGeAux'Comb3-5}\AgdaSpace{}%
\AgdaBound{msg₁}\AgdaSpace{}%
\AgdaBound{pbk1}\AgdaSpace{}%
\AgdaBound{pbk2}\AgdaSpace{}%
\AgdaBound{pbk3}\AgdaSpace{}%
\AgdaBound{pbk4}\AgdaSpace{}%
\AgdaBound{pbk5}\AgdaSpace{}%
\AgdaBound{sig1}\AgdaSpace{}%
\AgdaBound{sig2}\AgdaSpace{}%
\AgdaBound{sig3}\AgdaSpace{}%
\AgdaBound{x}\AgdaSpace{}%
\AgdaSymbol{|}\AgdaSpace{}%
\AgdaInductiveConstructor{true}\AgdaSpace{}%
\AgdaSymbol{|}\AgdaSpace{}%
\AgdaInductiveConstructor{true}\AgdaSpace{}%
\AgdaSymbol{|}\AgdaSpace{}%
\AgdaInductiveConstructor{true}\AgdaSpace{}%
\AgdaSymbol{=}\AgdaSpace{}%
\AgdaInductiveConstructor{inj₁}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaInductiveConstructor{conj}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaInductiveConstructor{conj}\AgdaSpace{}%
\AgdaInductiveConstructor{tt}\AgdaSpace{}%
\AgdaInductiveConstructor{tt}\AgdaSymbol{)}\AgdaSpace{}%
\AgdaInductiveConstructor{tt}\AgdaSymbol{)}\<%
\\
\>[0]\<%
\end{code}
} % END AgdaHide

\newcommand{\multisigoppushlistofpublickey}{
\begin{code}%
\>[0]\AgdaFunction{opPushList}\AgdaSpace{}%
\AgdaSymbol{:}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaBound{pbkList}\AgdaSpace{}%
\AgdaSymbol{:}\AgdaSpace{}%
\AgdaDatatype{List}\AgdaSpace{}%
\AgdaDatatype{ℕ}\AgdaSymbol{)}\AgdaSpace{}%
\AgdaSymbol{→}\AgdaSpace{}%
\AgdaFunction{BitcoinScriptBasic}\<%
\\
\>[0]\AgdaFunction{opPushList}\AgdaSpace{}%
\AgdaInductiveConstructor{[]}\AgdaSpace{}%
\AgdaSymbol{=}\AgdaSpace{}%
\AgdaInductiveConstructor{[]}\<%
\\
\>[0]\AgdaFunction{opPushList}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaBound{pbk₁}\AgdaSpace{}%
\AgdaOperator{\AgdaInductiveConstructor{∷}}\AgdaSpace{}%
\AgdaBound{pbkList}\AgdaSymbol{)}\AgdaSpace{}%
\AgdaSymbol{=}\AgdaSpace{}%
\AgdaInductiveConstructor{opPush}\AgdaSpace{}%
\AgdaBound{pbk₁}\AgdaSpace{}%
\AgdaOperator{\AgdaInductiveConstructor{∷}}\AgdaSpace{}%
\AgdaFunction{opPushList}\AgdaSpace{}%
\AgdaBound{pbkList}\<%
\end{code}
} % END newcommand

\AgdaHide{
\begin{code}%
\>[0]\<%
\\
\>[0]\AgdaComment{--\ The\ multisig\ script\ m\ out\ of\ (length\ pbkList)}\<%
\\
\>[0]\AgdaComment{--\ where\ pbkList\ is\ a\ list\ of\ public\ keys.}\<%
\\
\>[0]\<%
\end{code}
} % END AgdaHide

\newcommand{\multisigmultiSigscriptmoutoflengthpbkList}{
\begin{code}%
\>[0]\AgdaFunction{multiSigScriptm-nᵇ}%
\>[7661I]\AgdaSymbol{:}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaBound{m}\AgdaSpace{}%
\AgdaSymbol{:}\AgdaSpace{}%
\AgdaDatatype{ℕ}\AgdaSymbol{)(}\AgdaBound{pbkList}\AgdaSpace{}%
\AgdaSymbol{:}\AgdaSpace{}%
\AgdaDatatype{List}\AgdaSpace{}%
\AgdaDatatype{ℕ}\AgdaSymbol{)(}\AgdaBound{m<n}\AgdaSpace{}%
\AgdaSymbol{:}\AgdaSpace{}%
\AgdaBound{m}\AgdaSpace{}%
\AgdaOperator{\AgdaFunction{<}}\AgdaSpace{}%
\AgdaFunction{length}\AgdaSpace{}%
\AgdaBound{pbkList}\AgdaSymbol{)}\<%
\\
\>[7661I][@{}l@{\AgdaIndent{0}}]%
\>[20]\AgdaSymbol{→}\AgdaSpace{}%
\AgdaFunction{BitcoinScriptBasic}\<%
\\
\>[0]\AgdaFunction{multiSigScriptm-nᵇ}\AgdaSpace{}%
\AgdaBound{m}\AgdaSpace{}%
\AgdaBound{pbkList}\AgdaSpace{}%
\AgdaBound{m<n}\AgdaSpace{}%
\AgdaSymbol{=}\<%
\\
\>[0][@{}l@{\AgdaIndent{0}}]%
\>[3]\AgdaInductiveConstructor{opPush}\AgdaSpace{}%
\AgdaBound{m}%
\>[13]\AgdaOperator{\AgdaInductiveConstructor{∷}}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaFunction{opPushList}\AgdaSpace{}%
\AgdaBound{pbkList}\AgdaSpace{}%
\AgdaOperator{\AgdaFunction{++}}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaInductiveConstructor{opPush}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaFunction{length}\AgdaSpace{}%
\AgdaBound{pbkList}\AgdaSymbol{)}\AgdaSpace{}%
\AgdaOperator{\AgdaInductiveConstructor{∷}}\AgdaSpace{}%
\AgdaOperator{\AgdaFunction{[}}%
\>[68]\AgdaInductiveConstructor{opMultiSig}\AgdaSpace{}%
\AgdaOperator{\AgdaFunction{]}}\AgdaSymbol{))}\<%
\end{code}
} % END newcommand

\AgdaHide{
\begin{code}%
\>[0]\<%
\\
%
\\[\AgdaEmptyExtraSkip]%
\>[0]\<%
\end{code}
} % END AgdaHide

\newcommand{\multisigcomplexmultisig}{
\begin{code}%
\>[0]\AgdaFunction{multiSigScript2-4ᵇ}\AgdaSpace{}%
\AgdaSymbol{:}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaBound{pbk₁}\AgdaSpace{}%
\AgdaBound{pbk₂}\AgdaSpace{}%
\AgdaBound{pbk₃}\AgdaSpace{}%
\AgdaBound{pbk₄}\AgdaSpace{}%
\AgdaSymbol{:}%
\>[45]\AgdaDatatype{ℕ}\AgdaSymbol{)}\AgdaSpace{}%
\AgdaSymbol{→}\AgdaSpace{}%
\AgdaFunction{BitcoinScriptBasic}\<%
\\
\>[0]\AgdaFunction{multiSigScript2-4ᵇ}\AgdaSpace{}%
\AgdaBound{pbk₁}\AgdaSpace{}%
\AgdaBound{pbk₂}\AgdaSpace{}%
\AgdaBound{pbk₃}\AgdaSpace{}%
\AgdaBound{pbk₄}\AgdaSpace{}%
\AgdaSymbol{=}\<%
\\
\>[0][@{}l@{\AgdaIndent{0}}]%
\>[3]\AgdaFunction{multiSigScriptm-nᵇ}\AgdaSpace{}%
\AgdaNumber{2}%
\>[25]\AgdaSymbol{(}\AgdaBound{pbk₁}\AgdaSpace{}%
\AgdaOperator{\AgdaInductiveConstructor{∷}}\AgdaSpace{}%
\AgdaBound{pbk₂}\AgdaSpace{}%
\AgdaOperator{\AgdaInductiveConstructor{∷}}\AgdaSpace{}%
\AgdaBound{pbk₃}\AgdaSpace{}%
\AgdaOperator{\AgdaInductiveConstructor{∷}}\AgdaSpace{}%
\AgdaOperator{\AgdaFunction{[}}\AgdaSpace{}%
\AgdaBound{pbk₄}\AgdaSpace{}%
\AgdaOperator{\AgdaFunction{]}}\AgdaSymbol{)}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaInductiveConstructor{s≤s}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaInductiveConstructor{s≤s}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaInductiveConstructor{s≤s}\AgdaSpace{}%
\AgdaInductiveConstructor{z≤n}\AgdaSymbol{)))}\<%
\end{code}
} % END newcommand

\AgdaHide{
\begin{code}%
\>[0]\<%
\\
\>[0]\AgdaComment{\{-}\<%
\\
\>[0]\AgdaComment{-@BEGIN@complexmultisig}\<%
\\
\>[0]\AgdaComment{multiSigScript2-4ᵇ\ :\ (pbk₁\ pbk₂\ pbk₃\ pbk₄\ :\ \ ℕ)\ →\ BitcoinScriptBasic}\<%
\\
\>[0]\AgdaComment{multiSigScript2-4ᵇ\ \ pbk₁\ pbk₂\ pbk₃\ pbk₄\ =\ \ (opPush\ 2)\ ∷\ (opPush\ pbk₁)\ ∷\ \ (opPush\ pbk₂)\ ∷}\<%
\\
\>[0]\AgdaComment{\ \ \ \ \ \ \ \ \ \ \ \ \ \ \ \ \ \ \ \ (opPush\ pbk₃)\ ∷\ \ (opPush\ pbk₄)\ ∷\ (opPush\ 4)\ ∷\ \ [\ \ opMultiSig\ ]}\<%
\\
\>[0]\AgdaComment{-@END}\<%
\\
\>[0]\AgdaComment{-\}}\<%
\\
%
\\[\AgdaEmptyExtraSkip]%
\>[0]\AgdaFunction{multiSigScript-3-5-b}\AgdaSpace{}%
\AgdaSymbol{:}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaBound{pbk1}\AgdaSpace{}%
\AgdaBound{pbk2}\AgdaSpace{}%
\AgdaBound{pbk3}\AgdaSpace{}%
\AgdaBound{pbk4}\AgdaSpace{}%
\AgdaBound{pbk5}\AgdaSpace{}%
\AgdaSymbol{:}%
\>[52]\AgdaDatatype{ℕ}\AgdaSymbol{)}\AgdaSpace{}%
\AgdaSymbol{→}\AgdaSpace{}%
\AgdaFunction{BitcoinScriptBasic}\<%
\\
\>[0]\AgdaFunction{multiSigScript-3-5-b}\AgdaSpace{}%
\AgdaBound{pbk1}\AgdaSpace{}%
\AgdaBound{pbk2}\AgdaSpace{}%
\AgdaBound{pbk3}\AgdaSpace{}%
\AgdaBound{pbk4}\AgdaSpace{}%
\AgdaBound{pbk5}\AgdaSpace{}%
\AgdaSymbol{=}\<%
\\
\>[0][@{}l@{\AgdaIndent{0}}]%
\>[6]\AgdaSymbol{(}\AgdaInductiveConstructor{opPush}\AgdaSpace{}%
\AgdaNumber{3}\AgdaSymbol{)}\AgdaSpace{}%
\AgdaOperator{\AgdaInductiveConstructor{∷}}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaInductiveConstructor{opPush}\AgdaSpace{}%
\AgdaBound{pbk1}\AgdaSymbol{)}\AgdaSpace{}%
\AgdaOperator{\AgdaInductiveConstructor{∷}}%
\>[36]\AgdaSymbol{(}\AgdaInductiveConstructor{opPush}\AgdaSpace{}%
\AgdaBound{pbk2}\AgdaSymbol{)}\AgdaSpace{}%
\AgdaOperator{\AgdaInductiveConstructor{∷}}%
\>[53]\AgdaSymbol{(}\AgdaInductiveConstructor{opPush}\AgdaSpace{}%
\AgdaBound{pbk3}\AgdaSymbol{)}\AgdaSpace{}%
\AgdaOperator{\AgdaInductiveConstructor{∷}}%
\>[70]\AgdaSymbol{(}\AgdaInductiveConstructor{opPush}\AgdaSpace{}%
\AgdaBound{pbk4}\AgdaSymbol{)}\AgdaSpace{}%
\AgdaOperator{\AgdaInductiveConstructor{∷}}%
\>[87]\AgdaSymbol{(}\AgdaInductiveConstructor{opPush}\AgdaSpace{}%
\AgdaBound{pbk5}\AgdaSymbol{)}\AgdaSpace{}%
\AgdaOperator{\AgdaInductiveConstructor{∷}}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaInductiveConstructor{opPush}\AgdaSpace{}%
\AgdaNumber{5}\AgdaSymbol{)}\AgdaSpace{}%
\AgdaOperator{\AgdaInductiveConstructor{∷}}\AgdaSpace{}%
\AgdaInductiveConstructor{opMultiSig}\AgdaSpace{}%
\AgdaOperator{\AgdaInductiveConstructor{∷}}\AgdaSpace{}%
\AgdaInductiveConstructor{[]}\<%
\\
%
\\[\AgdaEmptyExtraSkip]%
\>[0]\AgdaComment{--\textbackslash{}multisigcheckTimeScript}\<%
\end{code}
} % END AgdaHide

\newcommand{\multisigcheckTimeScript}{
\begin{code}%
\>[0]\AgdaFunction{checkTimeScriptᵇ}\AgdaSpace{}%
\AgdaSymbol{:}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaBound{time₁}\AgdaSpace{}%
\AgdaSymbol{:}\AgdaSpace{}%
\AgdaFunction{Time}\AgdaSymbol{)}\AgdaSpace{}%
\AgdaSymbol{→}\AgdaSpace{}%
\AgdaFunction{BitcoinScriptBasic}\<%
\\
\>[0]\AgdaFunction{checkTimeScriptᵇ}\AgdaSpace{}%
\AgdaBound{time₁}\AgdaSpace{}%
\AgdaSymbol{=}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaInductiveConstructor{opPush}\AgdaSpace{}%
\AgdaBound{time₁}\AgdaSymbol{)}\AgdaSpace{}%
\AgdaOperator{\AgdaInductiveConstructor{∷}}\AgdaSpace{}%
\AgdaInductiveConstructor{opCHECKLOCKTIMEVERIFY}\AgdaSpace{}%
\AgdaOperator{\AgdaInductiveConstructor{∷}}\AgdaSpace{}%
\AgdaOperator{\AgdaFunction{[}}\AgdaSpace{}%
\AgdaInductiveConstructor{opDrop}%
\>[76]\AgdaOperator{\AgdaFunction{]}}\<%
\end{code}
} % END newcommand

\AgdaHide{
\begin{code}%
\>[0]\<%
\\
%
\\[\AgdaEmptyExtraSkip]%
%
\\[\AgdaEmptyExtraSkip]%
%
\\[\AgdaEmptyExtraSkip]%
%
\\[\AgdaEmptyExtraSkip]%
%
\\[\AgdaEmptyExtraSkip]%
%
\\[\AgdaEmptyExtraSkip]%
\>[0]\AgdaComment{\{-\ Next\ steps\ -\}}\<%
\\
%
\\[\AgdaEmptyExtraSkip]%
%
\\[\AgdaEmptyExtraSkip]%
%
\\[\AgdaEmptyExtraSkip]%
\>[0]\AgdaComment{--new}\<%
\\
%
\\[\AgdaEmptyExtraSkip]%
\>[0]\AgdaFunction{lemmaHoareTripleStackGeAux'5}%
\>[7763I]\AgdaSymbol{:}%
\>[7764I]\AgdaSymbol{(}\AgdaBound{msg}\AgdaSpace{}%
\AgdaSymbol{:}\AgdaSpace{}%
\AgdaDatatype{Msg}\AgdaSymbol{)}\<%
\\
\>[.][@{}l@{}]\<[7764I]%
\>[31]\AgdaSymbol{(}\AgdaBound{pbk1}\AgdaSpace{}%
\AgdaBound{pbk2}\AgdaSpace{}%
\AgdaBound{pbk3}\AgdaSpace{}%
\AgdaBound{sig1}\AgdaSpace{}%
\AgdaBound{sig3}\AgdaSpace{}%
\AgdaSymbol{:}\AgdaSpace{}%
\AgdaDatatype{ℕ}\AgdaSymbol{)}\<%
\\
%
\>[31]\AgdaSymbol{→}\AgdaSpace{}%
\AgdaFunction{True}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaFunction{isSigned}%
\>[49]\AgdaBound{msg}\AgdaSpace{}%
\AgdaBound{sig1}\AgdaSpace{}%
\AgdaBound{pbk1}\AgdaSymbol{)}\<%
\\
\>[7763I][@{}l@{\AgdaIndent{0}}]%
\>[30]\AgdaSymbol{→}%
\>[33]\AgdaFunction{True}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaFunction{isSigned}%
\>[49]\AgdaBound{msg}\AgdaSpace{}%
\AgdaBound{sig3}\AgdaSpace{}%
\AgdaBound{pbk3}\AgdaSymbol{)}\<%
\\
\>[30][@{}l@{\AgdaIndent{0}}]%
\>[31]\AgdaSymbol{→}\AgdaSpace{}%
\AgdaFunction{True}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaFunction{compareSigsMultiSig}\AgdaSpace{}%
\AgdaBound{msg}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaSpace{}%
\AgdaBound{sig1}\AgdaSpace{}%
\AgdaOperator{\AgdaInductiveConstructor{∷}}\AgdaSpace{}%
\AgdaBound{sig3}\AgdaSpace{}%
\AgdaOperator{\AgdaInductiveConstructor{∷}}\AgdaSpace{}%
\AgdaInductiveConstructor{[]}\AgdaSymbol{)}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaBound{pbk1}\AgdaSpace{}%
\AgdaOperator{\AgdaInductiveConstructor{∷}}\AgdaSpace{}%
\AgdaBound{pbk2}\AgdaSpace{}%
\AgdaOperator{\AgdaInductiveConstructor{∷}}\AgdaSpace{}%
\AgdaBound{pbk3}\AgdaSpace{}%
\AgdaOperator{\AgdaInductiveConstructor{∷}}\AgdaSpace{}%
\AgdaInductiveConstructor{[]}\AgdaSymbol{))}\<%
\\
\>[0]\AgdaFunction{lemmaHoareTripleStackGeAux'5}\AgdaSpace{}%
\AgdaBound{msg}\AgdaSpace{}%
\AgdaBound{pbk1}\AgdaSpace{}%
\AgdaBound{pbk2}\AgdaSpace{}%
\AgdaBound{pbk3}\AgdaSpace{}%
\AgdaBound{sig1}\AgdaSpace{}%
\AgdaBound{sig3}\AgdaSpace{}%
\AgdaBound{x}\AgdaSpace{}%
\AgdaBound{x₁}%
\>[64]\AgdaKeyword{with}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaFunction{isSigned}%
\>[80]\AgdaBound{msg}\AgdaSpace{}%
\AgdaBound{sig1}\AgdaSpace{}%
\AgdaBound{pbk1}\AgdaSymbol{)}\<%
\\
\>[0]\AgdaFunction{lemmaHoareTripleStackGeAux'5}\AgdaSpace{}%
\AgdaBound{msg}\AgdaSpace{}%
\AgdaBound{pbk1}\AgdaSpace{}%
\AgdaBound{pbk2}\AgdaSpace{}%
\AgdaBound{pbk3}\AgdaSpace{}%
\AgdaBound{sig1}\AgdaSpace{}%
\AgdaBound{sig3}\AgdaSpace{}%
\AgdaBound{x}\AgdaSpace{}%
\AgdaBound{x₁}\AgdaSpace{}%
\AgdaSymbol{|}\AgdaSpace{}%
\AgdaInductiveConstructor{true}\AgdaSpace{}%
\AgdaKeyword{with}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaFunction{isSigned}%
\>[86]\AgdaBound{msg}\AgdaSpace{}%
\AgdaBound{sig3}\AgdaSpace{}%
\AgdaBound{pbk2}\AgdaSymbol{)}\<%
\\
\>[0]\AgdaFunction{lemmaHoareTripleStackGeAux'5}\AgdaSpace{}%
\AgdaBound{msg}\AgdaSpace{}%
\AgdaBound{pbk1}\AgdaSpace{}%
\AgdaBound{pbk2}\AgdaSpace{}%
\AgdaBound{pbk3}\AgdaSpace{}%
\AgdaBound{sig1}\AgdaSpace{}%
\AgdaBound{sig3}\AgdaSpace{}%
\AgdaBound{x}\AgdaSpace{}%
\AgdaBound{x₁}\AgdaSpace{}%
\AgdaSymbol{|}\AgdaSpace{}%
\AgdaInductiveConstructor{true}\AgdaSpace{}%
\AgdaSymbol{|}\AgdaSpace{}%
\AgdaInductiveConstructor{false}\AgdaSpace{}%
\AgdaKeyword{with}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaFunction{isSigned}%
\>[94]\AgdaBound{msg}\AgdaSpace{}%
\AgdaBound{sig3}\AgdaSpace{}%
\AgdaBound{pbk3}\AgdaSymbol{)}\<%
\\
\>[0]\AgdaFunction{lemmaHoareTripleStackGeAux'5}\AgdaSpace{}%
\AgdaBound{msg}\AgdaSpace{}%
\AgdaBound{pbk1}\AgdaSpace{}%
\AgdaBound{pbk2}\AgdaSpace{}%
\AgdaBound{pbk3}\AgdaSpace{}%
\AgdaBound{sig1}\AgdaSpace{}%
\AgdaBound{sig3}\AgdaSpace{}%
\AgdaBound{x}\AgdaSpace{}%
\AgdaBound{x₁}\AgdaSpace{}%
\AgdaSymbol{|}\AgdaSpace{}%
\AgdaInductiveConstructor{true}\AgdaSpace{}%
\AgdaSymbol{|}\AgdaSpace{}%
\AgdaInductiveConstructor{false}\AgdaSpace{}%
\AgdaSymbol{|}\AgdaSpace{}%
\AgdaInductiveConstructor{true}\AgdaSpace{}%
\AgdaSymbol{=}\AgdaSpace{}%
\AgdaInductiveConstructor{tt}\<%
\\
\>[0]\AgdaFunction{lemmaHoareTripleStackGeAux'5}\AgdaSpace{}%
\AgdaBound{msg}\AgdaSpace{}%
\AgdaBound{pbk1}\AgdaSpace{}%
\AgdaBound{pbk2}\AgdaSpace{}%
\AgdaBound{pbk3}\AgdaSpace{}%
\AgdaBound{sig1}\AgdaSpace{}%
\AgdaBound{sig3}\AgdaSpace{}%
\AgdaBound{x}\AgdaSpace{}%
\AgdaBound{x₁}\AgdaSpace{}%
\AgdaSymbol{|}\AgdaSpace{}%
\AgdaInductiveConstructor{true}\AgdaSpace{}%
\AgdaSymbol{|}\AgdaSpace{}%
\AgdaInductiveConstructor{true}\AgdaSpace{}%
\AgdaSymbol{=}\AgdaSpace{}%
\AgdaInductiveConstructor{tt}\<%
\\
%
\\[\AgdaEmptyExtraSkip]%
%
\\[\AgdaEmptyExtraSkip]%
%
\\[\AgdaEmptyExtraSkip]%
%
\\[\AgdaEmptyExtraSkip]%
%
\\[\AgdaEmptyExtraSkip]%
%
\\[\AgdaEmptyExtraSkip]%
%
\\[\AgdaEmptyExtraSkip]%
\>[0]\AgdaComment{--\textbackslash{}multisigtimeCheckPreCond}\<%
\end{code}
} % END AgdaHide

\newcommand{\multisigtimeCheckPreCond}{
\begin{code}%
\>[0]\AgdaFunction{timeCheckPreCond}\AgdaSpace{}%
\AgdaSymbol{:}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaBound{time₁}\AgdaSpace{}%
\AgdaSymbol{:}\AgdaSpace{}%
\AgdaFunction{Time}\AgdaSymbol{)}\AgdaSpace{}%
\AgdaSymbol{→}\AgdaSpace{}%
\AgdaFunction{StackPredicate}\<%
\\
\>[0]\AgdaFunction{timeCheckPreCond}\AgdaSpace{}%
\AgdaBound{time₁}\AgdaSpace{}%
\AgdaBound{time₂}\AgdaSpace{}%
\AgdaBound{msg}\AgdaSpace{}%
\AgdaBound{stack₁}\AgdaSpace{}%
\AgdaSymbol{=}\AgdaSpace{}%
\AgdaBound{time₁}\AgdaSpace{}%
\AgdaOperator{\AgdaFunction{≤}}\AgdaSpace{}%
\AgdaBound{time₂}\<%
\end{code}
} % END newcommand

\AgdaHide{
\begin{code}%
\>[0]\<%
\end{code}
} % END AgdaHide


==> latex-before-sed/verificationP2PKHbasic.tex <==
%% This file has been generated automatically by mkLagda.awk
%% DO NOT EDIT! ALL YOUR CHANGES WILL BE LOST!

\AgdaHide{
\begin{code}%
\>[0]\AgdaComment{\{-\ OPTIONS\ --allow-unsolved-metas\ \#-\}}\<%
\\
\>[0]\AgdaKeyword{open}\AgdaSpace{}%
\AgdaKeyword{import}\AgdaSpace{}%
\AgdaModule{basicBitcoinDataType}\<%
\\
%
\\[\AgdaEmptyExtraSkip]%
\>[0]\AgdaKeyword{module}\AgdaSpace{}%
\AgdaModule{verificationP2PKHbasic}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaBound{param}\AgdaSpace{}%
\AgdaSymbol{:}\AgdaSpace{}%
\AgdaRecord{GlobalParameters}\AgdaSymbol{)}\AgdaSpace{}%
\AgdaKeyword{where}\<%
\\
%
\\[\AgdaEmptyExtraSkip]%
\>[0]\AgdaKeyword{open}\AgdaSpace{}%
\AgdaKeyword{import}\AgdaSpace{}%
\AgdaModule{libraries.listLib}\<%
\\
\>[0]\AgdaKeyword{open}\AgdaSpace{}%
\AgdaKeyword{import}\AgdaSpace{}%
\AgdaModule{Data.List.Base}\<%
\\
\>[0]\AgdaKeyword{open}\AgdaSpace{}%
\AgdaKeyword{import}\AgdaSpace{}%
\AgdaModule{libraries.natLib}\<%
\\
\>[0]\AgdaKeyword{open}\AgdaSpace{}%
\AgdaKeyword{import}\AgdaSpace{}%
\AgdaModule{Data.Nat}%
\>[22]\AgdaKeyword{renaming}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaOperator{\AgdaDatatype{\AgdaUnderscore{}≤\AgdaUnderscore{}}}\AgdaSpace{}%
\AgdaSymbol{to}\AgdaSpace{}%
\AgdaOperator{\AgdaDatatype{\AgdaUnderscore{}≤'\AgdaUnderscore{}}}\AgdaSpace{}%
\AgdaSymbol{;}\AgdaSpace{}%
\AgdaOperator{\AgdaFunction{\AgdaUnderscore{}<\AgdaUnderscore{}}}\AgdaSpace{}%
\AgdaSymbol{to}\AgdaSpace{}%
\AgdaOperator{\AgdaFunction{\AgdaUnderscore{}<'\AgdaUnderscore{}}}\AgdaSymbol{)}\<%
\\
\>[0]\AgdaKeyword{open}\AgdaSpace{}%
\AgdaKeyword{import}\AgdaSpace{}%
\AgdaModule{Data.List}\AgdaSpace{}%
\AgdaKeyword{hiding}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaOperator{\AgdaFunction{\AgdaUnderscore{}++\AgdaUnderscore{}}}\AgdaSymbol{)}\<%
\\
\>[0]\AgdaKeyword{open}\AgdaSpace{}%
\AgdaKeyword{import}\AgdaSpace{}%
\AgdaModule{Data.Unit}%
\>[23]\AgdaKeyword{hiding}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaOperator{\AgdaRecord{\AgdaUnderscore{}≤\AgdaUnderscore{}}}\AgdaSymbol{)}\<%
\\
\>[0]\AgdaKeyword{open}\AgdaSpace{}%
\AgdaKeyword{import}\AgdaSpace{}%
\AgdaModule{Data.Empty}\<%
\\
\>[0]\AgdaKeyword{open}\AgdaSpace{}%
\AgdaKeyword{import}\AgdaSpace{}%
\AgdaModule{Data.Bool}%
\>[23]\AgdaKeyword{hiding}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaOperator{\AgdaDatatype{\AgdaUnderscore{}≤\AgdaUnderscore{}}}\AgdaSpace{}%
\AgdaSymbol{;}\AgdaSpace{}%
\AgdaOperator{\AgdaDatatype{\AgdaUnderscore{}<\AgdaUnderscore{}}}\AgdaSpace{}%
\AgdaSymbol{;}\AgdaSpace{}%
\AgdaOperator{\AgdaFunction{if\AgdaUnderscore{}then\AgdaUnderscore{}else\AgdaUnderscore{}}}\AgdaSpace{}%
\AgdaSymbol{)}\AgdaSpace{}%
\AgdaKeyword{renaming}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaOperator{\AgdaFunction{\AgdaUnderscore{}∧\AgdaUnderscore{}}}\AgdaSpace{}%
\AgdaSymbol{to}\AgdaSpace{}%
\AgdaOperator{\AgdaFunction{\AgdaUnderscore{}∧b\AgdaUnderscore{}}}\AgdaSpace{}%
\AgdaSymbol{;}\AgdaSpace{}%
\AgdaOperator{\AgdaFunction{\AgdaUnderscore{}∨\AgdaUnderscore{}}}\AgdaSpace{}%
\AgdaSymbol{to}\AgdaSpace{}%
\AgdaOperator{\AgdaFunction{\AgdaUnderscore{}∨b\AgdaUnderscore{}}}\AgdaSpace{}%
\AgdaSymbol{;}\AgdaSpace{}%
\AgdaFunction{T}\AgdaSpace{}%
\AgdaSymbol{to}\AgdaSpace{}%
\AgdaFunction{True}\AgdaSymbol{)}\<%
\\
\>[0]\AgdaKeyword{open}\AgdaSpace{}%
\AgdaKeyword{import}\AgdaSpace{}%
\AgdaModule{Data.Product}\AgdaSpace{}%
\AgdaKeyword{renaming}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaOperator{\AgdaInductiveConstructor{\AgdaUnderscore{},\AgdaUnderscore{}}}\AgdaSpace{}%
\AgdaSymbol{to}\AgdaSpace{}%
\AgdaOperator{\AgdaInductiveConstructor{\AgdaUnderscore{},,\AgdaUnderscore{}}}\AgdaSpace{}%
\AgdaSymbol{)}\<%
\\
\>[0]\AgdaKeyword{open}\AgdaSpace{}%
\AgdaKeyword{import}\AgdaSpace{}%
\AgdaModule{Data.Nat.Base}\AgdaSpace{}%
\AgdaKeyword{hiding}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaOperator{\AgdaDatatype{\AgdaUnderscore{}≤\AgdaUnderscore{}}}\AgdaSpace{}%
\AgdaSymbol{;}\AgdaSpace{}%
\AgdaOperator{\AgdaFunction{\AgdaUnderscore{}<\AgdaUnderscore{}}}\AgdaSymbol{)}\<%
\\
\>[0]\AgdaKeyword{open}\AgdaSpace{}%
\AgdaKeyword{import}\AgdaSpace{}%
\AgdaModule{Data.List.NonEmpty}\AgdaSpace{}%
\AgdaKeyword{hiding}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaField{head}\AgdaSpace{}%
\AgdaSymbol{)}\<%
\\
\>[0]\AgdaKeyword{open}\AgdaSpace{}%
\AgdaKeyword{import}\AgdaSpace{}%
\AgdaModule{Data.Nat}\AgdaSpace{}%
\AgdaKeyword{using}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaDatatype{ℕ}\AgdaSymbol{;}\AgdaSpace{}%
\AgdaOperator{\AgdaPrimitive{\AgdaUnderscore{}+\AgdaUnderscore{}}}\AgdaSymbol{;}\AgdaSpace{}%
\AgdaOperator{\AgdaFunction{\AgdaUnderscore{}≥\AgdaUnderscore{}}}\AgdaSymbol{;}\AgdaSpace{}%
\AgdaOperator{\AgdaFunction{\AgdaUnderscore{}>\AgdaUnderscore{}}}\AgdaSymbol{;}\AgdaSpace{}%
\AgdaInductiveConstructor{zero}\AgdaSymbol{;}\AgdaSpace{}%
\AgdaInductiveConstructor{suc}\AgdaSymbol{;}\AgdaSpace{}%
\AgdaInductiveConstructor{s≤s}\AgdaSymbol{;}\AgdaSpace{}%
\AgdaInductiveConstructor{z≤n}\AgdaSymbol{)}\<%
\\
\>[0]\AgdaKeyword{import}\AgdaSpace{}%
\AgdaModule{Relation.Binary.PropositionalEquality}\AgdaSpace{}%
\AgdaSymbol{as}\AgdaSpace{}%
\AgdaModule{Eq}\<%
\\
\>[0]\AgdaKeyword{open}\AgdaSpace{}%
\AgdaModule{Eq}\AgdaSpace{}%
\AgdaKeyword{using}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaOperator{\AgdaDatatype{\AgdaUnderscore{}≡\AgdaUnderscore{}}}\AgdaSymbol{;}\AgdaSpace{}%
\AgdaInductiveConstructor{refl}\AgdaSymbol{;}\AgdaSpace{}%
\AgdaFunction{cong}\AgdaSymbol{;}\AgdaSpace{}%
\AgdaKeyword{module}\AgdaSpace{}%
\AgdaModule{≡-Reasoning}\AgdaSymbol{;}\AgdaSpace{}%
\AgdaFunction{sym}\AgdaSymbol{)}\<%
\\
\>[0]\AgdaKeyword{open}\AgdaSpace{}%
\AgdaModule{≡-Reasoning}\<%
\\
\>[0]\AgdaKeyword{open}\AgdaSpace{}%
\AgdaKeyword{import}\AgdaSpace{}%
\AgdaModule{Agda.Builtin.Equality}\<%
\\
\>[0]\AgdaComment{--open\ import\ Agda.Builtin.Equality.Rewrite}\<%
\\
%
\\[\AgdaEmptyExtraSkip]%
\>[0]\AgdaKeyword{open}\AgdaSpace{}%
\AgdaKeyword{import}\AgdaSpace{}%
\AgdaModule{libraries.andLib}\<%
\\
\>[0]\AgdaKeyword{open}\AgdaSpace{}%
\AgdaKeyword{import}\AgdaSpace{}%
\AgdaModule{libraries.miscLib}\<%
\\
\>[0]\AgdaKeyword{open}\AgdaSpace{}%
\AgdaKeyword{import}\AgdaSpace{}%
\AgdaModule{libraries.maybeLib}\<%
\\
\>[0]\AgdaKeyword{open}\AgdaSpace{}%
\AgdaKeyword{import}\AgdaSpace{}%
\AgdaModule{libraries.boolLib}\<%
\\
%
\\[\AgdaEmptyExtraSkip]%
\>[0]\AgdaKeyword{open}\AgdaSpace{}%
\AgdaKeyword{import}\AgdaSpace{}%
\AgdaModule{stack}\<%
\\
\>[0]\AgdaKeyword{open}\AgdaSpace{}%
\AgdaKeyword{import}\AgdaSpace{}%
\AgdaModule{stackPredicate}\<%
\\
\>[0]\AgdaKeyword{open}\AgdaSpace{}%
\AgdaKeyword{import}\AgdaSpace{}%
\AgdaModule{instruction}\<%
\\
\>[0]\AgdaKeyword{open}\AgdaSpace{}%
\AgdaKeyword{import}\AgdaSpace{}%
\AgdaModule{instructionBasic}\<%
\\
\>[0]\AgdaComment{--\ open\ import\ ledger\ param}\<%
\\
\>[0]\AgdaKeyword{open}\AgdaSpace{}%
\AgdaKeyword{import}\AgdaSpace{}%
\AgdaModule{semanticBasicOperations}\AgdaSpace{}%
\AgdaBound{param}\<%
\\
%
\\[\AgdaEmptyExtraSkip]%
%
\\[\AgdaEmptyExtraSkip]%
\>[0]\AgdaFunction{instruction-1}\AgdaSpace{}%
\AgdaSymbol{:}\AgdaSpace{}%
\AgdaDatatype{InstructionBasic}\<%
\\
\>[0]\AgdaFunction{instruction-1}\AgdaSpace{}%
\AgdaSymbol{=}\AgdaSpace{}%
\AgdaInductiveConstructor{opCheckSig}\<%
\\
%
\\[\AgdaEmptyExtraSkip]%
\>[0]\AgdaFunction{instruction-2}\AgdaSpace{}%
\AgdaSymbol{:}\AgdaSpace{}%
\AgdaDatatype{InstructionBasic}\<%
\\
\>[0]\AgdaFunction{instruction-2}\AgdaSpace{}%
\AgdaSymbol{=}\AgdaSpace{}%
\AgdaInductiveConstructor{opVerify}\<%
\\
%
\\[\AgdaEmptyExtraSkip]%
\>[0]\AgdaFunction{instruction-3}\AgdaSpace{}%
\AgdaSymbol{:}\AgdaSpace{}%
\AgdaDatatype{InstructionBasic}\<%
\\
\>[0]\AgdaFunction{instruction-3}\AgdaSpace{}%
\AgdaSymbol{=}\AgdaSpace{}%
\AgdaInductiveConstructor{opEqual}\<%
\\
%
\\[\AgdaEmptyExtraSkip]%
\>[0]\AgdaFunction{instruction-4}\AgdaSpace{}%
\AgdaSymbol{:}\AgdaSpace{}%
\AgdaDatatype{ℕ}\AgdaSpace{}%
\AgdaSymbol{→}%
\>[21]\AgdaDatatype{InstructionBasic}\<%
\\
\>[0]\AgdaFunction{instruction-4}\AgdaSpace{}%
\AgdaBound{pbkh}\AgdaSpace{}%
\AgdaSymbol{=}\AgdaSpace{}%
\AgdaInductiveConstructor{opPush}%
\>[29]\AgdaBound{pbkh}\<%
\\
%
\\[\AgdaEmptyExtraSkip]%
\>[0]\AgdaFunction{instruction-5}\AgdaSpace{}%
\AgdaSymbol{:}\AgdaSpace{}%
\AgdaDatatype{InstructionBasic}\<%
\\
\>[0]\AgdaFunction{instruction-5}\AgdaSpace{}%
\AgdaSymbol{=}\AgdaSpace{}%
\AgdaInductiveConstructor{opHash}\<%
\\
%
\\[\AgdaEmptyExtraSkip]%
\>[0]\AgdaFunction{instruction-6}\AgdaSpace{}%
\AgdaSymbol{:}\AgdaSpace{}%
\AgdaDatatype{InstructionBasic}\<%
\\
\>[0]\AgdaFunction{instruction-6}\AgdaSpace{}%
\AgdaSymbol{=}\AgdaSpace{}%
\AgdaInductiveConstructor{opDup}\<%
\\
%
\\[\AgdaEmptyExtraSkip]%
\>[0]\AgdaFunction{accept-0Basic}\AgdaSpace{}%
\AgdaSymbol{:}\AgdaSpace{}%
\AgdaFunction{StackPredicate}\<%
\\
\>[0]\AgdaFunction{accept-0Basic}\AgdaSpace{}%
\AgdaSymbol{=}\AgdaSpace{}%
\AgdaFunction{acceptStateˢ}\<%
\\
\>[0]\<%
\end{code}
} % END AgdaHide

\newcommand{\verificationptopbasicposcontitionone}{
\begin{code}[inline]%
\>[0]\AgdaFunction{accept₁ˢ}\AgdaSpace{}%
\AgdaSymbol{:}\AgdaSpace{}%
\AgdaFunction{StackPredicate}\<%
\\
\>[0]\AgdaFunction{accept₁ˢ}\AgdaSpace{}%
\AgdaBound{time}\AgdaSpace{}%
\AgdaBound{m}\AgdaSpace{}%
\AgdaInductiveConstructor{[]}\AgdaSpace{}%
\AgdaSymbol{=}\AgdaSpace{}%
\AgdaDatatype{⊥}\<%
\\
\>[0]\AgdaFunction{accept₁ˢ}\AgdaSpace{}%
\AgdaBound{time}\AgdaSpace{}%
\AgdaBound{m}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaBound{sig}\AgdaSpace{}%
\AgdaOperator{\AgdaInductiveConstructor{∷}}\AgdaSpace{}%
\AgdaInductiveConstructor{[]}\AgdaSymbol{)}\AgdaSpace{}%
\AgdaSymbol{=}\AgdaSpace{}%
\AgdaDatatype{⊥}\<%
\\
\>[0]\AgdaFunction{accept₁ˢ}\AgdaSpace{}%
\AgdaBound{time}\AgdaSpace{}%
\AgdaBound{m}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaSpace{}%
\AgdaBound{pbk}%
\>[23]\AgdaOperator{\AgdaInductiveConstructor{∷}}\AgdaSpace{}%
\AgdaBound{sig}\AgdaSpace{}%
\AgdaOperator{\AgdaInductiveConstructor{∷}}\AgdaSpace{}%
\AgdaBound{st}\AgdaSymbol{)}\AgdaSpace{}%
\AgdaSymbol{=}\AgdaSpace{}%
\AgdaFunction{IsSigned}\AgdaSpace{}%
\AgdaBound{m}%
\>[49]\AgdaBound{sig}\AgdaSpace{}%
\AgdaBound{pbk}\<%
\end{code}
} % END newcommand

\AgdaHide{
\begin{code}%
\>[0]\AgdaFunction{accept₂ˢCore}\AgdaSpace{}%
\AgdaSymbol{:}\AgdaSpace{}%
\AgdaFunction{Time}\AgdaSpace{}%
\AgdaSymbol{→}\AgdaSpace{}%
\AgdaDatatype{Msg}\AgdaSpace{}%
\AgdaSymbol{→}\AgdaSpace{}%
\AgdaDatatype{ℕ}\AgdaSpace{}%
\AgdaSymbol{→}\AgdaSpace{}%
\AgdaDatatype{ℕ}\AgdaSpace{}%
\AgdaSymbol{→}\AgdaSpace{}%
\AgdaDatatype{ℕ}\AgdaSpace{}%
\AgdaSymbol{→}\AgdaSpace{}%
\AgdaPrimitive{Set}\<%
\\
\>[0]\AgdaFunction{accept₂ˢCore}\AgdaSpace{}%
\AgdaBound{time}\AgdaSpace{}%
\AgdaBound{m}\AgdaSpace{}%
\AgdaInductiveConstructor{zero}\AgdaSpace{}%
\AgdaBound{pbk}\AgdaSpace{}%
\AgdaBound{sig}\AgdaSpace{}%
\AgdaSymbol{=}\AgdaSpace{}%
\AgdaDatatype{⊥}\<%
\\
\>[0]\AgdaFunction{accept₂ˢCore}\AgdaSpace{}%
\AgdaBound{time}\AgdaSpace{}%
\AgdaBound{m}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaInductiveConstructor{suc}\AgdaSpace{}%
\AgdaBound{x}\AgdaSymbol{)}\AgdaSpace{}%
\AgdaBound{pbk}\AgdaSpace{}%
\AgdaBound{sig}\AgdaSpace{}%
\AgdaSymbol{=}%
\>[39]\AgdaFunction{IsSigned}%
\>[49]\AgdaBound{m}\AgdaSpace{}%
\AgdaBound{sig}\AgdaSpace{}%
\AgdaBound{pbk}\<%
\\
\>[0]\<%
\end{code}
} % END AgdaHide

\newcommand{\verificationptopbasicacceptTwo}{
\begin{code}[inline]%
\>[0]\AgdaFunction{accept₂ˢ}\AgdaSpace{}%
\AgdaSymbol{:}\AgdaSpace{}%
\AgdaFunction{StackPredicate}\<%
\\
\>[0]\AgdaFunction{accept₂ˢ}\AgdaSpace{}%
\AgdaBound{time}\AgdaSpace{}%
\AgdaBound{m}\AgdaSpace{}%
\AgdaInductiveConstructor{[]}\AgdaSpace{}%
\AgdaSymbol{=}\AgdaSpace{}%
\AgdaDatatype{⊥}\<%
\\
\>[0]\AgdaFunction{accept₂ˢ}\AgdaSpace{}%
\AgdaBound{time}\AgdaSpace{}%
\AgdaBound{m}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaBound{x}\AgdaSpace{}%
\AgdaOperator{\AgdaInductiveConstructor{∷}}\AgdaSpace{}%
\AgdaInductiveConstructor{[]}\AgdaSymbol{)}\AgdaSpace{}%
\AgdaSymbol{=}\AgdaSpace{}%
\AgdaDatatype{⊥}\<%
\\
\>[0]\AgdaFunction{accept₂ˢ}\AgdaSpace{}%
\AgdaBound{time}\AgdaSpace{}%
\AgdaBound{m}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaBound{x}\AgdaSpace{}%
\AgdaOperator{\AgdaInductiveConstructor{∷}}\AgdaSpace{}%
\AgdaBound{x₁}\AgdaSpace{}%
\AgdaOperator{\AgdaInductiveConstructor{∷}}\AgdaSpace{}%
\AgdaInductiveConstructor{[]}\AgdaSymbol{)}\AgdaSpace{}%
\AgdaSymbol{=}\AgdaSpace{}%
\AgdaDatatype{⊥}\<%
\\
\>[0]\AgdaFunction{accept₂ˢ}\AgdaSpace{}%
\AgdaBound{time}\AgdaSpace{}%
\AgdaBound{m}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaBound{x}\AgdaSpace{}%
\AgdaOperator{\AgdaInductiveConstructor{∷}}\AgdaSpace{}%
\AgdaBound{pbk}\AgdaSpace{}%
\AgdaOperator{\AgdaInductiveConstructor{∷}}\AgdaSpace{}%
\AgdaBound{sig}\AgdaSpace{}%
\AgdaOperator{\AgdaInductiveConstructor{∷}}\AgdaSpace{}%
\AgdaBound{rest}\AgdaSymbol{)}\AgdaSpace{}%
\AgdaSymbol{=}\AgdaSpace{}%
\AgdaFunction{accept₂ˢCore}\AgdaSpace{}%
\AgdaBound{time}\AgdaSpace{}%
\AgdaBound{m}\AgdaSpace{}%
\AgdaBound{x}\AgdaSpace{}%
\AgdaBound{pbk}\AgdaSpace{}%
\AgdaBound{sig}\<%
\end{code}
} % END newcommand

\AgdaHide{
\begin{code}%
\>[0]\<%
\\
\>[0]\<%
\end{code}
} % END AgdaHide

\newcommand{\verificationptopbasicacceptThree}{
\begin{code}[inline]%
\>[0]\AgdaFunction{accept₃ˢ}\AgdaSpace{}%
\AgdaSymbol{:}\AgdaSpace{}%
\AgdaFunction{StackPredicate}\<%
\\
\>[0]\AgdaFunction{accept₃ˢ}\AgdaSpace{}%
\AgdaBound{time}\AgdaSpace{}%
\AgdaBound{m}\AgdaSpace{}%
\AgdaInductiveConstructor{[]}\AgdaSpace{}%
\AgdaSymbol{=}\AgdaSpace{}%
\AgdaDatatype{⊥}\<%
\\
\>[0]\AgdaFunction{accept₃ˢ}\AgdaSpace{}%
\AgdaBound{time}\AgdaSpace{}%
\AgdaBound{m}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaBound{x}\AgdaSpace{}%
\AgdaOperator{\AgdaInductiveConstructor{∷}}\AgdaSpace{}%
\AgdaInductiveConstructor{[]}\AgdaSymbol{)}\AgdaSpace{}%
\AgdaSymbol{=}\AgdaSpace{}%
\AgdaDatatype{⊥}\<%
\\
\>[0]\AgdaFunction{accept₃ˢ}\AgdaSpace{}%
\AgdaBound{time}\AgdaSpace{}%
\AgdaBound{m}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaBound{x}\AgdaSpace{}%
\AgdaOperator{\AgdaInductiveConstructor{∷}}\AgdaSpace{}%
\AgdaBound{x₁}\AgdaSpace{}%
\AgdaOperator{\AgdaInductiveConstructor{∷}}\AgdaSpace{}%
\AgdaInductiveConstructor{[]}\AgdaSymbol{)}\AgdaSpace{}%
\AgdaSymbol{=}\AgdaSpace{}%
\AgdaDatatype{⊥}\<%
\\
\>[0]\AgdaFunction{accept₃ˢ}\AgdaSpace{}%
\AgdaBound{time}\AgdaSpace{}%
\AgdaBound{m}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaBound{x}\AgdaSpace{}%
\AgdaOperator{\AgdaInductiveConstructor{∷}}\AgdaSpace{}%
\AgdaBound{x₁}\AgdaSpace{}%
\AgdaOperator{\AgdaInductiveConstructor{∷}}\AgdaSpace{}%
\AgdaBound{x2}\AgdaSpace{}%
\AgdaOperator{\AgdaInductiveConstructor{∷}}\AgdaSpace{}%
\AgdaInductiveConstructor{[]}\AgdaSymbol{)}\AgdaSpace{}%
\AgdaSymbol{=}\AgdaSpace{}%
\AgdaDatatype{⊥}\<%
\\
\>[0]\AgdaFunction{accept₃ˢ}\AgdaSpace{}%
\AgdaBound{time}\AgdaSpace{}%
\AgdaBound{m}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaBound{pbkh2}\AgdaSpace{}%
\AgdaOperator{\AgdaInductiveConstructor{∷}}\AgdaSpace{}%
\AgdaBound{pbkh1}\AgdaSpace{}%
\AgdaOperator{\AgdaInductiveConstructor{∷}}\AgdaSpace{}%
\AgdaBound{pbk}\AgdaSpace{}%
\AgdaOperator{\AgdaInductiveConstructor{∷}}\AgdaSpace{}%
\AgdaBound{sig}\AgdaSpace{}%
\AgdaOperator{\AgdaInductiveConstructor{∷}}\AgdaSpace{}%
\AgdaBound{rest}\AgdaSymbol{)}\<%
\\
\>[0][@{}l@{\AgdaIndent{0}}]%
\>[5]\AgdaSymbol{=}%
\>[8]\AgdaSymbol{(}\AgdaBound{pbkh2}\AgdaSpace{}%
\AgdaOperator{\AgdaDatatype{≡}}%
\>[18]\AgdaBound{pbkh1}\AgdaSymbol{)}\AgdaSpace{}%
\AgdaOperator{\AgdaRecord{∧}}\AgdaSpace{}%
\AgdaFunction{IsSigned}%
\>[37]\AgdaBound{m}\AgdaSpace{}%
\AgdaBound{sig}\AgdaSpace{}%
\AgdaBound{pbk}\<%
\end{code}
} % END newcommand

\AgdaHide{
\begin{code}%
\>[0]\<%
\\
\>[0]\<%
\end{code}
} % END AgdaHide

\newcommand{\verificationptopbasicacceptFour}{
\begin{code}[inline]%
\>[0]\AgdaFunction{accept₄ˢ}\AgdaSpace{}%
\AgdaSymbol{:}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaSpace{}%
\AgdaBound{pbkh1}\AgdaSpace{}%
\AgdaSymbol{:}\AgdaSpace{}%
\AgdaDatatype{ℕ}\AgdaSpace{}%
\AgdaSymbol{)}\AgdaSpace{}%
\AgdaSymbol{→}\AgdaSpace{}%
\AgdaFunction{StackPredicate}\<%
\\
\>[0]\AgdaFunction{accept₄ˢ}\AgdaSpace{}%
\AgdaBound{pbkh1}\AgdaSpace{}%
\AgdaBound{time}\AgdaSpace{}%
\AgdaBound{m}\AgdaSpace{}%
\AgdaInductiveConstructor{[]}\AgdaSpace{}%
\AgdaSymbol{=}\AgdaSpace{}%
\AgdaDatatype{⊥}\<%
\\
\>[0]\AgdaFunction{accept₄ˢ}\AgdaSpace{}%
\AgdaBound{pbkh1}\AgdaSpace{}%
\AgdaBound{time}\AgdaSpace{}%
\AgdaBound{m}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaBound{x}\AgdaSpace{}%
\AgdaOperator{\AgdaInductiveConstructor{∷}}\AgdaSpace{}%
\AgdaInductiveConstructor{[]}\AgdaSymbol{)}\AgdaSpace{}%
\AgdaSymbol{=}\AgdaSpace{}%
\AgdaDatatype{⊥}\<%
\\
\>[0]\AgdaFunction{accept₄ˢ}\AgdaSpace{}%
\AgdaBound{pbkh1}\AgdaSpace{}%
\AgdaBound{time}\AgdaSpace{}%
\AgdaBound{m}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaBound{x}\AgdaSpace{}%
\AgdaOperator{\AgdaInductiveConstructor{∷}}\AgdaSpace{}%
\AgdaBound{x1}%
\>[31]\AgdaOperator{\AgdaInductiveConstructor{∷}}\AgdaSpace{}%
\AgdaInductiveConstructor{[]}\AgdaSymbol{)}\AgdaSpace{}%
\AgdaSymbol{=}\AgdaSpace{}%
\AgdaDatatype{⊥}\<%
\\
\>[0]\AgdaFunction{accept₄ˢ}\AgdaSpace{}%
\AgdaBound{pbkh1}\AgdaSpace{}%
\AgdaBound{time}\AgdaSpace{}%
\AgdaBound{m}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaSpace{}%
\AgdaBound{pbkh2}%
\>[32]\AgdaOperator{\AgdaInductiveConstructor{∷}}\AgdaSpace{}%
\AgdaBound{pbk}\AgdaSpace{}%
\AgdaOperator{\AgdaInductiveConstructor{∷}}\AgdaSpace{}%
\AgdaBound{sig}\AgdaSpace{}%
\AgdaOperator{\AgdaInductiveConstructor{∷}}\AgdaSpace{}%
\AgdaBound{st}\AgdaSymbol{)}\<%
\\
\>[0][@{}l@{\AgdaIndent{0}}]%
\>[8]\AgdaSymbol{=}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaBound{pbkh2}\AgdaSpace{}%
\AgdaOperator{\AgdaDatatype{≡}}%
\>[20]\AgdaBound{pbkh1}\AgdaSymbol{)}\AgdaSpace{}%
\AgdaOperator{\AgdaRecord{∧}}%
\>[30]\AgdaFunction{IsSigned}%
\>[40]\AgdaBound{m}\AgdaSpace{}%
\AgdaBound{sig}\AgdaSpace{}%
\AgdaBound{pbk}\<%
\end{code}
} % END newcommand

\AgdaHide{
\begin{code}%
\>[0]\<%
\\
\>[0]\<%
\end{code}
} % END AgdaHide

\newcommand{\verificationptopbasicacceptFive}{
\begin{code}[inline]%
\>[0]\AgdaFunction{accept₅ˢ}\AgdaSpace{}%
\AgdaSymbol{:}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaSpace{}%
\AgdaBound{pbkh1}\AgdaSpace{}%
\AgdaSymbol{:}\AgdaSpace{}%
\AgdaDatatype{ℕ}\AgdaSpace{}%
\AgdaSymbol{)}\AgdaSpace{}%
\AgdaSymbol{→}\AgdaSpace{}%
\AgdaFunction{StackPredicate}\<%
\\
\>[0]\AgdaFunction{accept₅ˢ}%
\>[10]\AgdaBound{pbkh1}\AgdaSpace{}%
\AgdaBound{time}\AgdaSpace{}%
\AgdaBound{m}\AgdaSpace{}%
\AgdaInductiveConstructor{[]}\AgdaSpace{}%
\AgdaSymbol{=}\AgdaSpace{}%
\AgdaDatatype{⊥}\<%
\\
\>[0]\AgdaFunction{accept₅ˢ}%
\>[10]\AgdaBound{pbkh1}\AgdaSpace{}%
\AgdaBound{time}\AgdaSpace{}%
\AgdaBound{m}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaBound{x}\AgdaSpace{}%
\AgdaOperator{\AgdaInductiveConstructor{∷}}\AgdaSpace{}%
\AgdaInductiveConstructor{[]}\AgdaSymbol{)}\AgdaSpace{}%
\AgdaSymbol{=}\AgdaSpace{}%
\AgdaDatatype{⊥}\<%
\\
\>[0]\AgdaFunction{accept₅ˢ}%
\>[10]\AgdaBound{pbkh1}\AgdaSpace{}%
\AgdaBound{time}\AgdaSpace{}%
\AgdaBound{m}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaBound{x}\AgdaSpace{}%
\AgdaOperator{\AgdaInductiveConstructor{∷}}\AgdaSpace{}%
\AgdaBound{x₁}\AgdaSpace{}%
\AgdaOperator{\AgdaInductiveConstructor{∷}}\AgdaSpace{}%
\AgdaInductiveConstructor{[]}\AgdaSymbol{)}\AgdaSpace{}%
\AgdaSymbol{=}\AgdaSpace{}%
\AgdaDatatype{⊥}\<%
\\
\>[0]\AgdaFunction{accept₅ˢ}%
\>[10]\AgdaBound{pbkh1}\AgdaSpace{}%
\AgdaBound{time}\AgdaSpace{}%
\AgdaBound{m}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaSpace{}%
\AgdaBound{pbk1}%
\>[32]\AgdaOperator{\AgdaInductiveConstructor{∷}}\AgdaSpace{}%
\AgdaBound{pbk2}\AgdaSpace{}%
\AgdaOperator{\AgdaInductiveConstructor{∷}}\AgdaSpace{}%
\AgdaBound{sig}\AgdaSpace{}%
\AgdaOperator{\AgdaInductiveConstructor{∷}}\AgdaSpace{}%
\AgdaBound{st}\AgdaSymbol{)}\<%
\\
\>[0][@{}l@{\AgdaIndent{0}}]%
\>[7]\AgdaSymbol{=}%
\>[10]\AgdaSymbol{(}\AgdaFunction{hashFun}\AgdaSpace{}%
\AgdaBound{pbk1}\AgdaSpace{}%
\AgdaOperator{\AgdaDatatype{≡}}%
\>[27]\AgdaBound{pbkh1}\AgdaSymbol{)}\AgdaSpace{}%
\AgdaOperator{\AgdaRecord{∧}}%
\>[37]\AgdaFunction{IsSigned}%
\>[48]\AgdaBound{m}%
\>[51]\AgdaBound{sig}%
\>[56]\AgdaBound{pbk2}\<%
\end{code}
} % END newcommand

\AgdaHide{
\begin{code}%
\>[0]\<%
\\
\>[0]\<%
\end{code}
} % END AgdaHide

\newcommand{\verificationptopbasicweakestprecondition}{
\begin{code}%
\>[0]\AgdaFunction{wPreCondP2PKHˢ}\AgdaSpace{}%
\AgdaSymbol{:}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaBound{pbkh}\AgdaSpace{}%
\AgdaSymbol{:}\AgdaSpace{}%
\AgdaDatatype{ℕ}\AgdaSpace{}%
\AgdaSymbol{)}\AgdaSpace{}%
\AgdaSymbol{→}\AgdaSpace{}%
\AgdaFunction{StackPredicate}\<%
\\
\>[0]\AgdaFunction{wPreCondP2PKHˢ}%
\>[16]\AgdaBound{pbkh}%
\>[22]\AgdaBound{time}%
\>[28]\AgdaBound{m}%
\>[31]\AgdaInductiveConstructor{[]}%
\>[53]\AgdaSymbol{=}%
\>[56]\AgdaDatatype{⊥}\<%
\\
\>[0]\AgdaFunction{wPreCondP2PKHˢ}%
\>[16]\AgdaBound{pbkh}%
\>[22]\AgdaBound{time}%
\>[28]\AgdaBound{m}%
\>[31]\AgdaSymbol{(}\AgdaBound{x}\AgdaSpace{}%
\AgdaOperator{\AgdaInductiveConstructor{∷}}\AgdaSpace{}%
\AgdaInductiveConstructor{[]}\AgdaSymbol{)}%
\>[53]\AgdaSymbol{=}%
\>[56]\AgdaDatatype{⊥}\<%
\\
\>[0]\AgdaFunction{wPreCondP2PKHˢ}%
\>[16]\AgdaBound{pbkh}%
\>[22]\AgdaBound{time}%
\>[28]\AgdaBound{m}%
\>[31]\AgdaSymbol{(}\AgdaSpace{}%
\AgdaBound{pbk}\AgdaSpace{}%
\AgdaOperator{\AgdaInductiveConstructor{∷}}\AgdaSpace{}%
\AgdaBound{sig}\AgdaSpace{}%
\AgdaOperator{\AgdaInductiveConstructor{∷}}\AgdaSpace{}%
\AgdaBound{st}\AgdaSymbol{)}%
\>[50]\AgdaSymbol{=}\<%
\\
%
\>[16]\AgdaSymbol{(}\AgdaFunction{hashFun}\AgdaSpace{}%
\AgdaBound{pbk}\AgdaSpace{}%
\AgdaOperator{\AgdaDatatype{≡}}%
\>[32]\AgdaBound{pbkh}\AgdaSpace{}%
\AgdaSymbol{)}\AgdaSpace{}%
\AgdaOperator{\AgdaRecord{∧}}\AgdaSpace{}%
\AgdaFunction{IsSigned}%
\>[51]\AgdaBound{m}\AgdaSpace{}%
\AgdaBound{sig}\AgdaSpace{}%
\AgdaBound{pbk}\<%
\end{code}
} % END newcommand

\AgdaHide{
\begin{code}%
\>[0]\<%
\\
%
\\[\AgdaEmptyExtraSkip]%
\>[0]\AgdaFunction{correct3Aux1}\AgdaSpace{}%
\AgdaSymbol{:}%
\>[394I]\AgdaSymbol{(}\AgdaBound{x}\AgdaSpace{}%
\AgdaSymbol{:}\AgdaSpace{}%
\AgdaDatatype{ℕ}\AgdaSymbol{)(}\AgdaBound{rest}\AgdaSpace{}%
\AgdaSymbol{:}\AgdaSpace{}%
\AgdaDatatype{List}\AgdaSpace{}%
\AgdaDatatype{ℕ}\AgdaSymbol{)(}\AgdaBound{time}\AgdaSpace{}%
\AgdaSymbol{:}\AgdaSpace{}%
\AgdaFunction{Time}\AgdaSymbol{)(}\AgdaBound{msg}\AgdaSpace{}%
\AgdaSymbol{:}\AgdaSpace{}%
\AgdaDatatype{Msg}\AgdaSymbol{)}\AgdaSpace{}%
\AgdaSymbol{→}\AgdaSpace{}%
\AgdaFunction{accept₂ˢ}\AgdaSpace{}%
\AgdaBound{time}\AgdaSpace{}%
\AgdaBound{msg}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaBound{x}\AgdaSpace{}%
\AgdaOperator{\AgdaInductiveConstructor{∷}}\AgdaSpace{}%
\AgdaBound{rest}\AgdaSymbol{)}\<%
\\
\>[.][@{}l@{}]\<[394I]%
\>[15]\AgdaSymbol{→}%
\>[18]\AgdaFunction{isTrueNat}\AgdaSpace{}%
\AgdaBound{x}\<%
\\
\>[0]\AgdaFunction{correct3Aux1}\AgdaSpace{}%
\AgdaInductiveConstructor{zero}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaInductiveConstructor{zero}\AgdaSpace{}%
\AgdaOperator{\AgdaInductiveConstructor{∷}}\AgdaSpace{}%
\AgdaInductiveConstructor{[]}\AgdaSymbol{)}\AgdaSpace{}%
\AgdaBound{time}\AgdaSpace{}%
\AgdaBound{msg}\AgdaSpace{}%
\AgdaBound{accept}\AgdaSpace{}%
\AgdaSymbol{=}\AgdaSpace{}%
\AgdaBound{accept}\<%
\\
\>[0]\AgdaFunction{correct3Aux1}\AgdaSpace{}%
\AgdaInductiveConstructor{zero}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaInductiveConstructor{zero}\AgdaSpace{}%
\AgdaOperator{\AgdaInductiveConstructor{∷}}\AgdaSpace{}%
\AgdaBound{x}\AgdaSpace{}%
\AgdaOperator{\AgdaInductiveConstructor{∷}}\AgdaSpace{}%
\AgdaBound{rest}\AgdaSymbol{)}\AgdaSpace{}%
\AgdaBound{time}\AgdaSpace{}%
\AgdaBound{msg}\AgdaSpace{}%
\AgdaBound{accept}\AgdaSpace{}%
\AgdaSymbol{=}\AgdaSpace{}%
\AgdaBound{accept}\<%
\\
\>[0]\AgdaFunction{correct3Aux1}\AgdaSpace{}%
\AgdaInductiveConstructor{zero}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaInductiveConstructor{suc}\AgdaSpace{}%
\AgdaBound{x}\AgdaSpace{}%
\AgdaOperator{\AgdaInductiveConstructor{∷}}\AgdaSpace{}%
\AgdaInductiveConstructor{[]}\AgdaSymbol{)}\AgdaSpace{}%
\AgdaBound{time}\AgdaSpace{}%
\AgdaBound{msg}\AgdaSpace{}%
\AgdaBound{accept}\AgdaSpace{}%
\AgdaSymbol{=}\AgdaSpace{}%
\AgdaBound{accept}\<%
\\
\>[0]\AgdaFunction{correct3Aux1}\AgdaSpace{}%
\AgdaInductiveConstructor{zero}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaInductiveConstructor{suc}\AgdaSpace{}%
\AgdaBound{x}\AgdaSpace{}%
\AgdaOperator{\AgdaInductiveConstructor{∷}}\AgdaSpace{}%
\AgdaBound{x₁}\AgdaSpace{}%
\AgdaOperator{\AgdaInductiveConstructor{∷}}\AgdaSpace{}%
\AgdaBound{rest}\AgdaSymbol{)}\AgdaSpace{}%
\AgdaBound{time}\AgdaSpace{}%
\AgdaBound{msg}\AgdaSpace{}%
\AgdaBound{accept}\AgdaSpace{}%
\AgdaSymbol{=}\AgdaSpace{}%
\AgdaBound{accept}\<%
\\
\>[0]\AgdaFunction{correct3Aux1}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaInductiveConstructor{suc}\AgdaSpace{}%
\AgdaBound{x}\AgdaSymbol{)}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaBound{x₁}\AgdaSpace{}%
\AgdaOperator{\AgdaInductiveConstructor{∷}}\AgdaSpace{}%
\AgdaBound{rest}\AgdaSymbol{)}\AgdaSpace{}%
\AgdaBound{time}\AgdaSpace{}%
\AgdaBound{msg}\AgdaSpace{}%
\AgdaBound{accept}\AgdaSpace{}%
\AgdaSymbol{=}\AgdaSpace{}%
\AgdaInductiveConstructor{tt}\<%
\\
%
\\[\AgdaEmptyExtraSkip]%
%
\\[\AgdaEmptyExtraSkip]%
\>[0]\AgdaFunction{correct3Aux2}\AgdaSpace{}%
\AgdaSymbol{:}%
\>[465I]\AgdaSymbol{(}\AgdaSpace{}%
\AgdaBound{x}\AgdaSpace{}%
\AgdaBound{pbk}\AgdaSpace{}%
\AgdaBound{sig}\AgdaSpace{}%
\AgdaSymbol{:}\AgdaSpace{}%
\AgdaDatatype{ℕ}\AgdaSpace{}%
\AgdaSymbol{)(}\AgdaSpace{}%
\AgdaBound{rest}\AgdaSpace{}%
\AgdaSymbol{:}\AgdaSpace{}%
\AgdaDatatype{List}\AgdaSpace{}%
\AgdaDatatype{ℕ}\AgdaSymbol{)(}\AgdaBound{time}\AgdaSpace{}%
\AgdaSymbol{:}\AgdaSpace{}%
\AgdaFunction{Time}\AgdaSymbol{)(}\AgdaBound{m}\AgdaSpace{}%
\AgdaSymbol{:}\AgdaSpace{}%
\AgdaDatatype{Msg}\AgdaSymbol{)}\<%
\\
\>[465I][@{}l@{\AgdaIndent{0}}]%
\>[16]\AgdaSymbol{→}\AgdaSpace{}%
\AgdaFunction{accept₂ˢ}\AgdaSpace{}%
\AgdaBound{time}\AgdaSpace{}%
\AgdaBound{m}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaBound{x}\AgdaSpace{}%
\AgdaOperator{\AgdaInductiveConstructor{∷}}\AgdaSpace{}%
\AgdaBound{pbk}\AgdaSpace{}%
\AgdaOperator{\AgdaInductiveConstructor{∷}}\AgdaSpace{}%
\AgdaBound{sig}\AgdaSpace{}%
\AgdaOperator{\AgdaInductiveConstructor{∷}}\AgdaSpace{}%
\AgdaBound{rest}\AgdaSymbol{)}\<%
\\
%
\>[16]\AgdaSymbol{→}\AgdaSpace{}%
\AgdaFunction{IsSigned}%
\>[28]\AgdaBound{m}\AgdaSpace{}%
\AgdaBound{sig}\AgdaSpace{}%
\AgdaBound{pbk}\<%
\\
\>[0]\AgdaFunction{correct3Aux2}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaInductiveConstructor{suc}\AgdaSpace{}%
\AgdaBound{x}\AgdaSymbol{)}\AgdaSpace{}%
\AgdaBound{pubkey}\AgdaSpace{}%
\AgdaBound{sig}\AgdaSpace{}%
\AgdaBound{rest}\AgdaSpace{}%
\AgdaBound{time}\AgdaSpace{}%
\AgdaBound{m}\AgdaSpace{}%
\AgdaBound{accept}\AgdaSpace{}%
\AgdaSymbol{=}\AgdaSpace{}%
\AgdaBound{accept}\<%
\\
%
\\[\AgdaEmptyExtraSkip]%
%
\\[\AgdaEmptyExtraSkip]%
%
\\[\AgdaEmptyExtraSkip]%
\>[0]\AgdaFunction{lemmaCorrect3From1}%
\>[503I]\AgdaSymbol{:}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaBound{x}\AgdaSpace{}%
\AgdaBound{z}\AgdaSpace{}%
\AgdaBound{t}\AgdaSpace{}%
\AgdaSymbol{:}\AgdaSpace{}%
\AgdaDatatype{ℕ}\AgdaSymbol{)(}\AgdaBound{time}\AgdaSpace{}%
\AgdaSymbol{:}\AgdaSpace{}%
\AgdaFunction{Time}\AgdaSpace{}%
\AgdaSymbol{)(}\AgdaBound{m}\AgdaSpace{}%
\AgdaSymbol{:}\AgdaSpace{}%
\AgdaDatatype{Msg}\AgdaSymbol{)}\<%
\\
\>[503I][@{}l@{\AgdaIndent{0}}]%
\>[20]\AgdaSymbol{→}%
\>[23]\AgdaFunction{accept₂ˢCore}\AgdaSpace{}%
\AgdaBound{time}\AgdaSpace{}%
\AgdaBound{m}\AgdaSpace{}%
\AgdaBound{x}\AgdaSpace{}%
\AgdaBound{z}\AgdaSpace{}%
\AgdaBound{t}\AgdaSpace{}%
\AgdaSymbol{→}\AgdaSpace{}%
\AgdaFunction{isTrueNat}\AgdaSpace{}%
\AgdaBound{x}\<%
\\
\>[0]\AgdaFunction{lemmaCorrect3From1}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaInductiveConstructor{suc}\AgdaSpace{}%
\AgdaBound{x}\AgdaSymbol{)}\AgdaSpace{}%
\AgdaBound{z}\AgdaSpace{}%
\AgdaBound{t}\AgdaSpace{}%
\AgdaBound{time}\AgdaSpace{}%
\AgdaBound{m}\AgdaSpace{}%
\AgdaBound{p}\AgdaSpace{}%
\AgdaSymbol{=}\AgdaSpace{}%
\AgdaInductiveConstructor{tt}\<%
\\
%
\\[\AgdaEmptyExtraSkip]%
%
\\[\AgdaEmptyExtraSkip]%
\>[0]\AgdaFunction{lemmaCorrect3From}\AgdaSpace{}%
\AgdaSymbol{:}%
\>[532I]\AgdaSymbol{(}\AgdaBound{x}\AgdaSpace{}%
\AgdaBound{y}\AgdaSpace{}%
\AgdaBound{z}\AgdaSpace{}%
\AgdaBound{t}\AgdaSpace{}%
\AgdaSymbol{:}\AgdaSpace{}%
\AgdaDatatype{ℕ}\AgdaSymbol{)(}\AgdaBound{time}\AgdaSpace{}%
\AgdaSymbol{:}\AgdaSpace{}%
\AgdaFunction{Time}\AgdaSymbol{)(}\AgdaBound{m}\AgdaSpace{}%
\AgdaSymbol{:}\AgdaSpace{}%
\AgdaDatatype{Msg}\AgdaSymbol{)}\<%
\\
\>[.][@{}l@{}]\<[532I]%
\>[20]\AgdaSymbol{→}%
\>[23]\AgdaFunction{accept₂ˢCore}\AgdaSpace{}%
\AgdaBound{time}\AgdaSpace{}%
\AgdaBound{m}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaFunction{compareNaturals}\AgdaSpace{}%
\AgdaBound{x}\AgdaSpace{}%
\AgdaBound{y}\AgdaSymbol{)}\AgdaSpace{}%
\AgdaBound{z}\AgdaSpace{}%
\AgdaBound{t}\AgdaSpace{}%
\AgdaSymbol{→}\AgdaSpace{}%
\AgdaBound{x}\AgdaSpace{}%
\AgdaOperator{\AgdaDatatype{≡}}\AgdaSpace{}%
\AgdaBound{y}\<%
\\
\>[0]\AgdaFunction{lemmaCorrect3From}\AgdaSpace{}%
\AgdaBound{x}\AgdaSpace{}%
\AgdaBound{y}\AgdaSpace{}%
\AgdaBound{z}\AgdaSpace{}%
\AgdaBound{t}\AgdaSpace{}%
\AgdaBound{time}\AgdaSpace{}%
\AgdaBound{m}\AgdaSpace{}%
\AgdaBound{p}\AgdaSpace{}%
\AgdaSymbol{=}\AgdaSpace{}%
\AgdaFunction{compareNatToEq}\AgdaSpace{}%
\AgdaBound{x}%
\>[55]\AgdaBound{y}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaFunction{lemmaCorrect3From1}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaFunction{compareNaturals}\AgdaSpace{}%
\AgdaBound{x}\AgdaSpace{}%
\AgdaBound{y}\AgdaSymbol{)}\AgdaSpace{}%
\AgdaBound{z}\AgdaSpace{}%
\AgdaBound{t}\AgdaSpace{}%
\AgdaBound{time}\AgdaSpace{}%
\AgdaBound{m}\AgdaSpace{}%
\AgdaBound{p}\AgdaSymbol{)}\<%
\\
%
\\[\AgdaEmptyExtraSkip]%
%
\\[\AgdaEmptyExtraSkip]%
\>[0]\AgdaFunction{script-1-b}%
\>[12]\AgdaSymbol{:}\AgdaSpace{}%
\AgdaFunction{BitcoinScriptBasic}\<%
\\
\>[0]\AgdaFunction{script-1-b}\AgdaSpace{}%
\AgdaSymbol{=}\AgdaSpace{}%
\AgdaInductiveConstructor{opCheckSig}\AgdaSpace{}%
\AgdaOperator{\AgdaInductiveConstructor{∷}}\AgdaSpace{}%
\AgdaInductiveConstructor{[]}\<%
\\
%
\\[\AgdaEmptyExtraSkip]%
\>[0]\AgdaFunction{script-2-b}\AgdaSpace{}%
\AgdaSymbol{:}\AgdaSpace{}%
\AgdaFunction{BitcoinScriptBasic}\<%
\\
\>[0]\AgdaFunction{script-2-b}\AgdaSpace{}%
\AgdaSymbol{=}\AgdaSpace{}%
\AgdaInductiveConstructor{opVerify}\AgdaSpace{}%
\AgdaOperator{\AgdaInductiveConstructor{∷}}\AgdaSpace{}%
\AgdaFunction{script-1-b}\<%
\\
%
\\[\AgdaEmptyExtraSkip]%
\>[0]\AgdaFunction{script-3-b}\AgdaSpace{}%
\AgdaSymbol{:}\AgdaSpace{}%
\AgdaFunction{BitcoinScriptBasic}\<%
\\
\>[0]\AgdaFunction{script-3-b}\AgdaSpace{}%
\AgdaSymbol{=}\AgdaSpace{}%
\AgdaInductiveConstructor{opEqual}\AgdaSpace{}%
\AgdaOperator{\AgdaInductiveConstructor{∷}}\AgdaSpace{}%
\AgdaFunction{script-2-b}\<%
\\
%
\\[\AgdaEmptyExtraSkip]%
\>[0]\AgdaFunction{script-4-b}\AgdaSpace{}%
\AgdaSymbol{:}\AgdaSpace{}%
\AgdaDatatype{ℕ}\AgdaSpace{}%
\AgdaSymbol{→}\AgdaSpace{}%
\AgdaFunction{BitcoinScriptBasic}\<%
\\
\>[0]\AgdaFunction{script-4-b}\AgdaSpace{}%
\AgdaBound{pbkh}%
\>[17]\AgdaSymbol{=}%
\>[20]\AgdaInductiveConstructor{opPush}%
\>[28]\AgdaBound{pbkh}\AgdaSpace{}%
\AgdaOperator{\AgdaInductiveConstructor{∷}}\AgdaSpace{}%
\AgdaFunction{script-3-b}\<%
\\
%
\\[\AgdaEmptyExtraSkip]%
\>[0]\AgdaFunction{script-5-b}\AgdaSpace{}%
\AgdaSymbol{:}\AgdaSpace{}%
\AgdaDatatype{ℕ}\AgdaSpace{}%
\AgdaSymbol{→}%
\>[18]\AgdaFunction{BitcoinScriptBasic}\<%
\\
\>[0]\AgdaFunction{script-5-b}\AgdaSpace{}%
\AgdaBound{pbkh}\AgdaSpace{}%
\AgdaSymbol{=}\AgdaSpace{}%
\AgdaInductiveConstructor{opHash}%
\>[26]\AgdaOperator{\AgdaInductiveConstructor{∷}}\AgdaSpace{}%
\AgdaFunction{script-4-b}%
\>[40]\AgdaBound{pbkh}\<%
\\
%
\\[\AgdaEmptyExtraSkip]%
\>[0]\AgdaFunction{script-6-b}\AgdaSpace{}%
\AgdaSymbol{:}\AgdaSpace{}%
\AgdaDatatype{ℕ}\AgdaSpace{}%
\AgdaSymbol{→}\AgdaSpace{}%
\AgdaFunction{BitcoinScriptBasic}\<%
\\
\>[0]\AgdaFunction{script-6-b}\AgdaSpace{}%
\AgdaBound{pbkh}%
\>[17]\AgdaSymbol{=}\AgdaSpace{}%
\AgdaInductiveConstructor{opDup}\AgdaSpace{}%
\AgdaOperator{\AgdaInductiveConstructor{∷}}\AgdaSpace{}%
\AgdaFunction{script-5-b}\AgdaSpace{}%
\AgdaBound{pbkh}\<%
\\
%
\\[\AgdaEmptyExtraSkip]%
%
\\[\AgdaEmptyExtraSkip]%
\>[0]\AgdaComment{--new}\<%
\\
\>[0]\AgdaFunction{script-7-b}\AgdaSpace{}%
\AgdaSymbol{:}\AgdaSpace{}%
\AgdaDatatype{ℕ}\AgdaSpace{}%
\AgdaSymbol{→}\AgdaSpace{}%
\AgdaFunction{BitcoinScriptBasic}\<%
\\
\>[0]\AgdaFunction{script-7-b}\AgdaSpace{}%
\AgdaBound{pbkh}\AgdaSpace{}%
\AgdaSymbol{=}\AgdaSpace{}%
\AgdaInductiveConstructor{opMultiSig}\AgdaSpace{}%
\AgdaOperator{\AgdaInductiveConstructor{∷}}\AgdaSpace{}%
\AgdaFunction{script-6-b}\AgdaSpace{}%
\AgdaBound{pbkh}\<%
\\
%
\\[\AgdaEmptyExtraSkip]%
\>[0]\AgdaFunction{script-7'-b}\AgdaSpace{}%
\AgdaSymbol{:}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaBound{pbkh}\AgdaSpace{}%
\AgdaBound{pbk1}\AgdaSpace{}%
\AgdaBound{pbk2}\AgdaSpace{}%
\AgdaSymbol{:}\AgdaSpace{}%
\AgdaDatatype{ℕ}\AgdaSymbol{)}\AgdaSpace{}%
\AgdaSymbol{→}\AgdaSpace{}%
\AgdaFunction{BitcoinScriptBasic}\<%
\\
\>[0]\AgdaFunction{script-7'-b}\AgdaSpace{}%
\AgdaBound{pbkh}\AgdaSpace{}%
\AgdaBound{pbk1}\AgdaSpace{}%
\AgdaBound{pbk2}\AgdaSpace{}%
\AgdaSymbol{=}\AgdaSpace{}%
\AgdaInductiveConstructor{opMultiSig}\AgdaSpace{}%
\AgdaOperator{\AgdaInductiveConstructor{∷}}\AgdaSpace{}%
\AgdaFunction{script-6-b}\AgdaSpace{}%
\AgdaBound{pbkh}\<%
\\
%
\\[\AgdaEmptyExtraSkip]%
%
\\[\AgdaEmptyExtraSkip]%
\>[0]\AgdaFunction{script-1}%
\>[10]\AgdaSymbol{:}\AgdaSpace{}%
\AgdaFunction{BitcoinScript}\<%
\\
\>[0]\AgdaFunction{script-1}%
\>[10]\AgdaSymbol{=}\AgdaSpace{}%
\AgdaFunction{basicBScript2BScript}\AgdaSpace{}%
\AgdaFunction{script-1-b}\<%
\\
%
\\[\AgdaEmptyExtraSkip]%
\>[0]\AgdaFunction{script-2}%
\>[10]\AgdaSymbol{:}\AgdaSpace{}%
\AgdaFunction{BitcoinScript}\<%
\\
\>[0]\AgdaFunction{script-2}%
\>[10]\AgdaSymbol{=}\AgdaSpace{}%
\AgdaFunction{basicBScript2BScript}\AgdaSpace{}%
\AgdaFunction{script-2-b}\<%
\\
%
\\[\AgdaEmptyExtraSkip]%
\>[0]\AgdaFunction{script-3}%
\>[10]\AgdaSymbol{:}\AgdaSpace{}%
\AgdaFunction{BitcoinScript}\<%
\\
\>[0]\AgdaFunction{script-3}%
\>[10]\AgdaSymbol{=}\AgdaSpace{}%
\AgdaFunction{basicBScript2BScript}\AgdaSpace{}%
\AgdaFunction{script-3-b}\<%
\\
%
\\[\AgdaEmptyExtraSkip]%
\>[0]\AgdaFunction{script-4}%
\>[10]\AgdaSymbol{:}\AgdaSpace{}%
\AgdaDatatype{ℕ}\AgdaSpace{}%
\AgdaSymbol{→}\AgdaSpace{}%
\AgdaFunction{BitcoinScript}\<%
\\
\>[0]\AgdaFunction{script-4}%
\>[10]\AgdaBound{pbk}\AgdaSpace{}%
\AgdaSymbol{=}\AgdaSpace{}%
\AgdaFunction{basicBScript2BScript}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaFunction{script-4-b}\AgdaSpace{}%
\AgdaBound{pbk}\AgdaSymbol{)}\<%
\\
%
\\[\AgdaEmptyExtraSkip]%
\>[0]\AgdaFunction{script-5}%
\>[10]\AgdaSymbol{:}\AgdaSpace{}%
\AgdaDatatype{ℕ}\AgdaSpace{}%
\AgdaSymbol{→}\AgdaSpace{}%
\AgdaFunction{BitcoinScript}\<%
\\
\>[0]\AgdaFunction{script-5}%
\>[10]\AgdaBound{pbk}\AgdaSpace{}%
\AgdaSymbol{=}\AgdaSpace{}%
\AgdaFunction{basicBScript2BScript}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaFunction{script-5-b}\AgdaSpace{}%
\AgdaBound{pbk}\AgdaSymbol{)}\<%
\\
%
\\[\AgdaEmptyExtraSkip]%
\>[0]\AgdaFunction{script-6}%
\>[10]\AgdaSymbol{:}\AgdaSpace{}%
\AgdaDatatype{ℕ}\AgdaSpace{}%
\AgdaSymbol{→}\AgdaSpace{}%
\AgdaFunction{BitcoinScript}\<%
\\
\>[0]\AgdaFunction{script-6}%
\>[10]\AgdaBound{pbk}\AgdaSpace{}%
\AgdaSymbol{=}\AgdaSpace{}%
\AgdaFunction{basicBScript2BScript}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaFunction{script-6-b}\AgdaSpace{}%
\AgdaBound{pbk}\AgdaSymbol{)}\<%
\\
%
\\[\AgdaEmptyExtraSkip]%
\>[0]\AgdaFunction{script-7}%
\>[10]\AgdaSymbol{:}\AgdaSpace{}%
\AgdaDatatype{ℕ}\AgdaSpace{}%
\AgdaSymbol{→}\AgdaSpace{}%
\AgdaFunction{BitcoinScript}\<%
\\
\>[0]\AgdaFunction{script-7}%
\>[10]\AgdaBound{pbk}\AgdaSpace{}%
\AgdaSymbol{=}\AgdaSpace{}%
\AgdaFunction{basicBScript2BScript}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaFunction{script-7-b}\AgdaSpace{}%
\AgdaBound{pbk}\AgdaSymbol{)}\<%
\\
%
\\[\AgdaEmptyExtraSkip]%
%
\\[\AgdaEmptyExtraSkip]%
\>[0]\AgdaFunction{script-7'}\AgdaSpace{}%
\AgdaSymbol{:}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaBound{pbkh}\AgdaSpace{}%
\AgdaBound{pbk1}\AgdaSpace{}%
\AgdaBound{pbk2}\AgdaSpace{}%
\AgdaSymbol{:}\AgdaSpace{}%
\AgdaDatatype{ℕ}\AgdaSymbol{)}\AgdaSpace{}%
\AgdaSymbol{→}\AgdaSpace{}%
\AgdaFunction{BitcoinScript}\<%
\\
\>[0]\AgdaFunction{script-7'}%
\>[11]\AgdaBound{pbkh}\AgdaSpace{}%
\AgdaBound{pbk1}\AgdaSpace{}%
\AgdaBound{pbk2}\AgdaSpace{}%
\AgdaSymbol{=}\AgdaSpace{}%
\AgdaFunction{basicBScript2BScript}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaFunction{script-7'-b}\AgdaSpace{}%
\AgdaBound{pbkh}\AgdaSpace{}%
\AgdaBound{pbk1}\AgdaSpace{}%
\AgdaBound{pbk2}\AgdaSymbol{)}\<%
\\
%
\\[\AgdaEmptyExtraSkip]%
%
\\[\AgdaEmptyExtraSkip]%
%
\\[\AgdaEmptyExtraSkip]%
\>[0]\AgdaFunction{instructionsBasic}\AgdaSpace{}%
\AgdaSymbol{:}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaBound{pbkh}\AgdaSpace{}%
\AgdaSymbol{:}\AgdaSpace{}%
\AgdaDatatype{ℕ}\AgdaSymbol{)}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaBound{n}\AgdaSpace{}%
\AgdaSymbol{:}\AgdaSpace{}%
\AgdaDatatype{ℕ}\AgdaSymbol{)}\AgdaSpace{}%
\AgdaSymbol{→}\AgdaSpace{}%
\AgdaBound{n}\AgdaSpace{}%
\AgdaOperator{\AgdaFunction{≤}}\AgdaSpace{}%
\AgdaNumber{5}\AgdaSpace{}%
\AgdaSymbol{→}\AgdaSpace{}%
\AgdaDatatype{InstructionBasic}\<%
\\
\>[0]\AgdaFunction{instructionsBasic}\AgdaSpace{}%
\AgdaBound{pbkh}\AgdaSpace{}%
\AgdaNumber{0}\AgdaSpace{}%
\AgdaSymbol{\AgdaUnderscore{}}\AgdaSpace{}%
\AgdaSymbol{=}\AgdaSpace{}%
\AgdaInductiveConstructor{opCheckSig}\<%
\\
\>[0]\AgdaFunction{instructionsBasic}\AgdaSpace{}%
\AgdaBound{pbkh}\AgdaSpace{}%
\AgdaNumber{1}\AgdaSpace{}%
\AgdaSymbol{\AgdaUnderscore{}}\AgdaSpace{}%
\AgdaSymbol{=}\AgdaSpace{}%
\AgdaInductiveConstructor{opVerify}\<%
\\
\>[0]\AgdaFunction{instructionsBasic}\AgdaSpace{}%
\AgdaBound{pbkh}\AgdaSpace{}%
\AgdaNumber{2}\AgdaSpace{}%
\AgdaSymbol{\AgdaUnderscore{}}\AgdaSpace{}%
\AgdaSymbol{=}\AgdaSpace{}%
\AgdaInductiveConstructor{opEqual}\<%
\\
\>[0]\AgdaFunction{instructionsBasic}\AgdaSpace{}%
\AgdaBound{pbkh}\AgdaSpace{}%
\AgdaNumber{3}\AgdaSpace{}%
\AgdaSymbol{\AgdaUnderscore{}}\AgdaSpace{}%
\AgdaSymbol{=}\AgdaSpace{}%
\AgdaInductiveConstructor{opPush}\AgdaSpace{}%
\AgdaBound{pbkh}\<%
\\
\>[0]\AgdaFunction{instructionsBasic}\AgdaSpace{}%
\AgdaBound{pbkh}\AgdaSpace{}%
\AgdaNumber{4}\AgdaSpace{}%
\AgdaSymbol{\AgdaUnderscore{}}\AgdaSpace{}%
\AgdaSymbol{=}\AgdaSpace{}%
\AgdaInductiveConstructor{opHash}\<%
\\
\>[0]\AgdaFunction{instructionsBasic}\AgdaSpace{}%
\AgdaBound{pbkh}\AgdaSpace{}%
\AgdaNumber{5}\AgdaSpace{}%
\AgdaSymbol{\AgdaUnderscore{}}\AgdaSpace{}%
\AgdaSymbol{=}\AgdaSpace{}%
\AgdaInductiveConstructor{opDup}\<%
\\
%
\\[\AgdaEmptyExtraSkip]%
\>[0]\AgdaFunction{scriptP2PKH}\AgdaSpace{}%
\AgdaSymbol{:}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaBound{pbkh}\AgdaSpace{}%
\AgdaSymbol{:}\AgdaSpace{}%
\AgdaDatatype{ℕ}\AgdaSymbol{)}\AgdaSpace{}%
\AgdaSymbol{→}\AgdaSpace{}%
\AgdaFunction{BitcoinScript}\<%
\\
\>[0]\AgdaFunction{scriptP2PKH}\AgdaSpace{}%
\AgdaBound{pbkh}\AgdaSpace{}%
\AgdaSymbol{=}\AgdaSpace{}%
\AgdaInductiveConstructor{opDup}\AgdaSpace{}%
\AgdaOperator{\AgdaInductiveConstructor{∷}}\AgdaSpace{}%
\AgdaInductiveConstructor{opHash}\AgdaSpace{}%
\AgdaOperator{\AgdaInductiveConstructor{∷}}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaInductiveConstructor{opPush}\AgdaSpace{}%
\AgdaBound{pbkh}\AgdaSymbol{)}\AgdaSpace{}%
\AgdaOperator{\AgdaInductiveConstructor{∷}}\AgdaSpace{}%
\AgdaInductiveConstructor{opEqual}\AgdaSpace{}%
\AgdaOperator{\AgdaInductiveConstructor{∷}}\AgdaSpace{}%
\AgdaInductiveConstructor{opVerify}\AgdaSpace{}%
\AgdaOperator{\AgdaInductiveConstructor{∷}}\AgdaSpace{}%
\AgdaInductiveConstructor{opCheckSig}\AgdaSpace{}%
\AgdaOperator{\AgdaInductiveConstructor{∷}}\AgdaSpace{}%
\AgdaInductiveConstructor{[]}\<%
\\
%
\\[\AgdaEmptyExtraSkip]%
\>[0]\AgdaFunction{weakestPreConditionP2PKHˢ}\AgdaSpace{}%
\AgdaSymbol{:}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaBound{pbkh}\AgdaSpace{}%
\AgdaSymbol{:}\AgdaSpace{}%
\AgdaDatatype{ℕ}\AgdaSymbol{)}\AgdaSpace{}%
\AgdaSymbol{→}\AgdaSpace{}%
\AgdaFunction{StackPredicate}\<%
\\
\>[0]\AgdaFunction{weakestPreConditionP2PKHˢ}\AgdaSpace{}%
\AgdaSymbol{=}\AgdaSpace{}%
\AgdaFunction{wPreCondP2PKHˢ}\<%
\end{code}
} % END AgdaHide


==> latex-before-sed/verificationStackScripts/sPredicate.tex <==
%% This file has been generated automatically by mkLagda.awk
%% DO NOT EDIT! ALL YOUR CHANGES WILL BE LOST!

\AgdaHide{
\begin{code}%
\>[0]\AgdaKeyword{open}\AgdaSpace{}%
\AgdaKeyword{import}\AgdaSpace{}%
\AgdaModule{basicBitcoinDataType}\<%
\\
%
\\[\AgdaEmptyExtraSkip]%
\>[0]\AgdaKeyword{module}\AgdaSpace{}%
\AgdaModule{verificationStackScripts.sPredicate}\AgdaSpace{}%
\AgdaKeyword{where}\<%
\\
%
\\[\AgdaEmptyExtraSkip]%
\>[0]\AgdaKeyword{open}\AgdaSpace{}%
\AgdaKeyword{import}\AgdaSpace{}%
\AgdaModule{Data.Nat}%
\>[22]\AgdaKeyword{hiding}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaOperator{\AgdaDatatype{\AgdaUnderscore{}≤\AgdaUnderscore{}}}\AgdaSymbol{)}\<%
\\
\>[0]\AgdaKeyword{open}\AgdaSpace{}%
\AgdaKeyword{import}\AgdaSpace{}%
\AgdaModule{Data.List}\AgdaSpace{}%
\AgdaKeyword{hiding}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaOperator{\AgdaFunction{\AgdaUnderscore{}++\AgdaUnderscore{}}}\AgdaSymbol{)}\<%
\\
\>[0]\AgdaKeyword{open}\AgdaSpace{}%
\AgdaKeyword{import}\AgdaSpace{}%
\AgdaModule{Data.Unit}%
\>[23]\AgdaKeyword{hiding}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaOperator{\AgdaRecord{\AgdaUnderscore{}≤\AgdaUnderscore{}}}\AgdaSymbol{)}\<%
\\
\>[0]\AgdaKeyword{open}\AgdaSpace{}%
\AgdaKeyword{import}\AgdaSpace{}%
\AgdaModule{Data.Empty}\<%
\\
\>[0]\AgdaKeyword{open}\AgdaSpace{}%
\AgdaKeyword{import}\AgdaSpace{}%
\AgdaModule{Data.Sum}\<%
\\
\>[0]\AgdaKeyword{open}\AgdaSpace{}%
\AgdaKeyword{import}\AgdaSpace{}%
\AgdaModule{Data.Maybe}\<%
\\
\>[0]\AgdaKeyword{open}\AgdaSpace{}%
\AgdaKeyword{import}\AgdaSpace{}%
\AgdaModule{Data.Bool}%
\>[23]\AgdaKeyword{hiding}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaOperator{\AgdaDatatype{\AgdaUnderscore{}≤\AgdaUnderscore{}}}\AgdaSpace{}%
\AgdaSymbol{;}\AgdaSpace{}%
\AgdaOperator{\AgdaFunction{if\AgdaUnderscore{}then\AgdaUnderscore{}else\AgdaUnderscore{}}}\AgdaSpace{}%
\AgdaSymbol{)}\AgdaSpace{}%
\AgdaKeyword{renaming}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaOperator{\AgdaFunction{\AgdaUnderscore{}∧\AgdaUnderscore{}}}\AgdaSpace{}%
\AgdaSymbol{to}\AgdaSpace{}%
\AgdaOperator{\AgdaFunction{\AgdaUnderscore{}∧b\AgdaUnderscore{}}}\AgdaSpace{}%
\AgdaSymbol{;}\AgdaSpace{}%
\AgdaOperator{\AgdaFunction{\AgdaUnderscore{}∨\AgdaUnderscore{}}}\AgdaSpace{}%
\AgdaSymbol{to}\AgdaSpace{}%
\AgdaOperator{\AgdaFunction{\AgdaUnderscore{}∨b\AgdaUnderscore{}}}\AgdaSpace{}%
\AgdaSymbol{;}\AgdaSpace{}%
\AgdaFunction{T}\AgdaSpace{}%
\AgdaSymbol{to}\AgdaSpace{}%
\AgdaFunction{True}\AgdaSymbol{)}\<%
\\
\>[0]\AgdaKeyword{open}\AgdaSpace{}%
\AgdaKeyword{import}\AgdaSpace{}%
\AgdaModule{Data.Bool.Base}\AgdaSpace{}%
\AgdaKeyword{hiding}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaOperator{\AgdaDatatype{\AgdaUnderscore{}≤\AgdaUnderscore{}}}\AgdaSpace{}%
\AgdaSymbol{;}\AgdaSpace{}%
\AgdaOperator{\AgdaFunction{if\AgdaUnderscore{}then\AgdaUnderscore{}else\AgdaUnderscore{}}}\AgdaSpace{}%
\AgdaSymbol{)}\AgdaSpace{}%
\AgdaKeyword{renaming}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaOperator{\AgdaFunction{\AgdaUnderscore{}∧\AgdaUnderscore{}}}\AgdaSpace{}%
\AgdaSymbol{to}\AgdaSpace{}%
\AgdaOperator{\AgdaFunction{\AgdaUnderscore{}∧b\AgdaUnderscore{}}}\AgdaSpace{}%
\AgdaSymbol{;}\AgdaSpace{}%
\AgdaOperator{\AgdaFunction{\AgdaUnderscore{}∨\AgdaUnderscore{}}}\AgdaSpace{}%
\AgdaSymbol{to}\AgdaSpace{}%
\AgdaOperator{\AgdaFunction{\AgdaUnderscore{}∨b\AgdaUnderscore{}}}\AgdaSpace{}%
\AgdaSymbol{;}\AgdaSpace{}%
\AgdaFunction{T}\AgdaSpace{}%
\AgdaSymbol{to}\AgdaSpace{}%
\AgdaFunction{True}\AgdaSymbol{)}\<%
\\
\>[0]\AgdaKeyword{open}\AgdaSpace{}%
\AgdaKeyword{import}\AgdaSpace{}%
\AgdaModule{Data.Product}\AgdaSpace{}%
\AgdaKeyword{renaming}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaOperator{\AgdaInductiveConstructor{\AgdaUnderscore{},\AgdaUnderscore{}}}\AgdaSpace{}%
\AgdaSymbol{to}\AgdaSpace{}%
\AgdaOperator{\AgdaInductiveConstructor{\AgdaUnderscore{},,\AgdaUnderscore{}}}\AgdaSpace{}%
\AgdaSymbol{)}\<%
\\
\>[0]\AgdaKeyword{open}\AgdaSpace{}%
\AgdaKeyword{import}\AgdaSpace{}%
\AgdaModule{Data.Nat.Base}\AgdaSpace{}%
\AgdaKeyword{hiding}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaOperator{\AgdaDatatype{\AgdaUnderscore{}≤\AgdaUnderscore{}}}\AgdaSymbol{)}\<%
\\
\>[0]\AgdaKeyword{open}\AgdaSpace{}%
\AgdaKeyword{import}\AgdaSpace{}%
\AgdaModule{Data.List.NonEmpty}\AgdaSpace{}%
\AgdaKeyword{hiding}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaField{head}\AgdaSymbol{)}\<%
\\
\>[0]\AgdaKeyword{import}\AgdaSpace{}%
\AgdaModule{Relation.Binary.PropositionalEquality}\AgdaSpace{}%
\AgdaSymbol{as}\AgdaSpace{}%
\AgdaModule{Eq}\<%
\\
\>[0]\AgdaKeyword{open}\AgdaSpace{}%
\AgdaModule{Eq}\AgdaSpace{}%
\AgdaKeyword{using}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaOperator{\AgdaDatatype{\AgdaUnderscore{}≡\AgdaUnderscore{}}}\AgdaSymbol{;}\AgdaSpace{}%
\AgdaInductiveConstructor{refl}\AgdaSymbol{;}\AgdaSpace{}%
\AgdaFunction{cong}\AgdaSymbol{;}\AgdaSpace{}%
\AgdaKeyword{module}\AgdaSpace{}%
\AgdaModule{≡-Reasoning}\AgdaSymbol{;}\AgdaSpace{}%
\AgdaFunction{sym}\AgdaSymbol{)}\<%
\\
\>[0]\AgdaKeyword{open}\AgdaSpace{}%
\AgdaModule{≡-Reasoning}\<%
\\
\>[0]\AgdaKeyword{open}\AgdaSpace{}%
\AgdaKeyword{import}\AgdaSpace{}%
\AgdaModule{Agda.Builtin.Equality}\<%
\\
%
\\[\AgdaEmptyExtraSkip]%
%
\\[\AgdaEmptyExtraSkip]%
%
\\[\AgdaEmptyExtraSkip]%
\>[0]\AgdaComment{--our\ libraries}\<%
\\
%
\\[\AgdaEmptyExtraSkip]%
\>[0]\AgdaKeyword{open}\AgdaSpace{}%
\AgdaKeyword{import}\AgdaSpace{}%
\AgdaModule{libraries.listLib}\<%
\\
\>[0]\AgdaKeyword{open}\AgdaSpace{}%
\AgdaKeyword{import}\AgdaSpace{}%
\AgdaModule{libraries.natLib}\<%
\\
\>[0]\AgdaKeyword{open}\AgdaSpace{}%
\AgdaKeyword{import}\AgdaSpace{}%
\AgdaModule{libraries.boolLib}\<%
\\
\>[0]\AgdaKeyword{open}\AgdaSpace{}%
\AgdaKeyword{import}\AgdaSpace{}%
\AgdaModule{libraries.andLib}\<%
\\
\>[0]\AgdaKeyword{open}\AgdaSpace{}%
\AgdaKeyword{import}\AgdaSpace{}%
\AgdaModule{libraries.miscLib}\<%
\\
\>[0]\AgdaKeyword{open}\AgdaSpace{}%
\AgdaKeyword{import}\AgdaSpace{}%
\AgdaModule{libraries.maybeLib}\<%
\\
%
\\[\AgdaEmptyExtraSkip]%
%
\\[\AgdaEmptyExtraSkip]%
\>[0]\AgdaKeyword{open}\AgdaSpace{}%
\AgdaKeyword{import}\AgdaSpace{}%
\AgdaModule{stack}\<%
\\
\>[0]\AgdaKeyword{open}\AgdaSpace{}%
\AgdaKeyword{import}\AgdaSpace{}%
\AgdaModule{stackPredicate}\<%
\\
\>[0]\AgdaKeyword{open}\AgdaSpace{}%
\AgdaKeyword{import}\AgdaSpace{}%
\AgdaModule{verificationStackScripts.stackState}\<%
\\
%
\\[\AgdaEmptyExtraSkip]%
%
\\[\AgdaEmptyExtraSkip]%
%
\\[\AgdaEmptyExtraSkip]%
\>[0]\AgdaComment{--\ Boolean\ valued\ Stack\ Predicate}\<%
\end{code}
} % END AgdaHide

\newcommand{\sPredicatettt}{
\begin{code}%
\>[0]\AgdaFunction{BStackStatePred}%
\>[17]\AgdaSymbol{:}\AgdaSpace{}%
\AgdaPrimitive{Set}\<%
\\
\>[0]\AgdaFunction{BStackStatePred}\AgdaSpace{}%
\AgdaSymbol{=}%
\>[19]\AgdaRecord{StackState}\AgdaSpace{}%
\AgdaSymbol{→}%
\>[33]\AgdaDatatype{Bool}\<%
\end{code}
} % END newcommand

\AgdaHide{
\begin{code}%
\>[0]\<%
\\
%
\\[\AgdaEmptyExtraSkip]%
\>[0]\AgdaFunction{MaybeBStackStatePred}\AgdaSpace{}%
\AgdaSymbol{:}\AgdaSpace{}%
\AgdaPrimitive{Set}\<%
\\
\>[0]\AgdaFunction{MaybeBStackStatePred}\AgdaSpace{}%
\AgdaSymbol{=}\AgdaSpace{}%
\AgdaDatatype{Maybe}\AgdaSpace{}%
\AgdaRecord{StackState}\AgdaSpace{}%
\AgdaSymbol{→}%
\>[43]\AgdaDatatype{Bool}\<%
\\
%
\\[\AgdaEmptyExtraSkip]%
%
\\[\AgdaEmptyExtraSkip]%
\>[0]\AgdaComment{--\ Stack\ Predicate}\<%
\\
\>[0]\AgdaFunction{StackStatePred}\AgdaSpace{}%
\AgdaSymbol{:}\AgdaSpace{}%
\AgdaPrimitive{Set₁}\<%
\\
\>[0]\AgdaComment{--\textbackslash{}sPredicatestackstatepred}\<%
\end{code}
} % END AgdaHide

\newcommand{\sPredicatestackstatepred}{
\begin{code}[inline]%
\>[0]\AgdaFunction{StackStatePred}\AgdaSpace{}%
\AgdaSymbol{=}\AgdaSpace{}%
\AgdaRecord{StackState}\AgdaSpace{}%
\AgdaSymbol{→}\AgdaSpace{}%
\AgdaPrimitive{Set}\<%
\end{code}
} % END newcommand

\AgdaHide{
\begin{code}%
\>[0]\<%
\\
%
\\[\AgdaEmptyExtraSkip]%
%
\\[\AgdaEmptyExtraSkip]%
\>[0]\AgdaFunction{predicateAfterPushingx}\AgdaSpace{}%
\AgdaSymbol{:}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaBound{n}\AgdaSpace{}%
\AgdaSymbol{:}\AgdaSpace{}%
\AgdaDatatype{ℕ}\AgdaSymbol{)(}\AgdaBound{φ}\AgdaSpace{}%
\AgdaSymbol{:}\AgdaSpace{}%
\AgdaFunction{StackStatePred}\AgdaSymbol{)}\AgdaSpace{}%
\AgdaSymbol{→}\AgdaSpace{}%
\AgdaFunction{StackStatePred}\<%
\\
\>[0]\AgdaFunction{predicateAfterPushingx}\AgdaSpace{}%
\AgdaBound{n}\AgdaSpace{}%
\AgdaBound{φ}\AgdaSpace{}%
\AgdaOperator{\AgdaInductiveConstructor{⟨}}\AgdaSpace{}%
\AgdaBound{time}\AgdaSpace{}%
\AgdaOperator{\AgdaInductiveConstructor{,}}\AgdaSpace{}%
\AgdaBound{msg₁}\AgdaSpace{}%
\AgdaOperator{\AgdaInductiveConstructor{,}}\AgdaSpace{}%
\AgdaBound{stack₁}\AgdaSpace{}%
\AgdaOperator{\AgdaInductiveConstructor{⟩}}\AgdaSpace{}%
\AgdaSymbol{=}\AgdaSpace{}%
\AgdaBound{φ}\AgdaSpace{}%
\AgdaOperator{\AgdaInductiveConstructor{⟨}}\AgdaSpace{}%
\AgdaBound{time}\AgdaSpace{}%
\AgdaOperator{\AgdaInductiveConstructor{,}}\AgdaSpace{}%
\AgdaBound{msg₁}\AgdaSpace{}%
\AgdaOperator{\AgdaInductiveConstructor{,}}\AgdaSpace{}%
\AgdaBound{n}\AgdaSpace{}%
\AgdaOperator{\AgdaInductiveConstructor{∷}}\AgdaSpace{}%
\AgdaBound{stack₁}\AgdaSpace{}%
\AgdaOperator{\AgdaInductiveConstructor{⟩}}\<%
\\
%
\\[\AgdaEmptyExtraSkip]%
%
\\[\AgdaEmptyExtraSkip]%
\>[0]\AgdaFunction{predicateForTopElOfStack}\AgdaSpace{}%
\AgdaSymbol{:}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaBound{n}\AgdaSpace{}%
\AgdaSymbol{:}\AgdaSpace{}%
\AgdaDatatype{ℕ}\AgdaSymbol{)}\AgdaSpace{}%
\AgdaSymbol{→}\AgdaSpace{}%
\AgdaFunction{StackStatePred}\<%
\\
\>[0]\AgdaFunction{predicateForTopElOfStack}\AgdaSpace{}%
\AgdaBound{n}\AgdaSpace{}%
\AgdaOperator{\AgdaInductiveConstructor{⟨}}\AgdaSpace{}%
\AgdaBound{time}\AgdaSpace{}%
\AgdaOperator{\AgdaInductiveConstructor{,}}\AgdaSpace{}%
\AgdaBound{msg₁}\AgdaSpace{}%
\AgdaOperator{\AgdaInductiveConstructor{,}}\AgdaSpace{}%
\AgdaInductiveConstructor{[]}\AgdaSpace{}%
\AgdaOperator{\AgdaInductiveConstructor{⟩}}\AgdaSpace{}%
\AgdaSymbol{=}\AgdaSpace{}%
\AgdaDatatype{⊥}\<%
\\
\>[0]\AgdaFunction{predicateForTopElOfStack}\AgdaSpace{}%
\AgdaBound{n}\AgdaSpace{}%
\AgdaOperator{\AgdaInductiveConstructor{⟨}}\AgdaSpace{}%
\AgdaBound{time}\AgdaSpace{}%
\AgdaOperator{\AgdaInductiveConstructor{,}}\AgdaSpace{}%
\AgdaBound{msg₁}\AgdaSpace{}%
\AgdaOperator{\AgdaInductiveConstructor{,}}\AgdaSpace{}%
\AgdaBound{x}\AgdaSpace{}%
\AgdaOperator{\AgdaInductiveConstructor{∷}}\AgdaSpace{}%
\AgdaBound{stack₁}\AgdaSpace{}%
\AgdaOperator{\AgdaInductiveConstructor{⟩}}\AgdaSpace{}%
\AgdaSymbol{=}\AgdaSpace{}%
\AgdaBound{x}\AgdaSpace{}%
\AgdaOperator{\AgdaDatatype{≡}}\AgdaSpace{}%
\AgdaBound{n}\<%
\\
%
\\[\AgdaEmptyExtraSkip]%
%
\\[\AgdaEmptyExtraSkip]%
%
\\[\AgdaEmptyExtraSkip]%
\>[0]\AgdaOperator{\AgdaFunction{\AgdaUnderscore{}∧p\AgdaUnderscore{}}}\AgdaSpace{}%
\AgdaSymbol{:}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaSpace{}%
\AgdaBound{φ}\AgdaSpace{}%
\AgdaBound{ψ}%
\>[14]\AgdaSymbol{:}\AgdaSpace{}%
\AgdaFunction{StackStatePred}\AgdaSpace{}%
\AgdaSymbol{)}\AgdaSpace{}%
\AgdaSymbol{→}\AgdaSpace{}%
\AgdaFunction{StackStatePred}\<%
\\
\>[0]\AgdaSymbol{(}\AgdaBound{φ}\AgdaSpace{}%
\AgdaOperator{\AgdaFunction{∧p}}\AgdaSpace{}%
\AgdaBound{ψ}\AgdaSpace{}%
\AgdaSymbol{)}\AgdaSpace{}%
\AgdaBound{s}%
\>[13]\AgdaSymbol{=}%
\>[16]\AgdaBound{φ}\AgdaSpace{}%
\AgdaBound{s}%
\>[21]\AgdaOperator{\AgdaRecord{∧}}%
\>[24]\AgdaBound{ψ}\AgdaSpace{}%
\AgdaBound{s}\<%
\\
%
\\[\AgdaEmptyExtraSkip]%
%
\\[\AgdaEmptyExtraSkip]%
%
\\[\AgdaEmptyExtraSkip]%
\>[0]\AgdaFunction{⊥p}\AgdaSpace{}%
\AgdaSymbol{:}\AgdaSpace{}%
\AgdaFunction{StackStatePred}\<%
\\
\>[0]\AgdaFunction{⊥p}\AgdaSpace{}%
\AgdaBound{s}\AgdaSpace{}%
\AgdaSymbol{=}\AgdaSpace{}%
\AgdaDatatype{⊥}\<%
\\
%
\\[\AgdaEmptyExtraSkip]%
\>[0]\AgdaKeyword{infixl}\AgdaSpace{}%
\AgdaNumber{4}\AgdaSpace{}%
\AgdaOperator{\AgdaFunction{\AgdaUnderscore{}⊎p\AgdaUnderscore{}}}\<%
\\
%
\\[\AgdaEmptyExtraSkip]%
\>[0]\AgdaOperator{\AgdaFunction{\AgdaUnderscore{}⊎p\AgdaUnderscore{}}}%
\>[7]\AgdaSymbol{:}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaBound{φ}\AgdaSpace{}%
\AgdaBound{ψ}\AgdaSpace{}%
\AgdaSymbol{:}\AgdaSpace{}%
\AgdaFunction{StackStatePred}\AgdaSymbol{)}\AgdaSpace{}%
\AgdaSymbol{→}\AgdaSpace{}%
\AgdaFunction{StackStatePred}\<%
\\
\>[0]\AgdaSymbol{(}\AgdaBound{φ}\AgdaSpace{}%
\AgdaOperator{\AgdaFunction{⊎p}}\AgdaSpace{}%
\AgdaBound{ψ}\AgdaSymbol{)}\AgdaSpace{}%
\AgdaBound{s}\AgdaSpace{}%
\AgdaSymbol{=}\AgdaSpace{}%
\AgdaBound{φ}\AgdaSpace{}%
\AgdaBound{s}\AgdaSpace{}%
\AgdaOperator{\AgdaDatatype{⊎}}\AgdaSpace{}%
\AgdaBound{ψ}\AgdaSpace{}%
\AgdaBound{s}\<%
\\
%
\\[\AgdaEmptyExtraSkip]%
%
\\[\AgdaEmptyExtraSkip]%
%
\\[\AgdaEmptyExtraSkip]%
\>[0]\AgdaFunction{lemma⊎pleft}\AgdaSpace{}%
\AgdaSymbol{:}%
\>[214I]\AgdaSymbol{(}\AgdaBound{ψ}\AgdaSpace{}%
\AgdaBound{ψ'}\AgdaSpace{}%
\AgdaSymbol{:}\AgdaSpace{}%
\AgdaFunction{StackStatePred}\AgdaSymbol{)(}\AgdaBound{s}\AgdaSpace{}%
\AgdaSymbol{:}\AgdaSpace{}%
\AgdaDatatype{Maybe}\AgdaSpace{}%
\AgdaRecord{StackState}\AgdaSymbol{)}\<%
\\
\>[.][@{}l@{}]\<[214I]%
\>[14]\AgdaSymbol{→}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaBound{ψ}\AgdaSpace{}%
\AgdaOperator{\AgdaFunction{⁺}}\AgdaSymbol{)}\AgdaSpace{}%
\AgdaBound{s}\AgdaSpace{}%
\AgdaSymbol{→}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaBound{ψ}\AgdaSpace{}%
\AgdaOperator{\AgdaFunction{⊎p}}\AgdaSpace{}%
\AgdaBound{ψ'}\AgdaSymbol{)}\AgdaSpace{}%
\AgdaOperator{\AgdaFunction{⁺}}\AgdaSymbol{)}\AgdaSpace{}%
\AgdaBound{s}\<%
\\
\>[0]\AgdaFunction{lemma⊎pleft}\AgdaSpace{}%
\AgdaBound{ψ}\AgdaSpace{}%
\AgdaBound{ψ'}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaInductiveConstructor{just}\AgdaSpace{}%
\AgdaBound{x}\AgdaSymbol{)}\AgdaSpace{}%
\AgdaBound{p}\AgdaSpace{}%
\AgdaSymbol{=}\AgdaSpace{}%
\AgdaInductiveConstructor{inj₁}\AgdaSpace{}%
\AgdaBound{p}\<%
\\
%
\\[\AgdaEmptyExtraSkip]%
\>[0]\AgdaFunction{lemma⊎pright}\AgdaSpace{}%
\AgdaSymbol{:}%
\>[240I]\AgdaSymbol{(}\AgdaBound{ψ}\AgdaSpace{}%
\AgdaBound{ψ'}\AgdaSpace{}%
\AgdaSymbol{:}\AgdaSpace{}%
\AgdaFunction{StackStatePred}\AgdaSymbol{)}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaBound{s}\AgdaSpace{}%
\AgdaSymbol{:}\AgdaSpace{}%
\AgdaDatatype{Maybe}\AgdaSpace{}%
\AgdaRecord{StackState}\AgdaSymbol{)}\<%
\\
\>[.][@{}l@{}]\<[240I]%
\>[15]\AgdaSymbol{→}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaBound{ψ'}\AgdaSpace{}%
\AgdaOperator{\AgdaFunction{⁺}}\AgdaSymbol{)}\AgdaSpace{}%
\AgdaBound{s}\AgdaSpace{}%
\AgdaSymbol{→}\AgdaSpace{}%
\AgdaSymbol{((}\AgdaSpace{}%
\AgdaBound{ψ}\AgdaSpace{}%
\AgdaOperator{\AgdaFunction{⊎p}}\AgdaSpace{}%
\AgdaBound{ψ'}\AgdaSpace{}%
\AgdaSymbol{)}\AgdaSpace{}%
\AgdaOperator{\AgdaFunction{⁺}}\AgdaSpace{}%
\AgdaSymbol{)}\AgdaSpace{}%
\AgdaBound{s}\<%
\\
\>[0]\AgdaFunction{lemma⊎pright}%
\>[14]\AgdaBound{ψ}\AgdaSpace{}%
\AgdaBound{ψ'}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaInductiveConstructor{just}\AgdaSpace{}%
\AgdaBound{x}\AgdaSymbol{)}\AgdaSpace{}%
\AgdaBound{p}\AgdaSpace{}%
\AgdaSymbol{=}\AgdaSpace{}%
\AgdaInductiveConstructor{inj₂}\AgdaSpace{}%
\AgdaBound{p}\<%
\\
%
\\[\AgdaEmptyExtraSkip]%
\>[0]\AgdaFunction{lemma⊎pinv}\AgdaSpace{}%
\AgdaSymbol{:}%
\>[268I]\AgdaSymbol{(}\AgdaBound{ψ}\AgdaSpace{}%
\AgdaBound{ψ'}\AgdaSpace{}%
\AgdaSymbol{:}\AgdaSpace{}%
\AgdaFunction{StackStatePred}\AgdaSymbol{)(}\AgdaBound{A}\AgdaSpace{}%
\AgdaSymbol{:}\AgdaSpace{}%
\AgdaPrimitive{Set}\AgdaSymbol{)}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaBound{s}\AgdaSpace{}%
\AgdaSymbol{:}\AgdaSpace{}%
\AgdaDatatype{Maybe}\AgdaSpace{}%
\AgdaRecord{StackState}\AgdaSymbol{)}\<%
\\
\>[.][@{}l@{}]\<[268I]%
\>[13]\AgdaSymbol{→}\AgdaSpace{}%
\AgdaSymbol{((}\AgdaBound{ψ}\AgdaSpace{}%
\AgdaOperator{\AgdaFunction{⁺}}\AgdaSymbol{)}\AgdaSpace{}%
\AgdaBound{s}%
\>[25]\AgdaSymbol{→}\AgdaSpace{}%
\AgdaBound{A}\AgdaSymbol{)}\<%
\\
%
\>[13]\AgdaSymbol{→}\AgdaSpace{}%
\AgdaSymbol{((}\AgdaBound{ψ'}\AgdaSpace{}%
\AgdaOperator{\AgdaFunction{⁺}}\AgdaSymbol{)}\AgdaSpace{}%
\AgdaBound{s}%
\>[26]\AgdaSymbol{→}\AgdaSpace{}%
\AgdaBound{A}\AgdaSymbol{)}\<%
\\
%
\>[13]\AgdaSymbol{→}%
\>[16]\AgdaSymbol{((}\AgdaBound{ψ}\AgdaSpace{}%
\AgdaOperator{\AgdaFunction{⊎p}}\AgdaSpace{}%
\AgdaBound{ψ'}\AgdaSymbol{)}\AgdaSpace{}%
\AgdaOperator{\AgdaFunction{⁺}}\AgdaSymbol{)}\AgdaSpace{}%
\AgdaBound{s}\AgdaSpace{}%
\AgdaSymbol{→}\AgdaSpace{}%
\AgdaBound{A}\<%
\\
\>[0]\AgdaFunction{lemma⊎pinv}\AgdaSpace{}%
\AgdaBound{ψ}\AgdaSpace{}%
\AgdaBound{ψ'}\AgdaSpace{}%
\AgdaBound{A}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaInductiveConstructor{just}\AgdaSpace{}%
\AgdaBound{x}\AgdaSymbol{)}\AgdaSpace{}%
\AgdaBound{p}\AgdaSpace{}%
\AgdaBound{q}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaInductiveConstructor{inj₁}\AgdaSpace{}%
\AgdaBound{x₁}\AgdaSymbol{)}\AgdaSpace{}%
\AgdaSymbol{=}\AgdaSpace{}%
\AgdaBound{p}\AgdaSpace{}%
\AgdaBound{x₁}\<%
\\
\>[0]\AgdaFunction{lemma⊎pinv}\AgdaSpace{}%
\AgdaBound{ψ}\AgdaSpace{}%
\AgdaBound{ψ'}\AgdaSpace{}%
\AgdaBound{A}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaInductiveConstructor{just}\AgdaSpace{}%
\AgdaBound{x}\AgdaSymbol{)}\AgdaSpace{}%
\AgdaBound{p}\AgdaSpace{}%
\AgdaBound{q}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaInductiveConstructor{inj₂}\AgdaSpace{}%
\AgdaBound{y}\AgdaSymbol{)}\AgdaSpace{}%
\AgdaSymbol{=}\AgdaSpace{}%
\AgdaBound{q}\AgdaSpace{}%
\AgdaBound{y}\<%
\\
%
\\[\AgdaEmptyExtraSkip]%
%
\\[\AgdaEmptyExtraSkip]%
%
\\[\AgdaEmptyExtraSkip]%
%
\\[\AgdaEmptyExtraSkip]%
\>[0]\AgdaFunction{stackPred2SPred}\AgdaSpace{}%
\AgdaSymbol{:}\AgdaSpace{}%
\AgdaFunction{StackPredicate}\AgdaSpace{}%
\AgdaSymbol{→}\AgdaSpace{}%
\AgdaFunction{StackStatePred}\<%
\\
\>[0]\AgdaFunction{stackPred2SPred}\AgdaSpace{}%
\AgdaBound{f}\AgdaSpace{}%
\AgdaOperator{\AgdaInductiveConstructor{⟨}}\AgdaSpace{}%
\AgdaBound{time}\AgdaSpace{}%
\AgdaOperator{\AgdaInductiveConstructor{,}}\AgdaSpace{}%
\AgdaBound{msg₁}\AgdaSpace{}%
\AgdaOperator{\AgdaInductiveConstructor{,}}\AgdaSpace{}%
\AgdaBound{stack₁}\AgdaSpace{}%
\AgdaOperator{\AgdaInductiveConstructor{⟩}}\AgdaSpace{}%
\AgdaSymbol{=}\AgdaSpace{}%
\AgdaBound{f}\AgdaSpace{}%
\AgdaBound{time}\AgdaSpace{}%
\AgdaBound{msg₁}\AgdaSpace{}%
\AgdaBound{stack₁}\<%
\\
%
\\[\AgdaEmptyExtraSkip]%
%
\\[\AgdaEmptyExtraSkip]%
%
\\[\AgdaEmptyExtraSkip]%
\>[0]\AgdaFunction{stackPred2SPredBool}\AgdaSpace{}%
\AgdaSymbol{:}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaSpace{}%
\AgdaFunction{Time}\AgdaSpace{}%
\AgdaSymbol{→}\AgdaSpace{}%
\AgdaDatatype{Msg}\AgdaSpace{}%
\AgdaSymbol{→}\AgdaSpace{}%
\AgdaFunction{Stack}\AgdaSpace{}%
\AgdaSymbol{→}\AgdaSpace{}%
\AgdaDatatype{Bool}\AgdaSpace{}%
\AgdaSymbol{)}\AgdaSpace{}%
\AgdaSymbol{→}\AgdaSpace{}%
\AgdaSymbol{(}%
\>[57]\AgdaRecord{StackState}\AgdaSpace{}%
\AgdaSymbol{→}%
\>[71]\AgdaDatatype{Bool}\AgdaSpace{}%
\AgdaSymbol{)}\<%
\\
\>[0]\AgdaFunction{stackPred2SPredBool}\AgdaSpace{}%
\AgdaBound{f}\AgdaSpace{}%
\AgdaOperator{\AgdaInductiveConstructor{⟨}}\AgdaSpace{}%
\AgdaBound{currentTime₁}\AgdaSpace{}%
\AgdaOperator{\AgdaInductiveConstructor{,}}\AgdaSpace{}%
\AgdaBound{msg₁}\AgdaSpace{}%
\AgdaOperator{\AgdaInductiveConstructor{,}}\AgdaSpace{}%
\AgdaBound{stack₁}\AgdaSpace{}%
\AgdaOperator{\AgdaInductiveConstructor{⟩}}\<%
\\
\>[0][@{}l@{\AgdaIndent{0}}]%
\>[14]\AgdaSymbol{=}\AgdaSpace{}%
\AgdaBound{f}\AgdaSpace{}%
\AgdaBound{currentTime₁}\AgdaSpace{}%
\AgdaBound{msg₁}\AgdaSpace{}%
\AgdaBound{stack₁}\<%
\\
%
\\[\AgdaEmptyExtraSkip]%
%
\\[\AgdaEmptyExtraSkip]%
%
\\[\AgdaEmptyExtraSkip]%
\>[0]\AgdaFunction{topElStack=0}\AgdaSpace{}%
\AgdaSymbol{:}\AgdaSpace{}%
\AgdaFunction{StackStatePred}\<%
\\
\>[0]\AgdaFunction{topElStack=0}\AgdaSpace{}%
\AgdaOperator{\AgdaInductiveConstructor{⟨}}\AgdaSpace{}%
\AgdaBound{time}\AgdaSpace{}%
\AgdaOperator{\AgdaInductiveConstructor{,}}\AgdaSpace{}%
\AgdaBound{msg₁}\AgdaSpace{}%
\AgdaOperator{\AgdaInductiveConstructor{,}}\AgdaSpace{}%
\AgdaInductiveConstructor{[]}\AgdaSpace{}%
\AgdaOperator{\AgdaInductiveConstructor{⟩}}\AgdaSpace{}%
\AgdaSymbol{=}\AgdaSpace{}%
\AgdaDatatype{⊥}\<%
\\
\>[0]\AgdaFunction{topElStack=0}\AgdaSpace{}%
\AgdaOperator{\AgdaInductiveConstructor{⟨}}\AgdaSpace{}%
\AgdaBound{time}\AgdaSpace{}%
\AgdaOperator{\AgdaInductiveConstructor{,}}\AgdaSpace{}%
\AgdaBound{msg₁}\AgdaSpace{}%
\AgdaOperator{\AgdaInductiveConstructor{,}}\AgdaSpace{}%
\AgdaInductiveConstructor{zero}\AgdaSpace{}%
\AgdaOperator{\AgdaInductiveConstructor{∷}}\AgdaSpace{}%
\AgdaBound{stack₁}\AgdaSpace{}%
\AgdaOperator{\AgdaInductiveConstructor{⟩}}\AgdaSpace{}%
\AgdaSymbol{=}\AgdaSpace{}%
\AgdaRecord{⊤}\<%
\\
\>[0]\AgdaFunction{topElStack=0}\AgdaSpace{}%
\AgdaOperator{\AgdaInductiveConstructor{⟨}}\AgdaSpace{}%
\AgdaBound{time}\AgdaSpace{}%
\AgdaOperator{\AgdaInductiveConstructor{,}}\AgdaSpace{}%
\AgdaBound{msg₁}\AgdaSpace{}%
\AgdaOperator{\AgdaInductiveConstructor{,}}\AgdaSpace{}%
\AgdaInductiveConstructor{suc}\AgdaSpace{}%
\AgdaBound{x}\AgdaSpace{}%
\AgdaOperator{\AgdaInductiveConstructor{∷}}\AgdaSpace{}%
\AgdaBound{stack₁}\AgdaSpace{}%
\AgdaOperator{\AgdaInductiveConstructor{⟩}}\AgdaSpace{}%
\AgdaSymbol{=}\AgdaSpace{}%
\AgdaDatatype{⊥}\<%
\\
%
\\[\AgdaEmptyExtraSkip]%
%
\\[\AgdaEmptyExtraSkip]%
%
\\[\AgdaEmptyExtraSkip]%
\>[0]\AgdaFunction{truePred}\AgdaSpace{}%
\AgdaSymbol{:}\AgdaSpace{}%
\AgdaFunction{StackPredicate}\AgdaSpace{}%
\AgdaSymbol{→}\AgdaSpace{}%
\AgdaFunction{StackStatePred}\<%
\\
\>[0]\AgdaFunction{truePred}\AgdaSpace{}%
\AgdaBound{φ}\AgdaSpace{}%
\AgdaSymbol{=}\AgdaSpace{}%
\AgdaFunction{stackPred2SPred}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaFunction{truePredaux}%
\>[43]\AgdaBound{φ}\AgdaSymbol{)}\<%
\\
%
\\[\AgdaEmptyExtraSkip]%
%
\\[\AgdaEmptyExtraSkip]%
%
\\[\AgdaEmptyExtraSkip]%
\>[0]\AgdaFunction{falsePredaux}\AgdaSpace{}%
\AgdaSymbol{:}\AgdaSpace{}%
\AgdaFunction{StackPredicate}\AgdaSpace{}%
\AgdaSymbol{→}\AgdaSpace{}%
\AgdaFunction{StackPredicate}\<%
\\
\>[0]\AgdaFunction{falsePredaux}\AgdaSpace{}%
\AgdaBound{φ}\AgdaSpace{}%
\AgdaBound{time}\AgdaSpace{}%
\AgdaBound{msg}\AgdaSpace{}%
\AgdaInductiveConstructor{[]}\AgdaSpace{}%
\AgdaSymbol{=}\AgdaSpace{}%
\AgdaDatatype{⊥}\<%
\\
\>[0]\AgdaFunction{falsePredaux}\AgdaSpace{}%
\AgdaBound{φ}\AgdaSpace{}%
\AgdaBound{time}\AgdaSpace{}%
\AgdaBound{msg}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaInductiveConstructor{zero}\AgdaSpace{}%
\AgdaOperator{\AgdaInductiveConstructor{∷}}\AgdaSpace{}%
\AgdaBound{st}\AgdaSymbol{)}\AgdaSpace{}%
\AgdaSymbol{=}\AgdaSpace{}%
\AgdaBound{φ}\AgdaSpace{}%
\AgdaBound{time}\AgdaSpace{}%
\AgdaBound{msg}%
\>[50]\AgdaBound{st}\<%
\\
\>[0]\AgdaFunction{falsePredaux}\AgdaSpace{}%
\AgdaBound{φ}\AgdaSpace{}%
\AgdaBound{time}\AgdaSpace{}%
\AgdaBound{msg}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaInductiveConstructor{suc}\AgdaSpace{}%
\AgdaBound{x}\AgdaSpace{}%
\AgdaOperator{\AgdaInductiveConstructor{∷}}\AgdaSpace{}%
\AgdaBound{st}\AgdaSymbol{)}\AgdaSpace{}%
\AgdaSymbol{=}\AgdaSpace{}%
\AgdaDatatype{⊥}\<%
\\
%
\\[\AgdaEmptyExtraSkip]%
\>[0]\AgdaFunction{falsePred}\AgdaSpace{}%
\AgdaSymbol{:}\AgdaSpace{}%
\AgdaFunction{StackPredicate}\AgdaSpace{}%
\AgdaSymbol{→}\AgdaSpace{}%
\AgdaFunction{StackStatePred}\<%
\\
\>[0]\AgdaFunction{falsePred}\AgdaSpace{}%
\AgdaBound{φ}\AgdaSpace{}%
\AgdaSymbol{=}\AgdaSpace{}%
\AgdaFunction{stackPred2SPred}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaFunction{falsePredaux}%
\>[45]\AgdaBound{φ}\AgdaSymbol{)}\<%
\\
%
\\[\AgdaEmptyExtraSkip]%
%
\\[\AgdaEmptyExtraSkip]%
\>[0]\AgdaFunction{liftAddingx}\AgdaSpace{}%
\AgdaSymbol{:}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaBound{n}\AgdaSpace{}%
\AgdaSymbol{:}\AgdaSpace{}%
\AgdaDatatype{ℕ}\AgdaSymbol{)(}\AgdaSpace{}%
\AgdaBound{φ}\AgdaSpace{}%
\AgdaSymbol{:}\AgdaSpace{}%
\AgdaFunction{StackPredicate}\AgdaSpace{}%
\AgdaSymbol{)}\AgdaSpace{}%
\AgdaSymbol{→}%
\>[47]\AgdaFunction{StackStatePred}\<%
\\
\>[0]\AgdaFunction{liftAddingx}\AgdaSpace{}%
\AgdaBound{n}\AgdaSpace{}%
\AgdaBound{φ}\AgdaSpace{}%
\AgdaSymbol{=}\AgdaSpace{}%
\AgdaFunction{predicateAfterPushingx}\AgdaSpace{}%
\AgdaBound{n}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaFunction{stackPred2SPred}\AgdaSpace{}%
\AgdaBound{φ}\AgdaSymbol{)}\<%
\\
%
\\[\AgdaEmptyExtraSkip]%
%
\\[\AgdaEmptyExtraSkip]%
%
\\[\AgdaEmptyExtraSkip]%
\>[0]\AgdaComment{--\ acceptingState\ \ :\ BStackStatePred}\<%
\\
\>[0]\AgdaComment{--\ acceptingState\ \ =\ stackPred2SPredBool\ acceptingBasic}\<%
\\
%
\\[\AgdaEmptyExtraSkip]%
%
\\[\AgdaEmptyExtraSkip]%
\>[0]\AgdaComment{--\ acceptingMaybeState\ \ :\ MaybeBStackStatePred}\<%
\\
\>[0]\AgdaComment{--\ acceptingMaybeState\ \ =\ acceptingState\ ⁺ᵇ}\<%
\\
%
\\[\AgdaEmptyExtraSkip]%
%
\\[\AgdaEmptyExtraSkip]%
\>[0]\AgdaFunction{acceptState}\AgdaSpace{}%
\AgdaSymbol{:}\AgdaSpace{}%
\AgdaFunction{StackStatePred}\<%
\\
\>[0]\AgdaFunction{acceptState}\AgdaSpace{}%
\AgdaSymbol{=}\AgdaSpace{}%
\AgdaFunction{stackPred2SPred}\AgdaSpace{}%
\AgdaFunction{acceptStateˢ}\<%
\\
%
\\[\AgdaEmptyExtraSkip]%
\>[0]\AgdaComment{--\ AcceptingMaybeState\ :\ Maybe\ StackState\ →\ Set}\<%
\\
\>[0]\AgdaComment{--\ AcceptingMaybeState\ s\ =\ True\ (acceptingMaybeState\ s)}\<%
\end{code}
} % END AgdaHide


==> latex-before-sed/verificationStackScripts/semanticsStackInstructions.tex <==
%% This file has been generated automatically by mkLagda.awk
%% DO NOT EDIT! ALL YOUR CHANGES WILL BE LOST!

\AgdaHide{
\begin{code}%
\>[0]\AgdaKeyword{open}\AgdaSpace{}%
\AgdaKeyword{import}\AgdaSpace{}%
\AgdaModule{basicBitcoinDataType}\<%
\\
%
\\[\AgdaEmptyExtraSkip]%
\>[0]\AgdaKeyword{module}\AgdaSpace{}%
\AgdaModule{verificationStackScripts.semanticsStackInstructions}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaBound{param}\AgdaSpace{}%
\AgdaSymbol{:}\AgdaSpace{}%
\AgdaRecord{GlobalParameters}\AgdaSymbol{)}\AgdaSpace{}%
\AgdaKeyword{where}\<%
\\
%
\\[\AgdaEmptyExtraSkip]%
%
\\[\AgdaEmptyExtraSkip]%
%
\\[\AgdaEmptyExtraSkip]%
\>[0]\AgdaKeyword{open}\AgdaSpace{}%
\AgdaKeyword{import}\AgdaSpace{}%
\AgdaModule{Data.Nat}%
\>[22]\AgdaKeyword{hiding}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaOperator{\AgdaDatatype{\AgdaUnderscore{}≤\AgdaUnderscore{}}}\AgdaSymbol{)}\<%
\\
\>[0]\AgdaKeyword{open}\AgdaSpace{}%
\AgdaKeyword{import}\AgdaSpace{}%
\AgdaModule{Data.List}\AgdaSpace{}%
\AgdaKeyword{hiding}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaOperator{\AgdaFunction{\AgdaUnderscore{}++\AgdaUnderscore{}}}\AgdaSymbol{)}\<%
\\
\>[0]\AgdaKeyword{open}\AgdaSpace{}%
\AgdaKeyword{import}\AgdaSpace{}%
\AgdaModule{Data.Unit}%
\>[23]\AgdaKeyword{hiding}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaOperator{\AgdaRecord{\AgdaUnderscore{}≤\AgdaUnderscore{}}}\AgdaSymbol{)}\<%
\\
\>[0]\AgdaKeyword{open}\AgdaSpace{}%
\AgdaKeyword{import}\AgdaSpace{}%
\AgdaModule{Data.Empty}\<%
\\
\>[0]\AgdaKeyword{open}\AgdaSpace{}%
\AgdaKeyword{import}\AgdaSpace{}%
\AgdaModule{Data.Bool}%
\>[23]\AgdaKeyword{hiding}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaOperator{\AgdaDatatype{\AgdaUnderscore{}≤\AgdaUnderscore{}}}\AgdaSpace{}%
\AgdaSymbol{;}\AgdaSpace{}%
\AgdaOperator{\AgdaFunction{if\AgdaUnderscore{}then\AgdaUnderscore{}else\AgdaUnderscore{}}}\AgdaSpace{}%
\AgdaSymbol{)}\AgdaSpace{}%
\AgdaKeyword{renaming}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaOperator{\AgdaFunction{\AgdaUnderscore{}∧\AgdaUnderscore{}}}\AgdaSpace{}%
\AgdaSymbol{to}\AgdaSpace{}%
\AgdaOperator{\AgdaFunction{\AgdaUnderscore{}∧b\AgdaUnderscore{}}}\AgdaSpace{}%
\AgdaSymbol{;}\AgdaSpace{}%
\AgdaOperator{\AgdaFunction{\AgdaUnderscore{}∨\AgdaUnderscore{}}}\AgdaSpace{}%
\AgdaSymbol{to}\AgdaSpace{}%
\AgdaOperator{\AgdaFunction{\AgdaUnderscore{}∨b\AgdaUnderscore{}}}\AgdaSpace{}%
\AgdaSymbol{;}\AgdaSpace{}%
\AgdaFunction{T}\AgdaSpace{}%
\AgdaSymbol{to}\AgdaSpace{}%
\AgdaFunction{True}\AgdaSymbol{)}\<%
\\
\>[0]\AgdaKeyword{open}\AgdaSpace{}%
\AgdaKeyword{import}\AgdaSpace{}%
\AgdaModule{Data.Product}\AgdaSpace{}%
\AgdaKeyword{renaming}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaOperator{\AgdaInductiveConstructor{\AgdaUnderscore{},\AgdaUnderscore{}}}\AgdaSpace{}%
\AgdaSymbol{to}\AgdaSpace{}%
\AgdaOperator{\AgdaInductiveConstructor{\AgdaUnderscore{},,\AgdaUnderscore{}}}\AgdaSpace{}%
\AgdaSymbol{)}\<%
\\
\>[0]\AgdaKeyword{open}\AgdaSpace{}%
\AgdaKeyword{import}\AgdaSpace{}%
\AgdaModule{Data.Nat.Base}\AgdaSpace{}%
\AgdaKeyword{hiding}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaOperator{\AgdaDatatype{\AgdaUnderscore{}≤\AgdaUnderscore{}}}\AgdaSymbol{)}\<%
\\
\>[0]\AgdaKeyword{open}\AgdaSpace{}%
\AgdaKeyword{import}\AgdaSpace{}%
\AgdaModule{Data.Maybe}\<%
\\
\>[0]\AgdaKeyword{import}\AgdaSpace{}%
\AgdaModule{Relation.Binary.PropositionalEquality}\AgdaSpace{}%
\AgdaSymbol{as}\AgdaSpace{}%
\AgdaModule{Eq}\<%
\\
\>[0]\AgdaKeyword{open}\AgdaSpace{}%
\AgdaModule{Eq}\AgdaSpace{}%
\AgdaKeyword{using}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaOperator{\AgdaDatatype{\AgdaUnderscore{}≡\AgdaUnderscore{}}}\AgdaSymbol{;}\AgdaSpace{}%
\AgdaInductiveConstructor{refl}\AgdaSymbol{;}\AgdaSpace{}%
\AgdaFunction{cong}\AgdaSymbol{;}\AgdaSpace{}%
\AgdaKeyword{module}\AgdaSpace{}%
\AgdaModule{≡-Reasoning}\AgdaSymbol{;}\AgdaSpace{}%
\AgdaFunction{sym}\AgdaSymbol{)}\<%
\\
\>[0]\AgdaKeyword{open}\AgdaSpace{}%
\AgdaModule{≡-Reasoning}\<%
\\
\>[0]\AgdaKeyword{open}\AgdaSpace{}%
\AgdaKeyword{import}\AgdaSpace{}%
\AgdaModule{Agda.Builtin.Equality}\<%
\\
%
\\[\AgdaEmptyExtraSkip]%
%
\\[\AgdaEmptyExtraSkip]%
\>[0]\AgdaComment{--our\ libraries}\<%
\\
\>[0]\AgdaKeyword{open}\AgdaSpace{}%
\AgdaKeyword{import}\AgdaSpace{}%
\AgdaModule{libraries.listLib}\<%
\\
\>[0]\AgdaKeyword{open}\AgdaSpace{}%
\AgdaKeyword{import}\AgdaSpace{}%
\AgdaModule{libraries.natLib}\<%
\\
\>[0]\AgdaKeyword{open}\AgdaSpace{}%
\AgdaKeyword{import}\AgdaSpace{}%
\AgdaModule{libraries.boolLib}\<%
\\
\>[0]\AgdaKeyword{open}\AgdaSpace{}%
\AgdaKeyword{import}\AgdaSpace{}%
\AgdaModule{libraries.andLib}\<%
\\
\>[0]\AgdaKeyword{open}\AgdaSpace{}%
\AgdaKeyword{import}\AgdaSpace{}%
\AgdaModule{libraries.miscLib}\<%
\\
\>[0]\AgdaKeyword{open}\AgdaSpace{}%
\AgdaKeyword{import}\AgdaSpace{}%
\AgdaModule{libraries.maybeLib}\<%
\\
%
\\[\AgdaEmptyExtraSkip]%
\>[0]\AgdaKeyword{open}\AgdaSpace{}%
\AgdaKeyword{import}\AgdaSpace{}%
\AgdaModule{stack}\<%
\\
\>[0]\AgdaKeyword{open}\AgdaSpace{}%
\AgdaKeyword{import}\AgdaSpace{}%
\AgdaModule{semanticBasicOperations}\AgdaSpace{}%
\AgdaBound{param}\<%
\\
\>[0]\AgdaKeyword{open}\AgdaSpace{}%
\AgdaKeyword{import}\AgdaSpace{}%
\AgdaModule{instructionBasic}\<%
\\
\>[0]\AgdaKeyword{open}\AgdaSpace{}%
\AgdaKeyword{import}\AgdaSpace{}%
\AgdaModule{verificationStackScripts.stackState}\<%
\\
\>[0]\AgdaKeyword{open}\AgdaSpace{}%
\AgdaKeyword{import}\AgdaSpace{}%
\AgdaModule{verificationStackScripts.sPredicate}\<%
\\
\>[0]\AgdaKeyword{open}\AgdaSpace{}%
\AgdaKeyword{import}\AgdaSpace{}%
\AgdaModule{verificationStackScripts.stackSemanticsInstructionsBasic}\AgdaSpace{}%
\AgdaBound{param}\<%
\\
%
\\[\AgdaEmptyExtraSkip]%
%
\\[\AgdaEmptyExtraSkip]%
\>[0]\AgdaComment{--\ Note\ that\ ⟦\ p\ ⟧sˢ\ \ is\ defined\ in}\<%
\\
\>[0]\AgdaComment{--\ verificationStackScripts.stackSemanticsInstructionsBasic}\<%
\\
\>[0]\AgdaComment{--\ \textbackslash{}semanticsStackInstructionssemanticS}\<%
\\
\>[0]\<%
\end{code}
} % END AgdaHide

\newcommand{\semanticsStackInstructionssemanticS}{
\begin{code}%
\>[0]\AgdaOperator{\AgdaFunction{⟦\AgdaUnderscore{}⟧ₛ}}\AgdaSpace{}%
\AgdaSymbol{:}\AgdaSpace{}%
\AgdaDatatype{InstructionBasic}\AgdaSpace{}%
\AgdaSymbol{→}\AgdaSpace{}%
\AgdaRecord{StackState}\AgdaSpace{}%
\AgdaSymbol{→}\AgdaSpace{}%
\AgdaDatatype{Maybe}\AgdaSpace{}%
\AgdaRecord{StackState}\<%
\\
\>[0]\AgdaOperator{\AgdaFunction{⟦}}\AgdaSpace{}%
\AgdaBound{op}\AgdaSpace{}%
\AgdaOperator{\AgdaFunction{⟧ₛ}}%
\>[10]\AgdaSymbol{=}\AgdaSpace{}%
\AgdaFunction{liftStackFun2StackState}\AgdaSpace{}%
\AgdaOperator{\AgdaFunction{⟦}}\AgdaSpace{}%
\AgdaBound{op}\AgdaSpace{}%
\AgdaOperator{\AgdaFunction{⟧ₛˢ}}\<%
\end{code}
} % END newcommand

\AgdaHide{
\begin{code}%
\>[0]\<%
\\
%
\\[\AgdaEmptyExtraSkip]%
\>[0]\AgdaComment{\{-}\<%
\\
\>[0]\AgdaComment{⟦\AgdaUnderscore{}⟧s\ :\ InstructionBasic\ →\ StackState\ →\ Maybe\ StackState}\<%
\\
\>[0]\AgdaComment{⟦\ opEqual\ ⟧s\ \ \ \ \ \ \ \ =\ \ liftStackToStackStateTransformer'\ \ executeStackEquality}\<%
\\
\>[0]\AgdaComment{⟦\ opAdd\ ⟧s\ \ \ \ \ \ \ \ \ \ =\ \ liftStackToStackStateTransformer'\ \ executeStackAdd}\<%
\\
\>[0]\AgdaComment{⟦\ (opPush\ x)\ ⟧s\ \ \ \ \ =\ \ liftStackToStackStateTransformer'\ \ (executeStackPush\ x)}\<%
\\
\>[0]\AgdaComment{⟦\ opSub\ ⟧s\ \ \ \ \ \ \ \ \ \ =\ \ liftStackToStackStateTransformer'\ \ executeStackSub}\<%
\\
\>[0]\AgdaComment{⟦\ opVerify\ ⟧s\ \ \ \ \ \ \ =\ \ liftStackToStackStateTransformer'\ \ executeStackVerify}\<%
\\
\>[0]\AgdaComment{⟦\ opCheckSig\ ⟧s\ \ \ \ \ =\ \ liftMsgStackToStateTransformer'\ \ \ \ executeStackCheckSig}\<%
\\
\>[0]\AgdaComment{⟦\ opEqualVerify\ ⟧s\ \ =\ \ liftStackToStackStateTransformer'\ \ executeStackVerify}\<%
\\
\>[0]\AgdaComment{⟦\ opDup\ ⟧s\ \ \ \ \ \ \ \ \ \ =\ \ liftStackToStackStateTransformer'\ \ executeStackDup}\<%
\\
\>[0]\AgdaComment{⟦\ opDrop\ ⟧s\ \ \ \ \ \ \ \ \ =\ \ liftStackToStackStateTransformer'\ \ executeStackDrop}\<%
\\
\>[0]\AgdaComment{⟦\ opSwap\ ⟧s\ \ \ \ \ \ \ \ \ =\ \ liftStackToStackStateTransformer'\ \ executeStackSwap}\<%
\\
\>[0]\AgdaComment{⟦\ opCHECKLOCKTIMEVERIFY\ ⟧s\ =\ liftTimeStackToStateTransformer'\ executeOpCHECKLOCKTIMEVERIFY}\<%
\\
\>[0]\AgdaComment{⟦\ opCheckSig3\ \ ⟧s\ \ \ =\ \ liftMsgStackToStateTransformer'\ \ \ \ executeStackCheckSig3Aux}\<%
\\
\>[0]\AgdaComment{⟦\ opHash\ \ ⟧s\ \ \ \ \ \ \ \ =\ \ liftStackToStackStateTransformer'\ \ executeOpHash}\<%
\\
\>[0]\AgdaComment{⟦\ opMultiSig\ ⟧s\ \ \ \ \ =\ \ liftMsgStackToStateTransformer'\ \ \ \ executeMultiSig}\<%
\\
\>[0]\AgdaComment{-\}}\<%
\\
%
\\[\AgdaEmptyExtraSkip]%
%
\\[\AgdaEmptyExtraSkip]%
\>[0]\AgdaOperator{\AgdaFunction{⟦\AgdaUnderscore{}⟧ₛ⁺}}\AgdaSpace{}%
\AgdaSymbol{:}\AgdaSpace{}%
\AgdaDatatype{InstructionBasic}\AgdaSpace{}%
\AgdaSymbol{→}\AgdaSpace{}%
\AgdaDatatype{Maybe}\AgdaSpace{}%
\AgdaRecord{StackState}\AgdaSpace{}%
\AgdaSymbol{→}\AgdaSpace{}%
\AgdaDatatype{Maybe}\AgdaSpace{}%
\AgdaRecord{StackState}\<%
\\
\>[0]\AgdaOperator{\AgdaFunction{⟦}}\AgdaSpace{}%
\AgdaBound{op}\AgdaSpace{}%
\AgdaOperator{\AgdaFunction{⟧ₛ⁺}}\AgdaSpace{}%
\AgdaBound{t}\AgdaSpace{}%
\AgdaSymbol{=}\AgdaSpace{}%
\AgdaBound{t}\AgdaSpace{}%
\AgdaOperator{\AgdaFunction{>>=}}\AgdaSpace{}%
\AgdaOperator{\AgdaFunction{⟦}}\AgdaSpace{}%
\AgdaBound{op}\AgdaSpace{}%
\AgdaOperator{\AgdaFunction{⟧ₛ}}\<%
\\
\>[0]\AgdaComment{--\ ⟦\ op\ ⟧s⁺\ nothing\ =\ nothing}\<%
\\
\>[0]\AgdaComment{--\ ⟦\ op\ ⟧s⁺\ (just\ s\ )\ =\ ⟦\ op\ ⟧s\ s}\<%
\\
%
\\[\AgdaEmptyExtraSkip]%
%
\\[\AgdaEmptyExtraSkip]%
\>[0]\AgdaOperator{\AgdaFunction{⟦\AgdaUnderscore{}⟧}}\AgdaSpace{}%
\AgdaSymbol{:}\AgdaSpace{}%
\AgdaFunction{BitcoinScriptBasic}\AgdaSpace{}%
\AgdaSymbol{→}\AgdaSpace{}%
\AgdaRecord{StackState}\AgdaSpace{}%
\AgdaSymbol{→}\AgdaSpace{}%
\AgdaDatatype{Maybe}\AgdaSpace{}%
\AgdaRecord{StackState}\<%
\\
\>[0]\AgdaOperator{\AgdaFunction{⟦}}\AgdaSpace{}%
\AgdaInductiveConstructor{[]}%
\>[6]\AgdaOperator{\AgdaFunction{⟧}}%
\>[9]\AgdaSymbol{=}\AgdaSpace{}%
\AgdaInductiveConstructor{just}\<%
\\
\>[0]\AgdaOperator{\AgdaFunction{⟦}}\AgdaSpace{}%
\AgdaBound{op}\AgdaSpace{}%
\AgdaOperator{\AgdaInductiveConstructor{∷}}\AgdaSpace{}%
\AgdaInductiveConstructor{[]}%
\>[11]\AgdaOperator{\AgdaFunction{⟧}}%
\>[14]\AgdaSymbol{=}\AgdaSpace{}%
\AgdaOperator{\AgdaFunction{⟦}}\AgdaSpace{}%
\AgdaBound{op}\AgdaSpace{}%
\AgdaOperator{\AgdaFunction{⟧ₛ}}\<%
\\
\>[0]\AgdaCatchallClause{\AgdaOperator{\AgdaFunction{⟦}}}\AgdaSpace{}%
\AgdaCatchallClause{\AgdaBound{op}}\AgdaSpace{}%
\AgdaCatchallClause{\AgdaOperator{\AgdaInductiveConstructor{∷}}}\AgdaSpace{}%
\AgdaCatchallClause{\AgdaBound{p}}%
\>[11]\AgdaCatchallClause{\AgdaOperator{\AgdaFunction{⟧}}}%
\>[14]\AgdaCatchallClause{\AgdaBound{s}}\AgdaSpace{}%
\AgdaSymbol{=}\AgdaSpace{}%
\AgdaOperator{\AgdaFunction{⟦}}\AgdaSpace{}%
\AgdaBound{op}\AgdaSpace{}%
\AgdaOperator{\AgdaFunction{⟧ₛ}}\AgdaSpace{}%
\AgdaBound{s}\AgdaSpace{}%
\AgdaOperator{\AgdaFunction{>>=}}%
\>[33]\AgdaOperator{\AgdaFunction{⟦}}\AgdaSpace{}%
\AgdaBound{p}\AgdaSpace{}%
\AgdaOperator{\AgdaFunction{⟧}}\<%
\\
%
\\[\AgdaEmptyExtraSkip]%
\>[0]\AgdaOperator{\AgdaFunction{⟦\AgdaUnderscore{}⟧⁺}}\AgdaSpace{}%
\AgdaSymbol{:}\AgdaSpace{}%
\AgdaFunction{BitcoinScriptBasic}\AgdaSpace{}%
\AgdaSymbol{→}\AgdaSpace{}%
\AgdaDatatype{Maybe}\AgdaSpace{}%
\AgdaRecord{StackState}\AgdaSpace{}%
\AgdaSymbol{→}\AgdaSpace{}%
\AgdaDatatype{Maybe}\AgdaSpace{}%
\AgdaRecord{StackState}\<%
\\
\>[0]\AgdaOperator{\AgdaFunction{⟦}}\AgdaSpace{}%
\AgdaBound{p}\AgdaSpace{}%
\AgdaOperator{\AgdaFunction{⟧⁺}}\AgdaSpace{}%
\AgdaBound{s}\AgdaSpace{}%
\AgdaSymbol{=}\AgdaSpace{}%
\AgdaBound{s}\AgdaSpace{}%
\AgdaOperator{\AgdaFunction{>>=}}\AgdaSpace{}%
\AgdaOperator{\AgdaFunction{⟦}}\AgdaSpace{}%
\AgdaBound{p}\AgdaSpace{}%
\AgdaOperator{\AgdaFunction{⟧}}\<%
\\
%
\\[\AgdaEmptyExtraSkip]%
%
\\[\AgdaEmptyExtraSkip]%
\>[0]\AgdaFunction{validStackAux}\AgdaSpace{}%
\AgdaSymbol{:}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaBound{pbkh}\AgdaSpace{}%
\AgdaSymbol{:}\AgdaSpace{}%
\AgdaDatatype{ℕ}\AgdaSymbol{)}\AgdaSpace{}%
\AgdaSymbol{→}%
\>[30]\AgdaSymbol{(}\AgdaBound{msg}\AgdaSpace{}%
\AgdaSymbol{:}\AgdaSpace{}%
\AgdaDatatype{Msg}\AgdaSymbol{)}\AgdaSpace{}%
\AgdaSymbol{→}%
\>[45]\AgdaFunction{Stack}\AgdaSpace{}%
\AgdaSymbol{→}%
\>[54]\AgdaDatatype{Bool}\<%
\\
\>[0]\AgdaFunction{validStackAux}\AgdaSpace{}%
\AgdaBound{pkh}\AgdaSpace{}%
\AgdaBound{msg[]}%
\>[25]\AgdaInductiveConstructor{[]}%
\>[29]\AgdaSymbol{=}\AgdaSpace{}%
\AgdaInductiveConstructor{false}\<%
\\
\>[0]\AgdaFunction{validStackAux}\AgdaSpace{}%
\AgdaBound{pkh}\AgdaSpace{}%
\AgdaBound{msg}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaBound{pbk}\AgdaSpace{}%
\AgdaOperator{\AgdaInductiveConstructor{∷}}\AgdaSpace{}%
\AgdaInductiveConstructor{[]}\AgdaSymbol{)}\AgdaSpace{}%
\AgdaSymbol{=}\AgdaSpace{}%
\AgdaInductiveConstructor{false}\<%
\\
\>[0]\AgdaFunction{validStackAux}\AgdaSpace{}%
\AgdaBound{pkh}\AgdaSpace{}%
\AgdaBound{msg}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaBound{pbk}\AgdaSpace{}%
\AgdaOperator{\AgdaInductiveConstructor{∷}}\AgdaSpace{}%
\AgdaBound{sig}\AgdaSpace{}%
\AgdaOperator{\AgdaInductiveConstructor{∷}}\AgdaSpace{}%
\AgdaBound{s}\AgdaSymbol{)}\AgdaSpace{}%
\AgdaSymbol{=}\AgdaSpace{}%
\AgdaFunction{hashFun}\AgdaSpace{}%
\AgdaBound{pbk}%
\>[53]\AgdaOperator{\AgdaFunction{==b}}\AgdaSpace{}%
\AgdaBound{pkh}\AgdaSpace{}%
\AgdaOperator{\AgdaFunction{∧b}}\AgdaSpace{}%
\AgdaFunction{isSigned}%
\>[74]\AgdaBound{msg}\AgdaSpace{}%
\AgdaBound{sig}\AgdaSpace{}%
\AgdaBound{pbk}\<%
\\
%
\\[\AgdaEmptyExtraSkip]%
\>[0]\AgdaFunction{validStack}\AgdaSpace{}%
\AgdaSymbol{:}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaBound{pkh}\AgdaSpace{}%
\AgdaSymbol{:}\AgdaSpace{}%
\AgdaDatatype{ℕ}\AgdaSymbol{)}\AgdaSpace{}%
\AgdaSymbol{→}%
\>[26]\AgdaFunction{BStackStatePred}\<%
\\
\>[0]\AgdaFunction{validStack}\AgdaSpace{}%
\AgdaBound{pkh}\AgdaSpace{}%
\AgdaOperator{\AgdaInductiveConstructor{⟨}}\AgdaSpace{}%
\AgdaBound{time}\AgdaSpace{}%
\AgdaOperator{\AgdaInductiveConstructor{,}}\AgdaSpace{}%
\AgdaBound{msg₁}\AgdaSpace{}%
\AgdaOperator{\AgdaInductiveConstructor{,}}\AgdaSpace{}%
\AgdaBound{stack₁}\AgdaSpace{}%
\AgdaOperator{\AgdaInductiveConstructor{⟩}}\AgdaSpace{}%
\AgdaSymbol{=}\AgdaSpace{}%
\AgdaFunction{validStackAux}%
\>[57]\AgdaBound{pkh}%
\>[63]\AgdaBound{msg₁}%
\>[69]\AgdaBound{stack₁}\<%
\end{code}
} % END AgdaHide


==> latex-before-sed/verificationStackScripts/stackSemanticsInstructionsBasic.tex <==
%% This file has been generated automatically by mkLagda.awk
%% DO NOT EDIT! ALL YOUR CHANGES WILL BE LOST!

\AgdaHide{
\begin{code}%
\>[0]\AgdaKeyword{open}\AgdaSpace{}%
\AgdaKeyword{import}\AgdaSpace{}%
\AgdaModule{basicBitcoinDataType}\<%
\\
%
\\[\AgdaEmptyExtraSkip]%
\>[0]\AgdaKeyword{module}\AgdaSpace{}%
\AgdaModule{verificationStackScripts.stackSemanticsInstructionsBasic}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaBound{param}\AgdaSpace{}%
\AgdaSymbol{:}\AgdaSpace{}%
\AgdaRecord{GlobalParameters}\AgdaSymbol{)}%
\>[92]\AgdaKeyword{where}\<%
\\
%
\\[\AgdaEmptyExtraSkip]%
\>[0]\AgdaKeyword{open}\AgdaSpace{}%
\AgdaKeyword{import}\AgdaSpace{}%
\AgdaModule{Data.Nat}%
\>[22]\AgdaKeyword{hiding}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaOperator{\AgdaDatatype{\AgdaUnderscore{}≤\AgdaUnderscore{}}}\AgdaSymbol{)}\<%
\\
\>[0]\AgdaKeyword{open}\AgdaSpace{}%
\AgdaKeyword{import}\AgdaSpace{}%
\AgdaModule{Data.List}\AgdaSpace{}%
\AgdaKeyword{hiding}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaOperator{\AgdaFunction{\AgdaUnderscore{}++\AgdaUnderscore{}}}\AgdaSymbol{)}\<%
\\
\>[0]\AgdaKeyword{open}\AgdaSpace{}%
\AgdaKeyword{import}\AgdaSpace{}%
\AgdaModule{Data.Unit}%
\>[23]\AgdaKeyword{hiding}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaOperator{\AgdaRecord{\AgdaUnderscore{}≤\AgdaUnderscore{}}}\AgdaSymbol{)}\<%
\\
\>[0]\AgdaKeyword{open}\AgdaSpace{}%
\AgdaKeyword{import}\AgdaSpace{}%
\AgdaModule{Data.Empty}\<%
\\
\>[0]\AgdaKeyword{open}\AgdaSpace{}%
\AgdaKeyword{import}\AgdaSpace{}%
\AgdaModule{Data.Bool}%
\>[23]\AgdaKeyword{hiding}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaOperator{\AgdaDatatype{\AgdaUnderscore{}≤\AgdaUnderscore{}}}\AgdaSpace{}%
\AgdaSymbol{;}\AgdaSpace{}%
\AgdaOperator{\AgdaFunction{if\AgdaUnderscore{}then\AgdaUnderscore{}else\AgdaUnderscore{}}}\AgdaSpace{}%
\AgdaSymbol{)}\AgdaSpace{}%
\AgdaKeyword{renaming}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaOperator{\AgdaFunction{\AgdaUnderscore{}∧\AgdaUnderscore{}}}\AgdaSpace{}%
\AgdaSymbol{to}\AgdaSpace{}%
\AgdaOperator{\AgdaFunction{\AgdaUnderscore{}∧b\AgdaUnderscore{}}}\AgdaSpace{}%
\AgdaSymbol{;}\AgdaSpace{}%
\AgdaOperator{\AgdaFunction{\AgdaUnderscore{}∨\AgdaUnderscore{}}}\AgdaSpace{}%
\AgdaSymbol{to}\AgdaSpace{}%
\AgdaOperator{\AgdaFunction{\AgdaUnderscore{}∨b\AgdaUnderscore{}}}\AgdaSpace{}%
\AgdaSymbol{;}\AgdaSpace{}%
\AgdaFunction{T}\AgdaSpace{}%
\AgdaSymbol{to}\AgdaSpace{}%
\AgdaFunction{True}\AgdaSymbol{)}\<%
\\
\>[0]\AgdaKeyword{open}\AgdaSpace{}%
\AgdaKeyword{import}\AgdaSpace{}%
\AgdaModule{Data.Product}\AgdaSpace{}%
\AgdaKeyword{renaming}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaOperator{\AgdaInductiveConstructor{\AgdaUnderscore{},\AgdaUnderscore{}}}\AgdaSpace{}%
\AgdaSymbol{to}\AgdaSpace{}%
\AgdaOperator{\AgdaInductiveConstructor{\AgdaUnderscore{},,\AgdaUnderscore{}}}\AgdaSpace{}%
\AgdaSymbol{)}\<%
\\
\>[0]\AgdaKeyword{open}\AgdaSpace{}%
\AgdaKeyword{import}\AgdaSpace{}%
\AgdaModule{Data.Nat.Base}\AgdaSpace{}%
\AgdaKeyword{hiding}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaOperator{\AgdaDatatype{\AgdaUnderscore{}≤\AgdaUnderscore{}}}\AgdaSymbol{)}\<%
\\
\>[0]\AgdaKeyword{open}\AgdaSpace{}%
\AgdaKeyword{import}\AgdaSpace{}%
\AgdaModule{Data.Maybe}\<%
\\
\>[0]\AgdaKeyword{import}\AgdaSpace{}%
\AgdaModule{Relation.Binary.PropositionalEquality}\AgdaSpace{}%
\AgdaSymbol{as}\AgdaSpace{}%
\AgdaModule{Eq}\<%
\\
\>[0]\AgdaKeyword{open}\AgdaSpace{}%
\AgdaModule{Eq}\AgdaSpace{}%
\AgdaKeyword{using}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaOperator{\AgdaDatatype{\AgdaUnderscore{}≡\AgdaUnderscore{}}}\AgdaSymbol{;}\AgdaSpace{}%
\AgdaInductiveConstructor{refl}\AgdaSymbol{;}\AgdaSpace{}%
\AgdaFunction{cong}\AgdaSymbol{;}\AgdaSpace{}%
\AgdaKeyword{module}\AgdaSpace{}%
\AgdaModule{≡-Reasoning}\AgdaSymbol{;}\AgdaSpace{}%
\AgdaFunction{sym}\AgdaSymbol{)}\<%
\\
\>[0]\AgdaKeyword{open}\AgdaSpace{}%
\AgdaModule{≡-Reasoning}\<%
\\
\>[0]\AgdaKeyword{open}\AgdaSpace{}%
\AgdaKeyword{import}\AgdaSpace{}%
\AgdaModule{Agda.Builtin.Equality}\<%
\\
%
\\[\AgdaEmptyExtraSkip]%
%
\\[\AgdaEmptyExtraSkip]%
\>[0]\AgdaComment{--our\ libraries}\<%
\\
\>[0]\AgdaKeyword{open}\AgdaSpace{}%
\AgdaKeyword{import}\AgdaSpace{}%
\AgdaModule{libraries.listLib}\<%
\\
\>[0]\AgdaKeyword{open}\AgdaSpace{}%
\AgdaKeyword{import}\AgdaSpace{}%
\AgdaModule{libraries.natLib}\<%
\\
\>[0]\AgdaKeyword{open}\AgdaSpace{}%
\AgdaKeyword{import}\AgdaSpace{}%
\AgdaModule{libraries.boolLib}\<%
\\
\>[0]\AgdaKeyword{open}\AgdaSpace{}%
\AgdaKeyword{import}\AgdaSpace{}%
\AgdaModule{libraries.andLib}\<%
\\
\>[0]\AgdaKeyword{open}\AgdaSpace{}%
\AgdaKeyword{import}\AgdaSpace{}%
\AgdaModule{libraries.miscLib}\<%
\\
\>[0]\AgdaKeyword{open}\AgdaSpace{}%
\AgdaKeyword{import}\AgdaSpace{}%
\AgdaModule{libraries.maybeLib}\<%
\\
%
\\[\AgdaEmptyExtraSkip]%
%
\\[\AgdaEmptyExtraSkip]%
\>[0]\AgdaKeyword{open}\AgdaSpace{}%
\AgdaKeyword{import}\AgdaSpace{}%
\AgdaModule{stack}\<%
\\
\>[0]\AgdaKeyword{open}\AgdaSpace{}%
\AgdaKeyword{import}\AgdaSpace{}%
\AgdaModule{semanticBasicOperations}\AgdaSpace{}%
\AgdaBound{param}\<%
\\
\>[0]\AgdaKeyword{open}\AgdaSpace{}%
\AgdaKeyword{import}\AgdaSpace{}%
\AgdaModule{instructionBasic}\<%
\\
%
\\[\AgdaEmptyExtraSkip]%
\>[0]\AgdaKeyword{open}\AgdaSpace{}%
\AgdaKeyword{import}\AgdaSpace{}%
\AgdaModule{verificationStackScripts.stackState}\<%
\\
\>[0]\AgdaKeyword{open}\AgdaSpace{}%
\AgdaKeyword{import}\AgdaSpace{}%
\AgdaModule{verificationStackScripts.sPredicate}\<%
\\
\>[0]\AgdaKeyword{open}\AgdaSpace{}%
\AgdaKeyword{import}\AgdaSpace{}%
\AgdaModule{verificationStackScripts.stackInstruction}\<%
\\
%
\\[\AgdaEmptyExtraSkip]%
%
\\[\AgdaEmptyExtraSkip]%
%
\\[\AgdaEmptyExtraSkip]%
\>[0]\AgdaComment{--\ The\ stack\ operation\ of\ type}\<%
\\
\>[0]\AgdaComment{--\ \ \ Time\ →\ Msg\ →\ \ Stack\ →\ Maybe\ Stack}\<%
\\
\>[0]\AgdaComment{--\ on\ which\ the\ semantics\ is\ based}\<%
\\
\>[0]\AgdaComment{--\ we\ have\ (see\ next\ lemma)\ for\ nonif\ instructions}\<%
\\
\>[0]\AgdaComment{--\ ⟦\ op\ ⟧s\ \ ≡\ stackTransform2StateTransform\ ⟦\ op\ ⟧sˢ\ \ ⟧ₛˢ}\<%
\\
%
\\[\AgdaEmptyExtraSkip]%
\>[0]\AgdaComment{--\ The\ stacks\ operations\ is\ only\ corret\ for\ non-if\ instructions}\<%
\\
\>[0]\AgdaComment{--\ original\ name\ was\ \ \ executeStackPartOfInstr}\<%
\\
%
\\[\AgdaEmptyExtraSkip]%
\>[0]\AgdaComment{--\ \textbackslash{}stackSemanticsInstructionsBasicsemanticsstype}\<%
\end{code}
} % END AgdaHide

\newcommand{\stackSemanticsInstructionsBasicsemanticsstype}{
\begin{code}%
\>[0]\AgdaOperator{\AgdaFunction{⟦\AgdaUnderscore{}⟧ₛˢ}}\AgdaSpace{}%
\AgdaSymbol{:}\AgdaSpace{}%
\AgdaDatatype{InstructionBasic}\AgdaSpace{}%
\AgdaSymbol{→}%
\>[28]\AgdaFunction{Time}\AgdaSpace{}%
\AgdaSymbol{→}\AgdaSpace{}%
\AgdaDatatype{Msg}\AgdaSpace{}%
\AgdaSymbol{→}%
\>[42]\AgdaFunction{Stack}\AgdaSpace{}%
\AgdaSymbol{→}\AgdaSpace{}%
\AgdaDatatype{Maybe}\AgdaSpace{}%
\AgdaFunction{Stack}\<%
\\
\>[0]\AgdaOperator{\AgdaFunction{⟦}}\AgdaSpace{}%
\AgdaInductiveConstructor{opEqual}%
\>[11]\AgdaOperator{\AgdaFunction{⟧ₛˢ}}\AgdaSpace{}%
\AgdaBound{time₁}\AgdaSpace{}%
\AgdaBound{msg}\AgdaSpace{}%
\AgdaSymbol{=}\AgdaSpace{}%
\AgdaFunction{executeStackEquality}\<%
\end{code}
} % END newcommand

\AgdaHide{
\begin{code}%
\>[0]\AgdaOperator{\AgdaFunction{⟦}}\AgdaSpace{}%
\AgdaInductiveConstructor{opAdd}%
\>[11]\AgdaOperator{\AgdaFunction{⟧ₛˢ}}\AgdaSpace{}%
\AgdaBound{time₁}\AgdaSpace{}%
\AgdaBound{msg}\AgdaSpace{}%
\AgdaSymbol{=}\AgdaSpace{}%
\AgdaFunction{executeStackAdd}\<%
\\
\>[0]\AgdaOperator{\AgdaFunction{⟦}}\AgdaSpace{}%
\AgdaInductiveConstructor{opPush}\AgdaSpace{}%
\AgdaBound{x}\AgdaSpace{}%
\AgdaOperator{\AgdaFunction{⟧ₛˢ}}\AgdaSpace{}%
\AgdaBound{time₁}\AgdaSpace{}%
\AgdaBound{msg}\AgdaSpace{}%
\AgdaSymbol{=}\AgdaSpace{}%
\AgdaFunction{executeStackPush}\AgdaSpace{}%
\AgdaBound{x}\<%
\\
\>[0]\AgdaOperator{\AgdaFunction{⟦}}\AgdaSpace{}%
\AgdaInductiveConstructor{opSub}%
\>[11]\AgdaOperator{\AgdaFunction{⟧ₛˢ}}\AgdaSpace{}%
\AgdaBound{time₁}\AgdaSpace{}%
\AgdaBound{msg}\AgdaSpace{}%
\AgdaSymbol{=}\AgdaSpace{}%
\AgdaFunction{executeStackSub}\<%
\\
\>[0]\AgdaOperator{\AgdaFunction{⟦}}\AgdaSpace{}%
\AgdaInductiveConstructor{opVerify}\AgdaSpace{}%
\AgdaOperator{\AgdaFunction{⟧ₛˢ}}\AgdaSpace{}%
\AgdaBound{time₁}\AgdaSpace{}%
\AgdaBound{msg}\AgdaSpace{}%
\AgdaSymbol{=}\AgdaSpace{}%
\AgdaFunction{executeStackVerify}\<%
\\
\>[0]\AgdaComment{--\ \textbackslash{}stackSemanticsInstructionsBasicsemanticss}\<%
\end{code}
} % END AgdaHide

\newcommand{\stackSemanticsInstructionsBasicsemanticss}{
\begin{code}%
\>[0]\AgdaOperator{\AgdaFunction{⟦}}\AgdaSpace{}%
\AgdaInductiveConstructor{opCheckSig}\AgdaSpace{}%
\AgdaOperator{\AgdaFunction{⟧ₛˢ}}\AgdaSpace{}%
\AgdaBound{time₁}\AgdaSpace{}%
\AgdaBound{msg}\AgdaSpace{}%
\AgdaSymbol{=}\AgdaSpace{}%
\AgdaFunction{executeStackCheckSig}\AgdaSpace{}%
\AgdaBound{msg}\<%
\end{code}
} % END newcommand

\AgdaHide{
\begin{code}%
\>[0]\AgdaOperator{\AgdaFunction{⟦}}\AgdaSpace{}%
\AgdaInductiveConstructor{opEqualVerify}\AgdaSpace{}%
\AgdaOperator{\AgdaFunction{⟧ₛˢ}}\AgdaSpace{}%
\AgdaBound{time₁}\AgdaSpace{}%
\AgdaBound{msg}\AgdaSpace{}%
\AgdaSymbol{=}\AgdaSpace{}%
\AgdaFunction{executeStackVerify}\<%
\\
\>[0]\AgdaOperator{\AgdaFunction{⟦}}\AgdaSpace{}%
\AgdaInductiveConstructor{opDup}%
\>[11]\AgdaOperator{\AgdaFunction{⟧ₛˢ}}\AgdaSpace{}%
\AgdaBound{time₁}\AgdaSpace{}%
\AgdaBound{msg}\AgdaSpace{}%
\AgdaSymbol{=}\AgdaSpace{}%
\AgdaFunction{executeStackDup}\<%
\\
\>[0]\AgdaOperator{\AgdaFunction{⟦}}\AgdaSpace{}%
\AgdaInductiveConstructor{opDrop}%
\>[11]\AgdaOperator{\AgdaFunction{⟧ₛˢ}}\AgdaSpace{}%
\AgdaBound{time₁}\AgdaSpace{}%
\AgdaBound{msg}\AgdaSpace{}%
\AgdaSymbol{=}\AgdaSpace{}%
\AgdaFunction{executeStackDrop}\<%
\\
\>[0]\AgdaOperator{\AgdaFunction{⟦}}\AgdaSpace{}%
\AgdaInductiveConstructor{opSwap}%
\>[11]\AgdaOperator{\AgdaFunction{⟧ₛˢ}}\AgdaSpace{}%
\AgdaBound{time₁}\AgdaSpace{}%
\AgdaBound{msg}\AgdaSpace{}%
\AgdaSymbol{=}\AgdaSpace{}%
\AgdaFunction{executeStackSwap}\<%
\\
\>[0]\AgdaOperator{\AgdaFunction{⟦}}\AgdaSpace{}%
\AgdaInductiveConstructor{opHash}%
\>[11]\AgdaOperator{\AgdaFunction{⟧ₛˢ}}\AgdaSpace{}%
\AgdaBound{time₁}\AgdaSpace{}%
\AgdaBound{msg}\AgdaSpace{}%
\AgdaSymbol{=}\AgdaSpace{}%
\AgdaFunction{executeOpHash}\<%
\\
\>[0]\AgdaOperator{\AgdaFunction{⟦}}\AgdaSpace{}%
\AgdaInductiveConstructor{opCHECKLOCKTIMEVERIFY}\AgdaSpace{}%
\AgdaOperator{\AgdaFunction{⟧ₛˢ}}\AgdaSpace{}%
\AgdaBound{time₁}\AgdaSpace{}%
\AgdaBound{msg}\AgdaSpace{}%
\AgdaSymbol{=}\AgdaSpace{}%
\AgdaFunction{executeOpCHECKLOCKTIMEVERIFY}\AgdaSpace{}%
\AgdaBound{time₁}\<%
\\
\>[0]\AgdaOperator{\AgdaFunction{⟦}}\AgdaSpace{}%
\AgdaInductiveConstructor{opCheckSig3}\AgdaSpace{}%
\AgdaOperator{\AgdaFunction{⟧ₛˢ}}\AgdaSpace{}%
\AgdaBound{time₁}\AgdaSpace{}%
\AgdaBound{msg}\AgdaSpace{}%
\AgdaSymbol{=}\AgdaSpace{}%
\AgdaFunction{executeStackCheckSig3Aux}\AgdaSpace{}%
\AgdaBound{msg}\<%
\\
\>[0]\AgdaOperator{\AgdaFunction{⟦}}\AgdaSpace{}%
\AgdaInductiveConstructor{opMultiSig}\AgdaSpace{}%
\AgdaOperator{\AgdaFunction{⟧ₛˢ}}%
\>[18]\AgdaBound{time₁}\AgdaSpace{}%
\AgdaBound{msg}\AgdaSpace{}%
\AgdaSymbol{=}%
\>[31]\AgdaFunction{executeMultiSig}\AgdaSpace{}%
\AgdaBound{msg}\<%
\\
%
\\[\AgdaEmptyExtraSkip]%
\>[0]\AgdaComment{--\ execute\ only\ the\ stack\ operations\ of\ a\ bitcoin\ script}\<%
\\
\>[0]\AgdaComment{--\ \ is\ correct\ only\ for\ non-if\ instructiosn}\<%
\\
\>[0]\AgdaOperator{\AgdaFunction{⟦\AgdaUnderscore{}⟧ˢ}}\AgdaSpace{}%
\AgdaSymbol{:}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaBound{prog}\AgdaSpace{}%
\AgdaSymbol{:}\AgdaSpace{}%
\AgdaFunction{BitcoinScriptBasic}\AgdaSymbol{)(}\AgdaBound{time₁}\AgdaSpace{}%
\AgdaSymbol{:}\AgdaSpace{}%
\AgdaFunction{Time}\AgdaSymbol{)(}\AgdaBound{msg}\AgdaSpace{}%
\AgdaSymbol{:}\AgdaSpace{}%
\AgdaDatatype{Msg}\AgdaSymbol{)(}\AgdaBound{stack₁}\AgdaSpace{}%
\AgdaSymbol{:}\AgdaSpace{}%
\AgdaFunction{Stack}\AgdaSymbol{)}\AgdaSpace{}%
\AgdaSymbol{→}\AgdaSpace{}%
\AgdaDatatype{Maybe}\AgdaSpace{}%
\AgdaFunction{Stack}\<%
\\
\>[0]\AgdaOperator{\AgdaFunction{⟦}}\AgdaSpace{}%
\AgdaInductiveConstructor{[]}%
\>[12]\AgdaOperator{\AgdaFunction{⟧ˢ}}\AgdaSpace{}%
\AgdaBound{time₁}\AgdaSpace{}%
\AgdaBound{msg}\AgdaSpace{}%
\AgdaBound{stack₁}\AgdaSpace{}%
\AgdaSymbol{=}\AgdaSpace{}%
\AgdaInductiveConstructor{just}\AgdaSpace{}%
\AgdaBound{stack₁}\<%
\\
\>[0]\AgdaOperator{\AgdaFunction{⟦}}\AgdaSpace{}%
\AgdaBound{op}\AgdaSpace{}%
\AgdaOperator{\AgdaInductiveConstructor{∷}}\AgdaSpace{}%
\AgdaInductiveConstructor{[]}%
\>[12]\AgdaOperator{\AgdaFunction{⟧ˢ}}\AgdaSpace{}%
\AgdaBound{time₁}\AgdaSpace{}%
\AgdaBound{msg}\AgdaSpace{}%
\AgdaBound{stack₁}\AgdaSpace{}%
\AgdaSymbol{=}\AgdaSpace{}%
\AgdaOperator{\AgdaFunction{⟦}}\AgdaSpace{}%
\AgdaBound{op}\AgdaSpace{}%
\AgdaOperator{\AgdaFunction{⟧ₛˢ}}\AgdaSpace{}%
\AgdaBound{time₁}\AgdaSpace{}%
\AgdaBound{msg}\AgdaSpace{}%
\AgdaBound{stack₁}\<%
\\
\>[0]\AgdaCatchallClause{\AgdaOperator{\AgdaFunction{⟦}}}\AgdaSpace{}%
\AgdaCatchallClause{\AgdaBound{op}}\AgdaSpace{}%
\AgdaCatchallClause{\AgdaOperator{\AgdaInductiveConstructor{∷}}}\AgdaSpace{}%
\AgdaCatchallClause{\AgdaBound{prog}}\AgdaSpace{}%
\AgdaCatchallClause{\AgdaOperator{\AgdaFunction{⟧ˢ}}}\AgdaSpace{}%
\AgdaCatchallClause{\AgdaBound{time₁}}\AgdaSpace{}%
\AgdaCatchallClause{\AgdaBound{msg}}\AgdaSpace{}%
\AgdaCatchallClause{\AgdaBound{stack₁}}\AgdaSpace{}%
\AgdaSymbol{=}%
\>[35]\AgdaOperator{\AgdaFunction{⟦}}\AgdaSpace{}%
\AgdaBound{op}\AgdaSpace{}%
\AgdaOperator{\AgdaFunction{⟧ₛˢ}}\AgdaSpace{}%
\AgdaBound{time₁}\AgdaSpace{}%
\AgdaBound{msg}\AgdaSpace{}%
\AgdaBound{stack₁}\AgdaSpace{}%
\AgdaOperator{\AgdaFunction{>>=}}\AgdaSpace{}%
\AgdaOperator{\AgdaFunction{⟦}}\AgdaSpace{}%
\AgdaBound{prog}\AgdaSpace{}%
\AgdaOperator{\AgdaFunction{⟧ˢ}}\AgdaSpace{}%
\AgdaBound{time₁}\AgdaSpace{}%
\AgdaBound{msg}\<%
\end{code}
} % END AgdaHide


==> latex-before-sed/verificationStackScripts/stackState.tex <==
%% This file has been generated automatically by mkLagda.awk
%% DO NOT EDIT! ALL YOUR CHANGES WILL BE LOST!

\AgdaHide{
\begin{code}%
\>[0]\AgdaKeyword{module}\AgdaSpace{}%
\AgdaModule{verificationStackScripts.stackState}\AgdaSpace{}%
\AgdaKeyword{where}\<%
\\
%
\\[\AgdaEmptyExtraSkip]%
\>[0]\AgdaKeyword{open}\AgdaSpace{}%
\AgdaKeyword{import}\AgdaSpace{}%
\AgdaModule{Data.Nat}%
\>[22]\AgdaKeyword{hiding}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaOperator{\AgdaDatatype{\AgdaUnderscore{}≤\AgdaUnderscore{}}}\AgdaSymbol{)}\<%
\\
\>[0]\AgdaKeyword{open}\AgdaSpace{}%
\AgdaKeyword{import}\AgdaSpace{}%
\AgdaModule{Data.List}\AgdaSpace{}%
\AgdaKeyword{hiding}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaOperator{\AgdaFunction{\AgdaUnderscore{}++\AgdaUnderscore{}}}\AgdaSymbol{)}\<%
\\
\>[0]\AgdaKeyword{open}\AgdaSpace{}%
\AgdaKeyword{import}\AgdaSpace{}%
\AgdaModule{Data.Unit}%
\>[23]\AgdaKeyword{hiding}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaOperator{\AgdaRecord{\AgdaUnderscore{}≤\AgdaUnderscore{}}}\AgdaSymbol{)}\<%
\\
\>[0]\AgdaKeyword{open}\AgdaSpace{}%
\AgdaKeyword{import}\AgdaSpace{}%
\AgdaModule{Data.Empty}\<%
\\
\>[0]\AgdaKeyword{open}\AgdaSpace{}%
\AgdaKeyword{import}\AgdaSpace{}%
\AgdaModule{Data.Maybe}\<%
\\
\>[0]\AgdaKeyword{open}\AgdaSpace{}%
\AgdaKeyword{import}\AgdaSpace{}%
\AgdaModule{Data.Bool}%
\>[23]\AgdaKeyword{hiding}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaOperator{\AgdaDatatype{\AgdaUnderscore{}≤\AgdaUnderscore{}}}\AgdaSpace{}%
\AgdaSymbol{;}\AgdaSpace{}%
\AgdaOperator{\AgdaFunction{if\AgdaUnderscore{}then\AgdaUnderscore{}else\AgdaUnderscore{}}}\AgdaSpace{}%
\AgdaSymbol{)}\AgdaSpace{}%
\AgdaKeyword{renaming}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaOperator{\AgdaFunction{\AgdaUnderscore{}∧\AgdaUnderscore{}}}\AgdaSpace{}%
\AgdaSymbol{to}\AgdaSpace{}%
\AgdaOperator{\AgdaFunction{\AgdaUnderscore{}∧b\AgdaUnderscore{}}}\AgdaSpace{}%
\AgdaSymbol{;}\AgdaSpace{}%
\AgdaOperator{\AgdaFunction{\AgdaUnderscore{}∨\AgdaUnderscore{}}}\AgdaSpace{}%
\AgdaSymbol{to}\AgdaSpace{}%
\AgdaOperator{\AgdaFunction{\AgdaUnderscore{}∨b\AgdaUnderscore{}}}\AgdaSpace{}%
\AgdaSymbol{;}\AgdaSpace{}%
\AgdaFunction{T}\AgdaSpace{}%
\AgdaSymbol{to}\AgdaSpace{}%
\AgdaFunction{True}\AgdaSymbol{)}\<%
\\
\>[0]\AgdaKeyword{open}\AgdaSpace{}%
\AgdaKeyword{import}\AgdaSpace{}%
\AgdaModule{Data.Bool.Base}\AgdaSpace{}%
\AgdaKeyword{hiding}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaOperator{\AgdaDatatype{\AgdaUnderscore{}≤\AgdaUnderscore{}}}\AgdaSpace{}%
\AgdaSymbol{;}\AgdaSpace{}%
\AgdaOperator{\AgdaFunction{if\AgdaUnderscore{}then\AgdaUnderscore{}else\AgdaUnderscore{}}}\AgdaSpace{}%
\AgdaSymbol{)}\AgdaSpace{}%
\AgdaKeyword{renaming}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaOperator{\AgdaFunction{\AgdaUnderscore{}∧\AgdaUnderscore{}}}\AgdaSpace{}%
\AgdaSymbol{to}\AgdaSpace{}%
\AgdaOperator{\AgdaFunction{\AgdaUnderscore{}∧b\AgdaUnderscore{}}}\AgdaSpace{}%
\AgdaSymbol{;}\AgdaSpace{}%
\AgdaOperator{\AgdaFunction{\AgdaUnderscore{}∨\AgdaUnderscore{}}}\AgdaSpace{}%
\AgdaSymbol{to}\AgdaSpace{}%
\AgdaOperator{\AgdaFunction{\AgdaUnderscore{}∨b\AgdaUnderscore{}}}\AgdaSpace{}%
\AgdaSymbol{;}\AgdaSpace{}%
\AgdaFunction{T}\AgdaSpace{}%
\AgdaSymbol{to}\AgdaSpace{}%
\AgdaFunction{True}\AgdaSymbol{)}\<%
\\
\>[0]\AgdaKeyword{open}\AgdaSpace{}%
\AgdaKeyword{import}\AgdaSpace{}%
\AgdaModule{Data.Product}\AgdaSpace{}%
\AgdaKeyword{renaming}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaOperator{\AgdaInductiveConstructor{\AgdaUnderscore{},\AgdaUnderscore{}}}\AgdaSpace{}%
\AgdaSymbol{to}\AgdaSpace{}%
\AgdaOperator{\AgdaInductiveConstructor{\AgdaUnderscore{},,\AgdaUnderscore{}}}\AgdaSpace{}%
\AgdaSymbol{)}\<%
\\
\>[0]\AgdaKeyword{open}\AgdaSpace{}%
\AgdaKeyword{import}\AgdaSpace{}%
\AgdaModule{Data.Nat.Base}\AgdaSpace{}%
\AgdaKeyword{hiding}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaOperator{\AgdaDatatype{\AgdaUnderscore{}≤\AgdaUnderscore{}}}\AgdaSymbol{)}\<%
\\
\>[0]\AgdaKeyword{open}\AgdaSpace{}%
\AgdaKeyword{import}\AgdaSpace{}%
\AgdaModule{Data.List.NonEmpty}\AgdaSpace{}%
\AgdaKeyword{hiding}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaField{head}\AgdaSymbol{)}\<%
\\
\>[0]\AgdaKeyword{import}\AgdaSpace{}%
\AgdaModule{Relation.Binary.PropositionalEquality}\AgdaSpace{}%
\AgdaSymbol{as}\AgdaSpace{}%
\AgdaModule{Eq}\<%
\\
\>[0]\AgdaKeyword{open}\AgdaSpace{}%
\AgdaModule{Eq}\AgdaSpace{}%
\AgdaKeyword{using}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaOperator{\AgdaDatatype{\AgdaUnderscore{}≡\AgdaUnderscore{}}}\AgdaSymbol{;}\AgdaSpace{}%
\AgdaInductiveConstructor{refl}\AgdaSymbol{;}\AgdaSpace{}%
\AgdaFunction{cong}\AgdaSymbol{;}\AgdaSpace{}%
\AgdaKeyword{module}\AgdaSpace{}%
\AgdaModule{≡-Reasoning}\AgdaSymbol{;}\AgdaSpace{}%
\AgdaFunction{sym}\AgdaSymbol{)}\<%
\\
\>[0]\AgdaKeyword{open}\AgdaSpace{}%
\AgdaModule{≡-Reasoning}\<%
\\
\>[0]\AgdaKeyword{open}\AgdaSpace{}%
\AgdaKeyword{import}\AgdaSpace{}%
\AgdaModule{Agda.Builtin.Equality}\<%
\\
%
\\[\AgdaEmptyExtraSkip]%
\>[0]\AgdaComment{--our\ libraries}\<%
\\
\>[0]\AgdaKeyword{open}\AgdaSpace{}%
\AgdaKeyword{import}\AgdaSpace{}%
\AgdaModule{libraries.listLib}\<%
\\
\>[0]\AgdaKeyword{open}\AgdaSpace{}%
\AgdaKeyword{import}\AgdaSpace{}%
\AgdaModule{libraries.natLib}\<%
\\
\>[0]\AgdaKeyword{open}\AgdaSpace{}%
\AgdaKeyword{import}\AgdaSpace{}%
\AgdaModule{libraries.boolLib}\<%
\\
\>[0]\AgdaKeyword{open}\AgdaSpace{}%
\AgdaKeyword{import}\AgdaSpace{}%
\AgdaModule{libraries.andLib}\<%
\\
\>[0]\AgdaKeyword{open}\AgdaSpace{}%
\AgdaKeyword{import}\AgdaSpace{}%
\AgdaModule{libraries.miscLib}\<%
\\
\>[0]\AgdaKeyword{open}\AgdaSpace{}%
\AgdaKeyword{import}\AgdaSpace{}%
\AgdaModule{libraries.maybeLib}\<%
\\
%
\\[\AgdaEmptyExtraSkip]%
\>[0]\AgdaKeyword{open}\AgdaSpace{}%
\AgdaKeyword{import}\AgdaSpace{}%
\AgdaModule{basicBitcoinDataType}\<%
\\
\>[0]\AgdaKeyword{open}\AgdaSpace{}%
\AgdaKeyword{import}\AgdaSpace{}%
\AgdaModule{stack}\<%
\\
\>[0]\<%
\end{code}
} % END AgdaHide

\newcommand{\stackStateStackState}{
\begin{code}%
\>[0]\AgdaKeyword{record}%
\>[98I]\AgdaRecord{StackState}%
\>[19]\AgdaSymbol{:}\AgdaSpace{}%
\AgdaPrimitive{Set}%
\>[26]\AgdaKeyword{where}\<%
\\
\>[.][@{}l@{}]\<[98I]%
\>[7]\AgdaKeyword{constructor}\AgdaSpace{}%
\AgdaOperator{\AgdaInductiveConstructor{⟨\AgdaUnderscore{},\AgdaUnderscore{},\AgdaUnderscore{}⟩}}\<%
\\
%
\>[7]\AgdaKeyword{field}%
\>[14]\AgdaField{currentTime}\AgdaSpace{}%
\AgdaSymbol{:}%
\>[29]\AgdaFunction{Time}%
\>[35]\AgdaComment{--\ current\ time,\ i.e.\ time\ when\ the\ the\ smart\ contract\ is\ executed}\<%
\\
%
\>[14]\AgdaField{msg}%
\>[26]\AgdaSymbol{:}%
\>[29]\AgdaDatatype{Msg}\<%
\\
%
\>[14]\AgdaField{stack}%
\>[26]\AgdaSymbol{:}%
\>[29]\AgdaFunction{Stack}\<%
\end{code}
} % END newcommand

\AgdaHide{
\begin{code}%
\>[0]\<%
\\
\>[0]\AgdaKeyword{open}\AgdaSpace{}%
\AgdaModule{StackState}\AgdaSpace{}%
\AgdaKeyword{public}\<%
\\
%
\\[\AgdaEmptyExtraSkip]%
%
\\[\AgdaEmptyExtraSkip]%
\>[0]\AgdaKeyword{record}%
\>[104I]\AgdaRecord{StackStateWithMaybe}%
\>[28]\AgdaSymbol{:}\AgdaSpace{}%
\AgdaPrimitive{Set}%
\>[35]\AgdaKeyword{where}\<%
\\
\>[.][@{}l@{}]\<[104I]%
\>[7]\AgdaKeyword{constructor}\AgdaSpace{}%
\AgdaOperator{\AgdaInductiveConstructor{⟨\AgdaUnderscore{},\AgdaUnderscore{},\AgdaUnderscore{}⟩}}\<%
\\
%
\>[7]\AgdaKeyword{field}\<%
\\
\>[7][@{}l@{\AgdaIndent{0}}]%
\>[9]\AgdaField{currentTime}\AgdaSpace{}%
\AgdaSymbol{:}\AgdaSpace{}%
\AgdaFunction{Time}%
\>[29]\AgdaComment{--\ current\ time,\ i.e.\ time\ when\ the}\<%
\\
%
\>[29]\AgdaComment{--\ the\ smart\ contract\ is\ executed}\<%
\\
%
\>[9]\AgdaField{msg}\AgdaSpace{}%
\AgdaSymbol{:}\AgdaSpace{}%
\AgdaDatatype{Msg}\<%
\\
%
\>[9]\AgdaField{maybeStack}\AgdaSpace{}%
\AgdaSymbol{:}\AgdaSpace{}%
\AgdaDatatype{Maybe}\AgdaSpace{}%
\AgdaFunction{Stack}\<%
\\
%
\\[\AgdaEmptyExtraSkip]%
\>[0]\AgdaKeyword{open}\AgdaSpace{}%
\AgdaModule{StackStateWithMaybe}\AgdaSpace{}%
\AgdaKeyword{public}\<%
\\
%
\\[\AgdaEmptyExtraSkip]%
%
\\[\AgdaEmptyExtraSkip]%
\>[0]\AgdaFunction{stackState2WithMaybe}\AgdaSpace{}%
\AgdaSymbol{:}\AgdaSpace{}%
\AgdaRecord{StackStateWithMaybe}\AgdaSpace{}%
\AgdaSymbol{→}\AgdaSpace{}%
\AgdaDatatype{Maybe}\AgdaSpace{}%
\AgdaRecord{StackState}\<%
\\
\>[0]\AgdaFunction{stackState2WithMaybe}\AgdaSpace{}%
\AgdaOperator{\AgdaInductiveConstructor{⟨}}\AgdaSpace{}%
\AgdaBound{currentTime₁}\AgdaSpace{}%
\AgdaOperator{\AgdaInductiveConstructor{,}}\AgdaSpace{}%
\AgdaBound{msg₁}\AgdaSpace{}%
\AgdaOperator{\AgdaInductiveConstructor{,}}\AgdaSpace{}%
\AgdaInductiveConstructor{just}\AgdaSpace{}%
\AgdaBound{x}%
\>[53]\AgdaOperator{\AgdaInductiveConstructor{⟩}}\AgdaSpace{}%
\AgdaSymbol{=}\AgdaSpace{}%
\AgdaInductiveConstructor{just}\AgdaSpace{}%
\AgdaOperator{\AgdaInductiveConstructor{⟨}}\AgdaSpace{}%
\AgdaBound{currentTime₁}\AgdaSpace{}%
\AgdaOperator{\AgdaInductiveConstructor{,}}\AgdaSpace{}%
\AgdaBound{msg₁}\AgdaSpace{}%
\AgdaOperator{\AgdaInductiveConstructor{,}}\AgdaSpace{}%
\AgdaBound{x}%
\>[89]\AgdaOperator{\AgdaInductiveConstructor{⟩}}\<%
\\
\>[0]\AgdaFunction{stackState2WithMaybe}\AgdaSpace{}%
\AgdaOperator{\AgdaInductiveConstructor{⟨}}\AgdaSpace{}%
\AgdaBound{currentTime₁}\AgdaSpace{}%
\AgdaOperator{\AgdaInductiveConstructor{,}}\AgdaSpace{}%
\AgdaBound{msg₁}\AgdaSpace{}%
\AgdaOperator{\AgdaInductiveConstructor{,}}\AgdaSpace{}%
\AgdaInductiveConstructor{nothing}\AgdaSpace{}%
\AgdaOperator{\AgdaInductiveConstructor{⟩}}\AgdaSpace{}%
\AgdaSymbol{=}\AgdaSpace{}%
\AgdaInductiveConstructor{nothing}\<%
\\
%
\\[\AgdaEmptyExtraSkip]%
%
\\[\AgdaEmptyExtraSkip]%
%
\\[\AgdaEmptyExtraSkip]%
%
\\[\AgdaEmptyExtraSkip]%
\>[0]\AgdaKeyword{mutual}\<%
\\
%
\\[\AgdaEmptyExtraSkip]%
\>[0][@{}l@{\AgdaIndent{0}}]%
\>[2]\AgdaFunction{liftStackToStateTransformerAux'}\AgdaSpace{}%
\AgdaSymbol{:}\AgdaSpace{}%
\AgdaDatatype{Maybe}\AgdaSpace{}%
\AgdaFunction{Stack}\AgdaSpace{}%
\AgdaSymbol{→}\AgdaSpace{}%
\AgdaRecord{StackState}\AgdaSpace{}%
\AgdaSymbol{→}\AgdaSpace{}%
\AgdaRecord{StackStateWithMaybe}\<%
\\
%
\>[2]\AgdaFunction{liftStackToStateTransformerAux'}\AgdaSpace{}%
\AgdaBound{maybest}\AgdaSpace{}%
\AgdaOperator{\AgdaInductiveConstructor{⟨}}\AgdaSpace{}%
\AgdaBound{currentTime₁}\AgdaSpace{}%
\AgdaOperator{\AgdaInductiveConstructor{,}}\AgdaSpace{}%
\AgdaBound{msg₁}\AgdaSpace{}%
\AgdaOperator{\AgdaInductiveConstructor{,}}\AgdaSpace{}%
\AgdaBound{stack₁}%
\>[74]\AgdaOperator{\AgdaInductiveConstructor{⟩}}\AgdaSpace{}%
\AgdaSymbol{=}\AgdaSpace{}%
\AgdaOperator{\AgdaInductiveConstructor{⟨}}\AgdaSpace{}%
\AgdaBound{currentTime₁}\AgdaSpace{}%
\AgdaOperator{\AgdaInductiveConstructor{,}}\AgdaSpace{}%
\AgdaBound{msg₁}\AgdaSpace{}%
\AgdaOperator{\AgdaInductiveConstructor{,}}\AgdaSpace{}%
\AgdaBound{maybest}%
\>[111]\AgdaOperator{\AgdaInductiveConstructor{⟩}}\<%
\\
%
\\[\AgdaEmptyExtraSkip]%
%
\\[\AgdaEmptyExtraSkip]%
%
\\[\AgdaEmptyExtraSkip]%
%
\\[\AgdaEmptyExtraSkip]%
\>[0]\AgdaFunction{exeTransformerDepIfStack'}\AgdaSpace{}%
\AgdaSymbol{:}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaSpace{}%
\AgdaRecord{StackState}\AgdaSpace{}%
\AgdaSymbol{→}\AgdaSpace{}%
\AgdaRecord{StackStateWithMaybe}\AgdaSpace{}%
\AgdaSymbol{)}\AgdaSpace{}%
\AgdaSymbol{→}%
\>[68]\AgdaRecord{StackState}\AgdaSpace{}%
\AgdaSymbol{→}\AgdaSpace{}%
\AgdaDatatype{Maybe}\AgdaSpace{}%
\AgdaRecord{StackState}\<%
\\
\>[0]\AgdaFunction{exeTransformerDepIfStack'}\AgdaSpace{}%
\AgdaBound{f}\AgdaSpace{}%
\AgdaBound{s}\AgdaSpace{}%
\AgdaSymbol{=}\AgdaSpace{}%
\AgdaFunction{stackState2WithMaybe}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaBound{f}\AgdaSpace{}%
\AgdaBound{s}\AgdaSymbol{)}\<%
\\
%
\\[\AgdaEmptyExtraSkip]%
%
\\[\AgdaEmptyExtraSkip]%
\>[0]\AgdaFunction{stackTransform2StackStateTransform}\AgdaSpace{}%
\AgdaSymbol{:}\AgdaSpace{}%
\AgdaFunction{StackTransformer}%
\>[55]\AgdaSymbol{→}\AgdaSpace{}%
\AgdaRecord{StackState}\AgdaSpace{}%
\AgdaSymbol{→}\AgdaSpace{}%
\AgdaDatatype{Maybe}\AgdaSpace{}%
\AgdaRecord{StackState}\<%
\\
\>[0]\AgdaFunction{stackTransform2StackStateTransform}\AgdaSpace{}%
\AgdaBound{f}\AgdaSpace{}%
\AgdaBound{s}\<%
\\
\>[0][@{}l@{\AgdaIndent{0}}]%
\>[5]\AgdaSymbol{=}\AgdaSpace{}%
\AgdaFunction{stackState2WithMaybe}\AgdaSpace{}%
\AgdaSymbol{((}\AgdaFunction{liftStackToStateTransformerAux'}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaBound{f}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaBound{s}\AgdaSpace{}%
\AgdaSymbol{.}\AgdaField{currentTime}\AgdaSymbol{)}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaBound{s}\AgdaSpace{}%
\AgdaSymbol{.}\AgdaField{msg}\AgdaSymbol{)}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaBound{s}\AgdaSpace{}%
\AgdaSymbol{.}\AgdaField{stack}\AgdaSymbol{)))}\AgdaSpace{}%
\AgdaBound{s}\AgdaSpace{}%
\AgdaSymbol{)}\<%
\\
%
\\[\AgdaEmptyExtraSkip]%
%
\\[\AgdaEmptyExtraSkip]%
\>[0]\AgdaFunction{liftStackToStackStateTransformer'}\AgdaSpace{}%
\AgdaSymbol{:}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaFunction{Stack}\AgdaSpace{}%
\AgdaSymbol{→}\AgdaSpace{}%
\AgdaDatatype{Maybe}\AgdaSpace{}%
\AgdaFunction{Stack}\AgdaSymbol{)}%
\>[59]\AgdaSymbol{→}\AgdaSpace{}%
\AgdaRecord{StackState}\AgdaSpace{}%
\AgdaSymbol{→}\AgdaSpace{}%
\AgdaDatatype{Maybe}\AgdaSpace{}%
\AgdaRecord{StackState}\<%
\\
\>[0]\AgdaFunction{liftStackToStackStateTransformer'}\AgdaSpace{}%
\AgdaBound{f}\AgdaSpace{}%
\AgdaSymbol{=}\AgdaSpace{}%
\AgdaFunction{stackTransform2StackStateTransform}\AgdaSpace{}%
\AgdaSymbol{(λ}\AgdaSpace{}%
\AgdaBound{time}\AgdaSpace{}%
\AgdaBound{msg}\AgdaSpace{}%
\AgdaSymbol{→}\AgdaSpace{}%
\AgdaBound{f}\AgdaSymbol{)}\<%
\\
%
\\[\AgdaEmptyExtraSkip]%
%
\\[\AgdaEmptyExtraSkip]%
\>[0]\AgdaFunction{liftTimeStackToStateTransformer'}\AgdaSpace{}%
\AgdaSymbol{:}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaFunction{Time}\AgdaSpace{}%
\AgdaSymbol{→}\AgdaSpace{}%
\AgdaFunction{Stack}\AgdaSpace{}%
\AgdaSymbol{→}\AgdaSpace{}%
\AgdaDatatype{Maybe}\AgdaSpace{}%
\AgdaFunction{Stack}\AgdaSymbol{)}%
\>[65]\AgdaSymbol{→}\AgdaSpace{}%
\AgdaRecord{StackState}\AgdaSpace{}%
\AgdaSymbol{→}\AgdaSpace{}%
\AgdaDatatype{Maybe}\AgdaSpace{}%
\AgdaRecord{StackState}\<%
\\
\>[0]\AgdaFunction{liftTimeStackToStateTransformer'}\AgdaSpace{}%
\AgdaBound{f}\AgdaSpace{}%
\AgdaSymbol{=}\AgdaSpace{}%
\AgdaFunction{stackTransform2StackStateTransform}\AgdaSpace{}%
\AgdaSymbol{(λ}\AgdaSpace{}%
\AgdaBound{time}\AgdaSpace{}%
\AgdaBound{msg}\AgdaSpace{}%
\AgdaSymbol{→}\AgdaSpace{}%
\AgdaBound{f}\AgdaSpace{}%
\AgdaBound{time}\AgdaSymbol{)}\<%
\\
%
\\[\AgdaEmptyExtraSkip]%
\>[0]\AgdaFunction{liftMsgStackToStateTransformer'}\AgdaSpace{}%
\AgdaSymbol{:}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaDatatype{Msg}\AgdaSpace{}%
\AgdaSymbol{→}\AgdaSpace{}%
\AgdaFunction{Stack}\AgdaSpace{}%
\AgdaSymbol{→}\AgdaSpace{}%
\AgdaDatatype{Maybe}\AgdaSpace{}%
\AgdaFunction{Stack}\AgdaSymbol{)}%
\>[63]\AgdaSymbol{→}\AgdaSpace{}%
\AgdaRecord{StackState}\AgdaSpace{}%
\AgdaSymbol{→}\AgdaSpace{}%
\AgdaDatatype{Maybe}\AgdaSpace{}%
\AgdaRecord{StackState}\<%
\\
\>[0]\AgdaFunction{liftMsgStackToStateTransformer'}\AgdaSpace{}%
\AgdaBound{f}\AgdaSpace{}%
\AgdaSymbol{=}\AgdaSpace{}%
\AgdaFunction{stackTransform2StackStateTransform}\AgdaSpace{}%
\AgdaSymbol{(λ}\AgdaSpace{}%
\AgdaBound{time}\AgdaSpace{}%
\AgdaBound{msg}\AgdaSpace{}%
\AgdaSymbol{→}\AgdaSpace{}%
\AgdaBound{f}\AgdaSpace{}%
\AgdaBound{msg}\AgdaSymbol{)}\<%
\\
%
\\[\AgdaEmptyExtraSkip]%
%
\\[\AgdaEmptyExtraSkip]%
%
\\[\AgdaEmptyExtraSkip]%
%
\\[\AgdaEmptyExtraSkip]%
\>[0]\AgdaFunction{msgToMStackToIfStackToMState}\AgdaSpace{}%
\AgdaSymbol{:}\AgdaSpace{}%
\AgdaFunction{Time}\AgdaSpace{}%
\AgdaSymbol{→}\AgdaSpace{}%
\AgdaDatatype{Msg}%
\>[43]\AgdaSymbol{→}\AgdaSpace{}%
\AgdaDatatype{Maybe}\AgdaSpace{}%
\AgdaFunction{Stack}\AgdaSpace{}%
\AgdaSymbol{→}\AgdaSpace{}%
\AgdaDatatype{Maybe}\AgdaSpace{}%
\AgdaRecord{StackState}\<%
\\
\>[0]\AgdaFunction{msgToMStackToIfStackToMState}\AgdaSpace{}%
\AgdaBound{time}\AgdaSpace{}%
\AgdaBound{msg}\AgdaSpace{}%
\AgdaInductiveConstructor{nothing}\AgdaSpace{}%
\AgdaSymbol{=}\AgdaSpace{}%
\AgdaInductiveConstructor{nothing}\<%
\\
\>[0]\AgdaFunction{msgToMStackToIfStackToMState}\AgdaSpace{}%
\AgdaBound{time}\AgdaSpace{}%
\AgdaBound{msg}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaInductiveConstructor{just}\AgdaSpace{}%
\AgdaBound{x}\AgdaSymbol{)}\AgdaSpace{}%
\AgdaSymbol{=}\AgdaSpace{}%
\AgdaInductiveConstructor{just}\AgdaSpace{}%
\AgdaOperator{\AgdaInductiveConstructor{⟨}}\AgdaSpace{}%
\AgdaBound{time}\AgdaSpace{}%
\AgdaOperator{\AgdaInductiveConstructor{,}}\AgdaSpace{}%
\AgdaBound{msg}\AgdaSpace{}%
\AgdaOperator{\AgdaInductiveConstructor{,}}\AgdaSpace{}%
\AgdaBound{x}\AgdaSpace{}%
\AgdaOperator{\AgdaInductiveConstructor{⟩}}\<%
\\
%
\\[\AgdaEmptyExtraSkip]%
%
\\[\AgdaEmptyExtraSkip]%
\>[0]\AgdaFunction{liftStackFun2StackState}\AgdaSpace{}%
\AgdaSymbol{:}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaFunction{Time}\AgdaSpace{}%
\AgdaSymbol{→}\AgdaSpace{}%
\AgdaDatatype{Msg}\AgdaSpace{}%
\AgdaSymbol{→}\AgdaSpace{}%
\AgdaFunction{Stack}\AgdaSpace{}%
\AgdaSymbol{→}\AgdaSpace{}%
\AgdaDatatype{Maybe}\AgdaSpace{}%
\AgdaFunction{Stack}\AgdaSymbol{)}\AgdaSpace{}%
\AgdaSymbol{→}\AgdaSpace{}%
\AgdaRecord{StackState}\AgdaSpace{}%
\AgdaSymbol{→}\AgdaSpace{}%
\AgdaDatatype{Maybe}\AgdaSpace{}%
\AgdaRecord{StackState}\<%
\\
\>[0]\AgdaFunction{liftStackFun2StackState}\AgdaSpace{}%
\AgdaBound{f}\AgdaSpace{}%
\AgdaOperator{\AgdaInductiveConstructor{⟨}}\AgdaSpace{}%
\AgdaBound{currentTime₁}\AgdaSpace{}%
\AgdaOperator{\AgdaInductiveConstructor{,}}\AgdaSpace{}%
\AgdaBound{msg₁}\AgdaSpace{}%
\AgdaOperator{\AgdaInductiveConstructor{,}}\AgdaSpace{}%
\AgdaBound{stack₁}\AgdaSpace{}%
\AgdaOperator{\AgdaInductiveConstructor{⟩}}\AgdaSpace{}%
\AgdaSymbol{=}\<%
\\
\>[0][@{}l@{\AgdaIndent{0}}]%
\>[4]\AgdaFunction{stackState2WithMaybe}\AgdaSpace{}%
\AgdaOperator{\AgdaInductiveConstructor{⟨}}\AgdaSpace{}%
\AgdaBound{currentTime₁}\AgdaSpace{}%
\AgdaOperator{\AgdaInductiveConstructor{,}}\AgdaSpace{}%
\AgdaBound{msg₁}\AgdaSpace{}%
\AgdaOperator{\AgdaInductiveConstructor{,}}\AgdaSymbol{(}\AgdaBound{f}\AgdaSpace{}%
\AgdaBound{currentTime₁}%
\>[65]\AgdaBound{msg₁}%
\>[71]\AgdaBound{stack₁}\AgdaSymbol{)}\AgdaSpace{}%
\AgdaOperator{\AgdaInductiveConstructor{⟩}}\<%
\\
%
\\[\AgdaEmptyExtraSkip]%
\>[0]\AgdaComment{\{-
semanticBasicOperations.executeStackEquality\ param\ (x₁\ .stack)\ ⟩


msgToMStackToIfStackToMState\ currentTime₁\ msg₁
\ \ \ \ \ \ \ \ \ \ \ \ \ \ \ \ \ \ \ \ \ \ \ \ \ \ \ \ \ \ \ \ \ \ \ \ \ \ \ \ \ \ \ \ \ \ \ \ \ \ \ \ \ \ \ \ \ \ \ \ \ \ \ \ \ \ \ \ \ \ (f\ currentTime₁\ \ msg₁\ \ stack₁)
-\}}\<%
\end{code}
} % END AgdaHide


==> latex-before-sed/verificationStackScripts/stackVerificationP2PKH.tex <==
%% This file has been generated automatically by mkLagda.awk
%% DO NOT EDIT! ALL YOUR CHANGES WILL BE LOST!

\AgdaHide{
\begin{code}%
\>[0]\AgdaKeyword{open}\AgdaSpace{}%
\AgdaKeyword{import}\AgdaSpace{}%
\AgdaModule{basicBitcoinDataType}\<%
\\
%
\\[\AgdaEmptyExtraSkip]%
\>[0]\AgdaKeyword{module}%
\>[8]\AgdaModule{verificationStackScripts.stackVerificationP2PKH}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaBound{param}\AgdaSpace{}%
\AgdaSymbol{:}\AgdaSpace{}%
\AgdaRecord{GlobalParameters}\AgdaSymbol{)}\AgdaSpace{}%
\AgdaKeyword{where}\<%
\\
%
\\[\AgdaEmptyExtraSkip]%
\>[0]\AgdaKeyword{open}\AgdaSpace{}%
\AgdaKeyword{import}\AgdaSpace{}%
\AgdaModule{libraries.listLib}\<%
\\
\>[0]\AgdaKeyword{open}\AgdaSpace{}%
\AgdaKeyword{import}\AgdaSpace{}%
\AgdaModule{Data.List.Base}\<%
\\
\>[0]\AgdaKeyword{open}\AgdaSpace{}%
\AgdaKeyword{import}\AgdaSpace{}%
\AgdaModule{libraries.natLib}\<%
\\
\>[0]\AgdaKeyword{open}\AgdaSpace{}%
\AgdaKeyword{import}\AgdaSpace{}%
\AgdaModule{Data.Nat}%
\>[22]\AgdaKeyword{renaming}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaOperator{\AgdaDatatype{\AgdaUnderscore{}≤\AgdaUnderscore{}}}\AgdaSpace{}%
\AgdaSymbol{to}\AgdaSpace{}%
\AgdaOperator{\AgdaDatatype{\AgdaUnderscore{}≤'\AgdaUnderscore{}}}\AgdaSpace{}%
\AgdaSymbol{;}\AgdaSpace{}%
\AgdaOperator{\AgdaFunction{\AgdaUnderscore{}<\AgdaUnderscore{}}}\AgdaSpace{}%
\AgdaSymbol{to}\AgdaSpace{}%
\AgdaOperator{\AgdaFunction{\AgdaUnderscore{}<'\AgdaUnderscore{}}}\AgdaSymbol{)}\<%
\\
\>[0]\AgdaKeyword{open}\AgdaSpace{}%
\AgdaKeyword{import}\AgdaSpace{}%
\AgdaModule{Data.List}\AgdaSpace{}%
\AgdaKeyword{hiding}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaOperator{\AgdaFunction{\AgdaUnderscore{}++\AgdaUnderscore{}}}\AgdaSymbol{)}\<%
\\
\>[0]\AgdaKeyword{open}\AgdaSpace{}%
\AgdaKeyword{import}\AgdaSpace{}%
\AgdaModule{Data.Unit}%
\>[23]\AgdaKeyword{hiding}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaOperator{\AgdaRecord{\AgdaUnderscore{}≤\AgdaUnderscore{}}}\AgdaSymbol{)}\<%
\\
\>[0]\AgdaKeyword{open}\AgdaSpace{}%
\AgdaKeyword{import}\AgdaSpace{}%
\AgdaModule{Data.Empty}\<%
\\
\>[0]\AgdaKeyword{open}\AgdaSpace{}%
\AgdaKeyword{import}\AgdaSpace{}%
\AgdaModule{Data.Bool}%
\>[23]\AgdaKeyword{hiding}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaOperator{\AgdaDatatype{\AgdaUnderscore{}≤\AgdaUnderscore{}}}\AgdaSpace{}%
\AgdaSymbol{;}\AgdaSpace{}%
\AgdaOperator{\AgdaDatatype{\AgdaUnderscore{}<\AgdaUnderscore{}}}\AgdaSpace{}%
\AgdaSymbol{;}\AgdaSpace{}%
\AgdaOperator{\AgdaFunction{if\AgdaUnderscore{}then\AgdaUnderscore{}else\AgdaUnderscore{}}}\AgdaSpace{}%
\AgdaSymbol{)}\AgdaSpace{}%
\AgdaKeyword{renaming}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaOperator{\AgdaFunction{\AgdaUnderscore{}∧\AgdaUnderscore{}}}\AgdaSpace{}%
\AgdaSymbol{to}\AgdaSpace{}%
\AgdaOperator{\AgdaFunction{\AgdaUnderscore{}∧b\AgdaUnderscore{}}}\AgdaSpace{}%
\AgdaSymbol{;}\AgdaSpace{}%
\AgdaOperator{\AgdaFunction{\AgdaUnderscore{}∨\AgdaUnderscore{}}}\AgdaSpace{}%
\AgdaSymbol{to}\AgdaSpace{}%
\AgdaOperator{\AgdaFunction{\AgdaUnderscore{}∨b\AgdaUnderscore{}}}\AgdaSpace{}%
\AgdaSymbol{;}\AgdaSpace{}%
\AgdaFunction{T}\AgdaSpace{}%
\AgdaSymbol{to}\AgdaSpace{}%
\AgdaFunction{True}\AgdaSymbol{)}\<%
\\
\>[0]\AgdaKeyword{open}\AgdaSpace{}%
\AgdaKeyword{import}\AgdaSpace{}%
\AgdaModule{Data.Product}\AgdaSpace{}%
\AgdaKeyword{renaming}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaOperator{\AgdaInductiveConstructor{\AgdaUnderscore{},\AgdaUnderscore{}}}\AgdaSpace{}%
\AgdaSymbol{to}\AgdaSpace{}%
\AgdaOperator{\AgdaInductiveConstructor{\AgdaUnderscore{},,\AgdaUnderscore{}}}\AgdaSpace{}%
\AgdaSymbol{)}\<%
\\
\>[0]\AgdaKeyword{open}\AgdaSpace{}%
\AgdaKeyword{import}\AgdaSpace{}%
\AgdaModule{Data.Nat.Base}\AgdaSpace{}%
\AgdaKeyword{hiding}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaOperator{\AgdaDatatype{\AgdaUnderscore{}≤\AgdaUnderscore{}}}\AgdaSpace{}%
\AgdaSymbol{;}\AgdaSpace{}%
\AgdaOperator{\AgdaFunction{\AgdaUnderscore{}<\AgdaUnderscore{}}}\AgdaSymbol{)}\<%
\\
\>[0]\AgdaKeyword{open}\AgdaSpace{}%
\AgdaKeyword{import}\AgdaSpace{}%
\AgdaModule{Data.List.NonEmpty}\AgdaSpace{}%
\AgdaKeyword{hiding}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaField{head}\AgdaSymbol{;}\AgdaSpace{}%
\AgdaOperator{\AgdaFunction{[\AgdaUnderscore{}]}}\AgdaSymbol{)}\<%
\\
\>[0]\AgdaKeyword{open}\AgdaSpace{}%
\AgdaKeyword{import}\AgdaSpace{}%
\AgdaModule{Data.Nat}\AgdaSpace{}%
\AgdaKeyword{using}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaDatatype{ℕ}\AgdaSymbol{;}\AgdaSpace{}%
\AgdaOperator{\AgdaPrimitive{\AgdaUnderscore{}+\AgdaUnderscore{}}}\AgdaSymbol{;}\AgdaSpace{}%
\AgdaOperator{\AgdaFunction{\AgdaUnderscore{}≥\AgdaUnderscore{}}}\AgdaSymbol{;}\AgdaSpace{}%
\AgdaOperator{\AgdaFunction{\AgdaUnderscore{}>\AgdaUnderscore{}}}\AgdaSymbol{;}\AgdaSpace{}%
\AgdaInductiveConstructor{zero}\AgdaSymbol{;}\AgdaSpace{}%
\AgdaInductiveConstructor{suc}\AgdaSymbol{;}\AgdaSpace{}%
\AgdaInductiveConstructor{s≤s}\AgdaSymbol{;}\AgdaSpace{}%
\AgdaInductiveConstructor{z≤n}\AgdaSymbol{)}\<%
\\
\>[0]\AgdaKeyword{import}\AgdaSpace{}%
\AgdaModule{Relation.Binary.PropositionalEquality}\AgdaSpace{}%
\AgdaSymbol{as}\AgdaSpace{}%
\AgdaModule{Eq}\<%
\\
\>[0]\AgdaKeyword{open}\AgdaSpace{}%
\AgdaModule{Eq}\AgdaSpace{}%
\AgdaKeyword{using}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaOperator{\AgdaDatatype{\AgdaUnderscore{}≡\AgdaUnderscore{}}}\AgdaSymbol{;}\AgdaSpace{}%
\AgdaInductiveConstructor{refl}\AgdaSymbol{;}\AgdaSpace{}%
\AgdaFunction{cong}\AgdaSymbol{;}\AgdaSpace{}%
\AgdaKeyword{module}\AgdaSpace{}%
\AgdaModule{≡-Reasoning}\AgdaSymbol{;}\AgdaSpace{}%
\AgdaFunction{sym}\AgdaSymbol{)}\<%
\\
\>[0]\AgdaKeyword{open}\AgdaSpace{}%
\AgdaModule{≡-Reasoning}\<%
\\
\>[0]\AgdaKeyword{open}\AgdaSpace{}%
\AgdaKeyword{import}\AgdaSpace{}%
\AgdaModule{Agda.Builtin.Equality}\<%
\\
%
\\[\AgdaEmptyExtraSkip]%
%
\\[\AgdaEmptyExtraSkip]%
\>[0]\AgdaComment{--our\ libraries}\<%
\\
\>[0]\AgdaKeyword{open}\AgdaSpace{}%
\AgdaKeyword{import}\AgdaSpace{}%
\AgdaModule{libraries.andLib}\<%
\\
\>[0]\AgdaKeyword{open}\AgdaSpace{}%
\AgdaKeyword{import}\AgdaSpace{}%
\AgdaModule{libraries.miscLib}\<%
\\
\>[0]\AgdaKeyword{open}\AgdaSpace{}%
\AgdaKeyword{import}\AgdaSpace{}%
\AgdaModule{libraries.maybeLib}\<%
\\
\>[0]\AgdaKeyword{open}\AgdaSpace{}%
\AgdaKeyword{import}\AgdaSpace{}%
\AgdaModule{libraries.boolLib}\<%
\\
%
\\[\AgdaEmptyExtraSkip]%
\>[0]\AgdaKeyword{open}\AgdaSpace{}%
\AgdaKeyword{import}\AgdaSpace{}%
\AgdaModule{stack}\<%
\\
\>[0]\AgdaKeyword{open}\AgdaSpace{}%
\AgdaKeyword{import}\AgdaSpace{}%
\AgdaModule{stackPredicate}\<%
\\
\>[0]\AgdaKeyword{open}\AgdaSpace{}%
\AgdaKeyword{import}\AgdaSpace{}%
\AgdaModule{semanticBasicOperations}\AgdaSpace{}%
\AgdaBound{param}\<%
\\
\>[0]\AgdaKeyword{open}\AgdaSpace{}%
\AgdaKeyword{import}\AgdaSpace{}%
\AgdaModule{instructionBasic}\<%
\\
\>[0]\AgdaKeyword{open}\AgdaSpace{}%
\AgdaKeyword{import}\AgdaSpace{}%
\AgdaModule{verificationP2PKHbasic}\AgdaSpace{}%
\AgdaBound{param}\<%
\\
%
\\[\AgdaEmptyExtraSkip]%
\>[0]\AgdaKeyword{open}\AgdaSpace{}%
\AgdaKeyword{import}\AgdaSpace{}%
\AgdaModule{verificationStackScripts.stackHoareTriple}\AgdaSpace{}%
\AgdaBound{param}\<%
\\
\>[0]\AgdaKeyword{open}\AgdaSpace{}%
\AgdaKeyword{import}\AgdaSpace{}%
\AgdaModule{verificationStackScripts.stackState}\<%
\\
\>[0]\AgdaKeyword{open}\AgdaSpace{}%
\AgdaKeyword{import}\AgdaSpace{}%
\AgdaModule{verificationStackScripts.sPredicate}\<%
\\
\>[0]\AgdaKeyword{open}\AgdaSpace{}%
\AgdaKeyword{import}\AgdaSpace{}%
\AgdaModule{verificationStackScripts.semanticsStackInstructions}\AgdaSpace{}%
\AgdaBound{param}\<%
\\
\>[0]\AgdaKeyword{open}\AgdaSpace{}%
\AgdaKeyword{import}\AgdaSpace{}%
\AgdaModule{verificationStackScripts.stackVerificationLemmas}\AgdaSpace{}%
\AgdaBound{param}\<%
\\
%
\\[\AgdaEmptyExtraSkip]%
%
\\[\AgdaEmptyExtraSkip]%
%
\\[\AgdaEmptyExtraSkip]%
\>[0]\AgdaComment{--\ note\ accept\AgdaUnderscore{}0\ is\ the\ same\ as\ acceptState}\<%
\\
\>[0]\AgdaFunction{accept-0}\AgdaSpace{}%
\AgdaSymbol{:}\AgdaSpace{}%
\AgdaFunction{StackStatePred}\<%
\\
\>[0]\AgdaFunction{accept-0}\AgdaSpace{}%
\AgdaSymbol{=}\AgdaSpace{}%
\AgdaFunction{stackPred2SPred}\AgdaSpace{}%
\AgdaFunction{accept-0Basic}\<%
\\
%
\\[\AgdaEmptyExtraSkip]%
%
\\[\AgdaEmptyExtraSkip]%
\>[0]\AgdaFunction{accept₁}\AgdaSpace{}%
\AgdaSymbol{:}\AgdaSpace{}%
\AgdaFunction{StackStatePred}\<%
\\
\>[0]\AgdaFunction{accept₁}%
\>[9]\AgdaSymbol{=}\AgdaSpace{}%
\AgdaFunction{stackPred2SPred}\AgdaSpace{}%
\AgdaFunction{accept₁ˢ}\<%
\\
%
\\[\AgdaEmptyExtraSkip]%
\>[0]\AgdaFunction{accept₂}\AgdaSpace{}%
\AgdaSymbol{:}\AgdaSpace{}%
\AgdaFunction{StackStatePred}\<%
\\
\>[0]\AgdaFunction{accept₂}\AgdaSpace{}%
\AgdaSymbol{=}\AgdaSpace{}%
\AgdaFunction{stackPred2SPred}\AgdaSpace{}%
\AgdaFunction{accept₂ˢ}\<%
\\
%
\\[\AgdaEmptyExtraSkip]%
\>[0]\AgdaFunction{accept₃}\AgdaSpace{}%
\AgdaSymbol{:}\AgdaSpace{}%
\AgdaFunction{StackStatePred}\<%
\\
\>[0]\AgdaFunction{accept₃}\AgdaSpace{}%
\AgdaSymbol{=}\AgdaSpace{}%
\AgdaFunction{stackPred2SPred}\AgdaSpace{}%
\AgdaFunction{accept₃ˢ}\<%
\\
%
\\[\AgdaEmptyExtraSkip]%
\>[0]\AgdaComment{--\ checked\ needs\ to\ be\ pbkh\ not\ pbk}\<%
\\
\>[0]\AgdaFunction{accept₄}\AgdaSpace{}%
\AgdaSymbol{:}\AgdaSpace{}%
\AgdaDatatype{ℕ}\AgdaSpace{}%
\AgdaSymbol{→}\AgdaSpace{}%
\AgdaFunction{StackStatePred}\<%
\\
\>[0]\AgdaFunction{accept₄}\AgdaSpace{}%
\AgdaBound{pbkh}%
\>[14]\AgdaSymbol{=}\AgdaSpace{}%
\AgdaFunction{stackPred2SPred}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaFunction{accept₄ˢ}\AgdaSpace{}%
\AgdaBound{pbkh}\AgdaSymbol{)}\<%
\\
%
\\[\AgdaEmptyExtraSkip]%
\>[0]\AgdaComment{--\ checked\ needs\ to\ be\ pbkh\ not\ pbk}\<%
\\
\>[0]\AgdaFunction{accept₅}\AgdaSpace{}%
\AgdaSymbol{:}\AgdaSpace{}%
\AgdaDatatype{ℕ}\AgdaSpace{}%
\AgdaSymbol{→}\AgdaSpace{}%
\AgdaFunction{StackStatePred}\<%
\\
\>[0]\AgdaFunction{accept₅}\AgdaSpace{}%
\AgdaBound{pbkh}%
\>[14]\AgdaSymbol{=}\AgdaSpace{}%
\AgdaFunction{stackPred2SPred}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaFunction{accept₅ˢ}\AgdaSpace{}%
\AgdaBound{pbkh}\AgdaSymbol{)}\<%
\\
%
\\[\AgdaEmptyExtraSkip]%
\>[0]\AgdaComment{--\ accept-6\ :\ ℕ\ →\ StackStatePred}\<%
\\
\>[0]\AgdaComment{--\ accept-6\ pbkh\ \ =\ stackPred2SPred\ (wPreCondP2PKHˢ\ pbkh)}\<%
\\
%
\\[\AgdaEmptyExtraSkip]%
\>[0]\AgdaComment{--\ checked\ needs\ to\ be\ pbkh\ not\ pbk}\<%
\\
\>[0]\AgdaFunction{wPreCondP2PKH}\AgdaSpace{}%
\AgdaSymbol{:}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaBound{pbkh}\AgdaSpace{}%
\AgdaSymbol{:}\AgdaSpace{}%
\AgdaDatatype{ℕ}\AgdaSymbol{)}%
\>[28]\AgdaSymbol{→}\AgdaSpace{}%
\AgdaFunction{StackStatePred}\<%
\\
\>[0]\AgdaFunction{wPreCondP2PKH}\AgdaSpace{}%
\AgdaBound{pbkh}%
\>[20]\AgdaSymbol{=}\AgdaSpace{}%
\AgdaFunction{stackPred2SPred}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaFunction{wPreCondP2PKHˢ}\AgdaSpace{}%
\AgdaBound{pbkh}\AgdaSymbol{)}\<%
\\
%
\\[\AgdaEmptyExtraSkip]%
\>[0]\AgdaComment{--\ we\ use\ pbk\ and\ not\ pbkh\ because\ that\ is\ what\ is\ provided\ by\ the\ unlocking\ script}\<%
\\
\>[0]\AgdaFunction{correct-opCheckSig-to}\AgdaSpace{}%
\AgdaSymbol{:}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaBound{s}\AgdaSpace{}%
\AgdaSymbol{:}\AgdaSpace{}%
\AgdaRecord{StackState}\AgdaSymbol{)}\AgdaSpace{}%
\AgdaSymbol{→}\AgdaSpace{}%
\AgdaFunction{accept₁}\AgdaSpace{}%
\AgdaBound{s}\AgdaSpace{}%
\AgdaSymbol{→}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaFunction{accept-0}\AgdaSpace{}%
\AgdaOperator{\AgdaFunction{⁺}}\AgdaSymbol{)}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaOperator{\AgdaFunction{⟦}}\AgdaSpace{}%
\AgdaInductiveConstructor{opCheckSig}\AgdaSpace{}%
\AgdaOperator{\AgdaFunction{⟧ₛ}}\AgdaSpace{}%
\AgdaBound{s}\AgdaSpace{}%
\AgdaSymbol{)}\<%
\\
\>[0]\AgdaFunction{correct-opCheckSig-to}\AgdaSpace{}%
\AgdaOperator{\AgdaInductiveConstructor{⟨}}\AgdaSpace{}%
\AgdaBound{time}\AgdaSpace{}%
\AgdaOperator{\AgdaInductiveConstructor{,}}\AgdaSpace{}%
\AgdaBound{msg₁}\AgdaSpace{}%
\AgdaOperator{\AgdaInductiveConstructor{,}}\AgdaSpace{}%
\AgdaBound{pbk}%
\>[43]\AgdaOperator{\AgdaInductiveConstructor{∷}}\AgdaSpace{}%
\AgdaBound{sig}\AgdaSpace{}%
\AgdaOperator{\AgdaInductiveConstructor{∷}}\AgdaSpace{}%
\AgdaBound{st}\AgdaSpace{}%
\AgdaOperator{\AgdaInductiveConstructor{⟩}}\AgdaSpace{}%
\AgdaBound{p}\AgdaSpace{}%
\AgdaSymbol{=}%
\>[61]\AgdaFunction{boolToNatNotFalseLemma}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaFunction{isSigned}%
\>[95]\AgdaBound{msg₁}\AgdaSpace{}%
\AgdaBound{sig}\AgdaSpace{}%
\AgdaBound{pbk}\AgdaSymbol{)}\AgdaSpace{}%
\AgdaBound{p}\<%
\\
%
\\[\AgdaEmptyExtraSkip]%
\>[0]\AgdaComment{\{-\ old}\<%
\\
\>[0]\AgdaComment{correct-1-to\ :\ (s\ :\ StackState)\ →\ accept₁\ s\ →\ (accept-0\ ⁺)\ (⟦\ opCheckSig\ ⟧s\ s\ )}\<%
\\
\>[0]\AgdaComment{correct-1-to\ ⟨\ time\ ,\ msg₁\ ,\ pbk\ \ ∷\ sig\ ∷\ st\ ⟩\ p\ =\ \ boolToNatNotFalseLemma\ (isSigned\ \ msg₁\ sig\ pbk)\ p}\<%
\\
\>[0]\AgdaComment{-\}}\<%
\\
%
\\[\AgdaEmptyExtraSkip]%
\>[0]\AgdaFunction{correct-opCheckSig-from}\AgdaSpace{}%
\AgdaSymbol{:}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaBound{s}\AgdaSpace{}%
\AgdaSymbol{:}\AgdaSpace{}%
\AgdaRecord{StackState}\AgdaSymbol{)}\AgdaSpace{}%
\AgdaSymbol{→}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaFunction{accept-0}\AgdaSpace{}%
\AgdaOperator{\AgdaFunction{⁺}}\AgdaSymbol{)}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaOperator{\AgdaFunction{⟦}}\AgdaSpace{}%
\AgdaInductiveConstructor{opCheckSig}\AgdaSpace{}%
\AgdaOperator{\AgdaFunction{⟧ₛ}}\AgdaSpace{}%
\AgdaBound{s}\AgdaSpace{}%
\AgdaSymbol{)}\AgdaSpace{}%
\AgdaSymbol{→}\AgdaSpace{}%
\AgdaFunction{accept₁}\AgdaSpace{}%
\AgdaBound{s}\<%
\\
\>[0]\AgdaFunction{correct-opCheckSig-from}\AgdaSpace{}%
\AgdaOperator{\AgdaInductiveConstructor{⟨}}\AgdaSpace{}%
\AgdaBound{time}\AgdaSpace{}%
\AgdaOperator{\AgdaInductiveConstructor{,}}\AgdaSpace{}%
\AgdaBound{msg₁}\AgdaSpace{}%
\AgdaOperator{\AgdaInductiveConstructor{,}}\AgdaSpace{}%
\AgdaBound{pbk}\AgdaSpace{}%
\AgdaOperator{\AgdaInductiveConstructor{∷}}\AgdaSpace{}%
\AgdaBound{sig}\AgdaSpace{}%
\AgdaOperator{\AgdaInductiveConstructor{∷}}\AgdaSpace{}%
\AgdaBound{stack₁}%
\>[60]\AgdaOperator{\AgdaInductiveConstructor{⟩}}\AgdaSpace{}%
\AgdaBound{p}\AgdaSpace{}%
\AgdaSymbol{=}\AgdaSpace{}%
\AgdaFunction{boolToNatNotFalseLemma2}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaFunction{isSigned}%
\>[101]\AgdaBound{msg₁}\AgdaSpace{}%
\AgdaBound{sig}\AgdaSpace{}%
\AgdaBound{pbk}\AgdaSymbol{)}\AgdaSpace{}%
\AgdaBound{p}\<%
\\
%
\\[\AgdaEmptyExtraSkip]%
\>[0]\AgdaComment{\{-old}\<%
\\
\>[0]\AgdaComment{correct-1-from\ :\ (s\ :\ StackState)\ →\ (accept-0\ ⁺)\ (⟦\ opCheckSig\ ⟧s\ s\ )\ →\ accept₁\ s}\<%
\\
\>[0]\AgdaComment{correct-1-from\ ⟨\ time\ ,\ msg₁\ ,\ pbk\ ∷\ sig\ ∷\ stack₁\ \ ⟩\ p\ =\ boolToNatNotFalseLemma2\ (isSigned\ \ msg₁\ sig\ pbk)\ p}\<%
\\
\>[0]\AgdaComment{-\}}\<%
\end{code}
} % END AgdaHide

\newcommand{\stackVerificationPtoPKHcorrectone}{
\begin{code}[inline]%
\>[0]\AgdaFunction{correct-opCheckSig}\AgdaSpace{}%
\AgdaSymbol{:}\AgdaSpace{}%
\AgdaOperator{\AgdaRecord{<}}\AgdaSpace{}%
\AgdaFunction{accept₁}\AgdaSpace{}%
\AgdaOperator{\AgdaRecord{>ⁱᶠᶠ}}%
\>[37]\AgdaSymbol{(}\AgdaOperator{\AgdaFunction{[}}\AgdaSpace{}%
\AgdaInductiveConstructor{opCheckSig}\AgdaSpace{}%
\AgdaOperator{\AgdaFunction{]}}\AgdaSymbol{)}\AgdaSpace{}%
\AgdaOperator{\AgdaRecord{<}}\AgdaSpace{}%
\AgdaFunction{acceptState}\AgdaSpace{}%
\AgdaOperator{\AgdaRecord{>}}\<%
\end{code}
} % END newcommand

\AgdaHide{
\begin{code}%
\>[0]\AgdaFunction{correct-opCheckSig}\AgdaSpace{}%
\AgdaSymbol{.}\AgdaField{==>}\AgdaSpace{}%
\AgdaSymbol{=}\AgdaSpace{}%
\AgdaFunction{correct-opCheckSig-to}\<%
\\
\>[0]\AgdaFunction{correct-opCheckSig}\AgdaSpace{}%
\AgdaSymbol{.}\AgdaField{<==}\AgdaSpace{}%
\AgdaSymbol{=}\AgdaSpace{}%
\AgdaFunction{correct-opCheckSig-from}\<%
\\
\>[0]\AgdaComment{\{-old}\<%
\\
\>[0]\AgdaComment{-@BEGININLINE@correctone}\<%
\\
\>[0]\AgdaComment{correct-1\ :\ <\ accept₁\ >iff\ \ ([\ opCheckSig\ ])\ <\ acceptState\ >}\<%
\\
\>[0]\AgdaComment{-@END}\<%
\\
\>[0]\AgdaComment{correct-1\ .==>\ =\ correct-1-to}\<%
\\
\>[0]\AgdaComment{correct-1\ .<==\ =\ correct-1-from}\<%
\\
\>[0]\AgdaComment{-\}}\<%
\\
%
\\[\AgdaEmptyExtraSkip]%
\>[0]\AgdaFunction{correct-opVerify-to}\AgdaSpace{}%
\AgdaSymbol{:}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaBound{s}\AgdaSpace{}%
\AgdaSymbol{:}\AgdaSpace{}%
\AgdaRecord{StackState}\AgdaSymbol{)}\AgdaSpace{}%
\AgdaSymbol{→}\AgdaSpace{}%
\AgdaFunction{accept₂}\AgdaSpace{}%
\AgdaBound{s}\AgdaSpace{}%
\AgdaSymbol{→}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaFunction{accept₁}\AgdaSpace{}%
\AgdaOperator{\AgdaFunction{⁺}}\AgdaSymbol{)}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaOperator{\AgdaFunction{⟦}}\AgdaSpace{}%
\AgdaInductiveConstructor{opVerify}\AgdaSpace{}%
\AgdaOperator{\AgdaFunction{⟧ₛ}}\AgdaSpace{}%
\AgdaBound{s}\AgdaSpace{}%
\AgdaSymbol{)}\<%
\\
\>[0]\AgdaFunction{correct-opVerify-to}\AgdaSpace{}%
\AgdaOperator{\AgdaInductiveConstructor{⟨}}\AgdaSpace{}%
\AgdaBound{time}\AgdaSpace{}%
\AgdaOperator{\AgdaInductiveConstructor{,}}\AgdaSpace{}%
\AgdaBound{msg₁}\AgdaSpace{}%
\AgdaOperator{\AgdaInductiveConstructor{,}}\AgdaSpace{}%
\AgdaInductiveConstructor{suc}\AgdaSpace{}%
\AgdaBound{x}\AgdaSpace{}%
\AgdaOperator{\AgdaInductiveConstructor{∷}}\AgdaSpace{}%
\AgdaBound{x₁}\AgdaSpace{}%
\AgdaOperator{\AgdaInductiveConstructor{∷}}\AgdaSpace{}%
\AgdaBound{x₂}\AgdaSpace{}%
\AgdaOperator{\AgdaInductiveConstructor{∷}}\AgdaSpace{}%
\AgdaBound{stack₁}\AgdaSpace{}%
\AgdaOperator{\AgdaInductiveConstructor{⟩}}\AgdaSpace{}%
\AgdaBound{p}\AgdaSpace{}%
\AgdaSymbol{=}\AgdaSpace{}%
\AgdaBound{p}\<%
\\
%
\\[\AgdaEmptyExtraSkip]%
\>[0]\AgdaFunction{correct-opVerify-from}\AgdaSpace{}%
\AgdaSymbol{:}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaBound{s}\AgdaSpace{}%
\AgdaSymbol{:}\AgdaSpace{}%
\AgdaRecord{StackState}\AgdaSymbol{)}\AgdaSpace{}%
\AgdaSymbol{→}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaFunction{accept₁}\AgdaSpace{}%
\AgdaOperator{\AgdaFunction{⁺}}\AgdaSymbol{)}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaOperator{\AgdaFunction{⟦}}\AgdaSpace{}%
\AgdaInductiveConstructor{opVerify}\AgdaSpace{}%
\AgdaOperator{\AgdaFunction{⟧ₛ}}\AgdaSpace{}%
\AgdaBound{s}\AgdaSpace{}%
\AgdaSymbol{)}\AgdaSpace{}%
\AgdaSymbol{→}\AgdaSpace{}%
\AgdaFunction{accept₂}\AgdaSpace{}%
\AgdaBound{s}\<%
\\
\>[0]\AgdaFunction{correct-opVerify-from}\AgdaSpace{}%
\AgdaOperator{\AgdaInductiveConstructor{⟨}}\AgdaSpace{}%
\AgdaBound{time}\AgdaSpace{}%
\AgdaOperator{\AgdaInductiveConstructor{,}}\AgdaSpace{}%
\AgdaBound{msg₁}\AgdaSpace{}%
\AgdaOperator{\AgdaInductiveConstructor{,}}\AgdaSpace{}%
\AgdaInductiveConstructor{suc}\AgdaSpace{}%
\AgdaBound{x}\AgdaSpace{}%
\AgdaOperator{\AgdaInductiveConstructor{∷}}\AgdaSpace{}%
\AgdaBound{x₁}\AgdaSpace{}%
\AgdaOperator{\AgdaInductiveConstructor{∷}}\AgdaSpace{}%
\AgdaBound{x₂}\AgdaSpace{}%
\AgdaOperator{\AgdaInductiveConstructor{∷}}\AgdaSpace{}%
\AgdaBound{stack₁}\AgdaSpace{}%
\AgdaOperator{\AgdaInductiveConstructor{⟩}}\AgdaSpace{}%
\AgdaBound{p}\AgdaSpace{}%
\AgdaSymbol{=}\AgdaSpace{}%
\AgdaBound{p}\<%
\\
\>[0]\<%
\end{code}
} % END AgdaHide

\newcommand{\stackVerificationPtoPKHcorrecttwo}{
\begin{code}[inline]%
\>[0]\AgdaFunction{correct-opVerify}\AgdaSpace{}%
\AgdaSymbol{:}\AgdaSpace{}%
\AgdaOperator{\AgdaRecord{<}}\AgdaSpace{}%
\AgdaFunction{accept₂}\AgdaSpace{}%
\AgdaOperator{\AgdaRecord{>ⁱᶠᶠ}}%
\>[35]\AgdaSymbol{(}\AgdaOperator{\AgdaFunction{[}}\AgdaSpace{}%
\AgdaInductiveConstructor{opVerify}\AgdaSpace{}%
\AgdaOperator{\AgdaFunction{]}}\AgdaSymbol{)}\AgdaSpace{}%
\AgdaOperator{\AgdaRecord{<}}\AgdaSpace{}%
\AgdaFunction{accept₁}\AgdaSpace{}%
\AgdaOperator{\AgdaRecord{>}}\<%
\end{code}
} % END newcommand

\AgdaHide{
\begin{code}%
\>[0]\AgdaFunction{correct-opVerify}\AgdaSpace{}%
\AgdaSymbol{.}\AgdaField{==>}\AgdaSpace{}%
\AgdaSymbol{=}\AgdaSpace{}%
\AgdaFunction{correct-opVerify-to}\<%
\\
\>[0]\AgdaFunction{correct-opVerify}\AgdaSpace{}%
\AgdaSymbol{.}\AgdaField{<==}\AgdaSpace{}%
\AgdaSymbol{=}\AgdaSpace{}%
\AgdaFunction{correct-opVerify-from}\<%
\\
%
\\[\AgdaEmptyExtraSkip]%
\>[0]\AgdaComment{\{-old}\<%
\\
\>[0]\AgdaComment{correct-2-to\ :\ (s\ :\ StackState)\ →\ accept₂\ s\ →\ (accept₁\ ⁺)\ (⟦\ opVerify\ ⟧s\ s\ )}\<%
\\
\>[0]\AgdaComment{correct-2-to\ ⟨\ time\ ,\ msg₁\ ,\ suc\ x\ ∷\ x₁\ ∷\ x₂\ ∷\ stack₁\ ⟩\ p\ =\ p}\<%
\\
\>[0]\<%
\\
\>[0]\AgdaComment{correct-2-from\ :\ (s\ :\ StackState)\ →\ (accept₁\ ⁺)\ (⟦\ opVerify\ ⟧s\ s\ )\ →\ accept₂\ s}\<%
\\
\>[0]\AgdaComment{correct-2-from\ ⟨\ time\ ,\ msg₁\ ,\ suc\ x\ ∷\ x₁\ ∷\ x₂\ ∷\ stack₁\ ⟩\ p\ =\ p}\<%
\\
\>[0]\<%
\\
\>[0]\AgdaComment{-@BEGININLINE@correcttwo}\<%
\\
\>[0]\AgdaComment{correct-2\ :\ <\ accept₂\ >iff\ \ ([\ opVerify\ ])\ <\ accept₁\ >}\<%
\\
\>[0]\AgdaComment{-@END}\<%
\\
\>[0]\AgdaComment{correct-2\ .==>\ =\ correct-2-to}\<%
\\
\>[0]\AgdaComment{correct-2\ .<==\ =\ correct-2-from}\<%
\\
\>[0]\AgdaComment{-\}}\<%
\\
%
\\[\AgdaEmptyExtraSkip]%
%
\\[\AgdaEmptyExtraSkip]%
\>[0]\AgdaFunction{correct-opEqual-to}\AgdaSpace{}%
\AgdaSymbol{:}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaBound{s}\AgdaSpace{}%
\AgdaSymbol{:}\AgdaSpace{}%
\AgdaRecord{StackState}\AgdaSymbol{)}\AgdaSpace{}%
\AgdaSymbol{→}\AgdaSpace{}%
\AgdaFunction{accept₃}\AgdaSpace{}%
\AgdaBound{s}\AgdaSpace{}%
\AgdaSymbol{→}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaFunction{accept₂}\AgdaSpace{}%
\AgdaOperator{\AgdaFunction{⁺}}\AgdaSymbol{)}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaOperator{\AgdaFunction{⟦}}\AgdaSpace{}%
\AgdaInductiveConstructor{opEqual}\AgdaSpace{}%
\AgdaOperator{\AgdaFunction{⟧ₛ}}\AgdaSpace{}%
\AgdaBound{s}\AgdaSpace{}%
\AgdaSymbol{)}\<%
\\
\>[0]\AgdaFunction{correct-opEqual-to}\AgdaSpace{}%
\AgdaOperator{\AgdaInductiveConstructor{⟨}}\AgdaSpace{}%
\AgdaBound{time}\AgdaSpace{}%
\AgdaOperator{\AgdaInductiveConstructor{,}}\AgdaSpace{}%
\AgdaBound{msg₁}\AgdaSpace{}%
\AgdaOperator{\AgdaInductiveConstructor{,}}\AgdaSpace{}%
\AgdaBound{pbk1}%
\>[41]\AgdaOperator{\AgdaInductiveConstructor{∷}}\AgdaSpace{}%
\AgdaDottedPattern{\AgdaSymbol{.}}\AgdaDottedPattern{\AgdaBound{pbk1}}\AgdaSpace{}%
\AgdaOperator{\AgdaInductiveConstructor{∷}}\AgdaSpace{}%
\AgdaBound{pbk2}\AgdaSpace{}%
\AgdaOperator{\AgdaInductiveConstructor{∷}}%
\>[59]\AgdaBound{sig}\AgdaSpace{}%
\AgdaOperator{\AgdaInductiveConstructor{∷}}\AgdaSpace{}%
\AgdaInductiveConstructor{[]}%
\>[69]\AgdaOperator{\AgdaInductiveConstructor{⟩}}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaInductiveConstructor{conj}\AgdaSpace{}%
\AgdaInductiveConstructor{refl}\AgdaSpace{}%
\AgdaBound{checkSig}\AgdaSymbol{)}%
\>[93]\AgdaKeyword{rewrite}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaSpace{}%
\AgdaFunction{lemmaCompareNat}\AgdaSpace{}%
\AgdaBound{pbk1}\AgdaSpace{}%
\AgdaSymbol{)}\AgdaSpace{}%
\AgdaSymbol{=}%
\>[129]\AgdaBound{checkSig}\<%
\\
\>[0]\AgdaFunction{correct-opEqual-to}\AgdaSpace{}%
\AgdaOperator{\AgdaInductiveConstructor{⟨}}\AgdaSpace{}%
\AgdaBound{time}\AgdaSpace{}%
\AgdaOperator{\AgdaInductiveConstructor{,}}\AgdaSpace{}%
\AgdaBound{msg₁}\AgdaSpace{}%
\AgdaOperator{\AgdaInductiveConstructor{,}}\AgdaSpace{}%
\AgdaBound{pbk1}\AgdaSpace{}%
\AgdaOperator{\AgdaInductiveConstructor{∷}}\AgdaSpace{}%
\AgdaDottedPattern{\AgdaSymbol{.}}\AgdaDottedPattern{\AgdaBound{pbk1}}\AgdaSpace{}%
\AgdaOperator{\AgdaInductiveConstructor{∷}}\AgdaSpace{}%
\AgdaBound{pbk2}%
\>[56]\AgdaOperator{\AgdaInductiveConstructor{∷}}\AgdaSpace{}%
\AgdaBound{sig}\AgdaSpace{}%
\AgdaOperator{\AgdaInductiveConstructor{∷}}\AgdaSpace{}%
\AgdaBound{x}\AgdaSpace{}%
\AgdaOperator{\AgdaInductiveConstructor{∷}}\AgdaSpace{}%
\AgdaBound{rest}%
\>[74]\AgdaOperator{\AgdaInductiveConstructor{⟩}}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaInductiveConstructor{conj}\AgdaSpace{}%
\AgdaInductiveConstructor{refl}\AgdaSpace{}%
\AgdaBound{checkSig}\AgdaSymbol{)}\AgdaSpace{}%
\AgdaKeyword{rewrite}%
\>[106]\AgdaSymbol{(}\AgdaSpace{}%
\AgdaFunction{lemmaCompareNat}\AgdaSpace{}%
\AgdaBound{pbk1}\AgdaSpace{}%
\AgdaSymbol{)}\AgdaSpace{}%
\AgdaSymbol{=}\AgdaSpace{}%
\AgdaBound{checkSig}\<%
\\
%
\\[\AgdaEmptyExtraSkip]%
\>[0]\AgdaFunction{correct-opEqual-from}%
\>[22]\AgdaSymbol{:}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaBound{s}\AgdaSpace{}%
\AgdaSymbol{:}\AgdaSpace{}%
\AgdaRecord{StackState}\AgdaSymbol{)}%
\>[42]\AgdaSymbol{→}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaFunction{accept₂}\AgdaSpace{}%
\AgdaOperator{\AgdaFunction{⁺}}\AgdaSymbol{)}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaOperator{\AgdaFunction{⟦}}\AgdaSpace{}%
\AgdaInductiveConstructor{opEqual}\AgdaSpace{}%
\AgdaOperator{\AgdaFunction{⟧ₛ}}\AgdaSpace{}%
\AgdaBound{s}\AgdaSpace{}%
\AgdaSymbol{)}\AgdaSpace{}%
\AgdaSymbol{→}\AgdaSpace{}%
\AgdaFunction{accept₃}\AgdaSpace{}%
\AgdaBound{s}\<%
\\
\>[0]\AgdaFunction{correct-opEqual-from}\AgdaSpace{}%
\AgdaOperator{\AgdaInductiveConstructor{⟨}}\AgdaSpace{}%
\AgdaBound{time}\AgdaSpace{}%
\AgdaOperator{\AgdaInductiveConstructor{,}}\AgdaSpace{}%
\AgdaBound{msg₁}\AgdaSpace{}%
\AgdaOperator{\AgdaInductiveConstructor{,}}\AgdaSpace{}%
\AgdaBound{x}\AgdaSpace{}%
\AgdaOperator{\AgdaInductiveConstructor{∷}}\AgdaSpace{}%
\AgdaBound{x₁}\AgdaSpace{}%
\AgdaOperator{\AgdaInductiveConstructor{∷}}\AgdaSpace{}%
\AgdaBound{pbk}\AgdaSpace{}%
\AgdaOperator{\AgdaInductiveConstructor{∷}}\AgdaSpace{}%
\AgdaBound{sig}\AgdaSpace{}%
\AgdaOperator{\AgdaInductiveConstructor{∷}}\AgdaSpace{}%
\AgdaBound{stack₁}%
\>[66]\AgdaOperator{\AgdaInductiveConstructor{⟩}}\AgdaSpace{}%
\AgdaBound{p}\AgdaSpace{}%
\AgdaKeyword{rewrite}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaSpace{}%
\AgdaFunction{lemmaCorrect3From}\AgdaSpace{}%
\AgdaBound{x}\AgdaSpace{}%
\AgdaBound{x₁}\AgdaSpace{}%
\AgdaBound{pbk}\AgdaSpace{}%
\AgdaBound{sig}\AgdaSpace{}%
\AgdaBound{time}\AgdaSpace{}%
\AgdaBound{msg₁}\AgdaSpace{}%
\AgdaBound{p}\AgdaSpace{}%
\AgdaSymbol{)}\<%
\\
\>[0][@{}l@{\AgdaIndent{0}}]%
\>[2]\AgdaSymbol{=}%
\>[6]\AgdaKeyword{let}\<%
\\
\>[6][@{}l@{\AgdaIndent{0}}]%
\>[8]\AgdaBound{q}\AgdaSpace{}%
\AgdaSymbol{:}\AgdaSpace{}%
\AgdaFunction{True}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaFunction{isSigned}%
\>[28]\AgdaBound{msg₁}\AgdaSpace{}%
\AgdaBound{sig}\AgdaSpace{}%
\AgdaBound{pbk}\AgdaSymbol{)}\<%
\\
%
\>[8]\AgdaBound{q}\AgdaSpace{}%
\AgdaSymbol{=}\AgdaSpace{}%
\AgdaFunction{correct3Aux2}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaFunction{compareNaturals}\AgdaSpace{}%
\AgdaBound{x}\AgdaSpace{}%
\AgdaBound{x₁}\AgdaSymbol{)}\AgdaSpace{}%
\AgdaBound{pbk}\AgdaSpace{}%
\AgdaBound{sig}\AgdaSpace{}%
\AgdaBound{stack₁}\AgdaSpace{}%
\AgdaBound{time}\AgdaSpace{}%
\AgdaBound{msg₁}\AgdaSpace{}%
\AgdaBound{p}\<%
\\
%
\>[6]\AgdaKeyword{in}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaInductiveConstructor{conj}\AgdaSpace{}%
\AgdaInductiveConstructor{refl}\AgdaSpace{}%
\AgdaBound{q}\AgdaSymbol{)}\<%
\\
\>[0]\<%
\end{code}
} % END AgdaHide

\newcommand{\stackVerificationPtoPKHcorrectthree}{
\begin{code}[inline]%
\>[0]\AgdaFunction{correct-opEqual}\AgdaSpace{}%
\AgdaSymbol{:}\AgdaSpace{}%
\AgdaOperator{\AgdaRecord{<}}\AgdaSpace{}%
\AgdaFunction{accept₃}\AgdaSpace{}%
\AgdaOperator{\AgdaRecord{>ⁱᶠᶠ}}%
\>[34]\AgdaSymbol{(}\AgdaOperator{\AgdaFunction{[}}\AgdaSpace{}%
\AgdaInductiveConstructor{opEqual}\AgdaSpace{}%
\AgdaOperator{\AgdaFunction{]}}\AgdaSymbol{)}\AgdaSpace{}%
\AgdaOperator{\AgdaRecord{<}}\AgdaSpace{}%
\AgdaFunction{accept₂}\AgdaSpace{}%
\AgdaOperator{\AgdaRecord{>}}\<%
\end{code}
} % END newcommand

\AgdaHide{
\begin{code}%
\>[0]\AgdaFunction{correct-opEqual}\AgdaSpace{}%
\AgdaSymbol{.}\AgdaField{==>}\AgdaSpace{}%
\AgdaSymbol{=}\AgdaSpace{}%
\AgdaFunction{correct-opEqual-to}\<%
\\
\>[0]\AgdaFunction{correct-opEqual}\AgdaSpace{}%
\AgdaSymbol{.}\AgdaField{<==}\AgdaSpace{}%
\AgdaSymbol{=}\AgdaSpace{}%
\AgdaFunction{correct-opEqual-from}\<%
\\
%
\\[\AgdaEmptyExtraSkip]%
\>[0]\AgdaComment{\{-old}\<%
\\
\>[0]\<%
\\
\>[0]\AgdaComment{correct-3-to\ :\ (s\ :\ StackState)\ →\ accept₃\ s\ →\ (accept₂\ ⁺)\ (⟦\ opEqual\ ⟧s\ s\ )}\<%
\\
\>[0]\AgdaComment{correct-3-to\ ⟨\ time\ ,\ msg₁\ ,\ pbk1\ \ ∷\ .pbk1\ ∷\ pbk2\ ∷\ \ sig\ ∷\ []\ \ ⟩\ (conj\ refl\ checkSig)\ \ rewrite\ (\ lemmaCompareNat\ pbk1\ )\ =\ \ checkSig}\<%
\\
\>[0]\AgdaComment{correct-3-to\ ⟨\ time\ ,\ msg₁\ ,\ pbk1\ ∷\ .pbk1\ ∷\ pbk2\ \ ∷\ sig\ ∷\ x\ ∷\ rest\ \ ⟩\ (conj\ refl\ checkSig)\ rewrite\ \ (\ lemmaCompareNat\ pbk1\ )\ =\ checkSig}\<%
\\
\>[0]\<%
\\
\>[0]\AgdaComment{correct-3-from\ \ :\ (s\ :\ StackState)\ \ →\ (accept₂\ ⁺)\ (⟦\ opEqual\ ⟧s\ s\ )\ →\ accept₃\ s}\<%
\\
\>[0]\AgdaComment{correct-3-from\ ⟨\ time\ ,\ msg₁\ ,\ x\ ∷\ x₁\ ∷\ pbk\ ∷\ sig\ ∷\ stack₁\ \ ⟩\ p\ rewrite\ (\ lemmaCorrect3From\ x\ x₁\ pbk\ sig\ time\ msg₁\ p\ )}\<%
\\
\>[0]\AgdaComment{\ \ =\ \ \ let}\<%
\\
\>[0]\AgdaComment{\ \ \ \ \ \ \ \ q\ :\ True\ (isSigned\ \ msg₁\ sig\ pbk)}\<%
\\
\>[0]\AgdaComment{\ \ \ \ \ \ \ \ q\ =\ correct3Aux2\ (compareNaturals\ x\ x₁)\ pbk\ sig\ stack₁\ time\ msg₁\ p}\<%
\\
\>[0]\AgdaComment{\ \ \ \ \ \ in\ (conj\ refl\ q)}\<%
\\
\>[0]\<%
\\
\>[0]\AgdaComment{-@BEGININLINE@correctthree}\<%
\\
\>[0]\AgdaComment{correct-3\ :\ <\ accept₃\ >iff\ \ ([\ opEqual\ ])\ <\ accept₂\ >}\<%
\\
\>[0]\AgdaComment{-@END}\<%
\\
\>[0]\AgdaComment{correct-3\ .==>\ =\ correct-3-to}\<%
\\
\>[0]\AgdaComment{correct-3\ .<==\ =\ correct-3-from}\<%
\\
\>[0]\AgdaComment{-\}}\<%
\\
%
\\[\AgdaEmptyExtraSkip]%
\>[0]\AgdaComment{--\ needs\ to\ be\ pbkh\ since\ opPush\ refers\ to\ it}\<%
\\
\>[0]\AgdaFunction{correct-opPush-to}\AgdaSpace{}%
\AgdaSymbol{:}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaSpace{}%
\AgdaBound{pbkh}\AgdaSpace{}%
\AgdaSymbol{:}\AgdaSpace{}%
\AgdaDatatype{ℕ}\AgdaSpace{}%
\AgdaSymbol{)}\AgdaSpace{}%
\AgdaSymbol{→}%
\>[36]\AgdaSymbol{(}\AgdaBound{s}\AgdaSpace{}%
\AgdaSymbol{:}\AgdaSpace{}%
\AgdaRecord{StackState}\AgdaSymbol{)}\AgdaSpace{}%
\AgdaSymbol{→}\AgdaSpace{}%
\AgdaFunction{accept₄}\AgdaSpace{}%
\AgdaBound{pbkh}%
\>[69]\AgdaBound{s}\AgdaSpace{}%
\AgdaSymbol{→}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaFunction{accept₃}\AgdaSpace{}%
\AgdaOperator{\AgdaFunction{⁺}}\AgdaSymbol{)}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaOperator{\AgdaFunction{⟦}}\AgdaSpace{}%
\AgdaInductiveConstructor{opPush}\AgdaSpace{}%
\AgdaBound{pbkh}\AgdaSpace{}%
\AgdaOperator{\AgdaFunction{⟧ₛ}}\AgdaSpace{}%
\AgdaBound{s}\AgdaSpace{}%
\AgdaSymbol{)}\<%
\\
\>[0]\AgdaFunction{correct-opPush-to}\AgdaSpace{}%
\AgdaBound{pbkh}\AgdaSpace{}%
\AgdaOperator{\AgdaInductiveConstructor{⟨}}\AgdaSpace{}%
\AgdaBound{currentTime₁}\AgdaSpace{}%
\AgdaOperator{\AgdaInductiveConstructor{,}}\AgdaSpace{}%
\AgdaBound{msg₁}\AgdaSpace{}%
\AgdaOperator{\AgdaInductiveConstructor{,}}\AgdaSpace{}%
\AgdaDottedPattern{\AgdaSymbol{.}}\AgdaDottedPattern{\AgdaBound{pbkh}}\AgdaSpace{}%
\AgdaOperator{\AgdaInductiveConstructor{∷}}\AgdaSpace{}%
\AgdaBound{x₁}\AgdaSpace{}%
\AgdaOperator{\AgdaInductiveConstructor{∷}}\AgdaSpace{}%
\AgdaBound{x₂}\AgdaSpace{}%
\AgdaOperator{\AgdaInductiveConstructor{∷}}\AgdaSpace{}%
\AgdaBound{stack₁}\AgdaSpace{}%
\AgdaOperator{\AgdaInductiveConstructor{⟩}}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaInductiveConstructor{conj}\AgdaSpace{}%
\AgdaInductiveConstructor{refl}\AgdaSpace{}%
\AgdaBound{and4}\AgdaSymbol{)}\AgdaSpace{}%
\AgdaSymbol{=}\AgdaSpace{}%
\AgdaInductiveConstructor{conj}\AgdaSpace{}%
\AgdaInductiveConstructor{refl}\AgdaSpace{}%
\AgdaBound{and4}\<%
\\
%
\\[\AgdaEmptyExtraSkip]%
%
\\[\AgdaEmptyExtraSkip]%
\>[0]\AgdaFunction{correct-opPush-from}\AgdaSpace{}%
\AgdaSymbol{:}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaSpace{}%
\AgdaBound{pbkh}\AgdaSpace{}%
\AgdaSymbol{:}\AgdaSpace{}%
\AgdaDatatype{ℕ}\AgdaSpace{}%
\AgdaSymbol{)}\AgdaSpace{}%
\AgdaSymbol{→}%
\>[38]\AgdaSymbol{(}\AgdaBound{s}\AgdaSpace{}%
\AgdaSymbol{:}\AgdaSpace{}%
\AgdaRecord{StackState}\AgdaSymbol{)}\AgdaSpace{}%
\AgdaSymbol{→}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaFunction{accept₃}\AgdaSpace{}%
\AgdaOperator{\AgdaFunction{⁺}}\AgdaSymbol{)}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaOperator{\AgdaFunction{⟦}}\AgdaSpace{}%
\AgdaInductiveConstructor{opPush}\AgdaSpace{}%
\AgdaBound{pbkh}\AgdaSpace{}%
\AgdaOperator{\AgdaFunction{⟧ₛ}}\AgdaSpace{}%
\AgdaBound{s}\AgdaSpace{}%
\AgdaSymbol{)}\AgdaSpace{}%
\AgdaSymbol{→}\AgdaSpace{}%
\AgdaFunction{accept₄}\AgdaSpace{}%
\AgdaBound{pbkh}%
\>[107]\AgdaBound{s}\<%
\\
\>[0]\AgdaFunction{correct-opPush-from}\AgdaSpace{}%
\AgdaBound{pbkh}\AgdaSpace{}%
\AgdaOperator{\AgdaInductiveConstructor{⟨}}\AgdaSpace{}%
\AgdaBound{currentTime₁}\AgdaSpace{}%
\AgdaOperator{\AgdaInductiveConstructor{,}}\AgdaSpace{}%
\AgdaBound{msg₁}\AgdaSpace{}%
\AgdaOperator{\AgdaInductiveConstructor{,}}\AgdaSpace{}%
\AgdaDottedPattern{\AgdaSymbol{.}}\AgdaDottedPattern{\AgdaBound{pbkh}}\AgdaSpace{}%
\AgdaOperator{\AgdaInductiveConstructor{∷}}\AgdaSpace{}%
\AgdaBound{x₁}\AgdaSpace{}%
\AgdaOperator{\AgdaInductiveConstructor{∷}}\AgdaSpace{}%
\AgdaBound{x₂}\AgdaSpace{}%
\AgdaOperator{\AgdaInductiveConstructor{∷}}\AgdaSpace{}%
\AgdaBound{stack₁}%
\>[76]\AgdaOperator{\AgdaInductiveConstructor{⟩}}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaInductiveConstructor{conj}\AgdaSpace{}%
\AgdaInductiveConstructor{refl}\AgdaSpace{}%
\AgdaBound{and4}\AgdaSymbol{)}\AgdaSpace{}%
\AgdaSymbol{=}\AgdaSpace{}%
\AgdaInductiveConstructor{conj}\AgdaSpace{}%
\AgdaInductiveConstructor{refl}\AgdaSpace{}%
\AgdaBound{and4}\<%
\\
\>[0]\<%
\end{code}
} % END AgdaHide

\newcommand{\stackVerificationPtoPKHcorrectfour}{
\begin{code}[inline]%
\>[0]\AgdaFunction{correct-opPush}\AgdaSpace{}%
\AgdaSymbol{:(}\AgdaSpace{}%
\AgdaBound{pbkh}\AgdaSpace{}%
\AgdaSymbol{:}\AgdaSpace{}%
\AgdaDatatype{ℕ}\AgdaSpace{}%
\AgdaSymbol{)}\AgdaSpace{}%
\AgdaSymbol{→}%
\>[32]\AgdaOperator{\AgdaRecord{<}}\AgdaSpace{}%
\AgdaFunction{accept₄}\AgdaSpace{}%
\AgdaBound{pbkh}\AgdaSpace{}%
\AgdaOperator{\AgdaRecord{>ⁱᶠᶠ}}%
\>[53]\AgdaSymbol{(}\AgdaOperator{\AgdaFunction{[}}\AgdaSpace{}%
\AgdaInductiveConstructor{opPush}\AgdaSpace{}%
\AgdaBound{pbkh}\AgdaSpace{}%
\AgdaOperator{\AgdaFunction{]}}\AgdaSymbol{)}\AgdaSpace{}%
\AgdaOperator{\AgdaRecord{<}}\AgdaSpace{}%
\AgdaFunction{accept₃}\AgdaSpace{}%
\AgdaOperator{\AgdaRecord{>}}\<%
\end{code}
} % END newcommand

\AgdaHide{
\begin{code}%
\>[0]\AgdaFunction{correct-opPush}\AgdaSpace{}%
\AgdaBound{pbkh}\AgdaSpace{}%
\AgdaSymbol{.}\AgdaField{==>}\AgdaSpace{}%
\AgdaSymbol{=}\AgdaSpace{}%
\AgdaFunction{correct-opPush-to}\AgdaSpace{}%
\AgdaBound{pbkh}\<%
\\
\>[0]\AgdaFunction{correct-opPush}\AgdaSpace{}%
\AgdaBound{pbkh}\AgdaSpace{}%
\AgdaSymbol{.}\AgdaField{<==}\AgdaSpace{}%
\AgdaSymbol{=}\AgdaSpace{}%
\AgdaFunction{correct-opPush-from}\AgdaSpace{}%
\AgdaBound{pbkh}\<%
\\
%
\\[\AgdaEmptyExtraSkip]%
%
\\[\AgdaEmptyExtraSkip]%
\>[0]\AgdaComment{\{-old}\<%
\\
\>[0]\<%
\\
\>[0]\<%
\\
\>[0]\AgdaComment{correct-4-to\ :\ (\ pbk\ :\ ℕ\ )\ →\ \ (s\ :\ StackState)\ →\ accept₄\ pbk\ \ s\ →\ (accept₃\ ⁺)\ (⟦\ opPush\ pbk\ ⟧s\ s\ )}\<%
\\
\>[0]\AgdaComment{correct-4-to\ pbk\ ⟨\ currentTime₁\ ,\ msg₁\ ,\ .pbk\ ∷\ x₁\ ∷\ x₂\ ∷\ stack₁\ ⟩\ (conj\ refl\ and4)\ =\ conj\ refl\ and4}\<%
\\
\>[0]\<%
\\
\>[0]\<%
\\
\>[0]\AgdaComment{correct-4-from\ :\ (\ pbk\ :\ ℕ\ )\ →\ \ (s\ :\ StackState)\ →\ (accept₃\ ⁺)\ (⟦\ opPush\ pbk\ ⟧s\ s\ )\ →\ accept₄\ pbk\ \ s}\<%
\\
\>[0]\AgdaComment{correct-4-from\ pbk\ ⟨\ currentTime₁\ ,\ msg₁\ ,\ .pbk\ ∷\ x₁\ ∷\ x₂\ ∷\ stack₁\ \ \ ⟩\ (conj\ refl\ and4)\ =\ conj\ refl\ and4}\<%
\\
\>[0]\<%
\\
\>[0]\AgdaComment{-@BEGININLINE@correctfour}\<%
\\
\>[0]\AgdaComment{correct-4\ :(\ pbk\ :\ ℕ\ )\ →\ \ <\ accept₄\ pbk\ >iff\ \ ([\ opPush\ pbk\ ])\ <\ accept₃\ >}\<%
\\
\>[0]\AgdaComment{-@END}\<%
\\
\>[0]\AgdaComment{correct-4\ pbk\ .==>\ =\ correct-4-to\ pbk}\<%
\\
\>[0]\AgdaComment{correct-4\ pbk\ .<==\ =\ correct-4-from\ pbk}\<%
\\
\>[0]\<%
\\
\>[0]\AgdaComment{-\}}\<%
\\
%
\\[\AgdaEmptyExtraSkip]%
\>[0]\AgdaComment{--\ needs\ to\ be\ pbkh\ since\ accept₄\ and\ accept₅\ refer\ to\ pbkh}\<%
\\
\>[0]\AgdaFunction{correct-opHash-to}\AgdaSpace{}%
\AgdaSymbol{:}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaBound{pbkh}\AgdaSpace{}%
\AgdaSymbol{:}\AgdaSpace{}%
\AgdaDatatype{ℕ}\AgdaSpace{}%
\AgdaSymbol{)}\AgdaSpace{}%
\AgdaSymbol{→}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaBound{s}\AgdaSpace{}%
\AgdaSymbol{:}\AgdaSpace{}%
\AgdaRecord{StackState}\AgdaSymbol{)}\AgdaSpace{}%
\AgdaSymbol{→}\AgdaSpace{}%
\AgdaFunction{accept₅}\AgdaSpace{}%
\AgdaBound{pbkh}\AgdaSpace{}%
\AgdaBound{s}\AgdaSpace{}%
\AgdaSymbol{→}%
\>[71]\AgdaSymbol{((}\AgdaSpace{}%
\AgdaFunction{accept₄}\AgdaSpace{}%
\AgdaBound{pbkh}\AgdaSpace{}%
\AgdaSymbol{)}\AgdaSpace{}%
\AgdaOperator{\AgdaFunction{⁺}}\AgdaSymbol{)}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaOperator{\AgdaFunction{⟦}}\AgdaSpace{}%
\AgdaInductiveConstructor{opHash}\AgdaSpace{}%
\AgdaOperator{\AgdaFunction{⟧ₛ}}\AgdaSpace{}%
\AgdaBound{s}\AgdaSpace{}%
\AgdaSymbol{)}\<%
\\
\>[0]\AgdaFunction{correct-opHash-to}\AgdaSpace{}%
\AgdaBound{pbkh}\AgdaSpace{}%
\AgdaOperator{\AgdaInductiveConstructor{⟨}}\AgdaSpace{}%
\AgdaBound{time}\AgdaSpace{}%
\AgdaOperator{\AgdaInductiveConstructor{,}}\AgdaSpace{}%
\AgdaBound{msg₁}\AgdaSpace{}%
\AgdaOperator{\AgdaInductiveConstructor{,}}\AgdaSpace{}%
\AgdaBound{x}\AgdaSpace{}%
\AgdaOperator{\AgdaInductiveConstructor{∷}}\AgdaSpace{}%
\AgdaBound{x₁}\AgdaSpace{}%
\AgdaOperator{\AgdaInductiveConstructor{∷}}\AgdaSpace{}%
\AgdaBound{x₂}\AgdaSpace{}%
\AgdaOperator{\AgdaInductiveConstructor{∷}}\AgdaSpace{}%
\AgdaBound{stack₁}\AgdaSpace{}%
\AgdaOperator{\AgdaInductiveConstructor{⟩}}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaInductiveConstructor{conj}\AgdaSpace{}%
\AgdaInductiveConstructor{refl}\AgdaSpace{}%
\AgdaBound{checkSig}\AgdaSymbol{)}\AgdaSpace{}%
\AgdaSymbol{=}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaInductiveConstructor{conj}\AgdaSpace{}%
\AgdaInductiveConstructor{refl}\AgdaSpace{}%
\AgdaBound{checkSig}\AgdaSymbol{)}\<%
\\
%
\\[\AgdaEmptyExtraSkip]%
\>[0]\AgdaFunction{correct-opHash-from}\AgdaSpace{}%
\AgdaSymbol{:}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaSpace{}%
\AgdaBound{pbkh}\AgdaSpace{}%
\AgdaSymbol{:}\AgdaSpace{}%
\AgdaDatatype{ℕ}\AgdaSpace{}%
\AgdaSymbol{)}\AgdaSpace{}%
\AgdaSymbol{→}%
\>[38]\AgdaSymbol{(}\AgdaBound{s}\AgdaSpace{}%
\AgdaSymbol{:}\AgdaSpace{}%
\AgdaRecord{StackState}\AgdaSymbol{)}%
\>[56]\AgdaSymbol{→}\AgdaSpace{}%
\AgdaSymbol{((}\AgdaSpace{}%
\AgdaFunction{accept₄}\AgdaSpace{}%
\AgdaBound{pbkh}\AgdaSymbol{)}\AgdaSpace{}%
\AgdaOperator{\AgdaFunction{⁺}}\AgdaSymbol{)}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaOperator{\AgdaFunction{⟦}}\AgdaSpace{}%
\AgdaInductiveConstructor{opHash}\AgdaSpace{}%
\AgdaOperator{\AgdaFunction{⟧ₛ}}\AgdaSpace{}%
\AgdaBound{s}\AgdaSpace{}%
\AgdaSymbol{)}\AgdaSpace{}%
\AgdaSymbol{→}\AgdaSpace{}%
\AgdaFunction{accept₅}\AgdaSpace{}%
\AgdaBound{pbkh}%
\>[111]\AgdaBound{s}\<%
\\
\>[0]\AgdaFunction{correct-opHash-from}\AgdaSpace{}%
\AgdaDottedPattern{\AgdaSymbol{.(}}\AgdaDottedPattern{\AgdaFunction{hashFun}}\AgdaSpace{}%
\AgdaDottedPattern{\AgdaBound{x}}\AgdaDottedPattern{\AgdaSymbol{)}}\AgdaSpace{}%
\AgdaOperator{\AgdaInductiveConstructor{⟨}}\AgdaSpace{}%
\AgdaBound{time}\AgdaSpace{}%
\AgdaOperator{\AgdaInductiveConstructor{,}}\AgdaSpace{}%
\AgdaBound{msg₁}\AgdaSpace{}%
\AgdaOperator{\AgdaInductiveConstructor{,}}\AgdaSpace{}%
\AgdaBound{x}\AgdaSpace{}%
\AgdaOperator{\AgdaInductiveConstructor{∷}}\AgdaSpace{}%
\AgdaBound{x₁}\AgdaSpace{}%
\AgdaOperator{\AgdaInductiveConstructor{∷}}\AgdaSpace{}%
\AgdaBound{x₂}\AgdaSpace{}%
\AgdaOperator{\AgdaInductiveConstructor{∷}}\AgdaSpace{}%
\AgdaBound{stack₁}\AgdaSpace{}%
\AgdaOperator{\AgdaInductiveConstructor{⟩}}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaInductiveConstructor{conj}\AgdaSpace{}%
\AgdaInductiveConstructor{refl}\AgdaSpace{}%
\AgdaBound{checkSig}\AgdaSymbol{)}\AgdaSpace{}%
\AgdaSymbol{=}\AgdaSpace{}%
\AgdaInductiveConstructor{conj}\AgdaSpace{}%
\AgdaInductiveConstructor{refl}\AgdaSpace{}%
\AgdaBound{checkSig}\<%
\\
\>[0]\<%
\end{code}
} % END AgdaHide

\newcommand{\stackVerificationPtoPKHcorrectfive}{
\begin{code}[inline]%
\>[0]\AgdaFunction{correct-opHash}\AgdaSpace{}%
\AgdaSymbol{:(}\AgdaSpace{}%
\AgdaBound{pbkh}\AgdaSpace{}%
\AgdaSymbol{:}\AgdaSpace{}%
\AgdaDatatype{ℕ}\AgdaSpace{}%
\AgdaSymbol{)}\AgdaSpace{}%
\AgdaSymbol{→}%
\>[32]\AgdaOperator{\AgdaRecord{<}}\AgdaSpace{}%
\AgdaFunction{accept₅}\AgdaSpace{}%
\AgdaBound{pbkh}\AgdaSpace{}%
\AgdaOperator{\AgdaRecord{>ⁱᶠᶠ}}%
\>[53]\AgdaSymbol{(}\AgdaOperator{\AgdaFunction{[}}\AgdaSpace{}%
\AgdaInductiveConstructor{opHash}%
\>[64]\AgdaOperator{\AgdaFunction{]}}\AgdaSymbol{)}\AgdaSpace{}%
\AgdaOperator{\AgdaRecord{<}}\AgdaSpace{}%
\AgdaFunction{accept₄}\AgdaSpace{}%
\AgdaBound{pbkh}\AgdaSpace{}%
\AgdaOperator{\AgdaRecord{>}}\<%
\end{code}
} % END newcommand

\AgdaHide{
\begin{code}%
\>[0]\AgdaFunction{correct-opHash}\AgdaSpace{}%
\AgdaBound{pbkh}\AgdaSpace{}%
\AgdaSymbol{.}\AgdaField{==>}\AgdaSpace{}%
\AgdaSymbol{=}\AgdaSpace{}%
\AgdaFunction{correct-opHash-to}\AgdaSpace{}%
\AgdaBound{pbkh}\<%
\\
\>[0]\AgdaFunction{correct-opHash}\AgdaSpace{}%
\AgdaBound{pbkh}\AgdaSpace{}%
\AgdaSymbol{.}\AgdaField{<==}\AgdaSpace{}%
\AgdaSymbol{=}\AgdaSpace{}%
\AgdaFunction{correct-opHash-from}\AgdaSpace{}%
\AgdaBound{pbkh}\<%
\\
%
\\[\AgdaEmptyExtraSkip]%
%
\\[\AgdaEmptyExtraSkip]%
\>[0]\AgdaComment{\{-old}\<%
\\
\>[0]\<%
\\
\>[0]\<%
\\
\>[0]\AgdaComment{correct-5-to\ :\ (pbk\ :\ ℕ\ )\ →\ (s\ :\ StackState)\ →\ accept₅\ pbk\ s\ →\ \ ((\ accept₄\ pbk\ )\ ⁺)\ (⟦\ opHash\ ⟧s\ s\ )}\<%
\\
\>[0]\AgdaComment{correct-5-to\ pbk\ ⟨\ time\ ,\ msg₁\ ,\ x\ ∷\ x₁\ ∷\ x₂\ ∷\ stack₁\ ⟩\ (conj\ refl\ checkSig)\ =\ (conj\ refl\ checkSig)}\<%
\\
\>[0]\<%
\\
\>[0]\AgdaComment{correct-5-from\ :\ (\ pbk\ :\ ℕ\ )\ →\ \ (s\ :\ StackState)\ \ →\ ((\ accept₄\ pbk)\ ⁺)\ (⟦\ opHash\ ⟧s\ s\ )\ →\ accept₅\ pbk\ \ s}\<%
\\
\>[0]\AgdaComment{correct-5-from\ .(hashFun\ x)\ ⟨\ time\ ,\ msg₁\ ,\ x\ ∷\ x₁\ ∷\ x₂\ ∷\ stack₁\ ⟩\ (conj\ refl\ checkSig)\ =\ conj\ refl\ checkSig}\<%
\\
\>[0]\<%
\\
\>[0]\AgdaComment{-@BEGININLINE@correctfive}\<%
\\
\>[0]\AgdaComment{correct-5\ :(\ pbk\ :\ ℕ\ )\ →\ \ <\ accept₅\ pbk\ >iff\ \ ([\ opHash\ \ ])\ <\ accept₄\ pbk\ >}\<%
\\
\>[0]\AgdaComment{-@END}\<%
\\
\>[0]\AgdaComment{correct-5\ pbk\ .==>\ =\ correct-5-to\ pbk}\<%
\\
\>[0]\AgdaComment{correct-5\ pbk\ .<==\ =\ correct-5-from\ pbk}\<%
\\
\>[0]\<%
\\
\>[0]\AgdaComment{-\}}\<%
\\
\>[0]\AgdaComment{--\ needs\ to\ be\ pbkh\ since\ accept₅\ refer\ to\ pbkh}\<%
\\
\>[0]\AgdaFunction{correct-opDup-to}\AgdaSpace{}%
\AgdaSymbol{:}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaBound{pbkh}\AgdaSpace{}%
\AgdaSymbol{:}\AgdaSpace{}%
\AgdaDatatype{ℕ}\AgdaSpace{}%
\AgdaSymbol{)}\AgdaSpace{}%
\AgdaSymbol{→}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaBound{s}\AgdaSpace{}%
\AgdaSymbol{:}\AgdaSpace{}%
\AgdaRecord{StackState}\AgdaSymbol{)}\AgdaSpace{}%
\AgdaSymbol{→}\AgdaSpace{}%
\AgdaFunction{wPreCondP2PKH}\AgdaSpace{}%
\AgdaBound{pbkh}\AgdaSpace{}%
\AgdaBound{s}\AgdaSpace{}%
\AgdaSymbol{→}%
\>[76]\AgdaSymbol{((}\AgdaSpace{}%
\AgdaFunction{accept₅}\AgdaSpace{}%
\AgdaBound{pbkh}\AgdaSpace{}%
\AgdaSymbol{)}\AgdaSpace{}%
\AgdaOperator{\AgdaFunction{⁺}}\AgdaSymbol{)}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaOperator{\AgdaFunction{⟦}}\AgdaSpace{}%
\AgdaInductiveConstructor{opDup}\AgdaSpace{}%
\AgdaOperator{\AgdaFunction{⟧ₛ}}\AgdaSpace{}%
\AgdaBound{s}\AgdaSpace{}%
\AgdaSymbol{)}\<%
\\
\>[0]\AgdaFunction{correct-opDup-to}\AgdaSpace{}%
\AgdaBound{pbkh}\AgdaSpace{}%
\AgdaOperator{\AgdaInductiveConstructor{⟨}}\AgdaSpace{}%
\AgdaBound{time}\AgdaSpace{}%
\AgdaOperator{\AgdaInductiveConstructor{,}}\AgdaSpace{}%
\AgdaBound{msg₁}\AgdaSpace{}%
\AgdaOperator{\AgdaInductiveConstructor{,}}\AgdaSpace{}%
\AgdaBound{x}\AgdaSpace{}%
\AgdaOperator{\AgdaInductiveConstructor{∷}}\AgdaSpace{}%
\AgdaBound{x₁}\AgdaSpace{}%
\AgdaOperator{\AgdaInductiveConstructor{∷}}\AgdaSpace{}%
\AgdaInductiveConstructor{[]}\AgdaSpace{}%
\AgdaOperator{\AgdaInductiveConstructor{⟩}}\AgdaSpace{}%
\AgdaBound{p}\AgdaSpace{}%
\AgdaSymbol{=}\AgdaSpace{}%
\AgdaBound{p}\<%
\\
\>[0]\AgdaFunction{correct-opDup-to}\AgdaSpace{}%
\AgdaBound{pbkh}\AgdaSpace{}%
\AgdaOperator{\AgdaInductiveConstructor{⟨}}\AgdaSpace{}%
\AgdaBound{time}\AgdaSpace{}%
\AgdaOperator{\AgdaInductiveConstructor{,}}\AgdaSpace{}%
\AgdaBound{msg₁}\AgdaSpace{}%
\AgdaOperator{\AgdaInductiveConstructor{,}}\AgdaSpace{}%
\AgdaBound{x}\AgdaSpace{}%
\AgdaOperator{\AgdaInductiveConstructor{∷}}\AgdaSpace{}%
\AgdaBound{x₁}\AgdaSpace{}%
\AgdaOperator{\AgdaInductiveConstructor{∷}}\AgdaSpace{}%
\AgdaBound{x₂}\AgdaSpace{}%
\AgdaOperator{\AgdaInductiveConstructor{∷}}\AgdaSpace{}%
\AgdaBound{stack₁}\AgdaSpace{}%
\AgdaOperator{\AgdaInductiveConstructor{⟩}}\AgdaSpace{}%
\AgdaBound{p}\AgdaSpace{}%
\AgdaSymbol{=}\AgdaSpace{}%
\AgdaBound{p}\<%
\\
%
\\[\AgdaEmptyExtraSkip]%
\>[0]\AgdaFunction{correct-opDup-from}\AgdaSpace{}%
\AgdaSymbol{:}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaSpace{}%
\AgdaBound{pbkh}\AgdaSpace{}%
\AgdaSymbol{:}\AgdaSpace{}%
\AgdaDatatype{ℕ}\AgdaSpace{}%
\AgdaSymbol{)}\AgdaSpace{}%
\AgdaSymbol{→}%
\>[37]\AgdaSymbol{(}\AgdaBound{s}\AgdaSpace{}%
\AgdaSymbol{:}\AgdaSpace{}%
\AgdaRecord{StackState}\AgdaSymbol{)}%
\>[55]\AgdaSymbol{→}\AgdaSpace{}%
\AgdaSymbol{((}\AgdaSpace{}%
\AgdaFunction{accept₅}\AgdaSpace{}%
\AgdaBound{pbkh}\AgdaSymbol{)}\AgdaSpace{}%
\AgdaOperator{\AgdaFunction{⁺}}\AgdaSymbol{)}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaOperator{\AgdaFunction{⟦}}\AgdaSpace{}%
\AgdaInductiveConstructor{opDup}\AgdaSpace{}%
\AgdaOperator{\AgdaFunction{⟧ₛ}}\AgdaSpace{}%
\AgdaBound{s}\AgdaSpace{}%
\AgdaSymbol{)}\AgdaSpace{}%
\AgdaSymbol{→}\AgdaSpace{}%
\AgdaFunction{wPreCondP2PKH}\AgdaSpace{}%
\AgdaBound{pbkh}%
\>[115]\AgdaBound{s}\<%
\\
\>[0]\AgdaFunction{correct-opDup-from}\AgdaSpace{}%
\AgdaBound{pbkh}\AgdaSpace{}%
\AgdaOperator{\AgdaInductiveConstructor{⟨}}\AgdaSpace{}%
\AgdaBound{time}\AgdaSpace{}%
\AgdaOperator{\AgdaInductiveConstructor{,}}\AgdaSpace{}%
\AgdaBound{msg₁}\AgdaSpace{}%
\AgdaOperator{\AgdaInductiveConstructor{,}}\AgdaSpace{}%
\AgdaBound{x}\AgdaSpace{}%
\AgdaOperator{\AgdaInductiveConstructor{∷}}\AgdaSpace{}%
\AgdaBound{x₁}\AgdaSpace{}%
\AgdaOperator{\AgdaInductiveConstructor{∷}}\AgdaSpace{}%
\AgdaBound{stack₁}\AgdaSpace{}%
\AgdaOperator{\AgdaInductiveConstructor{⟩}}\AgdaSpace{}%
\AgdaBound{p}\AgdaSpace{}%
\AgdaSymbol{=}\AgdaSpace{}%
\AgdaBound{p}\<%
\\
\>[0]\<%
\end{code}
} % END AgdaHide

\newcommand{\stackVerificationPtoPKHcorrectsix}{
\begin{code}[inline]%
\>[0]\AgdaFunction{correct-opDup}\AgdaSpace{}%
\AgdaSymbol{:(}\AgdaSpace{}%
\AgdaBound{pbkh}\AgdaSpace{}%
\AgdaSymbol{:}\AgdaSpace{}%
\AgdaDatatype{ℕ}\AgdaSpace{}%
\AgdaSymbol{)}\AgdaSpace{}%
\AgdaSymbol{→}%
\>[31]\AgdaOperator{\AgdaRecord{<}}\AgdaSpace{}%
\AgdaFunction{wPreCondP2PKH}\AgdaSpace{}%
\AgdaBound{pbkh}\AgdaSpace{}%
\AgdaOperator{\AgdaRecord{>ⁱᶠᶠ}}%
\>[58]\AgdaSymbol{(}\AgdaOperator{\AgdaFunction{[}}\AgdaSpace{}%
\AgdaInductiveConstructor{opDup}%
\>[68]\AgdaOperator{\AgdaFunction{]}}\AgdaSymbol{)}\AgdaSpace{}%
\AgdaOperator{\AgdaRecord{<}}\AgdaSpace{}%
\AgdaFunction{accept₅}\AgdaSpace{}%
\AgdaBound{pbkh}\AgdaSpace{}%
\AgdaOperator{\AgdaRecord{>}}\<%
\end{code}
} % END newcommand

\AgdaHide{
\begin{code}%
\>[0]\AgdaFunction{correct-opDup}\AgdaSpace{}%
\AgdaBound{pbkh}\AgdaSpace{}%
\AgdaSymbol{.}\AgdaField{==>}\AgdaSpace{}%
\AgdaSymbol{=}\AgdaSpace{}%
\AgdaFunction{correct-opDup-to}\AgdaSpace{}%
\AgdaBound{pbkh}\<%
\\
\>[0]\AgdaFunction{correct-opDup}\AgdaSpace{}%
\AgdaBound{pbkh}\AgdaSpace{}%
\AgdaSymbol{.}\AgdaField{<==}\AgdaSpace{}%
\AgdaSymbol{=}\AgdaSpace{}%
\AgdaFunction{correct-opDup-from}\AgdaSpace{}%
\AgdaBound{pbkh}\<%
\\
%
\\[\AgdaEmptyExtraSkip]%
\>[0]\AgdaComment{\{-old}\<%
\\
\>[0]\AgdaComment{correct-6-to\ :\ (pbkh\ :\ ℕ\ )\ →\ (s\ :\ StackState)\ →\ wPreCondP2PKH\ pbkh\ s\ →\ \ ((\ accept₅\ pbkh\ )\ ⁺)\ (⟦\ opDup\ ⟧s\ s\ )}\<%
\\
\>[0]\AgdaComment{correct-6-to\ pbkh\ ⟨\ time\ ,\ msg₁\ ,\ x\ ∷\ x₁\ ∷\ []\ ⟩\ p\ =\ p}\<%
\\
\>[0]\AgdaComment{correct-6-to\ pbkh\ ⟨\ time\ ,\ msg₁\ ,\ x\ ∷\ x₁\ ∷\ x₂\ ∷\ stack₁\ ⟩\ p\ =\ p}\<%
\\
\>[0]\<%
\\
\>[0]\AgdaComment{correct-6-from\ :\ (\ pbkh\ :\ ℕ\ )\ →\ \ (s\ :\ StackState)\ \ →\ ((\ accept₅\ pbkh)\ ⁺)\ (⟦\ opDup\ ⟧s\ s\ )\ →\ wPreCondP2PKH\ pbkh\ \ s}\<%
\\
\>[0]\AgdaComment{correct-6-from\ pbkh\ ⟨\ time\ ,\ msg₁\ ,\ x\ ∷\ x₁\ ∷\ stack₁\ ⟩\ p\ =\ p}\<%
\\
\>[0]\<%
\\
\>[0]\AgdaComment{-@BEGININLINE@correctsix}\<%
\\
\>[0]\AgdaComment{correct-6\ :(\ pbk\ :\ ℕ\ )\ →\ \ <\ wPreCondP2PKH\ pbk\ >iff\ \ ([\ opDup\ \ ])\ <\ accept₅\ pbk\ >}\<%
\\
\>[0]\AgdaComment{-@END}\<%
\\
\>[0]\AgdaComment{correct-6\ pbk\ .==>\ =\ correct-6-to\ pbk}\<%
\\
\>[0]\AgdaComment{correct-6\ pbk\ .<==\ =\ correct-6-from\ pbk}\<%
\\
\>[0]\<%
\\
\>[0]\AgdaComment{-\}}\<%
\\
%
\\[\AgdaEmptyExtraSkip]%
\>[0]\AgdaComment{--\ P2PKH\ script\ refers\ to\ pbkh\ not\ pbk}\<%
\end{code}
} % END AgdaHide

\newcommand{\stackVerificationPtoPKHscriptppkh}{
\begin{code}%
\>[0]\AgdaFunction{scriptP2PKHᵇ}\AgdaSpace{}%
\AgdaSymbol{:}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaBound{pbkh}\AgdaSpace{}%
\AgdaSymbol{:}\AgdaSpace{}%
\AgdaDatatype{ℕ}\AgdaSymbol{)}\AgdaSpace{}%
\AgdaSymbol{→}\AgdaSpace{}%
\AgdaFunction{BitcoinScriptBasic}\<%
\\
\>[0]\AgdaFunction{scriptP2PKHᵇ}\AgdaSpace{}%
\AgdaBound{pbkh}\AgdaSpace{}%
\AgdaSymbol{=}\AgdaSpace{}%
\AgdaInductiveConstructor{opDup}\AgdaSpace{}%
\AgdaOperator{\AgdaInductiveConstructor{∷}}\AgdaSpace{}%
\AgdaInductiveConstructor{opHash}\AgdaSpace{}%
\AgdaOperator{\AgdaInductiveConstructor{∷}}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaInductiveConstructor{opPush}\AgdaSpace{}%
\AgdaBound{pbkh}\AgdaSymbol{)}\AgdaSpace{}%
\AgdaOperator{\AgdaInductiveConstructor{∷}}\AgdaSpace{}%
\AgdaInductiveConstructor{opEqual}\AgdaSpace{}%
\AgdaOperator{\AgdaInductiveConstructor{∷}}\AgdaSpace{}%
\AgdaInductiveConstructor{opVerify}\AgdaSpace{}%
\AgdaOperator{\AgdaInductiveConstructor{∷}}\AgdaSpace{}%
\AgdaOperator{\AgdaFunction{[}}\AgdaSpace{}%
\AgdaInductiveConstructor{opCheckSig}\AgdaSpace{}%
\AgdaOperator{\AgdaFunction{]}}\<%
\end{code}
} % END newcommand

\AgdaHide{
\begin{code}%
\>[0]\<%
\\
\>[0]\AgdaComment{\{-\ Reminder\ \ from\ stackPredicate.agda}\<%
\\
\>[0]\<%
\\
\>[0]\<%
\\
\>[0]\AgdaComment{--\ acceptingBasic\ means\ that\ the\ stack\ has\ at\ hight\ >=\ 1\ and\ top\ element\ >0}\<%
\\
\>[0]\AgdaComment{acceptingBasic\ :\ Time\ →\ Msg\ →\ Stack\ →\ Bool}\<%
\\
\>[0]\AgdaComment{acceptingBasic\ time\ msg₁\ []\ =\ false}\<%
\\
\>[0]\AgdaComment{acceptingBasic\ time\ msg₁\ (x\ ∷\ stack₁)\ =\ notFalse\ x}\<%
\\
\>[0]\<%
\\
\>[0]\<%
\\
\>[0]\AgdaComment{acceptStateˢ\ :\ StackPredicate}\<%
\\
\>[0]\AgdaComment{acceptStateˢ\ time\ msg₁\ s\ =\ acceptingBasic\ time\ msg₁\ s)}\<%
\\
\>[0]\<%
\\
\>[0]\<%
\\
\>[0]\AgdaComment{--\ wPreCondP2PKHˢ\ expresses:}\<%
\\
\>[0]\AgdaComment{--\ \ \ \ stack\ has\ height\ at\ least\ 2}\<%
\\
\>[0]\AgdaComment{--\ \ \ \ for\ the\ two\ top\ elements\ pbk\ and\ sig\ we\ have}\<%
\\
\>[0]\AgdaComment{--\ \ \ \ hashFun\ pbk\ ≡\ \ pbkh\ \ \ and\ \ \ isSigned\ \ m\ sig\ pbk}\<%
\\
\>[0]\AgdaComment{wPreCondP2PKHˢ\ :\ (pbkh\ :\ ℕ\ )\ →\ StackPredicate}\<%
\\
\>[0]\AgdaComment{wPreCondP2PKHˢ\ pbkh\ time\ m\ []\ =\ ⊥}\<%
\\
\>[0]\AgdaComment{wPreCondP2PKHˢ\ pbkh\ time\ m\ (x\ ∷\ [])\ =\ ⊥}\<%
\\
\>[0]\AgdaComment{wPreCondP2PKHˢ\ pbkh\ time\ m\ (\ pbK\ ∷\ sig\ ∷\ st)}\<%
\\
\>[0]\AgdaComment{\ \ \ \ =\ \ (hashFun\ pbk\ ≡\ \ pbkh\ )\ ∧\ \ True\ (\ isSigned\ \ m\ sig\ pbk\ )}\<%
\\
\>[0]\<%
\\
\>[0]\AgdaComment{-\}}\<%
\\
%
\\[\AgdaEmptyExtraSkip]%
%
\\[\AgdaEmptyExtraSkip]%
\>[0]\AgdaComment{--\ acceptState\ :\ StackStatePred}\<%
\\
\>[0]\AgdaComment{--\ acceptState\ =\ stackPred2SPred\ acceptStateˢ\ --\ accept-0Basic}\<%
\\
%
\\[\AgdaEmptyExtraSkip]%
\>[0]\AgdaComment{--\ acceptState\ =\ accept-0Basic}\<%
\\
%
\\[\AgdaEmptyExtraSkip]%
\>[0]\AgdaComment{--\ wPreCondP2PKH\ pbkh\ =\ accept-6\ pbkh}\<%
\\
%
\\[\AgdaEmptyExtraSkip]%
\>[0]\<%
\end{code}
} % END AgdaHide

\newcommand{\stackVerificationPtoPKHmainthro}{
\begin{code}%
\>[0]\AgdaFunction{theoremP2PKH}\AgdaSpace{}%
\AgdaSymbol{:}%
\>[16]\AgdaSymbol{(}\AgdaBound{pbkh}\AgdaSpace{}%
\AgdaSymbol{:}\AgdaSpace{}%
\AgdaDatatype{ℕ}\AgdaSymbol{)}\AgdaSpace{}%
\AgdaSymbol{→}\AgdaSpace{}%
\AgdaOperator{\AgdaRecord{<}}\AgdaSpace{}%
\AgdaFunction{wPreCondP2PKH}\AgdaSpace{}%
\AgdaBound{pbkh}\AgdaSpace{}%
\AgdaOperator{\AgdaRecord{>ⁱᶠᶠ}}\AgdaSpace{}%
\AgdaFunction{scriptP2PKHᵇ}\AgdaSpace{}%
\AgdaBound{pbkh}\AgdaSpace{}%
\AgdaOperator{\AgdaRecord{<}}\AgdaSpace{}%
\AgdaFunction{acceptState}\AgdaSpace{}%
\AgdaOperator{\AgdaRecord{>}}\<%
\\
\>[0]\AgdaFunction{theoremP2PKH}\AgdaSpace{}%
\AgdaBound{pbkh}%
\>[19]\AgdaSymbol{=}%
\>[829I]\AgdaFunction{wPreCondP2PKH}\AgdaSpace{}%
\AgdaBound{pbkh}\AgdaSpace{}%
\AgdaFunction{<><>⟨}\AgdaSpace{}%
\AgdaOperator{\AgdaFunction{[}}\AgdaSpace{}%
\AgdaInductiveConstructor{opDup}\AgdaSpace{}%
\AgdaOperator{\AgdaFunction{]}}%
\>[61]\AgdaFunction{⟩⟨}%
\>[65]\AgdaFunction{correct-opDup}%
\>[80]\AgdaBound{pbkh}\AgdaSpace{}%
\AgdaFunction{⟩}\<%
\\
\>[.][@{}l@{}]\<[829I]%
\>[21]\AgdaFunction{accept₅}%
\>[30]\AgdaBound{pbkh}%
\>[36]\AgdaFunction{<><>⟨}%
\>[43]\AgdaOperator{\AgdaFunction{[}}%
\>[46]\AgdaInductiveConstructor{opHash}\AgdaSpace{}%
\AgdaOperator{\AgdaFunction{]}}%
\>[61]\AgdaFunction{⟩⟨}%
\>[65]\AgdaFunction{correct-opHash}\AgdaSpace{}%
\AgdaBound{pbkh}\AgdaSpace{}%
\AgdaFunction{⟩}\<%
\\
%
\>[21]\AgdaFunction{accept₄}%
\>[30]\AgdaBound{pbkh}%
\>[36]\AgdaFunction{<><>⟨}%
\>[43]\AgdaOperator{\AgdaFunction{[}}%
\>[46]\AgdaInductiveConstructor{opPush}\AgdaSpace{}%
\AgdaBound{pbkh}\AgdaSpace{}%
\AgdaOperator{\AgdaFunction{]}}%
\>[61]\AgdaFunction{⟩⟨}%
\>[65]\AgdaFunction{correct-opPush}\AgdaSpace{}%
\AgdaBound{pbkh}\AgdaSpace{}%
\AgdaFunction{⟩}\<%
\\
%
\>[21]\AgdaFunction{accept₃}%
\>[36]\AgdaFunction{<><>⟨}%
\>[43]\AgdaOperator{\AgdaFunction{[}}%
\>[46]\AgdaInductiveConstructor{opEqual}\AgdaSpace{}%
\AgdaOperator{\AgdaFunction{]}}%
\>[61]\AgdaFunction{⟩⟨}%
\>[65]\AgdaFunction{correct-opEqual}%
\>[85]\AgdaFunction{⟩}\<%
\\
%
\>[21]\AgdaFunction{accept₂}%
\>[36]\AgdaFunction{<><>⟨}%
\>[43]\AgdaOperator{\AgdaFunction{[}}%
\>[46]\AgdaInductiveConstructor{opVerify}\AgdaSpace{}%
\AgdaOperator{\AgdaFunction{]}}%
\>[61]\AgdaFunction{⟩⟨}%
\>[65]\AgdaFunction{correct-opVerify}%
\>[85]\AgdaFunction{⟩}\<%
\\
%
\>[21]\AgdaFunction{accept₁}%
\>[36]\AgdaFunction{<><>⟨}%
\>[43]\AgdaOperator{\AgdaFunction{[}}%
\>[46]\AgdaInductiveConstructor{opCheckSig}\AgdaSpace{}%
\AgdaOperator{\AgdaFunction{]}}%
\>[61]\AgdaFunction{⟩⟨}%
\>[65]\AgdaFunction{correct-opCheckSig}%
\>[85]\AgdaFunction{⟩ᵉ}\<%
\\
%
\>[21]\AgdaFunction{acceptState}%
\>[34]\AgdaOperator{\AgdaFunction{∎p}}\<%
\end{code}
} % END newcommand

\AgdaHide{
\begin{code}%
\>[0]\<%
\\
\>[0]\AgdaComment{\{-old}\<%
\\
\>[0]\<%
\\
\>[0]\<%
\\
\>[0]\AgdaComment{-@BEGIN@mainthro}\<%
\\
\>[0]\AgdaComment{theoremP2PKH\ :\ (pbkh\ :\ ℕ)\ →\ <\ wPreCondP2PKH\ pbkh\ >iff\ scriptP2PKHᵇ\ pbkh\ <\ acceptState\ >}\<%
\\
\>[0]\AgdaComment{theoremP2PKH\ pbkh\ \ =\ wPreCondP2PKH\ pbkh\ <><>⟨\ [\ opDup\ ]\ \ \ ⟩⟨\ \ correct-6\ \ pbkh\ \ ⟩}\<%
\\
\>[0]\AgdaComment{\ \ \ \ \ \ \ \ \ \ \ \ \ \ \ \ \ \ \ \ \ accept₅\ \ pbkh\ \ <><>⟨\ \ [\ \ opHash\ ]\ \ \ \ \ \ \ ⟩⟨\ \ correct-5\ \ pbkh\ \ ⟩}\<%
\\
\>[0]\AgdaComment{\ \ \ \ \ \ \ \ \ \ \ \ \ \ \ \ \ \ \ \ \ accept₄\ \ pbkh\ \ <><>⟨\ \ [\ \ opPush\ pbkh\ ]\ \ ⟩⟨\ \ correct-4\ \ pbkh\ \ ⟩}\<%
\\
\>[0]\AgdaComment{\ \ \ \ \ \ \ \ \ \ \ \ \ \ \ \ \ \ \ \ \ accept₃\ \ \ \ \ \ \ \ <><>⟨\ \ [\ \ opEqual\ ]\ \ \ \ \ \ ⟩⟨\ \ correct-3\ \ ⟩}\<%
\\
\>[0]\AgdaComment{\ \ \ \ \ \ \ \ \ \ \ \ \ \ \ \ \ \ \ \ \ accept₂\ \ \ \ \ \ \ \ <><>⟨\ \ [\ \ opVerify\ ]\ \ \ \ \ ⟩⟨\ \ correct-2\ \ ⟩}\<%
\\
\>[0]\AgdaComment{\ \ \ \ \ \ \ \ \ \ \ \ \ \ \ \ \ \ \ \ \ accept₁\ \ \ \ \ \ \ \ <><>⟨\ \ [\ \ opCheckSig\ ]\ \ \ ⟩⟨\ \ correct-1\ \ ⟩e\ \ acceptState\ \ ∎p}\<%
\\
\>[0]\AgdaComment{-@END}\<%
\\
\>[0]\AgdaComment{-\}}\<%
\\
%
\\[\AgdaEmptyExtraSkip]%
%
\\[\AgdaEmptyExtraSkip]%
\>[0]\AgdaComment{\{-\ We\ have\ natural\ accepting\ condition\ expressing\ that\ the\ stack\ has\ height\ >=\ 1\ and\ top\ element\ >\ 0}\<%
\\
\>[0]\AgdaComment{\ \ \ We\ have\ a\ natural\ weakest\ precondition\ expressing\ \ blablabla}\<%
\\
\>[0]\AgdaComment{\ \ \ and\ a\ proof\ that\ it\ is\ the\ weakest\ precondtion\ for\ the\ scriptP2PKH\ w.r.t.\ the\ acceptState}\<%
\\
\>[0]\<%
\\
\>[0]\AgdaComment{\ \ \ NOTE:\ \ here\ we\ used\ single\ instructions.\ However\ opPush\ pbkh\ is\ already\ a\ composed\ instruction}\<%
\\
\>[0]\AgdaComment{\ \ \ \ \ \ \ \ \ \ and\ we\ could\ use\ whole\ program\ pieces\ instead\ of\ single\ instructions.}\<%
\\
\>[0]\<%
\\
\>[0]\AgdaComment{\ \ \ \ \ \ \ \ \ \ The\ complication\ is\ due\ to\ the\ fact\ that\ instructions\ can\ lead\ to\ failure,\ and\ therefore}\<%
\\
\>[0]\AgdaComment{\ \ \ \ \ \ \ \ \ \ \ \ \ the\ operational\ semantics\ of\ the\ resulting\ programs\ become\ quite\ long\ and\ complicated}\<%
\\
\>[0]\AgdaComment{\ \ \ \ \ \ \ \ \ \ \ \ \ because\ if\ we\ have\ \ \ instructions\ p1\ p2\ p3\ \ in\ Agda\ syntax\ we\ get}\<%
\\
\>[0]\AgdaComment{\ \ \ \ \ \ \ \ \ \ \ \ \ [[\ p1\ ::\ p2\ ::\ p3\ ::[]\ ]]s\ =}\<%
\\
\>[0]\AgdaComment{\ \ \ \ \ \ \ \ \ \ \ \ \ \ \ \ case\ [[\ p1\ ]]s\ \ of}\<%
\\
\>[0]\AgdaComment{\ \ \ \ \ \ \ \ \ \ \ \ \ \ \ \ \ \ \ nothing\ ->\ nothing}\<%
\\
\>[0]\AgdaComment{\ \ \ \ \ \ \ \ \ \ \ \ \ \ \ \ \ \ \ just\ s1\ ->\ case\ [[\ p2\ ]]\ s1\ of}\<%
\\
\>[0]\AgdaComment{\ \ \ \ \ \ \ \ \ \ \ \ \ \ \ \ \ \ \ \ \ \ \ \ \ \ \ \ \ \ \ \ nothing\ ->\ nothing}\<%
\\
\>[0]\AgdaComment{\ \ \ \ \ \ \ \ \ \ \ \ \ \ \ \ \ \ \ \ \ \ \ \ \ \ \ \ \ \ \ \ just\ s2\ ->\ [[\ p3\ ]]\ s2}\<%
\\
\>[0]\AgdaComment{\ \ \ \ \ \ \ \ \ \ \ \ So\ one\ gets\ a\ very\ involved\ case\ distinction\ which\ quickly\ becomes\ difficult\ to\ view.}\<%
\\
\>[0]\AgdaComment{\ \ \ \ \ \ \ \ \ \ \ \ By\ having\ intermediate\ conditions\ we\ make\ this\ manageable.}\<%
\\
\>[0]\<%
\\
\>[0]\<%
\\
\>[0]\<%
\\
\>[0]\AgdaComment{Not\ for\ paper:}\<%
\\
\>[0]\AgdaComment{Current\ agda\ we\ have}\<%
\\
\>[0]\<%
\\
\>[0]\AgdaComment{f\ \ zero\ \ \ =\ ??}\<%
\\
\>[0]\AgdaComment{f\ (suc\ y)\ =\ ??}\<%
\\
\>[0]\<%
\\
\>[0]\AgdaComment{in\ Agda1\ we\ had}\<%
\\
\>[0]\AgdaComment{f\ x\ =\ \ case\ x\ of}\<%
\\
\>[0]\AgdaComment{\ \ \ \ \ \ \ \ \ \ \ \ zero\ ->\ ??}\<%
\\
\>[0]\AgdaComment{\ \ \ \ \ \ \ \ \ \ \ \ suc\ y\ ->\ ??}\<%
\\
\>[0]\<%
\\
\>[0]\AgdaComment{-\}}\<%
\end{code}
} % END AgdaHide


==> latex-before-sed/verificationStackScripts/stackVerificationP2PKHUsingEqualityOfPrograms.tex <==
%% This file has been generated automatically by mkLagda.awk
%% DO NOT EDIT! ALL YOUR CHANGES WILL BE LOST!

\AgdaHide{
\begin{code}%
\>[0]\AgdaComment{--\ \textbackslash{}stackVerificationPtoPKHUsingEqualityOfPrograms}\<%
\\
\>[0]\AgdaKeyword{open}\AgdaSpace{}%
\AgdaKeyword{import}\AgdaSpace{}%
\AgdaModule{basicBitcoinDataType}\<%
\\
%
\\[\AgdaEmptyExtraSkip]%
\>[0]\AgdaKeyword{module}\AgdaSpace{}%
\AgdaModule{verificationStackScripts.stackVerificationP2PKHUsingEqualityOfPrograms}\AgdaSymbol{(}\AgdaBound{param}\AgdaSpace{}%
\AgdaSymbol{:}\AgdaSpace{}%
\AgdaRecord{GlobalParameters}\AgdaSymbol{)}%
\>[105]\AgdaKeyword{where}\<%
\\
%
\\[\AgdaEmptyExtraSkip]%
%
\\[\AgdaEmptyExtraSkip]%
%
\\[\AgdaEmptyExtraSkip]%
\>[0]\AgdaKeyword{open}\AgdaSpace{}%
\AgdaKeyword{import}\AgdaSpace{}%
\AgdaModule{Data.Nat}%
\>[22]\AgdaKeyword{hiding}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaOperator{\AgdaDatatype{\AgdaUnderscore{}≤\AgdaUnderscore{}}}\AgdaSymbol{)}\<%
\\
\>[0]\AgdaKeyword{open}\AgdaSpace{}%
\AgdaKeyword{import}\AgdaSpace{}%
\AgdaModule{Data.List}\AgdaSpace{}%
\AgdaKeyword{hiding}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaOperator{\AgdaFunction{\AgdaUnderscore{}++\AgdaUnderscore{}}}\AgdaSymbol{)}\<%
\\
\>[0]\AgdaKeyword{open}\AgdaSpace{}%
\AgdaKeyword{import}\AgdaSpace{}%
\AgdaModule{Data.Unit}%
\>[23]\AgdaKeyword{hiding}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaOperator{\AgdaRecord{\AgdaUnderscore{}≤\AgdaUnderscore{}}}\AgdaSymbol{)}\<%
\\
\>[0]\AgdaKeyword{open}\AgdaSpace{}%
\AgdaKeyword{import}\AgdaSpace{}%
\AgdaModule{Data.Empty}\<%
\\
\>[0]\AgdaKeyword{open}\AgdaSpace{}%
\AgdaKeyword{import}\AgdaSpace{}%
\AgdaModule{Data.Sum}\<%
\\
\>[0]\AgdaKeyword{open}\AgdaSpace{}%
\AgdaKeyword{import}\AgdaSpace{}%
\AgdaModule{Data.Bool}%
\>[23]\AgdaKeyword{hiding}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaOperator{\AgdaDatatype{\AgdaUnderscore{}≤\AgdaUnderscore{}}}\AgdaSpace{}%
\AgdaSymbol{;}\AgdaSpace{}%
\AgdaOperator{\AgdaFunction{if\AgdaUnderscore{}then\AgdaUnderscore{}else\AgdaUnderscore{}}}\AgdaSpace{}%
\AgdaSymbol{)}\AgdaSpace{}%
\AgdaKeyword{renaming}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaOperator{\AgdaFunction{\AgdaUnderscore{}∧\AgdaUnderscore{}}}\AgdaSpace{}%
\AgdaSymbol{to}\AgdaSpace{}%
\AgdaOperator{\AgdaFunction{\AgdaUnderscore{}∧b\AgdaUnderscore{}}}\AgdaSpace{}%
\AgdaSymbol{;}\AgdaSpace{}%
\AgdaOperator{\AgdaFunction{\AgdaUnderscore{}∨\AgdaUnderscore{}}}\AgdaSpace{}%
\AgdaSymbol{to}\AgdaSpace{}%
\AgdaOperator{\AgdaFunction{\AgdaUnderscore{}∨b\AgdaUnderscore{}}}\AgdaSpace{}%
\AgdaSymbol{;}\AgdaSpace{}%
\AgdaFunction{T}\AgdaSpace{}%
\AgdaSymbol{to}\AgdaSpace{}%
\AgdaFunction{True}\AgdaSymbol{)}\<%
\\
\>[0]\AgdaKeyword{open}\AgdaSpace{}%
\AgdaKeyword{import}\AgdaSpace{}%
\AgdaModule{Data.Product}\AgdaSpace{}%
\AgdaKeyword{renaming}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaOperator{\AgdaInductiveConstructor{\AgdaUnderscore{},\AgdaUnderscore{}}}\AgdaSpace{}%
\AgdaSymbol{to}\AgdaSpace{}%
\AgdaOperator{\AgdaInductiveConstructor{\AgdaUnderscore{},,\AgdaUnderscore{}}}\AgdaSpace{}%
\AgdaSymbol{)}\<%
\\
\>[0]\AgdaKeyword{open}\AgdaSpace{}%
\AgdaKeyword{import}\AgdaSpace{}%
\AgdaModule{Data.Nat.Base}\AgdaSpace{}%
\AgdaKeyword{hiding}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaOperator{\AgdaDatatype{\AgdaUnderscore{}≤\AgdaUnderscore{}}}\AgdaSymbol{)}\<%
\\
\>[0]\AgdaKeyword{open}\AgdaSpace{}%
\AgdaKeyword{import}\AgdaSpace{}%
\AgdaModule{Data.List.NonEmpty}\AgdaSpace{}%
\AgdaKeyword{hiding}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaField{head}\AgdaSpace{}%
\AgdaSymbol{;}\AgdaSpace{}%
\AgdaOperator{\AgdaFunction{[\AgdaUnderscore{}]}}\AgdaSpace{}%
\AgdaSymbol{)}\<%
\\
\>[0]\AgdaKeyword{open}\AgdaSpace{}%
\AgdaKeyword{import}\AgdaSpace{}%
\AgdaModule{Data.Maybe}\<%
\\
\>[0]\AgdaKeyword{open}\AgdaSpace{}%
\AgdaKeyword{import}\AgdaSpace{}%
\AgdaModule{Relation.Nullary}\<%
\\
%
\\[\AgdaEmptyExtraSkip]%
\>[0]\AgdaKeyword{import}\AgdaSpace{}%
\AgdaModule{Relation.Binary.PropositionalEquality}\AgdaSpace{}%
\AgdaSymbol{as}\AgdaSpace{}%
\AgdaModule{Eq}\<%
\\
\>[0]\AgdaKeyword{open}\AgdaSpace{}%
\AgdaModule{Eq}\AgdaSpace{}%
\AgdaKeyword{using}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaOperator{\AgdaDatatype{\AgdaUnderscore{}≡\AgdaUnderscore{}}}\AgdaSymbol{;}\AgdaSpace{}%
\AgdaInductiveConstructor{refl}\AgdaSymbol{;}\AgdaSpace{}%
\AgdaFunction{cong}\AgdaSymbol{;}\AgdaSpace{}%
\AgdaKeyword{module}\AgdaSpace{}%
\AgdaModule{≡-Reasoning}\AgdaSymbol{;}\AgdaSpace{}%
\AgdaFunction{sym}\AgdaSymbol{)}\<%
\\
\>[0]\AgdaKeyword{open}\AgdaSpace{}%
\AgdaModule{≡-Reasoning}\<%
\\
\>[0]\AgdaKeyword{open}\AgdaSpace{}%
\AgdaKeyword{import}\AgdaSpace{}%
\AgdaModule{Agda.Builtin.Equality}\<%
\\
%
\\[\AgdaEmptyExtraSkip]%
%
\\[\AgdaEmptyExtraSkip]%
\>[0]\AgdaComment{--our\ libraries}\<%
\\
\>[0]\AgdaKeyword{open}\AgdaSpace{}%
\AgdaKeyword{import}\AgdaSpace{}%
\AgdaModule{libraries.listLib}\<%
\\
\>[0]\AgdaKeyword{open}\AgdaSpace{}%
\AgdaKeyword{import}\AgdaSpace{}%
\AgdaModule{libraries.equalityLib}\<%
\\
\>[0]\AgdaKeyword{open}\AgdaSpace{}%
\AgdaKeyword{import}\AgdaSpace{}%
\AgdaModule{libraries.natLib}\<%
\\
\>[0]\AgdaKeyword{open}\AgdaSpace{}%
\AgdaKeyword{import}\AgdaSpace{}%
\AgdaModule{libraries.boolLib}\<%
\\
\>[0]\AgdaKeyword{open}\AgdaSpace{}%
\AgdaKeyword{import}\AgdaSpace{}%
\AgdaModule{libraries.emptyLib}\<%
\\
\>[0]\AgdaKeyword{open}\AgdaSpace{}%
\AgdaKeyword{import}\AgdaSpace{}%
\AgdaModule{libraries.andLib}\<%
\\
\>[0]\AgdaKeyword{open}\AgdaSpace{}%
\AgdaKeyword{import}\AgdaSpace{}%
\AgdaModule{libraries.miscLib}\<%
\\
\>[0]\AgdaKeyword{open}\AgdaSpace{}%
\AgdaKeyword{import}\AgdaSpace{}%
\AgdaModule{libraries.maybeLib}\<%
\\
%
\\[\AgdaEmptyExtraSkip]%
\>[0]\AgdaKeyword{open}\AgdaSpace{}%
\AgdaKeyword{import}\AgdaSpace{}%
\AgdaModule{stack}\<%
\\
\>[0]\AgdaKeyword{open}\AgdaSpace{}%
\AgdaKeyword{import}\AgdaSpace{}%
\AgdaModule{stackPredicate}\<%
\\
\>[0]\AgdaKeyword{open}\AgdaSpace{}%
\AgdaKeyword{import}\AgdaSpace{}%
\AgdaModule{semanticBasicOperations}\AgdaSpace{}%
\AgdaBound{param}\<%
\\
\>[0]\AgdaKeyword{open}\AgdaSpace{}%
\AgdaKeyword{import}\AgdaSpace{}%
\AgdaModule{stackSemanticsInstructions}\AgdaSpace{}%
\AgdaBound{param}\<%
\\
\>[0]\AgdaKeyword{open}\AgdaSpace{}%
\AgdaKeyword{import}\AgdaSpace{}%
\AgdaModule{hoareTripleStack}\AgdaSpace{}%
\AgdaBound{param}\<%
\\
\>[0]\AgdaKeyword{open}\AgdaSpace{}%
\AgdaKeyword{import}\AgdaSpace{}%
\AgdaModule{instruction}\<%
\\
\>[0]\AgdaKeyword{open}\AgdaSpace{}%
\AgdaKeyword{import}\AgdaSpace{}%
\AgdaModule{verificationP2PKHbasic}\AgdaSpace{}%
\AgdaBound{param}\<%
\\
\>[0]\AgdaKeyword{open}\AgdaSpace{}%
\AgdaKeyword{import}\AgdaSpace{}%
\AgdaModule{verificationStackScripts.stackState}\<%
\\
\>[0]\AgdaKeyword{open}\AgdaSpace{}%
\AgdaKeyword{import}\AgdaSpace{}%
\AgdaModule{verificationStackScripts.sPredicate}\<%
\\
\>[0]\AgdaKeyword{open}\AgdaSpace{}%
\AgdaKeyword{import}\AgdaSpace{}%
\AgdaModule{verificationStackScripts.stackHoareTriple}\AgdaSpace{}%
\AgdaBound{param}\<%
\\
\>[0]\AgdaKeyword{open}\AgdaSpace{}%
\AgdaKeyword{import}\AgdaSpace{}%
\AgdaModule{verificationStackScripts.stackVerificationLemmas}\AgdaSpace{}%
\AgdaBound{param}\<%
\\
\>[0]\AgdaKeyword{open}\AgdaSpace{}%
\AgdaKeyword{import}\AgdaSpace{}%
\AgdaModule{verificationStackScripts.stackSemanticsInstructionsBasic}\AgdaSpace{}%
\AgdaBound{param}\<%
\\
\>[0]\AgdaKeyword{open}\AgdaSpace{}%
\AgdaKeyword{import}\AgdaSpace{}%
\AgdaModule{verificationStackScripts.semanticsStackInstructions}\AgdaSpace{}%
\AgdaBound{param}\<%
\\
\>[0]\AgdaKeyword{open}\AgdaSpace{}%
\AgdaKeyword{import}\AgdaSpace{}%
\AgdaModule{verificationStackScripts.stackVerificationP2PKH}\AgdaSpace{}%
\AgdaBound{param}\<%
\\
\>[0]\AgdaKeyword{open}\AgdaSpace{}%
\AgdaKeyword{import}\AgdaSpace{}%
\AgdaModule{verificationStackScripts.stackVerificationP2PKHindexed}\AgdaSpace{}%
\AgdaBound{param}\<%
\\
\>[0]\AgdaKeyword{open}\AgdaSpace{}%
\AgdaKeyword{import}\AgdaSpace{}%
\AgdaModule{verificationStackScripts.stackVerificationP2PKHextractedProgram}\AgdaSpace{}%
\AgdaBound{param}\<%
\\
\>[0]\AgdaKeyword{open}\AgdaSpace{}%
\AgdaKeyword{import}\AgdaSpace{}%
\AgdaModule{verificationStackScripts.hoareTripleStackBasic}\AgdaSpace{}%
\AgdaBound{param}\<%
\\
\>[0]\AgdaKeyword{open}\AgdaSpace{}%
\AgdaKeyword{import}\AgdaSpace{}%
\AgdaModule{verificationStackScripts.stackVerificationLemmasPart2}\AgdaSpace{}%
\AgdaBound{param}\<%
\\
\>[0]\AgdaComment{-------------------------------------------------------}\<%
\\
\>[0]\AgdaComment{--\ The\ symbolic\ execution\ has\ been\ moved\ to}\<%
\\
\>[0]\AgdaComment{--}\<%
\\
\>[0]\AgdaComment{--\ \ \ \ \ stackVerificationP2PKHsymbolicExecution.agda}\<%
\\
\>[0]\AgdaComment{--}\<%
\\
\>[0]\AgdaComment{--\ The\ extracted\ program\ obtained\ by\ the\ symbolic\ execution\ has\ been\ moved\ to}\<%
\\
\>[0]\AgdaComment{--}\<%
\\
\>[0]\AgdaComment{--\ \ stackVerificationP2PKHextractedProgram.agda}\<%
\\
\>[0]\AgdaComment{--}\<%
\\
\>[0]\AgdaComment{------------------------------------------------------------------------------}\<%
\\
%
\\[\AgdaEmptyExtraSkip]%
%
\\[\AgdaEmptyExtraSkip]%
%
\\[\AgdaEmptyExtraSkip]%
\>[0]\AgdaComment{\{-\ \ \ Discussion\ with\ Arnold:}\<%
\\
\>[0]\AgdaComment{\ \ \ \ \ \ \ maybe\ better\ not\ to\ create\ the\ optimized\ program\ because\ we\ obtained\ this\ program\ in\ a\ systematic\ way}\<%
\\
\>[0]\AgdaComment{\ \ \ \ \ \ \ and\ can\ from\ it\ read\ off\ the\ weakest\ pre\ condition\ already}\<%
\\
\>[0]\AgdaComment{\ \ \ \ \ \ \ Discussion\ of\ further\ improvement\ (permutative\ conversions\ in\ a\ systematic\ way)\ for\ future\ work}\<%
\\
\>[0]\AgdaComment{-\}}\<%
\\
%
\\[\AgdaEmptyExtraSkip]%
%
\\[\AgdaEmptyExtraSkip]%
\>[0]\AgdaComment{--\ \textbackslash{}stackVerificationPtoPKHUsingEqualityOfProgramsptopkhNonEmptyStackAbstr}\<%
\end{code}
} % END AgdaHide

\newcommand{\stackVerificationPtoPKHUsingEqualityOfProgramsptopkhNonEmptyStackAbstr}{
\begin{code}%
\>[0]\AgdaFunction{p2PKHNonEmptyStackAbstr}\AgdaSpace{}%
\AgdaSymbol{:}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaBound{msg₁}\AgdaSpace{}%
\AgdaSymbol{:}\AgdaSpace{}%
\AgdaDatatype{Msg}\AgdaSymbol{)(}\AgdaBound{pbk}\AgdaSpace{}%
\AgdaSymbol{:}\AgdaSpace{}%
\AgdaDatatype{ℕ}\AgdaSymbol{)(}\AgdaBound{stack₁}\AgdaSpace{}%
\AgdaSymbol{:}\AgdaSpace{}%
\AgdaFunction{Stack}\AgdaSymbol{)(}\AgdaBound{cmp}\AgdaSpace{}%
\AgdaSymbol{:}\AgdaSpace{}%
\AgdaDatatype{ℕ}\AgdaSymbol{)}\AgdaSpace{}%
\AgdaSymbol{→}\AgdaSpace{}%
\AgdaDatatype{Maybe}\AgdaSpace{}%
\AgdaFunction{Stack}\<%
\\
\>[0]\AgdaFunction{p2PKHNonEmptyStackAbstr}\AgdaSpace{}%
\AgdaBound{msg₁}\AgdaSpace{}%
\AgdaBound{pbk}\AgdaSpace{}%
\AgdaBound{stack₁}\AgdaSpace{}%
\AgdaBound{cmp}\AgdaSpace{}%
\AgdaSymbol{=}%
\>[47]\AgdaFunction{executeStackVerify}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaBound{cmp}\AgdaSpace{}%
\AgdaOperator{\AgdaInductiveConstructor{∷}}%
\>[74]\AgdaBound{pbk}\AgdaSpace{}%
\AgdaOperator{\AgdaInductiveConstructor{∷}}\AgdaSpace{}%
\AgdaBound{stack₁}\AgdaSymbol{)}\AgdaSpace{}%
\AgdaOperator{\AgdaFunction{>>=}}\<%
\\
%
\>[47]\AgdaFunction{executeStackCheckSig}\AgdaSpace{}%
\AgdaBound{msg₁}\<%
\end{code}
} % END newcommand

\AgdaHide{
\begin{code}%
\>[0]\<%
\\
\>[0]\AgdaFunction{stackfunP2PKHNonEmptyStackAbstractedCorCompr0IsNothing}\AgdaSpace{}%
\AgdaSymbol{:}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaBound{msg₁}\AgdaSpace{}%
\AgdaSymbol{:}\AgdaSpace{}%
\AgdaDatatype{Msg}\AgdaSymbol{)(}\AgdaBound{pbk}\AgdaSpace{}%
\AgdaSymbol{:}\AgdaSpace{}%
\AgdaDatatype{ℕ}\AgdaSymbol{)(}\AgdaBound{stack₁}\AgdaSpace{}%
\AgdaSymbol{:}\AgdaSpace{}%
\AgdaFunction{Stack}\AgdaSymbol{)}\<%
\\
\>[0][@{}l@{\AgdaIndent{0}}]%
\>[6]\AgdaSymbol{→}%
\>[9]\AgdaFunction{p2PKHNonEmptyStackAbstr}\AgdaSpace{}%
\AgdaBound{msg₁}\AgdaSpace{}%
\AgdaBound{pbk}\AgdaSpace{}%
\AgdaBound{stack₁}\AgdaSpace{}%
\AgdaNumber{0}\AgdaSpace{}%
\AgdaOperator{\AgdaDatatype{≡}}\AgdaSpace{}%
\AgdaInductiveConstructor{nothing}\<%
\\
\>[0]\AgdaFunction{stackfunP2PKHNonEmptyStackAbstractedCorCompr0IsNothing}\AgdaSpace{}%
\AgdaBound{msg₁}\AgdaSpace{}%
\AgdaBound{pbk}\AgdaSpace{}%
\AgdaBound{stack₁}\AgdaSpace{}%
\AgdaSymbol{=}\AgdaSpace{}%
\AgdaInductiveConstructor{refl}\<%
\\
%
\\[\AgdaEmptyExtraSkip]%
%
\\[\AgdaEmptyExtraSkip]%
\>[0]\AgdaFunction{stackfunP2PKHNonEmptyStackAbstractedCorEmptysNothing}\AgdaSpace{}%
\AgdaSymbol{:}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaBound{msg₁}\AgdaSpace{}%
\AgdaSymbol{:}\AgdaSpace{}%
\AgdaDatatype{Msg}\AgdaSymbol{)(}\AgdaBound{pbk}\AgdaSpace{}%
\AgdaSymbol{:}\AgdaSpace{}%
\AgdaDatatype{ℕ}\AgdaSymbol{)(}\AgdaBound{x}\AgdaSpace{}%
\AgdaSymbol{:}\AgdaSpace{}%
\AgdaDatatype{ℕ}\AgdaSymbol{)}\<%
\\
\>[0][@{}l@{\AgdaIndent{0}}]%
\>[6]\AgdaSymbol{→}%
\>[9]\AgdaFunction{p2PKHNonEmptyStackAbstr}\AgdaSpace{}%
\AgdaBound{msg₁}\AgdaSpace{}%
\AgdaBound{pbk}\AgdaSpace{}%
\AgdaInductiveConstructor{[]}\AgdaSpace{}%
\AgdaBound{x}\AgdaSpace{}%
\AgdaOperator{\AgdaDatatype{≡}}\AgdaSpace{}%
\AgdaInductiveConstructor{nothing}\<%
\\
%
\\[\AgdaEmptyExtraSkip]%
\>[0]\AgdaFunction{stackfunP2PKHNonEmptyStackAbstractedCorEmptysNothing}\AgdaSpace{}%
\AgdaBound{msg₁}\AgdaSpace{}%
\AgdaBound{pbk₁}\AgdaSpace{}%
\AgdaInductiveConstructor{zero}\AgdaSpace{}%
\AgdaSymbol{=}\AgdaSpace{}%
\AgdaInductiveConstructor{refl}\<%
\\
\>[0]\AgdaFunction{stackfunP2PKHNonEmptyStackAbstractedCorEmptysNothing}\AgdaSpace{}%
\AgdaBound{msg₁}\AgdaSpace{}%
\AgdaBound{pbk₁}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaInductiveConstructor{suc}\AgdaSpace{}%
\AgdaBound{x}\AgdaSymbol{)}\AgdaSpace{}%
\AgdaSymbol{=}\AgdaSpace{}%
\AgdaInductiveConstructor{refl}\<%
\\
%
\\[\AgdaEmptyExtraSkip]%
\>[0]\AgdaFunction{stackfunP2PKHNonEmptyStackAbstractedCor}\AgdaSpace{}%
\AgdaSymbol{:}%
\>[43]\AgdaSymbol{(}\AgdaBound{pubKeyHash}\AgdaSpace{}%
\AgdaSymbol{:}\AgdaSpace{}%
\AgdaDatatype{ℕ}\AgdaSymbol{)(}\AgdaBound{time₁}\AgdaSpace{}%
\AgdaSymbol{:}\AgdaSpace{}%
\AgdaFunction{Time}\AgdaSymbol{)(}\AgdaBound{msg₁}\AgdaSpace{}%
\AgdaSymbol{:}\AgdaSpace{}%
\AgdaDatatype{Msg}\AgdaSymbol{)(}\AgdaBound{pbk}\AgdaSpace{}%
\AgdaSymbol{:}\AgdaSpace{}%
\AgdaDatatype{ℕ}\AgdaSymbol{)(}\AgdaBound{stack₁}\AgdaSpace{}%
\AgdaSymbol{:}\AgdaSpace{}%
\AgdaFunction{Stack}\AgdaSymbol{)}\<%
\\
\>[0][@{}l@{\AgdaIndent{0}}]%
\>[16]\AgdaSymbol{→}%
\>[217I]\AgdaOperator{\AgdaFunction{⟦}}\AgdaSpace{}%
\AgdaFunction{scriptP2PKHᵇ}\AgdaSpace{}%
\AgdaBound{pubKeyHash}\AgdaSpace{}%
\AgdaOperator{\AgdaFunction{⟧ˢ}}\AgdaSpace{}%
\AgdaBound{time₁}\AgdaSpace{}%
\AgdaBound{msg₁}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaBound{pbk}\AgdaSpace{}%
\AgdaOperator{\AgdaInductiveConstructor{∷}}\AgdaSpace{}%
\AgdaBound{stack₁}\AgdaSymbol{)}\<%
\\
\>[217I][@{}l@{\AgdaIndent{0}}]%
\>[19]\AgdaOperator{\AgdaDatatype{≡}}%
\>[226I]\AgdaFunction{p2PKHNonEmptyStackAbstr}%
\>[46]\AgdaBound{msg₁}\AgdaSpace{}%
\AgdaBound{pbk}\AgdaSpace{}%
\AgdaBound{stack₁}\<%
\\
\>[226I][@{}l@{\AgdaIndent{0}}]%
\>[27]\AgdaSymbol{(}\AgdaFunction{compareNaturals}\AgdaSpace{}%
\AgdaBound{pubKeyHash}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaFunction{hashFun}\AgdaSpace{}%
\AgdaBound{pbk}\AgdaSymbol{))}\<%
\\
\>[0]\AgdaFunction{stackfunP2PKHNonEmptyStackAbstractedCor}\AgdaSpace{}%
\AgdaBound{pubKeyHash}\AgdaSpace{}%
\AgdaBound{time₁}\AgdaSpace{}%
\AgdaBound{msg₁}\AgdaSpace{}%
\AgdaBound{pbk}\AgdaSpace{}%
\AgdaBound{stack₁}\AgdaSpace{}%
\AgdaSymbol{=}\AgdaSpace{}%
\AgdaInductiveConstructor{refl}\<%
\\
%
\\[\AgdaEmptyExtraSkip]%
%
\\[\AgdaEmptyExtraSkip]%
\>[0]\AgdaFunction{p2pkhFunctionDecodedAux1Cor}\AgdaSpace{}%
\AgdaSymbol{:}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaBound{pbk}\AgdaSpace{}%
\AgdaSymbol{:}\AgdaSpace{}%
\AgdaDatatype{ℕ}\AgdaSymbol{)(}\AgdaBound{msg₁}\AgdaSpace{}%
\AgdaSymbol{:}\AgdaSpace{}%
\AgdaDatatype{Msg}\AgdaSymbol{)(}\AgdaBound{stack₁}\AgdaSpace{}%
\AgdaSymbol{:}\AgdaSpace{}%
\AgdaFunction{Stack}\AgdaSymbol{)(}\AgdaBound{cpRes}\AgdaSpace{}%
\AgdaSymbol{:}\AgdaSpace{}%
\AgdaDatatype{ℕ}\AgdaSymbol{)}\<%
\\
\>[0][@{}l@{\AgdaIndent{0}}]%
\>[1]\AgdaSymbol{→}\AgdaSpace{}%
\AgdaFunction{p2PKHNonEmptyStackAbstr}\AgdaSpace{}%
\AgdaBound{msg₁}\AgdaSpace{}%
\AgdaBound{pbk}\AgdaSpace{}%
\AgdaBound{stack₁}\AgdaSpace{}%
\AgdaBound{cpRes}\AgdaSpace{}%
\AgdaOperator{\AgdaDatatype{≡}}\AgdaSpace{}%
\AgdaFunction{p2pkhFunctionDecodedAux1}\AgdaSpace{}%
\AgdaBound{pbk}\AgdaSpace{}%
\AgdaBound{msg₁}\AgdaSpace{}%
\AgdaBound{stack₁}\AgdaSpace{}%
\AgdaBound{cpRes}\<%
\\
%
\\[\AgdaEmptyExtraSkip]%
\>[0]\AgdaFunction{p2pkhFunctionDecodedAux1Cor}\AgdaSpace{}%
\AgdaBound{pbk₁}\AgdaSpace{}%
\AgdaBound{msg₁}\AgdaSpace{}%
\AgdaInductiveConstructor{[]}\AgdaSpace{}%
\AgdaBound{cpRes}\AgdaSpace{}%
\AgdaSymbol{=}\AgdaSpace{}%
\AgdaFunction{stackfunP2PKHNonEmptyStackAbstractedCorEmptysNothing}\AgdaSpace{}%
\AgdaBound{msg₁}\AgdaSpace{}%
\AgdaBound{pbk₁}\AgdaSpace{}%
\AgdaBound{cpRes}\<%
\\
\>[0]\AgdaFunction{p2pkhFunctionDecodedAux1Cor}\AgdaSpace{}%
\AgdaBound{pbk₁}\AgdaSpace{}%
\AgdaBound{msg₁}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaBound{x}\AgdaSpace{}%
\AgdaOperator{\AgdaInductiveConstructor{∷}}\AgdaSpace{}%
\AgdaBound{stack₁}\AgdaSymbol{)}\AgdaSpace{}%
\AgdaInductiveConstructor{zero}\AgdaSpace{}%
\AgdaSymbol{=}\AgdaSpace{}%
\AgdaInductiveConstructor{refl}\<%
\\
\>[0]\AgdaFunction{p2pkhFunctionDecodedAux1Cor}\AgdaSpace{}%
\AgdaBound{pbk₁}\AgdaSpace{}%
\AgdaBound{msg₁}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaBound{x}\AgdaSpace{}%
\AgdaOperator{\AgdaInductiveConstructor{∷}}\AgdaSpace{}%
\AgdaBound{stack₁}\AgdaSymbol{)}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaInductiveConstructor{suc}\AgdaSpace{}%
\AgdaBound{cpRes}\AgdaSymbol{)}\AgdaSpace{}%
\AgdaSymbol{=}\AgdaSpace{}%
\AgdaInductiveConstructor{refl}\<%
\\
%
\\[\AgdaEmptyExtraSkip]%
\>[0]\AgdaComment{--\ \textbackslash{}stackVerificationPtoPKHUsingEqualityOfProgramsptopkhFunctionDecodedcor}\<%
\end{code}
} % END AgdaHide

\newcommand{\stackVerificationPtoPKHUsingEqualityOfProgramsptopkhFunctionDecodedcor}{
\begin{code}%
\>[0]\AgdaFunction{p2pkhFunctionDecodedcor}\AgdaSpace{}%
\AgdaSymbol{:}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaBound{time₁}\AgdaSpace{}%
\AgdaSymbol{:}\AgdaSpace{}%
\AgdaDatatype{ℕ}\AgdaSymbol{)}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaBound{pbkh}\AgdaSpace{}%
\AgdaSymbol{:}\AgdaSpace{}%
\AgdaDatatype{ℕ}\AgdaSymbol{)(}\AgdaBound{msg₁}\AgdaSpace{}%
\AgdaSymbol{:}\AgdaSpace{}%
\AgdaDatatype{Msg}\AgdaSymbol{)(}\AgdaBound{stack₁}\AgdaSpace{}%
\AgdaSymbol{:}\AgdaSpace{}%
\AgdaFunction{Stack}\AgdaSymbol{)}\<%
\\
\>[0][@{}l@{\AgdaIndent{0}}]%
\>[1]\AgdaSymbol{→}\AgdaSpace{}%
\AgdaOperator{\AgdaFunction{⟦}}\AgdaSpace{}%
\AgdaFunction{scriptP2PKHᵇ}\AgdaSpace{}%
\AgdaBound{pbkh}\AgdaSpace{}%
\AgdaOperator{\AgdaFunction{⟧ˢ}}\AgdaSpace{}%
\AgdaBound{time₁}\AgdaSpace{}%
\AgdaBound{msg₁}\AgdaSpace{}%
\AgdaBound{stack₁}%
\>[45]\AgdaOperator{\AgdaDatatype{≡}}\AgdaSpace{}%
\AgdaFunction{p2pkhFunctionDecoded}\AgdaSpace{}%
\AgdaBound{pbkh}%
\>[74]\AgdaBound{msg₁}\AgdaSpace{}%
\AgdaBound{stack₁}\<%
\end{code}
} % END newcommand

\AgdaHide{
\begin{code}%
\>[0]\AgdaFunction{p2pkhFunctionDecodedcor}\AgdaSpace{}%
\AgdaBound{time₁}\AgdaSpace{}%
\AgdaBound{pbkh}\AgdaSpace{}%
\AgdaBound{msg₁}\AgdaSpace{}%
\AgdaInductiveConstructor{[]}\AgdaSpace{}%
\AgdaSymbol{=}\AgdaSpace{}%
\AgdaInductiveConstructor{refl}\<%
\\
\>[0]\AgdaFunction{p2pkhFunctionDecodedcor}\AgdaSpace{}%
\AgdaBound{time₁}\AgdaSpace{}%
\AgdaBound{pbkh}\AgdaSpace{}%
\AgdaBound{msg₁}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaBound{pbk}\AgdaSpace{}%
\AgdaOperator{\AgdaInductiveConstructor{∷}}\AgdaSpace{}%
\AgdaBound{stack₁}\AgdaSymbol{)}\AgdaSpace{}%
\AgdaSymbol{=}\<%
\\
\>[0][@{}l@{\AgdaIndent{0}}]%
\>[7]\AgdaOperator{\AgdaFunction{⟦}}%
\>[320I]\AgdaFunction{scriptP2PKHᵇ}\AgdaSpace{}%
\AgdaBound{pbkh}\AgdaSpace{}%
\AgdaOperator{\AgdaFunction{⟧ˢ}}\AgdaSpace{}%
\AgdaBound{time₁}\AgdaSpace{}%
\AgdaBound{msg₁}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaBound{pbk}\AgdaSpace{}%
\AgdaOperator{\AgdaInductiveConstructor{∷}}\AgdaSpace{}%
\AgdaBound{stack₁}\AgdaSymbol{)}\<%
\\
\>[320I][@{}l@{\AgdaIndent{0}}]%
\>[10]\AgdaFunction{≡⟨}\AgdaSpace{}%
\AgdaFunction{stackfunP2PKHNonEmptyStackAbstractedCor}\AgdaSpace{}%
\AgdaBound{pbkh}\AgdaSpace{}%
\AgdaBound{time₁}\AgdaSpace{}%
\AgdaBound{msg₁}\AgdaSpace{}%
\AgdaBound{pbk}\AgdaSpace{}%
\AgdaBound{stack₁}\AgdaSpace{}%
\AgdaFunction{⟩}\<%
\\
%
\>[7]\AgdaFunction{p2PKHNonEmptyStackAbstr}%
\>[32]\AgdaBound{msg₁}\AgdaSpace{}%
\AgdaBound{pbk}\AgdaSpace{}%
\AgdaBound{stack₁}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaFunction{compareNaturals}\AgdaSpace{}%
\AgdaBound{pbkh}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaFunction{hashFun}\AgdaSpace{}%
\AgdaBound{pbk}\AgdaSymbol{))}\<%
\\
\>[7][@{}l@{\AgdaIndent{0}}]%
\>[10]\AgdaFunction{≡⟨}\AgdaSpace{}%
\AgdaFunction{p2pkhFunctionDecodedAux1Cor}\AgdaSpace{}%
\AgdaBound{pbk}\AgdaSpace{}%
\AgdaBound{msg₁}\AgdaSpace{}%
\AgdaBound{stack₁}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaFunction{compareNaturals}\AgdaSpace{}%
\AgdaBound{pbkh}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaFunction{hashFun}\AgdaSpace{}%
\AgdaBound{pbk}\AgdaSymbol{))}\AgdaSpace{}%
\AgdaFunction{⟩}\<%
\\
%
\>[7]\AgdaFunction{p2pkhFunctionDecodedAux1}\AgdaSpace{}%
\AgdaBound{pbk}\AgdaSpace{}%
\AgdaBound{msg₁}\AgdaSpace{}%
\AgdaBound{stack₁}%
\>[51]\AgdaSymbol{(}\AgdaFunction{compareNaturals}\AgdaSpace{}%
\AgdaBound{pbkh}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaFunction{hashFun}\AgdaSpace{}%
\AgdaBound{pbk}\AgdaSymbol{))}\<%
\\
%
\>[7]\AgdaOperator{\AgdaFunction{∎}}\<%
\\
%
\\[\AgdaEmptyExtraSkip]%
\>[0]\AgdaComment{\{-\ Now\ we\ just\ verify\ the\ \ \ hoare\ triple\ for\ the\ function\ we\ have\ found\ we\ have\ decoded}\<%
\\
\>[0]\<%
\\
\>[0]\AgdaComment{-\}}\<%
\\
%
\\[\AgdaEmptyExtraSkip]%
\>[0]\AgdaFunction{lemmaPHKcoraux3}%
\>[356I]\AgdaSymbol{:}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaBound{x₁}\AgdaSpace{}%
\AgdaSymbol{:}\AgdaSpace{}%
\AgdaDatatype{ℕ}\AgdaSymbol{)(}\AgdaBound{time}\AgdaSpace{}%
\AgdaSymbol{:}\AgdaSpace{}%
\AgdaFunction{Time}\AgdaSymbol{)}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaBound{msg₁}\AgdaSpace{}%
\AgdaSymbol{:}\AgdaSpace{}%
\AgdaDatatype{Msg}\AgdaSymbol{)}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaBound{x₂}\AgdaSpace{}%
\AgdaSymbol{:}\AgdaSpace{}%
\AgdaDatatype{ℕ}\AgdaSymbol{)(}\AgdaBound{s}\AgdaSpace{}%
\AgdaSymbol{:}\AgdaSpace{}%
\AgdaFunction{Stack}\AgdaSymbol{)}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaBound{x}\AgdaSpace{}%
\AgdaSymbol{:}\AgdaSpace{}%
\AgdaDatatype{ℕ}\AgdaSymbol{)}\AgdaSpace{}%
\AgdaSymbol{→}\<%
\\
\>[356I][@{}l@{\AgdaIndent{0}}]%
\>[17]\AgdaFunction{liftPred2Maybe}\AgdaSpace{}%
\AgdaSymbol{(λ}\AgdaSpace{}%
\AgdaBound{s₁}\AgdaSpace{}%
\AgdaSymbol{→}\AgdaSpace{}%
\AgdaFunction{acceptStateˢ}\AgdaSpace{}%
\AgdaBound{time}\AgdaSpace{}%
\AgdaBound{msg₁}\AgdaSpace{}%
\AgdaBound{s₁}\AgdaSymbol{)}\<%
\\
\>[17][@{}l@{\AgdaIndent{0}}]%
\>[18]\AgdaSymbol{(}\AgdaFunction{p2pkhFunctionDecodedAux1}\AgdaSpace{}%
\AgdaBound{x₁}\AgdaSpace{}%
\AgdaBound{msg₁}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaBound{x₂}\AgdaSpace{}%
\AgdaOperator{\AgdaInductiveConstructor{∷}}\AgdaSpace{}%
\AgdaBound{s}\AgdaSymbol{)}\AgdaSpace{}%
\AgdaBound{x}\AgdaSymbol{)}\<%
\\
%
\>[18]\AgdaSymbol{→}\AgdaSpace{}%
\AgdaOperator{\AgdaFunction{¬}}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaBound{x}\AgdaSpace{}%
\AgdaOperator{\AgdaDatatype{≡}}\AgdaSpace{}%
\AgdaNumber{0}\AgdaSpace{}%
\AgdaSymbol{)}\<%
\\
\>[0]\AgdaFunction{lemmaPHKcoraux3}\AgdaSpace{}%
\AgdaBound{x₁}\AgdaSpace{}%
\AgdaBound{time}\AgdaSpace{}%
\AgdaBound{msg₁}\AgdaSpace{}%
\AgdaBound{x₂}\AgdaSpace{}%
\AgdaBound{s}\AgdaSpace{}%
\AgdaInductiveConstructor{zero}\AgdaSpace{}%
\AgdaSymbol{()}\AgdaSpace{}%
\AgdaBound{x₄}\<%
\\
\>[0]\AgdaFunction{lemmaPHKcoraux3}\AgdaSpace{}%
\AgdaBound{x₁}\AgdaSpace{}%
\AgdaBound{time}\AgdaSpace{}%
\AgdaBound{msg₁}\AgdaSpace{}%
\AgdaBound{x₂}\AgdaSpace{}%
\AgdaBound{s}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaInductiveConstructor{suc}\AgdaSpace{}%
\AgdaBound{x}\AgdaSymbol{)}\AgdaSpace{}%
\AgdaBound{x₃}\AgdaSpace{}%
\AgdaSymbol{()}\<%
\\
%
\\[\AgdaEmptyExtraSkip]%
\>[0]\AgdaFunction{lemmaCompareNat2}\AgdaSpace{}%
\AgdaSymbol{:}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaSpace{}%
\AgdaBound{x}\AgdaSpace{}%
\AgdaBound{y}\AgdaSpace{}%
\AgdaSymbol{:}\AgdaSpace{}%
\AgdaDatatype{ℕ}\AgdaSpace{}%
\AgdaSymbol{)}\AgdaSpace{}%
\AgdaSymbol{→}\AgdaSpace{}%
\AgdaOperator{\AgdaFunction{¬}}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaFunction{compareNaturals}\AgdaSpace{}%
\AgdaBound{x}\AgdaSpace{}%
\AgdaBound{y}\AgdaSpace{}%
\AgdaOperator{\AgdaDatatype{≡}}\AgdaSpace{}%
\AgdaNumber{0}\AgdaSpace{}%
\AgdaSymbol{)}\AgdaSpace{}%
\AgdaSymbol{→}\AgdaSpace{}%
\AgdaBound{x}\AgdaSpace{}%
\AgdaOperator{\AgdaDatatype{≡}}\AgdaSpace{}%
\AgdaBound{y}\<%
\\
\>[0]\AgdaFunction{lemmaCompareNat2}\AgdaSpace{}%
\AgdaInductiveConstructor{zero}\AgdaSpace{}%
\AgdaInductiveConstructor{zero}\AgdaSpace{}%
\AgdaBound{p}\AgdaSpace{}%
\AgdaSymbol{=}\AgdaSpace{}%
\AgdaInductiveConstructor{refl}\<%
\\
\>[0]\AgdaFunction{lemmaCompareNat2}\AgdaSpace{}%
\AgdaInductiveConstructor{zero}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaInductiveConstructor{suc}\AgdaSpace{}%
\AgdaBound{y}\AgdaSymbol{)}\AgdaSpace{}%
\AgdaBound{p}\AgdaSpace{}%
\AgdaSymbol{=}\AgdaSpace{}%
\AgdaFunction{efq}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaBound{p}\AgdaSpace{}%
\AgdaInductiveConstructor{refl}\AgdaSymbol{)}\<%
\\
\>[0]\AgdaFunction{lemmaCompareNat2}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaInductiveConstructor{suc}\AgdaSpace{}%
\AgdaBound{x}\AgdaSymbol{)}\AgdaSpace{}%
\AgdaInductiveConstructor{zero}\AgdaSpace{}%
\AgdaBound{p}\AgdaSpace{}%
\AgdaSymbol{=}\AgdaSpace{}%
\AgdaFunction{efq}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaBound{p}\AgdaSpace{}%
\AgdaInductiveConstructor{refl}\AgdaSymbol{)}\<%
\\
\>[0]\AgdaFunction{lemmaCompareNat2}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaInductiveConstructor{suc}\AgdaSpace{}%
\AgdaBound{x}\AgdaSymbol{)}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaInductiveConstructor{suc}\AgdaSpace{}%
\AgdaBound{y}\AgdaSymbol{)}\AgdaSpace{}%
\AgdaBound{p}\AgdaSpace{}%
\AgdaSymbol{=}\AgdaSpace{}%
\AgdaFunction{cong}\AgdaSpace{}%
\AgdaInductiveConstructor{suc}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaFunction{lemmaCompareNat2}\AgdaSpace{}%
\AgdaBound{x}\AgdaSpace{}%
\AgdaBound{y}\AgdaSpace{}%
\AgdaBound{p}\AgdaSymbol{)}\<%
\\
%
\\[\AgdaEmptyExtraSkip]%
%
\\[\AgdaEmptyExtraSkip]%
\>[0]\AgdaFunction{lemmaPHKcoraux2}%
\>[461I]\AgdaSymbol{:}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaBound{pbk}\AgdaSpace{}%
\AgdaSymbol{:}\AgdaSpace{}%
\AgdaDatatype{ℕ}\AgdaSymbol{)(}\AgdaBound{time}\AgdaSpace{}%
\AgdaSymbol{:}\AgdaSpace{}%
\AgdaFunction{Time}\AgdaSymbol{)}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaBound{msg₁}\AgdaSpace{}%
\AgdaSymbol{:}\AgdaSpace{}%
\AgdaDatatype{Msg}\AgdaSymbol{)}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaBound{sig}\AgdaSpace{}%
\AgdaSymbol{:}\AgdaSpace{}%
\AgdaDatatype{ℕ}\AgdaSymbol{)(}\AgdaBound{s}\AgdaSpace{}%
\AgdaSymbol{:}\AgdaSpace{}%
\AgdaFunction{Stack}\AgdaSymbol{)}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaBound{cpRes}\AgdaSpace{}%
\AgdaSymbol{:}\AgdaSpace{}%
\AgdaDatatype{ℕ}\AgdaSymbol{)}\AgdaSpace{}%
\AgdaSymbol{→}\<%
\\
\>[461I][@{}l@{\AgdaIndent{0}}]%
\>[17]\AgdaFunction{liftPred2Maybe}\AgdaSpace{}%
\AgdaSymbol{(λ}\AgdaSpace{}%
\AgdaBound{s₁}\AgdaSpace{}%
\AgdaSymbol{→}\AgdaSpace{}%
\AgdaFunction{acceptStateˢ}\AgdaSpace{}%
\AgdaBound{time}\AgdaSpace{}%
\AgdaBound{msg₁}\AgdaSpace{}%
\AgdaBound{s₁}\AgdaSymbol{)}\<%
\\
\>[17][@{}l@{\AgdaIndent{0}}]%
\>[18]\AgdaSymbol{(}\AgdaFunction{p2pkhFunctionDecodedAux1}\AgdaSpace{}%
\AgdaBound{pbk}\AgdaSpace{}%
\AgdaBound{msg₁}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaBound{sig}\AgdaSpace{}%
\AgdaOperator{\AgdaInductiveConstructor{∷}}\AgdaSpace{}%
\AgdaBound{s}\AgdaSymbol{)}\AgdaSpace{}%
\AgdaBound{cpRes}\AgdaSymbol{)}\<%
\\
%
\>[18]\AgdaSymbol{→}\AgdaSpace{}%
\AgdaFunction{NotFalse}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaFunction{boolToNat}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaFunction{isSigned}%
\>[51]\AgdaBound{msg₁}\AgdaSpace{}%
\AgdaBound{sig}\AgdaSpace{}%
\AgdaBound{pbk}\AgdaSymbol{))}\<%
\\
\>[0]\AgdaFunction{lemmaPHKcoraux2}\AgdaSpace{}%
\AgdaBound{pbk}\AgdaSpace{}%
\AgdaBound{time}\AgdaSpace{}%
\AgdaBound{msg₁}\AgdaSpace{}%
\AgdaBound{sig}\AgdaSpace{}%
\AgdaBound{s}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaInductiveConstructor{suc}\AgdaSpace{}%
\AgdaBound{cpRes}\AgdaSymbol{)}\AgdaSpace{}%
\AgdaBound{p}\AgdaSpace{}%
\AgdaSymbol{=}\AgdaSpace{}%
\AgdaBound{p}\<%
\\
%
\\[\AgdaEmptyExtraSkip]%
%
\\[\AgdaEmptyExtraSkip]%
\>[0]\AgdaComment{\{-\ This\ lemma\ \ is\ actually\ for\ the\ paper\ 1}\<%
\\
\>[0]\AgdaComment{\ \ \ and\ follows\ because}\<%
\\
\>[0]\AgdaComment{\ \ \ \ ⟦\ scriptP2PKHᵇ\ pbkh\ ⟧stack\ \ =\ \ (λ\ time\ msg₁\ s\ →\ p2pkhFunctionDecoded\ pbkh\ msg₁\ s)}\<%
\\
\>[0]\AgdaComment{-\}}\<%
\\
%
\\[\AgdaEmptyExtraSkip]%
\>[0]\AgdaComment{--\ \textbackslash{}stackVerificationPtoPKHUsingEqualityOfProgramslemmaPTKHcoraux}\<%
\end{code}
} % END AgdaHide

\newcommand{\stackVerificationPtoPKHUsingEqualityOfProgramslemmaPTKHcoraux}{
\begin{code}%
\>[0]\AgdaFunction{lemmaPTKHcoraux}\AgdaSpace{}%
\AgdaSymbol{:}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaBound{pbkh}\AgdaSpace{}%
\AgdaSymbol{:}\AgdaSpace{}%
\AgdaDatatype{ℕ}\AgdaSymbol{)}\AgdaSpace{}%
\AgdaSymbol{→}%
\>[32]\AgdaOperator{\AgdaRecord{<}}\AgdaSpace{}%
\AgdaFunction{weakestPreConditionP2PKHˢ}\AgdaSpace{}%
\AgdaBound{pbkh}\AgdaSpace{}%
\AgdaOperator{\AgdaRecord{>gˢ}}\<%
\\
%
\>[32]\AgdaSymbol{(λ}\AgdaSpace{}%
\AgdaBound{time}\AgdaSpace{}%
\AgdaBound{msg₁}\AgdaSpace{}%
\AgdaBound{s}\AgdaSpace{}%
\AgdaSymbol{→}\AgdaSpace{}%
\AgdaFunction{p2pkhFunctionDecoded}\AgdaSpace{}%
\AgdaBound{pbkh}\AgdaSpace{}%
\AgdaBound{msg₁}\AgdaSpace{}%
\AgdaBound{s}\AgdaSymbol{)}\<%
\\
%
\>[32]\AgdaOperator{\AgdaRecord{<}}\AgdaSpace{}%
\AgdaFunction{acceptStateˢ}\AgdaSpace{}%
\AgdaOperator{\AgdaRecord{>}}\<%
\end{code}
} % END newcommand

\AgdaHide{
\begin{code}%
\>[0]\AgdaFunction{lemmaPTKHcoraux}\AgdaSpace{}%
\AgdaDottedPattern{\AgdaSymbol{.(}}\AgdaDottedPattern{\AgdaFunction{hashFun}}\AgdaSpace{}%
\AgdaDottedPattern{\AgdaBound{pbk}}\AgdaDottedPattern{\AgdaSymbol{)}}\AgdaSpace{}%
\AgdaSymbol{.}\AgdaField{==>stg}\AgdaSpace{}%
\AgdaBound{time}\AgdaSpace{}%
\AgdaBound{msg₁}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaBound{pbk}\AgdaSpace{}%
\AgdaOperator{\AgdaInductiveConstructor{∷}}\AgdaSpace{}%
\AgdaBound{sig}\AgdaSpace{}%
\AgdaOperator{\AgdaInductiveConstructor{∷}}\AgdaSpace{}%
\AgdaBound{s}\AgdaSymbol{)}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaInductiveConstructor{conj}\AgdaSpace{}%
\AgdaInductiveConstructor{refl}\AgdaSpace{}%
\AgdaBound{and4}\AgdaSymbol{)}\<%
\\
\>[0][@{}l@{\AgdaIndent{0}}]%
\>[6]\AgdaKeyword{rewrite}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaFunction{lemmaCompareNat}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaFunction{hashFun}\AgdaSpace{}%
\AgdaBound{pbk}\AgdaSymbol{))}\<%
\\
%
\>[6]\AgdaSymbol{=}\AgdaSpace{}%
\AgdaFunction{boolToNatNotFalseLemma}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaFunction{isSigned}%
\>[42]\AgdaBound{msg₁}\AgdaSpace{}%
\AgdaBound{sig}\AgdaSpace{}%
\AgdaBound{pbk}\AgdaSymbol{)}\AgdaSpace{}%
\AgdaBound{and4}\<%
\\
\>[0]\AgdaFunction{lemmaPTKHcoraux}\AgdaSpace{}%
\AgdaBound{pbkh}\AgdaSpace{}%
\AgdaSymbol{.}\AgdaField{<==stg}\AgdaSpace{}%
\AgdaBound{time}\AgdaSpace{}%
\AgdaBound{msg₁}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaBound{pbk}\AgdaSpace{}%
\AgdaOperator{\AgdaInductiveConstructor{∷}}\AgdaSpace{}%
\AgdaBound{sig}\AgdaSpace{}%
\AgdaOperator{\AgdaInductiveConstructor{∷}}\AgdaSpace{}%
\AgdaBound{s}\AgdaSymbol{)}\AgdaSpace{}%
\AgdaBound{x}\<%
\\
\>[0][@{}l@{\AgdaIndent{0}}]%
\>[4]\AgdaSymbol{=}\AgdaSpace{}%
\AgdaInductiveConstructor{conj}%
\>[557I]\AgdaSymbol{(}\AgdaFunction{sym}%
\>[558I]\AgdaSymbol{(}\AgdaFunction{lemmaCompareNat2}\AgdaSpace{}%
\AgdaBound{pbkh}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaFunction{hashFun}\AgdaSpace{}%
\AgdaBound{pbk}\AgdaSymbol{)}\<%
\\
\>[558I][@{}l@{\AgdaIndent{0}}]%
\>[17]\AgdaSymbol{(}\AgdaFunction{lemmaPHKcoraux3}\AgdaSpace{}%
\AgdaBound{pbk}\AgdaSpace{}%
\AgdaBound{time}\AgdaSpace{}%
\AgdaBound{msg₁}\AgdaSpace{}%
\AgdaBound{sig}\AgdaSpace{}%
\AgdaBound{s}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaFunction{compareNaturals}\AgdaSpace{}%
\AgdaBound{pbkh}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaFunction{hashFun}\AgdaSpace{}%
\AgdaBound{pbk}\AgdaSymbol{))}\AgdaSpace{}%
\AgdaBound{x}\AgdaSymbol{)))}\<%
\\
\>[.][@{}l@{}]\<[557I]%
\>[11]\AgdaSymbol{(}\AgdaFunction{boolToNatNotFalseLemma2}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaFunction{isSigned}%
\>[47]\AgdaBound{msg₁}\AgdaSpace{}%
\AgdaBound{sig}\AgdaSpace{}%
\AgdaBound{pbk}\AgdaSymbol{)}\<%
\\
\>[11][@{}l@{\AgdaIndent{0}}]%
\>[13]\AgdaSymbol{(}\AgdaFunction{lemmaPHKcoraux2}\AgdaSpace{}%
\AgdaBound{pbk}\AgdaSpace{}%
\AgdaBound{time}\AgdaSpace{}%
\AgdaBound{msg₁}\AgdaSpace{}%
\AgdaBound{sig}\AgdaSpace{}%
\AgdaBound{s}\AgdaSpace{}%
\AgdaSymbol{((}\AgdaFunction{compareNaturals}\AgdaSpace{}%
\AgdaBound{pbkh}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaFunction{hashFun}\AgdaSpace{}%
\AgdaBound{pbk}\AgdaSymbol{)))}\AgdaSpace{}%
\AgdaBound{x}\AgdaSymbol{))}\<%
\\
%
\\[\AgdaEmptyExtraSkip]%
%
\\[\AgdaEmptyExtraSkip]%
\>[0]\AgdaFunction{LemmaPTPKHcor}\AgdaSpace{}%
\AgdaSymbol{:}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaBound{pubKeyHash}\AgdaSpace{}%
\AgdaSymbol{:}\AgdaSpace{}%
\AgdaDatatype{ℕ}\AgdaSymbol{)}\<%
\\
\>[0][@{}l@{\AgdaIndent{0}}]%
\>[2]\AgdaSymbol{→}%
\>[6]\AgdaOperator{\AgdaFunction{<}}%
\>[9]\AgdaFunction{weakestPreConditionP2PKHˢ}\AgdaSpace{}%
\AgdaBound{pubKeyHash}\AgdaSpace{}%
\AgdaOperator{\AgdaFunction{>stackb}}\<%
\\
\>[6][@{}l@{\AgdaIndent{0}}]%
\>[8]\AgdaFunction{scriptP2PKHᵇ}\AgdaSpace{}%
\AgdaBound{pubKeyHash}\<%
\\
%
\>[6]\AgdaOperator{\AgdaFunction{<}}\AgdaSpace{}%
\AgdaFunction{acceptStateˢ}%
\>[23]\AgdaOperator{\AgdaFunction{>}}\<%
\\
\>[0]\AgdaFunction{LemmaPTPKHcor}\AgdaSpace{}%
\AgdaBound{pbkh}\<%
\\
\>[0][@{}l@{\AgdaIndent{0}}]%
\>[4]\AgdaSymbol{=}%
\>[594I]\AgdaFunction{lemmaTransferHoareTripleStack}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaFunction{weakestPreConditionP2PKHˢ}\AgdaSpace{}%
\AgdaBound{pbkh}\AgdaSymbol{)}\AgdaSpace{}%
\AgdaFunction{acceptStateˢ}\<%
\\
\>[594I][@{}l@{\AgdaIndent{0}}]%
\>[8]\AgdaSymbol{(λ}\AgdaSpace{}%
\AgdaBound{time}\AgdaSpace{}%
\AgdaBound{msg}\AgdaSpace{}%
\AgdaBound{s}\AgdaSpace{}%
\AgdaSymbol{→}\AgdaSpace{}%
\AgdaFunction{p2pkhFunctionDecoded}\AgdaSpace{}%
\AgdaBound{pbkh}\AgdaSpace{}%
\AgdaBound{msg}\AgdaSpace{}%
\AgdaBound{s}\AgdaSpace{}%
\AgdaSymbol{)}\<%
\\
%
\>[8]\AgdaOperator{\AgdaFunction{⟦}}\AgdaSpace{}%
\AgdaFunction{scriptP2PKH}\AgdaSpace{}%
\AgdaBound{pbkh}\AgdaSpace{}%
\AgdaOperator{\AgdaFunction{⟧stack}}\<%
\\
%
\>[8]\AgdaSymbol{(λ}\AgdaSpace{}%
\AgdaBound{t}\AgdaSpace{}%
\AgdaBound{m}\AgdaSpace{}%
\AgdaBound{s}\AgdaSpace{}%
\AgdaSymbol{→}\AgdaSpace{}%
\AgdaFunction{sym}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaFunction{p2pkhFunctionDecodedcor}\AgdaSpace{}%
\AgdaBound{t}\AgdaSpace{}%
\AgdaBound{pbkh}\AgdaSpace{}%
\AgdaBound{m}\AgdaSpace{}%
\AgdaBound{s}\AgdaSymbol{))}\<%
\\
%
\>[8]\AgdaSymbol{(}\AgdaFunction{lemmaPTKHcoraux}\AgdaSpace{}%
\AgdaBound{pbkh}\AgdaSymbol{)}\<%
\\
%
\\[\AgdaEmptyExtraSkip]%
%
\\[\AgdaEmptyExtraSkip]%
\>[0]\AgdaComment{--\ \textbackslash{}stackVerificationPtoPKHUsingEqualityOfProgramstheoremPTPKHcor}\<%
\end{code}
} % END AgdaHide

\newcommand{\stackVerificationPtoPKHUsingEqualityOfProgramstheoremPTPKHcor}{
\begin{code}%
\>[0]\AgdaFunction{theoPTPKHcor}\AgdaSpace{}%
\AgdaSymbol{:}%
\>[16]\AgdaSymbol{(}\AgdaBound{pbkh}\AgdaSpace{}%
\AgdaSymbol{:}\AgdaSpace{}%
\AgdaDatatype{ℕ}\AgdaSymbol{)}\AgdaSpace{}%
\AgdaSymbol{→}\AgdaSpace{}%
\AgdaOperator{\AgdaRecord{<}}\AgdaSpace{}%
\AgdaFunction{wPreCondP2PKH}\AgdaSpace{}%
\AgdaBound{pbkh}\AgdaSpace{}%
\AgdaOperator{\AgdaRecord{>ⁱᶠᶠ}}\AgdaSpace{}%
\AgdaFunction{scriptP2PKHᵇ}\AgdaSpace{}%
\AgdaBound{pbkh}\AgdaSpace{}%
\AgdaOperator{\AgdaRecord{<}}\AgdaSpace{}%
\AgdaFunction{acceptState}\AgdaSpace{}%
\AgdaOperator{\AgdaRecord{>}}\<%
\end{code}
} % END newcommand

\AgdaHide{
\begin{code}%
\>[0]\AgdaFunction{theoPTPKHcor}\AgdaSpace{}%
\AgdaBound{pbkh}\AgdaSpace{}%
\AgdaSymbol{=}\<%
\\
\>[0][@{}l@{\AgdaIndent{0}}]%
\>[3]\AgdaFunction{hoareTripleStack2HoareTriple}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaFunction{scriptP2PKHᵇ}\AgdaSpace{}%
\AgdaBound{pbkh}\AgdaSymbol{)}\<%
\\
\>[3][@{}l@{\AgdaIndent{0}}]%
\>[6]\AgdaSymbol{(}\AgdaFunction{wPreCondP2PKHˢ}\AgdaSpace{}%
\AgdaBound{pbkh}\AgdaSymbol{)}\AgdaSpace{}%
\AgdaFunction{acceptStateˢ}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaFunction{LemmaPTPKHcor}\AgdaSpace{}%
\AgdaBound{pbkh}\AgdaSymbol{)}\<%
\\
%
\\[\AgdaEmptyExtraSkip]%
%
\\[\AgdaEmptyExtraSkip]%
%
\\[\AgdaEmptyExtraSkip]%
%
\\[\AgdaEmptyExtraSkip]%
%
\\[\AgdaEmptyExtraSkip]%
%
\\[\AgdaEmptyExtraSkip]%
%
\\[\AgdaEmptyExtraSkip]%
\>[0]\AgdaComment{--\ Some\ test\ cases\ used\ in\ the\ development}\<%
\\
\>[0]\AgdaComment{--\ shows\ how\ to\ check\ for\ each\ step\ \ what\ the\ functions\ are\ and\ how\ they\ compute}\<%
\\
%
\\[\AgdaEmptyExtraSkip]%
\>[0]\AgdaComment{-------------------------------------------\ Tests\ ------------------------------------------------------------}\<%
\\
%
\\[\AgdaEmptyExtraSkip]%
%
\\[\AgdaEmptyExtraSkip]%
%
\\[\AgdaEmptyExtraSkip]%
%
\\[\AgdaEmptyExtraSkip]%
%
\\[\AgdaEmptyExtraSkip]%
%
\\[\AgdaEmptyExtraSkip]%
\>[0]\AgdaComment{\{-}\<%
\\
\>[0]\AgdaComment{\ \ stackfunP2PKHemptyNotCorrectPbkIsNothing\ :\ (pubKeyHash\ :\ ℕ)(time₁\ :\ Time)(msg₁\ :\ Msg)(stack₁\ :\ State1)}\<%
\\
\>[0]\AgdaComment{\ \ \ \ \ \ \ \ →\ (\ neg\ (pubKeyHash\ ≡\ hashFun\ pbk)\ \ )}\<%
\\
\>[0]\AgdaComment{\ \ \ \ \ \ \ \ →\ ⟦\ scriptP2PKHᵇ\ pubKeyHash\ ⟧ˢ\ time₁\ msg₁\ (pbk\ ∷\ [])\ ≡\ nothing}\<%
\\
\>[0]\AgdaComment{\ \ stackfunP2PKHemptyNotCorrectPbkIsNothing\ pubKeyHash\ time₁\ msg₁\ stack₁\ =\ \{!!\}}\<%
\\
\>[0]\<%
\\
\>[0]\AgdaComment{-\}}\<%
\end{code}
} % END AgdaHide


==> latex-before-sed/verificationStackScripts/stackVerificationP2PKHextractedProgram.tex <==
%% This file has been generated automatically by mkLagda.awk
%% DO NOT EDIT! ALL YOUR CHANGES WILL BE LOST!

\AgdaHide{
\begin{code}%
\>[0]\AgdaKeyword{open}\AgdaSpace{}%
\AgdaKeyword{import}\AgdaSpace{}%
\AgdaModule{basicBitcoinDataType}\<%
\\
%
\\[\AgdaEmptyExtraSkip]%
\>[0]\AgdaKeyword{module}\AgdaSpace{}%
\AgdaModule{verificationStackScripts.stackVerificationP2PKHextractedProgram}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaBound{param}\AgdaSpace{}%
\AgdaSymbol{:}\AgdaSpace{}%
\AgdaRecord{GlobalParameters}\AgdaSymbol{)}%
\>[99]\AgdaKeyword{where}\<%
\\
%
\\[\AgdaEmptyExtraSkip]%
%
\\[\AgdaEmptyExtraSkip]%
%
\\[\AgdaEmptyExtraSkip]%
\>[0]\AgdaKeyword{open}\AgdaSpace{}%
\AgdaKeyword{import}\AgdaSpace{}%
\AgdaModule{Data.Nat}%
\>[22]\AgdaKeyword{hiding}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaOperator{\AgdaDatatype{\AgdaUnderscore{}≤\AgdaUnderscore{}}}\AgdaSymbol{)}\<%
\\
\>[0]\AgdaKeyword{open}\AgdaSpace{}%
\AgdaKeyword{import}\AgdaSpace{}%
\AgdaModule{Data.List}\AgdaSpace{}%
\AgdaKeyword{hiding}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaOperator{\AgdaFunction{\AgdaUnderscore{}++\AgdaUnderscore{}}}\AgdaSymbol{)}\<%
\\
\>[0]\AgdaKeyword{open}\AgdaSpace{}%
\AgdaKeyword{import}\AgdaSpace{}%
\AgdaModule{Data.Unit}%
\>[23]\AgdaKeyword{hiding}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaOperator{\AgdaRecord{\AgdaUnderscore{}≤\AgdaUnderscore{}}}\AgdaSymbol{)}\<%
\\
\>[0]\AgdaKeyword{open}\AgdaSpace{}%
\AgdaKeyword{import}\AgdaSpace{}%
\AgdaModule{Data.Empty}\<%
\\
\>[0]\AgdaKeyword{open}\AgdaSpace{}%
\AgdaKeyword{import}\AgdaSpace{}%
\AgdaModule{Data.Sum}\<%
\\
\>[0]\AgdaKeyword{open}\AgdaSpace{}%
\AgdaKeyword{import}\AgdaSpace{}%
\AgdaModule{Data.Bool}%
\>[23]\AgdaKeyword{hiding}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaOperator{\AgdaDatatype{\AgdaUnderscore{}≤\AgdaUnderscore{}}}\AgdaSpace{}%
\AgdaSymbol{;}\AgdaSpace{}%
\AgdaOperator{\AgdaFunction{if\AgdaUnderscore{}then\AgdaUnderscore{}else\AgdaUnderscore{}}}\AgdaSpace{}%
\AgdaSymbol{)}\AgdaSpace{}%
\AgdaKeyword{renaming}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaOperator{\AgdaFunction{\AgdaUnderscore{}∧\AgdaUnderscore{}}}\AgdaSpace{}%
\AgdaSymbol{to}\AgdaSpace{}%
\AgdaOperator{\AgdaFunction{\AgdaUnderscore{}∧b\AgdaUnderscore{}}}\AgdaSpace{}%
\AgdaSymbol{;}\AgdaSpace{}%
\AgdaOperator{\AgdaFunction{\AgdaUnderscore{}∨\AgdaUnderscore{}}}\AgdaSpace{}%
\AgdaSymbol{to}\AgdaSpace{}%
\AgdaOperator{\AgdaFunction{\AgdaUnderscore{}∨b\AgdaUnderscore{}}}\AgdaSpace{}%
\AgdaSymbol{;}\AgdaSpace{}%
\AgdaFunction{T}\AgdaSpace{}%
\AgdaSymbol{to}\AgdaSpace{}%
\AgdaFunction{True}\AgdaSymbol{)}\<%
\\
\>[0]\AgdaKeyword{open}\AgdaSpace{}%
\AgdaKeyword{import}\AgdaSpace{}%
\AgdaModule{Data.Product}\AgdaSpace{}%
\AgdaKeyword{renaming}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaOperator{\AgdaInductiveConstructor{\AgdaUnderscore{},\AgdaUnderscore{}}}\AgdaSpace{}%
\AgdaSymbol{to}\AgdaSpace{}%
\AgdaOperator{\AgdaInductiveConstructor{\AgdaUnderscore{},,\AgdaUnderscore{}}}\AgdaSpace{}%
\AgdaSymbol{)}\<%
\\
\>[0]\AgdaKeyword{open}\AgdaSpace{}%
\AgdaKeyword{import}\AgdaSpace{}%
\AgdaModule{Data.Nat.Base}\AgdaSpace{}%
\AgdaKeyword{hiding}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaOperator{\AgdaDatatype{\AgdaUnderscore{}≤\AgdaUnderscore{}}}\AgdaSymbol{)}\<%
\\
\>[0]\AgdaKeyword{open}\AgdaSpace{}%
\AgdaKeyword{import}\AgdaSpace{}%
\AgdaModule{Data.List.NonEmpty}\AgdaSpace{}%
\AgdaKeyword{hiding}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaField{head}\AgdaSpace{}%
\AgdaSymbol{;}\AgdaSpace{}%
\AgdaOperator{\AgdaFunction{[\AgdaUnderscore{}]}}\AgdaSpace{}%
\AgdaSymbol{)}\<%
\\
\>[0]\AgdaKeyword{open}\AgdaSpace{}%
\AgdaKeyword{import}\AgdaSpace{}%
\AgdaModule{Data.Maybe}\<%
\\
\>[0]\AgdaKeyword{open}\AgdaSpace{}%
\AgdaKeyword{import}\AgdaSpace{}%
\AgdaModule{Relation.Nullary}\<%
\\
%
\\[\AgdaEmptyExtraSkip]%
\>[0]\AgdaKeyword{import}\AgdaSpace{}%
\AgdaModule{Relation.Binary.PropositionalEquality}\AgdaSpace{}%
\AgdaSymbol{as}\AgdaSpace{}%
\AgdaModule{Eq}\<%
\\
\>[0]\AgdaKeyword{open}\AgdaSpace{}%
\AgdaModule{Eq}\AgdaSpace{}%
\AgdaKeyword{using}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaOperator{\AgdaDatatype{\AgdaUnderscore{}≡\AgdaUnderscore{}}}\AgdaSymbol{;}\AgdaSpace{}%
\AgdaInductiveConstructor{refl}\AgdaSymbol{;}\AgdaSpace{}%
\AgdaFunction{cong}\AgdaSymbol{;}\AgdaSpace{}%
\AgdaKeyword{module}\AgdaSpace{}%
\AgdaModule{≡-Reasoning}\AgdaSymbol{;}\AgdaSpace{}%
\AgdaFunction{sym}\AgdaSymbol{)}\<%
\\
\>[0]\AgdaKeyword{open}\AgdaSpace{}%
\AgdaModule{≡-Reasoning}\<%
\\
\>[0]\AgdaKeyword{open}\AgdaSpace{}%
\AgdaKeyword{import}\AgdaSpace{}%
\AgdaModule{Agda.Builtin.Equality}\<%
\\
%
\\[\AgdaEmptyExtraSkip]%
%
\\[\AgdaEmptyExtraSkip]%
\>[0]\AgdaComment{--our\ libraries}\<%
\\
\>[0]\AgdaKeyword{open}\AgdaSpace{}%
\AgdaKeyword{import}\AgdaSpace{}%
\AgdaModule{libraries.listLib}\<%
\\
\>[0]\AgdaKeyword{open}\AgdaSpace{}%
\AgdaKeyword{import}\AgdaSpace{}%
\AgdaModule{libraries.equalityLib}\<%
\\
\>[0]\AgdaKeyword{open}\AgdaSpace{}%
\AgdaKeyword{import}\AgdaSpace{}%
\AgdaModule{libraries.natLib}\<%
\\
\>[0]\AgdaKeyword{open}\AgdaSpace{}%
\AgdaKeyword{import}\AgdaSpace{}%
\AgdaModule{libraries.boolLib}\<%
\\
\>[0]\AgdaKeyword{open}\AgdaSpace{}%
\AgdaKeyword{import}\AgdaSpace{}%
\AgdaModule{libraries.emptyLib}\<%
\\
\>[0]\AgdaKeyword{open}\AgdaSpace{}%
\AgdaKeyword{import}\AgdaSpace{}%
\AgdaModule{libraries.andLib}\<%
\\
\>[0]\AgdaKeyword{open}\AgdaSpace{}%
\AgdaKeyword{import}\AgdaSpace{}%
\AgdaModule{libraries.miscLib}\<%
\\
\>[0]\AgdaKeyword{open}\AgdaSpace{}%
\AgdaKeyword{import}\AgdaSpace{}%
\AgdaModule{libraries.maybeLib}\<%
\\
%
\\[\AgdaEmptyExtraSkip]%
\>[0]\AgdaKeyword{open}\AgdaSpace{}%
\AgdaKeyword{import}\AgdaSpace{}%
\AgdaModule{stack}\<%
\\
\>[0]\AgdaKeyword{open}\AgdaSpace{}%
\AgdaKeyword{import}\AgdaSpace{}%
\AgdaModule{stackPredicate}\<%
\\
\>[0]\AgdaKeyword{open}\AgdaSpace{}%
\AgdaKeyword{import}\AgdaSpace{}%
\AgdaModule{semanticBasicOperations}\AgdaSpace{}%
\AgdaBound{param}\<%
\\
\>[0]\AgdaKeyword{open}\AgdaSpace{}%
\AgdaKeyword{import}\AgdaSpace{}%
\AgdaModule{hoareTripleStack}\AgdaSpace{}%
\AgdaBound{param}\<%
\\
\>[0]\AgdaKeyword{open}\AgdaSpace{}%
\AgdaKeyword{import}\AgdaSpace{}%
\AgdaModule{instruction}\<%
\\
\>[0]\AgdaKeyword{open}\AgdaSpace{}%
\AgdaKeyword{import}\AgdaSpace{}%
\AgdaModule{stackSemanticsInstructions}\AgdaSpace{}%
\AgdaBound{param}\<%
\\
\>[0]\AgdaKeyword{open}\AgdaSpace{}%
\AgdaKeyword{import}\AgdaSpace{}%
\AgdaModule{verificationP2PKHbasic}\AgdaSpace{}%
\AgdaBound{param}\<%
\\
%
\\[\AgdaEmptyExtraSkip]%
\>[0]\AgdaKeyword{open}\AgdaSpace{}%
\AgdaKeyword{import}\AgdaSpace{}%
\AgdaModule{verificationStackScripts.stackState}\<%
\\
\>[0]\AgdaKeyword{open}\AgdaSpace{}%
\AgdaKeyword{import}\AgdaSpace{}%
\AgdaModule{verificationStackScripts.sPredicate}\<%
\\
\>[0]\AgdaKeyword{open}\AgdaSpace{}%
\AgdaKeyword{import}\AgdaSpace{}%
\AgdaModule{verificationWithIfStack.hoareTripleStackScript}\AgdaSpace{}%
\AgdaBound{param}\<%
\\
\>[0]\AgdaKeyword{open}\AgdaSpace{}%
\AgdaKeyword{import}\AgdaSpace{}%
\AgdaModule{verificationStackScripts.stackHoareTriple}\AgdaSpace{}%
\AgdaBound{param}\<%
\\
\>[0]\AgdaKeyword{open}\AgdaSpace{}%
\AgdaKeyword{import}\AgdaSpace{}%
\AgdaModule{verificationStackScripts.stackVerificationLemmas}\AgdaSpace{}%
\AgdaBound{param}\<%
\\
\>[0]\AgdaKeyword{open}\AgdaSpace{}%
\AgdaKeyword{import}\AgdaSpace{}%
\AgdaModule{verificationStackScripts.stackSemanticsInstructionsBasic}\AgdaSpace{}%
\AgdaBound{param}\<%
\\
\>[0]\AgdaKeyword{open}\AgdaSpace{}%
\AgdaKeyword{import}\AgdaSpace{}%
\AgdaModule{verificationStackScripts.semanticsStackInstructions}\AgdaSpace{}%
\AgdaBound{param}\<%
\\
\>[0]\AgdaKeyword{open}\AgdaSpace{}%
\AgdaKeyword{import}\AgdaSpace{}%
\AgdaModule{verificationStackScripts.stackVerificationP2PKH}\AgdaSpace{}%
\AgdaBound{param}\<%
\\
\>[0]\AgdaKeyword{open}\AgdaSpace{}%
\AgdaKeyword{import}\AgdaSpace{}%
\AgdaModule{verificationStackScripts.stackVerificationP2PKHindexed}\AgdaSpace{}%
\AgdaBound{param}\<%
\\
\>[0]\AgdaKeyword{open}\AgdaSpace{}%
\AgdaKeyword{import}\AgdaSpace{}%
\AgdaModule{verificationStackScripts.hoareTripleStackBasic}\AgdaSpace{}%
\AgdaBound{param}\<%
\\
\>[0]\AgdaKeyword{open}\AgdaSpace{}%
\AgdaKeyword{import}\AgdaSpace{}%
\AgdaModule{verificationStackScripts.stackVerificationLemmasPart2}\AgdaSpace{}%
\AgdaBound{param}\<%
\\
%
\\[\AgdaEmptyExtraSkip]%
%
\\[\AgdaEmptyExtraSkip]%
\>[0]\AgdaComment{\{-\ Now\ we\ have\ decoded\ the\ function\ -\}}\<%
\\
%
\\[\AgdaEmptyExtraSkip]%
\>[0]\AgdaComment{--\ p2pkhFunctionDecodedAux1\ should\ be\ equal\ to\ p2PKHNonEmptyStackAbstr\ (ignorning\ time)}\<%
\\
\>[0]\AgdaComment{--\ p2pkhFunctionDecoded\ should\ be\ equal\ to\ \ \ ⟦\ scriptP2PKHᵇ\ pubKeyHash\ ⟧ˢ\ time₁\ msg₁\ stack₁\ \ \ (where\ time\ is\ irrelevant)}\<%
\\
%
\\[\AgdaEmptyExtraSkip]%
\>[0]\AgdaKeyword{mutual}\<%
\end{code}
} % END AgdaHide

\newcommand{\stackVerificationPtoPKHextractedProgramptopkhFunctionDecoded}{
\begin{code}%
\>[0][@{}l@{\AgdaIndent{1}}]%
\>[2]\AgdaFunction{p2pkhFunctionDecoded}\AgdaSpace{}%
\AgdaSymbol{:}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaBound{pbkh}\AgdaSpace{}%
\AgdaSymbol{:}\AgdaSpace{}%
\AgdaDatatype{ℕ}\AgdaSymbol{)(}\AgdaBound{msg₁}\AgdaSpace{}%
\AgdaSymbol{:}\AgdaSpace{}%
\AgdaDatatype{Msg}\AgdaSymbol{)(}\AgdaBound{stack₁}\AgdaSpace{}%
\AgdaSymbol{:}\AgdaSpace{}%
\AgdaFunction{Stack}\AgdaSymbol{)}\AgdaSpace{}%
\AgdaSymbol{→}\AgdaSpace{}%
\AgdaDatatype{Maybe}\AgdaSpace{}%
\AgdaFunction{Stack}\<%
\\
%
\>[2]\AgdaFunction{p2pkhFunctionDecoded}%
\>[24]\AgdaBound{pbkh}%
\>[30]\AgdaBound{msg₁}%
\>[36]\AgdaInductiveConstructor{[]}%
\>[52]\AgdaSymbol{=}%
\>[55]\AgdaInductiveConstructor{nothing}\<%
\\
%
\>[2]\AgdaFunction{p2pkhFunctionDecoded}%
\>[24]\AgdaBound{pbkh}%
\>[30]\AgdaBound{msg₁}%
\>[36]\AgdaSymbol{(}\AgdaBound{pbk}\AgdaSpace{}%
\AgdaOperator{\AgdaInductiveConstructor{∷}}\AgdaSpace{}%
\AgdaBound{stack₁}\AgdaSymbol{)}%
\>[52]\AgdaSymbol{=}%
\>[55]\AgdaFunction{p2pkhFunctionDecodedAux1}\AgdaSpace{}%
\AgdaBound{pbk}\AgdaSpace{}%
\AgdaBound{msg₁}\AgdaSpace{}%
\AgdaBound{stack₁}\<%
\\
%
\>[55]\AgdaSymbol{(}\AgdaFunction{compareNaturals}\AgdaSpace{}%
\AgdaBound{pbkh}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaFunction{hashFun}\AgdaSpace{}%
\AgdaBound{pbk}\AgdaSymbol{))}\<%
\\
%
\\[\AgdaEmptyExtraSkip]%
%
\>[2]\AgdaFunction{p2pkhFunctionDecodedAux1}\AgdaSpace{}%
\AgdaSymbol{:}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaBound{pbk}\AgdaSpace{}%
\AgdaSymbol{:}\AgdaSpace{}%
\AgdaDatatype{ℕ}\AgdaSymbol{)(}\AgdaBound{msg₁}\AgdaSpace{}%
\AgdaSymbol{:}\AgdaSpace{}%
\AgdaDatatype{Msg}\AgdaSymbol{)(}\AgdaBound{stack₁}\AgdaSpace{}%
\AgdaSymbol{:}\AgdaSpace{}%
\AgdaFunction{Stack}\AgdaSymbol{)(}\AgdaBound{cpRes}\AgdaSpace{}%
\AgdaSymbol{:}\AgdaSpace{}%
\AgdaDatatype{ℕ}\AgdaSymbol{)}\AgdaSpace{}%
\AgdaSymbol{→}\AgdaSpace{}%
\AgdaDatatype{Maybe}\AgdaSpace{}%
\AgdaFunction{Stack}\<%
\\
%
\>[2]\AgdaFunction{p2pkhFunctionDecodedAux1}%
\>[28]\AgdaBound{pbk}%
\>[33]\AgdaBound{msg₁}%
\>[39]\AgdaInductiveConstructor{[]}%
\>[56]\AgdaBound{cpRes}%
\>[69]\AgdaSymbol{=}%
\>[72]\AgdaInductiveConstructor{nothing}\<%
\\
%
\>[2]\AgdaFunction{p2pkhFunctionDecodedAux1}%
\>[28]\AgdaBound{pbk}%
\>[33]\AgdaBound{msg₁}%
\>[39]\AgdaSymbol{(}\AgdaBound{sig₁}\AgdaSpace{}%
\AgdaOperator{\AgdaInductiveConstructor{∷}}\AgdaSpace{}%
\AgdaBound{stack₁}\AgdaSymbol{)}%
\>[56]\AgdaInductiveConstructor{zero}%
\>[69]\AgdaSymbol{=}%
\>[72]\AgdaInductiveConstructor{nothing}\<%
\\
%
\>[2]\AgdaFunction{p2pkhFunctionDecodedAux1}%
\>[28]\AgdaBound{pbk}%
\>[33]\AgdaBound{msg₁}%
\>[39]\AgdaSymbol{(}\AgdaBound{sig₁}\AgdaSpace{}%
\AgdaOperator{\AgdaInductiveConstructor{∷}}\AgdaSpace{}%
\AgdaBound{stack₁}\AgdaSymbol{)}%
\>[56]\AgdaSymbol{(}\AgdaInductiveConstructor{suc}\AgdaSpace{}%
\AgdaBound{cpRes}\AgdaSymbol{)}%
\>[69]\AgdaSymbol{=}\<%
\\
%
\>[28]\AgdaInductiveConstructor{just}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaFunction{boolToNat}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaFunction{isSigned}%
\>[55]\AgdaBound{msg₁}\AgdaSpace{}%
\AgdaBound{sig₁}\AgdaSpace{}%
\AgdaBound{pbk}\AgdaSymbol{)}\AgdaSpace{}%
\AgdaOperator{\AgdaInductiveConstructor{∷}}\AgdaSpace{}%
\AgdaBound{stack₁}\AgdaSymbol{)}\<%
\end{code}
} % END newcommand

\AgdaHide{
\begin{code}%
\>[0]\<%
\end{code}
} % END AgdaHide


==> latex-before-sed/verificationStackScripts/verificationMultiSigBasic.tex <==
%% This file has been generated automatically by mkLagda.awk
%% DO NOT EDIT! ALL YOUR CHANGES WILL BE LOST!

\AgdaHide{
\begin{code}%
\>[0]\AgdaComment{--\textbackslash{}verificationMultiSigBasic}\<%
\\
\>[0]\AgdaKeyword{open}\AgdaSpace{}%
\AgdaKeyword{import}\AgdaSpace{}%
\AgdaModule{basicBitcoinDataType}\<%
\\
%
\\[\AgdaEmptyExtraSkip]%
\>[0]\AgdaKeyword{module}\AgdaSpace{}%
\AgdaModule{verificationStackScripts.verificationMultiSigBasic}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaBound{param}\AgdaSpace{}%
\AgdaSymbol{:}\AgdaSpace{}%
\AgdaRecord{GlobalParameters}\AgdaSymbol{)}\AgdaSpace{}%
\AgdaKeyword{where}\<%
\\
%
\\[\AgdaEmptyExtraSkip]%
%
\\[\AgdaEmptyExtraSkip]%
\>[0]\AgdaKeyword{open}\AgdaSpace{}%
\AgdaKeyword{import}\AgdaSpace{}%
\AgdaModule{Data.List.Base}\AgdaSpace{}%
\AgdaKeyword{hiding}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaOperator{\AgdaFunction{\AgdaUnderscore{}++\AgdaUnderscore{}}}\AgdaSpace{}%
\AgdaSymbol{)}\<%
\\
\>[0]\AgdaKeyword{open}\AgdaSpace{}%
\AgdaKeyword{import}\AgdaSpace{}%
\AgdaModule{Data.Nat}%
\>[22]\AgdaKeyword{renaming}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaOperator{\AgdaDatatype{\AgdaUnderscore{}≤\AgdaUnderscore{}}}\AgdaSpace{}%
\AgdaSymbol{to}\AgdaSpace{}%
\AgdaOperator{\AgdaDatatype{\AgdaUnderscore{}≤'\AgdaUnderscore{}}}\AgdaSpace{}%
\AgdaSymbol{;}\AgdaSpace{}%
\AgdaOperator{\AgdaFunction{\AgdaUnderscore{}<\AgdaUnderscore{}}}\AgdaSpace{}%
\AgdaSymbol{to}\AgdaSpace{}%
\AgdaOperator{\AgdaFunction{\AgdaUnderscore{}<'\AgdaUnderscore{}}}\AgdaSymbol{)}\<%
\\
\>[0]\AgdaKeyword{open}\AgdaSpace{}%
\AgdaKeyword{import}\AgdaSpace{}%
\AgdaModule{Data.List}\AgdaSpace{}%
\AgdaKeyword{hiding}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaOperator{\AgdaFunction{\AgdaUnderscore{}++\AgdaUnderscore{}}}%
\>[36]\AgdaSymbol{)}\<%
\\
\>[0]\AgdaKeyword{open}\AgdaSpace{}%
\AgdaKeyword{import}\AgdaSpace{}%
\AgdaModule{Data.Sum}\<%
\\
\>[0]\AgdaKeyword{open}\AgdaSpace{}%
\AgdaKeyword{import}\AgdaSpace{}%
\AgdaModule{Data.Unit}%
\>[23]\AgdaKeyword{hiding}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaOperator{\AgdaRecord{\AgdaUnderscore{}≤\AgdaUnderscore{}}}\AgdaSymbol{)}\<%
\\
\>[0]\AgdaKeyword{open}\AgdaSpace{}%
\AgdaKeyword{import}\AgdaSpace{}%
\AgdaModule{Data.Empty}\<%
\\
\>[0]\AgdaKeyword{open}\AgdaSpace{}%
\AgdaKeyword{import}\AgdaSpace{}%
\AgdaModule{Data.Maybe}\<%
\\
\>[0]\AgdaKeyword{open}\AgdaSpace{}%
\AgdaKeyword{import}\AgdaSpace{}%
\AgdaModule{Data.Bool}%
\>[23]\AgdaKeyword{hiding}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaOperator{\AgdaDatatype{\AgdaUnderscore{}≤\AgdaUnderscore{}}}\AgdaSpace{}%
\AgdaSymbol{;}\AgdaSpace{}%
\AgdaOperator{\AgdaDatatype{\AgdaUnderscore{}<\AgdaUnderscore{}}}\AgdaSpace{}%
\AgdaSymbol{;}\AgdaSpace{}%
\AgdaOperator{\AgdaFunction{if\AgdaUnderscore{}then\AgdaUnderscore{}else\AgdaUnderscore{}}}%
\>[58]\AgdaSymbol{)}%
\>[61]\AgdaKeyword{renaming}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaOperator{\AgdaFunction{\AgdaUnderscore{}∧\AgdaUnderscore{}}}\AgdaSpace{}%
\AgdaSymbol{to}\AgdaSpace{}%
\AgdaOperator{\AgdaFunction{\AgdaUnderscore{}∧b\AgdaUnderscore{}}}\AgdaSpace{}%
\AgdaSymbol{;}\AgdaSpace{}%
\AgdaOperator{\AgdaFunction{\AgdaUnderscore{}∨\AgdaUnderscore{}}}\AgdaSpace{}%
\AgdaSymbol{to}\AgdaSpace{}%
\AgdaOperator{\AgdaFunction{\AgdaUnderscore{}∨b\AgdaUnderscore{}}}\AgdaSpace{}%
\AgdaSymbol{;}\AgdaSpace{}%
\AgdaFunction{T}\AgdaSpace{}%
\AgdaSymbol{to}\AgdaSpace{}%
\AgdaFunction{True}\AgdaSymbol{)}\<%
\\
\>[0]\AgdaKeyword{open}\AgdaSpace{}%
\AgdaKeyword{import}\AgdaSpace{}%
\AgdaModule{Data.Product}\AgdaSpace{}%
\AgdaKeyword{renaming}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaOperator{\AgdaInductiveConstructor{\AgdaUnderscore{},\AgdaUnderscore{}}}\AgdaSpace{}%
\AgdaSymbol{to}\AgdaSpace{}%
\AgdaOperator{\AgdaInductiveConstructor{\AgdaUnderscore{},,\AgdaUnderscore{}}}\AgdaSpace{}%
\AgdaSymbol{)}\<%
\\
\>[0]\AgdaKeyword{open}\AgdaSpace{}%
\AgdaKeyword{import}\AgdaSpace{}%
\AgdaModule{Data.Nat.Base}\AgdaSpace{}%
\AgdaKeyword{hiding}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaOperator{\AgdaDatatype{\AgdaUnderscore{}≤\AgdaUnderscore{}}}\AgdaSpace{}%
\AgdaSymbol{;}\AgdaSpace{}%
\AgdaOperator{\AgdaFunction{\AgdaUnderscore{}<\AgdaUnderscore{}}}\AgdaSymbol{)}\<%
\\
\>[0]\AgdaKeyword{open}\AgdaSpace{}%
\AgdaKeyword{import}\AgdaSpace{}%
\AgdaModule{Data.List.NonEmpty}\AgdaSpace{}%
\AgdaKeyword{hiding}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaField{head}\AgdaSymbol{;}\AgdaSpace{}%
\AgdaOperator{\AgdaFunction{[\AgdaUnderscore{}]}}\AgdaSymbol{)}\<%
\\
\>[0]\AgdaKeyword{open}\AgdaSpace{}%
\AgdaKeyword{import}\AgdaSpace{}%
\AgdaModule{Data.Nat}\AgdaSpace{}%
\AgdaKeyword{using}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaDatatype{ℕ}\AgdaSymbol{;}\AgdaSpace{}%
\AgdaOperator{\AgdaPrimitive{\AgdaUnderscore{}+\AgdaUnderscore{}}}\AgdaSymbol{;}\AgdaSpace{}%
\AgdaOperator{\AgdaFunction{\AgdaUnderscore{}≥\AgdaUnderscore{}}}\AgdaSymbol{;}\AgdaSpace{}%
\AgdaOperator{\AgdaFunction{\AgdaUnderscore{}>\AgdaUnderscore{}}}\AgdaSymbol{;}\AgdaSpace{}%
\AgdaInductiveConstructor{zero}\AgdaSymbol{;}\AgdaSpace{}%
\AgdaInductiveConstructor{suc}\AgdaSymbol{;}\AgdaSpace{}%
\AgdaInductiveConstructor{s≤s}\AgdaSymbol{;}\AgdaSpace{}%
\AgdaInductiveConstructor{z≤n}\AgdaSymbol{)}\<%
\\
\>[0]\AgdaKeyword{import}\AgdaSpace{}%
\AgdaModule{Relation.Binary.PropositionalEquality}\AgdaSpace{}%
\AgdaSymbol{as}\AgdaSpace{}%
\AgdaModule{Eq}\<%
\\
\>[0]\AgdaKeyword{open}\AgdaSpace{}%
\AgdaModule{Eq}\AgdaSpace{}%
\AgdaKeyword{using}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaOperator{\AgdaDatatype{\AgdaUnderscore{}≡\AgdaUnderscore{}}}\AgdaSymbol{;}\AgdaSpace{}%
\AgdaInductiveConstructor{refl}\AgdaSymbol{;}\AgdaSpace{}%
\AgdaFunction{cong}\AgdaSymbol{;}\AgdaSpace{}%
\AgdaKeyword{module}\AgdaSpace{}%
\AgdaModule{≡-Reasoning}\AgdaSymbol{;}\AgdaSpace{}%
\AgdaFunction{sym}\AgdaSymbol{)}\<%
\\
\>[0]\AgdaKeyword{open}\AgdaSpace{}%
\AgdaModule{≡-Reasoning}\<%
\\
\>[0]\AgdaKeyword{open}\AgdaSpace{}%
\AgdaKeyword{import}\AgdaSpace{}%
\AgdaModule{Agda.Builtin.Equality}\<%
\\
%
\\[\AgdaEmptyExtraSkip]%
%
\\[\AgdaEmptyExtraSkip]%
\>[0]\AgdaComment{--our\ libraries}\<%
\\
\>[0]\AgdaKeyword{open}\AgdaSpace{}%
\AgdaKeyword{import}\AgdaSpace{}%
\AgdaModule{libraries.listLib}\<%
\\
\>[0]\AgdaKeyword{open}\AgdaSpace{}%
\AgdaKeyword{import}\AgdaSpace{}%
\AgdaModule{libraries.emptyLib}\<%
\\
\>[0]\AgdaKeyword{open}\AgdaSpace{}%
\AgdaKeyword{import}\AgdaSpace{}%
\AgdaModule{libraries.natLib}\<%
\\
\>[0]\AgdaKeyword{open}\AgdaSpace{}%
\AgdaKeyword{import}\AgdaSpace{}%
\AgdaModule{libraries.boolLib}\<%
\\
\>[0]\AgdaKeyword{open}\AgdaSpace{}%
\AgdaKeyword{import}\AgdaSpace{}%
\AgdaModule{libraries.equalityLib}\<%
\\
\>[0]\AgdaKeyword{open}\AgdaSpace{}%
\AgdaKeyword{import}\AgdaSpace{}%
\AgdaModule{libraries.andLib}\<%
\\
\>[0]\AgdaKeyword{open}\AgdaSpace{}%
\AgdaKeyword{import}\AgdaSpace{}%
\AgdaModule{libraries.miscLib}\<%
\\
\>[0]\AgdaKeyword{open}\AgdaSpace{}%
\AgdaKeyword{import}\AgdaSpace{}%
\AgdaModule{libraries.maybeLib}\<%
\\
%
\\[\AgdaEmptyExtraSkip]%
\>[0]\AgdaKeyword{open}\AgdaSpace{}%
\AgdaKeyword{import}\AgdaSpace{}%
\AgdaModule{stack}\<%
\\
\>[0]\AgdaKeyword{open}\AgdaSpace{}%
\AgdaKeyword{import}\AgdaSpace{}%
\AgdaModule{stackPredicate}\<%
\\
\>[0]\AgdaKeyword{open}\AgdaSpace{}%
\AgdaKeyword{import}\AgdaSpace{}%
\AgdaModule{semanticBasicOperations}\AgdaSpace{}%
\AgdaBound{param}\<%
\\
\>[0]\AgdaKeyword{open}\AgdaSpace{}%
\AgdaKeyword{import}\AgdaSpace{}%
\AgdaModule{instructionBasic}\<%
\\
\>[0]\AgdaKeyword{open}\AgdaSpace{}%
\AgdaKeyword{import}\AgdaSpace{}%
\AgdaModule{verificationMultiSig}\AgdaSpace{}%
\AgdaBound{param}\<%
\\
\>[0]\AgdaKeyword{open}\AgdaSpace{}%
\AgdaKeyword{import}\AgdaSpace{}%
\AgdaModule{hoareTripleStack}\AgdaSpace{}%
\AgdaBound{param}\<%
\\
\>[0]\AgdaKeyword{open}\AgdaSpace{}%
\AgdaKeyword{import}\AgdaSpace{}%
\AgdaModule{verificationStackScripts.semanticsStackInstructions}\AgdaSpace{}%
\AgdaBound{param}\<%
\\
\>[0]\AgdaKeyword{open}\AgdaSpace{}%
\AgdaKeyword{import}\AgdaSpace{}%
\AgdaModule{verificationStackScripts.stackVerificationLemmas}\AgdaSpace{}%
\AgdaBound{param}\<%
\\
\>[0]\AgdaKeyword{open}\AgdaSpace{}%
\AgdaKeyword{import}\AgdaSpace{}%
\AgdaModule{verificationStackScripts.stackHoareTriple}\AgdaSpace{}%
\AgdaBound{param}\<%
\\
\>[0]\AgdaKeyword{open}\AgdaSpace{}%
\AgdaKeyword{import}\AgdaSpace{}%
\AgdaModule{verificationStackScripts.sPredicate}\<%
\\
\>[0]\AgdaKeyword{open}\AgdaSpace{}%
\AgdaKeyword{import}\AgdaSpace{}%
\AgdaModule{verificationStackScripts.hoareTripleStackBasic}\AgdaSpace{}%
\AgdaBound{param}\<%
\\
\>[0]\AgdaKeyword{open}\AgdaSpace{}%
\AgdaKeyword{import}\AgdaSpace{}%
\AgdaModule{verificationStackScripts.stackState}\<%
\\
\>[0]\AgdaKeyword{open}\AgdaSpace{}%
\AgdaKeyword{import}\AgdaSpace{}%
\AgdaModule{verificationStackScripts.stackSemanticsInstructionsBasic}\AgdaSpace{}%
\AgdaBound{param}\<%
\\
\>[0]\AgdaKeyword{open}\AgdaSpace{}%
\AgdaKeyword{import}\AgdaSpace{}%
\AgdaModule{verificationStackScripts.stackVerificationLemmasPart2}\AgdaSpace{}%
\AgdaBound{param}\<%
\\
\>[0]\AgdaKeyword{open}\AgdaSpace{}%
\AgdaKeyword{import}\AgdaSpace{}%
\AgdaModule{verificationStackScripts.stackVerificationP2PKH}\AgdaSpace{}%
\AgdaBound{param}\<%
\\
%
\\[\AgdaEmptyExtraSkip]%
\>[0]\AgdaFunction{mainLemmaCorrectnessMultiSig-2-4}\AgdaSpace{}%
\AgdaSymbol{:}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaBound{msg₁}\AgdaSpace{}%
\AgdaSymbol{:}\AgdaSpace{}%
\AgdaDatatype{Msg}\AgdaSymbol{)(}\AgdaBound{pbk1}\AgdaSpace{}%
\AgdaBound{pbk2}\AgdaSpace{}%
\AgdaBound{pbk3}\AgdaSpace{}%
\AgdaBound{pbk4}%
\>[69]\AgdaSymbol{:}\AgdaSpace{}%
\AgdaDatatype{ℕ}\AgdaSymbol{)}\AgdaSpace{}%
\AgdaSymbol{→}\<%
\\
\>[0][@{}l@{\AgdaIndent{0}}]%
\>[19]\AgdaOperator{\AgdaFunction{<}}\AgdaSpace{}%
\AgdaFunction{weakestPreCondMultiSig-2-4ˢ}\AgdaSpace{}%
\AgdaBound{pbk1}\AgdaSpace{}%
\AgdaBound{pbk2}\AgdaSpace{}%
\AgdaBound{pbk3}\AgdaSpace{}%
\AgdaBound{pbk4}\AgdaSpace{}%
\AgdaOperator{\AgdaFunction{>stackb}}\<%
\\
\>[19][@{}l@{\AgdaIndent{0}}]%
\>[20]\AgdaFunction{multiSigScript2-4ᵇ}\AgdaSpace{}%
\AgdaBound{pbk1}\AgdaSpace{}%
\AgdaBound{pbk2}\AgdaSpace{}%
\AgdaBound{pbk3}\AgdaSpace{}%
\AgdaBound{pbk4}\<%
\\
\>[0][@{}l@{\AgdaIndent{0}}]%
\>[18]\AgdaOperator{\AgdaFunction{<}}\AgdaSpace{}%
\AgdaFunction{acceptStateˢ}\AgdaSpace{}%
\AgdaOperator{\AgdaFunction{>}}\<%
\\
\>[0]\AgdaFunction{mainLemmaCorrectnessMultiSig-2-4}\AgdaSpace{}%
\AgdaBound{msg₁}\AgdaSpace{}%
\AgdaBound{pbk1}\AgdaSpace{}%
\AgdaBound{pbk2}\AgdaSpace{}%
\AgdaBound{pbk3}\AgdaSpace{}%
\AgdaBound{pbk4}\AgdaSpace{}%
\AgdaSymbol{.}\AgdaField{==>stg}\AgdaSpace{}%
\AgdaBound{time}\AgdaSpace{}%
\AgdaBound{msg₂}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaBound{sig2}\AgdaSpace{}%
\AgdaOperator{\AgdaInductiveConstructor{∷}}\AgdaSpace{}%
\AgdaBound{sig1}\AgdaSpace{}%
\AgdaOperator{\AgdaInductiveConstructor{∷}}\AgdaSpace{}%
\AgdaBound{dummy}\AgdaSpace{}%
\AgdaOperator{\AgdaInductiveConstructor{∷}}\AgdaSpace{}%
\AgdaBound{stack}\AgdaSymbol{)}\<%
\\
\>[0][@{}l@{\AgdaIndent{0}}]%
\>[2]\AgdaSymbol{(}\AgdaInductiveConstructor{inj₁}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaInductiveConstructor{conj}\AgdaSpace{}%
\AgdaBound{and3}\AgdaSpace{}%
\AgdaBound{and4}\AgdaSymbol{))}\AgdaSpace{}%
\AgdaSymbol{=}\<%
\\
\>[2][@{}l@{\AgdaIndent{0}}]%
\>[3]\AgdaFunction{boolToNatNotFalseLemma}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaFunction{compareSigsMultiSigAux}\AgdaSpace{}%
\AgdaBound{msg₂}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaBound{sig2}\AgdaSpace{}%
\AgdaOperator{\AgdaInductiveConstructor{∷}}\AgdaSpace{}%
\AgdaInductiveConstructor{[]}\AgdaSymbol{)}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaBound{pbk2}\AgdaSpace{}%
\AgdaOperator{\AgdaInductiveConstructor{∷}}\AgdaSpace{}%
\AgdaBound{pbk3}\AgdaSpace{}%
\AgdaOperator{\AgdaInductiveConstructor{∷}}\AgdaSpace{}%
\AgdaBound{pbk4}\AgdaSpace{}%
\AgdaOperator{\AgdaInductiveConstructor{∷}}\AgdaSpace{}%
\AgdaInductiveConstructor{[]}\AgdaSymbol{)}\AgdaSpace{}%
\AgdaBound{sig1}\<%
\\
%
\>[3]\AgdaSymbol{(}\AgdaFunction{isSigned}%
\>[14]\AgdaBound{msg₂}\AgdaSpace{}%
\AgdaBound{sig1}\AgdaSpace{}%
\AgdaBound{pbk1}\AgdaSymbol{))}\<%
\\
%
\>[2]\AgdaSymbol{(}\AgdaFunction{lemmaHoareTripleStackGeAux'7}\AgdaSpace{}%
\AgdaBound{msg₂}\AgdaSpace{}%
\AgdaBound{pbk1}\AgdaSpace{}%
\AgdaBound{pbk2}\AgdaSpace{}%
\AgdaBound{pbk3}\AgdaSpace{}%
\AgdaBound{pbk4}\AgdaSpace{}%
\AgdaBound{sig1}\AgdaSpace{}%
\AgdaBound{sig2}\AgdaSpace{}%
\AgdaBound{and3}\AgdaSpace{}%
\AgdaBound{and4}\AgdaSymbol{)}\<%
\\
\>[0]\AgdaFunction{mainLemmaCorrectnessMultiSig-2-4}\AgdaSpace{}%
\AgdaBound{msg₁}\AgdaSpace{}%
\AgdaBound{pbk1}\AgdaSpace{}%
\AgdaBound{pbk2}\AgdaSpace{}%
\AgdaBound{pbk3}\AgdaSpace{}%
\AgdaBound{pbk4}\AgdaSpace{}%
\AgdaSymbol{.}\AgdaField{==>stg}\AgdaSpace{}%
\AgdaBound{time}\AgdaSpace{}%
\AgdaBound{msg₂}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaBound{sig2}\AgdaSpace{}%
\AgdaOperator{\AgdaInductiveConstructor{∷}}\AgdaSpace{}%
\AgdaBound{sig1}\AgdaSpace{}%
\AgdaOperator{\AgdaInductiveConstructor{∷}}\AgdaSpace{}%
\AgdaBound{dummy}\AgdaSpace{}%
\AgdaOperator{\AgdaInductiveConstructor{∷}}\AgdaSpace{}%
\AgdaBound{stack}\AgdaSymbol{)}\<%
\\
\>[0][@{}l@{\AgdaIndent{0}}]%
\>[2]\AgdaSymbol{(}\AgdaInductiveConstructor{inj₂}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaInductiveConstructor{inj₁}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaInductiveConstructor{conj}\AgdaSpace{}%
\AgdaBound{and3}\AgdaSpace{}%
\AgdaBound{and4}\AgdaSymbol{)))}\AgdaSpace{}%
\AgdaSymbol{=}\<%
\\
\>[2][@{}l@{\AgdaIndent{0}}]%
\>[3]\AgdaFunction{boolToNatNotFalseLemma}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaFunction{compareSigsMultiSigAux}\AgdaSpace{}%
\AgdaBound{msg₂}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaBound{sig2}\AgdaSpace{}%
\AgdaOperator{\AgdaInductiveConstructor{∷}}\AgdaSpace{}%
\AgdaInductiveConstructor{[]}\AgdaSymbol{)}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaBound{pbk2}\AgdaSpace{}%
\AgdaOperator{\AgdaInductiveConstructor{∷}}\AgdaSpace{}%
\AgdaBound{pbk3}\AgdaSpace{}%
\AgdaOperator{\AgdaInductiveConstructor{∷}}\AgdaSpace{}%
\AgdaBound{pbk4}\AgdaSpace{}%
\AgdaOperator{\AgdaInductiveConstructor{∷}}\AgdaSpace{}%
\AgdaInductiveConstructor{[]}\AgdaSymbol{)}\AgdaSpace{}%
\AgdaBound{sig1}\<%
\\
%
\>[3]\AgdaSymbol{(}\AgdaFunction{isSigned}%
\>[14]\AgdaBound{msg₂}\AgdaSpace{}%
\AgdaBound{sig1}\AgdaSpace{}%
\AgdaBound{pbk1}\AgdaSymbol{))}\<%
\\
%
\>[2]\AgdaSymbol{(}\AgdaFunction{lemmaHoareTripleStackGeAux'8}\AgdaSpace{}%
\AgdaBound{msg₂}\AgdaSpace{}%
\AgdaBound{pbk1}\AgdaSpace{}%
\AgdaBound{pbk2}\AgdaSpace{}%
\AgdaBound{pbk3}\AgdaSpace{}%
\AgdaBound{pbk4}\AgdaSpace{}%
\AgdaBound{sig1}\AgdaSpace{}%
\AgdaBound{sig2}\AgdaSpace{}%
\AgdaBound{and3}\AgdaSpace{}%
\AgdaBound{and4}\AgdaSymbol{)}\<%
\\
\>[0]\AgdaFunction{mainLemmaCorrectnessMultiSig-2-4}\AgdaSpace{}%
\AgdaBound{msg₁}\AgdaSpace{}%
\AgdaBound{pbk1}\AgdaSpace{}%
\AgdaBound{pbk2}\AgdaSpace{}%
\AgdaBound{pbk3}\AgdaSpace{}%
\AgdaBound{pbk4}\AgdaSpace{}%
\AgdaSymbol{.}\AgdaField{==>stg}\AgdaSpace{}%
\AgdaBound{time}\AgdaSpace{}%
\AgdaBound{msg₂}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaBound{sig2}\AgdaSpace{}%
\AgdaOperator{\AgdaInductiveConstructor{∷}}\AgdaSpace{}%
\AgdaBound{sig1}\AgdaSpace{}%
\AgdaOperator{\AgdaInductiveConstructor{∷}}\AgdaSpace{}%
\AgdaBound{dummy}\AgdaSpace{}%
\AgdaOperator{\AgdaInductiveConstructor{∷}}\AgdaSpace{}%
\AgdaBound{stack}\AgdaSymbol{)}\<%
\\
\>[0][@{}l@{\AgdaIndent{0}}]%
\>[2]\AgdaSymbol{(}\AgdaInductiveConstructor{inj₂}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaInductiveConstructor{inj₂}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaInductiveConstructor{inj₁}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaInductiveConstructor{conj}\AgdaSpace{}%
\AgdaBound{and3}\AgdaSpace{}%
\AgdaBound{and4}\AgdaSymbol{))))}\AgdaSpace{}%
\AgdaSymbol{=}\<%
\\
\>[2][@{}l@{\AgdaIndent{0}}]%
\>[3]\AgdaFunction{boolToNatNotFalseLemma}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaFunction{compareSigsMultiSigAux}\AgdaSpace{}%
\AgdaBound{msg₂}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaBound{sig2}\AgdaSpace{}%
\AgdaOperator{\AgdaInductiveConstructor{∷}}\AgdaSpace{}%
\AgdaInductiveConstructor{[]}\AgdaSymbol{)}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaBound{pbk2}\AgdaSpace{}%
\AgdaOperator{\AgdaInductiveConstructor{∷}}\AgdaSpace{}%
\AgdaBound{pbk3}\AgdaSpace{}%
\AgdaOperator{\AgdaInductiveConstructor{∷}}\AgdaSpace{}%
\AgdaBound{pbk4}\AgdaSpace{}%
\AgdaOperator{\AgdaInductiveConstructor{∷}}\AgdaSpace{}%
\AgdaInductiveConstructor{[]}\AgdaSymbol{)}\AgdaSpace{}%
\AgdaBound{sig1}\<%
\\
%
\>[3]\AgdaSymbol{(}\AgdaFunction{isSigned}%
\>[14]\AgdaBound{msg₂}\AgdaSpace{}%
\AgdaBound{sig1}\AgdaSpace{}%
\AgdaBound{pbk1}\AgdaSymbol{))}\<%
\\
%
\>[3]\AgdaSymbol{(}\AgdaFunction{lemmaHoareTripleStackGeAux'9}\AgdaSpace{}%
\AgdaBound{msg₂}\AgdaSpace{}%
\AgdaBound{pbk1}\AgdaSpace{}%
\AgdaBound{pbk2}\AgdaSpace{}%
\AgdaBound{pbk3}\AgdaSpace{}%
\AgdaBound{pbk4}\AgdaSpace{}%
\AgdaBound{sig1}\AgdaSpace{}%
\AgdaBound{sig2}\AgdaSpace{}%
\AgdaBound{and3}\AgdaSpace{}%
\AgdaBound{and4}\AgdaSymbol{)}\<%
\\
\>[0]\AgdaFunction{mainLemmaCorrectnessMultiSig-2-4}\AgdaSpace{}%
\AgdaBound{msg₁}\AgdaSpace{}%
\AgdaBound{pbk1}\AgdaSpace{}%
\AgdaBound{pbk2}\AgdaSpace{}%
\AgdaBound{pbk3}\AgdaSpace{}%
\AgdaBound{pbk4}\AgdaSpace{}%
\AgdaSymbol{.}\AgdaField{==>stg}\AgdaSpace{}%
\AgdaBound{time}\AgdaSpace{}%
\AgdaBound{msg₂}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaBound{sig2}\AgdaSpace{}%
\AgdaOperator{\AgdaInductiveConstructor{∷}}\AgdaSpace{}%
\AgdaBound{sig1}\AgdaSpace{}%
\AgdaOperator{\AgdaInductiveConstructor{∷}}\AgdaSpace{}%
\AgdaBound{dummy}\AgdaSpace{}%
\AgdaOperator{\AgdaInductiveConstructor{∷}}\AgdaSpace{}%
\AgdaBound{stack}\AgdaSymbol{)}\<%
\\
\>[0][@{}l@{\AgdaIndent{0}}]%
\>[2]\AgdaSymbol{(}\AgdaInductiveConstructor{inj₂}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaInductiveConstructor{inj₂}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaInductiveConstructor{inj₂}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaInductiveConstructor{inj₁}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaInductiveConstructor{conj}\AgdaSpace{}%
\AgdaBound{and3}\AgdaSpace{}%
\AgdaBound{and4}\AgdaSymbol{)))))}\AgdaSpace{}%
\AgdaSymbol{=}\<%
\\
\>[2][@{}l@{\AgdaIndent{0}}]%
\>[3]\AgdaFunction{boolToNatNotFalseLemma}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaFunction{compareSigsMultiSigAux}\AgdaSpace{}%
\AgdaBound{msg₂}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaBound{sig2}\AgdaSpace{}%
\AgdaOperator{\AgdaInductiveConstructor{∷}}\AgdaSpace{}%
\AgdaInductiveConstructor{[]}\AgdaSymbol{)}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaBound{pbk2}\AgdaSpace{}%
\AgdaOperator{\AgdaInductiveConstructor{∷}}\AgdaSpace{}%
\AgdaBound{pbk3}\AgdaSpace{}%
\AgdaOperator{\AgdaInductiveConstructor{∷}}\AgdaSpace{}%
\AgdaBound{pbk4}\AgdaSpace{}%
\AgdaOperator{\AgdaInductiveConstructor{∷}}\AgdaSpace{}%
\AgdaInductiveConstructor{[]}\AgdaSymbol{)}\AgdaSpace{}%
\AgdaBound{sig1}\<%
\\
%
\>[3]\AgdaSymbol{(}\AgdaFunction{isSigned}%
\>[14]\AgdaBound{msg₂}\AgdaSpace{}%
\AgdaBound{sig1}\AgdaSpace{}%
\AgdaBound{pbk1}\AgdaSymbol{))}\<%
\\
%
\>[3]\AgdaSymbol{(}\AgdaFunction{lemmaHoareTripleStackGeAux'10}\AgdaSpace{}%
\AgdaBound{msg₂}\AgdaSpace{}%
\AgdaBound{pbk1}\AgdaSpace{}%
\AgdaBound{pbk2}\AgdaSpace{}%
\AgdaBound{pbk3}\AgdaSpace{}%
\AgdaBound{pbk4}\AgdaSpace{}%
\AgdaBound{sig1}\AgdaSpace{}%
\AgdaBound{sig2}\AgdaSpace{}%
\AgdaBound{and3}\AgdaSpace{}%
\AgdaBound{and4}\AgdaSymbol{)}\<%
\\
\>[0]\AgdaFunction{mainLemmaCorrectnessMultiSig-2-4}\AgdaSpace{}%
\AgdaBound{msg₁}\AgdaSpace{}%
\AgdaBound{pbk1}\AgdaSpace{}%
\AgdaBound{pbk2}\AgdaSpace{}%
\AgdaBound{pbk3}\AgdaSpace{}%
\AgdaBound{pbk4}\AgdaSpace{}%
\AgdaSymbol{.}\AgdaField{==>stg}\AgdaSpace{}%
\AgdaBound{time}\AgdaSpace{}%
\AgdaBound{msg₂}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaBound{sig2}\AgdaSpace{}%
\AgdaOperator{\AgdaInductiveConstructor{∷}}\AgdaSpace{}%
\AgdaBound{sig1}\AgdaSpace{}%
\AgdaOperator{\AgdaInductiveConstructor{∷}}\AgdaSpace{}%
\AgdaBound{dummy}\AgdaSpace{}%
\AgdaOperator{\AgdaInductiveConstructor{∷}}\AgdaSpace{}%
\AgdaBound{stack}\AgdaSymbol{)}\<%
\\
\>[0][@{}l@{\AgdaIndent{0}}]%
\>[2]\AgdaSymbol{(}\AgdaInductiveConstructor{inj₂}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaInductiveConstructor{inj₂}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaInductiveConstructor{inj₂}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaInductiveConstructor{inj₂}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaInductiveConstructor{inj₁}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaInductiveConstructor{conj}\AgdaSpace{}%
\AgdaBound{and3}\AgdaSpace{}%
\AgdaBound{and4}\AgdaSymbol{))))))}\AgdaSpace{}%
\AgdaSymbol{=}\<%
\\
\>[2][@{}l@{\AgdaIndent{0}}]%
\>[3]\AgdaFunction{boolToNatNotFalseLemma}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaFunction{compareSigsMultiSigAux}\AgdaSpace{}%
\AgdaBound{msg₂}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaBound{sig2}\AgdaSpace{}%
\AgdaOperator{\AgdaInductiveConstructor{∷}}\AgdaSpace{}%
\AgdaInductiveConstructor{[]}\AgdaSymbol{)}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaBound{pbk2}\AgdaSpace{}%
\AgdaOperator{\AgdaInductiveConstructor{∷}}\AgdaSpace{}%
\AgdaBound{pbk3}\AgdaSpace{}%
\AgdaOperator{\AgdaInductiveConstructor{∷}}\AgdaSpace{}%
\AgdaBound{pbk4}\AgdaSpace{}%
\AgdaOperator{\AgdaInductiveConstructor{∷}}\AgdaSpace{}%
\AgdaInductiveConstructor{[]}\AgdaSymbol{)}\AgdaSpace{}%
\AgdaBound{sig1}\<%
\\
%
\>[3]\AgdaSymbol{(}\AgdaFunction{isSigned}%
\>[14]\AgdaBound{msg₂}\AgdaSpace{}%
\AgdaBound{sig1}\AgdaSpace{}%
\AgdaBound{pbk1}\AgdaSymbol{))}\<%
\\
%
\>[3]\AgdaSymbol{(}\AgdaFunction{lemmaHoareTripleStackGeAux'11}\AgdaSpace{}%
\AgdaBound{msg₂}\AgdaSpace{}%
\AgdaBound{pbk1}\AgdaSpace{}%
\AgdaBound{pbk2}\AgdaSpace{}%
\AgdaBound{pbk3}\AgdaSpace{}%
\AgdaBound{pbk4}\AgdaSpace{}%
\AgdaBound{sig1}\AgdaSpace{}%
\AgdaBound{sig2}\AgdaSpace{}%
\AgdaBound{and3}\AgdaSpace{}%
\AgdaBound{and4}\AgdaSymbol{)}\<%
\\
\>[0]\AgdaFunction{mainLemmaCorrectnessMultiSig-2-4}\AgdaSpace{}%
\AgdaBound{msg₁}\AgdaSpace{}%
\AgdaBound{pbk1}\AgdaSpace{}%
\AgdaBound{pbk2}\AgdaSpace{}%
\AgdaBound{pbk3}\AgdaSpace{}%
\AgdaBound{pbk4}\AgdaSpace{}%
\AgdaSymbol{.}\AgdaField{==>stg}\AgdaSpace{}%
\AgdaBound{time}\AgdaSpace{}%
\AgdaBound{msg₂}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaBound{sig2}\AgdaSpace{}%
\AgdaOperator{\AgdaInductiveConstructor{∷}}\AgdaSpace{}%
\AgdaBound{sig1}\AgdaSpace{}%
\AgdaOperator{\AgdaInductiveConstructor{∷}}\AgdaSpace{}%
\AgdaBound{dummy}\AgdaSpace{}%
\AgdaOperator{\AgdaInductiveConstructor{∷}}\AgdaSpace{}%
\AgdaBound{stack}\AgdaSymbol{)}\<%
\\
\>[0][@{}l@{\AgdaIndent{0}}]%
\>[2]\AgdaSymbol{(}\AgdaInductiveConstructor{inj₂}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaInductiveConstructor{inj₂}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaInductiveConstructor{inj₂}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaInductiveConstructor{inj₂}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaInductiveConstructor{inj₂}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaInductiveConstructor{conj}\AgdaSpace{}%
\AgdaBound{and3}\AgdaSpace{}%
\AgdaBound{and4}\AgdaSymbol{))))))}\AgdaSpace{}%
\AgdaSymbol{=}\<%
\\
\>[2][@{}l@{\AgdaIndent{0}}]%
\>[3]\AgdaFunction{boolToNatNotFalseLemma}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaFunction{compareSigsMultiSigAux}\AgdaSpace{}%
\AgdaBound{msg₂}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaBound{sig2}\AgdaSpace{}%
\AgdaOperator{\AgdaInductiveConstructor{∷}}\AgdaSpace{}%
\AgdaInductiveConstructor{[]}\AgdaSymbol{)}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaBound{pbk2}\AgdaSpace{}%
\AgdaOperator{\AgdaInductiveConstructor{∷}}\AgdaSpace{}%
\AgdaBound{pbk3}\AgdaSpace{}%
\AgdaOperator{\AgdaInductiveConstructor{∷}}\AgdaSpace{}%
\AgdaBound{pbk4}\AgdaSpace{}%
\AgdaOperator{\AgdaInductiveConstructor{∷}}\AgdaSpace{}%
\AgdaInductiveConstructor{[]}\AgdaSymbol{)}\AgdaSpace{}%
\AgdaBound{sig1}\<%
\\
%
\>[3]\AgdaSymbol{(}\AgdaFunction{isSigned}%
\>[14]\AgdaBound{msg₂}\AgdaSpace{}%
\AgdaBound{sig1}\AgdaSpace{}%
\AgdaBound{pbk1}\AgdaSymbol{))}\<%
\\
%
\>[3]\AgdaSymbol{(}\AgdaFunction{lemmaHoareTripleStackGeAux'12}\AgdaSpace{}%
\AgdaBound{msg₂}\AgdaSpace{}%
\AgdaBound{pbk1}\AgdaSpace{}%
\AgdaBound{pbk2}\AgdaSpace{}%
\AgdaBound{pbk3}\AgdaSpace{}%
\AgdaBound{pbk4}\AgdaSpace{}%
\AgdaBound{sig1}\AgdaSpace{}%
\AgdaBound{sig2}\AgdaSpace{}%
\AgdaBound{and3}\AgdaSpace{}%
\AgdaBound{and4}\AgdaSymbol{)}\<%
\\
\>[0]\AgdaFunction{mainLemmaCorrectnessMultiSig-2-4}\AgdaSpace{}%
\AgdaBound{msg₁}\AgdaSpace{}%
\AgdaBound{pbk1}\AgdaSpace{}%
\AgdaBound{pbk2}\AgdaSpace{}%
\AgdaBound{pbk3}\AgdaSpace{}%
\AgdaBound{pbk4}\AgdaSpace{}%
\AgdaSymbol{.}\AgdaField{<==stg}\AgdaSpace{}%
\AgdaBound{time}\AgdaSpace{}%
\AgdaBound{msg₂}%
\>[77]\AgdaSymbol{(}\AgdaBound{sig2}\AgdaSpace{}%
\AgdaOperator{\AgdaInductiveConstructor{∷}}\AgdaSpace{}%
\AgdaBound{sig1}\AgdaSpace{}%
\AgdaOperator{\AgdaInductiveConstructor{∷}}\AgdaSpace{}%
\AgdaBound{dummy}\AgdaSpace{}%
\AgdaOperator{\AgdaInductiveConstructor{∷}}\AgdaSpace{}%
\AgdaBound{stack}\AgdaSymbol{)}\AgdaSpace{}%
\AgdaBound{x}\AgdaSpace{}%
\AgdaSymbol{=}\<%
\\
\>[0][@{}l@{\AgdaIndent{0}}]%
\>[2]\AgdaFunction{lemmaHoareTripleStackGeAux'Comb2-4}\AgdaSpace{}%
\AgdaBound{msg₂}\AgdaSpace{}%
\AgdaBound{pbk1}\AgdaSpace{}%
\AgdaBound{pbk2}\AgdaSpace{}%
\AgdaBound{pbk3}\AgdaSpace{}%
\AgdaBound{pbk4}\AgdaSpace{}%
\AgdaBound{sig1}\AgdaSpace{}%
\AgdaBound{sig2}\<%
\\
%
\>[2]\AgdaSymbol{(}\AgdaFunction{boolToNatNotFalseLemma2}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaFunction{compareSigsMultiSigAux}\AgdaSpace{}%
\AgdaBound{msg₂}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaBound{sig2}\AgdaSpace{}%
\AgdaOperator{\AgdaInductiveConstructor{∷}}\AgdaSpace{}%
\AgdaInductiveConstructor{[]}\AgdaSymbol{)}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaBound{pbk2}\AgdaSpace{}%
\AgdaOperator{\AgdaInductiveConstructor{∷}}\AgdaSpace{}%
\AgdaBound{pbk3}\AgdaSpace{}%
\AgdaOperator{\AgdaInductiveConstructor{∷}}\AgdaSpace{}%
\AgdaBound{pbk4}\AgdaSpace{}%
\AgdaOperator{\AgdaInductiveConstructor{∷}}\AgdaSpace{}%
\AgdaInductiveConstructor{[]}\AgdaSymbol{)}\<%
\\
%
\>[2]\AgdaBound{sig1}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaFunction{isSigned}%
\>[18]\AgdaBound{msg₂}\AgdaSpace{}%
\AgdaBound{sig1}\AgdaSpace{}%
\AgdaBound{pbk1}\AgdaSymbol{))}\AgdaSpace{}%
\AgdaBound{x}\AgdaSymbol{)}\<%
\\
%
\\[\AgdaEmptyExtraSkip]%
%
\\[\AgdaEmptyExtraSkip]%
\>[0]\AgdaFunction{weakestPreCondMultiSig-2-4}\AgdaSpace{}%
\AgdaSymbol{:}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaBound{pbk1}\AgdaSpace{}%
\AgdaBound{pbk2}\AgdaSpace{}%
\AgdaBound{pbk3}\AgdaSpace{}%
\AgdaBound{pbk4}\AgdaSpace{}%
\AgdaSymbol{:}%
\>[53]\AgdaDatatype{ℕ}\AgdaSymbol{)→}\AgdaSpace{}%
\AgdaFunction{StackStatePred}\<%
\\
\>[0]\AgdaComment{--\textbackslash{}verificationMultiSigBasicweakestPreCondMultiSigNos}\<%
\end{code}
} % END AgdaHide

\newcommand{\verificationMultiSigBasicweakestPreCondMultiSigNos}{
\begin{code}%
\>[0]\AgdaFunction{weakestPreCondMultiSig-2-4}\AgdaSpace{}%
\AgdaBound{pbk1}\AgdaSpace{}%
\AgdaBound{pbk2}\AgdaSpace{}%
\AgdaBound{pbk3}\AgdaSpace{}%
\AgdaBound{pbk4}\<%
\\
\>[0][@{}l@{\AgdaIndent{0}}]%
\>[5]\AgdaSymbol{=}\AgdaSpace{}%
\AgdaFunction{stackPred2SPred}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaFunction{weakestPreCondMultiSig-2-4ˢ}\AgdaSpace{}%
\AgdaBound{pbk1}\AgdaSpace{}%
\AgdaBound{pbk2}\AgdaSpace{}%
\AgdaBound{pbk3}\AgdaSpace{}%
\AgdaBound{pbk4}\AgdaSymbol{)}\<%
\end{code}
} % END newcommand

\AgdaHide{
\begin{code}%
\>[0]\<%
\\
%
\\[\AgdaEmptyExtraSkip]%
%
\\[\AgdaEmptyExtraSkip]%
%
\\[\AgdaEmptyExtraSkip]%
\>[0]\AgdaComment{--\ Main\ theorem\ for\ multisig-2-4}\<%
\\
\>[0]\AgdaComment{--\textbackslash{}verificationMultiSigBasictheoremCorrectnessMultiSigTwoFour}\<%
\end{code}
} % END AgdaHide

\newcommand{\verificationMultiSigBasictheoremCorrectnessMultiSigTwoFour}{
\begin{code}%
\>[0]\AgdaFunction{theoremCorrectnessMultiSig-2-4}\AgdaSpace{}%
\AgdaSymbol{:}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaBound{pbk1}\AgdaSpace{}%
\AgdaBound{pbk2}\AgdaSpace{}%
\AgdaBound{pbk3}\AgdaSpace{}%
\AgdaBound{pbk4}\AgdaSpace{}%
\AgdaSymbol{:}%
\>[57]\AgdaDatatype{ℕ}\AgdaSymbol{)}\<%
\\
\>[0][@{}l@{\AgdaIndent{0}}]%
\>[3]\AgdaSymbol{→}%
\>[6]\AgdaOperator{\AgdaRecord{<}}%
\>[9]\AgdaFunction{stackPred2SPred}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaFunction{weakestPreCondMultiSig-2-4ˢ}\AgdaSpace{}%
\AgdaBound{pbk1}\AgdaSpace{}%
\AgdaBound{pbk2}\AgdaSpace{}%
\AgdaBound{pbk3}\AgdaSpace{}%
\AgdaBound{pbk4}\AgdaSymbol{)}\AgdaSpace{}%
\AgdaOperator{\AgdaRecord{>ⁱᶠᶠ}}\<%
\\
\>[6][@{}l@{\AgdaIndent{0}}]%
\>[7]\AgdaFunction{multiSigScript2-4ᵇ}\AgdaSpace{}%
\AgdaBound{pbk1}\AgdaSpace{}%
\AgdaBound{pbk2}\AgdaSpace{}%
\AgdaBound{pbk3}\AgdaSpace{}%
\AgdaBound{pbk4}\<%
\\
%
\>[7]\AgdaOperator{\AgdaRecord{<}}%
\>[10]\AgdaFunction{stackPred2SPred}\AgdaSpace{}%
\AgdaFunction{acceptStateˢ}%
\>[40]\AgdaOperator{\AgdaRecord{>}}\<%
\end{code}
} % END newcommand

\AgdaHide{
\begin{code}%
\>[0]\AgdaFunction{theoremCorrectnessMultiSig-2-4}\AgdaSpace{}%
\AgdaBound{pbk1}\AgdaSpace{}%
\AgdaBound{pbk2}\AgdaSpace{}%
\AgdaBound{pbk3}\AgdaSpace{}%
\AgdaBound{pbk4}\<%
\\
\>[0][@{}l@{\AgdaIndent{0}}]%
\>[26]\AgdaSymbol{=}\AgdaSpace{}%
\AgdaFunction{hoareTripleStack2HoareTriple}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaFunction{multiSigScript2-4ᵇ}\AgdaSpace{}%
\AgdaBound{pbk1}\AgdaSpace{}%
\AgdaBound{pbk2}\AgdaSpace{}%
\AgdaBound{pbk3}\AgdaSpace{}%
\AgdaBound{pbk4}\AgdaSymbol{)}\<%
\\
%
\>[26]\AgdaSymbol{(}\AgdaFunction{weakestPreCondMultiSig-2-4ˢ}\AgdaSpace{}%
\AgdaBound{pbk1}\AgdaSpace{}%
\AgdaBound{pbk2}\AgdaSpace{}%
\AgdaBound{pbk3}\AgdaSpace{}%
\AgdaBound{pbk4}\AgdaSpace{}%
\AgdaSymbol{)}\AgdaSpace{}%
\AgdaFunction{acceptStateˢ}\<%
\\
%
\>[26]\AgdaSymbol{(}\AgdaFunction{mainLemmaCorrectnessMultiSig-2-4}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaInductiveConstructor{nat}\AgdaSpace{}%
\AgdaBound{pbk4}\AgdaSymbol{)}\AgdaSpace{}%
\AgdaBound{pbk1}\AgdaSpace{}%
\AgdaBound{pbk2}\AgdaSpace{}%
\AgdaBound{pbk3}\AgdaSpace{}%
\AgdaBound{pbk4}\AgdaSymbol{)}\<%
\end{code}
} % END newcommand

\AgdaHide{
\begin{code}%
\>[0]\<%
\\
%
\\[\AgdaEmptyExtraSkip]%
\>[0]\AgdaComment{-------------------------------------------------------------}\<%
\\
\>[0]\AgdaComment{--\ \ Here\ we\ prove\ the\ correctness\ of\ a\ combined\ script}\<%
\\
\>[0]\AgdaComment{--\ \ namely\ the\ correctness\ of\ a\ combination\ of\ a\ check\ time\ script\ and\ themultisig\ script}\<%
\\
\>[0]\AgdaComment{--}\<%
\\
\>[0]\AgdaComment{--\ This\ demonstrates\ a\ combination\ of\ method1\ and\ method\ 2:}\<%
\\
\>[0]\AgdaComment{--\ \ we\ prove\ the\ correctness\ of\ the\ time\ script\ and\ the\ multisig\ script\ separately\ (the\ time\ script\ is\ trivial\ to\ verify)}\<%
\\
\>[0]\AgdaComment{--\ \ \ \ using\ \ method\ 2}\<%
\\
\>[0]\AgdaComment{--\ Then\ we\ prove\ the\ correctenss\ of\ the\ combined\ script\ using\ method1}\<%
\\
\>[0]\AgdaComment{--\ \ \ \ and\ this\ shows\ that\ we\ can\ make\ bigger\ jumps\ in\ method\ 1}\<%
\\
\>[0]\AgdaComment{-------------------------------}\<%
\\
\>[0]\AgdaComment{--\textbackslash{}verificationMultiSigBasictheoremCorrectnessTimeCheck}\<%
\end{code}
} % END AgdaHide

\newcommand{\verificationMultiSigBasictheoremCorrectnessTimeCheck}{
\begin{code}%
\>[0]\AgdaFunction{theoremCorrectnessTimeCheck}\AgdaSpace{}%
\AgdaSymbol{:}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaBound{φ}\AgdaSpace{}%
\AgdaSymbol{:}\AgdaSpace{}%
\AgdaFunction{StackPredicate}\AgdaSymbol{)(}\AgdaBound{time₁}\AgdaSpace{}%
\AgdaSymbol{:}\AgdaSpace{}%
\AgdaFunction{Time}\AgdaSymbol{)}\<%
\\
\>[0][@{}l@{\AgdaIndent{0}}]%
\>[3]\AgdaSymbol{→}%
\>[7]\AgdaOperator{\AgdaRecord{<}}%
\>[10]\AgdaFunction{stackPred2SPred}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaFunction{timeCheckPreCond}\AgdaSpace{}%
\AgdaBound{time₁}\AgdaSpace{}%
\AgdaOperator{\AgdaFunction{∧sp}}\AgdaSpace{}%
\AgdaBound{φ}\AgdaSymbol{)}%
\>[59]\AgdaOperator{\AgdaRecord{>ⁱᶠᶠ}}\AgdaSpace{}%
\AgdaFunction{checkTimeScriptᵇ}\AgdaSpace{}%
\AgdaBound{time₁}\<%
\\
%
\>[7]\AgdaOperator{\AgdaRecord{<}}%
\>[10]\AgdaFunction{stackPred2SPred}\AgdaSpace{}%
\AgdaBound{φ}%
\>[30]\AgdaOperator{\AgdaRecord{>}}\<%
\end{code}
} % END newcommand

\AgdaHide{
\begin{code}%
\>[0]\AgdaFunction{theoremCorrectnessTimeCheck}\AgdaSpace{}%
\AgdaBound{φ}\AgdaSpace{}%
\AgdaBound{time₁}\AgdaSpace{}%
\AgdaSymbol{.}\AgdaField{==>}\AgdaSpace{}%
\AgdaOperator{\AgdaInductiveConstructor{⟨}}\AgdaSpace{}%
\AgdaBound{currentTime₁}\AgdaSpace{}%
\AgdaOperator{\AgdaInductiveConstructor{,}}\AgdaSpace{}%
\AgdaBound{msg₁}\AgdaSpace{}%
\AgdaOperator{\AgdaInductiveConstructor{,}}\AgdaSpace{}%
\AgdaBound{stack₁}\AgdaSpace{}%
\AgdaOperator{\AgdaInductiveConstructor{⟩}}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaInductiveConstructor{conj}\AgdaSpace{}%
\AgdaBound{and3}\AgdaSpace{}%
\AgdaBound{and4}\AgdaSymbol{)}\AgdaSpace{}%
\AgdaKeyword{with}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaFunction{instructOpTime}\AgdaSpace{}%
\AgdaBound{currentTime₁}\AgdaSpace{}%
\AgdaBound{time₁}\AgdaSymbol{)}\<%
\\
\>[0]\AgdaFunction{theoremCorrectnessTimeCheck}\AgdaSpace{}%
\AgdaBound{φ}\AgdaSpace{}%
\AgdaBound{time₁}\AgdaSpace{}%
\AgdaSymbol{.}\AgdaField{==>}\AgdaSpace{}%
\AgdaOperator{\AgdaInductiveConstructor{⟨}}\AgdaSpace{}%
\AgdaBound{currentTime₁}\AgdaSpace{}%
\AgdaOperator{\AgdaInductiveConstructor{,}}\AgdaSpace{}%
\AgdaBound{msg₁}\AgdaSpace{}%
\AgdaOperator{\AgdaInductiveConstructor{,}}\AgdaSpace{}%
\AgdaBound{stack₁}\AgdaSpace{}%
\AgdaOperator{\AgdaInductiveConstructor{⟩}}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaInductiveConstructor{conj}\AgdaSpace{}%
\AgdaBound{and3}\AgdaSpace{}%
\AgdaBound{and4}\AgdaSymbol{)}\AgdaSpace{}%
\AgdaSymbol{|}\AgdaSpace{}%
\AgdaInductiveConstructor{true}\AgdaSpace{}%
\AgdaSymbol{=}\AgdaSpace{}%
\AgdaBound{and4}\<%
\\
\>[0]\AgdaFunction{theoremCorrectnessTimeCheck}\AgdaSpace{}%
\AgdaBound{φ}\AgdaSpace{}%
\AgdaBound{time₁}\AgdaSpace{}%
\AgdaSymbol{.}\AgdaField{<==}\AgdaSpace{}%
\AgdaOperator{\AgdaInductiveConstructor{⟨}}\AgdaSpace{}%
\AgdaBound{currentTime₁}\AgdaSpace{}%
\AgdaOperator{\AgdaInductiveConstructor{,}}\AgdaSpace{}%
\AgdaBound{msg₁}\AgdaSpace{}%
\AgdaOperator{\AgdaInductiveConstructor{,}}\AgdaSpace{}%
\AgdaBound{stack₁}\AgdaSpace{}%
\AgdaOperator{\AgdaInductiveConstructor{⟩}}\AgdaSpace{}%
\AgdaBound{p}\AgdaSpace{}%
\AgdaKeyword{with}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaFunction{instructOpTime}\AgdaSpace{}%
\AgdaBound{currentTime₁}\AgdaSpace{}%
\AgdaBound{time₁}\AgdaSymbol{)}\<%
\\
\>[0]\AgdaFunction{theoremCorrectnessTimeCheck}\AgdaSpace{}%
\AgdaBound{φ}\AgdaSpace{}%
\AgdaBound{time₁}\AgdaSpace{}%
\AgdaSymbol{.}\AgdaField{<==}\AgdaSpace{}%
\AgdaOperator{\AgdaInductiveConstructor{⟨}}\AgdaSpace{}%
\AgdaBound{currentTime₁}\AgdaSpace{}%
\AgdaOperator{\AgdaInductiveConstructor{,}}\AgdaSpace{}%
\AgdaBound{msg₁}\AgdaSpace{}%
\AgdaOperator{\AgdaInductiveConstructor{,}}\AgdaSpace{}%
\AgdaBound{stack₁}\AgdaSpace{}%
\AgdaOperator{\AgdaInductiveConstructor{⟩}}\AgdaSpace{}%
\AgdaBound{p}\AgdaSpace{}%
\AgdaSymbol{|}\AgdaSpace{}%
\AgdaInductiveConstructor{true}\AgdaSpace{}%
\AgdaSymbol{=}\AgdaSpace{}%
\AgdaInductiveConstructor{conj}\AgdaSpace{}%
\AgdaInductiveConstructor{tt}\AgdaSpace{}%
\AgdaBound{p}\<%
\\
%
\\[\AgdaEmptyExtraSkip]%
%
\\[\AgdaEmptyExtraSkip]%
\>[0]\AgdaComment{--\textbackslash{}verificationMultiSigBasictheoremCorrectnessCombinedMultiSigTimeCheck}\<%
\end{code}
} % END AgdaHide

\newcommand{\verificationMultiSigBasictheoremCorrectnessCombinedMultiSigTimeCheck}{
\begin{code}%
\>[0]\AgdaFunction{theoremCorrectnessCombinedMultiSigTimeCheck}\AgdaSpace{}%
\AgdaSymbol{:}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaBound{time₁}\AgdaSpace{}%
\AgdaSymbol{:}\AgdaSpace{}%
\AgdaFunction{Time}\AgdaSymbol{)}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaBound{pbk1}\AgdaSpace{}%
\AgdaBound{pbk2}\AgdaSpace{}%
\AgdaBound{pbk3}\AgdaSpace{}%
\AgdaBound{pbk4}\AgdaSpace{}%
\AgdaSymbol{:}%
\>[85]\AgdaDatatype{ℕ}\AgdaSymbol{)}\<%
\\
\>[0][@{}l@{\AgdaIndent{0}}]%
\>[3]\AgdaSymbol{→}%
\>[7]\AgdaOperator{\AgdaRecord{<}}\AgdaSpace{}%
\AgdaFunction{stackPred2SPred}\AgdaSpace{}%
\AgdaSymbol{(}%
\>[28]\AgdaFunction{timeCheckPreCond}\AgdaSpace{}%
\AgdaBound{time₁}\AgdaSpace{}%
\AgdaOperator{\AgdaFunction{∧sp}}\<%
\\
\>[28][@{}l@{\AgdaIndent{0}}]%
\>[29]\AgdaFunction{weakestPreCondMultiSig-2-4ˢ}%
\>[58]\AgdaBound{pbk1}\AgdaSpace{}%
\AgdaBound{pbk2}\AgdaSpace{}%
\AgdaBound{pbk3}\AgdaSpace{}%
\AgdaBound{pbk4}\AgdaSymbol{)}\AgdaSpace{}%
\AgdaOperator{\AgdaRecord{>ⁱᶠᶠ}}\<%
\\
\>[7][@{}l@{\AgdaIndent{0}}]%
\>[8]\AgdaFunction{checkTimeScriptᵇ}\AgdaSpace{}%
\AgdaBound{time₁}\AgdaSpace{}%
\AgdaOperator{\AgdaFunction{++}}\AgdaSpace{}%
\AgdaFunction{multiSigScript2-4ᵇ}\AgdaSpace{}%
\AgdaBound{pbk1}\AgdaSpace{}%
\AgdaBound{pbk2}\AgdaSpace{}%
\AgdaBound{pbk3}\AgdaSpace{}%
\AgdaBound{pbk4}\<%
\\
%
\>[8]\AgdaOperator{\AgdaRecord{<}}\AgdaSpace{}%
\AgdaFunction{acceptState}\AgdaSpace{}%
\AgdaOperator{\AgdaRecord{>}}\<%
\\
\>[0]\AgdaFunction{theoremCorrectnessCombinedMultiSigTimeCheck}\AgdaSpace{}%
\AgdaBound{time₁}\AgdaSpace{}%
\AgdaBound{pbk1}\AgdaSpace{}%
\AgdaBound{pbk2}\AgdaSpace{}%
\AgdaBound{pbk3}\AgdaSpace{}%
\AgdaBound{pbk4}\AgdaSpace{}%
\AgdaSymbol{=}\<%
\\
\>[0][@{}l@{\AgdaIndent{0}}]%
\>[2]\AgdaFunction{stackPred2SPred}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaFunction{timeCheckPreCond}\AgdaSpace{}%
\AgdaBound{time₁}\AgdaSpace{}%
\AgdaOperator{\AgdaFunction{∧sp}}\<%
\\
\>[2][@{}l@{\AgdaIndent{0}}]%
\>[5]\AgdaFunction{weakestPreCondMultiSig-2-4ˢ}%
\>[34]\AgdaBound{pbk1}\AgdaSpace{}%
\AgdaBound{pbk2}\AgdaSpace{}%
\AgdaBound{pbk3}\AgdaSpace{}%
\AgdaBound{pbk4}\AgdaSymbol{)}\<%
\\
\>[5][@{}l@{\AgdaIndent{0}}]%
\>[11]\AgdaFunction{<><>⟨}%
\>[18]\AgdaFunction{checkTimeScriptᵇ}\AgdaSpace{}%
\AgdaBound{time₁}%
\>[42]\AgdaFunction{⟩⟨}%
\>[46]\AgdaFunction{theoremCorrectnessTimeCheck}\<%
\\
%
\>[18]\AgdaSymbol{(}\AgdaFunction{weakestPreCondMultiSig-2-4ˢ}\AgdaSpace{}%
\AgdaBound{pbk1}\AgdaSpace{}%
\AgdaBound{pbk2}\AgdaSpace{}%
\AgdaBound{pbk3}\AgdaSpace{}%
\AgdaBound{pbk4}\AgdaSymbol{)}\AgdaSpace{}%
\AgdaBound{time₁}%
\>[75]\AgdaFunction{⟩}\<%
\\
%
\>[2]\AgdaFunction{stackPred2SPred}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaFunction{weakestPreCondMultiSig-2-4ˢ}\AgdaSpace{}%
\AgdaBound{pbk1}\AgdaSpace{}%
\AgdaBound{pbk2}\AgdaSpace{}%
\AgdaBound{pbk3}\AgdaSpace{}%
\AgdaBound{pbk4}\AgdaSymbol{)}\<%
\\
\>[2][@{}l@{\AgdaIndent{0}}]%
\>[11]\AgdaFunction{<><>⟨}%
\>[667I]\AgdaFunction{multiSigScript2-4ᵇ}\AgdaSpace{}%
\AgdaBound{pbk1}\AgdaSpace{}%
\AgdaBound{pbk2}\AgdaSpace{}%
\AgdaBound{pbk3}\AgdaSpace{}%
\AgdaBound{pbk4}\<%
\\
\>[.][@{}l@{}]\<[667I]%
\>[17]\AgdaFunction{⟩⟨}\AgdaSpace{}%
\AgdaFunction{theoremCorrectnessMultiSig-2-4}\AgdaSpace{}%
\AgdaBound{pbk1}\AgdaSpace{}%
\AgdaBound{pbk2}\AgdaSpace{}%
\AgdaBound{pbk3}\AgdaSpace{}%
\AgdaBound{pbk4}%
\>[73]\AgdaFunction{⟩ᵉ}\<%
\\
%
\>[2]\AgdaFunction{stackPred2SPred}\AgdaSpace{}%
\AgdaFunction{acceptStateˢ}\AgdaSpace{}%
\AgdaOperator{\AgdaFunction{∎p}}\<%
\end{code}
} % END newcommand

\AgdaHide{
\begin{code}%
\>[0]\<%
\end{code}
} % END AgdaHide


==> latex-before-sed/verificationWithIfStack/hoareTripleStackScript.tex <==
%% This file has been generated automatically by mkLagda.awk
%% DO NOT EDIT! ALL YOUR CHANGES WILL BE LOST!

\AgdaHide{
\begin{code}%
\>[0]\AgdaKeyword{open}\AgdaSpace{}%
\AgdaKeyword{import}\AgdaSpace{}%
\AgdaModule{basicBitcoinDataType}\<%
\\
%
\\[\AgdaEmptyExtraSkip]%
\>[0]\AgdaKeyword{module}\AgdaSpace{}%
\AgdaModule{verificationWithIfStack.hoareTripleStackScript}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaBound{param}\AgdaSpace{}%
\AgdaSymbol{:}\AgdaSpace{}%
\AgdaRecord{GlobalParameters}\AgdaSymbol{)}\AgdaSpace{}%
\AgdaKeyword{where}\<%
\\
%
\\[\AgdaEmptyExtraSkip]%
%
\\[\AgdaEmptyExtraSkip]%
\>[0]\AgdaKeyword{open}\AgdaSpace{}%
\AgdaKeyword{import}\AgdaSpace{}%
\AgdaModule{Data.List.Base}\AgdaSpace{}%
\AgdaKeyword{hiding}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaOperator{\AgdaFunction{\AgdaUnderscore{}++\AgdaUnderscore{}}}\AgdaSymbol{)}\<%
\\
\>[0]\AgdaKeyword{open}\AgdaSpace{}%
\AgdaKeyword{import}\AgdaSpace{}%
\AgdaModule{Data.Nat}%
\>[22]\AgdaKeyword{renaming}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaOperator{\AgdaDatatype{\AgdaUnderscore{}≤\AgdaUnderscore{}}}\AgdaSpace{}%
\AgdaSymbol{to}\AgdaSpace{}%
\AgdaOperator{\AgdaDatatype{\AgdaUnderscore{}≤'\AgdaUnderscore{}}}\AgdaSpace{}%
\AgdaSymbol{;}\AgdaSpace{}%
\AgdaOperator{\AgdaFunction{\AgdaUnderscore{}<\AgdaUnderscore{}}}\AgdaSpace{}%
\AgdaSymbol{to}\AgdaSpace{}%
\AgdaOperator{\AgdaFunction{\AgdaUnderscore{}<'\AgdaUnderscore{}}}\AgdaSymbol{)}\<%
\\
\>[0]\AgdaKeyword{open}\AgdaSpace{}%
\AgdaKeyword{import}\AgdaSpace{}%
\AgdaModule{Data.List}\AgdaSpace{}%
\AgdaKeyword{hiding}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaOperator{\AgdaFunction{\AgdaUnderscore{}++\AgdaUnderscore{}}}\AgdaSymbol{)}\<%
\\
\>[0]\AgdaKeyword{open}\AgdaSpace{}%
\AgdaKeyword{import}\AgdaSpace{}%
\AgdaModule{Data.Sum}\<%
\\
\>[0]\AgdaKeyword{open}\AgdaSpace{}%
\AgdaKeyword{import}\AgdaSpace{}%
\AgdaModule{Data.Unit}%
\>[23]\AgdaKeyword{hiding}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaOperator{\AgdaRecord{\AgdaUnderscore{}≤\AgdaUnderscore{}}}\AgdaSymbol{)}\<%
\\
\>[0]\AgdaKeyword{open}\AgdaSpace{}%
\AgdaKeyword{import}\AgdaSpace{}%
\AgdaModule{Data.Empty}\<%
\\
\>[0]\AgdaKeyword{open}\AgdaSpace{}%
\AgdaKeyword{import}\AgdaSpace{}%
\AgdaModule{Data.Maybe}\<%
\\
\>[0]\AgdaKeyword{open}\AgdaSpace{}%
\AgdaKeyword{import}\AgdaSpace{}%
\AgdaModule{Data.Bool}%
\>[23]\AgdaKeyword{hiding}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaOperator{\AgdaDatatype{\AgdaUnderscore{}≤\AgdaUnderscore{}}}\AgdaSpace{}%
\AgdaSymbol{;}\AgdaSpace{}%
\AgdaOperator{\AgdaDatatype{\AgdaUnderscore{}<\AgdaUnderscore{}}}\AgdaSpace{}%
\AgdaSymbol{;}\AgdaSpace{}%
\AgdaOperator{\AgdaFunction{if\AgdaUnderscore{}then\AgdaUnderscore{}else\AgdaUnderscore{}}}%
\>[58]\AgdaSymbol{)}%
\>[61]\AgdaKeyword{renaming}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaOperator{\AgdaFunction{\AgdaUnderscore{}∧\AgdaUnderscore{}}}\AgdaSpace{}%
\AgdaSymbol{to}\AgdaSpace{}%
\AgdaOperator{\AgdaFunction{\AgdaUnderscore{}∧b\AgdaUnderscore{}}}\AgdaSpace{}%
\AgdaSymbol{;}\AgdaSpace{}%
\AgdaOperator{\AgdaFunction{\AgdaUnderscore{}∨\AgdaUnderscore{}}}\AgdaSpace{}%
\AgdaSymbol{to}\AgdaSpace{}%
\AgdaOperator{\AgdaFunction{\AgdaUnderscore{}∨b\AgdaUnderscore{}}}\AgdaSpace{}%
\AgdaSymbol{;}\AgdaSpace{}%
\AgdaFunction{T}\AgdaSpace{}%
\AgdaSymbol{to}\AgdaSpace{}%
\AgdaFunction{True}\AgdaSymbol{)}\<%
\\
\>[0]\AgdaKeyword{open}\AgdaSpace{}%
\AgdaKeyword{import}\AgdaSpace{}%
\AgdaModule{Data.Product}\AgdaSpace{}%
\AgdaKeyword{renaming}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaOperator{\AgdaInductiveConstructor{\AgdaUnderscore{},\AgdaUnderscore{}}}\AgdaSpace{}%
\AgdaSymbol{to}\AgdaSpace{}%
\AgdaOperator{\AgdaInductiveConstructor{\AgdaUnderscore{},,\AgdaUnderscore{}}}\AgdaSpace{}%
\AgdaSymbol{)}\<%
\\
\>[0]\AgdaKeyword{open}\AgdaSpace{}%
\AgdaKeyword{import}\AgdaSpace{}%
\AgdaModule{Data.Nat.Base}\AgdaSpace{}%
\AgdaKeyword{hiding}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaOperator{\AgdaDatatype{\AgdaUnderscore{}≤\AgdaUnderscore{}}}\AgdaSpace{}%
\AgdaSymbol{;}\AgdaSpace{}%
\AgdaOperator{\AgdaFunction{\AgdaUnderscore{}<\AgdaUnderscore{}}}\AgdaSymbol{)}\<%
\\
\>[0]\AgdaKeyword{open}\AgdaSpace{}%
\AgdaKeyword{import}\AgdaSpace{}%
\AgdaModule{Data.List.NonEmpty}\AgdaSpace{}%
\AgdaKeyword{hiding}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaField{head}\AgdaSymbol{)}\<%
\\
\>[0]\AgdaKeyword{open}\AgdaSpace{}%
\AgdaKeyword{import}\AgdaSpace{}%
\AgdaModule{Data.Nat}\AgdaSpace{}%
\AgdaKeyword{using}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaDatatype{ℕ}\AgdaSymbol{;}\AgdaSpace{}%
\AgdaOperator{\AgdaPrimitive{\AgdaUnderscore{}+\AgdaUnderscore{}}}\AgdaSymbol{;}\AgdaSpace{}%
\AgdaOperator{\AgdaFunction{\AgdaUnderscore{}≥\AgdaUnderscore{}}}\AgdaSymbol{;}\AgdaSpace{}%
\AgdaOperator{\AgdaFunction{\AgdaUnderscore{}>\AgdaUnderscore{}}}\AgdaSymbol{;}\AgdaSpace{}%
\AgdaInductiveConstructor{zero}\AgdaSymbol{;}\AgdaSpace{}%
\AgdaInductiveConstructor{suc}\AgdaSymbol{;}\AgdaSpace{}%
\AgdaInductiveConstructor{s≤s}\AgdaSymbol{;}\AgdaSpace{}%
\AgdaInductiveConstructor{z≤n}\AgdaSymbol{)}\<%
\\
\>[0]\AgdaKeyword{import}\AgdaSpace{}%
\AgdaModule{Relation.Binary.PropositionalEquality}\AgdaSpace{}%
\AgdaSymbol{as}\AgdaSpace{}%
\AgdaModule{Eq}\<%
\\
\>[0]\AgdaKeyword{open}\AgdaSpace{}%
\AgdaModule{Eq}\AgdaSpace{}%
\AgdaKeyword{using}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaOperator{\AgdaDatatype{\AgdaUnderscore{}≡\AgdaUnderscore{}}}\AgdaSymbol{;}\AgdaSpace{}%
\AgdaInductiveConstructor{refl}\AgdaSymbol{;}\AgdaSpace{}%
\AgdaFunction{cong}\AgdaSymbol{;}\AgdaSpace{}%
\AgdaKeyword{module}\AgdaSpace{}%
\AgdaModule{≡-Reasoning}\AgdaSymbol{;}\AgdaSpace{}%
\AgdaFunction{sym}\AgdaSymbol{)}\<%
\\
\>[0]\AgdaKeyword{open}\AgdaSpace{}%
\AgdaModule{≡-Reasoning}\<%
\\
\>[0]\AgdaKeyword{open}\AgdaSpace{}%
\AgdaKeyword{import}\AgdaSpace{}%
\AgdaModule{Agda.Builtin.Equality}\<%
\\
\>[0]\AgdaComment{--open\ import\ Agda.Builtin.Equality.Rewrite}\<%
\\
%
\\[\AgdaEmptyExtraSkip]%
\>[0]\AgdaKeyword{open}\AgdaSpace{}%
\AgdaKeyword{import}\AgdaSpace{}%
\AgdaModule{libraries.listLib}\<%
\\
\>[0]\AgdaKeyword{open}\AgdaSpace{}%
\AgdaKeyword{import}\AgdaSpace{}%
\AgdaModule{libraries.emptyLib}\<%
\\
\>[0]\AgdaKeyword{open}\AgdaSpace{}%
\AgdaKeyword{import}\AgdaSpace{}%
\AgdaModule{libraries.natLib}\<%
\\
\>[0]\AgdaKeyword{open}\AgdaSpace{}%
\AgdaKeyword{import}\AgdaSpace{}%
\AgdaModule{libraries.boolLib}\<%
\\
\>[0]\AgdaKeyword{open}\AgdaSpace{}%
\AgdaKeyword{import}\AgdaSpace{}%
\AgdaModule{libraries.equalityLib}\<%
\\
\>[0]\AgdaKeyword{open}\AgdaSpace{}%
\AgdaKeyword{import}\AgdaSpace{}%
\AgdaModule{libraries.andLib}\<%
\\
\>[0]\AgdaKeyword{open}\AgdaSpace{}%
\AgdaKeyword{import}\AgdaSpace{}%
\AgdaModule{libraries.miscLib}\<%
\\
\>[0]\AgdaKeyword{open}\AgdaSpace{}%
\AgdaKeyword{import}\AgdaSpace{}%
\AgdaModule{libraries.maybeLib}\<%
\\
%
\\[\AgdaEmptyExtraSkip]%
\>[0]\AgdaKeyword{open}\AgdaSpace{}%
\AgdaKeyword{import}\AgdaSpace{}%
\AgdaModule{stack}\<%
\\
\>[0]\AgdaKeyword{open}\AgdaSpace{}%
\AgdaKeyword{import}\AgdaSpace{}%
\AgdaModule{stackPredicate}\<%
\\
\>[0]\AgdaKeyword{open}\AgdaSpace{}%
\AgdaKeyword{import}\AgdaSpace{}%
\AgdaModule{instruction}\<%
\\
\>[0]\AgdaComment{--\ open\ import\ ledger\ param}\<%
\\
\>[0]\AgdaKeyword{open}\AgdaSpace{}%
\AgdaKeyword{import}\AgdaSpace{}%
\AgdaModule{stackSemanticsInstructions}\AgdaSpace{}%
\AgdaBound{param}\<%
\\
\>[0]\AgdaKeyword{open}\AgdaSpace{}%
\AgdaKeyword{import}\AgdaSpace{}%
\AgdaModule{hoareTripleStack}\AgdaSpace{}%
\AgdaBound{param}\<%
\\
%
\\[\AgdaEmptyExtraSkip]%
\>[0]\AgdaKeyword{open}\AgdaSpace{}%
\AgdaKeyword{import}\AgdaSpace{}%
\AgdaModule{verificationWithIfStack.ifStack}\<%
\\
\>[0]\AgdaKeyword{open}\AgdaSpace{}%
\AgdaKeyword{import}\AgdaSpace{}%
\AgdaModule{verificationWithIfStack.state}\<%
\\
\>[0]\AgdaKeyword{open}\AgdaSpace{}%
\AgdaKeyword{import}\AgdaSpace{}%
\AgdaModule{verificationWithIfStack.predicate}\<%
\\
\>[0]\AgdaKeyword{open}\AgdaSpace{}%
\AgdaKeyword{import}\AgdaSpace{}%
\AgdaModule{verificationWithIfStack.semanticsInstructions}\AgdaSpace{}%
\AgdaBound{param}\<%
\\
\>[0]\AgdaKeyword{open}\AgdaSpace{}%
\AgdaKeyword{import}\AgdaSpace{}%
\AgdaModule{verificationWithIfStack.stackSemanticsInstructionsLemma}\AgdaSpace{}%
\AgdaBound{param}\<%
\\
\>[0]\AgdaKeyword{open}\AgdaSpace{}%
\AgdaKeyword{import}\AgdaSpace{}%
\AgdaModule{verificationWithIfStack.verificationLemmas}\AgdaSpace{}%
\AgdaBound{param}\<%
\\
\>[0]\AgdaKeyword{open}\AgdaSpace{}%
\AgdaKeyword{import}\AgdaSpace{}%
\AgdaModule{verificationWithIfStack.hoareTriple}\AgdaSpace{}%
\AgdaBound{param}\<%
\\
\>[0]\AgdaKeyword{open}\AgdaSpace{}%
\AgdaKeyword{import}\AgdaSpace{}%
\AgdaModule{verificationWithIfStack.hoareTripleStack2HoareTriple}\AgdaSpace{}%
\AgdaBound{param}\<%
\\
%
\\[\AgdaEmptyExtraSkip]%
\>[0]\AgdaComment{--\ open\ import\ verificationWithIfStack.verificationP2PKH}\<%
\\
\>[0]\AgdaComment{--\ open\ import\ verificationWithIfStack.ifThenElseTheoremPart1\ param}\<%
\\
\>[0]\AgdaComment{--\ open\ import\ verificationWithIfStack.ifThenElseTheoremPart2\ param}\<%
\\
\>[0]\AgdaComment{--\ open\ import\ verificationWithIfStack.ifThenElseTheoremPart3\ param}\<%
\\
\>[0]\AgdaComment{--\ open\ import\ verificationWithIfStack.ifThenElseTheoremPart4\ param}\<%
\\
%
\\[\AgdaEmptyExtraSkip]%
\>[0]\AgdaKeyword{open}\AgdaSpace{}%
\AgdaKeyword{import}\AgdaSpace{}%
\AgdaModule{verificationWithIfStack.hoareTripleStackNonActiveIfStack}\AgdaSpace{}%
\AgdaBound{param}\<%
\\
%
\\[\AgdaEmptyExtraSkip]%
%
\\[\AgdaEmptyExtraSkip]%
%
\\[\AgdaEmptyExtraSkip]%
%
\\[\AgdaEmptyExtraSkip]%
%
\\[\AgdaEmptyExtraSkip]%
\>[0]\AgdaFunction{lemmaStackSemIsSemScriptaux2}%
\>[145I]\AgdaSymbol{:}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaBound{g'}\AgdaSpace{}%
\AgdaSymbol{:}\AgdaSpace{}%
\AgdaFunction{Time}\AgdaSpace{}%
\AgdaSymbol{→}\AgdaSpace{}%
\AgdaDatatype{Msg}\AgdaSpace{}%
\AgdaSymbol{→}\AgdaSpace{}%
\AgdaFunction{Stack}\AgdaSpace{}%
\AgdaSymbol{→}\AgdaSpace{}%
\AgdaDatatype{Maybe}\AgdaSpace{}%
\AgdaFunction{Stack}\AgdaSymbol{)}\<%
\\
\>[.][@{}l@{}]\<[145I]%
\>[29]\AgdaSymbol{(}\AgdaBound{st}\AgdaSpace{}%
\AgdaSymbol{:}\AgdaSpace{}%
\AgdaRecord{State}\AgdaSymbol{)}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaBound{mst}\AgdaSpace{}%
\AgdaSymbol{:}\AgdaSpace{}%
\AgdaDatatype{Maybe}\AgdaSpace{}%
\AgdaFunction{Stack}\AgdaSymbol{)}\<%
\\
\>[0][@{}l@{\AgdaIndent{0}}]%
\>[3]\AgdaSymbol{→}%
\>[162I]\AgdaSymbol{(}\AgdaFunction{exeTransformerDepIfStack'}%
\>[33]\AgdaSymbol{(}\AgdaFunction{liftStackToStateTransformerAux'}\AgdaSpace{}%
\AgdaBound{mst}\AgdaSpace{}%
\AgdaSymbol{)}%
\>[73]\AgdaBound{st}\<%
\\
\>[162I][@{}l@{\AgdaIndent{0}}]%
\>[7]\AgdaOperator{\AgdaFunction{>>=}}\AgdaSpace{}%
\AgdaSymbol{λ}\AgdaSpace{}%
\AgdaBound{s}\AgdaSpace{}%
\AgdaSymbol{→}%
\>[18]\AgdaFunction{exeTransformerDepIfStack'}\<%
\\
\>[18][@{}l@{\AgdaIndent{0}}]%
\>[20]\AgdaSymbol{(}\AgdaFunction{liftStackToStateTransformerAux'}\<%
\\
%
\>[20]\AgdaSymbol{(}\AgdaBound{g'}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaBound{s}\AgdaSpace{}%
\AgdaSymbol{.}\AgdaField{currentTime}\AgdaSymbol{)}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaBound{s}\AgdaSpace{}%
\AgdaSymbol{.}\AgdaField{msg}\AgdaSymbol{)}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaBound{s}\AgdaSpace{}%
\AgdaSymbol{.}\AgdaField{stack}\AgdaSymbol{)))}\AgdaSpace{}%
\AgdaBound{s}\AgdaSymbol{)}\<%
\\
%
\\[\AgdaEmptyExtraSkip]%
\>[162I][@{}l@{\AgdaIndent{0}}]%
\>[6]\AgdaOperator{\AgdaDatatype{≡}}\<%
\\
%
\>[6]\AgdaFunction{exeTransformerDepIfStack'}%
\>[33]\AgdaSymbol{(}\AgdaFunction{liftStackToStateTransformerAux'}\<%
\\
\>[6][@{}l@{\AgdaIndent{0}}]%
\>[13]\AgdaSymbol{(}\AgdaBound{mst}\AgdaSpace{}%
\AgdaOperator{\AgdaFunction{>>=}}\AgdaSpace{}%
\AgdaBound{g'}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaBound{st}\AgdaSpace{}%
\AgdaSymbol{.}\AgdaField{currentTime}\AgdaSymbol{)}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaBound{st}\AgdaSpace{}%
\AgdaSymbol{.}\AgdaField{msg}\AgdaSymbol{))}%
\>[55]\AgdaSymbol{)}\AgdaSpace{}%
\AgdaBound{st}\<%
\\
\>[0]\AgdaFunction{lemmaStackSemIsSemScriptaux2}\AgdaSpace{}%
\AgdaBound{g'}\AgdaSpace{}%
\AgdaOperator{\AgdaInductiveConstructor{⟨}}\AgdaSpace{}%
\AgdaBound{currentTime₁}\AgdaSpace{}%
\AgdaOperator{\AgdaInductiveConstructor{,}}\AgdaSpace{}%
\AgdaBound{msg₁}\AgdaSpace{}%
\AgdaOperator{\AgdaInductiveConstructor{,}}\AgdaSpace{}%
\AgdaBound{stack₁}\AgdaSpace{}%
\AgdaOperator{\AgdaInductiveConstructor{,}}\AgdaSpace{}%
\AgdaInductiveConstructor{[]}\AgdaSpace{}%
\AgdaOperator{\AgdaInductiveConstructor{,}}\AgdaSpace{}%
\AgdaBound{consis₁}\AgdaSpace{}%
\AgdaOperator{\AgdaInductiveConstructor{⟩}}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaInductiveConstructor{just}\AgdaSpace{}%
\AgdaBound{x}\AgdaSymbol{)}\AgdaSpace{}%
\AgdaSymbol{=}\AgdaSpace{}%
\AgdaInductiveConstructor{refl}\<%
\\
\>[0]\AgdaFunction{lemmaStackSemIsSemScriptaux2}\AgdaSpace{}%
\AgdaBound{g'}\AgdaSpace{}%
\AgdaOperator{\AgdaInductiveConstructor{⟨}}\AgdaSpace{}%
\AgdaBound{currentTime₁}\AgdaSpace{}%
\AgdaOperator{\AgdaInductiveConstructor{,}}\AgdaSpace{}%
\AgdaBound{msg₁}\AgdaSpace{}%
\AgdaOperator{\AgdaInductiveConstructor{,}}\AgdaSpace{}%
\AgdaBound{stack₁}\AgdaSpace{}%
\AgdaOperator{\AgdaInductiveConstructor{,}}\AgdaSpace{}%
\AgdaInductiveConstructor{ifCase}\AgdaSpace{}%
\AgdaOperator{\AgdaInductiveConstructor{∷}}\AgdaSpace{}%
\AgdaBound{ifStack₁}\AgdaSpace{}%
\AgdaOperator{\AgdaInductiveConstructor{,}}\AgdaSpace{}%
\AgdaBound{consis₁}\AgdaSpace{}%
\AgdaOperator{\AgdaInductiveConstructor{⟩}}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaInductiveConstructor{just}\AgdaSpace{}%
\AgdaBound{x}\AgdaSymbol{)}\AgdaSpace{}%
\AgdaSymbol{=}\AgdaSpace{}%
\AgdaInductiveConstructor{refl}\<%
\\
\>[0]\AgdaFunction{lemmaStackSemIsSemScriptaux2}\AgdaSpace{}%
\AgdaBound{g'}\AgdaSpace{}%
\AgdaOperator{\AgdaInductiveConstructor{⟨}}\AgdaSpace{}%
\AgdaBound{currentTime₁}\AgdaSpace{}%
\AgdaOperator{\AgdaInductiveConstructor{,}}\AgdaSpace{}%
\AgdaBound{msg₁}\AgdaSpace{}%
\AgdaOperator{\AgdaInductiveConstructor{,}}\AgdaSpace{}%
\AgdaBound{stack₁}\AgdaSpace{}%
\AgdaOperator{\AgdaInductiveConstructor{,}}\AgdaSpace{}%
\AgdaInductiveConstructor{elseCase}\AgdaSpace{}%
\AgdaOperator{\AgdaInductiveConstructor{∷}}\AgdaSpace{}%
\AgdaBound{ifStack₁}\AgdaSpace{}%
\AgdaOperator{\AgdaInductiveConstructor{,}}\AgdaSpace{}%
\AgdaBound{consis₁}\AgdaSpace{}%
\AgdaOperator{\AgdaInductiveConstructor{⟩}}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaInductiveConstructor{just}\AgdaSpace{}%
\AgdaBound{x}\AgdaSymbol{)}\AgdaSpace{}%
\AgdaSymbol{=}\AgdaSpace{}%
\AgdaInductiveConstructor{refl}\<%
\\
\>[0]\AgdaFunction{lemmaStackSemIsSemScriptaux2}\AgdaSpace{}%
\AgdaBound{g'}\AgdaSpace{}%
\AgdaOperator{\AgdaInductiveConstructor{⟨}}\AgdaSpace{}%
\AgdaBound{currentTime₁}\AgdaSpace{}%
\AgdaOperator{\AgdaInductiveConstructor{,}}\AgdaSpace{}%
\AgdaBound{msg₁}\AgdaSpace{}%
\AgdaOperator{\AgdaInductiveConstructor{,}}\AgdaSpace{}%
\AgdaBound{stack₁}\AgdaSpace{}%
\AgdaOperator{\AgdaInductiveConstructor{,}}\AgdaSpace{}%
\AgdaInductiveConstructor{ifSkip}\AgdaSpace{}%
\AgdaOperator{\AgdaInductiveConstructor{∷}}\AgdaSpace{}%
\AgdaBound{ifStack₁}\AgdaSpace{}%
\AgdaOperator{\AgdaInductiveConstructor{,}}\AgdaSpace{}%
\AgdaBound{consis₁}\AgdaSpace{}%
\AgdaOperator{\AgdaInductiveConstructor{⟩}}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaInductiveConstructor{just}\AgdaSpace{}%
\AgdaBound{x}\AgdaSymbol{)}\AgdaSpace{}%
\AgdaSymbol{=}\AgdaSpace{}%
\AgdaInductiveConstructor{refl}\<%
\\
\>[0]\AgdaFunction{lemmaStackSemIsSemScriptaux2}\AgdaSpace{}%
\AgdaBound{g'}\AgdaSpace{}%
\AgdaOperator{\AgdaInductiveConstructor{⟨}}\AgdaSpace{}%
\AgdaBound{currentTime₁}\AgdaSpace{}%
\AgdaOperator{\AgdaInductiveConstructor{,}}\AgdaSpace{}%
\AgdaBound{msg₁}\AgdaSpace{}%
\AgdaOperator{\AgdaInductiveConstructor{,}}\AgdaSpace{}%
\AgdaBound{stack₁}\AgdaSpace{}%
\AgdaOperator{\AgdaInductiveConstructor{,}}\AgdaSpace{}%
\AgdaInductiveConstructor{elseSkip}\AgdaSpace{}%
\AgdaOperator{\AgdaInductiveConstructor{∷}}\AgdaSpace{}%
\AgdaBound{ifStack₁}\AgdaSpace{}%
\AgdaOperator{\AgdaInductiveConstructor{,}}\AgdaSpace{}%
\AgdaBound{consis₁}\AgdaSpace{}%
\AgdaOperator{\AgdaInductiveConstructor{⟩}}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaInductiveConstructor{just}\AgdaSpace{}%
\AgdaBound{x}\AgdaSymbol{)}\AgdaSpace{}%
\AgdaSymbol{=}\AgdaSpace{}%
\AgdaInductiveConstructor{refl}\<%
\\
\>[0]\AgdaFunction{lemmaStackSemIsSemScriptaux2}\AgdaSpace{}%
\AgdaBound{g'}\AgdaSpace{}%
\AgdaOperator{\AgdaInductiveConstructor{⟨}}\AgdaSpace{}%
\AgdaBound{currentTime₁}\AgdaSpace{}%
\AgdaOperator{\AgdaInductiveConstructor{,}}\AgdaSpace{}%
\AgdaBound{msg₁}\AgdaSpace{}%
\AgdaOperator{\AgdaInductiveConstructor{,}}\AgdaSpace{}%
\AgdaBound{stack₁}\AgdaSpace{}%
\AgdaOperator{\AgdaInductiveConstructor{,}}\AgdaSpace{}%
\AgdaInductiveConstructor{ifIgnore}\AgdaSpace{}%
\AgdaOperator{\AgdaInductiveConstructor{∷}}\AgdaSpace{}%
\AgdaBound{ifStack₁}\AgdaSpace{}%
\AgdaOperator{\AgdaInductiveConstructor{,}}\AgdaSpace{}%
\AgdaBound{consis₁}\AgdaSpace{}%
\AgdaOperator{\AgdaInductiveConstructor{⟩}}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaInductiveConstructor{just}\AgdaSpace{}%
\AgdaBound{x}\AgdaSymbol{)}\AgdaSpace{}%
\AgdaSymbol{=}\AgdaSpace{}%
\AgdaInductiveConstructor{refl}\<%
\\
\>[0]\AgdaFunction{lemmaStackSemIsSemScriptaux2}\AgdaSpace{}%
\AgdaBound{g'}\AgdaSpace{}%
\AgdaOperator{\AgdaInductiveConstructor{⟨}}\AgdaSpace{}%
\AgdaBound{currentTime₁}\AgdaSpace{}%
\AgdaOperator{\AgdaInductiveConstructor{,}}\AgdaSpace{}%
\AgdaBound{msg₁}\AgdaSpace{}%
\AgdaOperator{\AgdaInductiveConstructor{,}}\AgdaSpace{}%
\AgdaBound{stack₁}\AgdaSpace{}%
\AgdaOperator{\AgdaInductiveConstructor{,}}\AgdaSpace{}%
\AgdaInductiveConstructor{[]}\AgdaSpace{}%
\AgdaOperator{\AgdaInductiveConstructor{,}}\AgdaSpace{}%
\AgdaBound{consis₁}\AgdaSpace{}%
\AgdaOperator{\AgdaInductiveConstructor{⟩}}\AgdaSpace{}%
\AgdaInductiveConstructor{nothing}\AgdaSpace{}%
\AgdaSymbol{=}\AgdaSpace{}%
\AgdaInductiveConstructor{refl}\<%
\\
\>[0]\AgdaFunction{lemmaStackSemIsSemScriptaux2}\AgdaSpace{}%
\AgdaBound{g'}\AgdaSpace{}%
\AgdaOperator{\AgdaInductiveConstructor{⟨}}\AgdaSpace{}%
\AgdaBound{currentTime₁}\AgdaSpace{}%
\AgdaOperator{\AgdaInductiveConstructor{,}}\AgdaSpace{}%
\AgdaBound{msg₁}\AgdaSpace{}%
\AgdaOperator{\AgdaInductiveConstructor{,}}\AgdaSpace{}%
\AgdaBound{stack₁}\AgdaSpace{}%
\AgdaOperator{\AgdaInductiveConstructor{,}}\AgdaSpace{}%
\AgdaInductiveConstructor{ifCase}\AgdaSpace{}%
\AgdaOperator{\AgdaInductiveConstructor{∷}}\AgdaSpace{}%
\AgdaBound{ifStack₁}\AgdaSpace{}%
\AgdaOperator{\AgdaInductiveConstructor{,}}\AgdaSpace{}%
\AgdaBound{consis₁}\AgdaSpace{}%
\AgdaOperator{\AgdaInductiveConstructor{⟩}}\AgdaSpace{}%
\AgdaInductiveConstructor{nothing}\AgdaSpace{}%
\AgdaSymbol{=}\AgdaSpace{}%
\AgdaInductiveConstructor{refl}\<%
\\
\>[0]\AgdaFunction{lemmaStackSemIsSemScriptaux2}\AgdaSpace{}%
\AgdaBound{g'}\AgdaSpace{}%
\AgdaOperator{\AgdaInductiveConstructor{⟨}}\AgdaSpace{}%
\AgdaBound{currentTime₁}\AgdaSpace{}%
\AgdaOperator{\AgdaInductiveConstructor{,}}\AgdaSpace{}%
\AgdaBound{msg₁}\AgdaSpace{}%
\AgdaOperator{\AgdaInductiveConstructor{,}}\AgdaSpace{}%
\AgdaBound{stack₁}\AgdaSpace{}%
\AgdaOperator{\AgdaInductiveConstructor{,}}\AgdaSpace{}%
\AgdaInductiveConstructor{elseCase}\AgdaSpace{}%
\AgdaOperator{\AgdaInductiveConstructor{∷}}\AgdaSpace{}%
\AgdaBound{ifStack₁}\AgdaSpace{}%
\AgdaOperator{\AgdaInductiveConstructor{,}}\AgdaSpace{}%
\AgdaBound{consis₁}\AgdaSpace{}%
\AgdaOperator{\AgdaInductiveConstructor{⟩}}\AgdaSpace{}%
\AgdaInductiveConstructor{nothing}\AgdaSpace{}%
\AgdaSymbol{=}\AgdaSpace{}%
\AgdaInductiveConstructor{refl}\<%
\\
\>[0]\AgdaFunction{lemmaStackSemIsSemScriptaux2}\AgdaSpace{}%
\AgdaBound{g'}\AgdaSpace{}%
\AgdaOperator{\AgdaInductiveConstructor{⟨}}\AgdaSpace{}%
\AgdaBound{currentTime₁}\AgdaSpace{}%
\AgdaOperator{\AgdaInductiveConstructor{,}}\AgdaSpace{}%
\AgdaBound{msg₁}\AgdaSpace{}%
\AgdaOperator{\AgdaInductiveConstructor{,}}\AgdaSpace{}%
\AgdaBound{stack₁}\AgdaSpace{}%
\AgdaOperator{\AgdaInductiveConstructor{,}}\AgdaSpace{}%
\AgdaInductiveConstructor{ifSkip}\AgdaSpace{}%
\AgdaOperator{\AgdaInductiveConstructor{∷}}\AgdaSpace{}%
\AgdaBound{ifStack₁}\AgdaSpace{}%
\AgdaOperator{\AgdaInductiveConstructor{,}}\AgdaSpace{}%
\AgdaBound{consis₁}\AgdaSpace{}%
\AgdaOperator{\AgdaInductiveConstructor{⟩}}\AgdaSpace{}%
\AgdaInductiveConstructor{nothing}\AgdaSpace{}%
\AgdaSymbol{=}\AgdaSpace{}%
\AgdaInductiveConstructor{refl}\<%
\\
\>[0]\AgdaFunction{lemmaStackSemIsSemScriptaux2}\AgdaSpace{}%
\AgdaBound{g'}\AgdaSpace{}%
\AgdaOperator{\AgdaInductiveConstructor{⟨}}\AgdaSpace{}%
\AgdaBound{currentTime₁}\AgdaSpace{}%
\AgdaOperator{\AgdaInductiveConstructor{,}}\AgdaSpace{}%
\AgdaBound{msg₁}\AgdaSpace{}%
\AgdaOperator{\AgdaInductiveConstructor{,}}\AgdaSpace{}%
\AgdaBound{stack₁}\AgdaSpace{}%
\AgdaOperator{\AgdaInductiveConstructor{,}}\AgdaSpace{}%
\AgdaInductiveConstructor{elseSkip}\AgdaSpace{}%
\AgdaOperator{\AgdaInductiveConstructor{∷}}\AgdaSpace{}%
\AgdaBound{ifStack₁}\AgdaSpace{}%
\AgdaOperator{\AgdaInductiveConstructor{,}}\AgdaSpace{}%
\AgdaBound{consis₁}\AgdaSpace{}%
\AgdaOperator{\AgdaInductiveConstructor{⟩}}\AgdaSpace{}%
\AgdaInductiveConstructor{nothing}\AgdaSpace{}%
\AgdaSymbol{=}\AgdaSpace{}%
\AgdaInductiveConstructor{refl}\<%
\\
\>[0]\AgdaFunction{lemmaStackSemIsSemScriptaux2}\AgdaSpace{}%
\AgdaBound{g'}\AgdaSpace{}%
\AgdaOperator{\AgdaInductiveConstructor{⟨}}\AgdaSpace{}%
\AgdaBound{currentTime₁}\AgdaSpace{}%
\AgdaOperator{\AgdaInductiveConstructor{,}}\AgdaSpace{}%
\AgdaBound{msg₁}\AgdaSpace{}%
\AgdaOperator{\AgdaInductiveConstructor{,}}\AgdaSpace{}%
\AgdaBound{stack₁}\AgdaSpace{}%
\AgdaOperator{\AgdaInductiveConstructor{,}}\AgdaSpace{}%
\AgdaInductiveConstructor{ifIgnore}\AgdaSpace{}%
\AgdaOperator{\AgdaInductiveConstructor{∷}}\AgdaSpace{}%
\AgdaBound{ifStack₁}\AgdaSpace{}%
\AgdaOperator{\AgdaInductiveConstructor{,}}\AgdaSpace{}%
\AgdaBound{consis₁}\AgdaSpace{}%
\AgdaOperator{\AgdaInductiveConstructor{⟩}}\AgdaSpace{}%
\AgdaInductiveConstructor{nothing}\AgdaSpace{}%
\AgdaSymbol{=}\AgdaSpace{}%
\AgdaInductiveConstructor{refl}\<%
\\
%
\\[\AgdaEmptyExtraSkip]%
%
\\[\AgdaEmptyExtraSkip]%
\>[0]\AgdaFunction{lemmaStackSemIsSemScriptaux}%
\>[388I]\AgdaSymbol{:}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaBound{f}\AgdaSpace{}%
\AgdaBound{g}\AgdaSpace{}%
\AgdaSymbol{:}\AgdaSpace{}%
\AgdaRecord{State}\AgdaSpace{}%
\AgdaSymbol{→}\AgdaSpace{}%
\AgdaDatatype{Maybe}\AgdaSpace{}%
\AgdaRecord{State}\AgdaSymbol{)}\<%
\\
\>[388I][@{}l@{\AgdaIndent{0}}]%
\>[29]\AgdaSymbol{(}\AgdaBound{f'}\AgdaSpace{}%
\AgdaBound{g'}\AgdaSpace{}%
\AgdaSymbol{:}\AgdaSpace{}%
\AgdaFunction{Time}\AgdaSpace{}%
\AgdaSymbol{→}\AgdaSpace{}%
\AgdaDatatype{Msg}\AgdaSpace{}%
\AgdaSymbol{→}\AgdaSpace{}%
\AgdaFunction{Stack}\AgdaSpace{}%
\AgdaSymbol{→}\AgdaSpace{}%
\AgdaDatatype{Maybe}\AgdaSpace{}%
\AgdaFunction{Stack}\AgdaSymbol{)}\<%
\\
%
\>[29]\AgdaSymbol{(}\AgdaBound{p}\AgdaSpace{}%
\AgdaSymbol{:}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaBound{s}\AgdaSpace{}%
\AgdaSymbol{:}\AgdaSpace{}%
\AgdaRecord{State}\AgdaSymbol{)}\AgdaSpace{}%
\AgdaSymbol{→}\AgdaSpace{}%
\AgdaBound{f}\AgdaSpace{}%
\AgdaBound{s}\AgdaSpace{}%
\AgdaOperator{\AgdaDatatype{≡}}\AgdaSpace{}%
\AgdaFunction{stackTransform2StateTransform}\AgdaSpace{}%
\AgdaBound{f'}\AgdaSpace{}%
\AgdaBound{s}\AgdaSymbol{)}\<%
\\
%
\>[29]\AgdaSymbol{(}\AgdaBound{q}\AgdaSpace{}%
\AgdaSymbol{:}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaBound{s}\AgdaSpace{}%
\AgdaSymbol{:}\AgdaSpace{}%
\AgdaRecord{State}\AgdaSymbol{)}\AgdaSpace{}%
\AgdaSymbol{→}\AgdaSpace{}%
\AgdaBound{g}\AgdaSpace{}%
\AgdaBound{s}\AgdaSpace{}%
\AgdaOperator{\AgdaDatatype{≡}}\AgdaSpace{}%
\AgdaFunction{stackTransform2StateTransform}\AgdaSpace{}%
\AgdaBound{g'}\AgdaSpace{}%
\AgdaBound{s}\AgdaSymbol{)}\<%
\\
%
\>[29]\AgdaSymbol{(}\AgdaBound{st}\AgdaSpace{}%
\AgdaSymbol{:}\AgdaSpace{}%
\AgdaRecord{State}\AgdaSymbol{)}\<%
\\
%
\>[29]\AgdaSymbol{→}\<%
\\
\>[0][@{}l@{\AgdaIndent{0}}]%
\>[14]\AgdaSymbol{(}\AgdaBound{f}\AgdaSpace{}%
\AgdaBound{st}\AgdaSpace{}%
\AgdaOperator{\AgdaFunction{>>=}}\AgdaSpace{}%
\AgdaBound{g}\AgdaSymbol{)}%
\>[29]\AgdaOperator{\AgdaDatatype{≡}}%
\>[433I]\AgdaFunction{stackTransform2StateTransform}\<%
\\
\>[433I][@{}l@{\AgdaIndent{0}}]%
\>[35]\AgdaSymbol{(λ}\AgdaSpace{}%
\AgdaBound{time₁}\AgdaSpace{}%
\AgdaBound{msg}\AgdaSpace{}%
\AgdaBound{stack₁}\AgdaSpace{}%
\AgdaSymbol{→}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaBound{f'}\AgdaSpace{}%
\AgdaBound{time₁}\AgdaSpace{}%
\AgdaBound{msg}\AgdaSpace{}%
\AgdaBound{stack₁}\AgdaSpace{}%
\AgdaOperator{\AgdaFunction{>>=}}\AgdaSpace{}%
\AgdaBound{g'}\AgdaSpace{}%
\AgdaBound{time₁}\AgdaSpace{}%
\AgdaBound{msg}\AgdaSymbol{)}\AgdaSpace{}%
\AgdaSymbol{)}\<%
\\
%
\>[35]\AgdaBound{st}\<%
\\
\>[0]\AgdaFunction{lemmaStackSemIsSemScriptaux}\AgdaSpace{}%
\AgdaBound{f}\AgdaSpace{}%
\AgdaBound{g}\AgdaSpace{}%
\AgdaBound{f'}\AgdaSpace{}%
\AgdaBound{g'}\AgdaSpace{}%
\AgdaBound{p}\AgdaSpace{}%
\AgdaBound{q}\AgdaSpace{}%
\AgdaBound{st}\AgdaSpace{}%
\AgdaSymbol{=}\<%
\\
\>[0][@{}l@{\AgdaIndent{0}}]%
\>[4]\AgdaSymbol{(}\AgdaBound{f}%
\>[455I]\AgdaBound{st}\AgdaSpace{}%
\AgdaOperator{\AgdaFunction{>>=}}\AgdaSpace{}%
\AgdaBound{g}\AgdaSymbol{)}\<%
\\
\>[.][@{}l@{}]\<[455I]%
\>[7]\AgdaFunction{≡⟨}\AgdaSpace{}%
\AgdaFunction{cong}\AgdaSpace{}%
\AgdaSymbol{(λ}\AgdaSpace{}%
\AgdaBound{x}\AgdaSpace{}%
\AgdaSymbol{→}\AgdaSpace{}%
\AgdaBound{x}\AgdaSpace{}%
\AgdaOperator{\AgdaFunction{>>=}}\AgdaSpace{}%
\AgdaBound{g}\AgdaSymbol{)}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaBound{p}\AgdaSpace{}%
\AgdaBound{st}\AgdaSymbol{)}%
\>[39]\AgdaFunction{⟩}\<%
\\
%
\>[4]\AgdaSymbol{(}\AgdaFunction{stackTransform2StateTransform}\AgdaSpace{}%
\AgdaBound{f'}\AgdaSpace{}%
\AgdaBound{st}\AgdaSpace{}%
\AgdaOperator{\AgdaFunction{>>=}}\AgdaSpace{}%
\AgdaBound{g}\AgdaSpace{}%
\AgdaSymbol{)}\<%
\\
\>[4][@{}l@{\AgdaIndent{0}}]%
\>[7]\AgdaFunction{≡⟨}\AgdaSpace{}%
\AgdaFunction{lemmaEqualLift2Maybe}\AgdaSpace{}%
\AgdaBound{g}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaFunction{stackTransform2StateTransform}\AgdaSpace{}%
\AgdaBound{g'}\AgdaSpace{}%
\AgdaSymbol{)}\AgdaSpace{}%
\AgdaBound{q}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaFunction{stackTransform2StateTransform}\AgdaSpace{}%
\AgdaBound{f'}\AgdaSpace{}%
\AgdaBound{st}\AgdaSymbol{)}%
\>[110]\AgdaFunction{⟩}\<%
\\
%
\>[4]\AgdaSymbol{(}\AgdaFunction{stackTransform2StateTransform}\AgdaSpace{}%
\AgdaBound{f'}\AgdaSpace{}%
\AgdaBound{st}\AgdaSpace{}%
\AgdaOperator{\AgdaFunction{>>=}}\AgdaSpace{}%
\AgdaFunction{stackTransform2StateTransform}\AgdaSpace{}%
\AgdaBound{g'}\AgdaSymbol{)}\<%
\\
\>[4][@{}l@{\AgdaIndent{0}}]%
\>[7]\AgdaOperator{\AgdaFunction{≡⟨⟩}}\<%
\\
\>[4][@{}l@{\AgdaIndent{0}}]%
\>[5]\AgdaSymbol{(}\AgdaFunction{exeTransformerDepIfStack'}\<%
\\
\>[5][@{}l@{\AgdaIndent{0}}]%
\>[9]\AgdaSymbol{(}\AgdaFunction{liftStackToStateTransformerAux'}%
\>[43]\AgdaSymbol{(}\AgdaBound{f'}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaBound{st}\AgdaSpace{}%
\AgdaSymbol{.}\AgdaField{currentTime}\AgdaSymbol{)}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaBound{st}\AgdaSpace{}%
\AgdaSymbol{.}\AgdaField{msg}\AgdaSymbol{)}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaBound{st}\AgdaSpace{}%
\AgdaSymbol{.}\AgdaField{stack}\AgdaSymbol{)))}%
\>[90]\AgdaBound{st}\<%
\\
\>[5][@{}l@{\AgdaIndent{0}}]%
\>[8]\AgdaOperator{\AgdaFunction{>>=}}\<%
\\
%
\>[8]\AgdaSymbol{λ}\AgdaSpace{}%
\AgdaBound{s}%
\>[493I]\AgdaSymbol{→}%
\>[16]\AgdaFunction{exeTransformerDepIfStack'}\<%
\\
\>[.][@{}l@{}]\<[493I]%
\>[12]\AgdaSymbol{(}\AgdaFunction{liftStackToStateTransformerAux'}%
\>[46]\AgdaSymbol{(}\AgdaBound{g'}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaBound{s}\AgdaSpace{}%
\AgdaSymbol{.}\AgdaField{currentTime}\AgdaSymbol{)}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaBound{s}\AgdaSpace{}%
\AgdaSymbol{.}\AgdaField{msg}\AgdaSymbol{)}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaBound{s}\AgdaSpace{}%
\AgdaSymbol{.}\AgdaField{stack}\AgdaSymbol{)))}\AgdaSpace{}%
\AgdaBound{s}\AgdaSymbol{)}\<%
\\
%
\\[\AgdaEmptyExtraSkip]%
\>[5][@{}l@{\AgdaIndent{0}}]%
\>[7]\AgdaFunction{≡⟨}\AgdaSpace{}%
\AgdaFunction{lemmaStackSemIsSemScriptaux2}\AgdaSpace{}%
\AgdaBound{g'}\AgdaSpace{}%
\AgdaBound{st}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaBound{f'}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaBound{st}\AgdaSpace{}%
\AgdaSymbol{.}\AgdaField{currentTime}\AgdaSymbol{)}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaBound{st}\AgdaSpace{}%
\AgdaSymbol{.}\AgdaField{msg}\AgdaSymbol{)}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaBound{st}\AgdaSpace{}%
\AgdaSymbol{.}\AgdaField{stack}\AgdaSymbol{))}%
\>[91]\AgdaFunction{⟩}\<%
\\
%
\>[4]\AgdaFunction{exeTransformerDepIfStack'}\<%
\\
\>[0][@{}l@{\AgdaIndent{0}}]%
\>[2]\AgdaSymbol{(}\AgdaFunction{liftStackToStateTransformerAux'}\<%
\\
\>[2][@{}l@{\AgdaIndent{0}}]%
\>[3]\AgdaSymbol{(}\AgdaBound{f'}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaBound{st}\AgdaSpace{}%
\AgdaSymbol{.}\AgdaField{currentTime}\AgdaSymbol{)}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaBound{st}\AgdaSpace{}%
\AgdaSymbol{.}\AgdaField{msg}\AgdaSymbol{)}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaBound{st}\AgdaSpace{}%
\AgdaSymbol{.}\AgdaField{stack}\AgdaSymbol{)}\AgdaSpace{}%
\AgdaOperator{\AgdaFunction{>>=}}\AgdaSpace{}%
\AgdaBound{g'}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaBound{st}\AgdaSpace{}%
\AgdaSymbol{.}\AgdaField{currentTime}\AgdaSymbol{)}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaBound{st}\AgdaSpace{}%
\AgdaSymbol{.}\AgdaField{msg}\AgdaSymbol{)))}%
\>[85]\AgdaBound{st}%
\>[89]\AgdaOperator{\AgdaFunction{∎}}\<%
\\
%
\\[\AgdaEmptyExtraSkip]%
%
\\[\AgdaEmptyExtraSkip]%
%
\\[\AgdaEmptyExtraSkip]%
\>[0]\AgdaFunction{lemmaStackSemIsSemScript}%
\>[523I]\AgdaSymbol{:}%
\>[524I]\AgdaSymbol{(}\AgdaBound{prog}\AgdaSpace{}%
\AgdaSymbol{:}\AgdaSpace{}%
\AgdaFunction{BitcoinScript}\AgdaSymbol{)}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaBound{nonIfs}\AgdaSpace{}%
\AgdaSymbol{:}\AgdaSpace{}%
\AgdaFunction{NonIfScript}\AgdaSpace{}%
\AgdaBound{prog}\AgdaSymbol{)}\<%
\\
\>[.][@{}l@{}]\<[524I]%
\>[27]\AgdaSymbol{(}\AgdaBound{state₁}\AgdaSpace{}%
\AgdaSymbol{:}\AgdaSpace{}%
\AgdaRecord{State}\AgdaSymbol{)}\<%
\\
\>[523I][@{}l@{\AgdaIndent{0}}]%
\>[26]\AgdaSymbol{→}\AgdaSpace{}%
\AgdaOperator{\AgdaFunction{⟦}}\AgdaSpace{}%
\AgdaBound{prog}\AgdaSpace{}%
\AgdaOperator{\AgdaFunction{⟧}}\AgdaSpace{}%
\AgdaBound{state₁}%
\>[45]\AgdaOperator{\AgdaDatatype{≡}}\AgdaSpace{}%
\AgdaFunction{stackTransform2StateTransform}\AgdaSpace{}%
\AgdaOperator{\AgdaFunction{⟦}}\AgdaSpace{}%
\AgdaBound{prog}\AgdaSpace{}%
\AgdaOperator{\AgdaFunction{⟧stack}}\AgdaSpace{}%
\AgdaBound{state₁}\<%
\\
\>[0]\AgdaFunction{lemmaStackSemIsSemScript}\AgdaSpace{}%
\AgdaInductiveConstructor{[]}\AgdaSpace{}%
\AgdaBound{nonIfs}\AgdaSpace{}%
\AgdaOperator{\AgdaInductiveConstructor{⟨}}\AgdaSpace{}%
\AgdaBound{currentTime₁}\AgdaSpace{}%
\AgdaOperator{\AgdaInductiveConstructor{,}}\AgdaSpace{}%
\AgdaBound{msg₁}\AgdaSpace{}%
\AgdaOperator{\AgdaInductiveConstructor{,}}\AgdaSpace{}%
\AgdaBound{stack₁}\AgdaSpace{}%
\AgdaOperator{\AgdaInductiveConstructor{,}}\AgdaSpace{}%
\AgdaInductiveConstructor{[]}\AgdaSpace{}%
\AgdaOperator{\AgdaInductiveConstructor{,}}\AgdaSpace{}%
\AgdaBound{consis₁}\AgdaSpace{}%
\AgdaOperator{\AgdaInductiveConstructor{⟩}}\AgdaSpace{}%
\AgdaSymbol{=}\AgdaSpace{}%
\AgdaInductiveConstructor{refl}\<%
\\
\>[0]\AgdaFunction{lemmaStackSemIsSemScript}\AgdaSpace{}%
\AgdaInductiveConstructor{[]}\AgdaSpace{}%
\AgdaBound{nonIfs}\AgdaSpace{}%
\AgdaOperator{\AgdaInductiveConstructor{⟨}}\AgdaSpace{}%
\AgdaBound{currentTime₁}\AgdaSpace{}%
\AgdaOperator{\AgdaInductiveConstructor{,}}\AgdaSpace{}%
\AgdaBound{msg₁}\AgdaSpace{}%
\AgdaOperator{\AgdaInductiveConstructor{,}}\AgdaSpace{}%
\AgdaBound{stack₁}\AgdaSpace{}%
\AgdaOperator{\AgdaInductiveConstructor{,}}\AgdaSpace{}%
\AgdaInductiveConstructor{ifCase}\AgdaSpace{}%
\AgdaOperator{\AgdaInductiveConstructor{∷}}\AgdaSpace{}%
\AgdaBound{ifStack₁}\AgdaSpace{}%
\AgdaOperator{\AgdaInductiveConstructor{,}}\AgdaSpace{}%
\AgdaBound{consis₁}\AgdaSpace{}%
\AgdaOperator{\AgdaInductiveConstructor{⟩}}\AgdaSpace{}%
\AgdaSymbol{=}\AgdaSpace{}%
\AgdaInductiveConstructor{refl}\<%
\\
\>[0]\AgdaFunction{lemmaStackSemIsSemScript}\AgdaSpace{}%
\AgdaInductiveConstructor{[]}\AgdaSpace{}%
\AgdaBound{nonIfs}\AgdaSpace{}%
\AgdaOperator{\AgdaInductiveConstructor{⟨}}\AgdaSpace{}%
\AgdaBound{currentTime₁}\AgdaSpace{}%
\AgdaOperator{\AgdaInductiveConstructor{,}}\AgdaSpace{}%
\AgdaBound{msg₁}\AgdaSpace{}%
\AgdaOperator{\AgdaInductiveConstructor{,}}\AgdaSpace{}%
\AgdaBound{stack₁}\AgdaSpace{}%
\AgdaOperator{\AgdaInductiveConstructor{,}}\AgdaSpace{}%
\AgdaInductiveConstructor{elseCase}\AgdaSpace{}%
\AgdaOperator{\AgdaInductiveConstructor{∷}}\AgdaSpace{}%
\AgdaBound{ifStack₁}\AgdaSpace{}%
\AgdaOperator{\AgdaInductiveConstructor{,}}\AgdaSpace{}%
\AgdaBound{consis₁}\AgdaSpace{}%
\AgdaOperator{\AgdaInductiveConstructor{⟩}}\AgdaSpace{}%
\AgdaSymbol{=}\AgdaSpace{}%
\AgdaInductiveConstructor{refl}\<%
\\
\>[0]\AgdaFunction{lemmaStackSemIsSemScript}\AgdaSpace{}%
\AgdaInductiveConstructor{[]}\AgdaSpace{}%
\AgdaBound{nonIfs}\AgdaSpace{}%
\AgdaOperator{\AgdaInductiveConstructor{⟨}}\AgdaSpace{}%
\AgdaBound{currentTime₁}\AgdaSpace{}%
\AgdaOperator{\AgdaInductiveConstructor{,}}\AgdaSpace{}%
\AgdaBound{msg₁}\AgdaSpace{}%
\AgdaOperator{\AgdaInductiveConstructor{,}}\AgdaSpace{}%
\AgdaBound{stack₁}\AgdaSpace{}%
\AgdaOperator{\AgdaInductiveConstructor{,}}\AgdaSpace{}%
\AgdaInductiveConstructor{ifSkip}\AgdaSpace{}%
\AgdaOperator{\AgdaInductiveConstructor{∷}}\AgdaSpace{}%
\AgdaBound{ifStack₁}\AgdaSpace{}%
\AgdaOperator{\AgdaInductiveConstructor{,}}\AgdaSpace{}%
\AgdaBound{consis₁}\AgdaSpace{}%
\AgdaOperator{\AgdaInductiveConstructor{⟩}}\AgdaSpace{}%
\AgdaSymbol{=}\AgdaSpace{}%
\AgdaInductiveConstructor{refl}\<%
\\
\>[0]\AgdaFunction{lemmaStackSemIsSemScript}\AgdaSpace{}%
\AgdaInductiveConstructor{[]}\AgdaSpace{}%
\AgdaBound{nonIfs}\AgdaSpace{}%
\AgdaOperator{\AgdaInductiveConstructor{⟨}}\AgdaSpace{}%
\AgdaBound{currentTime₁}\AgdaSpace{}%
\AgdaOperator{\AgdaInductiveConstructor{,}}\AgdaSpace{}%
\AgdaBound{msg₁}\AgdaSpace{}%
\AgdaOperator{\AgdaInductiveConstructor{,}}\AgdaSpace{}%
\AgdaBound{stack₁}\AgdaSpace{}%
\AgdaOperator{\AgdaInductiveConstructor{,}}\AgdaSpace{}%
\AgdaInductiveConstructor{elseSkip}\AgdaSpace{}%
\AgdaOperator{\AgdaInductiveConstructor{∷}}\AgdaSpace{}%
\AgdaBound{ifStack₁}\AgdaSpace{}%
\AgdaOperator{\AgdaInductiveConstructor{,}}\AgdaSpace{}%
\AgdaBound{consis₁}\AgdaSpace{}%
\AgdaOperator{\AgdaInductiveConstructor{⟩}}\AgdaSpace{}%
\AgdaSymbol{=}\AgdaSpace{}%
\AgdaInductiveConstructor{refl}\<%
\\
\>[0]\AgdaFunction{lemmaStackSemIsSemScript}\AgdaSpace{}%
\AgdaInductiveConstructor{[]}\AgdaSpace{}%
\AgdaBound{nonIfs}\AgdaSpace{}%
\AgdaOperator{\AgdaInductiveConstructor{⟨}}\AgdaSpace{}%
\AgdaBound{currentTime₁}\AgdaSpace{}%
\AgdaOperator{\AgdaInductiveConstructor{,}}\AgdaSpace{}%
\AgdaBound{msg₁}\AgdaSpace{}%
\AgdaOperator{\AgdaInductiveConstructor{,}}\AgdaSpace{}%
\AgdaBound{stack₁}\AgdaSpace{}%
\AgdaOperator{\AgdaInductiveConstructor{,}}\AgdaSpace{}%
\AgdaInductiveConstructor{ifIgnore}\AgdaSpace{}%
\AgdaOperator{\AgdaInductiveConstructor{∷}}\AgdaSpace{}%
\AgdaBound{ifStack₁}\AgdaSpace{}%
\AgdaOperator{\AgdaInductiveConstructor{,}}\AgdaSpace{}%
\AgdaBound{consis₁}\AgdaSpace{}%
\AgdaOperator{\AgdaInductiveConstructor{⟩}}\AgdaSpace{}%
\AgdaSymbol{=}\AgdaSpace{}%
\AgdaInductiveConstructor{refl}\<%
\\
\>[0]\AgdaFunction{lemmaStackSemIsSemScript}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaBound{op}\AgdaSpace{}%
\AgdaOperator{\AgdaInductiveConstructor{∷}}\AgdaSpace{}%
\AgdaInductiveConstructor{[]}\AgdaSymbol{)}\AgdaSpace{}%
\AgdaBound{nonIfs}\AgdaSpace{}%
\AgdaBound{state1}\AgdaSpace{}%
\AgdaKeyword{rewrite}\AgdaSpace{}%
\AgdaFunction{lemmaStackSemIsSemantics}\AgdaSpace{}%
\AgdaBound{op}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaFunction{nonIfScript2NonIf2Head}\AgdaSpace{}%
\AgdaBound{op}\AgdaSpace{}%
\AgdaInductiveConstructor{[]}\AgdaSpace{}%
\AgdaBound{nonIfs}\AgdaSpace{}%
\AgdaSymbol{)}%
\>[125]\AgdaSymbol{=}\AgdaSpace{}%
\AgdaInductiveConstructor{refl}\<%
\\
\>[0]\AgdaFunction{lemmaStackSemIsSemScript}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaBound{op}\AgdaSpace{}%
\AgdaOperator{\AgdaInductiveConstructor{∷}}\AgdaSpace{}%
\AgdaBound{rest}\AgdaSymbol{@(}\AgdaBound{x₁}\AgdaSpace{}%
\AgdaOperator{\AgdaInductiveConstructor{∷}}\AgdaSpace{}%
\AgdaBound{prog}\AgdaSymbol{))}\AgdaSpace{}%
\AgdaBound{nonIfs}\AgdaSpace{}%
\AgdaOperator{\AgdaInductiveConstructor{⟨}}\AgdaSpace{}%
\AgdaBound{currentTime₁}\AgdaSpace{}%
\AgdaOperator{\AgdaInductiveConstructor{,}}\AgdaSpace{}%
\AgdaBound{msg₁}\AgdaSpace{}%
\AgdaOperator{\AgdaInductiveConstructor{,}}\AgdaSpace{}%
\AgdaBound{stack₁}\AgdaSpace{}%
\AgdaOperator{\AgdaInductiveConstructor{,}}\AgdaSpace{}%
\AgdaBound{ifstack₁}\AgdaSpace{}%
\AgdaOperator{\AgdaInductiveConstructor{,}}\AgdaSpace{}%
\AgdaBound{consis₁}\AgdaSpace{}%
\AgdaOperator{\AgdaInductiveConstructor{⟩}}\AgdaSpace{}%
\AgdaSymbol{=}\<%
\\
\>[0][@{}l@{\AgdaIndent{0}}]%
\>[7]\AgdaSymbol{(}\AgdaOperator{\AgdaFunction{⟦}}%
\>[674I]\AgdaBound{op}\AgdaSpace{}%
\AgdaOperator{\AgdaFunction{⟧s}}\AgdaSpace{}%
\AgdaOperator{\AgdaInductiveConstructor{⟨}}\AgdaSpace{}%
\AgdaBound{currentTime₁}\AgdaSpace{}%
\AgdaOperator{\AgdaInductiveConstructor{,}}\AgdaSpace{}%
\AgdaBound{msg₁}\AgdaSpace{}%
\AgdaOperator{\AgdaInductiveConstructor{,}}\AgdaSpace{}%
\AgdaBound{stack₁}\AgdaSpace{}%
\AgdaOperator{\AgdaInductiveConstructor{,}}\AgdaSpace{}%
\AgdaBound{ifstack₁}\AgdaSpace{}%
\AgdaOperator{\AgdaInductiveConstructor{,}}\AgdaSpace{}%
\AgdaBound{consis₁}\AgdaSpace{}%
\AgdaOperator{\AgdaInductiveConstructor{⟩}}\AgdaSpace{}%
\AgdaOperator{\AgdaFunction{>>=}}\AgdaSpace{}%
\AgdaOperator{\AgdaFunction{⟦}}\AgdaSpace{}%
\AgdaBound{rest}\AgdaSpace{}%
\AgdaOperator{\AgdaFunction{⟧}}\AgdaSymbol{)}\<%
\\
\>[.][@{}l@{}]\<[674I]%
\>[10]\AgdaFunction{≡⟨}\AgdaSpace{}%
\AgdaFunction{cong}%
\>[692I]\AgdaSymbol{(λ}\AgdaSpace{}%
\AgdaBound{x}\AgdaSpace{}%
\AgdaSymbol{→}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaBound{x}\AgdaSpace{}%
\AgdaOperator{\AgdaInductiveConstructor{⟨}}\AgdaSpace{}%
\AgdaBound{currentTime₁}\AgdaSpace{}%
\AgdaOperator{\AgdaInductiveConstructor{,}}\AgdaSpace{}%
\AgdaBound{msg₁}\AgdaSpace{}%
\AgdaOperator{\AgdaInductiveConstructor{,}}\AgdaSpace{}%
\AgdaBound{stack₁}\AgdaSpace{}%
\AgdaOperator{\AgdaInductiveConstructor{,}}\AgdaSpace{}%
\AgdaBound{ifstack₁}\AgdaSpace{}%
\AgdaOperator{\AgdaInductiveConstructor{,}}\AgdaSpace{}%
\AgdaBound{consis₁}\AgdaSpace{}%
\AgdaOperator{\AgdaInductiveConstructor{⟩}}\AgdaSpace{}%
\AgdaOperator{\AgdaFunction{>>=}}\AgdaSpace{}%
\AgdaOperator{\AgdaFunction{⟦}}\AgdaSpace{}%
\AgdaBound{rest}\AgdaSpace{}%
\AgdaOperator{\AgdaFunction{⟧}}\AgdaSpace{}%
\AgdaSymbol{))}\<%
\\
\>[.][@{}l@{}]\<[692I]%
\>[18]\AgdaSymbol{(}\AgdaFunction{lemmaStackSemIsSemantics}\AgdaSpace{}%
\AgdaBound{op}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaFunction{nonIfScript2NonIf2Head}\AgdaSpace{}%
\AgdaBound{op}\AgdaSpace{}%
\AgdaBound{rest}\AgdaSpace{}%
\AgdaBound{nonIfs}\AgdaSymbol{))}%
\>[89]\AgdaFunction{⟩}\<%
\\
%
\>[7]\AgdaSymbol{(}\AgdaFunction{stackTransform2StateTransform}\AgdaSpace{}%
\AgdaOperator{\AgdaFunction{⟦}}\AgdaSpace{}%
\AgdaBound{op}\AgdaSpace{}%
\AgdaOperator{\AgdaFunction{⟧stacks}}%
\>[52]\AgdaOperator{\AgdaInductiveConstructor{⟨}}\AgdaSpace{}%
\AgdaBound{currentTime₁}\AgdaSpace{}%
\AgdaOperator{\AgdaInductiveConstructor{,}}\AgdaSpace{}%
\AgdaBound{msg₁}\AgdaSpace{}%
\AgdaOperator{\AgdaInductiveConstructor{,}}\AgdaSpace{}%
\AgdaBound{stack₁}\AgdaSpace{}%
\AgdaOperator{\AgdaInductiveConstructor{,}}\AgdaSpace{}%
\AgdaBound{ifstack₁}\AgdaSpace{}%
\AgdaOperator{\AgdaInductiveConstructor{,}}\AgdaSpace{}%
\AgdaBound{consis₁}\AgdaSpace{}%
\AgdaOperator{\AgdaInductiveConstructor{⟩}}\<%
\\
\>[7][@{}l@{\AgdaIndent{0}}]%
\>[9]\AgdaOperator{\AgdaFunction{>>=}}\AgdaSpace{}%
\AgdaOperator{\AgdaFunction{⟦}}\AgdaSpace{}%
\AgdaBound{rest}\AgdaSpace{}%
\AgdaOperator{\AgdaFunction{⟧}}\AgdaSymbol{)}\<%
\\
%
\\[\AgdaEmptyExtraSkip]%
\>[9][@{}l@{\AgdaIndent{0}}]%
\>[10]\AgdaFunction{≡⟨}\AgdaSpace{}%
\AgdaFunction{lemmaEqualLift2Maybe}%
\>[35]\AgdaOperator{\AgdaFunction{⟦}}\AgdaSpace{}%
\AgdaBound{rest}\AgdaSpace{}%
\AgdaOperator{\AgdaFunction{⟧}}%
\>[45]\AgdaSymbol{(}\AgdaFunction{stackTransform2StateTransform}\AgdaSpace{}%
\AgdaOperator{\AgdaFunction{⟦}}\AgdaSpace{}%
\AgdaBound{rest}\AgdaSpace{}%
\AgdaOperator{\AgdaFunction{⟧stack}}\AgdaSpace{}%
\AgdaSymbol{)}\<%
\\
\>[10][@{}l@{\AgdaIndent{0}}]%
\>[12]\AgdaSymbol{(}\AgdaFunction{lemmaStackSemIsSemScript}\AgdaSpace{}%
\AgdaBound{rest}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaFunction{nonIfScript2NonIf2Tail}\AgdaSpace{}%
\AgdaBound{op}\AgdaSpace{}%
\AgdaBound{rest}\AgdaSpace{}%
\AgdaBound{nonIfs}\AgdaSymbol{))}\<%
\\
%
\>[12]\AgdaSymbol{((}\AgdaFunction{stackTransform2StateTransform}\AgdaSpace{}%
\AgdaOperator{\AgdaFunction{⟦}}\AgdaSpace{}%
\AgdaBound{op}\AgdaSpace{}%
\AgdaOperator{\AgdaFunction{⟧stacks}}%
\>[58]\AgdaOperator{\AgdaInductiveConstructor{⟨}}\AgdaSpace{}%
\AgdaBound{currentTime₁}\AgdaSpace{}%
\AgdaOperator{\AgdaInductiveConstructor{,}}\AgdaSpace{}%
\AgdaBound{msg₁}\AgdaSpace{}%
\AgdaOperator{\AgdaInductiveConstructor{,}}\AgdaSpace{}%
\AgdaBound{stack₁}\AgdaSpace{}%
\AgdaOperator{\AgdaInductiveConstructor{,}}\AgdaSpace{}%
\AgdaBound{ifstack₁}\AgdaSpace{}%
\AgdaOperator{\AgdaInductiveConstructor{,}}\AgdaSpace{}%
\AgdaBound{consis₁}\AgdaSpace{}%
\AgdaOperator{\AgdaInductiveConstructor{⟩}}\AgdaSymbol{))}\AgdaSpace{}%
\AgdaFunction{⟩}\<%
\\
%
\>[7]\AgdaSymbol{(}\AgdaFunction{stackTransform2StateTransform}\AgdaSpace{}%
\AgdaOperator{\AgdaFunction{⟦}}\AgdaSpace{}%
\AgdaBound{op}\AgdaSpace{}%
\AgdaOperator{\AgdaFunction{⟧stacks}}%
\>[52]\AgdaOperator{\AgdaInductiveConstructor{⟨}}\AgdaSpace{}%
\AgdaBound{currentTime₁}\AgdaSpace{}%
\AgdaOperator{\AgdaInductiveConstructor{,}}\AgdaSpace{}%
\AgdaBound{msg₁}\AgdaSpace{}%
\AgdaOperator{\AgdaInductiveConstructor{,}}\AgdaSpace{}%
\AgdaBound{stack₁}\AgdaSpace{}%
\AgdaOperator{\AgdaInductiveConstructor{,}}\AgdaSpace{}%
\AgdaBound{ifstack₁}\AgdaSpace{}%
\AgdaOperator{\AgdaInductiveConstructor{,}}\AgdaSpace{}%
\AgdaBound{consis₁}\AgdaSpace{}%
\AgdaOperator{\AgdaInductiveConstructor{⟩}}\<%
\\
\>[7][@{}l@{\AgdaIndent{0}}]%
\>[12]\AgdaOperator{\AgdaFunction{>>=}}%
\>[772I]\AgdaFunction{stackTransform2StateTransform}\AgdaSpace{}%
\AgdaOperator{\AgdaFunction{⟦}}\AgdaSpace{}%
\AgdaBound{rest}\AgdaSpace{}%
\AgdaOperator{\AgdaFunction{⟧stack}}\AgdaSymbol{)}\<%
\\
\>[.][@{}l@{}]\<[772I]%
\>[16]\AgdaFunction{≡⟨}%
\>[776I]\AgdaFunction{lemmaStackSemIsSemScriptaux2}\AgdaSpace{}%
\AgdaOperator{\AgdaFunction{⟦}}\AgdaSpace{}%
\AgdaBound{x₁}\AgdaSpace{}%
\AgdaOperator{\AgdaInductiveConstructor{∷}}\AgdaSpace{}%
\AgdaBound{prog}\AgdaSpace{}%
\AgdaOperator{\AgdaFunction{⟧stack}}\AgdaSpace{}%
\AgdaOperator{\AgdaInductiveConstructor{⟨}}\AgdaSpace{}%
\AgdaBound{currentTime₁}\AgdaSpace{}%
\AgdaOperator{\AgdaInductiveConstructor{,}}\AgdaSpace{}%
\AgdaBound{msg₁}\AgdaSpace{}%
\AgdaOperator{\AgdaInductiveConstructor{,}}\AgdaSpace{}%
\AgdaBound{stack₁}\AgdaSpace{}%
\AgdaOperator{\AgdaInductiveConstructor{,}}\AgdaSpace{}%
\AgdaBound{ifstack₁}\AgdaSpace{}%
\AgdaOperator{\AgdaInductiveConstructor{,}}\AgdaSpace{}%
\AgdaBound{consis₁}\AgdaSpace{}%
\AgdaOperator{\AgdaInductiveConstructor{⟩}}\<%
\\
\>[.][@{}l@{}]\<[776I]%
\>[19]\AgdaSymbol{(}\AgdaOperator{\AgdaFunction{⟦}}\AgdaSpace{}%
\AgdaBound{op}\AgdaSpace{}%
\AgdaOperator{\AgdaFunction{⟧stacks}}\AgdaSpace{}%
\AgdaBound{currentTime₁}\AgdaSpace{}%
\AgdaBound{msg₁}\AgdaSpace{}%
\AgdaBound{stack₁}\AgdaSymbol{)}\AgdaSpace{}%
\AgdaFunction{⟩}\<%
\\
\>[0][@{}l@{\AgdaIndent{0}}]%
\>[6]\AgdaFunction{exeTransformerDepIfStack'}\<%
\\
%
\>[6]\AgdaSymbol{(}\AgdaFunction{liftStackToStateTransformerAux'}\<%
\\
\>[6][@{}l@{\AgdaIndent{0}}]%
\>[7]\AgdaSymbol{(}\AgdaOperator{\AgdaFunction{⟦}}\AgdaSpace{}%
\AgdaBound{op}\AgdaSpace{}%
\AgdaOperator{\AgdaFunction{⟧stacks}}\AgdaSpace{}%
\AgdaBound{currentTime₁}\AgdaSpace{}%
\AgdaBound{msg₁}\AgdaSpace{}%
\AgdaBound{stack₁}\AgdaSpace{}%
\AgdaOperator{\AgdaFunction{>>=}}\AgdaSpace{}%
\AgdaOperator{\AgdaFunction{⟦}}\AgdaSpace{}%
\AgdaBound{rest}\AgdaSpace{}%
\AgdaOperator{\AgdaFunction{⟧stack}}\AgdaSpace{}%
\AgdaBound{currentTime₁}\AgdaSpace{}%
\AgdaBound{msg₁}\AgdaSymbol{))}\<%
\\
%
\>[6]\AgdaOperator{\AgdaInductiveConstructor{⟨}}\AgdaSpace{}%
\AgdaBound{currentTime₁}\AgdaSpace{}%
\AgdaOperator{\AgdaInductiveConstructor{,}}\AgdaSpace{}%
\AgdaBound{msg₁}\AgdaSpace{}%
\AgdaOperator{\AgdaInductiveConstructor{,}}\AgdaSpace{}%
\AgdaBound{stack₁}\AgdaSpace{}%
\AgdaOperator{\AgdaInductiveConstructor{,}}\AgdaSpace{}%
\AgdaBound{ifstack₁}\AgdaSpace{}%
\AgdaOperator{\AgdaInductiveConstructor{,}}\AgdaSpace{}%
\AgdaBound{consis₁}\AgdaSpace{}%
\AgdaOperator{\AgdaInductiveConstructor{⟩}}\<%
\\
\>[0][@{}l@{\AgdaIndent{0}}]%
\>[4]\AgdaOperator{\AgdaFunction{∎}}\<%
\\
%
\\[\AgdaEmptyExtraSkip]%
%
\\[\AgdaEmptyExtraSkip]%
%
\\[\AgdaEmptyExtraSkip]%
%
\\[\AgdaEmptyExtraSkip]%
%
\\[\AgdaEmptyExtraSkip]%
%
\\[\AgdaEmptyExtraSkip]%
%
\\[\AgdaEmptyExtraSkip]%
%
\\[\AgdaEmptyExtraSkip]%
%
\\[\AgdaEmptyExtraSkip]%
\>[0]\AgdaFunction{lemmaNonIfInstrGenericCondImpliesTripleaux'}\AgdaSpace{}%
\AgdaSymbol{:}\<%
\\
\>[0][@{}l@{\AgdaIndent{0}}]%
\>[10]\AgdaSymbol{(}\AgdaBound{prog}\AgdaSpace{}%
\AgdaSymbol{:}\AgdaSpace{}%
\AgdaFunction{BitcoinScript}\AgdaSymbol{)(}\AgdaBound{nonIf}\AgdaSpace{}%
\AgdaSymbol{:}\AgdaSpace{}%
\AgdaFunction{NonIfScript}\AgdaSpace{}%
\AgdaBound{prog}\AgdaSymbol{)}\<%
\\
%
\>[10]\AgdaSymbol{(}\AgdaBound{φ}\AgdaSpace{}%
\AgdaBound{ψ}\AgdaSpace{}%
\AgdaSymbol{:}\AgdaSpace{}%
\AgdaFunction{Predicate}\AgdaSymbol{)}\<%
\\
%
\>[10]\AgdaSymbol{→}\AgdaSpace{}%
\AgdaOperator{\AgdaRecord{<}}\AgdaSpace{}%
\AgdaBound{φ}\AgdaSpace{}%
\AgdaOperator{\AgdaRecord{>gen}}\AgdaSpace{}%
\AgdaFunction{stackTransform2StateTransform}\AgdaSpace{}%
\AgdaOperator{\AgdaFunction{⟦}}%
\>[54]\AgdaBound{prog}%
\>[60]\AgdaOperator{\AgdaFunction{⟧stack}}\AgdaSpace{}%
\AgdaOperator{\AgdaRecord{<}}\AgdaSpace{}%
\AgdaBound{ψ}\AgdaSpace{}%
\AgdaOperator{\AgdaRecord{>}}\<%
\\
%
\>[10]\AgdaSymbol{→}\AgdaSpace{}%
\AgdaOperator{\AgdaRecord{<}}\AgdaSpace{}%
\AgdaBound{φ}\AgdaSpace{}%
\AgdaOperator{\AgdaRecord{>gen}}\AgdaSpace{}%
\AgdaOperator{\AgdaFunction{⟦}}\AgdaSpace{}%
\AgdaBound{prog}\AgdaSpace{}%
\AgdaOperator{\AgdaFunction{⟧}}\AgdaSpace{}%
\AgdaOperator{\AgdaRecord{<}}\AgdaSpace{}%
\AgdaBound{ψ}\AgdaSpace{}%
\AgdaOperator{\AgdaRecord{>}}\<%
\\
\>[0]\AgdaFunction{lemmaNonIfInstrGenericCondImpliesTripleaux'}\AgdaSpace{}%
\AgdaBound{prog}\AgdaSpace{}%
\AgdaBound{nonIf}\AgdaSpace{}%
\AgdaBound{φ}\AgdaSpace{}%
\AgdaBound{ψ}\AgdaSpace{}%
\AgdaBound{x}\<%
\\
\>[0][@{}l@{\AgdaIndent{0}}]%
\>[4]\AgdaSymbol{=}%
\>[851I]\AgdaFunction{lemmaTransferHoareTripleGen}\AgdaSpace{}%
\AgdaBound{φ}\AgdaSpace{}%
\AgdaBound{ψ}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaFunction{stackTransform2StateTransform}\AgdaSpace{}%
\AgdaOperator{\AgdaFunction{⟦}}%
\>[72]\AgdaBound{prog}%
\>[78]\AgdaOperator{\AgdaFunction{⟧stack}}\AgdaSymbol{)}\AgdaSpace{}%
\AgdaOperator{\AgdaFunction{⟦}}\AgdaSpace{}%
\AgdaBound{prog}\AgdaSpace{}%
\AgdaOperator{\AgdaFunction{⟧}}\<%
\\
\>[.][@{}l@{}]\<[851I]%
\>[6]\AgdaSymbol{(λ}\AgdaSpace{}%
\AgdaBound{s}\AgdaSpace{}%
\AgdaSymbol{→}\AgdaSpace{}%
\AgdaFunction{sym}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaFunction{lemmaStackSemIsSemScript}\AgdaSpace{}%
\AgdaBound{prog}\AgdaSpace{}%
\AgdaBound{nonIf}\AgdaSpace{}%
\AgdaOperator{\AgdaInductiveConstructor{⟨}}\AgdaSpace{}%
\AgdaField{currentTime}\AgdaSpace{}%
\AgdaBound{s}\AgdaSpace{}%
\AgdaOperator{\AgdaInductiveConstructor{,}}\AgdaSpace{}%
\AgdaField{msg}\AgdaSpace{}%
\AgdaBound{s}\AgdaSpace{}%
\AgdaOperator{\AgdaInductiveConstructor{,}}\AgdaSpace{}%
\AgdaField{stack}\AgdaSpace{}%
\AgdaBound{s}\AgdaSpace{}%
\AgdaOperator{\AgdaInductiveConstructor{,}}\AgdaSpace{}%
\AgdaField{ifStack}\AgdaSpace{}%
\AgdaBound{s}\AgdaSpace{}%
\AgdaOperator{\AgdaInductiveConstructor{,}}\AgdaSpace{}%
\AgdaField{consis}\AgdaSpace{}%
\AgdaBound{s}\AgdaSpace{}%
\AgdaOperator{\AgdaInductiveConstructor{⟩}}\AgdaSymbol{))}\AgdaSpace{}%
\AgdaBound{x}\<%
\\
%
\\[\AgdaEmptyExtraSkip]%
%
\\[\AgdaEmptyExtraSkip]%
%
\\[\AgdaEmptyExtraSkip]%
%
\\[\AgdaEmptyExtraSkip]%
%
\\[\AgdaEmptyExtraSkip]%
%
\\[\AgdaEmptyExtraSkip]%
%
\\[\AgdaEmptyExtraSkip]%
\>[0]\AgdaFunction{lemmaGenericHoareTripleImpliesHoareTripleProg}\AgdaSpace{}%
\AgdaSymbol{:}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaBound{prog}\AgdaSpace{}%
\AgdaSymbol{:}\AgdaSpace{}%
\AgdaFunction{BitcoinScript}\AgdaSymbol{)}\<%
\\
\>[0][@{}l@{\AgdaIndent{0}}]%
\>[44]\AgdaSymbol{(}\AgdaBound{φ}\AgdaSpace{}%
\AgdaBound{ψ}\AgdaSpace{}%
\AgdaSymbol{:}\AgdaSpace{}%
\AgdaFunction{Predicate}\AgdaSymbol{)}\<%
\\
%
\>[44]\AgdaSymbol{→}\AgdaSpace{}%
\AgdaOperator{\AgdaRecord{<}}\AgdaSpace{}%
\AgdaBound{φ}\AgdaSpace{}%
\AgdaOperator{\AgdaRecord{>gen}}\AgdaSpace{}%
\AgdaOperator{\AgdaFunction{⟦}}\AgdaSpace{}%
\AgdaBound{prog}\AgdaSpace{}%
\AgdaOperator{\AgdaFunction{⟧}}\AgdaSpace{}%
\AgdaOperator{\AgdaRecord{<}}%
\>[67]\AgdaBound{ψ}\AgdaSpace{}%
\AgdaOperator{\AgdaRecord{>}}\<%
\\
%
\>[44]\AgdaSymbol{→}\AgdaSpace{}%
\AgdaOperator{\AgdaRecord{<}}\AgdaSpace{}%
\AgdaBound{φ}\AgdaSpace{}%
\AgdaOperator{\AgdaRecord{>ⁱᶠᶠ}}\AgdaSpace{}%
\AgdaBound{prog}\AgdaSpace{}%
\AgdaOperator{\AgdaRecord{<}}\AgdaSpace{}%
\AgdaBound{ψ}\AgdaSpace{}%
\AgdaOperator{\AgdaRecord{>}}\<%
\\
\>[0]\AgdaFunction{lemmaGenericHoareTripleImpliesHoareTripleProg}\AgdaSpace{}%
\AgdaBound{prog}\AgdaSpace{}%
\AgdaBound{φ}\AgdaSpace{}%
\AgdaBound{ψ}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaInductiveConstructor{hoareTripleGen}\AgdaSpace{}%
\AgdaBound{==>g₁}\AgdaSpace{}%
\AgdaBound{<==g₁}\AgdaSymbol{)}\AgdaSpace{}%
\AgdaSymbol{.}\AgdaField{==>}\AgdaSpace{}%
\AgdaSymbol{=}\AgdaSpace{}%
\AgdaBound{==>g₁}\<%
\\
\>[0]\AgdaFunction{lemmaGenericHoareTripleImpliesHoareTripleProg}\AgdaSpace{}%
\AgdaBound{prog}\AgdaSpace{}%
\AgdaBound{φ}\AgdaSpace{}%
\AgdaBound{ψ}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaInductiveConstructor{hoareTripleGen}\AgdaSpace{}%
\AgdaBound{==>g₁}\AgdaSpace{}%
\AgdaBound{<==g₁}\AgdaSymbol{)}\AgdaSpace{}%
\AgdaSymbol{.}\AgdaField{<==}\AgdaSpace{}%
\AgdaSymbol{=}\AgdaSpace{}%
\AgdaBound{<==g₁}\<%
\\
%
\\[\AgdaEmptyExtraSkip]%
\>[0]\AgdaFunction{lemmaNonIfInstrGenericCondImpliesTripleauxProg}\AgdaSpace{}%
\AgdaSymbol{:}\<%
\\
\>[0][@{}l@{\AgdaIndent{0}}]%
\>[10]\AgdaSymbol{(}\AgdaBound{prog}\AgdaSpace{}%
\AgdaSymbol{:}\AgdaSpace{}%
\AgdaFunction{BitcoinScript}\AgdaSymbol{)(}\AgdaBound{nonIf}\AgdaSpace{}%
\AgdaSymbol{:}\AgdaSpace{}%
\AgdaFunction{NonIfScript}\AgdaSpace{}%
\AgdaBound{prog}\AgdaSymbol{)}\<%
\\
%
\>[10]\AgdaSymbol{(}\AgdaBound{φ}\AgdaSpace{}%
\AgdaBound{ψ}\AgdaSpace{}%
\AgdaSymbol{:}\AgdaSpace{}%
\AgdaFunction{Predicate}\AgdaSymbol{)}\<%
\\
%
\>[10]\AgdaSymbol{→}\AgdaSpace{}%
\AgdaOperator{\AgdaRecord{<}}\AgdaSpace{}%
\AgdaBound{φ}\AgdaSpace{}%
\AgdaOperator{\AgdaRecord{>gen}}\AgdaSpace{}%
\AgdaFunction{stackTransform2StateTransform}\AgdaSpace{}%
\AgdaOperator{\AgdaFunction{⟦}}\AgdaSpace{}%
\AgdaBound{prog}\AgdaSpace{}%
\AgdaOperator{\AgdaFunction{⟧stack}}\AgdaSpace{}%
\AgdaOperator{\AgdaRecord{<}}\AgdaSpace{}%
\AgdaBound{ψ}\AgdaSpace{}%
\AgdaOperator{\AgdaRecord{>}}\<%
\\
%
\>[10]\AgdaSymbol{→}\AgdaSpace{}%
\AgdaOperator{\AgdaRecord{<}}\AgdaSpace{}%
\AgdaBound{φ}\AgdaSpace{}%
\AgdaOperator{\AgdaRecord{>gen}}\AgdaSpace{}%
\AgdaOperator{\AgdaFunction{⟦}}\AgdaSpace{}%
\AgdaBound{prog}\AgdaSpace{}%
\AgdaOperator{\AgdaFunction{⟧}}\AgdaSpace{}%
\AgdaOperator{\AgdaRecord{<}}\AgdaSpace{}%
\AgdaBound{ψ}\AgdaSpace{}%
\AgdaOperator{\AgdaRecord{>}}\<%
\\
\>[0]\AgdaFunction{lemmaNonIfInstrGenericCondImpliesTripleauxProg}\AgdaSpace{}%
\AgdaBound{prog}\AgdaSpace{}%
\AgdaBound{nonIf}\AgdaSpace{}%
\AgdaBound{φ}\AgdaSpace{}%
\AgdaBound{ψ}\AgdaSpace{}%
\AgdaBound{x}\AgdaSpace{}%
\AgdaSymbol{=}\<%
\\
\>[0][@{}l@{\AgdaIndent{0}}]%
\>[4]\AgdaFunction{lemmaTransferHoareTripleGen}\AgdaSpace{}%
\AgdaBound{φ}\AgdaSpace{}%
\AgdaBound{ψ}\<%
\\
\>[4][@{}l@{\AgdaIndent{0}}]%
\>[6]\AgdaSymbol{(}\AgdaFunction{stackTransform2StateTransform}\AgdaSpace{}%
\AgdaOperator{\AgdaFunction{⟦}}\AgdaSpace{}%
\AgdaBound{prog}\AgdaSpace{}%
\AgdaOperator{\AgdaFunction{⟧stack}}\AgdaSymbol{)}\AgdaSpace{}%
\AgdaOperator{\AgdaFunction{⟦}}\AgdaSpace{}%
\AgdaBound{prog}\AgdaSpace{}%
\AgdaOperator{\AgdaFunction{⟧}}\<%
\\
%
\>[6]\AgdaSymbol{(λ}\AgdaSpace{}%
\AgdaBound{s}\AgdaSpace{}%
\AgdaSymbol{→}\AgdaSpace{}%
\AgdaFunction{sym}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaFunction{lemmaStackSemIsSemScript}\AgdaSpace{}%
\AgdaBound{prog}\AgdaSpace{}%
\AgdaBound{nonIf}\AgdaSpace{}%
\AgdaBound{s}\AgdaSymbol{))}\AgdaSpace{}%
\AgdaBound{x}\<%
\\
%
\\[\AgdaEmptyExtraSkip]%
%
\\[\AgdaEmptyExtraSkip]%
\>[0]\AgdaComment{--\ Is\ now\ in}\<%
\\
\>[0]\AgdaComment{--\ \textasciitilde{}/git/Smart-contracts-verification-with-agda/ScriptTester/verificationStackScripts/stackVerificationLemmasPart2.agda}\<%
\\
%
\\[\AgdaEmptyExtraSkip]%
\>[0]\AgdaFunction{hoareTripleStack2HoareTripleIfStack}\AgdaSpace{}%
\AgdaSymbol{:}\<%
\\
\>[0][@{}l@{\AgdaIndent{0}}]%
\>[5]\AgdaSymbol{(}\AgdaBound{ifStack₁}\AgdaSpace{}%
\AgdaSymbol{:}\AgdaSpace{}%
\AgdaFunction{IfStack}\AgdaSymbol{)}\<%
\\
%
\>[5]\AgdaSymbol{(}\AgdaBound{active}\AgdaSpace{}%
\AgdaSymbol{:}\AgdaSpace{}%
\AgdaFunction{IsActiveIfStack}\AgdaSpace{}%
\AgdaBound{ifStack₁}\AgdaSymbol{)}\<%
\\
%
\>[5]\AgdaSymbol{(}\AgdaBound{prog}\AgdaSpace{}%
\AgdaSymbol{:}\AgdaSpace{}%
\AgdaFunction{BitcoinScript}\AgdaSymbol{)}\<%
\\
%
\>[5]\AgdaSymbol{(}\AgdaBound{nonIf}\AgdaSpace{}%
\AgdaSymbol{:}\AgdaSpace{}%
\AgdaFunction{NonIfScript}\AgdaSpace{}%
\AgdaBound{prog}\AgdaSymbol{)}\<%
\\
%
\>[5]\AgdaSymbol{(}\AgdaBound{φ}\AgdaSpace{}%
\AgdaBound{ψ}\AgdaSpace{}%
\AgdaSymbol{:}\AgdaSpace{}%
\AgdaFunction{StackPredicate}\AgdaSymbol{)}\<%
\\
%
\>[5]\AgdaSymbol{→}\AgdaSpace{}%
\AgdaOperator{\AgdaFunction{<}}\AgdaSpace{}%
\AgdaBound{φ}\AgdaSpace{}%
\AgdaOperator{\AgdaFunction{>stack}}\AgdaSpace{}%
\AgdaBound{prog}\AgdaSpace{}%
\AgdaOperator{\AgdaFunction{<}}\AgdaSpace{}%
\AgdaBound{ψ}\AgdaSpace{}%
\AgdaOperator{\AgdaFunction{>}}\<%
\\
%
\>[5]\AgdaSymbol{→}\AgdaSpace{}%
\AgdaOperator{\AgdaRecord{<}}\AgdaSpace{}%
\AgdaFunction{liftStackPred2Pred}\AgdaSpace{}%
\AgdaBound{φ}\AgdaSpace{}%
\AgdaBound{ifStack₁}%
\>[40]\AgdaOperator{\AgdaRecord{>ⁱᶠᶠ}}\AgdaSpace{}%
\AgdaBound{prog}\AgdaSpace{}%
\AgdaOperator{\AgdaRecord{<}}\AgdaSpace{}%
\AgdaFunction{liftStackPred2Pred}\AgdaSpace{}%
\AgdaBound{ψ}\AgdaSpace{}%
\AgdaBound{ifStack₁}%
\>[84]\AgdaOperator{\AgdaRecord{>}}\<%
\\
\>[0]\AgdaFunction{hoareTripleStack2HoareTripleIfStack}\AgdaSpace{}%
\AgdaBound{ifStack₁}\AgdaSpace{}%
\AgdaBound{active}\AgdaSpace{}%
\AgdaBound{prog}\AgdaSpace{}%
\AgdaBound{nonIf}\AgdaSpace{}%
\AgdaBound{φ}\AgdaSpace{}%
\AgdaBound{ψ}\AgdaSpace{}%
\AgdaBound{x}\<%
\\
\>[0][@{}l@{\AgdaIndent{0}}]%
\>[3]\AgdaSymbol{=}%
\>[1009I]\AgdaFunction{lemmaGenericHoareTripleImpliesHoareTripleProg}\AgdaSpace{}%
\AgdaBound{prog}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaFunction{liftStackPred2Pred}\AgdaSpace{}%
\AgdaBound{φ}\AgdaSpace{}%
\AgdaBound{ifStack₁}\AgdaSymbol{)}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaFunction{liftStackPred2Pred}\AgdaSpace{}%
\AgdaBound{ψ}\AgdaSpace{}%
\AgdaBound{ifStack₁}\AgdaSymbol{)}\<%
\\
\>[.][@{}l@{}]\<[1009I]%
\>[5]\AgdaSymbol{(}\AgdaFunction{lemmaNonIfInstrGenericCondImpliesTripleauxProg}\AgdaSpace{}%
\AgdaBound{prog}\AgdaSpace{}%
\AgdaBound{nonIf}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaFunction{liftStackPred2Pred}\AgdaSpace{}%
\AgdaBound{φ}\AgdaSpace{}%
\AgdaBound{ifStack₁}\AgdaSymbol{)}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaFunction{liftStackPred2Pred}\AgdaSpace{}%
\AgdaBound{ψ}\AgdaSpace{}%
\AgdaBound{ifStack₁}\AgdaSymbol{)}\<%
\\
%
\>[5]\AgdaSymbol{(}\AgdaFunction{lemmaHoareTripleStackPartToHoareTripleGeneric}\AgdaSpace{}%
\AgdaOperator{\AgdaFunction{⟦}}\AgdaSpace{}%
\AgdaBound{prog}\AgdaSpace{}%
\AgdaOperator{\AgdaFunction{⟧stack}}\AgdaSpace{}%
\AgdaBound{ifStack₁}\AgdaSpace{}%
\AgdaBound{active}\AgdaSpace{}%
\AgdaBound{φ}%
\>[85]\AgdaBound{ψ}\<%
\\
%
\>[5]\AgdaBound{x}\AgdaSymbol{))}\<%
\\
%
\\[\AgdaEmptyExtraSkip]%
%
\\[\AgdaEmptyExtraSkip]%
\>[0]\AgdaComment{--\ Is\ now\ in}\<%
\\
\>[0]\AgdaComment{--\ \textasciitilde{}/git/Smart-contracts-verification-with-agda/ScriptTester/verificationStackScripts/stackVerificationLemmasPart2.agda}\<%
\\
\>[0]\AgdaComment{--}\<%
\\
\>[0]\AgdaComment{\{-}\<%
\\
\>[0]\AgdaComment{lemmaTransferHoareTripleStack\ :\ (φ\ ψ\ :\ StackPredicate)}\<%
\\
\>[0]\AgdaComment{\ \ \ \ \ \ \ \ \ \ \ \ \ \ \ \ \ \ \ \ \ \ \ \ \ \ \ \ \ \ (f\ g\ :\ Time\ →\ Msg\ →\ Stack\ →\ Maybe\ Stack)}\<%
\\
\>[0]\AgdaComment{\ \ \ \ \ \ \ \ \ \ \ \ \ \ \ \ \ \ \ \ \ \ \ \ \ \ \ \ \ \ (p\ :\ (t\ :\ Time)(m\ :\ Msg)(s\ :\ Stack)\ →\ f\ t\ m\ s\ \ ≡\ g\ t\ m\ s)}\<%
\\
\>[0]\AgdaComment{\ \ \ \ \ \ \ \ \ \ \ \ \ \ \ \ \ \ \ \ \ \ \ \ \ \ \ \ \ \ →\ <\ \ φ\ >gˢ\ \ f\ <\ ψ\ >}\<%
\\
\>[0]\AgdaComment{\ \ \ \ \ \ \ \ \ \ \ \ \ \ \ \ \ \ \ \ \ \ \ \ \ \ \ \ \ \ →\ <\ φ\ >gˢ\ g\ <\ ψ\ >}\<%
\\
\>[0]\AgdaComment{lemmaTransferHoareTripleStack\ φ\ ψ\ f\ g\ p\ (hoareTripleStackGen\ ==>stg₁\ <==stg₁)\ .==>stg\ time\ msg₁\ s\ x}\<%
\\
\>[0]\AgdaComment{\ \ \ \ \ \ \ \ =\ transfer\ (liftPred2Maybe\ (ψ\ time\ msg₁))\ (p\ time\ msg₁\ s)\ (==>stg₁\ time\ msg₁\ s\ x)}\<%
\\
\>[0]\AgdaComment{lemmaTransferHoareTripleStack\ φ\ ψ\ f\ g\ p\ (hoareTripleStackGen\ ==>stg₁\ <==stg₁)\ .<==stg\ time\ msg₁\ s\ x}\<%
\\
\>[0]\AgdaComment{\ \ \ \ \ \ \ \ \ =\ <==stg₁\ time\ msg₁\ s\ (transfer\ (liftPred2Maybe\ (ψ\ time\ msg₁))\ (sym\ (p\ time\ msg₁\ s))\ x)}\<%
\\
\>[0]\AgdaComment{-\}}\<%
\\
%
\\[\AgdaEmptyExtraSkip]%
%
\\[\AgdaEmptyExtraSkip]%
%
\\[\AgdaEmptyExtraSkip]%
%
\\[\AgdaEmptyExtraSkip]%
%
\\[\AgdaEmptyExtraSkip]%
%
\\[\AgdaEmptyExtraSkip]%
%
\\[\AgdaEmptyExtraSkip]%
\>[0]\AgdaFunction{hoareTripleNonActiveIfStackIgnored}\AgdaSpace{}%
\AgdaSymbol{:}\<%
\\
\>[0][@{}l@{\AgdaIndent{0}}]%
\>[5]\AgdaSymbol{(}\AgdaBound{ifStack₁}\AgdaSpace{}%
\AgdaSymbol{:}\AgdaSpace{}%
\AgdaFunction{IfStack}\AgdaSymbol{)}\<%
\\
%
\>[5]\AgdaSymbol{(}\AgdaBound{nonactive}\AgdaSpace{}%
\AgdaSymbol{:}\AgdaSpace{}%
\AgdaFunction{IsNonActiveIfStack}\AgdaSpace{}%
\AgdaBound{ifStack₁}\AgdaSymbol{)}\<%
\\
%
\>[5]\AgdaSymbol{(}\AgdaBound{instr}\AgdaSpace{}%
\AgdaSymbol{:}\AgdaSpace{}%
\AgdaFunction{BitcoinScript}\AgdaSymbol{)}\<%
\\
%
\>[5]\AgdaSymbol{(}\AgdaBound{nonIf}\AgdaSpace{}%
\AgdaSymbol{:}\AgdaSpace{}%
\AgdaFunction{NonIfScript}\AgdaSpace{}%
\AgdaBound{instr}\AgdaSymbol{)}\<%
\\
%
\>[5]\AgdaSymbol{(}\AgdaBound{φ}\AgdaSpace{}%
\AgdaSymbol{:}\AgdaSpace{}%
\AgdaFunction{StackPredicate}\AgdaSymbol{)}\<%
\\
%
\>[5]\AgdaSymbol{→}\AgdaSpace{}%
\AgdaOperator{\AgdaRecord{<}}\AgdaSpace{}%
\AgdaFunction{liftStackPred2Pred}\AgdaSpace{}%
\AgdaBound{φ}\AgdaSpace{}%
\AgdaBound{ifStack₁}%
\>[40]\AgdaOperator{\AgdaRecord{>ⁱᶠᶠ}}\AgdaSpace{}%
\AgdaBound{instr}%
\>[52]\AgdaOperator{\AgdaRecord{<}}\AgdaSpace{}%
\AgdaFunction{liftStackPred2Pred}\AgdaSpace{}%
\AgdaBound{φ}\AgdaSpace{}%
\AgdaBound{ifStack₁}%
\>[85]\AgdaOperator{\AgdaRecord{>}}\<%
\\
\>[0]\AgdaFunction{hoareTripleNonActiveIfStackIgnored}\AgdaSpace{}%
\AgdaBound{ifStack₁}\AgdaSpace{}%
\AgdaBound{nonactive}\AgdaSpace{}%
\AgdaBound{instr}\AgdaSpace{}%
\AgdaBound{nonIf}\AgdaSpace{}%
\AgdaBound{φ}\<%
\\
\>[0][@{}l@{\AgdaIndent{0}}]%
\>[3]\AgdaSymbol{=}%
\>[6]\AgdaFunction{lemmaGenericHoareTripleImpliesHoareTriple''}\AgdaSpace{}%
\AgdaBound{instr}\<%
\\
%
\>[3]\AgdaSymbol{(}\AgdaFunction{liftStackPred2Pred}\AgdaSpace{}%
\AgdaBound{φ}\AgdaSpace{}%
\AgdaBound{ifStack₁}\AgdaSymbol{)}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaFunction{liftStackPred2Pred}\AgdaSpace{}%
\AgdaBound{φ}\AgdaSpace{}%
\AgdaBound{ifStack₁}\AgdaSymbol{)}\<%
\\
%
\>[3]\AgdaSymbol{(}\AgdaFunction{lemmaNonIfInstrGenericCondImpliesTripleaux'}\AgdaSpace{}%
\AgdaBound{instr}\AgdaSpace{}%
\AgdaBound{nonIf}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaFunction{liftStackPred2Pred}\AgdaSpace{}%
\AgdaBound{φ}\AgdaSpace{}%
\AgdaBound{ifStack₁}\AgdaSymbol{)}\<%
\\
%
\>[3]\AgdaSymbol{(}\AgdaFunction{liftStackPred2Pred}\AgdaSpace{}%
\AgdaBound{φ}\AgdaSpace{}%
\AgdaBound{ifStack₁}\AgdaSymbol{)}\<%
\\
%
\>[3]\AgdaSymbol{(}\AgdaFunction{lemmaHoareTripleStackPartToHoareTripleNonActiveGeneric}\AgdaSpace{}%
\AgdaBound{ifStack₁}\AgdaSpace{}%
\AgdaBound{nonactive}\AgdaSpace{}%
\AgdaBound{φ}\AgdaSpace{}%
\AgdaOperator{\AgdaFunction{⟦}}\AgdaSpace{}%
\AgdaBound{instr}\AgdaSpace{}%
\AgdaOperator{\AgdaFunction{⟧stack}}\AgdaSymbol{))}\<%
\\
%
\\[\AgdaEmptyExtraSkip]%
%
\\[\AgdaEmptyExtraSkip]%
%
\\[\AgdaEmptyExtraSkip]%
%
\\[\AgdaEmptyExtraSkip]%
\>[0]\AgdaComment{\{-}\<%
\\
\>[0]\AgdaComment{hoareTripleNonActiveIfStackIgnored\ :}\<%
\\
\>[0]\AgdaComment{\ \ \ \ \ (ifStack₁\ :\ IfStack)}\<%
\\
\>[0]\AgdaComment{\ \ \ \ \ (nonactive\ :\ IsNonActiveIfStack\ ifStack₁)}\<%
\\
\>[0]\AgdaComment{\ \ \ \ \ (prog\ :\ BitcoinScript)}\<%
\\
\>[0]\AgdaComment{\ \ \ \ \ (nonIf\ :\ NonIfScript\ prog)}\<%
\\
\>[0]\AgdaComment{\ \ \ \ \ (φ\ :\ StackPredicate)}\<%
\\
\>[0]\AgdaComment{\ \ \ \ \ →\ <\ liftStackPred2Pred\ φ\ ifStack₁\ \ >iff\ prog\ <\ liftStackPred2Pred\ φ\ ifStack₁\ \ \ >}\<%
\\
\>[0]\AgdaComment{hoarTripleNonActiveIfStackIgnored\ =\ lemmaNonActiveIfStackHoareTriple'\ -\}}\<%
\\
\>[0]\AgdaComment{\{-\ \ \ *********\ \ \ \ hoarTripleNonActiveIfStackIgnored\ \ \ \ should\ be\ deleted\ and\ replaced\ by}\<%
\\
\>[0]\AgdaComment{\ \ \ \ \ lemmaNonActiveIfStackHoareTriple'}\<%
\\
\>[0]\AgdaComment{\ \ \ \ \ \ (possibly\ you\ rename\ lemmaNonActiveIfStackHoareTriple'\ into\ something\ more\ memorable}\<%
\\
\>[0]\<%
\\
\>[0]\AgdaComment{call\ it\ hoareTripleNonActiveIfStackIgnored}\<%
\\
\>[0]\AgdaComment{-\}}\<%
\\
%
\\[\AgdaEmptyExtraSkip]%
\>[0]\AgdaComment{\{-}\<%
\\
\>[0]\AgdaComment{hoarTripleNonActiveIfStackIgnored\ ifStack₁\ nonactive\ []\ nonIf\ φ\ =\ \{!!\}\ --\ use\ \ \ \AgdaUnderscore{}∎p}\<%
\\
\>[0]\AgdaComment{hoarTripleNonActiveIfStackIgnored\ ifStack₁\ nonactive\ (x\ ∷\ [])\ nonIf\ φ\ =\ \{!!\}\ --\ 1\ element\ case}\<%
\\
\>[0]\AgdaComment{hoarTripleNonActiveIfStackIgnored\ ifStack₁\ nonactive\ (x\ ∷\ x₁\ ∷\ prog)\ nonIf\ φ\ =\ \{!!\}\ \ --lemmaNonActiveIfStackHoareTriple'\ ifStack₁\ nonactive\ prog\ nonIf\ φ}\<%
\\
\>[0]\<%
\\
\>[0]\AgdaComment{test\ =\ lemmaNonActiveIfStackHoareTriple'}\<%
\\
\>[0]\AgdaComment{-\}}\<%
\\
%
\\[\AgdaEmptyExtraSkip]%
\>[0]\AgdaComment{--\ Idea\ of\ proof:\ it\ is\ similar\ to}\<%
\\
\>[0]\AgdaComment{--\ lemmaP2PKHwithNonActiveIfStack}\<%
\\
\>[0]\AgdaComment{--\ in\ verificationP2PKHwithIfStackindexedPart4.agda}\<%
\\
\>[0]\AgdaComment{--\ Make\ use\ of\ lemmaNonActiveIfStackHoareTriple}\<%
\\
\>[0]\AgdaComment{--\ which\ proves\ the\ theorem\ for\ single\ instructions}\<%
\end{code}
} % END AgdaHide


==> latex/paperTypes2021PostProceed/stackVerificationP2PKHsymbolicExecutionPaperVersionPart2.tex <==
%% This file has been generated automatically by mkLagda.awk
%% DO NOT EDIT! ALL YOUR CHANGES WILL BE LOST!

\AgdaHide{
\begin{code}%
\>[0]\AgdaComment{--\ \textbackslash{}stackVerificationPtoPKHsymbolicExecutionPartTwo}\<%
\\
\>[0]\AgdaKeyword{open}\AgdaSpace{}%
\AgdaKeyword{import}\AgdaSpace{}%
\AgdaModule{basicBitcoinDataType}\<%
\\
%
\\[\AgdaEmptyExtraSkip]%
\>[0]\AgdaKeyword{module}\AgdaSpace{}%
\AgdaModule{paperTypes2021PostProceed.stackVerificationP2PKHsymbolicExecutionPaperVersionPart2}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaBound{param}\AgdaSpace{}%
\AgdaSymbol{:}\AgdaSpace{}%
\AgdaRecord{GlobalParameters}\AgdaSymbol{)}%
\>[118]\AgdaKeyword{where}\<%
\\
%
\\[\AgdaEmptyExtraSkip]%
\>[0]\AgdaKeyword{open}\AgdaSpace{}%
\AgdaKeyword{import}\AgdaSpace{}%
\AgdaModule{Data.Nat}%
\>[22]\AgdaKeyword{hiding}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaOperator{\AgdaDatatype{\AgdaUnderscore{}≤\AgdaUnderscore{}}}\AgdaSymbol{)}\<%
\\
\>[0]\AgdaKeyword{open}\AgdaSpace{}%
\AgdaKeyword{import}\AgdaSpace{}%
\AgdaModule{Data.List}\AgdaSpace{}%
\AgdaKeyword{hiding}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaOperator{\AgdaFunction{\AgdaUnderscore{}\ensuremath{+\!\!+}\AgdaUnderscore{}}}\AgdaSymbol{)}\<%
\\
\>[0]\AgdaKeyword{open}\AgdaSpace{}%
\AgdaKeyword{import}\AgdaSpace{}%
\AgdaModule{Data.Unit}%
\>[23]\AgdaKeyword{hiding}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaOperator{\AgdaRecord{\AgdaUnderscore{}≤\AgdaUnderscore{}}}\AgdaSymbol{)}\<%
\\
\>[0]\AgdaKeyword{open}\AgdaSpace{}%
\AgdaKeyword{import}\AgdaSpace{}%
\AgdaModule{Data.Empty}\<%
\\
\>[0]\AgdaKeyword{open}\AgdaSpace{}%
\AgdaKeyword{import}\AgdaSpace{}%
\AgdaModule{Data.Sum}\<%
\\
\>[0]\AgdaKeyword{open}\AgdaSpace{}%
\AgdaKeyword{import}\AgdaSpace{}%
\AgdaModule{Data.Bool}%
\>[23]\AgdaKeyword{hiding}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaOperator{\AgdaDatatype{\AgdaUnderscore{}≤\AgdaUnderscore{}}}\AgdaSpace{}%
\AgdaSymbol{;}\AgdaSpace{}%
\AgdaOperator{\AgdaFunction{if\AgdaUnderscore{}then\AgdaUnderscore{}else\AgdaUnderscore{}}}\AgdaSpace{}%
\AgdaSymbol{)}\AgdaSpace{}%
\AgdaKeyword{renaming}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaOperator{\AgdaFunction{\AgdaUnderscore{}∧\AgdaUnderscore{}}}\AgdaSpace{}%
\AgdaSymbol{to}\AgdaSpace{}%
\AgdaOperator{\AgdaFunction{\AgdaUnderscore{}∧b\AgdaUnderscore{}}}\AgdaSpace{}%
\AgdaSymbol{;}\AgdaSpace{}%
\AgdaOperator{\AgdaFunction{\AgdaUnderscore{}∨\AgdaUnderscore{}}}\AgdaSpace{}%
\AgdaSymbol{to}\AgdaSpace{}%
\AgdaOperator{\AgdaFunction{\AgdaUnderscore{}∨b\AgdaUnderscore{}}}\AgdaSpace{}%
\AgdaSymbol{;}\AgdaSpace{}%
\AgdaFunction{T}\AgdaSpace{}%
\AgdaSymbol{to}\AgdaSpace{}%
\AgdaFunction{True}\AgdaSymbol{)}\<%
\\
\>[0]\AgdaKeyword{open}\AgdaSpace{}%
\AgdaKeyword{import}\AgdaSpace{}%
\AgdaModule{Data.Product}\AgdaSpace{}%
\AgdaKeyword{renaming}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaOperator{\AgdaInductiveConstructor{\AgdaUnderscore{},\AgdaUnderscore{}}}\AgdaSpace{}%
\AgdaSymbol{to}\AgdaSpace{}%
\AgdaOperator{\AgdaInductiveConstructor{\AgdaUnderscore{},,\AgdaUnderscore{}}}\AgdaSpace{}%
\AgdaSymbol{)}\<%
\\
\>[0]\AgdaKeyword{open}\AgdaSpace{}%
\AgdaKeyword{import}\AgdaSpace{}%
\AgdaModule{Data.Nat.Base}\AgdaSpace{}%
\AgdaKeyword{hiding}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaOperator{\AgdaDatatype{\AgdaUnderscore{}≤\AgdaUnderscore{}}}\AgdaSymbol{)}\<%
\\
\>[0]\AgdaKeyword{open}\AgdaSpace{}%
\AgdaKeyword{import}\AgdaSpace{}%
\AgdaModule{Data.List.NonEmpty}\AgdaSpace{}%
\AgdaKeyword{hiding}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaField{head}\AgdaSpace{}%
\AgdaSymbol{;}\AgdaSpace{}%
\AgdaOperator{\AgdaFunction{[\AgdaUnderscore{}]}}\AgdaSpace{}%
\AgdaSymbol{)}\<%
\\
\>[0]\AgdaKeyword{open}\AgdaSpace{}%
\AgdaKeyword{import}\AgdaSpace{}%
\AgdaModule{Data.Maybe}\<%
\\
\>[0]\AgdaKeyword{open}\AgdaSpace{}%
\AgdaKeyword{import}\AgdaSpace{}%
\AgdaModule{Relation.Nullary}\<%
\\
%
\\[\AgdaEmptyExtraSkip]%
\>[0]\AgdaKeyword{import}\AgdaSpace{}%
\AgdaModule{Relation.Binary.PropositionalEquality}\AgdaSpace{}%
\AgdaSymbol{as}\AgdaSpace{}%
\AgdaModule{Eq}\<%
\\
\>[0]\AgdaKeyword{open}\AgdaSpace{}%
\AgdaModule{Eq}\AgdaSpace{}%
\AgdaKeyword{using}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaOperator{\AgdaDatatype{\AgdaUnderscore{}≡\AgdaUnderscore{}}}\AgdaSymbol{;}\AgdaSpace{}%
\AgdaInductiveConstructor{refl}\AgdaSymbol{;}\AgdaSpace{}%
\AgdaFunction{cong}\AgdaSymbol{;}\AgdaSpace{}%
\AgdaKeyword{module}\AgdaSpace{}%
\AgdaModule{≡-Reasoning}\AgdaSymbol{;}\AgdaSpace{}%
\AgdaFunction{sym}\AgdaSymbol{)}\<%
\\
\>[0]\AgdaKeyword{open}\AgdaSpace{}%
\AgdaModule{≡-Reasoning}\<%
\\
\>[0]\AgdaKeyword{open}\AgdaSpace{}%
\AgdaKeyword{import}\AgdaSpace{}%
\AgdaModule{Agda.Builtin.Equality}\<%
\\
%
\\[\AgdaEmptyExtraSkip]%
%
\\[\AgdaEmptyExtraSkip]%
\>[0]\AgdaComment{--our\ libraries}\<%
\\
\>[0]\AgdaKeyword{open}\AgdaSpace{}%
\AgdaKeyword{import}\AgdaSpace{}%
\AgdaModule{libraries.listLib}\<%
\\
\>[0]\AgdaKeyword{open}\AgdaSpace{}%
\AgdaKeyword{import}\AgdaSpace{}%
\AgdaModule{libraries.equalityLib}\<%
\\
\>[0]\AgdaKeyword{open}\AgdaSpace{}%
\AgdaKeyword{import}\AgdaSpace{}%
\AgdaModule{libraries.natLib}\<%
\\
\>[0]\AgdaKeyword{open}\AgdaSpace{}%
\AgdaKeyword{import}\AgdaSpace{}%
\AgdaModule{libraries.boolLib}\<%
\\
\>[0]\AgdaKeyword{open}\AgdaSpace{}%
\AgdaKeyword{import}\AgdaSpace{}%
\AgdaModule{libraries.emptyLib}\<%
\\
\>[0]\AgdaKeyword{open}\AgdaSpace{}%
\AgdaKeyword{import}\AgdaSpace{}%
\AgdaModule{libraries.andLib}\<%
\\
\>[0]\AgdaKeyword{open}\AgdaSpace{}%
\AgdaKeyword{import}\AgdaSpace{}%
\AgdaModule{libraries.miscLib}\<%
\\
\>[0]\AgdaKeyword{open}\AgdaSpace{}%
\AgdaKeyword{import}\AgdaSpace{}%
\AgdaModule{libraries.maybeLib}\<%
\\
%
\\[\AgdaEmptyExtraSkip]%
\>[0]\AgdaKeyword{open}\AgdaSpace{}%
\AgdaKeyword{import}\AgdaSpace{}%
\AgdaModule{stack}\<%
\\
\>[0]\AgdaKeyword{open}\AgdaSpace{}%
\AgdaKeyword{import}\AgdaSpace{}%
\AgdaModule{stackPredicate}\<%
\\
\>[0]\AgdaKeyword{open}\AgdaSpace{}%
\AgdaKeyword{import}\AgdaSpace{}%
\AgdaModule{semanticBasicOperations}\AgdaSpace{}%
\AgdaBound{param}\<%
\\
\>[0]\AgdaKeyword{open}\AgdaSpace{}%
\AgdaKeyword{import}\AgdaSpace{}%
\AgdaModule{hoareTripleStack}\AgdaSpace{}%
\AgdaBound{param}\<%
\\
\>[0]\AgdaKeyword{open}\AgdaSpace{}%
\AgdaKeyword{import}\AgdaSpace{}%
\AgdaModule{instruction}\<%
\\
\>[0]\AgdaKeyword{open}\AgdaSpace{}%
\AgdaKeyword{import}\AgdaSpace{}%
\AgdaModule{verificationStackScripts.stackState}\<%
\\
\>[0]\AgdaKeyword{open}\AgdaSpace{}%
\AgdaKeyword{import}\AgdaSpace{}%
\AgdaModule{verificationStackScripts.sPredicate}\<%
\\
\>[0]\AgdaKeyword{open}\AgdaSpace{}%
\AgdaKeyword{import}\AgdaSpace{}%
\AgdaModule{verificationStackScripts.stackHoareTriple}\AgdaSpace{}%
\AgdaBound{param}\<%
\\
\>[0]\AgdaKeyword{open}\AgdaSpace{}%
\AgdaKeyword{import}\AgdaSpace{}%
\AgdaModule{verificationStackScripts.stackVerificationLemmas}\AgdaSpace{}%
\AgdaBound{param}\<%
\\
\>[0]\AgdaKeyword{open}\AgdaSpace{}%
\AgdaKeyword{import}\AgdaSpace{}%
\AgdaModule{verificationStackScripts.stackSemanticsInstructionsBasic}\AgdaSpace{}%
\AgdaBound{param}\<%
\\
\>[0]\AgdaKeyword{open}\AgdaSpace{}%
\AgdaKeyword{import}\AgdaSpace{}%
\AgdaModule{verificationStackScripts.semanticsStackInstructions}\AgdaSpace{}%
\AgdaBound{param}\<%
\\
\>[0]\AgdaKeyword{open}\AgdaSpace{}%
\AgdaKeyword{import}\AgdaSpace{}%
\AgdaModule{verificationStackScripts.stackVerificationP2PKH}\AgdaSpace{}%
\AgdaBound{param}\<%
\\
\>[0]\AgdaKeyword{open}\AgdaSpace{}%
\AgdaKeyword{import}\AgdaSpace{}%
\AgdaModule{verificationStackScripts.stackVerificationP2PKHindexed}\AgdaSpace{}%
\AgdaBound{param}\<%
\\
\>[0]\AgdaKeyword{open}\AgdaSpace{}%
\AgdaKeyword{import}\AgdaSpace{}%
\AgdaModule{verificationStackScripts.stackVerificationP2PKHindexed}\AgdaSpace{}%
\AgdaBound{param}\<%
\\
\>[0]\AgdaKeyword{open}\AgdaSpace{}%
\AgdaKeyword{import}\AgdaSpace{}%
\AgdaModule{paperTypes2021PostProceed.stackVerificationP2PKHsymbolicExecutionPaperVersion}\AgdaSpace{}%
\AgdaBound{param}\<%
\\
%
\\[\AgdaEmptyExtraSkip]%
%
\\[\AgdaEmptyExtraSkip]%
\>[0]\AgdaComment{-------------------------------------------}\<%
\\
\>[0]\AgdaComment{--\ \ Currently\ empty}\<%
\\
\>[0]\AgdaComment{--}\<%
\\
\>[0]\AgdaComment{--\ \ Used\ to\ work\ independently\ on\ that\ part}\<%
\\
\>[0]\AgdaComment{--\ \ To\ be\ kept\ until\ paper\ is\ finished}\<%
\\
\>[0]\AgdaComment{----------------------------------------------}\<%
\end{code}
} % END AgdaHide


==> latex/verificationWithIfStack/hoareTripleStackScript.tex <==
%% This file has been generated automatically by mkLagda.awk
%% DO NOT EDIT! ALL YOUR CHANGES WILL BE LOST!

\AgdaHide{
\begin{code}%
\>[0]\AgdaKeyword{open}\AgdaSpace{}%
\AgdaKeyword{import}\AgdaSpace{}%
\AgdaModule{basicBitcoinDataType}\<%
\\
%
\\[\AgdaEmptyExtraSkip]%
\>[0]\AgdaKeyword{module}\AgdaSpace{}%
\AgdaModule{verificationWithIfStack.hoareTripleStackScript}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaBound{param}\AgdaSpace{}%
\AgdaSymbol{:}\AgdaSpace{}%
\AgdaRecord{GlobalParameters}\AgdaSymbol{)}\AgdaSpace{}%
\AgdaKeyword{where}\<%
\\
%
\\[\AgdaEmptyExtraSkip]%
%
\\[\AgdaEmptyExtraSkip]%
\>[0]\AgdaKeyword{open}\AgdaSpace{}%
\AgdaKeyword{import}\AgdaSpace{}%
\AgdaModule{Data.List.Base}\AgdaSpace{}%
\AgdaKeyword{hiding}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaOperator{\AgdaFunction{\AgdaUnderscore{}\ensuremath{+\!\!+}\AgdaUnderscore{}}}\AgdaSymbol{)}\<%
\\
\>[0]\AgdaKeyword{open}\AgdaSpace{}%
\AgdaKeyword{import}\AgdaSpace{}%
\AgdaModule{Data.Nat}%
\>[22]\AgdaKeyword{renaming}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaOperator{\AgdaDatatype{\AgdaUnderscore{}≤\AgdaUnderscore{}}}\AgdaSpace{}%
\AgdaSymbol{to}\AgdaSpace{}%
\AgdaOperator{\AgdaDatatype{\AgdaUnderscore{}≤'\AgdaUnderscore{}}}\AgdaSpace{}%
\AgdaSymbol{;}\AgdaSpace{}%
\AgdaOperator{\AgdaFunction{\AgdaUnderscore{}<\AgdaUnderscore{}}}\AgdaSpace{}%
\AgdaSymbol{to}\AgdaSpace{}%
\AgdaOperator{\AgdaFunction{\AgdaUnderscore{}<'\AgdaUnderscore{}}}\AgdaSymbol{)}\<%
\\
\>[0]\AgdaKeyword{open}\AgdaSpace{}%
\AgdaKeyword{import}\AgdaSpace{}%
\AgdaModule{Data.List}\AgdaSpace{}%
\AgdaKeyword{hiding}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaOperator{\AgdaFunction{\AgdaUnderscore{}\ensuremath{+\!\!+}\AgdaUnderscore{}}}\AgdaSymbol{)}\<%
\\
\>[0]\AgdaKeyword{open}\AgdaSpace{}%
\AgdaKeyword{import}\AgdaSpace{}%
\AgdaModule{Data.Sum}\<%
\\
\>[0]\AgdaKeyword{open}\AgdaSpace{}%
\AgdaKeyword{import}\AgdaSpace{}%
\AgdaModule{Data.Unit}%
\>[23]\AgdaKeyword{hiding}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaOperator{\AgdaRecord{\AgdaUnderscore{}≤\AgdaUnderscore{}}}\AgdaSymbol{)}\<%
\\
\>[0]\AgdaKeyword{open}\AgdaSpace{}%
\AgdaKeyword{import}\AgdaSpace{}%
\AgdaModule{Data.Empty}\<%
\\
\>[0]\AgdaKeyword{open}\AgdaSpace{}%
\AgdaKeyword{import}\AgdaSpace{}%
\AgdaModule{Data.Maybe}\<%
\\
\>[0]\AgdaKeyword{open}\AgdaSpace{}%
\AgdaKeyword{import}\AgdaSpace{}%
\AgdaModule{Data.Bool}%
\>[23]\AgdaKeyword{hiding}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaOperator{\AgdaDatatype{\AgdaUnderscore{}≤\AgdaUnderscore{}}}\AgdaSpace{}%
\AgdaSymbol{;}\AgdaSpace{}%
\AgdaOperator{\AgdaDatatype{\AgdaUnderscore{}<\AgdaUnderscore{}}}\AgdaSpace{}%
\AgdaSymbol{;}\AgdaSpace{}%
\AgdaOperator{\AgdaFunction{if\AgdaUnderscore{}then\AgdaUnderscore{}else\AgdaUnderscore{}}}%
\>[58]\AgdaSymbol{)}%
\>[61]\AgdaKeyword{renaming}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaOperator{\AgdaFunction{\AgdaUnderscore{}∧\AgdaUnderscore{}}}\AgdaSpace{}%
\AgdaSymbol{to}\AgdaSpace{}%
\AgdaOperator{\AgdaFunction{\AgdaUnderscore{}∧b\AgdaUnderscore{}}}\AgdaSpace{}%
\AgdaSymbol{;}\AgdaSpace{}%
\AgdaOperator{\AgdaFunction{\AgdaUnderscore{}∨\AgdaUnderscore{}}}\AgdaSpace{}%
\AgdaSymbol{to}\AgdaSpace{}%
\AgdaOperator{\AgdaFunction{\AgdaUnderscore{}∨b\AgdaUnderscore{}}}\AgdaSpace{}%
\AgdaSymbol{;}\AgdaSpace{}%
\AgdaFunction{T}\AgdaSpace{}%
\AgdaSymbol{to}\AgdaSpace{}%
\AgdaFunction{True}\AgdaSymbol{)}\<%
\\
\>[0]\AgdaKeyword{open}\AgdaSpace{}%
\AgdaKeyword{import}\AgdaSpace{}%
\AgdaModule{Data.Product}\AgdaSpace{}%
\AgdaKeyword{renaming}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaOperator{\AgdaInductiveConstructor{\AgdaUnderscore{},\AgdaUnderscore{}}}\AgdaSpace{}%
\AgdaSymbol{to}\AgdaSpace{}%
\AgdaOperator{\AgdaInductiveConstructor{\AgdaUnderscore{},,\AgdaUnderscore{}}}\AgdaSpace{}%
\AgdaSymbol{)}\<%
\\
\>[0]\AgdaKeyword{open}\AgdaSpace{}%
\AgdaKeyword{import}\AgdaSpace{}%
\AgdaModule{Data.Nat.Base}\AgdaSpace{}%
\AgdaKeyword{hiding}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaOperator{\AgdaDatatype{\AgdaUnderscore{}≤\AgdaUnderscore{}}}\AgdaSpace{}%
\AgdaSymbol{;}\AgdaSpace{}%
\AgdaOperator{\AgdaFunction{\AgdaUnderscore{}<\AgdaUnderscore{}}}\AgdaSymbol{)}\<%
\\
\>[0]\AgdaKeyword{open}\AgdaSpace{}%
\AgdaKeyword{import}\AgdaSpace{}%
\AgdaModule{Data.List.NonEmpty}\AgdaSpace{}%
\AgdaKeyword{hiding}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaField{head}\AgdaSymbol{)}\<%
\\
\>[0]\AgdaKeyword{open}\AgdaSpace{}%
\AgdaKeyword{import}\AgdaSpace{}%
\AgdaModule{Data.Nat}\AgdaSpace{}%
\AgdaKeyword{using}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaDatatype{ℕ}\AgdaSymbol{;}\AgdaSpace{}%
\AgdaOperator{\AgdaPrimitive{\AgdaUnderscore{}+\AgdaUnderscore{}}}\AgdaSymbol{;}\AgdaSpace{}%
\AgdaOperator{\AgdaFunction{\AgdaUnderscore{}≥\AgdaUnderscore{}}}\AgdaSymbol{;}\AgdaSpace{}%
\AgdaOperator{\AgdaFunction{\AgdaUnderscore{}>\AgdaUnderscore{}}}\AgdaSymbol{;}\AgdaSpace{}%
\AgdaInductiveConstructor{zero}\AgdaSymbol{;}\AgdaSpace{}%
\AgdaInductiveConstructor{suc}\AgdaSymbol{;}\AgdaSpace{}%
\AgdaInductiveConstructor{s≤s}\AgdaSymbol{;}\AgdaSpace{}%
\AgdaInductiveConstructor{z≤n}\AgdaSymbol{)}\<%
\\
\>[0]\AgdaKeyword{import}\AgdaSpace{}%
\AgdaModule{Relation.Binary.PropositionalEquality}\AgdaSpace{}%
\AgdaSymbol{as}\AgdaSpace{}%
\AgdaModule{Eq}\<%
\\
\>[0]\AgdaKeyword{open}\AgdaSpace{}%
\AgdaModule{Eq}\AgdaSpace{}%
\AgdaKeyword{using}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaOperator{\AgdaDatatype{\AgdaUnderscore{}≡\AgdaUnderscore{}}}\AgdaSymbol{;}\AgdaSpace{}%
\AgdaInductiveConstructor{refl}\AgdaSymbol{;}\AgdaSpace{}%
\AgdaFunction{cong}\AgdaSymbol{;}\AgdaSpace{}%
\AgdaKeyword{module}\AgdaSpace{}%
\AgdaModule{≡-Reasoning}\AgdaSymbol{;}\AgdaSpace{}%
\AgdaFunction{sym}\AgdaSymbol{)}\<%
\\
\>[0]\AgdaKeyword{open}\AgdaSpace{}%
\AgdaModule{≡-Reasoning}\<%
\\
\>[0]\AgdaKeyword{open}\AgdaSpace{}%
\AgdaKeyword{import}\AgdaSpace{}%
\AgdaModule{Agda.Builtin.Equality}\<%
\\
\>[0]\AgdaComment{--open\ import\ Agda.Builtin.Equality.Rewrite}\<%
\\
%
\\[\AgdaEmptyExtraSkip]%
\>[0]\AgdaKeyword{open}\AgdaSpace{}%
\AgdaKeyword{import}\AgdaSpace{}%
\AgdaModule{libraries.listLib}\<%
\\
\>[0]\AgdaKeyword{open}\AgdaSpace{}%
\AgdaKeyword{import}\AgdaSpace{}%
\AgdaModule{libraries.emptyLib}\<%
\\
\>[0]\AgdaKeyword{open}\AgdaSpace{}%
\AgdaKeyword{import}\AgdaSpace{}%
\AgdaModule{libraries.natLib}\<%
\\
\>[0]\AgdaKeyword{open}\AgdaSpace{}%
\AgdaKeyword{import}\AgdaSpace{}%
\AgdaModule{libraries.boolLib}\<%
\\
\>[0]\AgdaKeyword{open}\AgdaSpace{}%
\AgdaKeyword{import}\AgdaSpace{}%
\AgdaModule{libraries.equalityLib}\<%
\\
\>[0]\AgdaKeyword{open}\AgdaSpace{}%
\AgdaKeyword{import}\AgdaSpace{}%
\AgdaModule{libraries.andLib}\<%
\\
\>[0]\AgdaKeyword{open}\AgdaSpace{}%
\AgdaKeyword{import}\AgdaSpace{}%
\AgdaModule{libraries.miscLib}\<%
\\
\>[0]\AgdaKeyword{open}\AgdaSpace{}%
\AgdaKeyword{import}\AgdaSpace{}%
\AgdaModule{libraries.maybeLib}\<%
\\
%
\\[\AgdaEmptyExtraSkip]%
\>[0]\AgdaKeyword{open}\AgdaSpace{}%
\AgdaKeyword{import}\AgdaSpace{}%
\AgdaModule{stack}\<%
\\
\>[0]\AgdaKeyword{open}\AgdaSpace{}%
\AgdaKeyword{import}\AgdaSpace{}%
\AgdaModule{stackPredicate}\<%
\\
\>[0]\AgdaKeyword{open}\AgdaSpace{}%
\AgdaKeyword{import}\AgdaSpace{}%
\AgdaModule{instruction}\<%
\\
\>[0]\AgdaComment{--\ open\ import\ ledger\ param}\<%
\\
\>[0]\AgdaKeyword{open}\AgdaSpace{}%
\AgdaKeyword{import}\AgdaSpace{}%
\AgdaModule{stackSemanticsInstructions}\AgdaSpace{}%
\AgdaBound{param}\<%
\\
\>[0]\AgdaKeyword{open}\AgdaSpace{}%
\AgdaKeyword{import}\AgdaSpace{}%
\AgdaModule{hoareTripleStack}\AgdaSpace{}%
\AgdaBound{param}\<%
\\
%
\\[\AgdaEmptyExtraSkip]%
\>[0]\AgdaKeyword{open}\AgdaSpace{}%
\AgdaKeyword{import}\AgdaSpace{}%
\AgdaModule{verificationWithIfStack.ifStack}\<%
\\
\>[0]\AgdaKeyword{open}\AgdaSpace{}%
\AgdaKeyword{import}\AgdaSpace{}%
\AgdaModule{verificationWithIfStack.state}\<%
\\
\>[0]\AgdaKeyword{open}\AgdaSpace{}%
\AgdaKeyword{import}\AgdaSpace{}%
\AgdaModule{verificationWithIfStack.predicate}\<%
\\
\>[0]\AgdaKeyword{open}\AgdaSpace{}%
\AgdaKeyword{import}\AgdaSpace{}%
\AgdaModule{verificationWithIfStack.semanticsInstructions}\AgdaSpace{}%
\AgdaBound{param}\<%
\\
\>[0]\AgdaKeyword{open}\AgdaSpace{}%
\AgdaKeyword{import}\AgdaSpace{}%
\AgdaModule{verificationWithIfStack.stackSemanticsInstructionsLemma}\AgdaSpace{}%
\AgdaBound{param}\<%
\\
\>[0]\AgdaKeyword{open}\AgdaSpace{}%
\AgdaKeyword{import}\AgdaSpace{}%
\AgdaModule{verificationWithIfStack.verificationLemmas}\AgdaSpace{}%
\AgdaBound{param}\<%
\\
\>[0]\AgdaKeyword{open}\AgdaSpace{}%
\AgdaKeyword{import}\AgdaSpace{}%
\AgdaModule{verificationWithIfStack.hoareTriple}\AgdaSpace{}%
\AgdaBound{param}\<%
\\
\>[0]\AgdaKeyword{open}\AgdaSpace{}%
\AgdaKeyword{import}\AgdaSpace{}%
\AgdaModule{verificationWithIfStack.hoareTripleStack2HoareTriple}\AgdaSpace{}%
\AgdaBound{param}\<%
\\
%
\\[\AgdaEmptyExtraSkip]%
\>[0]\AgdaComment{--\ open\ import\ verificationWithIfStack.verificationP2PKH}\<%
\\
\>[0]\AgdaComment{--\ open\ import\ verificationWithIfStack.ifThenElseTheoremPart1\ param}\<%
\\
\>[0]\AgdaComment{--\ open\ import\ verificationWithIfStack.ifThenElseTheoremPart2\ param}\<%
\\
\>[0]\AgdaComment{--\ open\ import\ verificationWithIfStack.ifThenElseTheoremPart3\ param}\<%
\\
\>[0]\AgdaComment{--\ open\ import\ verificationWithIfStack.ifThenElseTheoremPart4\ param}\<%
\\
%
\\[\AgdaEmptyExtraSkip]%
\>[0]\AgdaKeyword{open}\AgdaSpace{}%
\AgdaKeyword{import}\AgdaSpace{}%
\AgdaModule{verificationWithIfStack.hoareTripleStackNonActiveIfStack}\AgdaSpace{}%
\AgdaBound{param}\<%
\\
%
\\[\AgdaEmptyExtraSkip]%
%
\\[\AgdaEmptyExtraSkip]%
%
\\[\AgdaEmptyExtraSkip]%
%
\\[\AgdaEmptyExtraSkip]%
%
\\[\AgdaEmptyExtraSkip]%
\>[0]\AgdaFunction{lemmaStackSemIsSemScriptaux2}%
\>[145I]\AgdaSymbol{:}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaBound{g'}\AgdaSpace{}%
\AgdaSymbol{:}\AgdaSpace{}%
\AgdaFunction{Time}\AgdaSpace{}%
\AgdaSymbol{→}\AgdaSpace{}%
\AgdaDatatype{Msg}\AgdaSpace{}%
\AgdaSymbol{→}\AgdaSpace{}%
\AgdaFunction{Stack}\AgdaSpace{}%
\AgdaSymbol{→}\AgdaSpace{}%
\AgdaDatatype{Maybe}\AgdaSpace{}%
\AgdaFunction{Stack}\AgdaSymbol{)}\<%
\\
\>[.][@{}l@{}]\<[145I]%
\>[29]\AgdaSymbol{(}\AgdaBound{st}\AgdaSpace{}%
\AgdaSymbol{:}\AgdaSpace{}%
\AgdaRecord{State}\AgdaSymbol{)}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaBound{mst}\AgdaSpace{}%
\AgdaSymbol{:}\AgdaSpace{}%
\AgdaDatatype{Maybe}\AgdaSpace{}%
\AgdaFunction{Stack}\AgdaSymbol{)}\<%
\\
\>[0][@{}l@{\AgdaIndent{0}}]%
\>[3]\AgdaSymbol{→}%
\>[162I]\AgdaSymbol{(}\AgdaFunction{exeTransformerDepIfStack'}%
\>[33]\AgdaSymbol{(}\AgdaFunction{liftStackToStateTransformerAux'}\AgdaSpace{}%
\AgdaBound{mst}\AgdaSpace{}%
\AgdaSymbol{)}%
\>[73]\AgdaBound{st}\<%
\\
\>[162I][@{}l@{\AgdaIndent{0}}]%
\>[7]\AgdaOperator{\AgdaFunction{\ensuremath{\mathbin{{>}\mkern-8.5mu{>}\mkern-2mu{=}}}}}\AgdaSpace{}%
\AgdaSymbol{λ}\AgdaSpace{}%
\AgdaBound{s}\AgdaSpace{}%
\AgdaSymbol{→}%
\>[18]\AgdaFunction{exeTransformerDepIfStack'}\<%
\\
\>[18][@{}l@{\AgdaIndent{0}}]%
\>[20]\AgdaSymbol{(}\AgdaFunction{liftStackToStateTransformerAux'}\<%
\\
%
\>[20]\AgdaSymbol{(}\AgdaBound{g'}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaBound{s}\AgdaSpace{}%
\AgdaSymbol{.}\AgdaField{currentTime}\AgdaSymbol{)}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaBound{s}\AgdaSpace{}%
\AgdaSymbol{.}\AgdaField{msg}\AgdaSymbol{)}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaBound{s}\AgdaSpace{}%
\AgdaSymbol{.}\AgdaField{stack}\AgdaSymbol{)))}\AgdaSpace{}%
\AgdaBound{s}\AgdaSymbol{)}\<%
\\
%
\\[\AgdaEmptyExtraSkip]%
\>[162I][@{}l@{\AgdaIndent{0}}]%
\>[6]\AgdaOperator{\AgdaDatatype{≡}}\<%
\\
%
\>[6]\AgdaFunction{exeTransformerDepIfStack'}%
\>[33]\AgdaSymbol{(}\AgdaFunction{liftStackToStateTransformerAux'}\<%
\\
\>[6][@{}l@{\AgdaIndent{0}}]%
\>[13]\AgdaSymbol{(}\AgdaBound{mst}\AgdaSpace{}%
\AgdaOperator{\AgdaFunction{\ensuremath{\mathbin{{>}\mkern-8.5mu{>}\mkern-2mu{=}}}}}\AgdaSpace{}%
\AgdaBound{g'}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaBound{st}\AgdaSpace{}%
\AgdaSymbol{.}\AgdaField{currentTime}\AgdaSymbol{)}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaBound{st}\AgdaSpace{}%
\AgdaSymbol{.}\AgdaField{msg}\AgdaSymbol{))}%
\>[55]\AgdaSymbol{)}\AgdaSpace{}%
\AgdaBound{st}\<%
\\
\>[0]\AgdaFunction{lemmaStackSemIsSemScriptaux2}\AgdaSpace{}%
\AgdaBound{g'}\AgdaSpace{}%
\AgdaOperator{\AgdaInductiveConstructor{⟨}}\AgdaSpace{}%
\AgdaBound{currentTime₁}\AgdaSpace{}%
\AgdaOperator{\AgdaInductiveConstructor{,}}\AgdaSpace{}%
\AgdaBound{msg₁}\AgdaSpace{}%
\AgdaOperator{\AgdaInductiveConstructor{,}}\AgdaSpace{}%
\AgdaBound{stack₁}\AgdaSpace{}%
\AgdaOperator{\AgdaInductiveConstructor{,}}\AgdaSpace{}%
\AgdaInductiveConstructor{[]}\AgdaSpace{}%
\AgdaOperator{\AgdaInductiveConstructor{,}}\AgdaSpace{}%
\AgdaBound{consis₁}\AgdaSpace{}%
\AgdaOperator{\AgdaInductiveConstructor{⟩}}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaInductiveConstructor{just}\AgdaSpace{}%
\AgdaBound{x}\AgdaSymbol{)}\AgdaSpace{}%
\AgdaSymbol{=}\AgdaSpace{}%
\AgdaInductiveConstructor{refl}\<%
\\
\>[0]\AgdaFunction{lemmaStackSemIsSemScriptaux2}\AgdaSpace{}%
\AgdaBound{g'}\AgdaSpace{}%
\AgdaOperator{\AgdaInductiveConstructor{⟨}}\AgdaSpace{}%
\AgdaBound{currentTime₁}\AgdaSpace{}%
\AgdaOperator{\AgdaInductiveConstructor{,}}\AgdaSpace{}%
\AgdaBound{msg₁}\AgdaSpace{}%
\AgdaOperator{\AgdaInductiveConstructor{,}}\AgdaSpace{}%
\AgdaBound{stack₁}\AgdaSpace{}%
\AgdaOperator{\AgdaInductiveConstructor{,}}\AgdaSpace{}%
\AgdaInductiveConstructor{ifCase}\AgdaSpace{}%
\AgdaOperator{\AgdaInductiveConstructor{∷}}\AgdaSpace{}%
\AgdaBound{ifStack₁}\AgdaSpace{}%
\AgdaOperator{\AgdaInductiveConstructor{,}}\AgdaSpace{}%
\AgdaBound{consis₁}\AgdaSpace{}%
\AgdaOperator{\AgdaInductiveConstructor{⟩}}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaInductiveConstructor{just}\AgdaSpace{}%
\AgdaBound{x}\AgdaSymbol{)}\AgdaSpace{}%
\AgdaSymbol{=}\AgdaSpace{}%
\AgdaInductiveConstructor{refl}\<%
\\
\>[0]\AgdaFunction{lemmaStackSemIsSemScriptaux2}\AgdaSpace{}%
\AgdaBound{g'}\AgdaSpace{}%
\AgdaOperator{\AgdaInductiveConstructor{⟨}}\AgdaSpace{}%
\AgdaBound{currentTime₁}\AgdaSpace{}%
\AgdaOperator{\AgdaInductiveConstructor{,}}\AgdaSpace{}%
\AgdaBound{msg₁}\AgdaSpace{}%
\AgdaOperator{\AgdaInductiveConstructor{,}}\AgdaSpace{}%
\AgdaBound{stack₁}\AgdaSpace{}%
\AgdaOperator{\AgdaInductiveConstructor{,}}\AgdaSpace{}%
\AgdaInductiveConstructor{elseCase}\AgdaSpace{}%
\AgdaOperator{\AgdaInductiveConstructor{∷}}\AgdaSpace{}%
\AgdaBound{ifStack₁}\AgdaSpace{}%
\AgdaOperator{\AgdaInductiveConstructor{,}}\AgdaSpace{}%
\AgdaBound{consis₁}\AgdaSpace{}%
\AgdaOperator{\AgdaInductiveConstructor{⟩}}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaInductiveConstructor{just}\AgdaSpace{}%
\AgdaBound{x}\AgdaSymbol{)}\AgdaSpace{}%
\AgdaSymbol{=}\AgdaSpace{}%
\AgdaInductiveConstructor{refl}\<%
\\
\>[0]\AgdaFunction{lemmaStackSemIsSemScriptaux2}\AgdaSpace{}%
\AgdaBound{g'}\AgdaSpace{}%
\AgdaOperator{\AgdaInductiveConstructor{⟨}}\AgdaSpace{}%
\AgdaBound{currentTime₁}\AgdaSpace{}%
\AgdaOperator{\AgdaInductiveConstructor{,}}\AgdaSpace{}%
\AgdaBound{msg₁}\AgdaSpace{}%
\AgdaOperator{\AgdaInductiveConstructor{,}}\AgdaSpace{}%
\AgdaBound{stack₁}\AgdaSpace{}%
\AgdaOperator{\AgdaInductiveConstructor{,}}\AgdaSpace{}%
\AgdaInductiveConstructor{ifSkip}\AgdaSpace{}%
\AgdaOperator{\AgdaInductiveConstructor{∷}}\AgdaSpace{}%
\AgdaBound{ifStack₁}\AgdaSpace{}%
\AgdaOperator{\AgdaInductiveConstructor{,}}\AgdaSpace{}%
\AgdaBound{consis₁}\AgdaSpace{}%
\AgdaOperator{\AgdaInductiveConstructor{⟩}}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaInductiveConstructor{just}\AgdaSpace{}%
\AgdaBound{x}\AgdaSymbol{)}\AgdaSpace{}%
\AgdaSymbol{=}\AgdaSpace{}%
\AgdaInductiveConstructor{refl}\<%
\\
\>[0]\AgdaFunction{lemmaStackSemIsSemScriptaux2}\AgdaSpace{}%
\AgdaBound{g'}\AgdaSpace{}%
\AgdaOperator{\AgdaInductiveConstructor{⟨}}\AgdaSpace{}%
\AgdaBound{currentTime₁}\AgdaSpace{}%
\AgdaOperator{\AgdaInductiveConstructor{,}}\AgdaSpace{}%
\AgdaBound{msg₁}\AgdaSpace{}%
\AgdaOperator{\AgdaInductiveConstructor{,}}\AgdaSpace{}%
\AgdaBound{stack₁}\AgdaSpace{}%
\AgdaOperator{\AgdaInductiveConstructor{,}}\AgdaSpace{}%
\AgdaInductiveConstructor{elseSkip}\AgdaSpace{}%
\AgdaOperator{\AgdaInductiveConstructor{∷}}\AgdaSpace{}%
\AgdaBound{ifStack₁}\AgdaSpace{}%
\AgdaOperator{\AgdaInductiveConstructor{,}}\AgdaSpace{}%
\AgdaBound{consis₁}\AgdaSpace{}%
\AgdaOperator{\AgdaInductiveConstructor{⟩}}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaInductiveConstructor{just}\AgdaSpace{}%
\AgdaBound{x}\AgdaSymbol{)}\AgdaSpace{}%
\AgdaSymbol{=}\AgdaSpace{}%
\AgdaInductiveConstructor{refl}\<%
\\
\>[0]\AgdaFunction{lemmaStackSemIsSemScriptaux2}\AgdaSpace{}%
\AgdaBound{g'}\AgdaSpace{}%
\AgdaOperator{\AgdaInductiveConstructor{⟨}}\AgdaSpace{}%
\AgdaBound{currentTime₁}\AgdaSpace{}%
\AgdaOperator{\AgdaInductiveConstructor{,}}\AgdaSpace{}%
\AgdaBound{msg₁}\AgdaSpace{}%
\AgdaOperator{\AgdaInductiveConstructor{,}}\AgdaSpace{}%
\AgdaBound{stack₁}\AgdaSpace{}%
\AgdaOperator{\AgdaInductiveConstructor{,}}\AgdaSpace{}%
\AgdaInductiveConstructor{ifIgnore}\AgdaSpace{}%
\AgdaOperator{\AgdaInductiveConstructor{∷}}\AgdaSpace{}%
\AgdaBound{ifStack₁}\AgdaSpace{}%
\AgdaOperator{\AgdaInductiveConstructor{,}}\AgdaSpace{}%
\AgdaBound{consis₁}\AgdaSpace{}%
\AgdaOperator{\AgdaInductiveConstructor{⟩}}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaInductiveConstructor{just}\AgdaSpace{}%
\AgdaBound{x}\AgdaSymbol{)}\AgdaSpace{}%
\AgdaSymbol{=}\AgdaSpace{}%
\AgdaInductiveConstructor{refl}\<%
\\
\>[0]\AgdaFunction{lemmaStackSemIsSemScriptaux2}\AgdaSpace{}%
\AgdaBound{g'}\AgdaSpace{}%
\AgdaOperator{\AgdaInductiveConstructor{⟨}}\AgdaSpace{}%
\AgdaBound{currentTime₁}\AgdaSpace{}%
\AgdaOperator{\AgdaInductiveConstructor{,}}\AgdaSpace{}%
\AgdaBound{msg₁}\AgdaSpace{}%
\AgdaOperator{\AgdaInductiveConstructor{,}}\AgdaSpace{}%
\AgdaBound{stack₁}\AgdaSpace{}%
\AgdaOperator{\AgdaInductiveConstructor{,}}\AgdaSpace{}%
\AgdaInductiveConstructor{[]}\AgdaSpace{}%
\AgdaOperator{\AgdaInductiveConstructor{,}}\AgdaSpace{}%
\AgdaBound{consis₁}\AgdaSpace{}%
\AgdaOperator{\AgdaInductiveConstructor{⟩}}\AgdaSpace{}%
\AgdaInductiveConstructor{nothing}\AgdaSpace{}%
\AgdaSymbol{=}\AgdaSpace{}%
\AgdaInductiveConstructor{refl}\<%
\\
\>[0]\AgdaFunction{lemmaStackSemIsSemScriptaux2}\AgdaSpace{}%
\AgdaBound{g'}\AgdaSpace{}%
\AgdaOperator{\AgdaInductiveConstructor{⟨}}\AgdaSpace{}%
\AgdaBound{currentTime₁}\AgdaSpace{}%
\AgdaOperator{\AgdaInductiveConstructor{,}}\AgdaSpace{}%
\AgdaBound{msg₁}\AgdaSpace{}%
\AgdaOperator{\AgdaInductiveConstructor{,}}\AgdaSpace{}%
\AgdaBound{stack₁}\AgdaSpace{}%
\AgdaOperator{\AgdaInductiveConstructor{,}}\AgdaSpace{}%
\AgdaInductiveConstructor{ifCase}\AgdaSpace{}%
\AgdaOperator{\AgdaInductiveConstructor{∷}}\AgdaSpace{}%
\AgdaBound{ifStack₁}\AgdaSpace{}%
\AgdaOperator{\AgdaInductiveConstructor{,}}\AgdaSpace{}%
\AgdaBound{consis₁}\AgdaSpace{}%
\AgdaOperator{\AgdaInductiveConstructor{⟩}}\AgdaSpace{}%
\AgdaInductiveConstructor{nothing}\AgdaSpace{}%
\AgdaSymbol{=}\AgdaSpace{}%
\AgdaInductiveConstructor{refl}\<%
\\
\>[0]\AgdaFunction{lemmaStackSemIsSemScriptaux2}\AgdaSpace{}%
\AgdaBound{g'}\AgdaSpace{}%
\AgdaOperator{\AgdaInductiveConstructor{⟨}}\AgdaSpace{}%
\AgdaBound{currentTime₁}\AgdaSpace{}%
\AgdaOperator{\AgdaInductiveConstructor{,}}\AgdaSpace{}%
\AgdaBound{msg₁}\AgdaSpace{}%
\AgdaOperator{\AgdaInductiveConstructor{,}}\AgdaSpace{}%
\AgdaBound{stack₁}\AgdaSpace{}%
\AgdaOperator{\AgdaInductiveConstructor{,}}\AgdaSpace{}%
\AgdaInductiveConstructor{elseCase}\AgdaSpace{}%
\AgdaOperator{\AgdaInductiveConstructor{∷}}\AgdaSpace{}%
\AgdaBound{ifStack₁}\AgdaSpace{}%
\AgdaOperator{\AgdaInductiveConstructor{,}}\AgdaSpace{}%
\AgdaBound{consis₁}\AgdaSpace{}%
\AgdaOperator{\AgdaInductiveConstructor{⟩}}\AgdaSpace{}%
\AgdaInductiveConstructor{nothing}\AgdaSpace{}%
\AgdaSymbol{=}\AgdaSpace{}%
\AgdaInductiveConstructor{refl}\<%
\\
\>[0]\AgdaFunction{lemmaStackSemIsSemScriptaux2}\AgdaSpace{}%
\AgdaBound{g'}\AgdaSpace{}%
\AgdaOperator{\AgdaInductiveConstructor{⟨}}\AgdaSpace{}%
\AgdaBound{currentTime₁}\AgdaSpace{}%
\AgdaOperator{\AgdaInductiveConstructor{,}}\AgdaSpace{}%
\AgdaBound{msg₁}\AgdaSpace{}%
\AgdaOperator{\AgdaInductiveConstructor{,}}\AgdaSpace{}%
\AgdaBound{stack₁}\AgdaSpace{}%
\AgdaOperator{\AgdaInductiveConstructor{,}}\AgdaSpace{}%
\AgdaInductiveConstructor{ifSkip}\AgdaSpace{}%
\AgdaOperator{\AgdaInductiveConstructor{∷}}\AgdaSpace{}%
\AgdaBound{ifStack₁}\AgdaSpace{}%
\AgdaOperator{\AgdaInductiveConstructor{,}}\AgdaSpace{}%
\AgdaBound{consis₁}\AgdaSpace{}%
\AgdaOperator{\AgdaInductiveConstructor{⟩}}\AgdaSpace{}%
\AgdaInductiveConstructor{nothing}\AgdaSpace{}%
\AgdaSymbol{=}\AgdaSpace{}%
\AgdaInductiveConstructor{refl}\<%
\\
\>[0]\AgdaFunction{lemmaStackSemIsSemScriptaux2}\AgdaSpace{}%
\AgdaBound{g'}\AgdaSpace{}%
\AgdaOperator{\AgdaInductiveConstructor{⟨}}\AgdaSpace{}%
\AgdaBound{currentTime₁}\AgdaSpace{}%
\AgdaOperator{\AgdaInductiveConstructor{,}}\AgdaSpace{}%
\AgdaBound{msg₁}\AgdaSpace{}%
\AgdaOperator{\AgdaInductiveConstructor{,}}\AgdaSpace{}%
\AgdaBound{stack₁}\AgdaSpace{}%
\AgdaOperator{\AgdaInductiveConstructor{,}}\AgdaSpace{}%
\AgdaInductiveConstructor{elseSkip}\AgdaSpace{}%
\AgdaOperator{\AgdaInductiveConstructor{∷}}\AgdaSpace{}%
\AgdaBound{ifStack₁}\AgdaSpace{}%
\AgdaOperator{\AgdaInductiveConstructor{,}}\AgdaSpace{}%
\AgdaBound{consis₁}\AgdaSpace{}%
\AgdaOperator{\AgdaInductiveConstructor{⟩}}\AgdaSpace{}%
\AgdaInductiveConstructor{nothing}\AgdaSpace{}%
\AgdaSymbol{=}\AgdaSpace{}%
\AgdaInductiveConstructor{refl}\<%
\\
\>[0]\AgdaFunction{lemmaStackSemIsSemScriptaux2}\AgdaSpace{}%
\AgdaBound{g'}\AgdaSpace{}%
\AgdaOperator{\AgdaInductiveConstructor{⟨}}\AgdaSpace{}%
\AgdaBound{currentTime₁}\AgdaSpace{}%
\AgdaOperator{\AgdaInductiveConstructor{,}}\AgdaSpace{}%
\AgdaBound{msg₁}\AgdaSpace{}%
\AgdaOperator{\AgdaInductiveConstructor{,}}\AgdaSpace{}%
\AgdaBound{stack₁}\AgdaSpace{}%
\AgdaOperator{\AgdaInductiveConstructor{,}}\AgdaSpace{}%
\AgdaInductiveConstructor{ifIgnore}\AgdaSpace{}%
\AgdaOperator{\AgdaInductiveConstructor{∷}}\AgdaSpace{}%
\AgdaBound{ifStack₁}\AgdaSpace{}%
\AgdaOperator{\AgdaInductiveConstructor{,}}\AgdaSpace{}%
\AgdaBound{consis₁}\AgdaSpace{}%
\AgdaOperator{\AgdaInductiveConstructor{⟩}}\AgdaSpace{}%
\AgdaInductiveConstructor{nothing}\AgdaSpace{}%
\AgdaSymbol{=}\AgdaSpace{}%
\AgdaInductiveConstructor{refl}\<%
\\
%
\\[\AgdaEmptyExtraSkip]%
%
\\[\AgdaEmptyExtraSkip]%
\>[0]\AgdaFunction{lemmaStackSemIsSemScriptaux}%
\>[388I]\AgdaSymbol{:}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaBound{\,f\,}\AgdaSpace{}%
\AgdaBound{g}\AgdaSpace{}%
\AgdaSymbol{:}\AgdaSpace{}%
\AgdaRecord{State}\AgdaSpace{}%
\AgdaSymbol{→}\AgdaSpace{}%
\AgdaDatatype{Maybe}\AgdaSpace{}%
\AgdaRecord{State}\AgdaSymbol{)}\<%
\\
\>[388I][@{}l@{\AgdaIndent{0}}]%
\>[29]\AgdaSymbol{(}\AgdaBound{f'}\AgdaSpace{}%
\AgdaBound{g'}\AgdaSpace{}%
\AgdaSymbol{:}\AgdaSpace{}%
\AgdaFunction{Time}\AgdaSpace{}%
\AgdaSymbol{→}\AgdaSpace{}%
\AgdaDatatype{Msg}\AgdaSpace{}%
\AgdaSymbol{→}\AgdaSpace{}%
\AgdaFunction{Stack}\AgdaSpace{}%
\AgdaSymbol{→}\AgdaSpace{}%
\AgdaDatatype{Maybe}\AgdaSpace{}%
\AgdaFunction{Stack}\AgdaSymbol{)}\<%
\\
%
\>[29]\AgdaSymbol{(}\AgdaBound{p}\AgdaSpace{}%
\AgdaSymbol{:}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaBound{s}\AgdaSpace{}%
\AgdaSymbol{:}\AgdaSpace{}%
\AgdaRecord{State}\AgdaSymbol{)}\AgdaSpace{}%
\AgdaSymbol{→}\AgdaSpace{}%
\AgdaBound{\,f\,}\AgdaSpace{}%
\AgdaBound{s}\AgdaSpace{}%
\AgdaOperator{\AgdaDatatype{≡}}\AgdaSpace{}%
\AgdaFunction{stackTransform2StateTransform}\AgdaSpace{}%
\AgdaBound{f'}\AgdaSpace{}%
\AgdaBound{s}\AgdaSymbol{)}\<%
\\
%
\>[29]\AgdaSymbol{(}\AgdaBound{q}\AgdaSpace{}%
\AgdaSymbol{:}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaBound{s}\AgdaSpace{}%
\AgdaSymbol{:}\AgdaSpace{}%
\AgdaRecord{State}\AgdaSymbol{)}\AgdaSpace{}%
\AgdaSymbol{→}\AgdaSpace{}%
\AgdaBound{g}\AgdaSpace{}%
\AgdaBound{s}\AgdaSpace{}%
\AgdaOperator{\AgdaDatatype{≡}}\AgdaSpace{}%
\AgdaFunction{stackTransform2StateTransform}\AgdaSpace{}%
\AgdaBound{g'}\AgdaSpace{}%
\AgdaBound{s}\AgdaSymbol{)}\<%
\\
%
\>[29]\AgdaSymbol{(}\AgdaBound{st}\AgdaSpace{}%
\AgdaSymbol{:}\AgdaSpace{}%
\AgdaRecord{State}\AgdaSymbol{)}\<%
\\
%
\>[29]\AgdaSymbol{→}\<%
\\
\>[0][@{}l@{\AgdaIndent{0}}]%
\>[14]\AgdaSymbol{(}\AgdaBound{\,f\,}\AgdaSpace{}%
\AgdaBound{st}\AgdaSpace{}%
\AgdaOperator{\AgdaFunction{\ensuremath{\mathbin{{>}\mkern-8.5mu{>}\mkern-2mu{=}}}}}\AgdaSpace{}%
\AgdaBound{g}\AgdaSymbol{)}%
\>[29]\AgdaOperator{\AgdaDatatype{≡}}%
\>[433I]\AgdaFunction{stackTransform2StateTransform}\<%
\\
\>[433I][@{}l@{\AgdaIndent{0}}]%
\>[35]\AgdaSymbol{(λ}\AgdaSpace{}%
\AgdaBound{time₁}\AgdaSpace{}%
\AgdaBound{msg}\AgdaSpace{}%
\AgdaBound{stack₁}\AgdaSpace{}%
\AgdaSymbol{→}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaBound{f'}\AgdaSpace{}%
\AgdaBound{time₁}\AgdaSpace{}%
\AgdaBound{msg}\AgdaSpace{}%
\AgdaBound{stack₁}\AgdaSpace{}%
\AgdaOperator{\AgdaFunction{\ensuremath{\mathbin{{>}\mkern-8.5mu{>}\mkern-2mu{=}}}}}\AgdaSpace{}%
\AgdaBound{g'}\AgdaSpace{}%
\AgdaBound{time₁}\AgdaSpace{}%
\AgdaBound{msg}\AgdaSymbol{)}\AgdaSpace{}%
\AgdaSymbol{)}\<%
\\
%
\>[35]\AgdaBound{st}\<%
\\
\>[0]\AgdaFunction{lemmaStackSemIsSemScriptaux}\AgdaSpace{}%
\AgdaBound{\,f\,}\AgdaSpace{}%
\AgdaBound{g}\AgdaSpace{}%
\AgdaBound{f'}\AgdaSpace{}%
\AgdaBound{g'}\AgdaSpace{}%
\AgdaBound{p}\AgdaSpace{}%
\AgdaBound{q}\AgdaSpace{}%
\AgdaBound{st}\AgdaSpace{}%
\AgdaSymbol{=}\<%
\\
\>[0][@{}l@{\AgdaIndent{0}}]%
\>[4]\AgdaSymbol{(}\AgdaBound{\,f\,}%
\>[455I]\AgdaBound{st}\AgdaSpace{}%
\AgdaOperator{\AgdaFunction{\ensuremath{\mathbin{{>}\mkern-8.5mu{>}\mkern-2mu{=}}}}}\AgdaSpace{}%
\AgdaBound{g}\AgdaSymbol{)}\<%
\\
\>[.][@{}l@{}]\<[455I]%
\>[7]\AgdaFunction{≡⟨}\AgdaSpace{}%
\AgdaFunction{cong}\AgdaSpace{}%
\AgdaSymbol{(λ}\AgdaSpace{}%
\AgdaBound{x}\AgdaSpace{}%
\AgdaSymbol{→}\AgdaSpace{}%
\AgdaBound{x}\AgdaSpace{}%
\AgdaOperator{\AgdaFunction{\ensuremath{\mathbin{{>}\mkern-8.5mu{>}\mkern-2mu{=}}}}}\AgdaSpace{}%
\AgdaBound{g}\AgdaSymbol{)}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaBound{p}\AgdaSpace{}%
\AgdaBound{st}\AgdaSymbol{)}%
\>[39]\AgdaFunction{⟩}\<%
\\
%
\>[4]\AgdaSymbol{(}\AgdaFunction{stackTransform2StateTransform}\AgdaSpace{}%
\AgdaBound{f'}\AgdaSpace{}%
\AgdaBound{st}\AgdaSpace{}%
\AgdaOperator{\AgdaFunction{\ensuremath{\mathbin{{>}\mkern-8.5mu{>}\mkern-2mu{=}}}}}\AgdaSpace{}%
\AgdaBound{g}\AgdaSpace{}%
\AgdaSymbol{)}\<%
\\
\>[4][@{}l@{\AgdaIndent{0}}]%
\>[7]\AgdaFunction{≡⟨}\AgdaSpace{}%
\AgdaFunction{lemmaEqualLift2Maybe}\AgdaSpace{}%
\AgdaBound{g}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaFunction{stackTransform2StateTransform}\AgdaSpace{}%
\AgdaBound{g'}\AgdaSpace{}%
\AgdaSymbol{)}\AgdaSpace{}%
\AgdaBound{q}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaFunction{stackTransform2StateTransform}\AgdaSpace{}%
\AgdaBound{f'}\AgdaSpace{}%
\AgdaBound{st}\AgdaSymbol{)}%
\>[110]\AgdaFunction{⟩}\<%
\\
%
\>[4]\AgdaSymbol{(}\AgdaFunction{stackTransform2StateTransform}\AgdaSpace{}%
\AgdaBound{f'}\AgdaSpace{}%
\AgdaBound{st}\AgdaSpace{}%
\AgdaOperator{\AgdaFunction{\ensuremath{\mathbin{{>}\mkern-8.5mu{>}\mkern-2mu{=}}}}}\AgdaSpace{}%
\AgdaFunction{stackTransform2StateTransform}\AgdaSpace{}%
\AgdaBound{g'}\AgdaSymbol{)}\<%
\\
\>[4][@{}l@{\AgdaIndent{0}}]%
\>[7]\AgdaOperator{\AgdaFunction{≡⟨⟩}}\<%
\\
\>[4][@{}l@{\AgdaIndent{0}}]%
\>[5]\AgdaSymbol{(}\AgdaFunction{exeTransformerDepIfStack'}\<%
\\
\>[5][@{}l@{\AgdaIndent{0}}]%
\>[9]\AgdaSymbol{(}\AgdaFunction{liftStackToStateTransformerAux'}%
\>[43]\AgdaSymbol{(}\AgdaBound{f'}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaBound{st}\AgdaSpace{}%
\AgdaSymbol{.}\AgdaField{currentTime}\AgdaSymbol{)}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaBound{st}\AgdaSpace{}%
\AgdaSymbol{.}\AgdaField{msg}\AgdaSymbol{)}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaBound{st}\AgdaSpace{}%
\AgdaSymbol{.}\AgdaField{stack}\AgdaSymbol{)))}%
\>[90]\AgdaBound{st}\<%
\\
\>[5][@{}l@{\AgdaIndent{0}}]%
\>[8]\AgdaOperator{\AgdaFunction{\ensuremath{\mathbin{{>}\mkern-8.5mu{>}\mkern-2mu{=}}}}}\<%
\\
%
\>[8]\AgdaSymbol{λ}\AgdaSpace{}%
\AgdaBound{s}%
\>[493I]\AgdaSymbol{→}%
\>[16]\AgdaFunction{exeTransformerDepIfStack'}\<%
\\
\>[.][@{}l@{}]\<[493I]%
\>[12]\AgdaSymbol{(}\AgdaFunction{liftStackToStateTransformerAux'}%
\>[46]\AgdaSymbol{(}\AgdaBound{g'}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaBound{s}\AgdaSpace{}%
\AgdaSymbol{.}\AgdaField{currentTime}\AgdaSymbol{)}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaBound{s}\AgdaSpace{}%
\AgdaSymbol{.}\AgdaField{msg}\AgdaSymbol{)}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaBound{s}\AgdaSpace{}%
\AgdaSymbol{.}\AgdaField{stack}\AgdaSymbol{)))}\AgdaSpace{}%
\AgdaBound{s}\AgdaSymbol{)}\<%
\\
%
\\[\AgdaEmptyExtraSkip]%
\>[5][@{}l@{\AgdaIndent{0}}]%
\>[7]\AgdaFunction{≡⟨}\AgdaSpace{}%
\AgdaFunction{lemmaStackSemIsSemScriptaux2}\AgdaSpace{}%
\AgdaBound{g'}\AgdaSpace{}%
\AgdaBound{st}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaBound{f'}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaBound{st}\AgdaSpace{}%
\AgdaSymbol{.}\AgdaField{currentTime}\AgdaSymbol{)}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaBound{st}\AgdaSpace{}%
\AgdaSymbol{.}\AgdaField{msg}\AgdaSymbol{)}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaBound{st}\AgdaSpace{}%
\AgdaSymbol{.}\AgdaField{stack}\AgdaSymbol{))}%
\>[91]\AgdaFunction{⟩}\<%
\\
%
\>[4]\AgdaFunction{exeTransformerDepIfStack'}\<%
\\
\>[0][@{}l@{\AgdaIndent{0}}]%
\>[2]\AgdaSymbol{(}\AgdaFunction{liftStackToStateTransformerAux'}\<%
\\
\>[2][@{}l@{\AgdaIndent{0}}]%
\>[3]\AgdaSymbol{(}\AgdaBound{f'}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaBound{st}\AgdaSpace{}%
\AgdaSymbol{.}\AgdaField{currentTime}\AgdaSymbol{)}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaBound{st}\AgdaSpace{}%
\AgdaSymbol{.}\AgdaField{msg}\AgdaSymbol{)}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaBound{st}\AgdaSpace{}%
\AgdaSymbol{.}\AgdaField{stack}\AgdaSymbol{)}\AgdaSpace{}%
\AgdaOperator{\AgdaFunction{\ensuremath{\mathbin{{>}\mkern-8.5mu{>}\mkern-2mu{=}}}}}\AgdaSpace{}%
\AgdaBound{g'}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaBound{st}\AgdaSpace{}%
\AgdaSymbol{.}\AgdaField{currentTime}\AgdaSymbol{)}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaBound{st}\AgdaSpace{}%
\AgdaSymbol{.}\AgdaField{msg}\AgdaSymbol{)))}%
\>[85]\AgdaBound{st}%
\>[89]\AgdaOperator{\AgdaFunction{∎}}\<%
\\
%
\\[\AgdaEmptyExtraSkip]%
%
\\[\AgdaEmptyExtraSkip]%
%
\\[\AgdaEmptyExtraSkip]%
\>[0]\AgdaFunction{lemmaStackSemIsSemScript}%
\>[523I]\AgdaSymbol{:}%
\>[524I]\AgdaSymbol{(}\AgdaBound{prog}\AgdaSpace{}%
\AgdaSymbol{:}\AgdaSpace{}%
\AgdaFunction{BitcoinScript}\AgdaSymbol{)}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaBound{nonIfs}\AgdaSpace{}%
\AgdaSymbol{:}\AgdaSpace{}%
\AgdaFunction{NonIfScript}\AgdaSpace{}%
\AgdaBound{prog}\AgdaSymbol{)}\<%
\\
\>[.][@{}l@{}]\<[524I]%
\>[27]\AgdaSymbol{(}\AgdaBound{state₁}\AgdaSpace{}%
\AgdaSymbol{:}\AgdaSpace{}%
\AgdaRecord{State}\AgdaSymbol{)}\<%
\\
\>[523I][@{}l@{\AgdaIndent{0}}]%
\>[26]\AgdaSymbol{→}\AgdaSpace{}%
\AgdaOperator{\AgdaFunction{⟦}}\AgdaSpace{}%
\AgdaBound{prog}\AgdaSpace{}%
\AgdaOperator{\AgdaFunction{⟧}}\AgdaSpace{}%
\AgdaBound{state₁}%
\>[45]\AgdaOperator{\AgdaDatatype{≡}}\AgdaSpace{}%
\AgdaFunction{stackTransform2StateTransform}\AgdaSpace{}%
\AgdaOperator{\AgdaFunction{⟦}}\AgdaSpace{}%
\AgdaBound{prog}\AgdaSpace{}%
\AgdaOperator{\AgdaFunction{⟧stack}}\AgdaSpace{}%
\AgdaBound{state₁}\<%
\\
\>[0]\AgdaFunction{lemmaStackSemIsSemScript}\AgdaSpace{}%
\AgdaInductiveConstructor{[]}\AgdaSpace{}%
\AgdaBound{nonIfs}\AgdaSpace{}%
\AgdaOperator{\AgdaInductiveConstructor{⟨}}\AgdaSpace{}%
\AgdaBound{currentTime₁}\AgdaSpace{}%
\AgdaOperator{\AgdaInductiveConstructor{,}}\AgdaSpace{}%
\AgdaBound{msg₁}\AgdaSpace{}%
\AgdaOperator{\AgdaInductiveConstructor{,}}\AgdaSpace{}%
\AgdaBound{stack₁}\AgdaSpace{}%
\AgdaOperator{\AgdaInductiveConstructor{,}}\AgdaSpace{}%
\AgdaInductiveConstructor{[]}\AgdaSpace{}%
\AgdaOperator{\AgdaInductiveConstructor{,}}\AgdaSpace{}%
\AgdaBound{consis₁}\AgdaSpace{}%
\AgdaOperator{\AgdaInductiveConstructor{⟩}}\AgdaSpace{}%
\AgdaSymbol{=}\AgdaSpace{}%
\AgdaInductiveConstructor{refl}\<%
\\
\>[0]\AgdaFunction{lemmaStackSemIsSemScript}\AgdaSpace{}%
\AgdaInductiveConstructor{[]}\AgdaSpace{}%
\AgdaBound{nonIfs}\AgdaSpace{}%
\AgdaOperator{\AgdaInductiveConstructor{⟨}}\AgdaSpace{}%
\AgdaBound{currentTime₁}\AgdaSpace{}%
\AgdaOperator{\AgdaInductiveConstructor{,}}\AgdaSpace{}%
\AgdaBound{msg₁}\AgdaSpace{}%
\AgdaOperator{\AgdaInductiveConstructor{,}}\AgdaSpace{}%
\AgdaBound{stack₁}\AgdaSpace{}%
\AgdaOperator{\AgdaInductiveConstructor{,}}\AgdaSpace{}%
\AgdaInductiveConstructor{ifCase}\AgdaSpace{}%
\AgdaOperator{\AgdaInductiveConstructor{∷}}\AgdaSpace{}%
\AgdaBound{ifStack₁}\AgdaSpace{}%
\AgdaOperator{\AgdaInductiveConstructor{,}}\AgdaSpace{}%
\AgdaBound{consis₁}\AgdaSpace{}%
\AgdaOperator{\AgdaInductiveConstructor{⟩}}\AgdaSpace{}%
\AgdaSymbol{=}\AgdaSpace{}%
\AgdaInductiveConstructor{refl}\<%
\\
\>[0]\AgdaFunction{lemmaStackSemIsSemScript}\AgdaSpace{}%
\AgdaInductiveConstructor{[]}\AgdaSpace{}%
\AgdaBound{nonIfs}\AgdaSpace{}%
\AgdaOperator{\AgdaInductiveConstructor{⟨}}\AgdaSpace{}%
\AgdaBound{currentTime₁}\AgdaSpace{}%
\AgdaOperator{\AgdaInductiveConstructor{,}}\AgdaSpace{}%
\AgdaBound{msg₁}\AgdaSpace{}%
\AgdaOperator{\AgdaInductiveConstructor{,}}\AgdaSpace{}%
\AgdaBound{stack₁}\AgdaSpace{}%
\AgdaOperator{\AgdaInductiveConstructor{,}}\AgdaSpace{}%
\AgdaInductiveConstructor{elseCase}\AgdaSpace{}%
\AgdaOperator{\AgdaInductiveConstructor{∷}}\AgdaSpace{}%
\AgdaBound{ifStack₁}\AgdaSpace{}%
\AgdaOperator{\AgdaInductiveConstructor{,}}\AgdaSpace{}%
\AgdaBound{consis₁}\AgdaSpace{}%
\AgdaOperator{\AgdaInductiveConstructor{⟩}}\AgdaSpace{}%
\AgdaSymbol{=}\AgdaSpace{}%
\AgdaInductiveConstructor{refl}\<%
\\
\>[0]\AgdaFunction{lemmaStackSemIsSemScript}\AgdaSpace{}%
\AgdaInductiveConstructor{[]}\AgdaSpace{}%
\AgdaBound{nonIfs}\AgdaSpace{}%
\AgdaOperator{\AgdaInductiveConstructor{⟨}}\AgdaSpace{}%
\AgdaBound{currentTime₁}\AgdaSpace{}%
\AgdaOperator{\AgdaInductiveConstructor{,}}\AgdaSpace{}%
\AgdaBound{msg₁}\AgdaSpace{}%
\AgdaOperator{\AgdaInductiveConstructor{,}}\AgdaSpace{}%
\AgdaBound{stack₁}\AgdaSpace{}%
\AgdaOperator{\AgdaInductiveConstructor{,}}\AgdaSpace{}%
\AgdaInductiveConstructor{ifSkip}\AgdaSpace{}%
\AgdaOperator{\AgdaInductiveConstructor{∷}}\AgdaSpace{}%
\AgdaBound{ifStack₁}\AgdaSpace{}%
\AgdaOperator{\AgdaInductiveConstructor{,}}\AgdaSpace{}%
\AgdaBound{consis₁}\AgdaSpace{}%
\AgdaOperator{\AgdaInductiveConstructor{⟩}}\AgdaSpace{}%
\AgdaSymbol{=}\AgdaSpace{}%
\AgdaInductiveConstructor{refl}\<%
\\
\>[0]\AgdaFunction{lemmaStackSemIsSemScript}\AgdaSpace{}%
\AgdaInductiveConstructor{[]}\AgdaSpace{}%
\AgdaBound{nonIfs}\AgdaSpace{}%
\AgdaOperator{\AgdaInductiveConstructor{⟨}}\AgdaSpace{}%
\AgdaBound{currentTime₁}\AgdaSpace{}%
\AgdaOperator{\AgdaInductiveConstructor{,}}\AgdaSpace{}%
\AgdaBound{msg₁}\AgdaSpace{}%
\AgdaOperator{\AgdaInductiveConstructor{,}}\AgdaSpace{}%
\AgdaBound{stack₁}\AgdaSpace{}%
\AgdaOperator{\AgdaInductiveConstructor{,}}\AgdaSpace{}%
\AgdaInductiveConstructor{elseSkip}\AgdaSpace{}%
\AgdaOperator{\AgdaInductiveConstructor{∷}}\AgdaSpace{}%
\AgdaBound{ifStack₁}\AgdaSpace{}%
\AgdaOperator{\AgdaInductiveConstructor{,}}\AgdaSpace{}%
\AgdaBound{consis₁}\AgdaSpace{}%
\AgdaOperator{\AgdaInductiveConstructor{⟩}}\AgdaSpace{}%
\AgdaSymbol{=}\AgdaSpace{}%
\AgdaInductiveConstructor{refl}\<%
\\
\>[0]\AgdaFunction{lemmaStackSemIsSemScript}\AgdaSpace{}%
\AgdaInductiveConstructor{[]}\AgdaSpace{}%
\AgdaBound{nonIfs}\AgdaSpace{}%
\AgdaOperator{\AgdaInductiveConstructor{⟨}}\AgdaSpace{}%
\AgdaBound{currentTime₁}\AgdaSpace{}%
\AgdaOperator{\AgdaInductiveConstructor{,}}\AgdaSpace{}%
\AgdaBound{msg₁}\AgdaSpace{}%
\AgdaOperator{\AgdaInductiveConstructor{,}}\AgdaSpace{}%
\AgdaBound{stack₁}\AgdaSpace{}%
\AgdaOperator{\AgdaInductiveConstructor{,}}\AgdaSpace{}%
\AgdaInductiveConstructor{ifIgnore}\AgdaSpace{}%
\AgdaOperator{\AgdaInductiveConstructor{∷}}\AgdaSpace{}%
\AgdaBound{ifStack₁}\AgdaSpace{}%
\AgdaOperator{\AgdaInductiveConstructor{,}}\AgdaSpace{}%
\AgdaBound{consis₁}\AgdaSpace{}%
\AgdaOperator{\AgdaInductiveConstructor{⟩}}\AgdaSpace{}%
\AgdaSymbol{=}\AgdaSpace{}%
\AgdaInductiveConstructor{refl}\<%
\\
\>[0]\AgdaFunction{lemmaStackSemIsSemScript}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaBound{op}\AgdaSpace{}%
\AgdaOperator{\AgdaInductiveConstructor{∷}}\AgdaSpace{}%
\AgdaInductiveConstructor{[]}\AgdaSymbol{)}\AgdaSpace{}%
\AgdaBound{nonIfs}\AgdaSpace{}%
\AgdaBound{state1}\AgdaSpace{}%
\AgdaKeyword{rewrite}\AgdaSpace{}%
\AgdaFunction{lemmaStackSemIsSemantics}\AgdaSpace{}%
\AgdaBound{op}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaFunction{nonIfScript2NonIf2Head}\AgdaSpace{}%
\AgdaBound{op}\AgdaSpace{}%
\AgdaInductiveConstructor{[]}\AgdaSpace{}%
\AgdaBound{nonIfs}\AgdaSpace{}%
\AgdaSymbol{)}%
\>[125]\AgdaSymbol{=}\AgdaSpace{}%
\AgdaInductiveConstructor{refl}\<%
\\
\>[0]\AgdaFunction{lemmaStackSemIsSemScript}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaBound{op}\AgdaSpace{}%
\AgdaOperator{\AgdaInductiveConstructor{∷}}\AgdaSpace{}%
\AgdaBound{rest}\AgdaSymbol{@(}\AgdaBound{x₁}\AgdaSpace{}%
\AgdaOperator{\AgdaInductiveConstructor{∷}}\AgdaSpace{}%
\AgdaBound{prog}\AgdaSymbol{))}\AgdaSpace{}%
\AgdaBound{nonIfs}\AgdaSpace{}%
\AgdaOperator{\AgdaInductiveConstructor{⟨}}\AgdaSpace{}%
\AgdaBound{currentTime₁}\AgdaSpace{}%
\AgdaOperator{\AgdaInductiveConstructor{,}}\AgdaSpace{}%
\AgdaBound{msg₁}\AgdaSpace{}%
\AgdaOperator{\AgdaInductiveConstructor{,}}\AgdaSpace{}%
\AgdaBound{stack₁}\AgdaSpace{}%
\AgdaOperator{\AgdaInductiveConstructor{,}}\AgdaSpace{}%
\AgdaBound{ifstack₁}\AgdaSpace{}%
\AgdaOperator{\AgdaInductiveConstructor{,}}\AgdaSpace{}%
\AgdaBound{consis₁}\AgdaSpace{}%
\AgdaOperator{\AgdaInductiveConstructor{⟩}}\AgdaSpace{}%
\AgdaSymbol{=}\<%
\\
\>[0][@{}l@{\AgdaIndent{0}}]%
\>[7]\AgdaSymbol{(}\AgdaOperator{\AgdaFunction{⟦}}%
\>[674I]\AgdaBound{op}\AgdaSpace{}%
\AgdaOperator{\AgdaFunction{⟧s}}\AgdaSpace{}%
\AgdaOperator{\AgdaInductiveConstructor{⟨}}\AgdaSpace{}%
\AgdaBound{currentTime₁}\AgdaSpace{}%
\AgdaOperator{\AgdaInductiveConstructor{,}}\AgdaSpace{}%
\AgdaBound{msg₁}\AgdaSpace{}%
\AgdaOperator{\AgdaInductiveConstructor{,}}\AgdaSpace{}%
\AgdaBound{stack₁}\AgdaSpace{}%
\AgdaOperator{\AgdaInductiveConstructor{,}}\AgdaSpace{}%
\AgdaBound{ifstack₁}\AgdaSpace{}%
\AgdaOperator{\AgdaInductiveConstructor{,}}\AgdaSpace{}%
\AgdaBound{consis₁}\AgdaSpace{}%
\AgdaOperator{\AgdaInductiveConstructor{⟩}}\AgdaSpace{}%
\AgdaOperator{\AgdaFunction{\ensuremath{\mathbin{{>}\mkern-8.5mu{>}\mkern-2mu{=}}}}}\AgdaSpace{}%
\AgdaOperator{\AgdaFunction{⟦}}\AgdaSpace{}%
\AgdaBound{rest}\AgdaSpace{}%
\AgdaOperator{\AgdaFunction{⟧}}\AgdaSymbol{)}\<%
\\
\>[.][@{}l@{}]\<[674I]%
\>[10]\AgdaFunction{≡⟨}\AgdaSpace{}%
\AgdaFunction{cong}%
\>[692I]\AgdaSymbol{(λ}\AgdaSpace{}%
\AgdaBound{x}\AgdaSpace{}%
\AgdaSymbol{→}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaBound{x}\AgdaSpace{}%
\AgdaOperator{\AgdaInductiveConstructor{⟨}}\AgdaSpace{}%
\AgdaBound{currentTime₁}\AgdaSpace{}%
\AgdaOperator{\AgdaInductiveConstructor{,}}\AgdaSpace{}%
\AgdaBound{msg₁}\AgdaSpace{}%
\AgdaOperator{\AgdaInductiveConstructor{,}}\AgdaSpace{}%
\AgdaBound{stack₁}\AgdaSpace{}%
\AgdaOperator{\AgdaInductiveConstructor{,}}\AgdaSpace{}%
\AgdaBound{ifstack₁}\AgdaSpace{}%
\AgdaOperator{\AgdaInductiveConstructor{,}}\AgdaSpace{}%
\AgdaBound{consis₁}\AgdaSpace{}%
\AgdaOperator{\AgdaInductiveConstructor{⟩}}\AgdaSpace{}%
\AgdaOperator{\AgdaFunction{\ensuremath{\mathbin{{>}\mkern-8.5mu{>}\mkern-2mu{=}}}}}\AgdaSpace{}%
\AgdaOperator{\AgdaFunction{⟦}}\AgdaSpace{}%
\AgdaBound{rest}\AgdaSpace{}%
\AgdaOperator{\AgdaFunction{⟧}}\AgdaSpace{}%
\AgdaSymbol{))}\<%
\\
\>[.][@{}l@{}]\<[692I]%
\>[18]\AgdaSymbol{(}\AgdaFunction{lemmaStackSemIsSemantics}\AgdaSpace{}%
\AgdaBound{op}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaFunction{nonIfScript2NonIf2Head}\AgdaSpace{}%
\AgdaBound{op}\AgdaSpace{}%
\AgdaBound{rest}\AgdaSpace{}%
\AgdaBound{nonIfs}\AgdaSymbol{))}%
\>[89]\AgdaFunction{⟩}\<%
\\
%
\>[7]\AgdaSymbol{(}\AgdaFunction{stackTransform2StateTransform}\AgdaSpace{}%
\AgdaOperator{\AgdaFunction{⟦}}\AgdaSpace{}%
\AgdaBound{op}\AgdaSpace{}%
\AgdaOperator{\AgdaFunction{⟧stacks}}%
\>[52]\AgdaOperator{\AgdaInductiveConstructor{⟨}}\AgdaSpace{}%
\AgdaBound{currentTime₁}\AgdaSpace{}%
\AgdaOperator{\AgdaInductiveConstructor{,}}\AgdaSpace{}%
\AgdaBound{msg₁}\AgdaSpace{}%
\AgdaOperator{\AgdaInductiveConstructor{,}}\AgdaSpace{}%
\AgdaBound{stack₁}\AgdaSpace{}%
\AgdaOperator{\AgdaInductiveConstructor{,}}\AgdaSpace{}%
\AgdaBound{ifstack₁}\AgdaSpace{}%
\AgdaOperator{\AgdaInductiveConstructor{,}}\AgdaSpace{}%
\AgdaBound{consis₁}\AgdaSpace{}%
\AgdaOperator{\AgdaInductiveConstructor{⟩}}\<%
\\
\>[7][@{}l@{\AgdaIndent{0}}]%
\>[9]\AgdaOperator{\AgdaFunction{\ensuremath{\mathbin{{>}\mkern-8.5mu{>}\mkern-2mu{=}}}}}\AgdaSpace{}%
\AgdaOperator{\AgdaFunction{⟦}}\AgdaSpace{}%
\AgdaBound{rest}\AgdaSpace{}%
\AgdaOperator{\AgdaFunction{⟧}}\AgdaSymbol{)}\<%
\\
%
\\[\AgdaEmptyExtraSkip]%
\>[9][@{}l@{\AgdaIndent{0}}]%
\>[10]\AgdaFunction{≡⟨}\AgdaSpace{}%
\AgdaFunction{lemmaEqualLift2Maybe}%
\>[35]\AgdaOperator{\AgdaFunction{⟦}}\AgdaSpace{}%
\AgdaBound{rest}\AgdaSpace{}%
\AgdaOperator{\AgdaFunction{⟧}}%
\>[45]\AgdaSymbol{(}\AgdaFunction{stackTransform2StateTransform}\AgdaSpace{}%
\AgdaOperator{\AgdaFunction{⟦}}\AgdaSpace{}%
\AgdaBound{rest}\AgdaSpace{}%
\AgdaOperator{\AgdaFunction{⟧stack}}\AgdaSpace{}%
\AgdaSymbol{)}\<%
\\
\>[10][@{}l@{\AgdaIndent{0}}]%
\>[12]\AgdaSymbol{(}\AgdaFunction{lemmaStackSemIsSemScript}\AgdaSpace{}%
\AgdaBound{rest}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaFunction{nonIfScript2NonIf2Tail}\AgdaSpace{}%
\AgdaBound{op}\AgdaSpace{}%
\AgdaBound{rest}\AgdaSpace{}%
\AgdaBound{nonIfs}\AgdaSymbol{))}\<%
\\
%
\>[12]\AgdaSymbol{((}\AgdaFunction{stackTransform2StateTransform}\AgdaSpace{}%
\AgdaOperator{\AgdaFunction{⟦}}\AgdaSpace{}%
\AgdaBound{op}\AgdaSpace{}%
\AgdaOperator{\AgdaFunction{⟧stacks}}%
\>[58]\AgdaOperator{\AgdaInductiveConstructor{⟨}}\AgdaSpace{}%
\AgdaBound{currentTime₁}\AgdaSpace{}%
\AgdaOperator{\AgdaInductiveConstructor{,}}\AgdaSpace{}%
\AgdaBound{msg₁}\AgdaSpace{}%
\AgdaOperator{\AgdaInductiveConstructor{,}}\AgdaSpace{}%
\AgdaBound{stack₁}\AgdaSpace{}%
\AgdaOperator{\AgdaInductiveConstructor{,}}\AgdaSpace{}%
\AgdaBound{ifstack₁}\AgdaSpace{}%
\AgdaOperator{\AgdaInductiveConstructor{,}}\AgdaSpace{}%
\AgdaBound{consis₁}\AgdaSpace{}%
\AgdaOperator{\AgdaInductiveConstructor{⟩}}\AgdaSymbol{))}\AgdaSpace{}%
\AgdaFunction{⟩}\<%
\\
%
\>[7]\AgdaSymbol{(}\AgdaFunction{stackTransform2StateTransform}\AgdaSpace{}%
\AgdaOperator{\AgdaFunction{⟦}}\AgdaSpace{}%
\AgdaBound{op}\AgdaSpace{}%
\AgdaOperator{\AgdaFunction{⟧stacks}}%
\>[52]\AgdaOperator{\AgdaInductiveConstructor{⟨}}\AgdaSpace{}%
\AgdaBound{currentTime₁}\AgdaSpace{}%
\AgdaOperator{\AgdaInductiveConstructor{,}}\AgdaSpace{}%
\AgdaBound{msg₁}\AgdaSpace{}%
\AgdaOperator{\AgdaInductiveConstructor{,}}\AgdaSpace{}%
\AgdaBound{stack₁}\AgdaSpace{}%
\AgdaOperator{\AgdaInductiveConstructor{,}}\AgdaSpace{}%
\AgdaBound{ifstack₁}\AgdaSpace{}%
\AgdaOperator{\AgdaInductiveConstructor{,}}\AgdaSpace{}%
\AgdaBound{consis₁}\AgdaSpace{}%
\AgdaOperator{\AgdaInductiveConstructor{⟩}}\<%
\\
\>[7][@{}l@{\AgdaIndent{0}}]%
\>[12]\AgdaOperator{\AgdaFunction{\ensuremath{\mathbin{{>}\mkern-8.5mu{>}\mkern-2mu{=}}}}}%
\>[772I]\AgdaFunction{stackTransform2StateTransform}\AgdaSpace{}%
\AgdaOperator{\AgdaFunction{⟦}}\AgdaSpace{}%
\AgdaBound{rest}\AgdaSpace{}%
\AgdaOperator{\AgdaFunction{⟧stack}}\AgdaSymbol{)}\<%
\\
\>[.][@{}l@{}]\<[772I]%
\>[16]\AgdaFunction{≡⟨}%
\>[776I]\AgdaFunction{lemmaStackSemIsSemScriptaux2}\AgdaSpace{}%
\AgdaOperator{\AgdaFunction{⟦}}\AgdaSpace{}%
\AgdaBound{x₁}\AgdaSpace{}%
\AgdaOperator{\AgdaInductiveConstructor{∷}}\AgdaSpace{}%
\AgdaBound{prog}\AgdaSpace{}%
\AgdaOperator{\AgdaFunction{⟧stack}}\AgdaSpace{}%
\AgdaOperator{\AgdaInductiveConstructor{⟨}}\AgdaSpace{}%
\AgdaBound{currentTime₁}\AgdaSpace{}%
\AgdaOperator{\AgdaInductiveConstructor{,}}\AgdaSpace{}%
\AgdaBound{msg₁}\AgdaSpace{}%
\AgdaOperator{\AgdaInductiveConstructor{,}}\AgdaSpace{}%
\AgdaBound{stack₁}\AgdaSpace{}%
\AgdaOperator{\AgdaInductiveConstructor{,}}\AgdaSpace{}%
\AgdaBound{ifstack₁}\AgdaSpace{}%
\AgdaOperator{\AgdaInductiveConstructor{,}}\AgdaSpace{}%
\AgdaBound{consis₁}\AgdaSpace{}%
\AgdaOperator{\AgdaInductiveConstructor{⟩}}\<%
\\
\>[.][@{}l@{}]\<[776I]%
\>[19]\AgdaSymbol{(}\AgdaOperator{\AgdaFunction{⟦}}\AgdaSpace{}%
\AgdaBound{op}\AgdaSpace{}%
\AgdaOperator{\AgdaFunction{⟧stacks}}\AgdaSpace{}%
\AgdaBound{currentTime₁}\AgdaSpace{}%
\AgdaBound{msg₁}\AgdaSpace{}%
\AgdaBound{stack₁}\AgdaSymbol{)}\AgdaSpace{}%
\AgdaFunction{⟩}\<%
\\
\>[0][@{}l@{\AgdaIndent{0}}]%
\>[6]\AgdaFunction{exeTransformerDepIfStack'}\<%
\\
%
\>[6]\AgdaSymbol{(}\AgdaFunction{liftStackToStateTransformerAux'}\<%
\\
\>[6][@{}l@{\AgdaIndent{0}}]%
\>[7]\AgdaSymbol{(}\AgdaOperator{\AgdaFunction{⟦}}\AgdaSpace{}%
\AgdaBound{op}\AgdaSpace{}%
\AgdaOperator{\AgdaFunction{⟧stacks}}\AgdaSpace{}%
\AgdaBound{currentTime₁}\AgdaSpace{}%
\AgdaBound{msg₁}\AgdaSpace{}%
\AgdaBound{stack₁}\AgdaSpace{}%
\AgdaOperator{\AgdaFunction{\ensuremath{\mathbin{{>}\mkern-8.5mu{>}\mkern-2mu{=}}}}}\AgdaSpace{}%
\AgdaOperator{\AgdaFunction{⟦}}\AgdaSpace{}%
\AgdaBound{rest}\AgdaSpace{}%
\AgdaOperator{\AgdaFunction{⟧stack}}\AgdaSpace{}%
\AgdaBound{currentTime₁}\AgdaSpace{}%
\AgdaBound{msg₁}\AgdaSymbol{))}\<%
\\
%
\>[6]\AgdaOperator{\AgdaInductiveConstructor{⟨}}\AgdaSpace{}%
\AgdaBound{currentTime₁}\AgdaSpace{}%
\AgdaOperator{\AgdaInductiveConstructor{,}}\AgdaSpace{}%
\AgdaBound{msg₁}\AgdaSpace{}%
\AgdaOperator{\AgdaInductiveConstructor{,}}\AgdaSpace{}%
\AgdaBound{stack₁}\AgdaSpace{}%
\AgdaOperator{\AgdaInductiveConstructor{,}}\AgdaSpace{}%
\AgdaBound{ifstack₁}\AgdaSpace{}%
\AgdaOperator{\AgdaInductiveConstructor{,}}\AgdaSpace{}%
\AgdaBound{consis₁}\AgdaSpace{}%
\AgdaOperator{\AgdaInductiveConstructor{⟩}}\<%
\\
\>[0][@{}l@{\AgdaIndent{0}}]%
\>[4]\AgdaOperator{\AgdaFunction{∎}}\<%
\\
%
\\[\AgdaEmptyExtraSkip]%
%
\\[\AgdaEmptyExtraSkip]%
%
\\[\AgdaEmptyExtraSkip]%
%
\\[\AgdaEmptyExtraSkip]%
%
\\[\AgdaEmptyExtraSkip]%
%
\\[\AgdaEmptyExtraSkip]%
%
\\[\AgdaEmptyExtraSkip]%
%
\\[\AgdaEmptyExtraSkip]%
%
\\[\AgdaEmptyExtraSkip]%
\>[0]\AgdaFunction{lemmaNonIfInstrGenericCondImpliesTripleaux'}\AgdaSpace{}%
\AgdaSymbol{:}\<%
\\
\>[0][@{}l@{\AgdaIndent{0}}]%
\>[10]\AgdaSymbol{(}\AgdaBound{prog}\AgdaSpace{}%
\AgdaSymbol{:}\AgdaSpace{}%
\AgdaFunction{BitcoinScript}\AgdaSymbol{)(}\AgdaBound{nonIf}\AgdaSpace{}%
\AgdaSymbol{:}\AgdaSpace{}%
\AgdaFunction{NonIfScript}\AgdaSpace{}%
\AgdaBound{prog}\AgdaSymbol{)}\<%
\\
%
\>[10]\AgdaSymbol{(}\AgdaBound{φ}\AgdaSpace{}%
\AgdaBound{ψ}\AgdaSpace{}%
\AgdaSymbol{:}\AgdaSpace{}%
\AgdaFunction{Predicate}\AgdaSymbol{)}\<%
\\
%
\>[10]\AgdaSymbol{→}\AgdaSpace{}%
\AgdaOperator{\AgdaRecord{<}}\AgdaSpace{}%
\AgdaBound{φ}\AgdaSpace{}%
\AgdaOperator{\AgdaRecord{>gen}}\AgdaSpace{}%
\AgdaFunction{stackTransform2StateTransform}\AgdaSpace{}%
\AgdaOperator{\AgdaFunction{⟦}}%
\>[54]\AgdaBound{prog}%
\>[60]\AgdaOperator{\AgdaFunction{⟧stack}}\AgdaSpace{}%
\AgdaOperator{\AgdaRecord{<}}\AgdaSpace{}%
\AgdaBound{ψ}\AgdaSpace{}%
\AgdaOperator{\AgdaRecord{>}}\<%
\\
%
\>[10]\AgdaSymbol{→}\AgdaSpace{}%
\AgdaOperator{\AgdaRecord{<}}\AgdaSpace{}%
\AgdaBound{φ}\AgdaSpace{}%
\AgdaOperator{\AgdaRecord{>gen}}\AgdaSpace{}%
\AgdaOperator{\AgdaFunction{⟦}}\AgdaSpace{}%
\AgdaBound{prog}\AgdaSpace{}%
\AgdaOperator{\AgdaFunction{⟧}}\AgdaSpace{}%
\AgdaOperator{\AgdaRecord{<}}\AgdaSpace{}%
\AgdaBound{ψ}\AgdaSpace{}%
\AgdaOperator{\AgdaRecord{>}}\<%
\\
\>[0]\AgdaFunction{lemmaNonIfInstrGenericCondImpliesTripleaux'}\AgdaSpace{}%
\AgdaBound{prog}\AgdaSpace{}%
\AgdaBound{nonIf}\AgdaSpace{}%
\AgdaBound{φ}\AgdaSpace{}%
\AgdaBound{ψ}\AgdaSpace{}%
\AgdaBound{x}\<%
\\
\>[0][@{}l@{\AgdaIndent{0}}]%
\>[4]\AgdaSymbol{=}%
\>[851I]\AgdaFunction{lemmaTransferHoareTripleGen}\AgdaSpace{}%
\AgdaBound{φ}\AgdaSpace{}%
\AgdaBound{ψ}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaFunction{stackTransform2StateTransform}\AgdaSpace{}%
\AgdaOperator{\AgdaFunction{⟦}}%
\>[72]\AgdaBound{prog}%
\>[78]\AgdaOperator{\AgdaFunction{⟧stack}}\AgdaSymbol{)}\AgdaSpace{}%
\AgdaOperator{\AgdaFunction{⟦}}\AgdaSpace{}%
\AgdaBound{prog}\AgdaSpace{}%
\AgdaOperator{\AgdaFunction{⟧}}\<%
\\
\>[.][@{}l@{}]\<[851I]%
\>[6]\AgdaSymbol{(λ}\AgdaSpace{}%
\AgdaBound{s}\AgdaSpace{}%
\AgdaSymbol{→}\AgdaSpace{}%
\AgdaFunction{sym}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaFunction{lemmaStackSemIsSemScript}\AgdaSpace{}%
\AgdaBound{prog}\AgdaSpace{}%
\AgdaBound{nonIf}\AgdaSpace{}%
\AgdaOperator{\AgdaInductiveConstructor{⟨}}\AgdaSpace{}%
\AgdaField{currentTime}\AgdaSpace{}%
\AgdaBound{s}\AgdaSpace{}%
\AgdaOperator{\AgdaInductiveConstructor{,}}\AgdaSpace{}%
\AgdaField{msg}\AgdaSpace{}%
\AgdaBound{s}\AgdaSpace{}%
\AgdaOperator{\AgdaInductiveConstructor{,}}\AgdaSpace{}%
\AgdaField{stack}\AgdaSpace{}%
\AgdaBound{s}\AgdaSpace{}%
\AgdaOperator{\AgdaInductiveConstructor{,}}\AgdaSpace{}%
\AgdaField{ifStack}\AgdaSpace{}%
\AgdaBound{s}\AgdaSpace{}%
\AgdaOperator{\AgdaInductiveConstructor{,}}\AgdaSpace{}%
\AgdaField{consis}\AgdaSpace{}%
\AgdaBound{s}\AgdaSpace{}%
\AgdaOperator{\AgdaInductiveConstructor{⟩}}\AgdaSymbol{))}\AgdaSpace{}%
\AgdaBound{x}\<%
\\
%
\\[\AgdaEmptyExtraSkip]%
%
\\[\AgdaEmptyExtraSkip]%
%
\\[\AgdaEmptyExtraSkip]%
%
\\[\AgdaEmptyExtraSkip]%
%
\\[\AgdaEmptyExtraSkip]%
%
\\[\AgdaEmptyExtraSkip]%
%
\\[\AgdaEmptyExtraSkip]%
\>[0]\AgdaFunction{lemmaGenericHoareTripleImpliesHoareTripleProg}\AgdaSpace{}%
\AgdaSymbol{:}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaBound{prog}\AgdaSpace{}%
\AgdaSymbol{:}\AgdaSpace{}%
\AgdaFunction{BitcoinScript}\AgdaSymbol{)}\<%
\\
\>[0][@{}l@{\AgdaIndent{0}}]%
\>[44]\AgdaSymbol{(}\AgdaBound{φ}\AgdaSpace{}%
\AgdaBound{ψ}\AgdaSpace{}%
\AgdaSymbol{:}\AgdaSpace{}%
\AgdaFunction{Predicate}\AgdaSymbol{)}\<%
\\
%
\>[44]\AgdaSymbol{→}\AgdaSpace{}%
\AgdaOperator{\AgdaRecord{<}}\AgdaSpace{}%
\AgdaBound{φ}\AgdaSpace{}%
\AgdaOperator{\AgdaRecord{>gen}}\AgdaSpace{}%
\AgdaOperator{\AgdaFunction{⟦}}\AgdaSpace{}%
\AgdaBound{prog}\AgdaSpace{}%
\AgdaOperator{\AgdaFunction{⟧}}\AgdaSpace{}%
\AgdaOperator{\AgdaRecord{<}}%
\>[67]\AgdaBound{ψ}\AgdaSpace{}%
\AgdaOperator{\AgdaRecord{>}}\<%
\\
%
\>[44]\AgdaSymbol{→}\AgdaSpace{}%
\AgdaOperator{\AgdaRecord{<}}\AgdaSpace{}%
\AgdaBound{φ}\AgdaSpace{}%
\AgdaOperator{\AgdaRecord{>ⁱᶠᶠ}}\AgdaSpace{}%
\AgdaBound{prog}\AgdaSpace{}%
\AgdaOperator{\AgdaRecord{<}}\AgdaSpace{}%
\AgdaBound{ψ}\AgdaSpace{}%
\AgdaOperator{\AgdaRecord{>}}\<%
\\
\>[0]\AgdaFunction{lemmaGenericHoareTripleImpliesHoareTripleProg}\AgdaSpace{}%
\AgdaBound{prog}\AgdaSpace{}%
\AgdaBound{φ}\AgdaSpace{}%
\AgdaBound{ψ}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaInductiveConstructor{hoareTripleGen}\AgdaSpace{}%
\AgdaBound{==>g₁}\AgdaSpace{}%
\AgdaBound{<==g₁}\AgdaSymbol{)}\AgdaSpace{}%
\AgdaSymbol{.}\AgdaField{==>}\AgdaSpace{}%
\AgdaSymbol{=}\AgdaSpace{}%
\AgdaBound{==>g₁}\<%
\\
\>[0]\AgdaFunction{lemmaGenericHoareTripleImpliesHoareTripleProg}\AgdaSpace{}%
\AgdaBound{prog}\AgdaSpace{}%
\AgdaBound{φ}\AgdaSpace{}%
\AgdaBound{ψ}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaInductiveConstructor{hoareTripleGen}\AgdaSpace{}%
\AgdaBound{==>g₁}\AgdaSpace{}%
\AgdaBound{<==g₁}\AgdaSymbol{)}\AgdaSpace{}%
\AgdaSymbol{.}\AgdaField{<==}\AgdaSpace{}%
\AgdaSymbol{=}\AgdaSpace{}%
\AgdaBound{<==g₁}\<%
\\
%
\\[\AgdaEmptyExtraSkip]%
\>[0]\AgdaFunction{lemmaNonIfInstrGenericCondImpliesTripleauxProg}\AgdaSpace{}%
\AgdaSymbol{:}\<%
\\
\>[0][@{}l@{\AgdaIndent{0}}]%
\>[10]\AgdaSymbol{(}\AgdaBound{prog}\AgdaSpace{}%
\AgdaSymbol{:}\AgdaSpace{}%
\AgdaFunction{BitcoinScript}\AgdaSymbol{)(}\AgdaBound{nonIf}\AgdaSpace{}%
\AgdaSymbol{:}\AgdaSpace{}%
\AgdaFunction{NonIfScript}\AgdaSpace{}%
\AgdaBound{prog}\AgdaSymbol{)}\<%
\\
%
\>[10]\AgdaSymbol{(}\AgdaBound{φ}\AgdaSpace{}%
\AgdaBound{ψ}\AgdaSpace{}%
\AgdaSymbol{:}\AgdaSpace{}%
\AgdaFunction{Predicate}\AgdaSymbol{)}\<%
\\
%
\>[10]\AgdaSymbol{→}\AgdaSpace{}%
\AgdaOperator{\AgdaRecord{<}}\AgdaSpace{}%
\AgdaBound{φ}\AgdaSpace{}%
\AgdaOperator{\AgdaRecord{>gen}}\AgdaSpace{}%
\AgdaFunction{stackTransform2StateTransform}\AgdaSpace{}%
\AgdaOperator{\AgdaFunction{⟦}}\AgdaSpace{}%
\AgdaBound{prog}\AgdaSpace{}%
\AgdaOperator{\AgdaFunction{⟧stack}}\AgdaSpace{}%
\AgdaOperator{\AgdaRecord{<}}\AgdaSpace{}%
\AgdaBound{ψ}\AgdaSpace{}%
\AgdaOperator{\AgdaRecord{>}}\<%
\\
%
\>[10]\AgdaSymbol{→}\AgdaSpace{}%
\AgdaOperator{\AgdaRecord{<}}\AgdaSpace{}%
\AgdaBound{φ}\AgdaSpace{}%
\AgdaOperator{\AgdaRecord{>gen}}\AgdaSpace{}%
\AgdaOperator{\AgdaFunction{⟦}}\AgdaSpace{}%
\AgdaBound{prog}\AgdaSpace{}%
\AgdaOperator{\AgdaFunction{⟧}}\AgdaSpace{}%
\AgdaOperator{\AgdaRecord{<}}\AgdaSpace{}%
\AgdaBound{ψ}\AgdaSpace{}%
\AgdaOperator{\AgdaRecord{>}}\<%
\\
\>[0]\AgdaFunction{lemmaNonIfInstrGenericCondImpliesTripleauxProg}\AgdaSpace{}%
\AgdaBound{prog}\AgdaSpace{}%
\AgdaBound{nonIf}\AgdaSpace{}%
\AgdaBound{φ}\AgdaSpace{}%
\AgdaBound{ψ}\AgdaSpace{}%
\AgdaBound{x}\AgdaSpace{}%
\AgdaSymbol{=}\<%
\\
\>[0][@{}l@{\AgdaIndent{0}}]%
\>[4]\AgdaFunction{lemmaTransferHoareTripleGen}\AgdaSpace{}%
\AgdaBound{φ}\AgdaSpace{}%
\AgdaBound{ψ}\<%
\\
\>[4][@{}l@{\AgdaIndent{0}}]%
\>[6]\AgdaSymbol{(}\AgdaFunction{stackTransform2StateTransform}\AgdaSpace{}%
\AgdaOperator{\AgdaFunction{⟦}}\AgdaSpace{}%
\AgdaBound{prog}\AgdaSpace{}%
\AgdaOperator{\AgdaFunction{⟧stack}}\AgdaSymbol{)}\AgdaSpace{}%
\AgdaOperator{\AgdaFunction{⟦}}\AgdaSpace{}%
\AgdaBound{prog}\AgdaSpace{}%
\AgdaOperator{\AgdaFunction{⟧}}\<%
\\
%
\>[6]\AgdaSymbol{(λ}\AgdaSpace{}%
\AgdaBound{s}\AgdaSpace{}%
\AgdaSymbol{→}\AgdaSpace{}%
\AgdaFunction{sym}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaFunction{lemmaStackSemIsSemScript}\AgdaSpace{}%
\AgdaBound{prog}\AgdaSpace{}%
\AgdaBound{nonIf}\AgdaSpace{}%
\AgdaBound{s}\AgdaSymbol{))}\AgdaSpace{}%
\AgdaBound{x}\<%
\\
%
\\[\AgdaEmptyExtraSkip]%
%
\\[\AgdaEmptyExtraSkip]%
\>[0]\AgdaComment{--\ Is\ now\ in}\<%
\\
\>[0]\AgdaComment{--\ \textasciitilde{}/git/Smart-contracts-verification-with-agda/ScriptTester/verificationStackScripts/stackVerificationLemmasPart2.agda}\<%
\\
%
\\[\AgdaEmptyExtraSkip]%
\>[0]\AgdaFunction{hoareTripleStack2HoareTripleIfStack}\AgdaSpace{}%
\AgdaSymbol{:}\<%
\\
\>[0][@{}l@{\AgdaIndent{0}}]%
\>[5]\AgdaSymbol{(}\AgdaBound{ifStack₁}\AgdaSpace{}%
\AgdaSymbol{:}\AgdaSpace{}%
\AgdaFunction{IfStack}\AgdaSymbol{)}\<%
\\
%
\>[5]\AgdaSymbol{(}\AgdaBound{active}\AgdaSpace{}%
\AgdaSymbol{:}\AgdaSpace{}%
\AgdaFunction{IsActiveIfStack}\AgdaSpace{}%
\AgdaBound{ifStack₁}\AgdaSymbol{)}\<%
\\
%
\>[5]\AgdaSymbol{(}\AgdaBound{prog}\AgdaSpace{}%
\AgdaSymbol{:}\AgdaSpace{}%
\AgdaFunction{BitcoinScript}\AgdaSymbol{)}\<%
\\
%
\>[5]\AgdaSymbol{(}\AgdaBound{nonIf}\AgdaSpace{}%
\AgdaSymbol{:}\AgdaSpace{}%
\AgdaFunction{NonIfScript}\AgdaSpace{}%
\AgdaBound{prog}\AgdaSymbol{)}\<%
\\
%
\>[5]\AgdaSymbol{(}\AgdaBound{φ}\AgdaSpace{}%
\AgdaBound{ψ}\AgdaSpace{}%
\AgdaSymbol{:}\AgdaSpace{}%
\AgdaFunction{StackPredicate}\AgdaSymbol{)}\<%
\\
%
\>[5]\AgdaSymbol{→}\AgdaSpace{}%
\AgdaOperator{\AgdaFunction{<}}\AgdaSpace{}%
\AgdaBound{φ}\AgdaSpace{}%
\AgdaOperator{\AgdaFunction{>stack}}\AgdaSpace{}%
\AgdaBound{prog}\AgdaSpace{}%
\AgdaOperator{\AgdaFunction{<}}\AgdaSpace{}%
\AgdaBound{ψ}\AgdaSpace{}%
\AgdaOperator{\AgdaFunction{>}}\<%
\\
%
\>[5]\AgdaSymbol{→}\AgdaSpace{}%
\AgdaOperator{\AgdaRecord{<}}\AgdaSpace{}%
\AgdaFunction{liftStackPred2Pred}\AgdaSpace{}%
\AgdaBound{φ}\AgdaSpace{}%
\AgdaBound{ifStack₁}%
\>[40]\AgdaOperator{\AgdaRecord{>ⁱᶠᶠ}}\AgdaSpace{}%
\AgdaBound{prog}\AgdaSpace{}%
\AgdaOperator{\AgdaRecord{<}}\AgdaSpace{}%
\AgdaFunction{liftStackPred2Pred}\AgdaSpace{}%
\AgdaBound{ψ}\AgdaSpace{}%
\AgdaBound{ifStack₁}%
\>[84]\AgdaOperator{\AgdaRecord{>}}\<%
\\
\>[0]\AgdaFunction{hoareTripleStack2HoareTripleIfStack}\AgdaSpace{}%
\AgdaBound{ifStack₁}\AgdaSpace{}%
\AgdaBound{active}\AgdaSpace{}%
\AgdaBound{prog}\AgdaSpace{}%
\AgdaBound{nonIf}\AgdaSpace{}%
\AgdaBound{φ}\AgdaSpace{}%
\AgdaBound{ψ}\AgdaSpace{}%
\AgdaBound{x}\<%
\\
\>[0][@{}l@{\AgdaIndent{0}}]%
\>[3]\AgdaSymbol{=}%
\>[1009I]\AgdaFunction{lemmaGenericHoareTripleImpliesHoareTripleProg}\AgdaSpace{}%
\AgdaBound{prog}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaFunction{liftStackPred2Pred}\AgdaSpace{}%
\AgdaBound{φ}\AgdaSpace{}%
\AgdaBound{ifStack₁}\AgdaSymbol{)}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaFunction{liftStackPred2Pred}\AgdaSpace{}%
\AgdaBound{ψ}\AgdaSpace{}%
\AgdaBound{ifStack₁}\AgdaSymbol{)}\<%
\\
\>[.][@{}l@{}]\<[1009I]%
\>[5]\AgdaSymbol{(}\AgdaFunction{lemmaNonIfInstrGenericCondImpliesTripleauxProg}\AgdaSpace{}%
\AgdaBound{prog}\AgdaSpace{}%
\AgdaBound{nonIf}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaFunction{liftStackPred2Pred}\AgdaSpace{}%
\AgdaBound{φ}\AgdaSpace{}%
\AgdaBound{ifStack₁}\AgdaSymbol{)}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaFunction{liftStackPred2Pred}\AgdaSpace{}%
\AgdaBound{ψ}\AgdaSpace{}%
\AgdaBound{ifStack₁}\AgdaSymbol{)}\<%
\\
%
\>[5]\AgdaSymbol{(}\AgdaFunction{lemmaHoareTripleStackPartToHoareTripleGeneric}\AgdaSpace{}%
\AgdaOperator{\AgdaFunction{⟦}}\AgdaSpace{}%
\AgdaBound{prog}\AgdaSpace{}%
\AgdaOperator{\AgdaFunction{⟧stack}}\AgdaSpace{}%
\AgdaBound{ifStack₁}\AgdaSpace{}%
\AgdaBound{active}\AgdaSpace{}%
\AgdaBound{φ}%
\>[85]\AgdaBound{ψ}\<%
\\
%
\>[5]\AgdaBound{x}\AgdaSymbol{))}\<%
\\
%
\\[\AgdaEmptyExtraSkip]%
%
\\[\AgdaEmptyExtraSkip]%
\>[0]\AgdaComment{--\ Is\ now\ in}\<%
\\
\>[0]\AgdaComment{--\ \textasciitilde{}/git/Smart-contracts-verification-with-agda/ScriptTester/verificationStackScripts/stackVerificationLemmasPart2.agda}\<%
\\
\>[0]\AgdaComment{--}\<%
\\
\>[0]\AgdaComment{\{-}\<%
\\
\>[0]\AgdaComment{lemmaTransferHoareTripleStack\ :\ (φ\ ψ\ :\ StackPredicate)}\<%
\\
\>[0]\AgdaComment{\ \ \ \ \ \ \ \ \ \ \ \ \ \ \ \ \ \ \ \ \ \ \ \ \ \ \ \ \ \ (f\ g\ :\ Time\ →\ Msg\ →\ Stack\ →\ Maybe\ Stack)}\<%
\\
\>[0]\AgdaComment{\ \ \ \ \ \ \ \ \ \ \ \ \ \ \ \ \ \ \ \ \ \ \ \ \ \ \ \ \ \ (p\ :\ (t\ :\ Time)(m\ :\ Msg)(s\ :\ Stack)\ →\ f\ t\ m\ s\ \ ≡\ g\ t\ m\ s)}\<%
\\
\>[0]\AgdaComment{\ \ \ \ \ \ \ \ \ \ \ \ \ \ \ \ \ \ \ \ \ \ \ \ \ \ \ \ \ \ →\ <\ \ φ\ >gˢ\ \ f\ <\ ψ\ >}\<%
\\
\>[0]\AgdaComment{\ \ \ \ \ \ \ \ \ \ \ \ \ \ \ \ \ \ \ \ \ \ \ \ \ \ \ \ \ \ →\ <\ φ\ >gˢ\ g\ <\ ψ\ >}\<%
\\
\>[0]\AgdaComment{lemmaTransferHoareTripleStack\ φ\ ψ\ f\ g\ p\ (hoareTripleStackGen\ ==>stg₁\ <==stg₁)\ .==>stg\ time\ msg₁\ s\ x}\<%
\\
\>[0]\AgdaComment{\ \ \ \ \ \ \ \ =\ transfer\ (liftPred2Maybe\ (ψ\ time\ msg₁))\ (p\ time\ msg₁\ s)\ (==>stg₁\ time\ msg₁\ s\ x)}\<%
\\
\>[0]\AgdaComment{lemmaTransferHoareTripleStack\ φ\ ψ\ f\ g\ p\ (hoareTripleStackGen\ ==>stg₁\ <==stg₁)\ .<==stg\ time\ msg₁\ s\ x}\<%
\\
\>[0]\AgdaComment{\ \ \ \ \ \ \ \ \ =\ <==stg₁\ time\ msg₁\ s\ (transfer\ (liftPred2Maybe\ (ψ\ time\ msg₁))\ (sym\ (p\ time\ msg₁\ s))\ x)}\<%
\\
\>[0]\AgdaComment{-\}}\<%
\\
%
\\[\AgdaEmptyExtraSkip]%
%
\\[\AgdaEmptyExtraSkip]%
%
\\[\AgdaEmptyExtraSkip]%
%
\\[\AgdaEmptyExtraSkip]%
%
\\[\AgdaEmptyExtraSkip]%
%
\\[\AgdaEmptyExtraSkip]%
%
\\[\AgdaEmptyExtraSkip]%
\>[0]\AgdaFunction{hoareTripleNonActiveIfStackIgnored}\AgdaSpace{}%
\AgdaSymbol{:}\<%
\\
\>[0][@{}l@{\AgdaIndent{0}}]%
\>[5]\AgdaSymbol{(}\AgdaBound{ifStack₁}\AgdaSpace{}%
\AgdaSymbol{:}\AgdaSpace{}%
\AgdaFunction{IfStack}\AgdaSymbol{)}\<%
\\
%
\>[5]\AgdaSymbol{(}\AgdaBound{nonactive}\AgdaSpace{}%
\AgdaSymbol{:}\AgdaSpace{}%
\AgdaFunction{IsNonActiveIfStack}\AgdaSpace{}%
\AgdaBound{ifStack₁}\AgdaSymbol{)}\<%
\\
%
\>[5]\AgdaSymbol{(}\AgdaBound{instr}\AgdaSpace{}%
\AgdaSymbol{:}\AgdaSpace{}%
\AgdaFunction{BitcoinScript}\AgdaSymbol{)}\<%
\\
%
\>[5]\AgdaSymbol{(}\AgdaBound{nonIf}\AgdaSpace{}%
\AgdaSymbol{:}\AgdaSpace{}%
\AgdaFunction{NonIfScript}\AgdaSpace{}%
\AgdaBound{instr}\AgdaSymbol{)}\<%
\\
%
\>[5]\AgdaSymbol{(}\AgdaBound{φ}\AgdaSpace{}%
\AgdaSymbol{:}\AgdaSpace{}%
\AgdaFunction{StackPredicate}\AgdaSymbol{)}\<%
\\
%
\>[5]\AgdaSymbol{→}\AgdaSpace{}%
\AgdaOperator{\AgdaRecord{<}}\AgdaSpace{}%
\AgdaFunction{liftStackPred2Pred}\AgdaSpace{}%
\AgdaBound{φ}\AgdaSpace{}%
\AgdaBound{ifStack₁}%
\>[40]\AgdaOperator{\AgdaRecord{>ⁱᶠᶠ}}\AgdaSpace{}%
\AgdaBound{instr}%
\>[52]\AgdaOperator{\AgdaRecord{<}}\AgdaSpace{}%
\AgdaFunction{liftStackPred2Pred}\AgdaSpace{}%
\AgdaBound{φ}\AgdaSpace{}%
\AgdaBound{ifStack₁}%
\>[85]\AgdaOperator{\AgdaRecord{>}}\<%
\\
\>[0]\AgdaFunction{hoareTripleNonActiveIfStackIgnored}\AgdaSpace{}%
\AgdaBound{ifStack₁}\AgdaSpace{}%
\AgdaBound{nonactive}\AgdaSpace{}%
\AgdaBound{instr}\AgdaSpace{}%
\AgdaBound{nonIf}\AgdaSpace{}%
\AgdaBound{φ}\<%
\\
\>[0][@{}l@{\AgdaIndent{0}}]%
\>[3]\AgdaSymbol{=}%
\>[6]\AgdaFunction{lemmaGenericHoareTripleImpliesHoareTriple''}\AgdaSpace{}%
\AgdaBound{instr}\<%
\\
%
\>[3]\AgdaSymbol{(}\AgdaFunction{liftStackPred2Pred}\AgdaSpace{}%
\AgdaBound{φ}\AgdaSpace{}%
\AgdaBound{ifStack₁}\AgdaSymbol{)}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaFunction{liftStackPred2Pred}\AgdaSpace{}%
\AgdaBound{φ}\AgdaSpace{}%
\AgdaBound{ifStack₁}\AgdaSymbol{)}\<%
\\
%
\>[3]\AgdaSymbol{(}\AgdaFunction{lemmaNonIfInstrGenericCondImpliesTripleaux'}\AgdaSpace{}%
\AgdaBound{instr}\AgdaSpace{}%
\AgdaBound{nonIf}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaFunction{liftStackPred2Pred}\AgdaSpace{}%
\AgdaBound{φ}\AgdaSpace{}%
\AgdaBound{ifStack₁}\AgdaSymbol{)}\<%
\\
%
\>[3]\AgdaSymbol{(}\AgdaFunction{liftStackPred2Pred}\AgdaSpace{}%
\AgdaBound{φ}\AgdaSpace{}%
\AgdaBound{ifStack₁}\AgdaSymbol{)}\<%
\\
%
\>[3]\AgdaSymbol{(}\AgdaFunction{lemmaHoareTripleStackPartToHoareTripleNonActiveGeneric}\AgdaSpace{}%
\AgdaBound{ifStack₁}\AgdaSpace{}%
\AgdaBound{nonactive}\AgdaSpace{}%
\AgdaBound{φ}\AgdaSpace{}%
\AgdaOperator{\AgdaFunction{⟦}}\AgdaSpace{}%
\AgdaBound{instr}\AgdaSpace{}%
\AgdaOperator{\AgdaFunction{⟧stack}}\AgdaSymbol{))}\<%
\\
%
\\[\AgdaEmptyExtraSkip]%
%
\\[\AgdaEmptyExtraSkip]%
%
\\[\AgdaEmptyExtraSkip]%
%
\\[\AgdaEmptyExtraSkip]%
\>[0]\AgdaComment{\{-}\<%
\\
\>[0]\AgdaComment{hoareTripleNonActiveIfStackIgnored\ :}\<%
\\
\>[0]\AgdaComment{\ \ \ \ \ (ifStack₁\ :\ IfStack)}\<%
\\
\>[0]\AgdaComment{\ \ \ \ \ (nonactive\ :\ IsNonActiveIfStack\ ifStack₁)}\<%
\\
\>[0]\AgdaComment{\ \ \ \ \ (prog\ :\ BitcoinScript)}\<%
\\
\>[0]\AgdaComment{\ \ \ \ \ (nonIf\ :\ NonIfScript\ prog)}\<%
\\
\>[0]\AgdaComment{\ \ \ \ \ (φ\ :\ StackPredicate)}\<%
\\
\>[0]\AgdaComment{\ \ \ \ \ →\ <\ liftStackPred2Pred\ φ\ ifStack₁\ \ >iff\ prog\ <\ liftStackPred2Pred\ φ\ ifStack₁\ \ \ >}\<%
\\
\>[0]\AgdaComment{hoarTripleNonActiveIfStackIgnored\ =\ lemmaNonActiveIfStackHoareTriple'\ -\}}\<%
\\
\>[0]\AgdaComment{\{-\ \ \ *********\ \ \ \ hoarTripleNonActiveIfStackIgnored\ \ \ \ should\ be\ deleted\ and\ replaced\ by}\<%
\\
\>[0]\AgdaComment{\ \ \ \ \ lemmaNonActiveIfStackHoareTriple'}\<%
\\
\>[0]\AgdaComment{\ \ \ \ \ \ (possibly\ you\ rename\ lemmaNonActiveIfStackHoareTriple'\ into\ something\ more\ memorable}\<%
\\
\>[0]\<%
\\
\>[0]\AgdaComment{call\ it\ hoareTripleNonActiveIfStackIgnored}\<%
\\
\>[0]\AgdaComment{-\}}\<%
\\
%
\\[\AgdaEmptyExtraSkip]%
\>[0]\AgdaComment{\{-}\<%
\\
\>[0]\AgdaComment{hoarTripleNonActiveIfStackIgnored\ ifStack₁\ nonactive\ []\ nonIf\ φ\ =\ \{!!\}\ --\ use\ \ \ \AgdaUnderscore{}∎p}\<%
\\
\>[0]\AgdaComment{hoarTripleNonActiveIfStackIgnored\ ifStack₁\ nonactive\ (x\ ∷\ [])\ nonIf\ φ\ =\ \{!!\}\ --\ 1\ element\ case}\<%
\\
\>[0]\AgdaComment{hoarTripleNonActiveIfStackIgnored\ ifStack₁\ nonactive\ (x\ ∷\ x₁\ ∷\ prog)\ nonIf\ φ\ =\ \{!!\}\ \ --lemmaNonActiveIfStackHoareTriple'\ ifStack₁\ nonactive\ prog\ nonIf\ φ}\<%
\\
\>[0]\<%
\\
\>[0]\AgdaComment{test\ =\ lemmaNonActiveIfStackHoareTriple'}\<%
\\
\>[0]\AgdaComment{-\}}\<%
\\
%
\\[\AgdaEmptyExtraSkip]%
\>[0]\AgdaComment{--\ Idea\ of\ proof:\ it\ is\ similar\ to}\<%
\\
\>[0]\AgdaComment{--\ lemmaP2PKHwithNonActiveIfStack}\<%
\\
\>[0]\AgdaComment{--\ in\ verificationP2PKHwithIfStackindexedPart4.agda}\<%
\\
\>[0]\AgdaComment{--\ Make\ use\ of\ lemmaNonActiveIfStackHoareTriple}\<%
\\
\>[0]\AgdaComment{--\ which\ proves\ the\ theorem\ for\ single\ instructions}\<%
\end{code}
} % END AgdaHide


==> macrosAgdaAdaption.tex <==
% Space inserted after tokens.
%\newcommand{\AgdaSpace}{ }
\newcommand{\AgdaOption}[1]{\AgdaNoSpaceMath{\AgdaCommentFontStyle{\textcolor{AgdaOption}{#1}}}}
\newcommand{\agdaField}{\AgdaKeyword{field}}

\usepackage[T1]{fontenc}
\RequirePackage[utf8]{inputenc}
\usepackage{stmaryrd}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%                                                      %%%
%%% Commands for dealing with lagda files                %%%
%%%                                                      %%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

\DeclareUnicodeCharacter{1D4D4}{\ensuremath{\mathcal{E}}}
\DeclareUnicodeCharacter{1D4C1}{\ensuremath{\ell}}
\DeclareUnicodeCharacter{01D49}{\ensuremath{{}^{\mathsf{e}}}} %ᵉ
\DeclareUnicodeCharacter{02E2}{\ensuremath{{}^{\mathsf{s}}}}  %ˢ
\DeclareUnicodeCharacter{1D9C}{\ensuremath{{}^{\mathsf{c}}}}
\DeclareUnicodeCharacter{1D52}{\ensuremath{{}^{\mathrm{o}}}}
\DeclareUnicodeCharacter{1D56}{\ensuremath{{}^{\mathrm{p}}}} %ᵖ
\DeclareUnicodeCharacter{228E}{\ensuremath{\uplus}}
\DeclareUnicodeCharacter{1D62}{\ensuremath{{}_{\mathsf{i}}}}
\DeclareUnicodeCharacter{209B}{\ensuremath{{}_{\mathsf{s}}}}
\DeclareUnicodeCharacter{2092}{\ensuremath{{}_{\mathsf{o}}}}
\DeclareUnicodeCharacter{2099}{\ensuremath{{}_{\mathsf{n}}}}
\DeclareUnicodeCharacter{2237}{\ensuremath{::}}
\DeclareUnicodeCharacter{25B9}{\ensuremath{\vartriangleright}}
\DeclareUnicodeCharacter{2115}{\ensuremath{\mathbb{N}}}
\DeclareUnicodeCharacter{2264}{\ensuremath{\leq}}
\DeclareUnicodeCharacter{2227}{\ensuremath{\land}}
\DeclareUnicodeCharacter{2228}{\ensuremath{\lor}}
\DeclareUnicodeCharacter{27E6}{\ensuremath{{}[[}}
\DeclareUnicodeCharacter{27E7}{\ensuremath{{}]]}}
\DeclareUnicodeCharacter{2081}{\ensuremath{{}_{\mathsf{1}}}}
\DeclareUnicodeCharacter{2261}{\ensuremath{\equiv}}
\DeclareUnicodeCharacter{220E}{\ensuremath{\sqbullet}}
\DeclareUnicodeCharacter{03BB}{\ensuremath{\lambda}} 
\DeclareUnicodeCharacter{2082}{\ensuremath{{}_{\mathsf{2}}}}
\DeclareUnicodeCharacter{27E8}{\textlangle}
\DeclareUnicodeCharacter{27E9}{\textrangle}
%\DeclareUnicodeCharacter{27E8}{\ensuremath{\langle}}
%\DeclareUnicodeCharacter{27E9}{\ensuremath{\rangle}}
\DeclareUnicodeCharacter{207A}{\ensuremath{{}^+}}
\DeclareUnicodeCharacter{22A5}{\ensuremath{\bot}}
\DeclareUnicodeCharacter{2080}{\ensuremath{{}_0}}
\DeclareUnicodeCharacter{2083}{\ensuremath{{}_3}}
\DeclareUnicodeCharacter{2084}{\ensuremath{{}_4}}
\DeclareUnicodeCharacter{2085}{\ensuremath{{}_5}}
\DeclareUnicodeCharacter{03C6}{\ensuremath{\phi}}
\DeclareUnicodeCharacter{1D47}{\ensuremath{{}^{\mathsf{b}}}}
\DeclareUnicodeCharacter{27E6}{\ensuremath{\llbracket}}
\DeclareUnicodeCharacter{27E7}{\ensuremath{\rrbracket}}
\DeclareUnicodeCharacter{209B}{\ensuremath{_{\mathsf{s}}}}
\DeclareUnicodeCharacter{2071}{\ensuremath{^{\mathsf{i}}}}
\DeclareUnicodeCharacter{1DA0}{\ensuremath{^{\mathsf{f}}}}
%\DeclareUnicodeCharacter{2071}{\ensuremath{{}^i}}
%\DeclareUnicodeCharacter{1DA0}{\ensuremath{{}^f}}

